The Black-Box Simulation Barrier Persists in a Fully Quantum World

Zero-Knowledge (ZK) protocols have been intensely studied due to their fundamental importance and versatility. However, quantum information's inherent differences significantly alter the landscape, necessitating a re-examination of ZK designs. A crucial aspect is round complexity, linked to $\textit{simulation}$, which forms the foundation of ZK definition and security proofs. In the $\textit{post-quantum}$ setting, where honest parties and channels are classical but adversaries quantum, Chia et al. [FOCS'21] showed constant-round $\textit{black-box-simulatable}$ ZK arguments (BBZK) for $\mathbf{NP}$ are impossible unless $\mathbf{NP} \subseteq \mathbf{BQP}$. But this problem remains open when all parties and communication are quantum. Indeed, this problem interests the broader theory of quantum computing. Investigating how quantum power alters tasks like the $\textit{unconditional}$ security of QKD and incorporating OT in MiniQCrypt has been crucial. Moreover, quantum communication has enabled round compression for commitments and interactive arguments. Along this line, understanding if quantum computing could fundamentally change ZK protocols is vital. We resolved this problem by proving that only languages in $\mathbf{BQP}$ admit constant-round $\textit{fully-quantum}$ BBZK. This result holds significant implications. Firstly, it illuminates the nature of quantum zero-knowledge and provides valuable insights for designing future protocols in the quantum realm. Secondly, it relates ZK round complexity with the intriguing problem of $\mathbf{BQP}$ vs $\mathbf{QMA}$, which is out of the reach of previous analogue impossibility results in the classical or post-quantum setting. Lastly, it justifies the need for the $\textit{non-black-box}$ simulation techniques or the relaxed security notions employed in existing constant-round fully-quantum BBZK protocols.

==> notes.tex <==
I'm using a package called FiXme to help us track comments better. It is simple---just use the following macros when you want to comment. Then, a record will be automatically added to the {\bf List of Corrections} in the first page.

\jiahui{Testing short commenting macro for Jiahui. This macro only allows in-line comments and equations. It does not allow you to change line. $x = y$.}

\begin{jiahuienv}{Title of comments}
Testing long commenting macros for Jiahui. 

This allows you to use any form of comments. E.g.,
$$E = MC^2.$$

\begin{itemize}
\item test
\item
 test 2
\end{itemize}
\end{jiahuienv}

\naihui{Testing short commenting macro for Nai-Hui. This macro only allows in-line comments and equations. It does not allow you to change line}

\begin{naihuienv}{Put the summary text here..}
Testing long commenting macros for Nai-Hui. 

This allows you to use any form of comments. E.g.,
$$E = MC^2.$$
\end{naihuienv}

\kaimin{Testing short commenting macro for Kai-Min. This macro only allows in-line comments and equations. It does not allow you to change line}
\begin{kaiminenv}{Put the summary text here..}
Testing long commenting macros for Kai-Min. 

This allows you to use any form of comments. E.g.,
$$E = MC^2.$$
\end{kaiminenv}


\section{Notes}

\begin{xiaoenv}{}
Things to discuss
\begin{itemize}
\item
Extension to expected QPT simulation?
\item
Extension to 3-round $\epsilon$-ZK?
\item
Do we already know impossibility of 3-round fully quantum ZK? If not, our warm-up case is a new result as well.
\item
The concurrent ZK results Jiahui previously worked on?
\end{itemize}
\end{xiaoenv}


Define black-box ZK in the {\em non-programmable} entanglement model. We will refer to it as $\NPEBBZK$ argument. \xiao{We gonna require by definition that $\NPEBBZK$ argument can only use classical channel.}

\xiao{Also, we when define $\BBZK$ (in the plain model), emphasize that we allow honest parties to be quantum machines that communicate over quantum channels. This is in contrast to the notion of post-quantum ZK where honest parties and their communication channel are totally classical.}



\begin{theorem}\label{thm:BBZK-to-NPEBBZK}
For all language $\Lang \in \QMA$, if there exists a $k$-round $\BBZK$ argument for $\Lang $, then there exits a $k$-round $\NPEBBZK$ argument for $\Lang$.
\end{theorem}       
\begin{remark}
It is worth reiterating that our definition of $\BBZK$ allows (both honest and malicious) parties to be QPT quantum algorithms and to communicate over quantum channel; In contrast, our definition of $\NPEBBZK$ stipulates that the parties can only use classical channel (while they can still perform {\em local} QPT computation). Also notice that since $\NP\subseteq \QMA$, \Cref{thm:BBZK-to-NPEBBZK} holds for all $\Lang \in\NP$ as well.
\end{remark}
\begin{proof}[(Proof Sketch)]
given a $k$-round $\NPEBBZK$ argument $\Prot_\textsc{qc}$ over quantum channel, we construct a $k$-round $\NPEBBZK$ argument $\Prot_\textsc{npe}$. The idea is to use teleportation to de-quantize the communication.

Completeness is straightforward. The reduction for soundness is also easy.

To prove the BBZK property of $\Prot_\textsc{npe}$, we start with an arbitrary QPT adversary $V^*(\rho_\secpar)$ for $\Prot_\textsc{npe}$. We first move to a hybrid game where we construct a new adversary $\tilde{V}^*(\rho_\secpar)$ talking to the honest prover $P'$ of $\Prot_\textsc{qc}$ over quantum channel. This $\tilde{V}^*(\rho_\secpar)$ enjoys the following properties:
\begin{itemize}
 \item
 $\tilde{V}^*(\rho_\secpar)$ can be constructed making black-box use of $V^*(\rho_\secpar)$;
 \item
 The final output of $\tilde{V}^*(\rho_\secpar)$ from the execution $\langle P'(x,w),\tilde{V}^*(\rho_\secpar)\rangle_\textsc{qc}$ is identically distributed as the output of $V^*(\rho_\secpar)$ from the execution $\langle P(x,w),V^*(\rho_\secpar)\rangle_\textsc{cc}$.
 \end{itemize} 
The above two properties, together with our assumption that there exists a black-box ZK simulator for $\Prot_\textsc{qc}$, implies a black-box ZK simulator for $\Prot_\textsc{npe}$. 

Now we only need to establish the existence of such a $\tilde{V}^*(\rho_\secpar)$. This is straightforward---$\tilde{V}^*(\rho_\secpar)$ just prepares EPR pairs and relays the messages between the external $P'(x,w)$ and the oracle $V^*(\rho_\secpar)$ by simulating the teleportation channel.

\end{proof}

\begin{theorem}\label{thm:impossibility-NPEBBZK}
There do not exist constant-round $\NPEBBZK$ arguments for $\NP$ (resp.\ $\QMA$) unless
$\NP \subseteq \BQP$ (resp.\ $\QMA \subseteq \BQP$).
\end{theorem}

\begin{proof}[(Proof Sketch)]
This is the hard step. 
The basic idea is to generalize the \cite{FOCS:CCLY21} technique to the $\NPEBBZK$ arguments. Two places require extra caution:
\begin{enumerate}
\item
\xiao{It seems to me that we need to modify the format measure-and-reprogram lemma \cite{C:DFMS19,C:DonFehMaj20,EC:YamZha21} to compensate for the intrinsic randomized behavior of honest QPT verifiers. (In particular, we cannot define the set $\msf{Acc}(x,r)$ as in \cite{FOCS:CCLY21}).}
\item
\xiao{\cite{FOCS:CCLY21} only claims the impossibility results for $\NP$. Need to check that it extends to $\QMA$ as well. (This is a benefit particularly of our model---\cite{FOCS:CCLY21} is in the post-quantum setting where the honest parties are totally classical. Thus, they cannot say anything about $\QMA$.)}
\end{enumerate}
\end{proof}

\begin{theorem}\label{thm:impossibility-BBZK}
There do not exist constant-round $\BBZK$ arguments for $\NP$ (resp.\ $\QMA$) unless
$\NP \subseteq \BQP$ (resp.\ $\QMA \subseteq \BQP$).
\end{theorem}
\begin{proof}
This theorem follows directly from \Cref{thm:BBZK-to-NPEBBZK,thm:impossibility-NPEBBZK}.

\end{proof}


==> sections/2-round-QCCC-xiao-new-backup.tex <==

\section{Warm Up: Three-Round BBZK in the CPM Model (Part 1/2)}


\xiao{I change the model to a classical-prover-message (CPM) model. This is to reflect the final soundness reduction, where we have to receive unmeasured Verifier's messages from the external verifier. Only in this way can we ensure that the view of the simulator is identical to that in our dummy up-and-down game.}


In this section, we show as a warm-up example that three-round ZK in the CPM model is impossible. This proof already illustrate the main ideas behind our general impossibility for the constant-round case. \xiao{Note that even such a result is not known yet.}






\subsection{The Model}

\subsubsection{Protocol Structure}
 We consider a three-round protocol where the prover $\Prover$ and verifier $\Verifier$ takes a statement $x \in \Lang$ and the security parameter $\secpar$ as the comment input. $\Prover$ additional takes a witness $w \in \Relation_\Lang(x)$ as the private input. $\Prover$ sends the first message $p_1$; $\Verifier$ responds with the second message $v_1$; then, $\Prover$ sends the final message $p_2$. W.l.o.g., we assume that all these massages are of the same length $\ell(\secpar)$, which is a polynomial in $\secpar$. Since we are in the CMP model, the messages $(p_1, p_2)$ are all classical, but the message $v_2$ could be quantum. 

 \xiao{from now one, we append one more message $v_2$ (possibly quantum) at the end of the execution. This message is just that the honest verifier let $P$ know if the execution is accepted or not. Not that this can only make our impossibility stronger! So, the protocol now has four rounds, i.e., $(p_1, v_1, p_2, v_2)$. And we will keep calling it four-round CPM BBZK.}

\para{Honest Verifier}  \xiao{need to explain to specify the model.}





\subsubsection{Generic Malicious Verifier}

\begin{xiaoenv}{Generic Malicious Verifier}
A malicious verifier $\tilde{\Verifier}$ could differ from the honest $\Verifier$ in the following way:
\begin{itemize}
\item
Its work space $\reg{w}$ could be larger than $\Verifier$;
\item
It make take an auxiliary input $\ket{\rho}$ of polynomial size, stored in some part in $\reg{w}$ at the beginning of the protocol;
\item
It may use a different unitary $V^*$ (can be implemented by poly-size quantum circuits) from the honest $\Verifier$.
\end{itemize}
Other than the above, it behaves in the same way as the honest $\Verifier$.
\end{xiaoenv}

 


\subsubsection{ZK Simulator}
 We now describe formally how the simulator $\Sim$ interacts with a generic malicious verifier $\tilde{\Verifier}$. Once again, there are multiple ways to do so and we choose the following one without loss of generality, which is particularly suitable for our proof of impossibility.

Note that we focus on black-box simulation. Thus, $\Sim$ can only query $\tilde{\Verifier}$ via its unitary $\tilde{V}$ and its inverse $\tilde{V}^\dagger$, but does not get to see the internal register $\reg{w}$ of $\tilde{\Verifier}$. 


Also, recall that $\reg{m}$ is used to exchange messages, and as explained above, it is always measured when a party is about to send message in the real execution (as we are in the LOCC setting). However, it is worth noticing that for simulation, $\reg{m}$ is considered as being held by $\Sim$, who could choose {\em not} to measure it. 

In more detail, a black-box simulator $\Sim$ is defined by a ``local'' unitary $S$. It is granted oracle access to $\tilde{V}$ and $\tilde{V}^\dagger$. It makes use of the following registers
\begin{itemize}
\item
Register $\reg{m}$ to exchange messages with the malicious verifier $\tilde{V}$;
\item
Register $\reg{s}$ which is her ``local'' work space;
\item
A query register $\reg{u}$ in a $2$-dimension Hilbert space spanned by the basis $\Set{ \ket{\downarrow}_{\reg{u}}, \ket{\uparrow}_{\reg{u}}}$ (explained shortly).
\end{itemize}
$\Sim$ behavior is nothing but iterations of the following three steps:
\begin{enumerate}
\item
Apply the local operator $S$ on registers $\reg{m}$, $\reg{u}$, and $\reg{s}$;
\item
Measure the $\reg{u}$ register to learn the type of the next query (see the next bullet);
\item
Make the oracle query according to the measurement outcome from the last step---if the measurement outcome is $\ket{\uparrow}$, it query the $\tilde{V}$ oracle on $\reg{m}$; otherwise (i.e., the measurement outcome is $\ket{\uparrow}$), it query the $\tilde{V}^\dagger$ oracle on $\reg{m}$.
\end{enumerate}
$\Sim$ keeps repeating the above three steps until she decides to stop. At that moment, the internal state of $\tilde{V}$ is defined to be the simulation output.



% \para{Formal Description of $\Sim^{\tilde{V}(x, \ket{\rho})}$.} With the above intuitive explanation, we proceed to present the formal description of the interaction between $\Sim$ and a malicious verifier $\tilde{V}(x, \ket{\rho})$. 

% The execution starts by initializing the following state:
% \begin{equation}\label{2-LOCC:S:inital:expr}
% \ket{\eta_0} \coloneqq \ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{\phi}_{\reg{o}} \ket{\downarrow_1}_{\reg{u_1}} \ldots \ket{\downarrow_1}_{\reg{u_q}} \ket{\rho}_{\reg{s}},
% \end{equation}





% \para{$\Sim$'s Behavior.} 
% \begin{xiaoenv}{}
% Start with the intermediate measurement. And then say that all the measurements on $\reg{u_j}$'s can be deferred, because a consequence of deferred measurement principle is:
% \begin{quote}
% {\em If after a measurement a qubit is used as a control qubit only, then the
% measurement can be deferred.}
% \end{quote}
% \end{xiaoenv}
% The behavior of a  $q$-query simulator can be described as follows. For $j \in [q]$, 
% \begin{itemize}
% \item
% Apply the local unitary $S_j$. $S_j$ is a unitary that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$; Intuitively, it represents the local operation $\Sim$ performs between two oracle queries. In particular, it computes and stores the type of the $j$-th query in register $\reg{u_j}$, possibly in superposition.
% \item
% Measure $\reg{u_j}$;
% \item
% Make the $j$-th oracle query according to the measurement outcome from the last step. Formally, we define this step as a unitary$O_{j}$ that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$ and $\reg{o}$. We present the formal definition of $O_{j}$ in \Cref{figbox:LOCC:3ZK:oracle}.
% \end{itemize}


% \begin{FigureBox}[label={figbox:LOCC:3ZK:oracle}]{Description of Unitary $O_j$}
% Each $O_j$ can be understood as unitary controlled on register $\reg{u_j}$. Formally, for each $j \in [q]$, $O_j$ is defined as follows 
% \begin{itemize}
% \item
% If $\reg{u_j}$ is of the form $\ket{\downarrow_1}_{\reg{u_j}}$, it applies $\tilde{U}_1$ on $\reg{m_1}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\uparrow_1}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_1$ on $\reg{m_1}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\downarrow_2}_{\reg{u_j}}$, it applies $\tilde{U}_2$ on $\reg{m_2}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\uparrow_2}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_2$ on $\reg{m_2}$ and $\reg{o}$.
% \end{itemize}
% \end{FigureBox}

% % is defined by a sequence of $q$ unitary operators $\Set{S_1,  \ldots, S_q}$. It proceeds as follows:
% % \begin{itemize}
% % \item
% % {\bf (First $q$ queries)} For $j\in [q]$, $\Sim$ repeats the following steps:
% % \begin{itemize}
% %  \item
% %  $\Sim$ first applies the ``local'' unitary $S_j$, which operates non-trivially on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$. 
% %  \item
% %  Then, controlled on the query type (possibly in superposition) stored in $\reg{u_j}$, the corresponding unitary is applied according to the rule described in \Cref{figbox:LOCC:3ZK:oracle}.
% %  \end{itemize} 

% % \item
% % {\bf (Final output.)} We denote by $\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho)$ the above execution; We denote by $\OUT(\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho))$ the output of $\tilde{\Verifier}$, i.e., final state in $\reg{out}$ tracing out all other registers after the execution
% % \end{itemize}
% \xiao{add a remark explaining two things: (1) $S_{j}$ only need to work on $\reg{u}_j$ and does not touch other $\reg{u}$ registers; (2) There's no need to add $S_{q+1}$ for $\Sim$'s post-processing, as the output will anyway trace $\Sim$'s registers out.}


% \subpara{$\Sim$ with Deferred Measurements.} Recall that a consequence of the deferred measurement principle is that {\em If after a measurement a qubit is used as a control qubit only, then the measurement can be deferred.} Also, observe in the above description of $\Sim$'s behavior that each $\reg{u_j}$ register is used {\em only} as a controlled register to determine the type of $O_j$. Thus, by the deferred measurement principle, we can equivalently describe $\Sim$ as the following two steps (assuming the starting state is $\ket{\eta_0}$):
% \begin{enumerate}
% \item
% Compute $\ket{\eta_q} \coloneqq O_q S_q O_{q-1} S_{q-1} \cdots O_1 S_1\cdot \ket{\eta_0}$.
% \item
% Measure registers $\reg{u_1},\ldots, \reg{u_q}$.
% \end{enumerate}
% From now on, we will use this deferred-measurement description of the simulator $\Sim$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comment some old materials
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% At a high-level, $\Sim$ can run $\tilde{\mathcal{V}}$ as a real prover, i.e., sending a message to $\tilde{\Verifier}$ and expecting $\tilde{\Verifier}$'s response (dubbed as ``down-queries''), or rewind $\tilde{\Verifier}$ (dubbed ``up-queries''). In the following, we formally define $\Sim$'s behavior. We also show in \Cref{figure:Sim-query:3-round} an exemplary execution of $\Sim$ where she makes 17 queries in total. We find it helpful to trace this concrete example while trying to understand the behavior of $\Sim$.
% \begin{figure}[!thb]
% \centering{
%     \fbox{
%          \includegraphics[width=0.5\textwidth]{figures/Three-round-real.jpg}
%     }         
% }
% \caption{An exemplary Query Pattern of $\Sim$}
% \label{figure:Sim-query:3-round}
% \end{figure}

% \subpara{Initialize $p_1$:} $\Sim$ starts by preparing a state in register $\reg{m_1}$ as her first message $p_1$. Formally, $\Sim$ applies a ``local'' unitary $S_0$ that works non-trivially on register $\reg{m_1}$ and $\reg{s}$. This yields a quantum state $p_1$ in $\reg{m_1}$ together with some residual internal state of $\Sim$ in $\reg{s}$. 


% \subpara{Obtain $v_1$:} $\Sim$ then queries $\tilde{\Verifier}$ to learn the response $v_1$. Formally, $\tilde{V}$ applies the unitary $\tilde{U}_3\tilde{U}_2\tilde{U}_1$ as defined earlier, which yields a state $v_1$ in register $\reg{m_1}$. This step is illustrated as the $\downarrow$ labeled by $\circled{1}$ in \Cref{figure:Sim-query:3-round}, and we say that the execution moves from Layer-1 to Layer-2.\footnote{It is worth noting that although both $p_1$ and $v_1$ are classical strings in the real execution, the simulator $\Sim$ may put a quantum state in $\reg{m_1}$ as her first message, and in that case, $\tilde{V}$'s response $v_1$ may also be a quantum state.} 


% \subpara{Subsequent Queries:} From now on, $\Sim$ can freely ask $\tilde{V}$ to perform $\tilde{U}$ or $\tilde{U}^\dagger$, and may modify the contains of $\reg{m_1}$ and $\reg{m_2}$ in between using her unitaries $S_1$, $S_2$, and $S_3$. Formally, $\Sim$ repeats the following procedure
% \begin{itemize}
% \item
% if the execution reaches Layer-$i$ (for $i \in [3]$), $\Sim$ will first apply the unitary $S_i$, and then measure the single-qubit register $\reg{q}$ \xiao{add this register when explaining $\Sim$'s registers} to decide if she wants to make a $\tilde{U}$ query or a $\tilde{U}^\dagger$ query. Depending on the query made, the execution will either move to Layer-$(i-1)$ (if a $\tilde{U}^\dagger$ query is made) or Layer-$(i+1)$ (if a $\tilde{U}$ query is made). 

% W.l.o.g., we use the following conventions. When the execution is at Layer-1 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\uparrow}$, then $\Sim$ aborts the execution immediately. Intuitively, this is because the execution is already rewound to the very beginning and it does not make sense to rewind it further; we simply view this as a failed simulation. Also, when the execution is at Layer-3 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\downarrow}$, then $\Sim$ terminates and announces the end of the simulation. Intuitively, Layer-3 represents the very end of the protocol and it does not make sense to continue to the next round; we simply view this as $\Sim$'s signal for the end of the simulation.
% \end{itemize}
% This procedure is best understood by tracing the example shown in \Cref{figure:Sim-query:3-round}. Consider the status of the execution right after the arrow $\circled{1}$. $\Sim$ then applies $S_2$ on $\reg{m_1}$ and $\reg{s}$ \xiao{probably on $\reg{m_2}$ as well?}, and measures $\reg{d}$. The situation shown in  \Cref{figure:Sim-query:3-round} corresponds to $\Sim$ decides to make a $\tilde{U}^\dagger$-query next (represented by arrow $\circled{2}$), which brings the execution back to Layer-1. $\Sim$ then applies $S_1$ on $\reg{m_1}$ and $\reg{s}$, and measures $\reg{d}$. By the assumption made above, $\Sim$ will make a $\tilde{U}$-query next, which brings the execution to Layer-2 (represented by arrow $\circled{3}$). 

% Another set of queries that deserve a closer look is from arrow $\circled{11}$ to arrow $\circled{12}$. They represent the following steps: Right after the $\tilde{U}$-query labeled by $\circled{10}$, $\Sim$ applies $S_3$ on $\reg{m_2}$ and $\reg{s}$, measures $\reg{q}$, and decides to make the  $\tilde{U}^\dagger$-query labeled by $\circled{11}$. This brings the execution to Layer-2. Then, $\Sim$ further rewinds the execution back to Layer-1 and ``jumps'' between Layer-1 and Layer-2 twice (as represented by arrow $\circled{12}$ to arrow $\circled{15}$). After that, $\Sim$ decides to go to Layer-3 as represented by arrow $\circled{16}$, which is the last query made by $\Sim$. That is, after applying $\circled{16}$, the measurement of $\reg{q}$ returns $\ket{\downarrow}$, indicating the end of the execution as we explained above. 


\subsection{Theorem Statement and Proof Outline}

\xiao{to do... As the title of the subsection indicates..}


\UpdateLine







\subsection{A Particular Malicious Verifier}
\label{sec:particular-mal-V}




\xiao{may need to explain the high-level picture: why are we defining $\tilde{V}$?} Similar as \cite{FOCS:CCLY21}, we first show the impossibility result with an inefficient $\tilde{V}$. The inefficiency is only due to a random function $H$ hard-wired in $\tilde{V}$. Jumping ahead, we will make $\tilde{V}$ efficient later (\xiao{Cref to sec}) by replacing $H$ with a $q$-wise independent hash.

\subsubsection{$\tilde{\Verifier}$'s registers}
\label{sec:LOCC-3ZK:Vtil:registers} 
$\tilde{\Verifier}$ starts by initializing the following registers (see \Cref{figure:2-LOCC-V:registers} for an explanation \xiao{add a figure explaining the meaning fo the registers.}):
\begin{equation}\label[Expression]{2-LOCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{\vb{0}}_{\reg{p_1}}\ket{\vb{0}}_{\reg{v_1}}\ket{\vb{0}}_{\reg{p_2}}\ket{\vb{0}}_{\reg{v_2}} \ket{\vb{0}}_{\reg{m}} \ket{\bot}_{\reg{t_1}}\ket{\bot}_{\reg{t_2}} \ket{0}_{\reg{d}} \ket{\vb{0}}_\reg{w} \ket{H}_{\reg{aux}} 
\end{equation}








% In the impossibility result, we construct a BQP algorithm that runs both the simulator $\simulator$ and verifier $V$.
% Our entire purified view therefore consists of all above registers $\reg{ins, a,b,m,aux,w,adv}$. 


\subsubsection{$\tilde{V}$'s Unitary.} 
\label{sec:LOCC-3ZK:Vtil:unitaries} 




\begin{xiaoenv}{Define the Counter}
Define the Counter

Both $\reg{gc}$ and $\reg{lc}$ registers are initialized to $0$. We set $C = 2^\secpar$,\footnote{We note that it suffices to set $C$ to any super-polynomial function on $\secpar$. We choose $2^\secpar$ only for concreteness.} and define the unitary $U_{gc}$ as the following mapping
 $$U_{gc} : 	\ket{i}_{\reg{gc}} \mapsto \ket{i+1 \mod C}_{\reg{gc}}.$$

 We also define the unitary to increase the local counter $U_{lc}$ as follows:
 $$U_{lc} : 	\ket{i}_{\reg{lc}} \mapsto \ket{i+1 \mod 3}_{\reg{lc}}.$$
 Note that modulus 3 is good enough for us, because we will show later that the local counter will never reach 3.
\end{xiaoenv}



We now desribe $\tilde{\Verifier}$'s unitary $\tilde{V}$. 

\begin{AlgorithmBox}[label={LOCC-3ZK:V:unitary}]{Unitary \textnormal{$\tilde{V}$} for the Malicious Verifier \textnormal{$\tilde{\Verifier}$}}
On each query, it first applies $U_{gc}$ to increase the global counter by 1. Then, it checks if the global counter value $i$ satisfies $i \in [2]$. If not, do nothing (technically, this can be understood as applying the identity operation). Otherwise, it compares $i$ with the local counter value $j$ and behaves accordingly (note that in the following we have $i \in [2]$):

\begin{description}
\item[Case $(i = j+1)$:] apply $D_i C_i B_i A_i$, where these unitaries are defined as follows:
\begin{itemize}	
\item 
{\bf $A_i$: swap $\reg{p_i}$ and $\reg{m}$.} This unitary swaps the contents of $\reg{p_i}$ and $\reg{m}$.

\item 
{\bf $B_i$: apply $V$'s unitary.}
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then apply $\sum_{p_i} \ketbra{p_i} \tensor V_{p_i}$, which is the honest $\Verifier$'s unitary to generate $v_i$ from $p_i$.
\item
If $H(p_1, \ldots, p_i) = 0$, then do nothing; 
\end{itemize}


\item 
{\bf $C_i$: deliver $v_i$.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_i}$.
\item
If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_i}$.
\end{itemize}


\item 
{\bf $D_i$: increase local counter.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
\item
If $H(p_1, \ldots, p_i) = 0$, then do nothing.
\end{itemize}
\end{itemize}

\item[Case ($i \ne j + 1$):] apply $C'_i A_i$, where $A_i$ is as defined above and $C'_i$ is defined as
\begin{itemize}
\item
{\bf $C'_i$: swap $\reg{t_i}$ and $\reg{m}$.} This unitary swaps the contents of $\reg{t_i}$ and $\reg{m}$.
\end{itemize}
\end{description}
\end{AlgorithmBox}



% \para{Compare Counters.} On each query, $\tilde{\Verifier}$ first checks if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% \begin{enumerate}
% \item
% If $i \ne j$, then $\tilde{\Verifier}$ only applies $U_{gc}$ to increase the global counter, and does nothing else.
% \item
% If $i = j$, then $\tilde{\Verifier}$ first applies $U_{gc}$ to increase the global counter, and then behaves differently according to the value of the global counter $i$. We describe it in the following.
% \end{enumerate}

% \para{Global Counter $i = 1$.} This corresponds to $\tilde{\Verifier}$'s behavior for the 1st slot, namely generating $v_1$ as the response to the $p_1$ she just received form the $\Prover$. $\tilde{\Verifier}$ applies $\tilde{V}_1$, which is defined as follows
% $$\tilde{V}_1 \coloneqq D_1 C_1 B_1 A_1, $$
% \xiao{old name: $\tilde{V}_1 \coloneqq \tilde{U}_3 \tilde{U}_2 \tilde{U}_1,$}
% with the unitaries defined as follows:
% \begin{enumerate}
% % \item
% % {\bf ($\tilde{U}_{\msf{c}}$: Increase the Counter.)} This unitary maps $\ket{i}_{\reg{count}}$ to $\ket{i+1 \mod 2}_{\reg{count}}$.

% \item \label{item:Vtil:unitary:1-1}
% {\bf ($A_1$: Swap $\reg{p_1}$ and $\reg{m}$.)} This unitary swaps the contents of $\reg{p_1}$ and $\reg{m}$ registers.
% \begin{MyComment}
% In the real execution, this steps is for $\tilde{V}$ to move the first message it received from the prover (in the $\reg{m_1}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_1}$), so that it can perform computation in subsequent steps.
% \end{MyComment}

% \item \label{item:Vtil:unitary:1-2}
% {\bf ($B_1$: Apply $V$'s Unitary.)}
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then do nothing; \xiao{need to recall where $p_1$ is stored.}
% \item
% If $H(p_1) = 1$, then apply $\sum_{p_1} \ketbra{p_1} \tensor V_{p_1}$, which is the honest $\Verifier$'s unitary to generate $v_1$ from $p_1$.
% \end{enumerate}
% \begin{MyComment}
% Recall \xiao{from XXX} that $U$ can be written in the form of $\sum_{p_1} \ketbra{p_1}\tensor U_{p_1}$ because the concerned protocol is LOCC. $V_{p_1}$ works non-trivially on registers $\reg{ins}$, $\reg{v_2}$, and $\reg{w}$. In particular, it generates $V$'s message $v_1$ in register $\reg{v_1}$ (together with some residual state on $\reg{w}$).
% \end{MyComment}


% \item \label{item:Vtil:unitary:1-3}
% {\bf ($C_1$: Deliver $v_1$.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% \item
% If $H(p_1) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_1}$.
% % set the content in register $\reg{m}$ to $\ket{v_1 \xor m}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_1$ is the content in register $\reg{v_1}$. 
% \end{enumerate}


% \item \label{item:Vtil:unitary:1-4}
% {\bf ($D_1$: Increase Local Counter.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then do nothing.

% \item
% If $H(p_1) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
% \end{enumerate}
% \end{enumerate}


% \para{Global Counter $i = 2$.} This corresponds to $\tilde{\Verifier}$'s behavior for the 2nd slot, namely generating $v_2$ as the response to the $p_2$ she just received form the $\Prover$. $\tilde{\Verifier}$ applies $\tilde{V}_2$, which is defined as follows
% $$\tilde{V}_2 \coloneqq D_2C_2B_2A_2, $$
% \xiao{old name: $\tilde{V}_2 \coloneqq \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,$}
% with the unitaries defined as follows:

% % This corresponds to $\tilde{\Verifier}$'s behavior for the 2nd slot, namely generating $v_2$ as the response to the $p_2$ she just received form the $\Prover$. This case is different from the above case of the 1st slot---$\tilde{\Verifier}$ will first query the oracle $H$ on input $p_1$ stored in the register $\reg{p_1}$, and behaves differently according to the answer from $H$. \xiao{(need to add a remark: technically, we need to first compute the output of $H$, then do the following computation, and then un-compute $H$?)} In particular, we need to consider the following two sub-cases:
% % \begin{enumerate}
% % \item \label[Case]{item:LOCC-3ZK:Vtil:slot-2:bad}
% % If $H(p_1) = 0$, then $\tilde{\Verifier}$ does not do anything. Equivalently, $\tilde{V}_2$ is defined as
% %  $$\tilde{V}_2 \coloneqq I.$$

% % \item \label[Case]{item:LOCC-3ZK:Vtil:slot-2:good}
% % Otherwise (i.e., $H(p_1) = 1$), then $\tilde{V}_2$ is defined as
% % $$\tilde{V}_2 \coloneqq \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,$$ 
% % with the unitaries defiend as follows:

% % \end{enumerate}
% \begin{enumerate}
% \item \label{item:Vtil:unitary:2-1}
% {\bf ($A_2$: Swap $\reg{p_2}$ and $\reg{m}$.)} This unitary swaps the contents of $\reg{p_2}$ and $\reg{m}$ registers.

% \begin{MyComment}
% In the real execution, this steps is for $\tilde{V}$ to move the $p_2$ message it received from the prover (in the $\reg{m_2}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_2}$), so that it can perform computation in the next step.
% \end{MyComment}

% \item \label{item:Vtil:unitary:2-2}
% {\bf ($B_2$: $\tilde{\Verifier}$'s Decision.)} This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then do nothing. \xiao{need to recall where $(p_1,p_2)$ are stored.}

% \item
% If $H(p_1, p_2) = 1$, then apply $\sum_{p_2} \ketbra{p_2} \tensor V_{p_2}$, which is the honest $\Verifier$'s unitary to generate $v_2$ from $p_2$.
%  % it applies $U_\msf{d}$, where  $U_\msf{d}$ is the honest verifier's decision unitary. \xiao{If necessary, we can decompose $U_\msf{d}$ as $U_{\msf{d}} \coloneqq \sum_{p_1, v_1, p_2}\ketbra{p_1, v_1, p_2} \tensor U_{p_1, v_1, p_2}$.}
% \end{enumerate}
% % \begin{MyComment}
% % Recall that $U_\msf{d}$ works non-trivially on registers $\reg{ins}$, $\reg{p_1}$, $\reg{v_1}$, $\reg{p_2}$, $\reg{d}$, and $\reg{w}$. In particular, it generates $V$'s final decision bit in register $\reg{d}$ (together with some residual state on $\reg{w}$).
% % \end{MyComment}



% \item \label{item:Vtil:unitary:2-3}
% \xiao{Add this to make the writing of my proof consistent event at the `last layer' (i.e., \Cref{lem:LOCC-3ZK-hyb02:proof:invariant}). This essentially allows Sim to see the verifier's final decision bit, which is a weaker notion of ZK. this makes our impossibility result stronger.} 

% {\bf ($C_2$:  Deliver $v_2$.)} This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% \item
% If $H(p_1, p_2) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_2}$.
% % set the content in register $\reg{m}$ to $\ket{v_2 \xor m}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_2$ is the content in register $\reg{v_2}$. 
% % then sets the content in register $\reg{m_2}$ to $\ket{d \xor m}_{\reg{m_2}}$, where $m$ is the original content in register $\reg{m_2}$ and $d$ is the content in register $\reg{d}$.
% \end{enumerate}

% \item \label{item:Vtil:unitary:2-4}
% {\bf ($D_2$: Increase Local Counter.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then do nothing.

% \item
% If $H(p_1, p_2) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
% \end{enumerate}

% \end{enumerate}



% \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.



\xiao{Add a lemma stating that for all $x\in \Lang$, the execution between the honest $\Prover$ and $\tilde{\Verifier}$ will lead to acceptance with probability $\epsilon^2$. This proof is simply, but it helps the reader to understand our model. Also, I want to high-light that in the real execution, \Cref{item:LOCC-3ZK:Vtil:slot-2:good} will always be triggered.	}






\subsection{$\BQP$ Decider}

\para{MnR Game with ZK Simulator.} We first define the measure-and-reprogram (MnR) game w.r.t. the simulator $\Sim$ and $\tilde{\Verifier}(x)$ defined in previous sections. This game is simply an instantiation of MnR game defined in \Cref{MnR:lem:game} with the following notation: 
\begin{enumerate}
\item \label{LOCC-3ZK:MnR:notation:item:1}
We treat the execution of the simulator (with oracle access to $\tilde{V}$ and $\tilde{V}^\dagger$) as an oracle machine $\Sim^{\tilde{\Verifier}}$ that has quantum oracle access to a random function $H: \mcal{X}^{\le 2} \rightarrow \mcal{Y}$, where $\mcal{X}=\bits^\ell$ and $\mcal{Y} = \bits$. Let $\vb{y} = (y_1, y_2) \in \mcal{Y}^2$.

\item \label{LOCC-3ZK:MnR:notation:item:2}
Recall that the output of  $\Sim^{\tilde{\Verifier}}$ is defined to be the output $\tilde{\Verifier}$ at halt, which is in turn defined to be all the internal registers of $\tilde{\Verifier}$. We will split $\tilde{\Verifier}$'s output as $(\vb{p} = (p_1, p_2), \rho_{\msf{out}})$,  where $\vb{p}$ is the string contained in the $\reg{p_1}$ and $\reg{p_2}$ registers, and $\rho_{\msf{out}}$ is the remaining state tracing out $\reg{p_1}$ and $\reg{p_2}$. In particular, $\rho$ contains the global counter register $\reg{gc}$ and register $\reg{d}$ that contains $\tilde{\Verifier}$'s final decision (qu)bit. 

\item \label{LOCC-3ZK:MnR:notation:item:3}
We assume that $\Sim^{\tilde{\Verifier}}$ as an oracle machine makes $q$ queries to $H$ in total.
\end{enumerate}

Since this game will be particularly important for the sequel sections, we choose to present it in full detail in \Cref{LOCC-3ZK:MnR:game}.


\begin{GameBox}[label={LOCC-3ZK:MnR:game}]{Measure-and-Reprogram Game \textnormal{$\Sim^{\tilde{\Verifier}}[H, \vb{y}]$}}
 It works as follows
\begin{enumerate}
\item
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$  conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$.

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes $H$, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item If $j=j_i$ for some $i\in[2]$, measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, 2_i})$ where $2_i\leq 2$ is determined by the measurement outcome, and then behaves according to the value $b_i$ as follows:
        \begin{enumerate}
        \item 
        If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$, and then answer the $j_i$-th query using the reprogrammed oracle. 
        \item 
        If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$. 
        \end{enumerate}
    \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [2]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{LOCC-3ZK:MnR:notation:item:2}).

\item
For all $i \in [2]$ such that $j_i = \bot$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}_i \coloneqq (p^*_1, \ldots, p^*_i)$. 

\item
{\bf Output:} The output of this game is defined as follows
\begin{itemize}
\item
If it holds for all $i \in [2]$ that $\vb{p}_i$ is a prefix of $\vb{p}_2$, then output $(\vb{p}_2, \rho_{\msf{out}})$;

\item
Otherwise, output $(\bot, \bot)$.
\end{itemize}
\end{enumerate}
\end{GameBox}

\para{Decider for $\BQP$.} We now define the $\BQP$ decider $\mcal{B}$ in \Cref{LOCC-3ZK:BQP-decider}.
\begin{AlgorithmBox}[label={LOCC-3ZK:BQP-decider}]{\textnormal{$\BQP$} Decider $\mcal{B}(x)$}
On input a classical string $x$, machine $\mcal{B}(x)$ works as follows:
\begin{enumerate}
\item
{\bf (Parameter Setting.)}
Let $\vb{1} \coloneqq (1,1)$. Let $\mcal{M} \coloneqq \bits^{\ell}$ and $H_0 :\mcal{M}^{\le 2} \ra \bits$ be the zero-function, i.e., $H_0(p_1, \ldots, p_i) = 0$ for all $(p_1, \ldots, p_i) \in \mcal{M}^{\le 2}$.

\item
{\bf (MnP Game with $\Sim^{\tilde{V}}$.)} Execute $(\vb{p} = (p_1, p_2), \rho) \la \Sim^{\tilde{V}}[H_0, \vb{1}]$ as per \Cref{LOCC-3ZK:MnR:game}. 
% and let $\hat{H}_0$ denote the oracle at halt (i.e., the re-programmed oracle). 
 That is, $\mcal{B}(x)$ executes \Cref{LOCC-3ZK:MnR:game} with $H \coloneqq H_0$ and $\vb{y} = (1,1)$ and  denotes the output of this procedure as $(\vb{p} = (p_1, p_2), \rho)$.
% , and denotes the oracle at the end of the MnR game as $\hat{H}_0$.
 Note that in this step, $\mcal{B}$ makes use of its input $x$, which is used as the input instance to $\tilde{V}$ (though we did not include it in the notation explicitly).

\item
{\bf (Output.)} It outputs 1 if and only if $\msf{Pred}(\rho) = 1$, where $\msf{Pred}(\rho)$ is a (quantum) predicate that outputs 1 if and only if all of the following conditions hold:
\begin{enumerate}
% \item
% $\hat{H}_0(p_1) = 1$ and $\hat{H}_0(p_1, p_2) = 1$. (Recall that $p_1$ and $p_2$ are contained in $\vb{p}$.)

\item
% The value contained in the global counter register $\reg{gc}$ is 2. (Recall that the $\reg{gc}$ register is contained in $\rho$ and remains classical throughout the whole execution.)
Measure the local counter register $\reg{lc}$ in the computational basis and the measurement outcome is 1. (Recall that the $\reg{lc}$ register is contained in $\rho$.)
\item
Measure register $\reg{d}$ in the computational basis and the measurement outcome is 1. (Recall that the $\reg{d}$ register is also contained in $\rho$.)
\end{enumerate}
\end{enumerate}
\end{AlgorithmBox}


Next, we argue that $\mcal{B}$ is a valid $\BQP$ decider. Toward that, it suffices to establish the following \Cref{LOCC-3ZK:decider:lem:completeness,LOCC-3ZK:decider:lem:soundness}.

\begin{lemma}[Completeness]\label{LOCC-3ZK:decider:lem:completeness}
\xiao{(need to talk about $\epsilon \le \epsilon_q = \frac{1}{256k^2q^2(4kq+1)^{2k}}$ in this lemma.)}
For all $\Lang \in \BQP$ and all $x \in \Lang \cap \bits^{\secpar}$, it holds for the $\mcal{B}$ defined in \Cref{LOCC-3ZK:BQP-decider} that
$$\Pr[\mcal{B}(x) = 1] \ge \frac{1}{8 \cdot (4kq + 1)^{2k}} -\negl(\secpar).$$
\xiao{need to change $k$ to 2 in this special case.}
\end{lemma}


\begin{lemma}[Soundness]\label{LOCC-3ZK:decider:lem:soundness}
For all $\Lang \in \BQP$ and all $x \in \bits^{\secpar} \setminus \Lang$, it holds for the $\mcal{B}$ defined in \Cref{LOCC-3ZK:BQP-decider} that
$$\Pr[\mcal{B}(x) = 1] = \negl(\secpar).$$
\xiao{need to change $k$ to 2 in this special case.}
\end{lemma}

We present the proof for \Cref{LOCC-3ZK:decider:lem:completeness} in \Cref{sec:LOCC-3ZK:decider:lem:completeness:proof}. 

The proof for \Cref{LOCC-3ZK:decider:lem:soundness} is one of the most technically involved part of this work, and thus we put it in a separate section in \Cref{sec:LOCC-3ZK:decider:lem:soundness:proof}.


\subsection{Proof of Completeness}
\label{sec:LOCC-3ZK:decider:lem:completeness:proof}

\xiao{need to modify $k$ to $2$.}

In this subsection, we prove \Cref{LOCC-3ZK:decider:lem:completeness}.

First, notice that 
\begin{align}
\Pr[\mcal{B}(x) = 1] 
& = 
\Pr[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_0, \vb{1}]] \label{LOCC-3ZK:decider:lem:completeness:proof:sparsity:1} \\ 
& \ge 
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]] - 32k^2q^2\epsilon \label[Inequality]{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2} 
\end{align}
where \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:1} follows from the definition and notation in \Cref{LOCC-3ZK:BQP-decider}, and \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2} follows from \Cref{lem:ind-sparse-and-zero}. 
% (In \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2}, the predicate $\msf{Pred}^{\hat{H}_\epsilon}$ works in the same manner as the $\msf{Pred}^{\hat{H}_0}$ defined in \xiao{Cref} , except that it replaces $\hat{H}_0$ with $\hat{H}_\epsilon$.)

\subpara{Additional Notation.} In the following, we make use of the following notation:
\begin{itemize}
\item
For any classical oracle $H$, we use $\msf{SIM}^{H}$ to refer to the execution of $\Sim^{\tilde{\Verifier}}$ where $\tilde{\Verifier}$ uses $H$ as the oracle. 

\item
When we write $\bs{\beta}$ in the subscribe of the $\Pr$ symbol, it means we sample $\bs{\beta}$ from a distribution $D_\epsilon$ over $\bits^2$, whose each coordinate takes 1 with probability $\epsilon$ independently. 

\item
For a function $H: \mcal{M}^{\le 2} \ra \mcal{Y}$ and a vector $\vb{p} = (p_1, p_2) \in \mcal{M}^2$,  let $\bar{H}(\vb{p}) \coloneqq  \big(H(p_1), H(p_1, p_2) \big)$.

\item
The bold-face $\vb{1}$ is defined to be $(1, 1)$.
\end{itemize}
With the above notation, it holds that:
\begin{align*}
& \Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]] \\  
=~&  
\sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}   \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]]  \numberthis \label{LOCC-3ZK:decider:lem:completeness:proof:final:1} \\ 
\ge~& 
\frac{1}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \msf{SIM}^{H^{\vb{p}^*, \vb{1}}_\epsilon}] \numberthis \label{LOCC-3ZK:decider:lem:completeness:proof:final:2} \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon, \bs{\beta}}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 \wedge \bs{\beta} = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H^{\vb{p}^*, \bs{\beta}}_\epsilon}] \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \Pr_{H_\epsilon}[ \msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \numberthis \label{LOCC-3ZK:decider:lem:completeness:proof:final:3} 
,\end{align*}
where \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:1} follows from the Law of Total Probability, \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:2} follows from \Cref{MnR:lem},  and \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:3} follows again from the Law of Total Probability.

Next, we bound the RHS of \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:3} via the ZK guarantee for simulator $\Sim$. First, recall that \xiao{This probably should be a lemma appeared earlier.} the honest $\Prover$ will make $\tilde{\Verifier}^{H_\epsilon}$ accept with probability $\epsilon^k$. That is,
\begin{equation}\label{LOCC-3ZK:decider:lem:completeness:proof:final:4}
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1}~:~ (\vb{p}, \rho) \la \msf{OUT}_{\tilde{\Verifier}}\big(\langle \Prover(w), \tilde{\Verifier}^{H_\epsilon} \rangle(x)\big)] = \epsilon^k,
\end{equation}
where we used the fact that by definition,  $\tilde{\Verifier}^{H_\epsilon}$ accepts if the $\reg{lc}$ register contains 2, the decision register $\reg{d}$ contains 1, and the transcript $(p_1, p_2)$ satisfies $H_\epsilon(p_1) = 1$ and $H_\epsilon(p_1, p_2) = 1$. 

It then follows from \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:4} and the ZK property that 
\begin{equation}\label{LOCC-3ZK:decider:lem:completeness:proof:final:5}
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1}~:~ (\vb{p}, \rho) \la (\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \ge \epsilon^k - \negl(\secpar) \ge \frac{\epsilon^k}{4} - \negl(\secpar).
\end{equation}

In summary, it holds that 
\begin{align*}
\Pr[\mcal{B}(x) = 1] 
& \ge 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \bigg(\frac{\epsilon^k}{4} - \negl(\secpar) \bigg) - 32k^2q^2\epsilon \numberthis \label[Inequality]{LOCC-3ZK:decider:lem:completeness:proof:final:6} \\ 
& \ge 
\frac{1}{4(4kq+1)^{2k}} - \negl(\secpar) - 32k^2q^2\epsilon \numberthis \label[Inequality]{LOCC-3ZK:decider:lem:completeness:proof:final:7} \\ 
& \ge
\frac{1}{8(4kq+1)^{2k}} - \negl(\secpar) 
,\end{align*}
where \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:6} follows from  \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2}, \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:3}, and \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:5}, and \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:7} follows from our parameter setting that $\epsilon \le \epsilon_q = \frac{1}{256k^2q^2(4kq+1)^{2k}}$. \xiao{need to talk about $\epsilon_q$ in the lemma.}

This completes the proof of \Cref{LOCC-3ZK:decider:lem:completeness}.







\section{Warm Up: Three-Round BBZK in the CPM Model (Part 2/2)}
\label{sec:LOCC-3ZK:decider:lem:soundness:proof}

In this section, we prove \Cref{LOCC-3ZK:decider:lem:soundness}. 

At a high level, we assume for contradiction that  \Cref{LOCC-3ZK:decider:lem:soundness} is false and show how to construct a malicious prover $\tilde{\Prover}$ breaking the soundness of the original LOCC ZK protocol. Toward that, we first need to make some modifications to the machine $\mcal{B}$ and the MnR game $\Sim^{\tilde{\Verifier}}$, making use of some particular properties of the $\tilde{\Verifier}$ we defined earlier. This is done in \xiao{cref}. Next, we will present the malicious prover $\tilde{\Prover}$ and prver that it can indeed break the soundness. This is done in \xiao{cref}.

\subsection{Preparation}
\subsubsection{Restating the MnR Game}
In \Cref{LOCC-3ZK:MnR:game:modify:1}, we present a modified version of the MnR game $\Sim^{\tilde{\Verifier}}[H, \vb{y}]$ defined in \Cref{LOCC-3ZK:MnR:game}. Since we will be interested only in the case $H = H_0$ and $\vb{y} = \vb{1} = (1, 1)$, we present this case only. We highlight its difference with \Cref{LOCC-3ZK:MnR:game} in \red{red color}.


\begin{GameBox}[label={LOCC-3ZK:MnR:game:modify:1}]{Measure-and-Reprogram Game \textnormal{$\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$}}
 It works as follows
\begin{enumerate}
\item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:1}
For each $i\in[2]$, uniformly pick \dlt{$(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$} \red{$(j_i,b_i)\in [q]\times \bits$} conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. \red{It re-label the tuples $\Set{(j_i, b_i)}_{i \in [2]}$ to make sure that $j_1 < j_2$.} \red{It also defines an empty vector $\vb{p}_0 = \emptyset$.}

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes \red{$H_0$}, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:2:a} 
      If $j=j_i$ for some $i\in[2]$, \dlt{measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, 2_i})$ where $2_i\leq 2$ is determined by the measurement outcome,} \red{measure this query to obtain  $\vb{p}_i=(p_{i,1}, \ldots,p_{i, i})$.} \red{If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_i$, the execution halts immediately and outputs $(\bot, \bot)$.}
      \red{\begin{itemize}
      \item
      
      {\bf Defining $\msf{sq}(i)$:} Note that the $j_i$-th query to $\mcal{O}$ must be invoked by $\Sim$'s query to $\tilde{\Verifier}$. We will call this $\Sim$'s query (that invokes the $j_i$-th query to $\mcal{O}$) as the $i$-th special query and denote it by $\msf{sq}(i)$. We establish certain properties of $\msf{sq}(i)$ in \Cref{LOCC-3ZK:MnR:game:modify:1:lem}, which will be useful later. 
      \end{itemize}
      }

      It then behaves according to the value $b_i$ as follows:
        \begin{enumerate}
        \item 
        If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$, and then answer the $j_i$-th query using the reprogrammed oracle. 
        \item 
        If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$. 
        \end{enumerate}
    \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [2]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{LOCC-3ZK:MnR:notation:item:2}).

\item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:4}
\dlt{For all $i \in [2]$ such that $j_i = \bot$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}^*_i \coloneqq (p^*_1, \ldots, p^*_i)$.} 

\item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:5}
{\bf Output:}  \red{Output $(\vb{p}_2, \rho_{\msf{out}})$.}
\begin{itemize}
\item
\dlt{If it holds for all $i \in [2]$ that $\vb{p}_i$ is a prefix of $\vb{p}_2$, then output $(\vb{p}_2, \rho_{\msf{out}})$;}

\item
\dlt{Otherwise, output $(\bot, \bot)$.}
\end{itemize}
\end{enumerate}
\end{GameBox}

\begin{lemma}\label{LOCC-3ZK:MnR:game:modify:1:lem}
For the $\dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ defined in \Cref{LOCC-3ZK:MnR:game:modify:1} and the $\mcal{B}(x)$ defined in \Cref{LOCC-3ZK:BQP-decider}, it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]]\ge \Pr[\mcal{B}(x) = 1].$$
Moreover, for the $\msf{sq}(i)$ $(\forall i \in [2])$ defined in \Cref{LOCC-3ZK:MnR:game:modify:1:step:2:a}, it enjoys the following properties:
\begin{itemize}
\item
Query $\msf{sq}(i)$ is a $\tilde{V}$-query (instead of being a $\tilde{V}^\dagger$-query).
\item
\xiao{to be added as needed.}
\end{itemize}
\end{lemma}
\begin{proof}
	\begin{xiaoenv}{Polish the language}
	The proof of this lemma follows from the way we set counters.

	Need to explain the order $j_1 < j_2$.

	Next, we argue that the change in \Cref{LOCC-3ZK:MnR:game:modify:1:step:1} does not decrease the accepting probability of the predicate. To see that, notice that we start with an all-$0$ function $H_0$, and the whole MnR game $\Sim^{\tilde{\Verifier}}[H_0, \vb{1}]$ measures at most 2 queries in total. Therefore, if there is a tuple $(j_i, b_i) = (\bot, \bot)$, then at most one query can be measured. Also, due to the way we set the global and local counters, it is clear that the measurement will not output $(p_1, p_2)$ unless an ealier measurement has output $(p_1)$. That is, the measured queries will appear in a length-increasing order. Thus, if only one query corresponds to $H_0$ being programmed at (at most) a single point $p_1$ (to output 1). This cannot bring the local counter to $2$. In this case, $\msf{Pred}(\rho)$ will always output 0. Thus, it will not decrease the winning probability by delete $\Set{(\bot, \bot)}$ from the support of $(j_i, b_i)$. 

	Also, note that if $(j_i, b_i)$ does not take the value $(\bot, \bot)$, the condition in \Cref{LOCC-3ZK:MnR:game:modify:1:step:4} will never be satisfied. Thus, we can safely delete  \Cref{LOCC-3ZK:MnR:game:modify:1:step:4} as well.

	The modification in \Cref{LOCC-3ZK:MnR:game:modify:1:step:2:a} is simply to say that the first measurement generate $(p'_1)$ and the second measurement generate $(p'_1, p'_2)$. We have argued this in the above.

	Also, as long as the measured queries appear in a length-increasing order, the modification in	\Cref{LOCC-3ZK:MnR:game:modify:1:step:5} becomes only cosmetic.
	\end{xiaoenv}

This completes the proof of \Cref{LOCC-3ZK:MnR:game:modify:1:lem}.

\end{proof}


\para{Looking into $\Sim^{\tilde{\Verifier}}$.} Next, we re-state the game $\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$ defined in \Cref{LOCC-3ZK:MnR:game}. This time, we will look into the execution of $\Sim^{\tilde{\Verifier}}$ and their registers. This is different from previous games where we always treat $\Sim^{\tilde{\Verifier}}$ as a ``black-box'' and only focus on how it accesses the oracle $H_0$. We denote this game as $\msf{Real}(\Sim, \tilde{\Verifier})$ and present it in \Cref{LOCC-3ZK:MnR:game:real}.	

It is straightforward that \Cref{LOCC-3ZK:MnR:game:real} is identical to \Cref{LOCC-3ZK:MnR:game} with only cosmetic changes. Therefore, it holds that
\begin{equation}\label{LOCC-3ZK:MnR:to:real:ind-eq}
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].
\end{equation}



\begin{GameBox}[label={LOCC-3ZK:MnR:game:real}]{Game \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier})$}}
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in [q]\times \bits$ conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. W.l.o.g., we assume that $j_1 < j_2$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner for each $i \in [2]$. 

\para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with $\tilde{V}$ and $\tilde{V}^\dagger$ accordingly, where $\tilde{\Verifier}$ uses $H^{(i-1)}_0$ as the oracle.


\para{For Query $\msf{sq}(i)$:} Note that by \Cref{LOCC-3ZK:MnR:game:modify:1:lem}, $\msf{sq}(i)$ is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.	Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and behaves according to the value $b_i$ as follows:
\begin{enumerate}
\item 
        If $b_i=0$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i)}_0$ as the oracle.
. 

\item 
        If $b_i=1$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i-1)}_0$ as the oracle.
\end{enumerate}


\para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Real}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_2, \rho_{\msf{out}})$.

\end{GameBox}


\subsubsection{A Dummy Game} 

\para{A Dummy Version of $\tilde{\Verifier}$.} We first define a unitary $\ddot{V}$, which should be treated as the ``dummy version'' of $\tilde{\Verifier}$'s unitary $\tilde{V}$. We present it in \Cref{LOCC-3ZK:V-dummy}, highlighting its difference with $\tilde{V}$ in \red{red color}.
\begin{AlgorithmBox}[label={LOCC-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}
On each query, it first applies $U_{gc}$ to increase the global counter by 1. Then, it checks if the global counter value $i$ satisfies $i \in [2]$. If not, do nothing (technically, this can be understood as applying the identity operation). Otherwise, it compares $i$ with the local counter value $j$ and behaves accordingly (note that in the following we have $i \in [2]$):

% On each query, check if the global counter value $i$ satisfies $i \in \Set{0,1}$. If not, do nothing (technically, this can be understood as applying the identity operation). Otherwise, it checks if $i$ is equal to the local counter value $j$ and behaves accordingly (note that in the following we have $i \in \Set{0,1}$):

\begin{description}
\item[Case ($i = j+1$):] apply $D_i \red{\ddot{C}_i} A_i$, where $D_i$ and $A_i$ are as defined in \Cref{LOCC-3ZK:V:unitary} and \red{$\ddot{C}_i$} is defined as follows:
\begin{itemize}	

\item
{\bf $\ddot{C}_i$: Swap $\reg{m}$ and $\reg{t_i}$.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

\item
If $H(p_1, \ldots, p_i) = 1$, \red{then do nothing}. 
\end{itemize}
\end{itemize}

\item[Case ($i \ne j+1$):] apply $C'_i A_i$, where $A_i$ and $C'_i$ are as defined in \Cref{LOCC-3ZK:V:unitary}.
\end{description}
\end{AlgorithmBox}




% \begin{AlgorithmBox}[label={LOCC-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}


% \para{Compare Counters.} On each query, check if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% \begin{itemize}
% \item
% If $i \ne j$, then apply $U_{gc}$ to increase the global counter, and do nothing else.
% \item
% If $i = j$, then first apply $U_{gc}$ to increase the global counter, and then behave differently according to the value of the global counter $i$. We describe it in the following.
% \end{itemize}

% \para{Global Counter $i = 1$.} Apply $\ddot{V}_1 \coloneqq D_1 \red{\ddot{C}_1} A_1$, where $D_1$ and $A_1$ are the same as for $\tilde{V}$ and $\ddot{C}_1$ is defined as follows:
% \begin{itemize}
% \item
% {\bf ($\ddot{C}_1$: Swap $\reg{m}$ and $\reg{t_1}$.)} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% \item
% If $H(p_1) = 1$, \red{then do nothing}. 
% \end{itemize}

% \end{itemize}


% \para{Global Counter $i = 2$.} Apply $\ddot{V}_2 \coloneqq D_2 \red{\ddot{C}_2} A_2$,
% where $D_2$ and $A_2$ are the same as for $\tilde{V}$ and $\ddot{C}_2$ is defined as follows:
% \begin{itemize}

% \item 
% {\bf ($\ddot{C}_2$: Swap $\reg{m}$ and $\reg{t_2}$.)} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% \item
% If $H(p_1, p_2) = 1$, \red{then do nothing}. 
% \end{itemize}

% \end{itemize}

% \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.

% \end{AlgorithmBox}


\para{A Dummy MnR Game.} We now define another game $\msf{Dummy}(\Sim, \tilde{\Verifier})$. This game will essentially serve as a malicious prover $\tilde{\Prover}$ that could break the soundness of the original ZK protocol, leading to our desired contradiction. Intuitively, $\msf{Dummy}(\Sim, \tilde{\Verifier})$ behaves identical to $\msf{Real}(\Sim, \tilde{\Verifier})$ except for that it answers $\Sim$'s queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$ using the dummy version of $\tilde{\Verifier}$ as we defined in \Cref{LOCC-3ZK:V-dummy}. We present the game in \Cref{LOCC-3ZK:MnR:game:dummy} and highlight its difference $\msf{Real}(\Sim, \tilde{\Verifier})$ (in \Cref{LOCC-3ZK:MnR:game:real}) in \red{red color}. 
\begin{GameBox}[label={LOCC-3ZK:MnR:game:dummy}]{Game \textnormal{$\msf{Dummy}(\Sim, \tilde{\Verifier})$}}
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in [q]\times \bits$ conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. W.l.o.g., we assume that $j_1 < j_2$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner for each $i \in [2]$. 

\para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with \red{$\ddot{V}$} and \red{$\ddot{V}^\dagger$} accordingly, using $H^{(i-1)}_0$ as the oracle. (Note that \red{$\ddot{V}$} is defined in \Cref{LOCC-3ZK:V-dummy}.)


\para{For Query $\msf{sq}(i)$:} Note that by \Cref{LOCC-3ZK:MnR:game:modify:1:lem}, $\msf{sq}(i)$ is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.	Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and behaves according to the value $b_i$ as follows:
\begin{enumerate}
\item 
        If $b_i=0$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i)}_0$ as the oracle.
. 

\item 
        If $b_i=1$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i-1)}_0$ as the oracle.
\end{enumerate}


\para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Dummy}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_2, \rho_{\msf{out}})$.

\end{GameBox}
The following is the most involved lemma in this section. We defer its proof to \xiao{Cref}, before which we first show (in \xiao{Cref}) how to finish the current proof of \Cref{LOCC-3ZK:decider:lem:soundness} assuming that \Cref{LOCC-3ZK:MnR:game:dummy:lem} holds.


\begin{lemma}\label{LOCC-3ZK:MnR:game:dummy:lem}
For the $\msf{Dummy}(\Sim, \tilde{\Verifier})$ defined in \Cref{LOCC-3ZK:MnR:game:dummy} and the $\msf{Real}(\Sim, \tilde{\Verifier})$ defined in \Cref{LOCC-3ZK:MnR:game:real}, it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].$$
\end{lemma}

\subsection{Finishing the Proof of \Cref{LOCC-3ZK:decider:lem:soundness}}
\xiao{In this part, we finish the proof of \Cref{LOCC-3ZK:decider:lem:soundness} assuming that \Cref{LOCC-3ZK:MnR:game:dummy:lem} holds. This step is simple. I'll do it later.}



\subsection{Branch-Wise Equivalence Suffices}
We first notice that \Cref{LOCC-3ZK:MnR:game:real} can be treated as a sequence of alternating unitaries and measurements. In particular, there are 3 types of measurements (and $(q+4)$ measurements are made in total):
\begin{enumerate}
\item
\label[Type]{LOCC-3ZK:branchwise:measure:type:1}
{\bf Type-1:} The simulator $\Sim$ simply alternates between her local unitary $S$ and the measurement on register $\reg{u}$, which determines the type of her next query (i.e., either $\tilde{V}$ or $\tilde{V}^\dagger$). Note that there are $q$ such measurements since $\Sim$ makes $q$ queries in total.
\item
\label[Type]{LOCC-3ZK:branchwise:measure:type:2}
{\bf Type-2:}
When $\Sim$ makes the $\msf{sq}(i)$-th query, it triggers a measurement on registers $\reg{p_1}, \ldots, \reg{p_i}$. Note that there are $k =2$ such measurements.

\item
\label[Type]{LOCC-3ZK:branchwise:measure:type:3}
{\bf Type-3:}
The $\msf{sq}(i)$-th query is answered according to a random bit $b_i$ sampled at the beginning. This can be equivalently understood as preparing a qubit $\ket{\psi}_{\reg{b_i}} = \frac{1}{\sqrt{2}} (\ket{0} + \ket{1})$ at the beginning and measuring it to define the classical bit $b_i$ used to answer the $\msf{sq}(i)$-th query. Note that there are $k =2$ such measurements as well.
\end{enumerate}
Also, notice that in \Cref{LOCC-3ZK:MnR:game:real}, the values $\Set{j_i}_{i \in [2]}$ are sampled at the very beginning and after that the timing of all the measurements are fixed. It then follows from \Cref{lem:branchwise:preparation} that the accepting probability $\Pr[\msf{Pred}(\rho)]$ w.r.t.\  \Cref{LOCC-3ZK:MnR:game:real} can be equivalently expressed as the summation of all accepting probabilities w.r.t.\ a ``sub-normalized'' version of \Cref{LOCC-3ZK:MnR:game:real} where all the $(q+4)$ measurements are replaced with projections. Formally, we defined the ``sub-normalized'' \Cref{LOCC-3ZK:MnR:game:real} (and similarly for \Cref{LOCC-3ZK:MnR:game:dummy}) in \Cref{LOCC-3ZK:MnR:game:subnormalized}.

\begin{FigureBox}[label={LOCC-3ZK:MnR:game:subnormalized}]{Sub-Normalized Games \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$} and \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$}}
{\bf Parameters.} Fix $J = (j_1, j_2)$ such that $j_1, j_2 \in [q]$ and $j_1 < j_2$. Also fix a classical string of $(q+4)$ symbols $\msf{pat} = (u_1, \ldots, u_q, p_1, b_{1}, p_1p_2,   b_2)$ with  $u_i \in \Set{\uparrow, \downarrow}$, $p_1 \in \Set{0, 1}^{\ell}$, $p_1p_2 \in \Set{0, 1}^{2\ell}$, and $b_1, b_2 \in\bits$. The following games are parameterized by $(J, \msf{pat})$.

\para{Game $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} It behaves identically to \Cref{LOCC-3ZK:MnR:game:real} except for the following differences: 
\begin{enumerate}
	\item
	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

\item
When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
\item
When the measurement on $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$) is triggered (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1}$ (resp.\ $\ketbra{p_1,p_2}$) to register $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$); 
\item
When it needs $b_i$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:3} above), it applies the projector $\ketbra{b_i}$ to register $\reg{b_i}$. 
\end{enumerate}

\para{Game $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} This is defined in a similar way w.r.t.\ \Cref{LOCC-3ZK:MnR:game:dummy}. Namely, It behaves identically to \Cref{LOCC-3ZK:MnR:game:dummy} except for the following differences: 
\begin{enumerate}
	\item
	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

\item
When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
\item
When the measurement on $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$) is triggered (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1}$ (resp.\ $\ketbra{p_1,p_2}$) to register $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$); 
\item
When it needs $b_i$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:3} above), it applies the projector $\ketbra{b_i}$ to register $\reg{b_i}$. 
\end{enumerate}
\end{FigureBox}

It then follows from \Cref{lem:branchwise:preparation} that
\begin{align*}
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})] 
& = 
\frac{2!}{\binom{q}{2}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] \\
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] 
& = 
\frac{2!}{\binom{q}{2}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})],
\end{align*}
where the summations are taken over all possible $J$ and $\msf{pat}$ satisfying the requirements in \Cref{LOCC-3ZK:MnR:game:subnormalized}. 

Therefore, to prove \Cref{LOCC-3ZK:MnR:game:dummy:lem}, it suffices to prove the following \Cref{LOCC-3ZK:branch-wise:suffices}.
\begin{lemma}[Branch-Wise Equivalence Suffices]\label{LOCC-3ZK:branch-wise:suffices}
For all $(J, \msf{pat})$ satisfying the requirements in \Cref{LOCC-3ZK:MnR:game:subnormalized}, it holds that 
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})].$$
\end{lemma}


\subsection{Proving \Cref{LOCC-3ZK:branch-wise:suffices}}
In this proof, we consider an (arbitrarily) fixed $J$ and $\msf{pat}$ that satisfy the requirements in \Cref{LOCC-3ZK:MnR:game:subnormalized}.

\para{Simplification Assumptions.} We first make three assumptions regarding the behavior of $\Sim$. As we will show, these assumptions will not affect the accepting probability of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ and $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$, but it will simplify the notation and ease the presentation of the current proof.
\begin{itemize}
\item 
\hypertarget{LOCC-3ZK:simp-assumption:1}{{\bf Assumption 1:}} When the global counter is $\ket{0}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}^\dagger$ (resp.\ $\ddot{V}^\dagger$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$).

\item 
\hypertarget{LOCC-3ZK:simp-assumption:2}{{\bf Assumption 2:}} When the global counter is $\ket{2}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ (resp.\ $\ddot{V}$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$).

\item 
\hypertarget{LOCC-3ZK:simp-assumption:3}{{\bf Assumption 3:}} For each $i \in [2]$, before the $\msf{sq}(i)$-th query is made, when the global counter is $\ket{i-1}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ (resp.\ $\ddot{V}$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$) 
\end{itemize}
\xiao{We argue that we can indeed make these assumptions when proving \Cref{LOCC-3ZK:branch-wise:suffices}. to do... 
} \xiao{A caveat is:} to make \hyperlink{LOCC-3ZK:simp-assumption:3}{Assumption 3}, we need to additionally assume that before the $\msf{sq}(i)$-th query is made, $\Sim$'s local operator may modify register $\reg{t_i}$. But we claim that this will not affect our proof of \Cref{LOCC-3ZK:branch-wise:suffices}. 




Next, we define a sequence of hybrids $H_0$, $H_1$, and $H_2$. To better illustrate these hybrids, we provide pictures in \Cref{figure:CPM-3ZK:hybrids}.

\para{Hybrid $H_0$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H0}.) This is exactly the execution of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. 

\xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H0}. 
Point out the position of $\msf{sq}(1)$ and $\msf{sq}(2)$. Also exaplain how the assumptions made above are reflected in this figure.}

Therefore, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$




\para{Hybrid $H_1$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H1}.) This hybrid is identical to the previous one except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (i.e., query $\msf{sq}(1)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (resp.\ from $\ket{1}_{\reg{gc}}$ to $\ket{0}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}
This is best illustrated by the \red{red-color} symbols in \Cref{figure:CPM-3ZK:hybrids:H1} \xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H1}} 

\para{Hybrid $H_2$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H2}.) This hybrid is identical to the previous one except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (i.e., query $\msf{sq}(2)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (resp.\ from $\ket{2}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}
This is best illustrated by the \red{red-color} symbols in \Cref{figure:CPM-3ZK:hybrids:H2} \xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H2}} 

It is straightforward that hybrid $H_2$ is exactly the execution of $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. Therefore, it holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_2 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$


\begin{figure}[!tb]
\centering
     \begin{subfigure}[t]{0.47\textwidth}
         \fbox{
         \includegraphics[width=\textwidth,page=1]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H0}
     \end{subfigure}
     \hspace{15pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=2]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H1}
     \end{subfigure}
     
     \centering\vspace{1em}
     \begin{subfigure}[t]{0.47\textwidth}
         
         \fbox{
         \includegraphics[width=\textwidth,page=3]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H2}
     \end{subfigure}
     \caption{Illustration of Hbyrids $H_0$, $H_1$, and $H_2$}
     \label{figure:CPM-3ZK:hybrids}
\end{figure}

With the above hybrids, to prove \Cref{LOCC-3ZK:branch-wise:suffices}, it now suffices to establish the following \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. 
\begin{lemma}\label{lem:CPM-3ZK:H01}
It holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_1 \big].$$
\end{lemma}

\begin{lemma}\label{lem:CPM-3ZK:H12}
It holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_1 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_2 \big].$$
\end{lemma}

\para{Preparation for the proofs of \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}.} In the sequel (\xiao{crefxxx}), we prove \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. Before we start, we first do some preparation work and set up some notations that will ease our presentation later.

First, recall from \Cref{LOCC-3ZK:MnR:game:real} that after the $\msf{sq}(i)$-th query is made, the malicious verifier $\tilde{\Verifier}$ will use $H^{\vb{p}_i, \vb{1}}_0$ as its oracle. Also, note that the above hybrids are defined w.r.t.\ a fixed $(J,\msf{pat})$. Therefore, we could re-write some of $\tilde{\Verifier}$'s unitaries in \Cref{LOCC-3ZK:V:unitary}, whose behavior depend on the value $H(p_1, \ldots, p_i)$, into a format that uses the $p_i$'s contained in (the a prior fixed) $\msf{pat}$ as a controlled unitary. 

In particular, for the $(p_1, p_2)$ contained in the fixed $\msf{pat}$, we keep the $U_{gc}$, $U_{lc}$, $A_i$ and $D_i$ the same as in \Cref{LOCC-3ZK:V:unitary}, but we re-write the unitaries $B_i$ and $C_i$ ($\forall i \in [2]$) in the following format:
\begin{enumerate}
\item \label{LOCC-3ZK:renaming:B1}
Let $B_1 = \ketbra{p_1}_{\reg{p_1}} \tensor B_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor I$. Note that $B_{1,1}$ is exactly the $V_{p_1}$ in \Cref{LOCC-3ZK:V:unitary}, and it acts non-trivially only on $\reg{v_1}$ and $\reg{w}$, and works as identity on other registers. 

\item \label{LOCC-3ZK:renaming:C1}
Let $C_1 = \ketbra{p_1}_{\reg{p_1}} \tensor C_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor C_{1,0}$. Note that $C_{1,1}$ is the swap operator between $\reg{v_1}$ and $\reg{m}$; $C_{1,0}$ is the swap operator between  $\reg{t_1}$ and $\reg{m}$.

\item \label{LOCC-3ZK:renaming:B2}
Let $B_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor B_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor I$. Note that $B_{2,1}$ is exactly the $V_{p_2}$ in \Cref{LOCC-3ZK:V:unitary}, which acts non-trivially only on $\reg{v_2}$ and $\reg{w}$, and works as identity on other registers.

\item \label{LOCC-3ZK:renaming:C2}
Let $C_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0}$. Note that $C_{2,1}$ is the swap operator between $\reg{m}$ and $\reg{v_2}$; $C_{2,0}$ is the swap operator between $\reg{m}$ and $\reg{t_2}$.
\end{enumerate}
It will be helpful to keep track of the registers on which the unitaries acts on {\em non-trivially}. For the reader's convenience, we summarize it in \Cref{LOCC-3ZK:non-trivial-registers:table}. For a unitary shown in the table, it acts as the identity on registers not shown in its row.
\begin{table}[!htb]
\centering
\caption{Registers on which the unitaries acts non-trivially}
\label{LOCC-3ZK:non-trivial-registers:table}
\vspace{0.5em}
\begin{tabular}{C{50pt} C{70pt} c C{50pt} C{70pt}}
\toprule
Unitary operators & Non-trivial registers & \phantom{abcde}  & Unitary operators & Non-trivial registers \\ 
\cmidrule{1-2} \cmidrule{4-5}
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$A_1$    	& $\reg{p_1}, \reg{m}$ & & 
$A_2$ 		& $\reg{p_2}, \reg{m}$ \\ 
\addlinespace[0.3em]
$B_1$ 		& $\reg{p_1}$, $\reg{v_1}$, $\reg{w}$   & & 
$B_2$ 		& $\reg{p_1}$, $\reg{p_2}$, $\reg{v_2}$, $\reg{w}$ \\
\addlinespace[0.3em]
$B_{1,1}$ 	& $\reg{v_1}$, $\reg{w}$  & & 
$B_{2,1}$ 	& $\reg{v_2}$, $\reg{w}$ \\ 
\addlinespace[0.3em]
$C_1$    	&  $\reg{p_1}$, $\reg{v_1}$, $\reg{t_1}$, $\reg{m}$ & & 
$C_2$    	&  $\reg{p_1}$, $\reg{p_2}$, $\reg{v_2}$, $\reg{t_2}$, $\reg{m}$  \\ 
\addlinespace[0.3em]
$C_{1,1}$   & $\reg{v_1}$, $\reg{m}$  & & 
$C_{2,1}$   & $\reg{v_2}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$C_{1,0}$  	& $\reg{t_1}$, $\reg{m}$ & & 
$C_{2,0}$  	& $\reg{t_2}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$D_1$		& $\reg{p_1}$, $\reg{lc}$  & & 
$D_2$		& $\reg{p_1}$, $\reg{p_2}$, $\reg{lc}$ \\ 
\addlinespace[0.3em]
& & &   $S$ 		& $\reg{m}$, $\reg{s}$, $\reg{u}$  \\   
\bottomrule
\end{tabular}
\end{table}


\subsection{Proving \Cref{lem:CPM-3ZK:H01}}

We first present the following \xiao{lemma}.
\xiao{add some intuitive explanation.}

\begin{lemma}[Invariance in $H_0$ and $H_1$]\label{lem:LOCC-3ZK-hyb01:proof:invariant}
Assume that during the execution of $H_0$ (and $H_1$), the global counter reaches value $1$ for $T$ times in total. For each $t \in [T]$, there exist (potentially sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds: in hybrid $H_0$ (resp.\ $H_1$), when the global counter reaches value $1$ for the $t$-th time, the overall state can be written as $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows
\begin{align}
\ket{\phi^{(t)}} 
& = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}}, \label{lem:LOCC-3ZK-hyb01:proof:target-format:H0}\\ 
\ket{\psi^{(t)}} 
& = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{C_{1,0}} \ket{\rho^{(t)}_{p'_1}}. \label{lem:LOCC-3ZK-hyb01:proof:target-format:H1}
\end{align}
where the unitaries $B_{1,1}$, $C_{1,0}$, and $C_{1,1}$  are as defined in \Cref{LOCC-3ZK:non-trivial-registers:table}.
\end{lemma}


\para{Finishing the proof of \Cref{lem:CPM-3ZK:H01}}. Let us consider the last time when the global counter reaches value $1$. By \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}, the overall states in $H_0$ and $H_1$ would be of the format 
\begin{align}
\ket{\phi^{(T)}} 
& = 
\overbrace{
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}} ,\\ 
\ket{\psi^{(T)}}
& = 
\overbrace{
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{C_{1,0}} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}}. 
\end{align}
Since this is the last time the global counter reaches value $1$, the two hybrids $H_0$ and $H_1$ by definition behave identically after that. That is, the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ will go through the same quantum procedure (let us denote it by $\mcal{F}$) and finally measured by the predicate $\msf{Pred}$.	

Next, note that the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the identical ``branch'' corresponding to $\ket{p_1}_{\reg{p_1}}$ (labeled as $\msf{Good}$ in the above equations). Also, the $\msf{Bad}$ branch will not contribute any shares to the accepting probability of the predicate $\msf{Pred}$---this is because the quantum procedure $\mcal{F}$ will never change the local counter for the $\msf{Bad}$ branch, and $\msf{Pred}$ will output $0$ if the local counter is not $\ket{2}_{\reg{lc}}$.	

In summary, only the $\msf{Good}$ branch matters for the remaining execution to contribute to the event $\msf{Pred}(\rho) = 1$. Therefore, \Cref{lem:CPM-3ZK:H01} holds because $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the same $\msf{Good}$ branch.

\para{Proving \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.} Now, the only thing left is to prove \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}. We establish this lemma by a mathematical induction on the number $t \in [T]$ indicating it is which time global counter reaches value $1$. We will keep track of how the overall states evolve in both $H_0$ and $H_1$ simultaneously.

\subsubsection{Base Case ($t = 1$)} 
This corresponds to the very first time the global counter reaches $1$. By definition, this is due to $\Sim$'s query $\msf{sq}(1)$. 

We first derive how the overall state evolves in $H_0$. Formally, $\Sim$'s local operation $S$ is applied to the initial state, preparing a superposition in register $\reg{m}$. Then, the first $\tilde{V}$-query (i.e., the query $\msf{sq}(1)$) is made. Note that at this moment, both the global and local values are of the value $0$. Thus, according to \Cref{LOCC-3ZK:V:unitary} and \Cref{LOCC-3ZK:MnR:game:subnormalized}, the state will evolves as follows:
\begin{enumerate}
\item
$U_{gc}$ increases the global counter from $0$ to $1$. Note that currently, the global counter and local counter are of the form $\ket{1}_{\reg{gc}}\ket{0}_{\reg{gc}}$. 

\item
The unitary $A_1$ is applied

\item
The $\reg{p_1}$ register is projected to $\ketbra{p_1}_{\reg{p_1}}$.
\item
The unitary $D_1C_1B_1$ is then applied.
\end{enumerate}
In summary, the state $\ket{\phi^{(1)}}$ is obtained by applying the operator $D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}S$ is applied to the initial state. If we assume the initial state across all the registers are $\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}$, then it holds that:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}S  
\big(
\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}
\big) \\
& = 
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}  
\big( 
\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}} S \ket{\rho}
\big)
 \numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:1} \\ 
& = 
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 
\big(
\ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} S \ket{\rho} 
\big) 
\\
& = 
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} 
\big(
 \ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} A_1 S \ket{\rho} 
 \big)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:2} \\ 
& = 
D_1C_1B_1  
\big(
 \ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} \ketbra{p_1}_{\reg{p_1}}  A_1 S \ket{\rho} 
 \big)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:3} \\ 
& = 
D_1C_1B_1  
\big(
\ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\rho_{p_1}} 
\big)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:4} \\ 
& = 
D_1  
\big(
 \ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} C_{1,1}B_{1,1} \ket{\rho_{p_1}}
 \big) 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:5} \\ 
& = 
 \ket{1}_{\reg{gc}}\ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} C_{1,1}B_{1,1} \ket{\rho_{p_1}} 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:6} \\ 
& = 
 \ket{1}_{\reg{gc}}\ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:1} follows from the fact $S$ acts as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:2} follows from the fact $A_1$ acts as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:3} follows from the fact that the projector $\ketbra{p_1}_{\reg{p_1}}$ has no effects on $\reg{gc}$ and $\reg{lc}$;
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:4} follows by defining the (sub-normalized) state $\ket{\rho_{p_1}} \coloneqq \bra{p_1}_{\reg{p_1}}  A_1 S \ket{\rho}$;
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:5} follows from the definition of $B_{1,1}$ and $C_{1,1}$ (see \Cref{LOCC-3ZK:renaming:B1,LOCC-3ZK:renaming:C1});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:6}  follows from the definition of $D_1$ (see \Cref{LOCC-3ZK:V:unitary});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} follows by defining $\ket{\rho^{(1)}_{p_1}} \coloneqq C_{1,1}B_{1,1} \ket{\rho_{p_1}}$.
\end{itemize}
% Obviously, $\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7}$ is a special case of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} when $t = 1$.
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} satisfies the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} when $t = 1$.


Also, note that the game $H_0$ and $H_1$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} that 
$$\ket{\psi^{(1)}} =  \ket{1}_{\reg{gc}}\ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} .$$ Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.


\UpdateLine{}






\subsection{Evolution of Registers in Simulation}

\begin{xiaoenv}{Some modifications needed for the model}
Further modify the modeling of the Simulator:
\begin{itemize}
\item
$\Sim$ prepares $q$ registers to store her query pattern, initialized to $\downarrow$: $\ket{\downarrow}_{\reg{u_1}} \ldots \ket{\downarrow}_{\reg{u_q}}$.
\item
Use a single unitary $S$ to denote $\Sim$'s algorithm, instead of $S_1$, $S_2$, $S_3$ as above. $S$ works on $\reg{m_1}$, $\reg{m_2}$, and $\reg{s}$. Actually, $S$ also need to work on the query pattern registers to determine the next query. Thus, we denote the $S$ as a sequence $S_1$, \ldots, $S_q$, $S_{q+1}$where $S_{i}$ works on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{s}$ and $\reg{u_i}$.
\item
State the lemma: The whole execution can be viewed as running $\Sim$ first for a fixed query pattern without intermediate measurement, and then project onto $\reg{u_1}\ldots\reg{u_q}$ w.r.t.\ the fixed query pattern to obtain a sub-normalized state. The norm of the state is the probability that this state would appear as a result of the real execution. 
\item
May also need to assume that $\Sim$ does not abort in the middle---She can always make dummy queries until the end. See how CCLY deal with this?
\end{itemize}
\end{xiaoenv}



In the following, we consider a fixed query patter of $q$ queries $\msf{Pat} \in \msf{PatSet}$.

We consider the setting where we measure the first messages when $\Sim$ tries to jump from Layer-$i$ to Layer-$(i+1)$ to obtain a classical prover message $p_i$. Right after this step, the oracle $H$ will be updated by adding $H(p_i) = 1$. ($H$ is initialized to output 0 on all inputs.)

We define the following hybrids:

\para{Hybrid $H_0$:} This is the game we just defined above. \xiao{refer to the picture} We use $\Pr[H_0 = 1]$ to denote the probability that at the last-step measurement of register $\reg{d}$ output 1. 

\para{Hybrid $H_1$:} This hybrid is identical to $H_0$, except that all the up (resp.\ down) queries between Layer-1 and Layer-2, {\em except the first $\downarrow$-query}, are answered by $\tilde{U}^\dagger_{\msf{dmy}}$ (resp.\ $\tilde{U}_{\msf{dmy}}$). \xiao{refer to the picture}

Importantly, we note that the behavior of $\tilde{U}_{\msf{dmy}}$ between Layer-1 and Layer-2 is defined to be $A_{\msf{dmy}} \tilde{U}_1$, where 
\begin{equation}\label{eq:A-dummy}
A_{\msf{dmy}} = \ketbra{p_1}_{\reg{p_1}} \tensor I + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \tilde{U}_{3,1}
\end{equation}
(see \Cref{LOCC-3ZK:renaming:2} below)

\para{Hybrid $H_2$:} This hybrid is identical to $H_1$, except that all the up (resp.\ down) queries between Layer-2 and Layer-3 are answered by $\tilde{U}^\dagger_{\msf{dmy}}$ (resp.\ $\tilde{U}_{\msf{dmy}}$). \xiao{refer to the picture}

Importantly, we note that the behavior of $\tilde{U}_{\msf{dmy}}$ between Layer-1 and Layer-2 is defined to be $B_{\msf{dmy}}\tilde{U}_3$, where
\begin{equation}\label{eq:B-dummy}
B_{\msf{dmy}} = \ketbra{p_1}_{\reg{p_1}}\ketbra{p_2}_{\reg{p_2}} \tensor I + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1}_{\reg{p_1}}\ketbra{p'_2}_{\reg{p'_2}} \tensor \tilde{U}_{6,1}
\end{equation}
(see \Cref{LOCC-3ZK:renaming:4} below)


In the following, we prove that $\Pr[H_0 = 1] = \Pr[H_2 = 1]$, which can be broken as the following two lemmas.
\begin{lemma}\label{lem:LOCC-3ZK-hyb01}
It holds that $\Pr[H_0 = 1] = \Pr[H_1 = 1]$.
\end{lemma}

\begin{lemma}\label{lem:LOCC-3ZK-hyb12}
It holds that $\Pr[H_1 = 1] = \Pr[H_2 = 1]$.
\end{lemma}


\xiao{Explain why these lemmas are important to our proof. Add some intuition. Say that the proof of these lemmas make use of the Error-Invariant Commutativity Lemma}


\para{Renaming Unitaries.} Before proving these lemmas, we first group and rename $\tilde{V}$'s unitaries (defined in \Cref{sec:particular-mal-V}). For a fixed $p_1, p_2 \in \bits^\ell$,
\begin{enumerate}
\item \label{LOCC-3ZK:renaming:1}
Let $\tilde{U}_2 = \ketbra{p_1}_{\reg{p_1}} \tensor \tilde{U}_{2,0} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor I$. Note that $\tilde{U}_{2,0}$ acts non-trivially only on $\reg{v_1}$ and $\reg{w}$, and works as identity on other registers. $I$ is identity on all registers.
\item \label{LOCC-3ZK:renaming:2}
Let $\tilde{U}_3 = \ketbra{p_1}_{\reg{p_1}} \tensor \tilde{U}_{3,0} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \tilde{U}_{3,1}$. Note that $\tilde{U}_{3,0}$ acts non-trivially only on $\reg{v_1}$ and $\reg{m_1}$, and is identity on other registers. $\tilde{U}_{3,1}$ is the swap operator between $\reg{m_1}$ and $\reg{t_1}$, and is identity on other registers. 
\item \label{LOCC-3ZK:renaming:3}
Let $\tilde{U}_5 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{5,0} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor I$. Note that $\tilde{U}_{5,0}$ is nothing but the $U_d$ operator, which acts non-trivially only on registers $\reg{d}$ and $\reg{w}$, and is identity on other registers.
\item \label{LOCC-3ZK:renaming:4}
\xiao{(newly added.)  }
Let $\tilde{U}_6 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{6,0} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{6,1}$. Note that $\tilde{U}_{6,0}$ acts non-trivially only on $\reg{d}$ and $\reg{m_2}$, and is identity on other registers. $\tilde{U}_{6,1}$ is the swap operator between $\reg{m_2}$ and $\reg{t_2}$, and is identity on other registers. 
\end{enumerate}


It will be important to keep track on the registers that the unitaries acts on {\em non-trivially}. For the reader's convenience, we summarize it in \Cref{LOCC-3ZK:table:non-trivial-registers}. For a unitary shown in the table, it acts as identity on registers not shown in its column.

% \begin{table}[h!]
% \caption{Registers the Unitary Operators Acts on Non-Trivially}
% \label{LOCC-3ZK:table:non-trivial-registers}
% \begin{center}\def\arraystretch{1.5}
% \begin{tabular}{ |C{50pt}|| C{30pt}|C{30pt}|C{30pt} | C{30pt}|C{30pt}| C{35pt}|C{30pt}|C{30pt}|C{30pt}| C{30pt} | C{30pt}| C{30pt}| C{30pt} | C{50pt}| }
%  \hline
% Unitary Operators & 
% $\tilde{U}_{1}$ &  
% $\tilde{U}_{2,0}$ & 
% $\tilde{U}_{2}$ & 
% $\tilde{U}_{3,0}$ & 
% $\tilde{U}_{3,1}$ & 
% $\tilde{U}_{3}$ & 
% $\tilde{U}_{4}$ & 
% $\tilde{U}_{5,0}$ & 
% $\tilde{U}_5$ & 
% $\tilde{U}_{6,0}$ & 
% $\tilde{U}_{6,1}$ & 
% $\tilde{U}_{6}$ & 
% $S_0$ & $S_j$ ($j \in [q]$) \\
% \hline
% Non-Trivial Registers & 
% $\reg{p_1}$, $\reg{m_1}$ & 
% $\reg{v_1}$, $\reg{w}$ & 
% $\reg{p_1}$, $\reg{v_1}$,  $\reg{w}$ & 
% $\reg{v_1}$, $\reg{m_1}$ & 
% $\reg{m_1}$, $\reg{tmp}$ & 
% $\reg{p_1}$, $\reg{v_1}$, $\reg{m_1}$, $\reg{tmp}$ & 
% $\reg{p_2}$, $\reg{m_2}$ & 
% $\reg{d}$, $\reg{w}$ & 
% $\reg{p_1}$, $\reg{p_2}$, $\reg{d}$, $\reg{w}$ &  
% $\reg{d}$, $\reg{m_2}$  &  
% $\reg{t_2}$, $\reg{m_2}$ &  
% $\reg{p_1}$, $\reg{p_2}$, $\reg{t_2}$, $\reg{m_2}$, $\reg{d}$ & 
% \red{place holder} & 
% $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, $\reg{s}$ \\
% \hline
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}[h!]
\caption{Registers the Unitary Operators Acts on Non-Trivially}
\label{LOCC-3ZK:table:non-trivial-registers}
\begin{center}\def\arraystretch{1.5}
\begin{tabular}{ |C{80pt}| L{100pt}|}
 \hline
Unitary Operators & Non-Trivial Registers   \\
\hline
$\tilde{U}_{1}$ & $\reg{p_1}$, $\reg{m_1}$ \\
\hline
$\tilde{U}_{2,0}$ & $\reg{v_1}$, $\reg{w}$ \\
\hline
$\tilde{U}_{2}$ & $\reg{p_1}$, $\reg{v_1}$,  $\reg{w}$ \\
\hline
$\tilde{U}_{3,0}$ & $\reg{v_1}$, $\reg{m_1}$  \\
\hline
$\tilde{U}_{3,1}$ & $\reg{m_1}$, $\reg{tmp}$ \\
\hline
$\tilde{U}_{3}$ & $\reg{p_1}$, $\reg{v_1}$, $\reg{m_1}$, $\reg{tmp}$  \\
\hline
$\tilde{U}_{4}$ & $\reg{p_2}$, $\reg{m_2}$ \\
\hline
$\tilde{U}_{5,0}$ & $\reg{d}$, $\reg{w}$ \\
\hline
$\tilde{U}_{5}$ & $\reg{p_1}$, $\reg{p_2}$, $\reg{d}$, $\reg{w}$  \\
\hline
$\tilde{U}_{6,0}$ & $\reg{d}$, $\reg{m_2}$  \\
\hline
$\tilde{U}_{6,1}$ & $\reg{t_2}$, $\reg{m_2}$ \\
\hline
$\tilde{U}_{6}$ & $\reg{p_1}$, $\reg{p_2}$, $\reg{t_2}$, $\reg{m_2}$, $\reg{d}$  \\
\hline
 $S_j$ ($j \in [q]$) & $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, $\reg{s}$  \\ 
 \hline
\end{tabular}
\end{center}
\end{table}



\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb01}}

\begin{xiaoenv}{Outline}
Outline of the proof	
\begin{itemize}
\item
We will fix a particular $\vb{u} = (u_1, \ldots, u_q)$ and $(p_1, p_2)$. We will eventually invoke the new branch-wise equivalence lemma (\Cref{sec:branch-wise-equiv-lemma-new}) to argue the IND between $H_0$ and $H_1$.
\item
Define another game $H'_0$ and $H'_1$, where the measurement is replaced with projections $\ketbra{u_1}_{\reg{u_1}}, \ldots, \ketbra{u_q}_{\reg{u_q}}$ and $\ketbra{p_1}_{\reg{p_1}}, \ketbra{p_2}_{\reg{p_2}}$.
\item
Focusing on the derivations for $H'_0$ and $H'_1$, and then invoke the new branch-wise equivalence lemma (\Cref{sec:branch-wise-equiv-lemma-new}) to argue the IND between $H_0$ and $H_1$.
\end{itemize}
\end{xiaoenv}

\begin{lemma}\label{lem:LOCC-3ZK-hyb01:proof:invariant}
Assume that the execution of $H'_0$ (and $H'_1$) \xiao{I think $H'_0$ is defined for fixed $p_1, p_2, u$} reaches Layer-2 for $K$ times in total. For each $k \in [K]$, there exist (potentially sub-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds: in hybrid $H'_0$ (resp.\ $H'_1$), when execution reaches Layer-2 for the $k$-th time, the overall state can be written as $\ket{\phi^{(k)}}$ (resp.\ $\ket{\psi^{(k)}}$) defined as follows
\begin{align}
\ket{\phi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}}\ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{\tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}} \ket{\rho^{(k)}_{p'_1}}, \label{lem:LOCC-3ZK-hyb01:proof:target-format:H0}\\ 
\ket{\psi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}}\ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{\tilde{U}_{3,1}} \ket{\rho^{(k)}_{p'_1}}. \label{lem:LOCC-3ZK-hyb01:proof:target-format:H1}
\end{align}
\end{lemma}

\xiao{say that the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} is post-poned to \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof}. For now, we use \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} to finish the current proof of \Cref{lem:LOCC-3ZK-hyb01}.}

\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}}
\label{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof}
We establish this lemma by a mathematical induction on the number $k \in [K]$ indicating it is which time the execution reaches Layer-2. We will keep track of how the overall states evolve in both $H'_0$ and $H'_1$ simultaneously.

\subsubsection{Base Case ($k = 1$)} 
\label{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:sec} 

This corresponds to the very first time the execution reaches Layer-2. 

We first derive how the overall state evolves in $H'_0$. Formally, $\Sim$'s local operation $S_0$ is applied to the initial state, preparing a superposition in register $\reg{m_1}$. Then, $\reg{m_1}$ and $\reg{p_1}$ are swapped, and $\reg{p_1}$ is projected onto $\ketbra{p_1}_{\reg{p_1}}$, resulting in a state of the format $\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}$, where $\rho_{p_1}$ is some sub-normalized pure state over registers other than $\reg{p_1}$. \xiao{need to talkb about $\Sim$'s other `attempts' to reach Layer-2 (but not succeed)} Then, the first  $\downarrow$ query is made, bringing the execution from Layer-1 to Layer-2 for the first time. This $\downarrow$ query corresponds to apply $\tilde{U}_3\tilde{U}_2$ on state $\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}$. Formally, the resulting state becomes:
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:H0}
\ket{\phi^{(1)}} = \tilde{U}_3\tilde{U}_2 \ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}
=
\ket{p_1}_{\reg{p_1}} \tilde{U}_{3,0}\tilde{U}_{2,0} \ket{\rho_{p_1}} 
=
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} 
,\end{equation} 
where the first equality follows from the definition of $\tilde{U}_3$ and $\tilde{U}_2$, and the second equality follows by renaming $\ket{\rho^{(1)}_{p_1}} \coloneqq\tilde{U}_{3,0}\tilde{U}_{2,0} \ket{\rho_{p_1}}$, which is again a (sub-normalized) pure state over registers other than $\reg{p_1}$.

It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:H0} satisfies the format shown in  \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} with $k = 1$. 


\xiao{add more explanation.} Also, note that the game $H'_0$ and $H'_1$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:H0} $\ket{\psi^{(1)}} = \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}}$. Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} with $k = 1$.

This finishes the proof for the base case $k = 1$.  

\subsubsection{Induction Step ($k\ge 2$)} 
\label{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:sec} 

We assume $\ket{\phi^{(k-1)}}$ and $\ket{\psi^{(k-1)}}$ satisfies \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}, and prove in the following that \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} holds when the execution reaches Layer-2 for the $k$-th time.

We establish this claim by considering the following MECE (mutually exclusive and collectively exhaustive) cases:
\begin{enumerate}
\item \label[Case]{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}
{\bf Case 1:} The $k$-th arrival is due to an immediate $\uparrow \downarrow$ after the $(k-1)$-th arrival. That is, after the $(k-1)$-th arrival, $\Sim$ first makes a $\uparrow$ query, jumping to Layer-1, and then makes an $\downarrow$ query, jumping back to Layer-2. \xiao{see picture XXX for an example}
\item \label[Case]{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}
{\bf Case 2:} The $k$-th arrival is due to an immediate $\downarrow \uparrow $ after the $(k-1)$-th arrival. That is, after the $(k-1)$-th arrival, $\Sim$ first makes a $\downarrow$ query, jumping to Layer-3, and then makes an $\uparrow$ query, jumping back to Layer-2. \xiao{see picture XXX for an example}
\end{enumerate}


\subsubsubsection{Proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}} 
We first describe formally how $\ket{\phi^{(k-1)}}$ (resp.\ $\ket{\psi^{(k-1)}}$) evolves into $\ket{\phi^{(k)}}$ (resp.\ $\ket{\psi^{(k)}}$) in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}:
\begin{enumerate}
 \item
$\Sim$'s local unitary $S_j$ is applied. Note that this step is identical for both $H'_0$ and $H'_1$. \xiao{say that we assume this is the $j$-th local step}. \item
An $\uparrow$-query is made, bringing the execution to Layer-1. 
\begin{itemize}
    \item
    In $H'_0$, this corresponds to applying $\tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3$; 
    \item
    In $H'_1$, this corresponds to applying $\tilde{U}^\dagger_1 A^\dagger_{\msf{dmy}}$ (as per \Cref{eq:A-dummy}). 
\end{itemize}
\item
The $(j+1)$-th local operation $S_{j+1}$ is applied. Note that this step is identical for both $H'_0$ and $H'_1$ as well.
\item
An $\downarrow$-query is made, bringing the execution back to Layer-2 for the $k$-th time.
\begin{itemize}
    \item
    In $H'_0$, this corresponds to applying $\tilde{U}_3 \tilde{U}_2 \tilde{U}_1$; 
    \item
    In $H'_1$, this corresponds to applying $A_{\msf{dmy}}\tilde{U}_1$ (as per \Cref{eq:A-dummy}). 
\end{itemize} 
\end{enumerate}
It follows from the above description that the states $\ket{\phi^{(k)}}$ and $\ket{\psi^{(k)}}$ can be written as:
\begin{align}
\ket{\phi^{(k)}}
& = \tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j \cdot \ket{\phi^{(k-1)}}, \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}\\ 
\ket{\psi^{(k)}}
& = A_{\msf{dmy}}\tilde{U}_1 S_{j+1}\tilde{U}^\dagger_1 A^\dagger_{\msf{dmy}} S_j \cdot \ket{\psi^{(k-1)}}. \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}
\end{align}

\begin{remark}[High-Level Idea for the Sequel]
Recall that our eventual goal is to prove that the states $\ket{\phi^{(k)}}$ and $\ket{\psi^{(k)}}$ are of the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0,lem:LOCC-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}. But we first need to perform some preparation work, putting \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}. Then, we show on \Cpageref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} how to combine \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:err-inv-com} to complete the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}. 
\end{remark}


\begin{MyClaim}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}
There exist (potentially sub-normalized) pure states $\Set{\dot{\rho}^{(k-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ so that the following holds
\begin{align}
\ket{\phi^{(k)}}
& = \tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(k)}}
& = 
A_{\msf{dmy}} S^{\reg{p_1}/\reg{m}}_{j+1}  A^\dagger_{\msf{dmy}}
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} \ket{\dot{\rho}^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} 
\end{align}
where $S^{\reg{p_1}/\reg{m}}_{j+1}$ is identical to $S_{j+1}$ except that it treats register $\reg{p_1}$ as $\reg{m}$.
\end{MyClaim}


\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}]

First, notice that  
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S} 
\tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 =  \tilde{U}_1 \tilde{U}^\dagger_1  S^{\reg{p_1}/\reg{m}}_{j+1} = S^{\reg{p_1}/\reg{m}}_{j+1},
\end{equation}
where the first equality follows from the fact that $S_{j+1}$ does not operate on $\reg{p_1}$ and $\tilde{U}^\dagger_1$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_1}$. 
% It is worth recalling  \xiao{cref to place} that $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ is the same unitary operator as $S_{j+1}$ but treating register $\reg{p_1}$ as $\reg{m_1}$. Thus, $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ acts non-trivially only on $\reg{p_1}$, $\reg{m_2}$, $\reg{u}_{j+1}$, and $\reg{s}$, and is identity on other registers.

\para{Proving \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(k)}}$:
\begin{align}
\ket{\phi^{(k)}}
& = 
\tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j \cdot \ket{\phi^{(k-1)}} \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} \\
& = 
\tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j \cdot 
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} \\
& = 
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} \\
& = 
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3 
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} S_j \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} \\
& = 
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3 
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} S^{\reg{t_1}/\reg{m}}_j  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} \\
& = 
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3 
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} \\
& = 
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} 
,\end{align}
where \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}, \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S}, \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} follows from fact that $S_j$ works as identity on $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} follows from the definition of $\tilde{U}_{3,1}$ (see \Cref{LOCC-3ZK:renaming:2}) and the definition of $S^{\reg{t_1}/\reg{m}}_j$, where \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} follows from that $S^{\reg{t_1}/\reg{m}}_j$ works on different registers from $\tilde{U}_{2,0}^\dagger\tilde{U}_{3,0}^\dagger$, and \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} follows by setting 
\begin{equation}
\label[Expression]{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}
\ket{\dot{\rho}^{(k-1)}_{p_1}}   \coloneqq S_j \ket{\rho^{(k-1)}_{p_1}} ~~~\text{and}~~~
\ket{\dot{\rho}^{(k-1)}_{p'_1}}  \coloneqq S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}).
\end{equation}
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7}  finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\para{Proving \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi}.} This proof is almost identical to the above proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align}
\ket{\psi^{(k)}}
& = 
A_{\msf{dmy}}\tilde{U}_1 S_{j+1}\tilde{U}^\dagger_1 A^\dagger_{\msf{dmy}} S_j  \cdot \ket{\psi^{(k-1)}} \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} \\
& = 
A_{\msf{dmy}}\tilde{U}_1 S_{j+1}\tilde{U}^\dagger_1 A^\dagger_{\msf{dmy}} S_j  \cdot 
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2} \\
& = 
A_{\msf{dmy}} S_{j+1} A^\dagger_{\msf{dmy}}
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} 
\bigg)  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:3} \\
& = 
A_{\msf{dmy}} S_{j+1} A^\dagger_{\msf{dmy}}
\cdot
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:4} 
,\end{align}
where \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}, \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:3} follows from a similar argument as we did to derive \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} (from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2}), and \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:4} follows from the same definitions of $\ket{\dot{\rho}^{(k-1)}_{p_1}}$ and $\ket{\dot{\rho}^{(k-1)}_{p'_1}}$ as shown in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}.

\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:4}  finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\vspace{1em}

This eventually finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\end{proof}


\para{Finishing the Proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}.}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish}
 With the above \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} in hand, we can finish the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1} by applying \Cref{lem:err-inv-com}. Formally, we apply \Cref{lem:err-inv-com} to the states and operators in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}, with the notation correspondence listed in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}. We provide a detailed explanation below.

%% deleted because Jiahu prefer it.
% \begin{table}[!htb]
% \centering
% \caption{Notation Correspondence between \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6} and \Cref{lem:err-inv-com}}
% \label{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}
%     \begin{subtable}[t]{.3\linewidth}
%       \centering
%         \caption{Registers}
%         \begin{tabular}{ C{50pt} C{60pt}}
%           \toprule
%           In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4} \\ \midrule 
%           $\reg{a}$    & $\reg{p_1}$ \\ 
%           $\reg{m}$    & $\reg{m_1}$  \\ 
%           $\reg{t}$    & $\reg{t_1}$ \\ 
%           $\reg{s}$    & $\reg{m_2}$,  $\reg{u_{j+1}}$, $\reg{s}$ \\ 
%           $\reg{o}$    & other registers \\ 
%           \bottomrule
%         \end{tabular}
%     \end{subtable}
%     \begin{subtable}[t]{.3\linewidth}
%       \centering
%         \caption{Operators}
%         \begin{tabular}{C{50pt} C{60pt}}
%           \toprule
%           In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4} \\ \hline 
%           \addlinespace[0.3em]
%           $W_0$ & $\tilde{U}_{3,0}$ \\ 
%           \addlinespace[0.3em] 
%           $W_1$ & $\tilde{U}_{3,1}$  \\
%           \addlinespace[0.3em] 
%           $W$   & $\tilde{U}_{3}$ \\
%           \addlinespace[0.3em] 
%           $U_0$ & $\tilde{U}_{2,0}$ \\
%           \addlinespace[0.3em] 
%           $U$   & $\tilde{U}_{2}$ \\
%           \addlinespace[0.3em] 
%           $S$   & $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ \\
%           \bottomrule
%         \end{tabular}
%     \end{subtable} 
%     \begin{subtable}[t]{.3\linewidth}
%       \centering
%         \caption{Random Variables}
%         \begin{tabular}{ C{50pt} C{60pt}}
%           \toprule
%           In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4} \\ \midrule 
%           \addlinespace[0.3em]
%           $a$    & $p_1$ \\ 
%           \addlinespace[0.3em]
%           $a'$    & $p'_1$  \\ 
%           \addlinespace[0.3em]
%           $\rho_a$    & $\dot{\rho}_{p_1}$ \\ 
%           \addlinespace[0.3em]
%           $\rho_{a'}$    & $\dot{\rho}_{p'_1}$ \\ 
%           \bottomrule
%         \end{tabular}
%     \end{subtable} 
% \end{table}

\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}}
\label{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1}$ & & $W_0$ & $\tilde{U}_{3,0}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_1$ & $\tilde{U}_{3,1}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_1}$ & & $W$   & $\tilde{U}_{3}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u_{j+1}}$, $\reg{s}$ & & $\tilde{W}$ & $A_{\msf{dmy}}$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p'_1}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_0$ & $\tilde{U}_{2,0}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish:def:eta-in-0} \\ 
\addlinespace[0.3em]
   & & & $U$   & $\tilde{U}_{2}$ & & $\ket{\eta^{(\msf{in})}_1}$ & \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish:def:eta-in-1}  \\ 
   \addlinespace[0.3em]
 &  & & $S$   & $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\phi^{(\msf{k})}}$  \\ 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\psi^{(\msf{k})}}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} notation, this is satisfied by $\tilde{U}_{3,0}$ (playing the role of $W_0$) who works as identity on registers $\reg{u_{j+1}}$ and $\reg{s}$ (playing the role of registers $\reg{s}$).

\item
\Cref{lem:err-inv-com} requires that $W_1$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} notation, this is satisfied by $\tilde{U}_{3,1}$ (playing the role of $W_1$), who is a swap operator between registers $\reg{m}$ and $\reg{t_1}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively).

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_1$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} notation, this is satisfied by $A_{\msf{dmy}}$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $\tilde{U}_{3,1}$ (playing the role of $W_1$) on branches $\ket{p'_1}_{\reg{p_1}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $p'_1 \ne p_1$.

\item
 \Cref{lem:err-inv-com} requires that $U_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} notation, this is satisfied by $\tilde{U}_{2,0}$ (playing the role of $U_0$), who works as identity on registers $\reg{u_{j+1}}$ and $\reg{s}$ (playing the role of register $\reg{s}$).

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} notation, this is satisfied by $S^{\reg{p_1}/\reg{m}}_{j+1}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{u_{j+1}}$ and $\reg{s}$ (playing the role of registers $\reg{a}$ and $\reg{s}$).
\end{itemize}

Next, using the above notation, we could define
\begin{align}
\ket{\eta^{(\msf{in})}_0}
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}^{(k-1)}_{p'_1}}, \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish:def:eta-in-0} \\ 
\ket{\eta^{(\msf{in})}_1}
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} \ket{\dot{\rho}^{(k-1)}_{p'_1}}.  \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish:def:eta-in-1}  
\end{align}


Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}) to the $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ defined in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish:def:eta-in-0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish:def:eta-in-1}. This implies the existence of (potentially non-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1}}}_{p'_1\in\bits^\ell }$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\phi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}}\ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k)}_{p'_1}} \\ 
\ket{\psi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}}\ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \ket{\rho^{(k)}_{p'_1}} 
,\end{align*}
which are exactly \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} and \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} in  \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}. 

This completes the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}.







\subsubsubsection{Proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}} 
First, we remark that the computation performed over $\ket{\phi^{(k-1)}}$ and $\ket{\psi^{(k-1)}}$ are identical, because $H'_0$ and $H'_1$ are identical for the execution below Layer-2.

We now describe formally how $\ket{\phi^{(k-1)}}$ (and thus $\ket{\psi^{(k-1)}}$) evolves in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}. 
\begin{enumerate}
\item
$\Sim$'s local operator $S_j$ is applied
\item
An $\downarrow$-query is made, bringing the execution to Layer-3. Here are two sub-cases to consider, depending if the $\downarrow$ query represents the first time the execution arrives at Layer-3. 
\begin{enumerate}
\item \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-1}
If it is the first time the execution arrives at Layer-3, the operator  $\tilde{U}_6 \tilde{U}_5 \ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} \tilde{U}_4$ will be applied;
\item \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-2}
Otherwise, the operator $\tilde{U}_6 \tilde{U}_5 \tilde{U}_4$ will be applied.   
\end{enumerate}
\item 
The $(j + 1)$-th local operation $S_{j+1}$ is applied. 
\item
An $\uparrow$-query is made, bringing the execution to Layer-2 for the $k$-th time. This corresponds to applying $\tilde{U}^\dagger_4\tilde{U}^\dagger_5 \tilde{U}^\dagger_6$.
\end{enumerate}
In summary, the evolution in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2} could be expressed as 
\begin{align}
\ket{\phi^{(k)}} &= \Lambda S_j \cdot \ket{\phi^{(k-1)}} \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi}\\ 
\ket{\psi^{(k)}} &= \Lambda S_j \cdot \ket{\psi^{(k-1)}} \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi},
\end{align}
where $\Lambda$ is defined to be {\em either}
\begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:def:Lambda}
\Lambda \coloneqq \tilde{U}^\dagger_4\tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_{j+1} \tilde{U}_6 \tilde{U}_5 \ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} \tilde{U}_4~~~\text{or}~~~\Lambda \coloneqq \tilde{U}^\dagger_4\tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_{j+1} \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,
\end{equation}
depending on which sub-case between \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-1,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-2} we are talking about.

Fortunately, we can finish the proof for both of these two sub-cases (i.e., the two versions of $\Lambda$) at one stroke. To do that, we first establish a claim regarding the operator $\Lambda$.
\begin{MyClaim}\label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}
The following holds for both forms of $\Lambda$ as defined in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:def:Lambda}. There exist two operators $\Lambda_0$ and $\Lambda_1$ operating on registers other than $\reg{p_1}$ so that the following holds
\begin{align}
& 
\Lambda = \ketbra{p_1}_{\reg{p_1}} \tensor \Lambda_0 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Lambda_1, \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} \\ 
& 
\Lambda_1 \tilde{U}_{3,1}  = \tilde{U}_{3,1} \Lambda^{\reg{t_1}/\reg{m}}_1, ~\text{and} \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} \\ 
& 
\Lambda_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Lambda^{\reg{t_1}/\reg{m}}_1 \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} 
,\end{align}
where $\Lambda^{\reg{t_1}/\reg{m_1}}_1$ is identical to $\Lambda_1$ except that it treats $\reg{t_1}$ as $\reg{m_1}$.  
\end{MyClaim}

\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}]
To prove \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, it suffices to show that for each operator $\Gamma \in \Set{S_{j+1}, \tilde{U}_6, \tilde{U}_5, \ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}},\tilde{U}_4}$, there exist operators $\Gamma_0$ and $\Gamma_1$ so that $\Gamma$ can be written as 
$$\Gamma = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_0 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_1$$
and it holds that $\Gamma_1 \tilde{U}_{3,1}  = \tilde{U}_{3,1} \Gamma^{\reg{t_1}/\reg{m}}_1$ and $\Gamma_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Gamma^{\reg{t_1}/\reg{m}}_1$.

Obviously, the above is true for $\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}}$, simply because such a $\Gamma$ can be written in the following format:
$$\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_0  + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor I,$$
with $\Gamma_0  \coloneqq \ketbra{p_2}_{\reg{p_2}}$ and $\Gamma_1  \coloneqq I$, and thus $\Gamma_1$ vacuously satisfies the requires $\Gamma_1 \tilde{U}_{3,1}  = \tilde{U}_{3,1} \Gamma^{\reg{t_1}/\reg{m}}_1$ and $\Gamma_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Gamma^{\reg{t_1}/\reg{m}}_1$.


% acts on neither $\reg{p_1}$ nor $\reg{m}$, and it acts non-trivially on different registers from that of $\tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}).

The above is true for $\Gamma =\tilde{U}_4$ as well, because $\tilde{U}_4$ is nothing but the swap operator between registers $\reg{p_2}$ and $\reg{m}$.

The above is also true for $\Gamma = S_{j+1}$ because (1) $S_{j+1}$ does not act on $\reg{p_1}$, (2) $S_{j+1}$ does not work on $\reg{t_1}$ and $\tilde{U}_{3,1}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_1}$, and (3) $S^{\reg{t_1}/\reg{m}}_{j+1}$ acts non-trivially on different registers from $\tilde{U}_{2,0}$ and $\tilde{U}_{3,0}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}).



% is easy to see (from \Cref{LOCC-3ZK:table:non-trivial-registers}) that $S_{j+1} \tilde{U}_{3,1}  = \tilde{U}_{3,1}   S^{\reg{t_1}/\reg{m_1}}_{j+1}$ and  $S_{j+1} \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m_1}}_{j+1}$.


The only  cases left are $\Gamma \in \Set{\tilde{U}_5, \tilde{U}_6}$. These two cases are a little trickier than the previous cases because they use $\reg{p_1}$ (and $\reg{p_2}$) as a control register (see \Cref{LOCC-3ZK:renaming:3,LOCC-3ZK:renaming:4}). In the following, we only prove it for $\Gamma = \tilde{U}_6$; the other case (i.e., $\Gamma = \tilde{U}_5$) follows from a similar argument.
\begin{align*}
\Gamma = \tilde{U}_6 
& = 
\ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{6,0} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{6,1} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:1} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor \tilde{U}_{6,0} 
+ 
\sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1}_{\reg{p_1}} \tensor \ketbra{p'_2}_{\reg{p_2}} \tensor \tilde{U}_{6,1} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor \tilde{U}_{6,0} 
+ \ketbra{p_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1} \\ 
& \hspace{15em} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1} \\ 
& = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_0 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_1 \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:2}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:1} follows from the definition of $\tilde{U}_6$ from \Cref{LOCC-3ZK:renaming:4}, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:2} follows from defining $\Gamma_0$ and $\Gamma_1$ as follows 
\begin{align*}
 \Gamma_0 & \coloneqq \ketbra{p_2}_{\reg{p_2}} \tensor \tilde{U}_{6,0} 
+ \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1} \\ 
 \Gamma_1 & \coloneqq \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1}.
\end{align*} 
Clearly, such a $\Gamma_1$ also satisfies $\Gamma_1 \tilde{U}_{3,1}   = \tilde{U}_{3,1}  \Gamma_1^{\reg{t_1}/\reg{m}}$ and $\Gamma_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Gamma_1^{\reg{t_1}/\reg{m}}$, because (1) such a $\Gamma_1$ does not operates on $\reg{t_1}$, (2) $\tilde{U}_{3,1}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_1}$, and (3) $\Gamma^{\reg{t_1}/\reg{m}}_1$ acts non-trivially on different registers from $\tilde{U}_{2,0}$ and $\tilde{U}_{3,0}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}).
% $\Gamma_1$ operates on different registers from $\tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ and $\Gamma_1$ does not work on $\reg{m_1}$ (therefore it is vacuously true that $\Gamma_1 = \Gamma^{\reg{t_1}/\reg{m_1}}_1$).


This finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.

\end{proof}



\para{Finishing the Proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}.} In the following, we show how to finish the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2} using \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.

First, we present the derivation for $\ket{\phi^{(k)}}$:
\begin{align}
 \ket{\phi^{(k)}} & = \Lambda S_j \cdot \ket{\phi^{(k-1)}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:0}\\ 
 & =  
\Lambda  S_j \cdot
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}}
\bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:1} \\ 
& = 
\Lambda \cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  S_j \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:2} \\
& = 
\Lambda \cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} S^{\reg{t_1}/\reg{m}}_j  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:3} \\ 
& = 
\Lambda \cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:4} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \Lambda_1 \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:5} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Lambda^{\reg{t_1}/\reg{m}}_1 S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:6} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k)}_{p'_1}},  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:7} 
\end{align}
where  \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:0} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:1} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:2}  follows from the fact that $S_j$ does not act on register $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:3} follows from the definition of $S_j$ and $\tilde{U}_{3,1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:4} follows from the fact that $S^{\reg{t_1}/\reg{m}}_j$ and $\tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ operate non-trivially on different registers (see \Cref{LOCC-3ZK:table:non-trivial-registers}), \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:5} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:6} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:7} follows by defining
\begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:def:rho-k}
\ket{\rho^{(k)}_{p_1}} 
\coloneqq 
 \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}} ~~~\text{and}~~~ 
\ket{\rho^{(k)}_{p'_1}} 
\coloneqq 
\Lambda^{\reg{t_1}/\reg{m}}_1 S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}). 
\end{equation}
Clearly, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:7} is of the same format as \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.


Next, we present the derivation for $\ket{\psi^{(k)}}$:
\begin{align}
 \ket{\psi^{(k)}} & = \Lambda S_j \cdot \ket{\psi^{(k-1)}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0}\\ 
 & =  
\Lambda  S_j \cdot
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \ket{\rho^{(k-1)}_{p'_1}}
\bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \Lambda_1 \tilde{U}_{3,1}     S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2} \\
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}    \Lambda^{\reg{t_1}/\reg{m}}_1 S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3} \\  
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}    \ket{\rho^{(k)}_{p'_1}},  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} 
,\end{align}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2} follows from a similar argument as we derived \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:5} (from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:1}), \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} follows from the same definitions of $\ket{\rho^{(k)}_{p_1}}$ and $\ket{\rho^{(k)}_{p'_1}}$ as shown in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:def:rho-k}.

Clearly, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} is of the same format as \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.

This finishes the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}.


\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:sec} together finish the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} eventually.





\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb12}}

\xiao{almost copy the proof for \Cref{lem:LOCC-3ZK-hyb01}. Include it for demonstration of the 4-round baby case. In the final constant-round case, such a lemma is indeed generic reduciton step between $H'_{i-1}$ and $H'_{i}$.}

\begin{lemma}\label{lem:LOCC-3ZK-hyb12:proof:invariant}
Assume that the execution of $H'_1$ (and $H'_2$) \xiao{I think $H'_1$ is defined for fixed $p_1, p_2, u$} reaches Layer-3 for $K$ times in total. For each $k \in [K]$, there exist (potentially sub-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1, p'_2}}}_{(p'_1, p'_2) \in \bits^\ell\times\bits^\ell}$ so that the following holds: in hybrid $H'_1$ (resp.\ $H'_2$), when execution reaches Layer-3 for the $k$-th time, the overall state can be written as $\ket{\phi^{(k)}}$ (resp.\ $\ket{\psi^{(k)}}$) defined as follows
\begin{align}
\ket{\phi^{(k)}} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \red{\tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0}} \ket{\rho^{(k)}_{p'_1, p'_2}}, \label{lem:LOCC-3ZK-hyb12:proof:target-format:H1}
\\ 
\ket{\psi^{(k)}} 
& = 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p'_2}}\red{\tilde{U}_{6,1}} \ket{\rho^{(k)}_{p'_1, p'_2}}, \label{lem:LOCC-3ZK-hyb12:proof:target-format:H2}
\end{align}
where the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
\end{lemma}

\xiao{finish the proof of \Cref{lem:LOCC-3ZK-hyb12} using \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}.}







\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}}

Similar as in the proof of \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof}, 
we establish \Cref{lem:LOCC-3ZK-hyb12:proof:invariant} by a mathematical induction on the number $k \in [K]$ indicating it is which time the execution reaches Layer-3. We will keep track of how the overall states evolve in both $H'_1$ and $H'_2$ simultaneously.







\subsubsection{Base Case ($k = 1$)}
\label{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:sec} 


This corresponds to the very first time the execution reaches Layer-3. 

Notice that the execution has to reach Layer-2 before it reaches Layer-3. Notation-wise, let $\ket{\eta}$ denote the overall state at this particular arrival at Layer-2 (i.e., the one right before it reaches Layer-3 for the first time). It then follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} that $\ket{\eta}$ in game $H'_1$ can be written as
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:initial-state}
\ket{\eta} = \ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \ket{\rho_{p'_1}}.
\end{equation}
Moreover, this $\ket{\eta}$ is also the overall state at the same time point {\em in game $H'_2$}, simply because the games $H'_1$ and $H'_2$ are identical so far. Also, $\ket{\eta}$ will evolve in an identical manner in $H'_1$ and $H'_2$ until the first arrival at Layer. Formally, in both games, $\Sim$'s local operation $S_j$ is applied to $\ket{\eta}$. Then, the operator $\tilde{U}_6\tilde{U}_5\ketbra{p_1, p_2}_{\reg{p_1p_2}}\tilde{U}_4$ is applied, bringing the execution to Layer-3 for the first time. In summary, it holds that
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi-psi-equal}
\ket{\phi^{(1)}} = \ket{\psi^{(1)}} = \tilde{U}_6\tilde{U}_5\ketbra{p_1, p_2}_{\reg{p_1p_2}}\tilde{U}_4 S_j \cdot \ket{\eta}.
\end{equation}

In the following, we show that such a $\ket{\phi^{(1)}}$ (resp.\ $\ket{\psi^{(1)}}$) indeed satisfies the requirement as stipulated by  \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1} (resp.\ \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H2}) in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}.


\xiao{Check with @Nai-Hui if a sub-normalized state can be decomposed as in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:4}...}

\begin{align*}
\ket{\phi^{(1)}}
& = 
\tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}\tilde{U}_4 S_j \cdot \ket{\eta} \\
& =
 \tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}\tilde{U}_4  S_j 
\cdot \bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1}  \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:1} \\ 
& =
 \tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}\tilde{U}_4  
\cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1}  S^{\reg{t_1}/\reg{m}}_j \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:2} \\ 
& =
\tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}
\cdot \bigg(
\ket{p_1}_{\reg{p_1}} \tilde{U}_4 S_j \ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_4 \tilde{U}_{3,1}  S^{\reg{t_1}/\reg{m}}_j \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:3} \\ 
& =
\tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}
\cdot \bigg(
\ket{p_1}_{\reg{p_1}} \sum_{p'_2 \in \bits^{\ell}}\ket{p'_2}_{\reg{p_2}} \ket{\rho_{p_1, p'_2}} + \\
& \hspace{19em} 
\sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \sum_{p'_2 \in \bits^{\ell}}\ket{p'_2}_{\reg{p_2}} \ket{\rho_{p'_1, p'_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:4} \\ 
& =
\tilde{U}_6\tilde{U}_5
\cdot 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho_{p_1, p_2}}  
\\ 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \tilde{U}_{6,0}\tilde{U}_{5,0} \ket{\rho_{p_1, p_2}} 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:5} \\ 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(1)}_{p_1, p_2}} 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:1} follows from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:initial-state}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:2} follows from the definitions of $S_j$ and $\tilde{U}_{3,1}$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:3} follows from the fact that $\tilde{U}_4$ works as identity on register $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:4} follows from decomposing the $\reg{p_2}$ register in the computational basis for states $\tilde{U}_4 S_j \ket{\rho_{p_1}}$ and $\tilde{U}_4 \tilde{U}_{3,1}  S^{\reg{t_1}/\reg{m}}_j \ket{\rho_{p'_1}}$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:5} follows from the definitions of $\tilde{U}_5$ and $\tilde{U}_6$, and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6} follows by defining $\ket{\rho^{(1)}_{p_1, p_2}}  \coloneqq \tilde{U}_{6,0}\tilde{U}_{5,0} \ket{\rho_{p_1, p_2}}$.
% \begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:7}
% \forall p'_1 \in \bits^{\ell}, ~~\ket{\rho^{(1)}_{p'_1, p_2}}  \coloneqq \tilde{U}_{6,0}\tilde{U}_{5,0} \ket{\rho_{p'_1, p_2}}.
% \end{equation}

It is straightforward that \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6} is a special case of \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1} with $k=1$, as stipulated by \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. 

Also, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi-psi-equal,lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6} together imply that 
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:psi:derivation:1}
 \ket{\psi^{(1)}} = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(1)}_{p_1, p_2}}.
\end{equation}
Clearly, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:psi:derivation:1} is a special case of \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H2} with $k=1$, as stipulated by \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. 

This finishes the proof for the base case $k =1$.






\subsubsection{Induction Step ($k\ge 2$)} 
\label{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:sec} 

We assume $\ket{\phi^{(k-1)}}$ and $\ket{\psi^{(k-1)}}$ satisfies \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}, and prove in the following that \Cref{lem:LOCC-3ZK-hyb12:proof:invariant} holds when the execution reaches Layer-2 for the $k$-th time.





Consider the execution between the $(k-1)$-th arrival and $k$-th arrival at Layer-3. It can be described as follows:
\begin{enumerate}
\item
 $\Sim$ first applies the local operator $S_j$. Note that this step is identical for both $H'_1$ and $H'_2$.
 \item
An $\uparrow$-query is made, bringing the execution to Layer-2. 
\begin{itemize}
\item
In $H'_1$, this corresponds to applying $\tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6$;
\item
In $H'_2$, this corresponds to applying $\tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}} $ (as per \Cref{eq:B-dummy}). 
\end{itemize}

\item
The $(j+1)$-th local operation $S_{j+1}$ is applied. Note that this step is identical for both $H'_1$ and $H'_2$ as well.

\item
At this point, there are two cases to consider: 
\begin{enumerate}
\item \label[Case]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-1}
 $\Sim$ can make a $\downarrow$-query immediately, bringing the execution back to Layer-3; {\em or } 
\item \label[Case]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-2}
 $\Sim$ can rewind $\tilde{V}$ further, bringing the execution to Layer-1.  
\end{enumerate}
Fortunately, our proof (to appear shortly) can handle these two cases at one stroke. To do that, we denote the execution from this point until (exclusively) {\em the next $\downarrow$ query  from Layer-2 to Layer-3} (i.e., the exact query that yields the $k$-th arrival at Layer-3) as an operator $\Lambda$. $\Lambda$ might be the $(j+1)$-th local operator $S_{j+1}$ {\em only}, corresponding to \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-1}; $\Lambda$ might also be some non-identity operator, representing the operations performed in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-2} before the next arrival at Layer-3. We do not specify the exact form of $\Lambda$. But we high-light an important fact:
\begin{itemize}
 \item
 {\bf Fact:} for both \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-1,lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-2}, $\Lambda$ works non-trivially only on registers $\reg{p_1}$, $\reg{m}$, $\reg{t_1}$, $\reg{s}$, $\reg{u}$'s  \xiao{This is true because the execution between Layer-1 and Layer-2 have already been replaced with dummy up-and-downs, which involves only swapping operations between $\reg{m}$ and $\reg{t}_1$. Need to provide a detailed explanation of this fact. Importantly, $\Lambda$ does not touch $\reg{p_2}$, $\reg{t_2}$, and $\reg{w}$.}  (i.e., it works as identity on other registers). 
 \end{itemize} 

\item
Finally, an $\downarrow$-query is made, bringing the execution back to Layer-3. 
\begin{itemize}
\item
In $H'_1$, this corresponds to applying $\tilde{U}_6 \tilde{U}_5 \tilde{U}_4$;
\item
In $H'_2$, this corresponds to applying $B_{\msf{dmy}} \tilde{U}_4$. 
\end{itemize}
\end{enumerate}

It follows from the above description that the states $\ket{\phi^{(k)}}$ and $\ket{\psi^{(k)}}$ can be written as:
\begin{align}
\ket{\phi^{(k)}}
& = \tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \ket{\phi^{(k-1)}}, \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi}\\ 
\ket{\psi^{(k)}}
& = B_{\msf{dmy}}\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}} S_j \cdot \ket{\psi^{(k-1)}}. \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}
\end{align}

\begin{remark}[High-Level Idea for the Sequel]
Recall that our eventual goal is to prove that the states $\ket{\phi^{(k)}}$ and $\ket{\psi^{(k)}}$ defined above can indeed be written in the format shown in \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1,lem:LOCC-3ZK-hyb12:proof:target-format:H2} in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. At a high level, we will prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi,lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}. But we first need to perform some preparation work, putting \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi,lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}. Then, we show on \Cpageref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish} how to combine \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} and \Cref{lem:err-inv-com} to complete the proof for the induction step. 
\end{remark}



\begin{MyClaim}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}
There exist (potentially sub-normalized) pure states $\Set{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds
\begin{align}
\ket{\phi^{(k)}}
& = \tilde{U}_6 \tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}}   \tilde{U}^\dagger_5 \tilde{U}^\dagger_6
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(k)}}
& = 
B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}}  B^\dagger_{\msf{dmy}}
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} 
\end{align}
where $\Lambda^{\reg{p_2}/\reg{m}}$ is identical to $\Lambda$ except that it treats register $\reg{p_2}$ as $\reg{m}$, and the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}]
First, notice that
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:case-2:eq:swap-Lambda} 
\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 = \tilde{U}_4  \tilde{U}^\dagger_4 \Lambda^{\reg{p_2}/\reg{m}} = \Lambda^{\reg{p_2}/\reg{m}},
\end{equation}
where the first equality follows from the fact that $\Lambda^{\reg{p_2}/\reg{m}}$ does not operate on $\reg{p_2}$ and $\tilde{U}^\dagger_4$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_2}$.

\para{Proving \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(k)}}$:

\begin{align*}
\ket{\phi^{(k)}}
& = 
\tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \ket{\phi^{(k-1)}} \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1} \\
& = 
\tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} S_j \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1}  follows from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3} follows from \Cref{lem:LOCC-3ZK-hyb12:proof:case-2:eq:swap-Lambda}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  follows from the fact that $S_j$ works as identity on registers $\reg{p_1}$ and $\reg{p_2}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}), \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  follows from the definitions of $\tilde{U}_{6,1}$ and $S^{\reg{t_2}/\reg{m}}_j$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  follows from the fact that $S^{\reg{t_2}/\reg{m}}_j$ and $\tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} $ act non-trivially on different registers (see \Cref{LOCC-3ZK:table:non-trivial-registers}), and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  follows by defining
\begin{equation}
\label[Expression]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}
\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}} \coloneqq S_j \ket{\rho^{(k-1)}_{p_1, p_2}} ~~~\text{and}~~~ \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \coloneqq S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}~~~(\forall (p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}).
\end{equation}
\Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  finishes the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\para{Proving \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi}.} This proof is almost identical to the above proof for \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align*}
\ket{\psi^{(k)}}
& = 
B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \ket{\psi^{(k-1)}} \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} \\
& = 
B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1}  \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2} \\ 
& =
B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}} B^\dagger_{\msf{dmy}} \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} follows from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2}  follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} follows from a similar argument as we did to \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6} from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2}, and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4} follows from the same definition of $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$ and $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ as shown in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}

\Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}  finishes the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.


This eventually finishes the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\end{proof}


\para{Finishing the Induction Step.}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish} 
 With the above \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} in hand, we can finish the induction step by applying \Cref{lem:err-inv-com}. Formally, we apply \Cref{lem:err-inv-com} to the states and operators in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}, with the notation correspondence listed in \Cref{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}}
\label{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1}$, $\reg{p_2}$ & & $W_0$ & $\tilde{U}_{6,0}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_1$ & $\tilde{U}_{6,1}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_2}$ & & $W$   & $\tilde{U}_{6}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{t_1}$,  $\reg{u}$, $\reg{s}$ & & $\tilde{W}$ & $B_{\msf{dmy}}$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_0$ & $\tilde{U}_{5,0}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0} \\ 
\addlinespace[0.3em]
   & & & $U$   & $\tilde{U}_{5}$ & & $\ket{\eta^{(\msf{in})}_1}$ & \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}  \\ 
   \addlinespace[0.3em]
 &  & & $S$   & $\Lambda^{\reg{p_2}/\reg{m}}$ & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\phi^{(\msf{k})}}$  \\ 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\psi^{(\msf{k})}}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises of \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,0}$ (playing the role of $W_0$) who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$ (playing the role of registers $\reg{s}$).

\item
\Cref{lem:err-inv-com} requires that $W_1$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,1}$ (playing the role of $W_1$), who is a swap operator between registers $\reg{m}$ and $\reg{t_2}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively).

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_1$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $B_{\msf{dmy}}$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $\tilde{U}_{6,1}$ (playing the role of $W_1$) on branches $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, p'_2) \ne (p_1, p_2)$.

\item
 \Cref{lem:err-inv-com} requires that $U_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{5,0}$ (playing the role of $U_0$), who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of register $\reg{s}$).

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\Lambda^{\reg{p_2}/\reg{m}}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{p_2}$,  $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of registers $\reg{a}$ and $\reg{s}$).
\end{itemize}

Next, using the above notation, we could define
\begin{align}
\ket{\eta^{(\msf{in})}_0}
& \coloneqq 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}   \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{4,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}, \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0}  \\ 
\ket{\eta^{(\msf{in})}_1}
& \coloneqq 
 \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}.  \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}   
\end{align}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}) to the $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ defined in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0,lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}. This implies the existence of (potentially non-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1, p'_2}}}_{(p'_1, p'_2) \in\bits^\ell \times \bits^\ell}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\phi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k)}_{p'_1,p'_2}} \\ 
\ket{\psi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\rho^{(k)}_{p'_1,p'_2}} 
,\end{align*}
which are exactly \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1,lem:LOCC-3ZK-hyb12:proof:target-format:H2} in  \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. 

This finishes the induction step.


\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:sec}   together finish the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant} eventually.






\UpdateLine
    











==> sections/2-round-QCCC-xiao.tex <==
\section{Warm Up: Impossibility of Three-Round LOCC ZK}



In this section, we show as a warm-up example that three-round ZK in the LOCC model is impossible. This proof already illustrate the main ideas behind our general impossibility for the constant-round case. \xiao{It seems even such a result is not known yet.}






\subsection{The Model}

\subsubsection{Protocol Structure}
 We consider a three-round protocol where the prover $\Prover$ and verifier $\Verifier$ takes a statement $x \in \Lang$ and the security parameter $\secpar$ as the comment input. $\Prover$ additional takes a witness $w \in \Relation_\Lang(x)$ as the private input. $\Prover$ sends the first message $p_1$; $\Verifier$ responds with the second message $v_1$; then, $\Prover$ sends the final message $p_2$. W.l.o.g., we assume that all these massages are of the same length $\ell(\secpar)$, which is a polynomial in $\secpar$. Since we are in the LOCC model, the messages $(p_1, v_1, p_2)$ are all classical but both parties $\Prover$ and $\Verifier$ could perform local QPT operation.

\subsubsection{Honest Verifier} 
We are particularly interested in the verifier's algorithm. In the following, we formally define the behavior of the honest verifier $\Verifier$. We remark that what shown below is not the only way to model honest verifiers for LOCC ZK protocols. We define this particular model because it works the best with our proof of impossibility. Of course, our modeling is without loss of generality---It is straightforward to see that the honest verifier of any three-round LOCC ZK protocols can indeed be modeled in this way.
 

\subpara{$\Verifier$'s Registers.} $\Verifier$ starts by initializing the following registers (see \Cref{figure:2-LOCC-V:registers} for details):
\begin{equation}\label[Expression]{2-LOCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{p_1}}\ket{\vb{0}}_{\reg{v_1}}\ket{\vb{0}}_{\reg{p_2}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{0}_{\reg{d}} \ket{\vb{0}}_\reg{w} 
\end{equation}



\begin{FigureBox}[label={figure:2-LOCC-V:registers}]{Honest Verifier's Registers}
We explain the meaning of the registers defined in \Cref{2-LOCC:V:inital:expr}:
\begin{itemize}
    \item
    $\reg{ins}$ stores the input instance $x$;
\item
$\reg{p_1}$, $\reg{v_1}$, and $\reg{p_2}$ will be used to store the execution transcript (i.e., the messages $p_1$, $v_1$ and $p_2$ exchanged between the prover and verifier); As will become clear in our proof, storing these messages turns out to be critical for our proof to work.

\item
$\reg{m_1}$ and $\reg{m_2}$ is the register to store messages from/to the prove. (See our description of $\Verifier$'s behavior for more details.)

\item
$\reg{d}$ stores a single qubit that will be used to indicate if the verifier accepts (when it is $\ket{1}_\reg{d}$) or rejects (when it is $\ket{0}_\reg{d}$) at the end of the execution.


\item
$\reg{w}$ is the working space of the verifier initialized with enough ancilla qubits that will be used for purposes like purification and dilation etc.

\end{itemize}
% We emphasize that all of these registers need to be initialized to proper length. To simplify the notation, we do not specify the length of them. But it is easy to see that their length is bounded by a fixed polynomial of the security parameter, and this polynomial can be determined in advance. 
\end{FigureBox}

\subpara{$\Verifier$'s Unitaries.} In our three-round setting, $\Verifier$'s behavior is defined by five unitary operators $U_1$ $V_1$, $W_1$, $U_2$, $V_2$ (with some measurements) as explained below:\label{LOCC:3ZK:honest-V:unitaries}
\begin{itemize}
\item 
{\bf ($U_1$: receive $p_1$.)}
When a (potentially malicious) prover sends the round-1 message $p_1$, register $\reg{m_1}$ is overwritten by the $p_1$. Then, $\Verifier$ applies $U_1$, which is defined to be a swap operator between $\reg{m_1}$ and $\reg{p_1}$. 

\item
{\bf ($V_1$: generate $v_1$.)}
Next, $\Verifier$ applies $V_1$, which acts non-trivially only on registers $\reg{p_1}$, $\reg{v_1}$, $\reg{w}$. The purpose of this step is to generate $\Verifier$'s response to prover's first message. Note that we are in the LOCC setting. Thus, the response generated by $V_1$ (and stored in $\reg{v_1}$) is possibly a quantum state (instead of being only a classical string).

\item
{\bf ($W_1$: send $v_1$.)} $\Verifier$ applies $W_1$, which is defined to be a swap operator between $\reg{v_1}$ and $\reg{m_2}$ \xiao{This shouldn't be a swap. It should be a $\ket{v_2\xor m_2}_{\reg{m_2}}$}. Then, $\Verifier$ measures $\reg{m_2}$ in computational basis, collapsing its contents to a classical string $v_1$. This classical $v_1$ is sent to the prover as the round-2 message.

\item 
{\bf ($U_2$: receive $p_2$.)}
When the prover sends the round-3 message $p_2$, register $\reg{m_2}$ is overwritten by the $p_2$. Then, $\Verifier$ applies $U_2$, which is a swap operator between $\reg{m_2}$ and $\reg{p_2}$. 

\item
{\bf ($V_2$: final decision.)}
Next, $\Verifier$ applies $V_2$, which acts non-trivially only on registers $\reg{p_2}$, $\reg{d}$, $\reg{w}$. The purpose of this step is to generate $\Verifier$'s final decision in register $\reg{d}$. The $\reg{d}$ register is then measured in computational basis, indicating if $\Verifier$ accepts (if $\ket{1}_{\reg{d}}$) or rejects (if $\ket{0}_{\reg{d}}$).
\end{itemize}
This concludes the description of $\Verifier$'s behavior.



\subsubsection{Generic Malicious Verifier}
 Note that a malicious verifier $\tilde{\Verifier}$ could deviate arbitrarily from the above description of $\Verifier$, as long as its operation is QPT. To establish impossibility results, we need to formally model a generic malicious verifier $\tilde{\Verifier}$ as well. Again, there are multiple ways to do so and we choose the following one without loss of generality.

\para{$\tilde{\Verifier}$'s Registers.} It starts by initializing the following registers:
\begin{equation}\label[Expression]{2-LOCC:malicious-V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{\phi}_{\reg{o}},
\end{equation}
where
\begin{itemize}
\item
$\reg{ins}$ is a read-only register that stores the instance $x$; 
\item 
$\reg{o}$ stores $\tilde{\Verifier}$'s (non-uniform) poly-size quantum advice $\phi$ (together with enough ancilla qubits) and it will also be used as $\tilde{\Verifier}$'s working space throughout the execution; also,  {\bf part of $\reg{o}$ is designated as the output register $\reg{out}$}; 
\item
 $\reg{m_1}$ and $\reg{m_2}$ serves for the same purpose as when we define the honest $\Verifier$---Though $\tilde{\Verifier}$ could deviate from $\Verifier$, it has to present the same I/O interface to the honest prover, which is exact the purpose of $\reg{m_1}$ and $\reg{m_2}$ (see below for more detail).
\end{itemize}

\para{$\tilde{\Verifier}$'s Unitaries.} A generic $\tilde{\Verifier}$ can be specified by two unitary operators $\tilde{U}_1$ and $\tilde{U}_2$ as described below.


\begin{itemize}
\item 
{\bf ($\tilde{U}_1$: generate $v_1$.)}
When a prover sends the round-1 message $p_1$, register $\reg{m_1}$ is overwritten by the $p_1$. Then, $\tilde{\Verifier}$ applies $\tilde{U}_1$, which operates non-trivially on registers $\reg{ins}$, $\reg{m_1}$ and $\reg{o}$. The purpose of this step is to generate $\tilde{\Verifier}$'s response in registers $\reg{m_1}$. Again, since we are in the LOCC model, this response may be a quantum state (instead of being a classical string) when it is generated in $\reg{m_1}$. The $\reg{m_1}$ register is then be measured in the computational basis, yielding a classical string $v_1$. This classical $v_1$ is sent to the prover as the round-2 message.

\item
{\bf ($\tilde{U}_2$: final step.)} When the prover sends the round-3 message $p_2$, register $\reg{m_2}$ is overwritten by this $p_2$. Then, $\tilde{\Verifier}$ applies $\tilde{U}_2$, which operates non-trivially on registers $\reg{m_2}$ and $\reg{o}$. This step represents any QPT operations that $\tilde{\Verifier}$ would like to perform after receiving the last message of the protocol. (One may wonder why we do not allow $\tilde{U}_2$ to operate on $\reg{ins}$ and $\reg{m_1}$. Indeed, our definition of $\tilde{U}_1$ and $\tilde{U}_2$ already captures this possibility---One can think that the ``contents'' of $\reg{ins}$ and $\reg{m_1}$ have already been copied to some area of register $\reg{o}$ when $\tilde{U}_1$ was applied, so that $\tilde{U}_2$ can make use of them.)
\end{itemize}
This concludes the description of $\tilde{\Verifier}$'s behavior.


\begin{remark}[Honest Verifier as a Malicious One]
It is illustrative to show that the above model of $\tilde{\Verifier}$ indeed captures the honest verifier $\Verifier$ (i.e., a ``malicious'' verifier who does not cheat at all). This is straightforward to see as long as one realizes the following correspondence: When $\Verifier$ is viewed as $\tilde{\Verifier}$, its registers $\reg{p_1}$, $\reg{v_1}$, $\reg{p_2}$, $\reg{d}$, and $\reg{w}$ play the role of $\tilde{\Verifier}$'s $\reg{o}$; its operator $W_1V_1U_1$ plays the role of  $\tilde{\Verifier}$'s operator $\tilde{U}_1$; its operator $V_2U_2$ plays the role of  $\tilde{\Verifier}$'s operator $\tilde{U}_2$.
\end{remark}


\subsubsection{ZK Simulator}
 We now describe formally how the simulator $\Sim$ interacts with a generic malicious verifier $\tilde{\Verifier}$. Once again, there are multiple ways to do so and we choose the following one without loss of generality, which is particularly suitable for our proof of impossibility. In the following, we first provide a high-level explanation of $\Sim$'s behavior, and then present the formal description.

\para{High-Level Description.} Note that we focus on black-box simulation. Thus, $\Sim$ can only query $\tilde{\Verifier}$ via its unitaries ($\tilde{U}_1$ and $\tilde{U}_2$) and their inverse, but does not get to see the internal register $\reg{o}$ of $\tilde{\Verifier}$. Recall that $\reg{m_1}$ and $\reg{m_2}$ are used to exchange messages, and as explained above, they are always measured when the parties is about to send message in the real execution (as we are in the LOCC setting). However, for simulation, $\reg{m_1}$ and $\reg{m_2}$ are considered as being held by $\Sim$, who could choose {\em not} to measure them. 
% That is, $\Sim$ has the power to perform exponentially many executions in superposition.

$\Sim$ is granted oracle access to $\tilde{U}_1$, $\tilde{U}^\dagger_1$, $\tilde{U}_2$, and $\tilde{U}^\dagger_2$. We let $\Sim$ make use of a query register $\reg{u}$ in a 4-dimension Hilbert space spanned by the basis $\Set{ \ket{\downarrow_1}_{\reg{u}}, \ket{\uparrow_1}_{\reg{u}}, \ket{\downarrow_2}_{\reg{u}}, \ket{\uparrow_2}_{\reg{u}}}$. These basis corresponds to the four oracles respectively.

% Moreover, $\Sim$ can even make superposition queries to these oracles \xiao{change the model: we do not allow super-position queries}. To define this formally, 
% We let $\Sim$ make use of a query register $\reg{u}$ in a 4-dimension Hilbert space spanned by the basis $\Set{ \ket{\downarrow_1}_{\reg{u}}, \ket{\uparrow_1}_{\reg{u}}, \ket{\downarrow_2}_{\reg{u}}, \ket{\uparrow_2}_{\reg{u}}}$. Each oracle query of $\Sim$ could be in a superposition over $\reg{u}$. It suffices to describe the oracle's behavior on each basis state:
% \begin{itemize}
% \item
% When being queried on $\ket{\downarrow_1}_{\reg{u}}$, the oracle applies $\tilde{U}_1$ on the $\reg{m_1}$ register provided by $\Sim$ and $\tilde{\Verifier}$'s internal registers $\reg{o}$ and $\reg{ins}$. \xiao{remove the $\reg{ins}$ here. this is w.l.o.g.\ as a malicious adversary can keep a copy of $x$ as a part of its non-uniform advice.}
% \item
% When being queried on $\ket{\uparrow_1}_{\reg{u}}$, the oracle applies $\tilde{U}^\dagger_1$ on the $\reg{m_1}$ register provided by $\Sim$ and $\tilde{\Verifier}$'s internal registers $\reg{o}$ and $\reg{ins}$. \xiao{remove the $\reg{ins}$ here. this is w.l.o.g.\ as a malicious adversary can keep a copy of $x$ as a part of its non-uniform advice.}
% \item
% When being queried on $\ket{\downarrow_2}_{\reg{u}}$, the oracle applies $\tilde{U}_2$ on the $\reg{m_2}$ register provided by $\Sim$ and $\tilde{\Verifier}$'s internal registers $\reg{o}$.
% \item
% When being queried on $\ket{\uparrow_2}_{\reg{u}}$, the oracle applies $\tilde{U}^\dagger_2$ on the $\reg{m_1}$ register provided by $\Sim$ and $\tilde{\Verifier}$'s internal registers $\reg{o}$.
% \end{itemize}
% With the above understanding, 
Then, $\Sim$ can be defined by a local unitary operator $S$ that works on $\Sim$'s internal register and registers $\reg{u}$, $\reg{m_1}$, and $\reg{m_2}$. $\Sim$'s behavior is nothing but  iterations of the following three steps:
\begin{itemize}
\item
Apply the local operator $S$;
\item
Measure the $\reg{u}$ register to learn the type of the next query. \xiao{Need to explain the correspondence.}
\item
Make the oracle query according to the measurement result from the last step.
\end{itemize}

% \footnote{The current model seems to ignore the measurements that $\Sim$ may want to perform during the execution. But this is not a problem as we can take a purified point of view by adding enough ancilla qubits and deferring all the intermediate measurements to the end of the execution.}


What we have presented so far is already a complete description of the ZK simulator. However, we actually need to modify this simulator a little bit, to obtain a functionally equivalent $\Sim$ with some additional ``structures,'' which will ease the presentation of our proof of impossibility. Roughly, we need to ask $\Sim$ to ``keep a record'' of all the oracle queries she made. This is for a technical purpose that will become clear later when we show the proof. But at a high level, this is because our proof technique relies on a ``branch-wise'' analysis for all possible ``execution branches.'' \xiao{(see xxx and xxx for more details.)}

We now describe the modifications. We assume that $\Sim$ makes at most $q(\secpar)$ oracle queries in total, where $q(\cdot)$ is a polynomial in $\secpar$. Instead of using a single $\reg{u}$ register, we let $\Sim$ make use of $q$ query registers $\reg{u_1}, \ldots, \reg{u_q}$, one for each query. Additionally, we label the local operator $S$ that $\Sim$ performs between adjacent queries as $(S_1, \ldots, S_q)$. Roughly, for each $j \in [q]$, $\Sim$ first executes $S_j$ to determine the type (i.e., $\downarrow_1$, $\uparrow_1$, $\downarrow_2$, or $\uparrow_2$) for the $j$-th oracle query, and store the type (possibly in superposition) in register $\reg{u_j}$. Next, the registers $\reg{u_j}$ is measured, resulting in a classical symbol from $\Set{\downarrow_1,\uparrow_1,\downarrow_2,\uparrow_2}$ indicating the type of the next oracle query. Then, this query is answered according to the contents of $\reg{u_j}$. Next, $\Sim$ continue to execute $S_{j+1}$ and make the $(j+1)$-th query, and so on. We remark that register $\reg{u_j}$ is used as the control register for the $j$-th oracle query only; after that, no future operation will touch upon it anymore. This point will become important for our proof later.




With the above intuitive explanation, we are now ready to present the formal description of $\Sim$. 

\para{$\Sim$'s Registers.} For a fixed polynomial $q(\secpar)$, a $q$-query simulator $\Sim$ starts by initializing the following state (shown along with $\tilde{\Verifier}$'s internal registers):
\begin{equation}\label{2-LOCC:S:inital:expr}
\ket{\eta_0} \coloneqq \ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{\phi}_{\reg{o}} \ket{\downarrow_1}_{\reg{u_1}} \ldots \ket{\downarrow_1}_{\reg{u_q}} \ket{\rho}_{\reg{s}},
\end{equation}
Compared with \Cref{2-LOCC:malicious-V:inital:expr}, the RHS of \Cref{2-LOCC:S:inital:expr} includes the following extra registers: 
\begin{itemize}
\item
A register $\reg{s}$ containing the (non-uniform) poly-size quantum advice $\rho$ of $\Sim$, which we can assume w.l.o.g.\ is pure. This register also contains enough ancilla qubits so that it will be used as $\Sim$'s internal working space throughout the execution.
\item
Another $q$ registers $\reg{u_1} \ldots \reg{u_q}$ initialized to the $\downarrow_1$ symbol. As explained previously, the $\reg{u_j}$'s will be used by $\Sim$ to determine the type of the $j$-th query. 
% We also provide more details below while describing $\Sim$'s behavior.
\end{itemize}




\para{$\Sim$'s Behavior.} 
\begin{xiaoenv}{}
Start with the intermediate measurement. And then say that all the measurements on $\reg{u_j}$'s can be deferred, because a consequence of deferred measurement principle is:
\begin{quote}
{\em If after a measurement a qubit is used as a control qubit only, then the
measurement can be deferred.}
\end{quote}
\end{xiaoenv}
The behavior of a  $q$-query simulator can be described as follows. For $j \in [q]$, 
\begin{itemize}
\item
Apply the local unitary $S_j$. $S_j$ is a unitary that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$; Intuitively, it represents the local operation $\Sim$ performs between two oracle queries. In particular, it computes and stores the type of the $j$-th query in register $\reg{u_j}$, possibly in superposition.
\item
Measure $\reg{u_j}$;
\item
Make the $j$-th oracle query according to the measurement outcome from the last step. Formally, we define this step as a unitary$O_{j}$ that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$ and $\reg{o}$. We present the formal definition of $O_{j}$ in \Cref{figbox:LOCC:3ZK:oracle}.
\end{itemize}


\begin{FigureBox}[label={figbox:LOCC:3ZK:oracle}]{Description of Unitary $O_j$}
Each $O_j$ can be understood as unitary controlled on register $\reg{u_j}$. Formally, for each $j \in [q]$, $O_j$ is defined as follows 
\begin{itemize}
\item
If $\reg{u_j}$ is of the form $\ket{\downarrow_1}_{\reg{u_j}}$, it applies $\tilde{U}_1$ on $\reg{m_1}$ and $\reg{o}$.
\item
If $\reg{u_j}$ is of the form $\ket{\uparrow_1}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_1$ on $\reg{m_1}$ and $\reg{o}$.
\item
If $\reg{u_j}$ is of the form $\ket{\downarrow_2}_{\reg{u_j}}$, it applies $\tilde{U}_2$ on $\reg{m_2}$ and $\reg{o}$.
\item
If $\reg{u_j}$ is of the form $\ket{\uparrow_2}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_2$ on $\reg{m_2}$ and $\reg{o}$.
\end{itemize}
\end{FigureBox}

% is defined by a sequence of $q$ unitary operators $\Set{S_1,  \ldots, S_q}$. It proceeds as follows:
% \begin{itemize}
% \item
% {\bf (First $q$ queries)} For $j\in [q]$, $\Sim$ repeats the following steps:
% \begin{itemize}
%  \item
%  $\Sim$ first applies the ``local'' unitary $S_j$, which operates non-trivially on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$. 
%  \item
%  Then, controlled on the query type (possibly in superposition) stored in $\reg{u_j}$, the corresponding unitary is applied according to the rule described in \Cref{figbox:LOCC:3ZK:oracle}.
%  \end{itemize} 

% \item
% {\bf (Final output.)} We denote by $\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho)$ the above execution; We denote by $\OUT(\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho))$ the output of $\tilde{\Verifier}$, i.e., final state in $\reg{out}$ tracing out all other registers after the execution
% \end{itemize}
\xiao{add a remark explaining two things: (1) $S_{j}$ only need to work on $\reg{u}_j$ and does not touch other $\reg{u}$ registers; (2) There's no need to add $S_{q+1}$ for $\Sim$'s post-processing, as the output will anyway trace $\Sim$'s registers out.}


\subpara{$\Sim$ with Deferred Measurements.} Recall that a consequence of the deferred measurement principle is that {\em If after a measurement a qubit is used as a control qubit only, then the measurement can be deferred.} Also, observe in the above description of $\Sim$'s behavior that each $\reg{u_j}$ register is used {\em only} as a controlled register to determine the type of $O_j$. Thus, by the deferred measurement principle, we can equivalently describe $\Sim$ as the following two steps (assuming the starting state is $\ket{\eta_0}$):
\begin{enumerate}
\item
Compute $\ket{\eta_q} \coloneqq O_q S_q O_{q-1} S_{q-1} \cdots O_1 S_1\cdot \ket{\eta_0}$.
\item
Measure registers $\reg{u_1},\ldots, \reg{u_q}$.
\end{enumerate}
From now on, we will use this deferred-measurement description of the simulator $\Sim$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comment some old materials
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% At a high-level, $\Sim$ can run $\tilde{\mathcal{V}}$ as a real prover, i.e., sending a message to $\tilde{\Verifier}$ and expecting $\tilde{\Verifier}$'s response (dubbed as ``down-queries''), or rewind $\tilde{\Verifier}$ (dubbed ``up-queries''). In the following, we formally define $\Sim$'s behavior. We also show in \Cref{figure:Sim-query:3-round} an exemplary execution of $\Sim$ where she makes 17 queries in total. We find it helpful to trace this concrete example while trying to understand the behavior of $\Sim$.
% \begin{figure}[!thb]
% \centering{
%     \fbox{
%          \includegraphics[width=0.5\textwidth]{figures/Three-round-real.jpg}
%     }         
% }
% \caption{An exemplary Query Pattern of $\Sim$}
% \label{figure:Sim-query:3-round}
% \end{figure}

% \subpara{Initialize $p_1$:} $\Sim$ starts by preparing a state in register $\reg{m_1}$ as her first message $p_1$. Formally, $\Sim$ applies a ``local'' unitary $S_0$ that works non-trivially on register $\reg{m_1}$ and $\reg{s}$. This yields a quantum state $p_1$ in $\reg{m_1}$ together with some residual internal state of $\Sim$ in $\reg{s}$. 


% \subpara{Obtain $v_1$:} $\Sim$ then queries $\tilde{\Verifier}$ to learn the response $v_1$. Formally, $\tilde{V}$ applies the unitary $\tilde{U}_3\tilde{U}_2\tilde{U}_1$ as defined earlier, which yields a state $v_1$ in register $\reg{m_1}$. This step is illustrated as the $\downarrow$ labeled by $\circled{1}$ in \Cref{figure:Sim-query:3-round}, and we say that the execution moves from Layer-1 to Layer-2.\footnote{It is worth noting that although both $p_1$ and $v_1$ are classical strings in the real execution, the simulator $\Sim$ may put a quantum state in $\reg{m_1}$ as her first message, and in that case, $\tilde{V}$'s response $v_1$ may also be a quantum state.} 


% \subpara{Subsequent Queries:} From now on, $\Sim$ can freely ask $\tilde{V}$ to perform $\tilde{U}$ or $\tilde{U}^\dagger$, and may modify the contains of $\reg{m_1}$ and $\reg{m_2}$ in between using her unitaries $S_1$, $S_2$, and $S_3$. Formally, $\Sim$ repeats the following procedure
% \begin{itemize}
% \item
% if the execution reaches Layer-$i$ (for $i \in [3]$), $\Sim$ will first apply the unitary $S_i$, and then measure the single-qubit register $\reg{q}$ \xiao{add this register when explaining $\Sim$'s registers} to decide if she wants to make a $\tilde{U}$ query or a $\tilde{U}^\dagger$ query. Depending on the query made, the execution will either move to Layer-$(i-1)$ (if a $\tilde{U}^\dagger$ query is made) or Layer-$(i+1)$ (if a $\tilde{U}$ query is made). 

% W.l.o.g., we use the following conventions. When the execution is at Layer-1 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\uparrow}$, then $\Sim$ aborts the execution immediately. Intuitively, this is because the execution is already rewound to the very beginning and it does not make sense to rewind it further; we simply view this as a failed simulation. Also, when the execution is at Layer-3 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\downarrow}$, then $\Sim$ terminates and announces the end of the simulation. Intuitively, Layer-3 represents the very end of the protocol and it does not make sense to continue to the next round; we simply view this as $\Sim$'s signal for the end of the simulation.
% \end{itemize}
% This procedure is best understood by tracing the example shown in \Cref{figure:Sim-query:3-round}. Consider the status of the execution right after the arrow $\circled{1}$. $\Sim$ then applies $S_2$ on $\reg{m_1}$ and $\reg{s}$ \xiao{probably on $\reg{m_2}$ as well?}, and measures $\reg{d}$. The situation shown in  \Cref{figure:Sim-query:3-round} corresponds to $\Sim$ decides to make a $\tilde{U}^\dagger$-query next (represented by arrow $\circled{2}$), which brings the execution back to Layer-1. $\Sim$ then applies $S_1$ on $\reg{m_1}$ and $\reg{s}$, and measures $\reg{d}$. By the assumption made above, $\Sim$ will make a $\tilde{U}$-query next, which brings the execution to Layer-2 (represented by arrow $\circled{3}$). 

% Another set of queries that deserve a closer look is from arrow $\circled{11}$ to arrow $\circled{12}$. They represent the following steps: Right after the $\tilde{U}$-query labeled by $\circled{10}$, $\Sim$ applies $S_3$ on $\reg{m_2}$ and $\reg{s}$, measures $\reg{q}$, and decides to make the  $\tilde{U}^\dagger$-query labeled by $\circled{11}$. This brings the execution to Layer-2. Then, $\Sim$ further rewinds the execution back to Layer-1 and ``jumps'' between Layer-1 and Layer-2 twice (as represented by arrow $\circled{12}$ to arrow $\circled{15}$). After that, $\Sim$ decides to go to Layer-3 as represented by arrow $\circled{16}$, which is the last query made by $\Sim$. That is, after applying $\circled{16}$, the measurement of $\reg{q}$ returns $\ket{\downarrow}$, indicating the end of the execution as we explained above. 


\subsection{Theorem Statement and Proof Outline}

\xiao{to do... As the title of the subsection indicates..}



\subsection{Branch-Wise Equivalence suffices}
\label{sec:branch-wise:equiv}

\begin{xiaoenv}{Necessary Definitions}
\begin{itemize}
\item
Define {\em query patterns}. Denote by $\msf{Pat}$ It is a classical sequence $\vec{u} = (u_1, \ldots, u_q)$ where for all $j \in [q]$, $u_j \in \Set{\downarrow_1, \uparrow_1, \downarrow_2, \uparrow_2}$.
\item
Define {\em admissible patterns}. Denote by $\msf{aPat}$. It is a query pattern satisfies the following property: If we trace the pattern, we stop at the end of the protocol.
\item
Define {\em inadmissible patterns}. Denote by $\msf{iPat}$. It is $\msf{Pat} \setminus \msf{aPat}$.
\end{itemize}
\end{xiaoenv}


Let $\dot{U}_1$ be a unitary that operates non-trivially on $\reg{m_1}$ and $\reg{o}$; Let $\dot{U}_2$ be a unitary that operates non-trivially on $\reg{m_2}$ and $\reg{o}$; Define the following sequence of $q$ unitary operators $\Set{\dot{O}_1, \ldots, \dot{O}_q}$ as shown in \Cref{figbox:LOCC:3ZK:dot-oracle}.
\begin{FigureBox}[label={figbox:LOCC:3ZK:dot-oracle}]{Description of Unitary $\dot{O}_j$}
Similar as the $O_j$'s defined in \Cref{figbox:LOCC:3ZK:oracle}, each $\dot{O}_j$ can be also understood as unitary controlled on register $\reg{u_j}$. Formally, for each $j \in [q]$, $\dot{O}_j$ is defined as follows 
\begin{itemize}
\item
If $\reg{u_j}$ is of the form $\ket{\downarrow_1}_{\reg{u_j}}$, it applies $\dot{U}_1$ on $\reg{m_1}$ and $\reg{o}$.
\item
If $\reg{u_j}$ is of the form $\ket{\uparrow_1}_{\reg{u_j}}$, it applies $\dot{U}^\dagger_1$ on $\reg{m_1}$ and $\reg{o}$.
\item
If $\reg{u_j}$ is of the form $\ket{\downarrow_2}_{\reg{u_j}}$, it applies $\dot{U}_2$ on $\reg{m_2}$ and $\reg{o}$.
\item
If $\reg{u_j}$ is of the form $\ket{\uparrow_2}_{\reg{u_j}}$, it applies $\dot{U}^\dagger_2$ on $\reg{m_2}$ and $\reg{o}$.
\end{itemize}
\end{FigureBox}

Consider the two games shown in \Cref{table:LOCC-3ZK:branch-wise:lem}, where the difference is high-lightened in \red{red color}:
\begin{table}
\begin{center}
\caption{\purple{need a good title}}
\label{table:LOCC-3ZK:branch-wise:lem}
\begin{tabular}{|c|c|}
\hline
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $G_0(\ket{\eta_0})$:}
    \begin{enumerate}
    \item \label[Step]{table:LOCC-3ZK:branch-wise:lem:G0:1}
    Compute $\ket{\eta_q} = O_q S_q O_{q-1} S_{q-1} \cdots O_1 S_1\cdot \ket{\eta_0}$;
    \item
    Measure  $\reg{u_1} \ldots \reg{u_1}$ to obtain a classical string $\vec{u}'$;
    \item
    Measure $\reg{d}$ to obtain a classical bit $d$.
    \item
    Output $1$ iff $\vec{u}' \in \msf{aPat}$ and $d = 1$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage} 
        &~
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $G_1(\ket{\eta_0})$:}
    \begin{enumerate}
    \item \label[Step]{table:LOCC-3ZK:branch-wise:lem:G1:1}
    Compute $\red{\ket{\dot{\eta}_q}} = \red{\dot{O}_q} S_q \red{\dot{O}_{q-1}} S_{q-1} \cdots \red{\dot{O}_1} S_1\cdot \ket{\eta_0}$;
    \item
    Measure  $\reg{u_1} \ldots \reg{u_1}$ to obtain a classical string $\vec{u}'$;
    \item
    Measure $\reg{d}$ to obtain a classical bit $d$.
    \item
    Output $1$ iff $\vec{u}' \in \msf{aPat}$ and $d = 1$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage}\\
\hline
\end{tabular}
\end{center}
\end{table}


We now set up more notations. For any $u \in\Set{\downarrow_1, \uparrow_1, \downarrow_2, \uparrow_2}$, define two unitary operators $Q_u$ and $\dot{Q}_u$ as follows:
\begin{equation}\label{eq:LOCC-3ZK:branch-wise:def:Q-dot-Q}
Q_u \coloneqq 
\begin{cases}
\tilde{U}_1 & \text{if}~u = \downarrow_1 \\ 
\tilde{U}^\dagger_1 & \text{if}~u = \uparrow_1 \\
\tilde{U}_2 & \text{if}~u = \downarrow_2 \\ 
\tilde{U}^\dagger_2 & \text{if}~u = \uparrow_2 
\end{cases},
~~\text{and}~~
\dot{Q}_u \coloneqq 
\begin{cases}
\dot{U}_1 & \text{if}~u = \downarrow_1 \\ 
\dot{U}^\dagger_1 & \text{if}~u = \uparrow_1 \\
\dot{U}_2 & \text{if}~u = \downarrow_2 \\ 
\dot{U}^\dagger_2 & \text{if}~u = \uparrow_2 
\end{cases}.
\end{equation}
From \Cref{eq:LOCC-3ZK:branch-wise:def:Q-dot-Q}, it is straightforward to see that for all $j \in[q]$, 
\begin{align}
O_j 
& = \sum_{u_j \in \Set{\downarrow_1, \uparrow_1, \downarrow_2, \uparrow_2}} \ketbra{u_j}_{\reg{u_j}} \tensor Q_{u_j}, ~\text{and} \label{eq:LOCC-3ZK:branch-wise:def:O-Q} \\ 
\dot{O}_j 
&= 
\sum_{u_j \in \Set{\downarrow_1, \uparrow_1, \downarrow_2, \uparrow_2}} \ketbra{u_j}_{\reg{u_j}} \tensor \dot{Q}_{u_j}. \label{eq:LOCC-3ZK:branch-wise:def:dot-O-Q}
\end{align}

For any $\vec{u} = (u_1, \ldots, u_q)\in\msf{Pat}$, we define two ``pattern-wise'' games $H_0(\vec{u}, \ket{\eta_0})$ and $H_1(\vec{u}, \ket{\eta_0})$ in \Cref{table:LOCC-3ZK:branch-wise:lem:pattern-wise}.

\begin{table}
\begin{center}
\caption{\purple{need a good title}}
\label{table:LOCC-3ZK:branch-wise:lem:pattern-wise}
\begin{tabular}{|c|c|}
\hline
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $H_0(\vec{u}, \ket{\eta_0})$:}
    \begin{enumerate}
    \item 
        Parse $\vec{u}$ as $(u_1, \ldots, u_q)$;
    \item \label[Step]{table:LOCC-3ZK:branch-wise:lem:H0:2}
    Compute $\ket{\eta^{\vec{u}}_q} = Q_{u_q} S_q \cdots Q_{u_1} S_1\cdot \ket{\eta_0}$;
    \item
    Measure  $\reg{u_1} \ldots \reg{u_q}$ to obtain a classical string $\vec{u}'$;
    \item
    Measure $\reg{d}$ to obtain a classical bit $d$.
    \item
    Output $1$ iff $\vec{u}'=\vec{u}$ and $d = 1$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage} 
        &~
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $H_1(\vec{u}, \ket{\eta_0})$:}
    \begin{enumerate}
    \item 
        Parse $\vec{u}$ as $(u_1, \ldots, u_q)$;
    \item \label[Step]{table:LOCC-3ZK:branch-wise:lem:H1:2}
    Compute $\red{\ket{\dot{\eta}^{\vec{u}}_q}} = \red{\dot{Q}_{u_q}} S_q \cdots \red{\dot{Q}_{u_1}} S_1\cdot \ket{\eta_0}$;
    \item
    Measure  $\reg{u_1} \ldots \reg{u_q}$ to obtain a classical string $\vec{u}'$;
    \item
    Measure $\reg{d}$ to obtain a classical bit $d$.
    \item
    Output $1$ iff $\vec{u}'=\vec{u}$ and $d = 1$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage}\\
\hline
\end{tabular}
\end{center}
\end{table}


Now, we are ready to show the branch-wise equivalence lemma

\xiao{delete this lemma}
\begin{lemma}[Branch-wise Equivalence]\label{lem:branch-wise:equiv:false}
Let $\ket{\eta_0}$ be as in \Cref{2-LOCC:S:inital:expr}. To prove that 
 $$\OUT(G_0(\ket{\eta_0})) \idind \OUT(G_1(\ket{\eta_0})),$$ 
 it suffices to prove that 
$$\forall \vec{u} \in \msf{aPat}, ~ \OUT(H_0(\vec{u}, \ket{\eta_0})) \idind \OUT(H_1(\vec{u}, \ket{\eta_0})).$$
\end{lemma}
\begin{proof}
 In the following, we use $\reg{u}$ to denote the concatenation of registers $\reg{u_1}, \ldots, \reg{u_q}$. For each $\vec{u} = (u_1, \ldots, u_q) \in \msf{Pat}$, we use $\ket{\vec{u}}_{\reg{u}}$ as an abbreviation for $\ket{u_1}_{\reg{u_1}}\ldots\ket{u_q}_{\reg{u_q}}$, and $\ketbra{\vec{u}}_{\reg{u}}$ denote the projector that projects each $\reg{u_j}$ to $u_j$, i.e.,
 $$\ketbra{\vec{u}}_{\reg{u}} \coloneqq \ketbra{u_1}_{\reg{u_1}}\tensor \ketbra{u_2}_{\reg{u_2}} \tensor \ldots \tensor \ketbra{u_q}_{\reg{u_q}}.$$

First, we claim that to prove \Cref{lem:branch-wise:equiv:false}, it suffices to prove the following equations
\begin{align}
& \forall \vec{u} \in \msf{aPat}, ~\ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\eta_q} = \ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\eta^{\vec{u}}_q}, ~\text{and} \label{lem:branch-wise:equiv:eq:goal:1} \\ 
& \forall \vec{u} \in \msf{aPat}, ~\ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\dot{\eta}_q} = \ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\dot{\eta}^{\vec{u}}_q}, \label{lem:branch-wise:equiv:eq:goal:2}
,\end{align}
where $\ket{\eta_q}$ is the state obtained in \Cref{table:LOCC-3ZK:branch-wise:lem:G0:1} of $G_0(\ket{\eta_0})$, $\ket{\eta^{\vec{u}}_q}$ is the state obtained in \Cref{table:LOCC-3ZK:branch-wise:lem:H0:2} of $H_0(\vec{u}, \ket{\eta_0})$,
 $\ket{\dot{\eta}_q}$ is the state obtained in \Cref{table:LOCC-3ZK:branch-wise:lem:G1:1} of $G_1(\ket{\eta_0})$, and $\ket{\dot{\eta}^{\vec{u}}_q}$ is the state obtained in \Cref{table:LOCC-3ZK:branch-wise:lem:H1:2} of $H_1(\vec{u}, \ket{\eta_0})$. This is straightforward to see as long as one notices that the $\reg{u}$ register is measured at the end of these games and that the inadmissible patterns (i.e., $\vec{u} \in \msf{iPat}$) do not contribute to the success (i.e., outputting 1) probability. 

To prove \Cref{lem:branch-wise:equiv:eq:goal:1}, consider an (arbitrarily) fixed $\vec{u} \in \msf{aPat}$:
\begin{align*}
\ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\eta_q} 
&= 
\ketbra{\vec{u}}_{\reg{u}} \cdot 
\bigg(
\sum_{\vec{u}' \in \msf{Pat}} \ketbra{\vec{u}'}_{\reg{u}} \cdot \ket{\eta_{q}}
\bigg) \numberthis \label{lem:branch-wise:equiv:eq:derive:1}\\ 
& =
\ketbra{\vec{u}}_{\reg{u}} \cdot 
\bigg(
\sum_{\vec{u}' \in \msf{Pat}} \ketbra{\vec{u}'}_{\reg{u}} \cdot O_qS_q\cdots O_1S_1 \cdot \ket{\eta_{0}}  
\bigg) \numberthis \label{lem:branch-wise:equiv:eq:derive:2} \\ 
& = 
\ketbra{\vec{u}}_{\reg{u}} \cdot 
\bigg(
\sum_{\vec{u}' \in \msf{Pat}} \big(\ketbra{u'_q}_{\reg{u_q}} \cdot O_q \big) S_q  \cdots \big(\ketbra{u'_1}_{\reg{u_1}} \cdot O_1 \big) S_1 \cdot \ket{\eta_{0}}  
\bigg) \numberthis \label{lem:branch-wise:equiv:eq:derive:3} \\ 
& =
\ketbra{\vec{u}}_{\reg{u}} \cdot 
\bigg(
\sum_{\vec{u}' \in \msf{Pat}} \big(\ketbra{u'_q}_{\reg{u_q}} \tensor Q_{u'_q} \big) S_q  \cdots \big(\ketbra{u'_1}_{\reg{u_1}} \tensor Q_{u'_1} \big) S_1 \cdot \ket{\eta_{0}} 
\bigg) \numberthis \label{lem:branch-wise:equiv:eq:derive:4} \\ 
& = 
\ketbra{\vec{u}}_{\reg{u}} \cdot 
\bigg(
\sum_{\vec{u}' \in \msf{Pat}} \ketbra{\vec{u}'}_{\reg{u}} \cdot Q_{u'_q} S_q\cdots Q_{u'_1}S_1 \cdot \ket{\eta_{0}} 
\bigg) \numberthis \label{lem:branch-wise:equiv:eq:derive:5} \\ 
& = 
\ketbra{\vec{u}}_{\reg{u}} \cdot 
\bigg(
\sum_{\vec{u}' \in \msf{Pat}} \ketbra{\vec{u}'}_{\reg{u}} \cdot \ket{\eta^{\vec{u}'}_q}
\bigg) \numberthis \label{lem:branch-wise:equiv:eq:derive:6} \\ 
& = 
\ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\eta^{\vec{u}}_q}
,\end{align*}
where \Cref{lem:branch-wise:equiv:eq:derive:1} follows from the identity $\sum_{\vec{u}' \in \msf{Pat}} \ketbra{\vec{u}'}_{\reg{u}} = I$, \Cref{lem:branch-wise:equiv:eq:derive:2} follows from \Cref{table:LOCC-3ZK:branch-wise:lem:G0:1} of $G_0(\ket{\eta_0})$, \Cref{lem:branch-wise:equiv:eq:derive:3} follows from the fact that neither $O_j$ nor $S_j$ operates on register $\reg{u_i}$ with $i < j$, \Cref{lem:branch-wise:equiv:eq:derive:4} follows from \Cref{eq:LOCC-3ZK:branch-wise:def:O-Q}, \Cref{lem:branch-wise:equiv:eq:derive:5} follows from the fact that neither $Q_{u'_j}$ nor $S_j$ operates on register $\reg{u_i}$ with $i < j$, \Cref{lem:branch-wise:equiv:eq:derive:6} follows from \Cref{table:LOCC-3ZK:branch-wise:lem:H0:2} of $H_0(\vec{u}', \ket{\eta_0})$.

\Cref{lem:branch-wise:equiv:eq:goal:2} can be established using almost the identical derivation as for \Cref{lem:branch-wise:equiv:eq:goal:1}. Thus, we omit the details.

This concludes the proof of \Cref{lem:branch-wise:equiv:false}.
\end{proof}



\xiao{Indeed, what I need is not the above \Cref{lem:branch-wise:equiv:false}. It should be the following \Cref{lem:branch-wise:equiv} (but the above proof already shows the following lemma). To do: delete the above \Cref{lem:branch-wise:equiv:false} and show the following \Cref{lem:branch-wise:equiv}
 instead. Moreover, in that case, \Cref{table:LOCC-3ZK:branch-wise:lem:pattern-wise} can simply appear as an intermediate step in the security proof.}


\xiao{I think the current version of \Cref{lem:branch-wise:equiv} (or \Cref{lem:branch-wise:equiv:false}) is not accurate. The game should be directly defined as ``measuring the first query jumping form Layer-$i$ to Layer-$(i+1)$.'' We need a branch-wise lemma (i.e., for each possible $\vb{u}$ pattern determined by $\Sim$ dynamically) in this ``final'' game to connect real and dummy.}

\begin{lemma}[Branch-wise Equivalence]\label{lem:branch-wise:equiv}
Let $\ket{\eta_0}$ be as in \Cref{2-LOCC:S:inital:expr}. To prove that 
 $$\OUT(G_0(\ket{\eta_0})) \idind \OUT(G_1(\ket{\eta_0})),$$ 
it suffices to prove the following equation
\begin{equation}\label{lem:branch-wise:equiv:eq} 
\forall \vec{u} \in \msf{aPat}, ~\ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\eta^{\vec{u}}_q} = \ketbra{\vec{u}}_{\reg{u}} \cdot \ket{\dot{\eta}^{\vec{u}}_q}, 
\end{equation}
where $\ket{\eta^{\vec{u}}_q}$ is the state obtained in \Cref{table:LOCC-3ZK:branch-wise:lem:H0:2} of $H_0(\vec{u}, \ket{\eta_0})$, and $\ket{\dot{\eta}^{\vec{u}}_q}$ is the state obtained in \Cref{table:LOCC-3ZK:branch-wise:lem:H1:2} of $H_1(\vec{u}, \ket{\eta_0})$. \xiao{Note that it is generally false that $\ket{\eta^{\vec{u}}_q} = \ket{\dot{\eta}^{\vec{u}}_q}$.}
\end{lemma}

\UpdateLine







\subsection{A Particular Malicious Verifier}
\label{sec:particular-mal-V}




\xiao{may need to explain the high-level picture: why are we defining $\tilde{V}$?} Similar as \cite{FOCS:CCLY21}, we first show the impossibility result with an inefficient $\tilde{V}$. The inefficiency is only due to a random function $H$ hard-wired in $\tilde{V}$. Jumping ahead, we will make $\tilde{V}$ efficient later (\xiao{Cref to sec}) by replacing $H$ with a $q$-wise independent hash.

$\tilde{V}$ starts by initializing the following registers (see \Cref{figure:2-LOCC-V:registers} for an explanation):
\begin{equation}\label[Expression]{2-LOCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{p_1}}\ket{\vb{0}}_{\reg{v_1}}\ket{\vb{0}}_{\reg{p_2}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{\bot}_{\reg{tmp}} \ket{0}_{\reg{d}} \ket{\vb{0}}_\reg{w} \ket{H}_{\reg{aux}} 
\end{equation}








% In the impossibility result, we construct a BQP algorithm that runs both the simulator $\simulator$ and verifier $V$.
% Our entire purified view therefore consists of all above registers $\reg{ins, a,b,m,aux,w,adv}$. 


\para{$\tilde{V}$'s Unitary.}  

\begin{xiaoenv}{Add counter register}
Importantly, we ask $V$ to explicitly maintain a $\reg{Count}$ register, initialized to $1$. This register will memorize which round the execution is currently at. Importantly, the value in $\reg{Count}$ will decide the length of preamble $\reg{p_1}, \reg{p_2}, ...$ to query $H$ on. 
 
(This step need to be inserted between \Cref{item:Vtil:unitary:1,item:Vtil:unitary:2} below.) On each Sim/$P$ query, $V$ will first query the $H$ to decide whether to response. If $H$ outputs 1, then $V$ will increase $\reg{Count}$ by 1, and then proceed to the following unitary operations. Otherwise, $V$ does nothing (technically, I think we still swap the $\reg{m}$ and $\reg{tmp}$ register.).  

Note that this is different from CCLY, where the $\reg{Count}$ will always increase upon a query. What we did here is to ensure that in the MnR game with $H_0$, $Sim$ won't skip a round (i.e., cannot see the $(i+1)$-th round unless the $i$-th round message is measured out.) this property is crucial. It allows me to focus on the layer diagram I'm currently using.
\end{xiaoenv}


We next describe the unitary $\tilde{U}$ for $\tilde{V}$, which consists of the following sub-unitaries:
\begin{enumerate}
\item \label{item:Vtil:unitary:1}
{\bf ($\tilde{U}_1$: Swap $\reg{p_1}$ and $\reg{m_1}$.)} Upon receiving the first-round message $p_1$ in register $\reg{m_1}$, $\tilde{V}$ first swaps the contents of $\reg{p_1}$ and $\reg{m_1}$ registers.
\begin{MyComment}
In the real execution, this steps is for $\tilde{V}$ to move the first message it received from the prover (in the $\reg{m_1}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_1}$), so that it can perform computation in subsequent steps.
\end{MyComment}

\item \label{item:Vtil:unitary:2}
{\bf ($\tilde{U}_2$: Apply $V$'s Unitary.)}
It proceeds as follows: 
\begin{enumerate}
\item
If $H(p_1) = 0$, then do nothing; \xiao{need to recall where $p_1$ is stored.}
\item
If $H(p_1) = 1$, then apply $U$, where recall that $U = \sum_{p_1} \ketbra{p_1} \tensor U_{p_1}$ is the honest verifier's unitary to generate $v_1$ from $p_1$.
\end{enumerate}
\begin{MyComment}
Recall \xiao{from XXX} that $U$ can be written in the form of $\sum_{p_1} \ketbra{p_1}\tensor U_{p_1}$ because the concerned protocol is LOCC. $U_{p_1}$ works non-trivially on registers $\reg{ins}$, $\reg{v_2}$, and $\reg{w}$. In particular, it generates $V$'s message $v_1$ in register $\reg{v_1}$ (together with some residual state on $\reg{w}$).
\end{MyComment}


\item \label{item:Vtil:unitary:3}
{\bf ($\tilde{U}_3$: XOR $\reg{v_1}$ into $\reg{m_1}$.)} It proceeds as follows:
\begin{enumerate}
\item
If $H(p_1) = 0$, then swap the contents of registers $\reg{m_1}$ and $\reg{tmp}$.

\item
If $H(p_1) = 1$, then sets the content in register $\reg{m_1}$ to $\ket{v_1 \xor m}_{\reg{m_1}}$, where $m$ is the original content in register $\reg{m_1}$ and $v_1$ is the content in register $\reg{v_1}$. 
\end{enumerate}
\begin{MyComment}
It is worth noting that in the real execution, the original content $m$ is nothing but an all-0 string; In that case, this step (when $H(p_1)=1$) is simply copying $\reg{v_1}$ into $\reg{m_1}$---it simply moves the $v_1$ message generated by the verifier in the last step to the register $\reg{m_1}$ so that the prover gets to see this message.
\end{MyComment}

\item \label{item:Vtil:unitary:4}
{\bf ($\tilde{U}_4$: Swap $\reg{p_2}$ and $\reg{m_2}$.)} Upon receiving the final message $p_2$ in register $\reg{m_2}$, $\tilde{V}$ swaps the contents of the $\reg{p_2}$ and $\reg{m_2}$ registers.
\begin{MyComment}
In the real execution, this steps is for $\tilde{V}$ to move the $p_2$ message it received from the prover (in the $\reg{m_2}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_2}$), so that it can perform computation in the next step.
\end{MyComment}

\item \label{item:Vtil:unitary:5}
{\bf ($\tilde{U}_5$: $\tilde{V}$'s Decision.)} It proceeds as follows:
\begin{enumerate}
\item
If $H(p_1, p_2) = 0$, then do nothing. \xiao{need to recall where $(p_1,p_2)$ are stored.}

\item
If $H(p_1, p_2) = 1$, then it applies $U_\msf{d}$, where  $U_\msf{d}$ is the honest verifier's decision unitary. \xiao{If necessary, we can decompose $U_\msf{d}$ as $U_{\msf{d}} \coloneqq \sum_{p_1, v_1, p_2}\ketbra{p_1, v_1, p_2} \tensor U_{p_1, v_1, p_2}$.}
\end{enumerate}
\begin{MyComment}
Recall that $U_\msf{d}$ works non-trivially on registers $\reg{ins}$, $\reg{p_1}$, $\reg{v_1}$, $\reg{p_2}$, $\reg{d}$, and $\reg{w}$. In particular, it generates $V$'s final decision bit in register $\reg{d}$ (together with some residual state on $\reg{w}$).
\end{MyComment}







\end{enumerate}


\begin{remark}[On $\tilde{V}$'s Counter]
Note that the above description of $\tilde{V}$ implicitly assumes that $\tilde{V}$ knows in which round it is. This is without loss of generality because we can equip $\tilde{V}$ with a counter register recording the current round number in the same manner as \cite[Section 3.1]{FOCS:CCLY21}. Since this counter is not crucial to our security proof, we choose to omit it to keep notation succinct. 
\end{remark}





\subsection{Evolution of Registers in Simulation}

\begin{xiaoenv}{Some modifications needed for the model}
Further modify the modeling of the Simulator:
\begin{itemize}
\item
$\Sim$ prepares $q$ registers to store her query pattern, initialized to $\downarrow$: $\ket{\downarrow}_{\reg{u_1}} \ldots \ket{\downarrow}_{\reg{u_q}}$.
\item
Use a single unitary $S$ to denote $\Sim$'s algorithm, instead of $S_1$, $S_2$, $S_3$ as above. $S$ works on $\reg{m_1}$, $\reg{m_2}$, and $\reg{s}$. Actually, $S$ also need to work on the query pattern registers to determine the next query. Thus, we denote the $S$ as a sequence $S_1$, \ldots, $S_q$, $S_{q+1}$where $S_{i}$ works on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{s}$ and $\reg{u_i}$.
\item
State the lemma: The whole execution can be viewed as running $\Sim$ first for a fixed query pattern without intermediate measurement, and then project onto $\reg{u_1}\ldots\reg{u_q}$ w.r.t.\ the fixed query pattern to obtain a sub-normalized state. The norm of the state is the probability that this state would appear as a result of the real execution. 
\item
May also need to assume that $\Sim$ does not abort in the middle---She can always make dummy queries until the end. See how CCLY deal with this?
\end{itemize}
\end{xiaoenv}



In the following, we consider a fixed query patter of $q$ queries $\msf{Pat} \in \msf{PatSet}$.

We consider the setting where we measure the first messages when $\Sim$ tries to jump from Layer-$i$ to Layer-$(i+1)$ to obtain a classical prover message $p_i$. Right after this step, the oracle $H$ will be updated by adding $H(p_i) = 1$. ($H$ is initialized to output 0 on all inputs.)

We define the following hybrids:

\para{Hybrid $H_0$:} This is the game we just defined above. \xiao{refer to the picture} We use $\Pr[H_0 = 1]$ to denote the probability that at the last-step measurement of register $\reg{d}$ output 1. 

\para{Hybrid $H_1$:} This hybrid is identical to $H_0$, except that all the up (resp.\ down) queries between Layer-1 and Layer-2 are answered by $\tilde{U}^\dagger_{\msf{dmy}}$ (resp.\ $\tilde{U}_{\msf{dmy}}$). \xiao{refer to the picture}

\para{Hybrid $H_2$:} This hybrid is identical to $H_1$, except that all the up (resp.\ down) queries between Layer-2 and Layer-3 are answered by $\tilde{U}^\dagger_{\msf{dmy}}$ (resp.\ $\tilde{U}_{\msf{dmy}}$). \xiao{refer to the picture}


In the following, we prove that $\Pr[H_0 = 1] = \Pr[H_2 = 1]$, which can be broken as the following two lemmas.
\begin{lemma}\label{lem:LOCC-3ZK-hyb01}
It holds that $\Pr[H_0 = 1] = \Pr[H_1 = 1]$.
\end{lemma}

\begin{lemma}\label{lem:LOCC-3ZK-hyb12}
It holds that $\Pr[H_1 = 1] = \Pr[H_2 = 1]$.
\end{lemma}


\xiao{Explain why these lemmas are important to our proof. Add some intuition. Say that the proof of these lemmas make use of the Error-Invariant Commutativity Lemma}


\para{Renaming Unitaries.} Before proving these lemmas, we first group and rename $\tilde{V}$'s unitaries (defined in \Cref{sec:particular-mal-V}). For a fixed $p_1, p_2 \in \bits^\ell$,
\begin{enumerate}
\item \label{LOCC-3ZK:renaming:1}
Let $\tilde{U}_2 = \ketbra{p_1}_{\reg{p_1}} \tensor \tilde{U}_{2,0} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor I$. Note that $\tilde{U}_{2,0}$ acts non-trivially only on $\reg{v_1}$ and $\reg{w}$, and works as identity on other registers. $I$ is identity on all registers.
\item \label{LOCC-3ZK:renaming:2}
Let $\tilde{U}_3 = \ketbra{p_1}_{\reg{p_1}} \tensor \tilde{U}_{3,0} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \tilde{U}_{3,1}$. Note that $\tilde{U}_{3,0}$ acts non-trivially only on $\reg{v_1}$ and $\reg{m_1}$, and is identity on other registers. $\tilde{U}_{3,1}$ is the swap operator between $\reg{m_1}$ and $\reg{tmp}$, and is identity on other registers. 
\item \label{LOCC-3ZK:renaming:3}
Let $\tilde{U}_5 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{5,0} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor I$. Note that $\tilde{U}_{5,0}$ is nothing but the $U_d$ operator, which acts non-trivially only on registers $\reg{d}$ and $\reg{w}$, and is identity on other registers.
\end{enumerate}


It will be important to keep track on the registers that the unitaries acts on {\em non-trivially}. For the reader's convenience, we summarize it in \Cref{LOCC-3ZK:table:non-trivial-registers}. For a unitary shown in the table, it acts as identity on registers not shown in its column.

\begin{table}[h!]
\caption{Registers that Unitary Operators act on Non-Trivially}
\label{LOCC-3ZK:table:non-trivial-registers}
\begin{center}\def\arraystretch{1.5}
\begin{tabular}{ |C{50pt}|| C{30pt}|C{30pt}|C{30pt} | C{30pt}|C{30pt}| C{35pt}|C{30pt}|C{30pt}|C{30pt}| C{70pt} | C{50pt}| }
 \hline
Unitary Operators & $\tilde{U}_{1}$ &  $\tilde{U}_{2,0}$ & $\tilde{U}_{2}$ & $\tilde{U}_{3,0}$ & $\tilde{U}_{3,1}$ & $\tilde{U}_{3}$ & $\tilde{U}_{4}$ & $\tilde{U}_{5,0}$ & $\tilde{U}_5$ & $S_0$ & $S_j$ ($j \in [q]$) \\
\hline
Non-Trivial Registers & $\reg{p_1}$, $\reg{m_1}$ & $\reg{v_1}$, $\reg{w}$ & $\reg{p_1}$, $\reg{v_1}$,  $\reg{w}$ & $\reg{v_1}$, $\reg{m_1}$ & $\reg{m_1}$, $\reg{tmp}$ & $\reg{p_1}$, $\reg{v_1}$, $\reg{m_1}$, $\reg{tmp}$ & $\reg{p_2}$, $\reg{m_2}$ & $\reg{d}$, $\reg{w}$ & $\reg{p_1}$, $\reg{p_2}$, $\reg{d}$, $\reg{w}$ & \red{place holder} & $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, $\reg{s}$ \\
\hline
\end{tabular}
\end{center}
\end{table}




\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb01}}

We first claim that in hybrid $H_0$, whenever the execution reaches Layer-2, the registers can be described by the following ensemble: there exist $p_1 \in \bits^{\ell}$ \xiao{existence of $\gamma_{p_1}$ and $\gamma_{p'_1}$} and $P_{p_1} \in [0,1]$ such that with probability $P_{p_1}$, the registers is of the following format:\xiao{say that we omit the register $\reg{ins}$}
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:target-format}
\ket{\eta} = \gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\end{equation}
\xiao{explain the red text} where $\ket{\rho_{p_1}}$ (resp.\ $\ket{\rho_{p'_1}}$) is a pure state on registers \xiao{XXX} that may depend on $p_1$ (resp.\ $p'_1$).

We establish this claim by a mathematical induction on the number $k$ indicating it is which time the execution reaches Layer-1.

\para{Base Case ($k = 1$):} This corresponds to the very first query made by $\Sim$. Formally, $\Sim$'s local operation $S_0$ is applied to the initial state, preparing a superposition \xiao{not accurate. Need to consider all the registers} in register $\reg{m_1}$. Then, $\reg{m_1}$ and $\reg{p_1}$ are swapped, and $\reg{p_1}$ is measured in computational basis, collapsing the state to $\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}$ with some probability $P_{p_1}$, where \xiao{$\ket{\rho_{p_1}}$ is a pure state over registers other than $\reg{p_1}$}, and $P_{p_1}$ is the probability that the $\reg{p_1}$ measures to the particular value $p_1$.

Then, the first  $\downarrow$ query is made, bringing the execution from Layer-1 to Layer-2 for the first time. This $\downarrow$ query corresponds to apply $\tilde{U}_3\tilde{U}_2$ on state $\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}$. Formally, the resulting state becomes:
\begin{equation*}
\tilde{U}_3\tilde{U}_2 \ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}
=
\ket{p_1}_{\reg{p_1}} \tilde{U}_{3,0}\tilde{U}_{2,0} \ket{\rho_{p_1}} 
=
\ket{p_1}_{\reg{p_1}} \ket{\tilde{\rho}_{p_1}} 
,\end{equation*} 
where the first equality follows from the definition of $\tilde{U}_3$ and $\tilde{U}_2$, and the second equality follows by renaming $\ket{\tilde{\rho}_{p_1}} \coloneqq\tilde{U}_{3,0}\tilde{U}_{2,0} \ket{\rho_{p_1}}$. 

It is straightforward that $\ket{p_1}_{\reg{p_1}} \ket{\tilde{\rho}_{p_1}}$ is a special case of the format shown in the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format}. This concludes the proof of the base case.




\para{Induction Step ($k\ge 2$):} We assume the registers are of the format shown in \xiao{cref to xxx} when the execution reaches Layer-2 for the $(k - 1)$-th time, and prove in the following that the format is maintained when it reaches Layer-2 for the $k$-th time.

We establish this claim by considering the following MECE (mutually exclusive and collectively exhaustive) cases:
\begin{itemize}
\item
{\bf Case 1:} The $k$-th arrival is due to an immediate $\uparrow \downarrow$ after the $(k-1)$-th arrival. That is, after the $(k-1)$-th arrival, $\Sim$ first makes a $\downarrow$ query, jumping to Layer-1, and then makes an $\uparrow$ query, jumping back to Layer-2. \xiao{see picture XXX for an example}
\item
{\bf Case 2:} The $k$-th arrival is due to an immediate $\downarrow \uparrow $ after the $(k-1)$-th arrival. That is, after the $(k-1)$-th arrival, $\Sim$ first makes a $\downarrow$ query, jumping to Layer-3, and then makes an $\uparrow$ query, jumping back to Layer-2. \xiao{see picture XXX for an example}
\end{itemize}

\subpara{For Case 1:} We first describe formally how $\ket{\eta}$ evolves in this case. First, $\Sim$'s local unitary $S_j$ is applied \xiao{say that we assume this is the $j$-th local step}; Then, an $\uparrow$-query is made, corresponding to applying $\tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3$, bringing the execution to Layer-1. Next, the $(j+1)$-th local operation $S_{j+1}$ is applied, followed by a $\downarrow$-query, corresponding to applying $\tilde{U}_3\tilde{U}_2 \tilde{U}_1$, bringing the execution back to Layer-2. In summary, the unitary $\tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j$ is applied to $\ket{\eta}$. 

In the following, we show that the state $\tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j\cdot\ket{\eta}$ can indeed be written in the same format as shown in the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format}. First, we remark that the operator 
$\tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1$ can be written as 
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:swap-S} 
\tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 =  \tilde{U}_1 \tilde{U}^\dagger_1  S^{\reg{p_1}/\reg{m_1}}_{j+1} = S^{\reg{p_1}/\reg{m_1}}_{j+1},
\end{equation}
where the first equality follows from the fact that $\tilde{U}^\dagger_1$ is nothing but a swap operator between $\reg{m_1}$ and $\reg{p_1}$. It is worth recalling  \red{cref to place} that $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ is the same unitary operator as $S_{j+1}$ but treating register $\reg{p_1}$ as $\reg{m_1}$. Thus, $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ acts non-trivially only on $\reg{p_1}$, $\reg{m_2}$, $\reg{u}_{j+1}$, and $\reg{s}$, and is identity on other registers.

With the above notation, we show the derivation below:

\begin{align*}
& \tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j \cdot \ket{\eta} \\ 
=~ &  
\tilde{U}_3\tilde{U}_2 \tilde{U}_1 S_{j+1}  \tilde{U}^\dagger_1 \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j 
\bigg( 
\gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\bigg) \\
=~ &  
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m_1}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3 S_j
\bigg( 
\gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:0} \\
=~ &  
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m_1}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3
\bigg( 
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S_j \ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} S_j \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:1} \\ 
=~ &  
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m_1}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3
\bigg( 
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S_j \ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} S^{\reg{tmp}/\reg{m_1}}_j \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:2} \\ 
=~ &  
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m_1}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3
\bigg( 
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S_j \ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{tmp}/\reg{m_1}}_j \ket{\rho_{p'_1}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:3} \\ 
=~ & 
\tilde{U}_3\tilde{U}_2 S^{\reg{p_1}/\reg{m_1}}_{j+1}  \tilde{U}^\dagger_2\tilde{U}^\dagger_3
\bigg( \gamma_{p_1}\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}_{p'_1}} \bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4} \\
=~ &  
\tilde{\gamma}_{p_1} \ket{p_1}_{\reg{p_1}} \ket{\tilde{\rho}_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \tilde{\gamma}_{p'_1}\ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\tilde{\rho}_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:0} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:swap-S}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:1} follows from the fact that $S_j$ works as identity on $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:2} follows from the definition of $\tilde{U}_{3,1}$ (see \Cref{LOCC-3ZK:renaming:2}) and the definition of $S^{\reg{tmp}/\reg{m_1}}_j$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:3} follows from the fact that $S^{\reg{tmp}/\reg{m_1}}_j$ works on different registers from $\tilde{U}_{2,0}^\dagger\tilde{U}_{3,0}^\dagger$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4} follows by renaming $\ket{\dot{\rho}_{p_1}}  \coloneqq S_j \ket{\rho_{p_1}}$ and $\ket{\dot{\rho}_{p'_1}} \coloneqq S^{\reg{tmp}/\reg{m_1}}_j \ket{\rho_{p'_1}}$, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6} follows from an application of \Cref{eq:lem:err-inv-com:property-2:real} of \Cref{lem:err-inv-com} (see \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:remark}).

\begin{table}[h!]
\caption{Notation Correspondence between \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6} and \Cref{lem:err-inv-com}}
\label{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}
\begin{center}\def\arraystretch{1.5}
\begin{tabular}{ |C{60pt}||C{20pt}|C{20pt}|C{20pt}|C{45pt}|C{45pt}|C{20pt}|C{20pt}|C{20pt}|C{20pt}|C{20pt}|C{30pt}|C{20pt}|C{20pt}|C{20pt}|C{20pt}| }
 \hline
 \multicolumn{1}{|c||}{ } & 
 \multicolumn{5}{c|}{Registers} &
 \multicolumn{6}{c|}{Operators} &
 \multicolumn{4}{c|}{Variables} \\
 \hline
 In \Cref{lem:err-inv-com} & $\reg{a}$ & $\reg{m}$ & $\reg{t}$ & $\reg{s}$ & $\reg{o}$ & $W_0$ & $W_1$ & $W$ & $U_0$ & $U$ & $S$ & $a$ & $a'$ & $\rho_a$ & $\rho_{a'}$ \\
 \hline
In \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4} & $\reg{p_1}$ & $\reg{m_1}$ & $\reg{tmp}$ & $\reg{m_2}, \reg{u_{j+1}}, \reg{s}$ & other registers & $\tilde{U}_{3,0}$ & $\tilde{U}_{3,1}$ & $\tilde{U}_{3}$ & $\tilde{U}_{2,0}$ & $\tilde{U}_2$ & $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ & $p_1$ & $p'_1$ & $\dot{\rho}_{p_1}$ & $\dot{\rho}_{p'_1}$ \\
\hline
\end{tabular}
\end{center}
\end{table}
\begin{remark}[Deriving \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6} via \Cref{lem:err-inv-com}]\label{lem:LOCC-3ZK-hyb01:proof:case-1:remark}
To obtain \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6}, one only needs to invoke \Cref{eq:lem:err-inv-com:property-2:real} of \Cref{lem:err-inv-com} in our current setting, with the corresponding notations summarized in the \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}. (Note that we do not need to define $\tilde{W}$ as it is irrelevant to \Cref{eq:lem:err-inv-com:property-2:real} of \Cref{lem:err-inv-com}.) In more detail, note that \Cref{lem:err-inv-com} requires that $W_0$ should work as identity on register $\reg{s}$, which is satisfied by $\tilde{U}_{3,0}$ (i.e., the $W_0$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}) who is identity on registers $\reg{m_2}$, $\reg{u_{j+1}}$, and $\reg{s}$ (i.e., the register $\reg{s}$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}); \Cref{lem:err-inv-com} requires that $W_1$ should be a swap operator between $\reg{m}$ and $\reg{t}$, which is satisfied by $\tilde{U}_{3,1}$ (i.e., the $W_1$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}) who is a swap operator between $\reg{m_2}$ and $\reg{tmp}$ (i.e., the register $\reg{m}$ and $\reg{t}$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}); \Cref{lem:err-inv-com} requires that $U_0$ should work as identity on register $\reg{s}$, which is satisfied by $\tilde{U}_{2,0}$ (i.e., the $U_0$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}) who is identity on registers $\reg{m_2}$, $\reg{u_{j+1}}$, and $\reg{s}$ (i.e., the register $\reg{s}$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}); Also, \Cref{lem:err-inv-com} requires that $S$ should act non-trivially only on registers $\reg{a}$ and $\reg{s}$, which is satisfied by $S^{\reg{p_1}/\reg{m_1}}_{j+1}$ (i.e., the $S$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}) who does not touch registers beyond $\reg{p_1}$, $\reg{m_2}$, $\reg{u_{j+1}}$ and $\reg{s}$ (i.e., the registers $\reg{a}$ and $\reg{s}$ in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:4}).
\end{remark}

It is obvious that the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:eq:6} is of the same format as the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format}. This finishes the proof for Case 1.


\subpara{For Case 2:}  We describe formally how $\ket{\eta}$ evolves in this case. First, $\Sim$'s local operator $S_j$ will be applied, followed by a $\downarrow$ query, $S_{j+1}$, and a $\uparrow$ query. Here are two sub-bases to consider, depending if this is the first time the execution arrives at Layer-3. In the following, we prove the two case separately.

\subpara{Sub-Case 2-1:} This is the case where the $\downarrow$ represents the first time the execution arrives at Layer-3. Thus, the $\tilde{U}_5$ is applied and the $\reg{p_2}$ register is measured in the computational basis, collapsing it to a particular value $p_2$ with some probability $P_{p_2}$. We now formally analyze the evolution of state $\ket{\eta}$ in this case.

First, the local operator $S_j$ is applied to $\ket{\eta}$, leading to
\begin{align*}
& S_j \cdot \ket{\eta} \\ 
=~& 
S_j 
\bigg( 
\gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\bigg) \\ 
=~& 
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} S_j  \ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} S_j \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:1} \\ 
=~& 
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} S_j  \ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} S^{\reg{m_1}/\reg{tmp}}_j \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:2} \\ 
=~& 
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} S_j  \ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{m_1}/\reg{tmp}}_j  \ket{\rho_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:3} \\
=~& 
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:4} \\ 
=~& 
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \sum_{p'_2\in \bits^\ell} \alpha_{p'_2} \ket{p'_2}_{\reg{p_2}} \ket{\dot{\rho}_{p_1, p'_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \sum_{p'_2\in \bits^\ell} \alpha_{p'_2} \ket{p'_2}_{\reg{p_2}} \ket{\dot{\rho}_{p'_1, p'_2}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:5} \\ 
=~& 
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \sum_{p'_2\in \bits^\ell} \alpha_{p'_2} \ket{p'_2}_{\reg{p_2}} \ket{\dot{\rho}_{p_1, p'_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}    \sum_{p'_2\in \bits^\ell} \alpha_{p'_2} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\dot{\rho}_{p'_1, p'_2}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:6}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:1} follows from the fact that $S_j$ acts as identity on $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:2} follows from the definitions of $\tilde{U}_{3,1}$ and $S^{\reg{m_1}/\reg{tmp}}_j$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:3}  follows from the fact that $S^{\reg{m_1}/\reg{tmp}}_j$ operates on different registers from $\tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:4} follows by renaming $\ket{\dot{\rho}_{p_1}} \coloneqq S_j  \ket{\rho_{p_1}}$ and $\ket{\dot{\rho}_{p'_1}} \coloneqq S^{\reg{m_1}/\reg{tmp}}_j  \ket{\rho_{p'_1}}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:5} \xiao{(actually, this \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:5} is problematic. The amplitudes for $p'_2$ in the two branches should be different.)} follows by expanding the $\reg{p_2}$ register in computational basis, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:6} follows from the fact that $\tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ acts as identity on $\reg{p_2}$.

Next, the $\reg{p_2}$ register is measured under computational basis. Due to \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:6}, we can describe the measurement outcome as follows: With probability $P_{p_2} \coloneqq |\alpha_{p_2}|^2$, the $S_j\ket{\eta}$ collapses to the following state:
\begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:7}
    \gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}  \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\dot{\rho}_{p'_1, p_2}} 
\end{equation}
Finally, the unitary $\tilde{U}^\dagger_4\tilde{U}^\dagger_5S_{j+1}\tilde{U}_5$ is applied to the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:7}. First, note that $S_{j+1}$ and $\tilde{U}_5$ commutes as they operate on different registers (see \Cref{LOCC-3ZK:table:non-trivial-registers}), and thus 
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:8}
\tilde{U}^\dagger_5S_{j+1}\tilde{U}_5 = S_{j+1} = \tilde{U}^\dagger_5 \tilde{U}_5 S_{j+1} = S_{j+1}.
\end{equation}
Then, the following holds:

\begin{align*}
&\tilde{U}^\dagger_4\tilde{U}^\dagger_5S_{j+1}\tilde{U}_5 
\bigg(
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}  \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\dot{\rho}_{p'_1, p_2}} 
\bigg) \\ 
=~&
\tilde{U}^\dagger_4 S_{j+1}
\bigg(
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}  \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\dot{\rho}_{p'_1, p_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:9} \\ 
=~&
\tilde{U}^\dagger_4
\bigg(
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}  S_{j+1} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\dot{\rho}_{p'_1, p_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:10} \\ 
=~&
\tilde{U}^\dagger_4
\bigg(
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}   \tilde{U}_{3,1} S^{\reg{tmp}/\reg{m_1}}_{j+1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\dot{\rho}_{p'_1, p_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:11} \\ 
=~&
\tilde{U}^\dagger_4
\bigg(
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}}   \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  S^{\reg{tmp}/\reg{m_1}}_{j+1}  \ket{\dot{\rho}_{p'_1, p_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:12} \\ 
=~&
\tilde{U}^\dagger_4
\bigg(
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{p_2}_{\reg{p_2}}    S^{\reg{tmp}/\reg{m_1}}_{j+1}  \ket{\dot{\rho}_{p'_1, p_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:13} \\ 
=~&
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \tilde{U}^\dagger_4 \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}^\dagger_4 \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{p_2}_{\reg{p_2}}    S^{\reg{tmp}/\reg{m_1}}_{j+1}  \ket{\dot{\rho}_{p'_1, p_2}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:14} \\ 
=~&
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \tilde{U}^\dagger_4 \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \tilde{U}^\dagger_4 \ket{p_2}_{\reg{p_2}}     S^{\reg{tmp}/\reg{m_1}}_{j+1}  \ket{\dot{\rho}_{p'_1, p_2}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:15} \\ 
=~&
\gamma_{p_1} \ket{p_1}_{\reg{p_1}} \ket{\tilde{\rho}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\tilde{\rho}_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:16}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:9} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:8}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:10} follows from the fact that $S_{j+1}$ acts as identity on registers $\reg{p_1}$ and $\reg{p_2}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:11} follows from the definition of $\tilde{U}_{3,1}$ and $S_{j+1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:12} follows from the fact that $S^{\reg{tmp}/\reg{m_1}}_{j+1}$ operates on different registers from  $\tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:13} follows from the fact that $\tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ acts as identity on $\reg{p_2}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:14} follows from the fact that $\tilde{U}^\dagger_4$ acts as identity on $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:15} follows from the fact that $\tilde{U}^\dagger_4$ commutes with $\tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ as they operate on different registers (see \Cref{LOCC-3ZK:table:non-trivial-registers}), and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:16} follows by renaming $\ket{\tilde{\rho}_{p_1}} \coloneqq \tilde{U}^\dagger_4 \ket{p_2}_{\reg{p_2}} S_{j+1}  \ket{\dot{\rho}_{p_1, p_2}}$ and $\ket{\tilde{\rho}_{p'_1}} \coloneqq \tilde{U}^\dagger_4 \ket{p_2}_{\reg{p_2}}     S^{\reg{tmp}/\reg{m_1}}_{j+1}  \ket{\dot{\rho}_{p'_1, p_2}}$.


It is easy to see that the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:16} is of the same format as the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format}. This concludes the proof of sub-case-2-1.


\subpara{Sub-Case-2-2:} This is the case where the $\downarrow$ is {\em not} the first time the execution arrives at Layer-3. In this case, the unitary $\tilde{U}^\dagger_4 \tilde{U}^\dagger_5 S_{j+1} \tilde{U}_5 \tilde{U}_4 S_j$ will be applied to $\ket{\eta}$. Before presenting the derivation, we first notice that 
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:0}
\tilde{U}^\dagger_4 S_{j+1}\tilde{U}_4 = \tilde{U}^\dagger_4 \tilde{U}_4 S^{\reg{p_2} /\reg{m_2}}_{j+1} = S^{\reg{p_2} /\reg{m_2}}_{j+1},
\end{equation}
where the first equality follows from the definition of $\tilde{U}_4$ and $S_{j+1}$.



The following holds:
\begin{align*}
& \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 S_{j+1} \tilde{U}_5 \tilde{U}_4 S_j \cdot \ket{\eta} \\
=~&  
\tilde{U}^\dagger_4 \tilde{U}^\dagger_5 S_{j+1} \tilde{U}_5 \tilde{U}_4 S_j
\bigg(
\gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\bigg)\\ 
=~&
\tilde{U}^\dagger_4  S_{j+1} \tilde{U}_4 S_j 
\bigg(
\gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:1} \\ 
=~&
 S^{\reg{p_2}/\reg{m_2}}_{j+1}  S_j 
\bigg(
\gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:2} \\ 
=~&
 S^{\reg{p_2}/\reg{m_2}}_{j+1}  
\bigg(
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S_j\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{tmp}/\reg{m_2}}_j \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:3} \\ 
=~&
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S^{\reg{p_2}/\reg{m_2}}_{j+1}  S_j\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} S^{\reg{p_2}/\reg{m_2}}_{j+1}  \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{tmp}/\reg{m_2}}_j \ket{\rho_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:4} \\ 
=~&
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S^{\reg{p_2}/\reg{m_2}}_{j+1}  S_j\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} S^{\reg{tmp}/\reg{m_1}, \reg{p_2}/\reg{m_2}}_{j+1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  S^{\reg{tmp}/\reg{m_2}}_j \ket{\rho_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:5} \\ 
=~&
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} S^{\reg{p_2}/\reg{m_2}}_{j+1}  S_j\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  S^{\reg{tmp}/\reg{m_1}, \reg{p_2}/\reg{m_2}}_{j+1}  S^{\reg{tmp}/\reg{m_2}}_j \ket{\rho_{p'_1}} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:6} \\ 
=~&
\gamma_{p_1}\ket{p_1}_{\reg{p_1}} \ket{\tilde{\rho}_{p_1}} +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}  \ket{\tilde{\rho}_{p'_1}}  \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:7} 
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:8}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:2} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:0}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:3} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:eq:3}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:4} follows from the fact that $S^{\reg{p_2}/\reg{m_2}}_{j+1}$ acts as identity on $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:5} follows from the definition of $\tilde{U}_{3,1}$ and $S^{\reg{tmp}/\reg{m_1}, \reg{p_2}/\reg{m_2}}_{j+1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:6} follows from the fact that $S^{\reg{tmp}/\reg{m_1}, \reg{p_2}/\reg{m_2}}_{j+1}$ and $\tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ operate on different registers, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:7} follows by renaming $\ket{\tilde{\rho}_{p_1}}  \coloneqq S^{\reg{p_2}/\reg{m_2}}_{j+1}  S_j\ket{\rho_{p_1}}$ and $\ket{\tilde{\rho}_{p'_1}}  \coloneqq S^{\reg{tmp}/\reg{m_1}, \reg{p_2}/\reg{m_2}}_{j+1}  S^{\reg{tmp}/\reg{m_2}}_j \ket{\rho_{p'_1}}$.

It is easy to see that the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-2:eq:7} is of the same format as the RHS of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format}. This concludes the proof of sub-case-2-2.



\UpdateLine





\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb12}}

We first claim that in hybrid $H_1$, whenever the execution reaches Layer-3, the registers can be described by the following ensemble: there exist $p_2 \in \bits^{\ell}$ \xiao{existence of $\gamma_{p_2}$ and $\gamma_{p'_2}$} and $P_{p_1},P_{p_2} \in [0,1]$ such that with probability $P_{p_1}\cdot P_{p_2}$, the registers is of the following format:\xiao{say that we omit the register $\reg{ins}$}
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:target-format}
\ket{\eta} = \gamma_{p_2}\ket{p_2}_{\reg{p_2}}\ket{\rho_{p_2}}  +  \sum_{p'_2 \in \bits^\ell \setminus \Set{p_2}} \gamma_{p'_2} \ket{p'_2}_{\reg{p_2}} \red{\hat{W}_1 \hat{U}^\dagger_0 \hat{W}^\dagger_0} \ket{\rho_{p'_2}}
\end{equation}
\xiao{explain the red text} where $\ket{\rho_{p_2}}$ (resp.\ $\ket{\rho_{p'_2}}$) is a pure state on registers \xiao{XXX} that may depend on $p_2$ (resp.\ $p'_2$).


\subpara{Base Case ($k = 1$):} Before the first time the execution arrives at Layer-3, the $\reg{p_2}$ register has not been touched. Consider the first $\downarrow$ query between Layer-2 and Layer-3. By definition, it consists of the procedure where $\Sim$ prepares a superposition in register $\reg{m_2}$ first; then the $\reg{m_2}$ is measured in computational basis, which collapses the state to the state $\ket{p_2}_{\reg{p_2}}\ket{\rho_{p_2}}$ with some probability $P_{p_2}$, where \xiao{$\ket{\rho_{p_2}}$ is a pure state over registers other than $\reg{p_2}$}, and $P_{p_2}$ is the probability that the $\reg{p_2}$ measures to the particular value $p_2$.

Obviously, $\ket{p_2}_{\reg{p_2}}\ket{\rho_{p_2}}$ is a particular case of the format shown in \Cref{lem:LOCC-3ZK-hyb12:proof:target-format}. This concludes the proof for the base case. 

\subpara{Induction Step ($k\ge 2$):} We assume the registers are of the format shown in \xiao{cref to xxx} when the execution reaches Layer-3 for the $(k - 1)$-th time, and prove in the following that the format is maintained when it reaches Layer-3 for the $k$-th time.

Consider the execution steps between the $(k-1)$-th arrival and $k$-th arrival at Layer-3. It can be described as follows:
\begin{enumerate}
\item
 $\Sim$ first applies the local operator $S_j$
 \item
 Then, the operator $\hat{U}^\dagger \hat{W}^\dagger$ is applied, bringing the execution to Layer-2.
 \item
At this point, there are two cases to consider: (i) $\Sim$ can make a $\downarrow$ immediately, bringing the execution back to Layer-3; {\em or } (ii) $\Sim$ can rewind $\tilde{V}$ further, bringing the execution to Layer-1.  Fortunately, our proof can handle these two cases at one stroke as follows: We define execution from this point until (exclusively) the next $\downarrow$ query {\em from Layer-2 to Layer-3} (i.e., the exact query that yields the $k$-th arrival at Layer-3) as a unitary $A$. $A$ might be an identity, corresponding to case (i); $A$ might also be some non-identity operator, representing the operations performed in case (ii) before the next arrival at Layer-3. We do not specify the exact form of $A$. But we remark that for both case (i) and (ii), $A$ works non-trivially on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{s}$, $\reg{u}$'s, $\reg{t_1}$ \xiao{note that the execution between Layer-1 and Layer-1 have already been replaced with dummy up-and-downs.}, while working as identity on other registers.  
\xiao{need to check the registers carefully to make sure that we can make use of \Cref{lem:err-inv-com}.}
\item
Finally, the operator $\hat{W} \hat{U}$ is applied, bringing the execution back to Layer-3.
\end{enumerate}
Now, we calculate the evolution of $\ket{\eta}$ state corresponding to the above procedure. It is
\begin{align*}
\hat{W}\hat{U}A\hat{U}^\dagger\hat{W}^\dagger \ket{\eta} 
&=  
\hat{W}\hat{U}A\hat{U}^\dagger\hat{W}^\dagger  \bigg(\gamma_{p_2}\ket{p_2}_{\reg{p_2}}\ket{\rho_{p_2}}  +  \sum_{p'_2 \in \bits^\ell \setminus \Set{p_2}} \gamma_{p'_2} \ket{p'_2}_{\reg{p_2}} \red{\hat{W}_1 \hat{U}^\dagger_0 \hat{W}^\dagger_0} \ket{\rho_{p'_2}}\bigg) \\ 
&=
 \tilde{\gamma}_{p_2}\ket{p_2}_{\reg{p_2}}\ket{\tilde{\rho}_{p_2}}  +  \sum_{p'_2 \in \bits^\ell \setminus \Set{p_2}} \tilde{\gamma}_{p'_2} \ket{p'_2}_{\reg{p_2}} \hat{W}_1 \hat{U}^\dagger_0 \hat{W}^\dagger_0 \ket{\tilde{\rho}_{p'_2}} \numberthis \label{lem:LOCC-3ZK-hyb12:proof:case-2:eq:1}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:case-2:eq:1} follows from an application of \Cref{eq:lem:err-inv-com:property-2:real} of \Cref{lem:err-inv-com}. \xiao{Here, I need to explain it in detail how to define the registers to make sure that I can indeed invoke }

It is obvious that the RHS of \Cref{lem:LOCC-3ZK-hyb12:proof:case-2:eq:1} is of the same format as \Cref{lem:LOCC-3ZK-hyb12:proof:target-format}. This finishes the proof for the induction step.

% \begin{align*}
% &
% \gamma_{p_1}\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \red{W_1 U^\dagger_0 W^\dagger_0} \ket{\rho_{p'_1}} \\
% =~&
% \sum_{p'_2 \in \bits^{\ell}} \dot{\gamma}_{p_2}\ket{p_2}_{\reg{p_2}}\ket{\dot{\rho}_{p_2}} 
% =~&
% \gamma_{p_1}\ket{p_1}_{\reg{p_1}} \sum_{p'_2\in \bits^\ell}\alpha_{p_1, p'_2} \ket{p'_2}_{\reg{p_2}}  \ket{\rho_{p_1, p'_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}} \red{W_1 U^\dagger_0 W^\dagger_0} \sum_{p'_2\in \bits^\ell}\alpha_{p'_1, p'_2} \ket{p'_2}_{\reg{p_2}} \ket{\rho_{p'_1, p'_2}}  \numberthis \label{lem:LOCC-3ZK-hyb12:proof:case-1:eq:1} \\ 
% =~&
% \gamma_{p_1}\ket{p_1}_{\reg{p_1}} \sum_{p'_2\in \bits^\ell}\alpha_{p_1, p'_2} \ket{p'_2}_{\reg{p_2}}  \ket{\rho_{p_1, p'_2}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \sum_{p'_2\in \bits^\ell}\alpha_{p'_1, p'_2} \ket{p'_2}_{\reg{p_2}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{p'_1, p'_2}}  \numberthis \label{lem:LOCC-3ZK-hyb12:proof:case-1:eq:2} \\ 
% =~&
% \gamma_{p_1}\ket{p_1}_{\reg{p_1}} \alpha_{p_1, p_2} \ket{p_2}_{\reg{p_2}}  \ket{\rho_{p_1, p_2}} 
% +
% \gamma_{p_1}\ket{p_1}_{\reg{p_1}} \sum_{p'_2\in \bits^\ell \setminus \Set{p_2}}\alpha_{p_1, p'_2} \ket{p'_2}_{\reg{p_2}}  \ket{\rho_{p_1, p'_2}}  ~+ \\ 
% & 
% \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \alpha_{p'_1, p_2} \ket{p_2}_{\reg{p_2}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{p'_1, p_2}}
% + 
% \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \ket{p'_1}_{\reg{p_1}}  \sum_{p'_2\in \bits^\ell \setminus \Set{p'_2}}\alpha_{p'_1, p'_2} \ket{p'_2}_{\reg{p_2}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{p'_1, p'_2}} \\ 
% =~&
% \gamma_{p_1}\alpha_{p_1, p_2}  \ket{p_2}_{\reg{p_2}} \ket{p_1}_{\reg{p_1}}  \ket{\rho_{p_1, p_2}} 
% +
%  \sum_{p'_2\in \bits^\ell \setminus \Set{p_2}} \gamma_{p_1} \alpha_{p_1, p'_2}  \ket{p'_2}_{\reg{p_2}} \ket{p_1}_{\reg{p_1}}   \ket{\rho_{p_1, p'_2}}  ~+ \\ 
% & 
% \ket{p_2}_{\reg{p_2}} \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1}  \alpha_{p'_1, p_2} \ket{p'_1}_{\reg{p_1}}   W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{p'_1, p_2}}
% + 
% \sum_{p'_2\in \bits^\ell \setminus \Set{p'_2}} \ket{p'_2}_{\reg{p_2}} \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \gamma_{p'_1} \alpha_{p'_1, p'_2} \ket{p'_1}_{\reg{p_1}}    W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{p'_1, p'_2}} 
% ,\end{align*}





\UpdateLine












==> sections/2-round-QCCC.tex <==
\section{Warm Up: Impossibility of Two-Round QCCC ZK}

\jiahui{in fact it's a one round protocol since the prover mesasge is the first one?}


In this section, we show as a warm-up example that two-round ZK in the QCCC model is impossible. This proof already illustrate the main ideas behind our general impossibility for the constant-round case.


Note that by ``two-round'', we mean that $P$ sends the first message $a$, and $V$ applies a unitary operator $U$ to generate the bit $b$ indicating if $V$ accepts or not. So, the second round is nothing but $V$'s decision bit. 




\subsection{The Model}


Similar as \cite{FOCS:CCLY21}, we first show the impossibility result with an inefficient $\tilde{V}$. The inefficiency is only due to a random function $H$ hard-wired in $\tilde{V}$. We will make $\tilde{V}$ efficient later by replacing $H$ by a $q$-wise independent hash.


We use $a$ and $b$ to denote $P$ and $\tilde{V}$'s respective message. In this particular setting, $b$ is a single bit. But as will become clear later, $b$'s length is not important for the proof to go through; This is important later when we try to generalize the proof to the constant-round setting, where $b$ could be a non-final-round message from $\tilde{V}$ that consists of multiple bits. We use $\ell(\secpar)$ to denote the length of $a$, which is a polynomial of the security parameter $\secpar$.


\para{$\tilde{V}$'s Registers.} $\tilde{V}$ starts by initializing the following registers (see \Cref{figure:2-QCCC-V:registers} for an explanation):
\begin{equation}\label[Expression]{2-QCCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{a}}\ket{\vb{0}}_{\reg{b}} \ket{1}_{\reg{f}} \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w}
\end{equation}

\jiahui{Should the $aux$ register also contain an initial internal state other than H?}

The simulator $\simulator$ also initializes its working register to some arbitrary
initial state: $\ket{\Init}_{\reg{adv}}$.




\begin{FigureBox}[label={figure:2-QCCC-V:registers}]{Registers}
We explain the meaning of the registers defined in \Cref{2-QCCC:V:inital:expr}:
\begin{itemize}
    \item
    $\reg{ins}$ stores the input instance $x$;
\item
$\reg{a}$ and $\reg{b}$ will be used to store the execution transcript (i.e., the messages $a$ and $b$ exchanged between the prover and verifier); As will become clear in our proof, storing all the exchanged messages turns out to be critical for our proof to work.

\item
$\reg{f}$ is a flag register, containing a single qubit. It will be used to ensure that the simulator must ``return'' the original message $b$ without modification when she wants to rewind/un-compute $\tilde{V}$. See \red{ref:XXX} for details. 

\item
$\reg{m}$ is the register to store messages from/to the prove.


\item
$\reg{aux}$ stores the truth table of the random function $H$. This is the only register that is of super-polynomial size. 

\item
$\reg{w}$ is the working space of the verifier initialized with enough ancilla qubits that will be used for purposes like purification and dilation etc.

\item $\reg{adv}$ is the working register (which also contains a polynomial-size auxiliary state) for the adversary/simulator.
\end{itemize}
% We emphasize that all of these registers need to be initialized to proper length. To simplify the notation, we do not specify the length of them. But it is easy to see that their length is bounded by a fixed polynomial of the security parameter, and this polynomial can be determined in advance. 
\end{FigureBox}


In the impossibility result, we construct a BQP algorithm that runs both the simulator $\simulator$ and verifier $V$.
Our entire purified view therefore consists of all above registers $\reg{ins, a,b,m,aux,w,adv}$. 


\para{$\tilde{V}$'s Unitary $\tilde{U}$.}  We next describe the unitary $\tilde{U}$ for $\tilde{V}$. Upon receiving message the first-round message $a$ in register $\reg{m}$, $\tilde{V}$ applies $\tilde{U} \coloneqq \tilde{U}_4\tilde{U}_3\tilde{U}_2\tilde{U}_1$, where the $\tilde{U}_i$'s are defined as follows:
\begin{enumerate}
\item
{\bf ($\tilde{U}_1$: Swap Message.)}
Conditioned on $\ket{1}_{\reg{f}}$,\footnote{This is a shortcut for the following sentence ``it first checks if the $\reg{f}$ register contains $1$; if so, it execute the following instruction, otherwise, it does nothing.'' We will use this convention through out the description of $\tilde{V}$.} it behaves as follows:

\begin{enumerate}

\jiahui{
If $H(a) = 0$, then return $\bot$}
\item
If $H(a) = 0$, then do nothing;


\item
If $H(a) = 1$, then swap the contents between $\reg{m}$ and $\reg{a}$.
\end{enumerate}
\jiahui{mentioned that $a$ is classical}
\begin{MyComment}
    Without loss of generality, we assume $a$ is a classical message. We will explain later in the proof why our model under this assumption suffices for our proof.
\end{MyComment}
 
\item
{\bf ($\tilde{U}_2$: Apply $V$'s Unitary.)}
Conditioned on $\ket{1}_{\reg{f}}$, it behaves as follows: 
\begin{enumerate}
\item
If $H(a) = 0$, then do nothing;
\item
If $H(a) = 1$, then apply $U$ to registers $\reg{a}, \reg{b}$. 
\end{enumerate}
\begin{MyComment}
Recall \xiao{from XXX} that $U$ is the unitary of the honest verifier $V$, which works non-trivially on registers $\reg{ins}$,  $\reg{a}$, $\reg{b}$, and $\reg{w}$. In particular, it generates $V$'s decision qubit on register $\reg{b}$ (together with some residual state on $\reg{w}$).
\end{MyComment}

\jiahui{mention that since we work with QCCC/LOCC, we can see the operator $U = \sum_a \ket{a} \bra{a} \otimes U_a$}

\item
Conditioned on $\ket{1}_{\reg{f}}$, it behaves as follows: 
\begin{enumerate}
\item
If $H(a) = 0$, then do nothing;
\item
If $H(a) = 1$, then sets the content in register $\reg{m}$ to $\ket{m \xor b}_{\reg{m}}$ \xiao{explain that $m$ and $b$ are of different length}, where $m$ is the original content in register $\reg{m}$ and $b$ is the content in register $\reg{b}$. 
\end{enumerate}


\begin{MyComment}
Note that this step can be understood as a controlled-XOR gate that is controlled by the $\reg{f}$ register and $H(a)$ to xor the $\reg{b}$ register into the $\reg{m}$ register.  It is  worth noting that in the real execution, the original content $m$ is nothing but an  all-0 string; In that case, this step is simply copy $\reg{b}$ into $\reg{m}$ (of course, controlled by $\reg{f}$).
\end{MyComment}

\jiahui{remove this step?}

\item
Conditioned on $\ket{1}_{\reg{f}}$, it behaves as follows: 
\begin{enumerate}
\item
If $H(a) = 0$, then do nothing;
\item
If $H(a) = 1$, do the following: Compare the contents of $\reg{b}$ and $\reg{m}$; If they are equal, modify the $\reg{f}$ register to $\ket{f \xor 1}_{\reg{f_i}}$, where $f$ is the original content on $\reg{f_i}$; Otherwise, do nothing.
\end{enumerate}


\begin{MyComment}
Assuming the conditions are satisfied (i.e., $\reg{f}$ contains 1 and $H(a)=1$), this step can be understood as first write the value $\neg (b \xor m)$ into a register $\reg{t}$ in the working space. Then,  apply a $\msf{CNOT}$ on  (the control register) $\reg{t}$ and  (the target register) $\reg{f}$. Note that in the real execution, the register $\reg{f}$ will contain a classical bit 0 after this step, because the original content $f$ is 1 and $\reg{b}$ and $\reg{m}$ have exactly the same content, right before this step (in the real execution).
\end{MyComment}

 
%\item 
%\begin{enumerate}
%    \item If $H(a) = 0$
%, then do nothing.
%\item 
%\end{enumerate}


\end{enumerate}


\begin{remark}[On $\tilde{V}$'s Counter]
Note that the above description of $\tilde{V}$ implicitly assumes that $\tilde{V}$ knows in which round it is. This is without loss of generality because we can quip $\tilde{V}$ with a counter register recording the current round number in the same manner as \cite[Section 3.1]{FOCS:CCLY21}. Since this counter is not crucial to our security proof, we choose to omit it to keep notation succinct. 
\end{remark}

Next we define a "dummy" version of the verifier's operation that we use in our proof.

\paragraph{Dummy Verifier Operator $\udummy$}

\jiahui{change to $\udummy$}

The operation $\udummy = \utilde_1 \cdot \mathbf{I} \cdot \mathbf{I} \cdot \mathbf{I} $ is simply an identity operator that does nothing except the SWAP operation between $\reg{m}$ and $\reg{a}$.

That is: $U_\bot = \swap_{\reg{a,m}}  \cdot \mathbf{I} \cdot \mathbf{I} \cdot \mathbf{I}  $
%in all the above steps
\subsection{Simulator's View in the world of $\tilde{U}$}
\label{sec:sim_view_utilde}

In this section, we show the evolution of the registers $\reg{a,b,m,aux}$ in the world where  $\utilde$ and $\utilde^\dagger$ are used when the simulator $\simulator$ queries the verifier.

\paragraph{First Time Calling $\utilde$}
\jiahui{give more explanation here on what it means by "first time"}

\begin{enumerate}
\item Before $\simulator$ makes any queries, the initial state is:
\begin{equation}\label[state_initial]{2-QCCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{a}}\ket{\vb{0}}_{\reg{b}} \ket{1}_{\reg{f}} \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w} \ket{\Init}_{\reg{adv}}
\end{equation}

\jiahui{explain more: why this $a$ message is classical, due to being measured in the actual BQP algorithm}

\item $\simulator$ writes the first prover message $a$ in the communication register $\reg{m}$ and its state evolves into $\ket{\advstate_a}_{\reg{adv}}$:
\begin{equation}\label[state_step0]{2-QCCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{a}}\ket{\vb{0}}_{\reg{b}} \ket{1}_{\reg{f}} \ket{a}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w} \ket{\advstate_a}_{\reg{adv}}
\end{equation}

\item At step 1, $\utilde_1$ performs the SWAP operation between $\reg{a}$ and $\reg{m}$ (conditioned on $H(a) = 1$, which is satisfied); the state in registers will look like:
    \begin{equation}\label[state_step1]{2-QCCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{a}_{\reg{a}}\ket{\vb{0}}_{\reg{b}} \ket{1}_{\reg{f}} \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w} \ket{\advstate_a}_{\reg{adv}}
\end{equation}

\item At step 2, $\utilde_2$ applies the honest verifier operation $U$ to $\reg{ins, a,b, aux, w}$ and writes the verifier message in $\reg{b}$.The auxiliary state and working register state also evolves.
Note that the honest verifier's operation is a purified version; $a$ is w.l.o.g a classical message, so we have:
$U\ket{x}_{\reg{ins}} \ket{a}_{\reg{a}}\ket{\vb{0}}_\reg{b}\ket{\vb{0}}_\reg{w} = \ket{x}_{\reg{ins}} \ket{a}_{\reg{a}}\sum_b \alpha_b \ket{b}_{\reg{b}}\ket{\psi_{a,b}}_\reg{w}$. 
 


We will therefore obtain a purified view on the current state:
\begin{equation}\label[state_step2]{2-QCCC:V:inital:expr}
\sum_b \alpha_b \ket{x}_{\reg{ins}} \ket{a}_{\reg{a}}  \ket{b}_{\reg{b}} \ket{1}_{\reg{f}} \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_a}_{\reg{adv}}
\end{equation}

\begin{MyComment}
    For the sake of clarity, we will ignore the instance register $\reg{x}$ in the expression of the state from now on since it will not be changed during the interaction. But note that the $U$ and $\simulator$ still takes it as input during the computation. 

    As we discussed, because we work in LOCC model (and after we omit $x$), the honest verifier's $U$ can be seen as $U = \sum_a \ket{a}\bra{a}_{\reg{a}} \otimes U_a$
 where $U_a$ operates only on $\reg{b,aux,w}$ registers.
 Here, since $a$ is classical and fixed, we have $U_a \ket{\vb{0}}_\reg{b}\ket{\vb{0}}_\reg{w} =  \sum_b \alpha_b \ket{b}_{\reg{b}}\ket{\psi_{a,b}}_\reg{w}$.
Also note that the basis for the state in register $\reg{b}$ is the computational basis due to classical communication. 
\end{MyComment}

\item At step 3, $\utilde_3$ is a CNOT operation where it copies information in register $\reg{b}$ to $\reg{m}$:

\begin{equation}\label[state_step3]{2-QCCC:V:inital:expr}
\ket{a}_{\reg{a}}  
\sum_b \alpha_b \ket{b}_{\reg{b}} \ket{b}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_a}_{\reg{adv}}
\end{equation}



\item At the end of step 3, the adversary is ready to rewind and call $\utilde^\dagger$. But before rewinding,
the adversary can apply an arbitrary unitary $A_1$ on the communication register $\reg{m}$ and its internal state $\reg{adv}$:

$A_1 (\sum_b \alpha_b^2 \ket{b} \bra{b}_m) \otimes (\ket{\advstate_a} \bra{\advstate_a}_{\reg{adv}}) A_1^\dagger = \sum_{b'} p_{b'} \ket{b',\advstate_{a,b'}}\bra{b',\advstate_{a,b'}}_{\reg{m,adv}} $. By viewing the entire system of $\reg{b,m,w,adv}$, we can decompose them into orthogonal components as follows:
 


\begin{equation}\label[state_step3]{2-QCCC:V:inital:expr}
 \ket{a}_{\reg{a}} 
\sum_{b, b'} \beta_{b',b} 
\ket{b,b'}_{\reg{b,m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b'}}_\reg{w} \ket{\advstate_{a,b,b'}}_{\reg{adv}}
\end{equation}


\end{enumerate}

\paragraph{Rewinding with $\utilde^\dagger$}
\begin{enumerate}
    \item The first step of calling $\utilde^\dagger$ is $\utilde^\dagger_3$, which is the CNOT operation from $\reg{b}$ to $\reg{m}$. The state will split into two branches, those where register $\reg{b}$ and register $\reg{m}$ are equaland those where they are not:
    \begin{equation}\label[state_rewind1]{2-QCCC:V:inital:expr}
\ket{a}_{\reg{a}}   ( \sum_{b = b'} \beta_{b = b'} \ket{b}_{\reg{b}}  \ket{b \oplus b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b}}_{\reg{adv}} +   \sum_{b'\neq b} \beta_{b \neq b'} \ket{b}_{\reg{b}}  \ket{b' \oplus b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b'}}_\reg{w} \ket{\advstate_{a,b,b'}}_{\reg{adv}}) 
\end{equation}
which gives 
\begin{equation}\label[state_rewind1.2]{2-QCCC:V:inital:expr}
\ket{a}_{\reg{a}}   ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \sum_{b'\neq b} \beta_{b'} \ket{b}_{\reg{b}}  \ket{b' \oplus b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b'}}_\reg{w} \ket{\advstate_{a,b,b'}}_{\reg{adv}})
\end{equation}

For convenience, we denote the state $\sum_{b'\neq b} \beta_{b'} \ket{b}_{\reg{b}}  \ket{b' \oplus b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b'}}_\reg{w}\ket{\advstate_{a,b,b'}}_{\reg{adv}}$ as $\ket{\bot_0}$.
Note that $\ket{\bot_0}$ is orthogonal to the "good part" $\sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}}$

\begin{MyComment}
      To keep notations simple, throughout future evolution of the state, $\ket{\bot_0}$ does not denote a particular state, but denotes the''bad'' component where the information register $\reg{m}$ does not equal $\mathbf{0}$. 
\end{MyComment}

\item The second step of $\utilde^\dagger$ is $\utilde^\dagger_2$, which is the honest verifier's $U^\dagger$. As we discussed, once given $a$, we can see $U^\dagger$ as a specific $U^\dagger_a$ operating only on $\reg{b,aux,w}$ registers.
We obtain:

\begin{equation}\label[state_rewind1.2]{2-QCCC:V:inital:expr}
\ket{a}_{\reg{a}} U^\dagger_a  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0})
\end{equation}


\item The last step of $\utilde$ is a $\swap$ operation between register $\reg{a}$ and $\reg{m}$.

Afterwards, $\simulator$
gets to access and makes changes to $\reg{m}$ before it calls $\utilde$ again.
$\simulator$ can perform an arbitrary $A_2$ $\reg{m,adv}$: $A_2 \ket{a}_{\reg{a}} \ket{\advstate}_{\reg{adv}} = \sum_{a'} \ket{a'}_{\reg{a}}\ket{\advstate_{a'}}_{\reg{adv}} $. 

Then we run $\utilde$ which is again a $\swap$ operation between $\reg{m}$ and $\reg{a}$
We can then view the operation $\swap \cdot A_2 \cdot \swap$ as one step:

\begin{align}
\label[state:rewind1.3]{QCCC:V:rewind-one:expr} 
& \gamma_{a}\ket{a}_{\reg{a}} U^\dagger_a  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0}) \\ \nonumber
& + \sum_{a' \neq a} \gamma_{a'}\ket{a'}_{\reg{a}} U^\dagger_a  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a',b,b}}_{\reg{adv}} +   \ket{\bot_0})
%\label[state:rewind1.3]{QCCC:V:rewind-1-3:expr}
\end{align}

We denote the (unnormalized) state $\sum_{a' \neq a} \gamma_{a'}\ket{a'}_{\reg{a}} U^\dagger_a  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a',b,b}}_{\reg{adv}} +   \ket{\bot_0})$ as $\ket{\bot_1}$.

\begin{MyComment}
    Similar to $\ket{\bot_0}$, starting from now on we will use $\ket{\bot_1}$ as the general notation for ''bad'' components where $a' \neq a$ in register $\reg{a}$.
\end{MyComment}



\end{enumerate}

\paragraph{Running $\utilde$ Again} 
Now $\simulator$ is ready to run $\utilde$ again. 

\begin{enumerate}
\item We have already performed the first step $\utilde_1$, which is a SWAP between register $\reg{a}$ and register $\reg{m}$. Therefore we proceed to the next step $\utilde_2$, which is a controlled version of the honest verifier's operation $U_a$ on registers $\reg{b, w}$, \emph{conditioned on that $H(a) = 1$ in $\reg{a}$ register}. Accordingly, $U$ will only apply to the components where $a$ in register $\reg{a}$ stays unchanged and not to the $\ket{\bot_1}$ part:


\begin{align}
\label[state_down2.1]{QCCC:V:down2:expr}
& \gamma_{a}\ket{a}_{\reg{a}} U_a U^\dagger_a  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0}) +  \ket{\bot_1} \\ \nonumber
& = \gamma_{a}\ket{a}_{\reg{a}}  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{0}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0}) 
 +  \ket{\bot_1} 
 \end{align}


\item Next, we apply $\utilde_3$ which is a controlled CNOT:
\begin{align}
\label[state_down2.2]{QCCC:V:down2:expr}
& \gamma_{a}\ket{a}_{\reg{a}}  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0}) 
 +  \ket{\bot_1} 
 \end{align}

 \item At the end of running $\utilde$, the adversary is ready to rewind and call $\utilde^\dagger$. But before rewinding,
the adversary can apply an arbitrary unitary $A_1$ on the communication register $\reg{m}$ and its internal state $\reg{adv}$:

$A_1 (\sum_b \alpha_b^2 \ket{b} \bra{b}_m) \otimes (\ket{\advstate_a} \bra{\advstate_a}_{\reg{adv}}) A_1^\dagger = \sum_{b'} p_{b'} \ket{b',\advstate_{a,b'}}\bra{b',\advstate_{a,b'}}_{\reg{m,adv}} $. By viewing the entire system of $\reg{b,m,w,adv}$, we can decompose them into orthogonal components as follows:
\begin{align}
\label[state_down2.3]{QCCC:V:down3:expr}
& \gamma_{a}\ket{a}_{\reg{a}}  ( \sum_{b} \beta_{b,2} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,2}}_\reg{w} \ket{\advstate_{a,b,b,2}}_{\reg{adv}} +   \ket{\bot_0}) 
 +  \ket{\bot_1} 
 \end{align}

 Note that the amplitude for the components in the above state where register $\reg{b}$ equals register $\reg{m}$ has changed after the adversarial operation $A_1$. To differentiate this amplitude from its previous value, we name it $\beta_{b,2}$.
 

 \jiahui{Maybe color the different components?}

\end{enumerate}


\subsection{Simulator's View in the World of $U_\bot$}
\label{sec:sim_view_udummy}

In this section, we show the evolution of the registers where we use $U_\bot$ and $U_\bot^\dagger$ instead of $\utilde, \utilde^\dagger$, \emph{except for the "first time".}

\jiahui{explain why this is the "first time" due to measure-and-reprogram}

\paragraph{First Time Calling $\utilde$}

Since we use the same $\utilde$ for the first time, not $U_\bot$, we obtain the same state after calling $\utilde$ and after $\simulator$ has applied $A_2$ as in \cref{sec:sim_view_udummy}:

\begin{align}
\label[state_dummy_step3]{2-QCCC:V:initial:dummy}
 & \ket{a}_{\reg{a}} 
\sum_{b, b'} \beta_{b',b} 
\ket{b,b'}_{\reg{b,m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b'}}_\reg{w} \ket{\advstate_{a,b,b'}}_{\reg{adv}} \nonumber \\
& = \ket{a}_{\reg{a}} 
(\sum_{b} \beta_{b} 
\ket{b,b}_{\reg{b,m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} + \sum_{b} \beta_{b'\neq b} 
\ket{b,b'}_{\reg{b,m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b'}}_\reg{w} \ket{\advstate_{a,b,b'}}_{\reg{adv}} ) \nonumber  \\
& = \ket{a}_{\reg{a}} 
(\sum_{b} \beta_{b} 
\ket{b,b}_{\reg{b,m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} + \ket{\bot_0} )
\end{align}


\paragraph{Rewinding with $U^\dagger_\bot$}
 \begin{enumerate}
     \item Recall that $U_\bot =\swap_{\reg{a,m}}  \cdot \mathbf{I} \cdot \mathbf{I} \cdot \mathbf{I} $ is an identity operator except for the first step on SWAP  registers $\reg{a,m}$, so  $U^\dagger_\bot = \mathbf{I} \cdot \mathbf{I} \cdot \mathbf{I} \cdot \swap_{\reg{a,m}}$.

   Therefore, upon rewinding, the state we obtain before calling $\swap_{\reg{a,m}}$ is still as in expression \ref{2-QCCC:V:initial:dummy}.

\item After we call $\swap_{\reg{a,m}}$, $\simulator$
gets to access and make changes to $\reg{m}$.

$\simulator$ can perform an arbitrary $A_2$ jointly to registers $\reg{m,adv}$: $A_2 \ket{a}_{\reg{a}} \ket{\advstate}_{\reg{adv}} = \sum_{a'} \ket{a'}_{\reg{a}}\ket{\advstate_{a'}}_{\reg{adv}}$. 

Then we will run $U_\bot$ which begins with a $\swap$ operation between $\reg{m}$ and $\reg{a}$ .
For convenience, We can then view the operation $\swap_{\reg{a,m}} \cdot A_2 \cdot \swap_{\reg{a,m}}$ as one step:
\begin{align}
\label[state_dummy:rewind1.3]{QCCC:V:dummy:rewind-three:expr} 
& \gamma_{a}\ket{a}_{\reg{a}}  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0}) \nonumber \\ 
& + \sum_{a' \neq a} \gamma_{a'}\ket{a'}_{\reg{a}}   ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a',b,b}}_{\reg{adv}} +   \ket{\bot_0}) \nonumber \\
& = \gamma_{a}\ket{a}_{\reg{a}}  ( \sum_{b} \beta_{b} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b}}_\reg{w} \ket{\advstate_{a,b,b}}_{\reg{adv}} +   \ket{\bot_0}) + \ket{\bot_1}
\end{align}

 \end{enumerate}

\paragraph{Running $U_\bot$}
\begin{enumerate}
\item Now when $\simulator$ queries the verifier again, we start to use  $U_\bot$. 
Since we have already performed the first step of $U_\bot$, $\swap_{\reg{a,m}}$ above, we only need to perform the rest identity operators. Our state remains unchanged from \ref{QCCC:V:dummy:rewind-three:expr} after performing the rest of $U_\bot$.

\item At the end of running $U_\bot$, $\simulator$ is ready to rewind and call $U_\bot^\dagger$. But before rewinding,
it can apply an arbitrary unitary $A_1$ on the communication register $\reg{m}$ and its internal state $\reg{adv}$. Thus we obtain:
\begin{align}
\label[state_dummy_down2.3]{QCCC:V:dummy:down3:expr}
& \gamma_{a}\ket{a}_{\reg{a}}  ( \sum_{b} \beta_{b,2} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,2}}_\reg{w} \ket{\advstate_{a,b,b,2}}_{\reg{adv}} +   \ket{\bot_0}) 
 +  \ket{\bot_1} 
 \end{align}
 
 Note that the amplitude for the components in the above state where register $\reg{b}$ equals register $\reg{m}$ has changed after the adversarial operation $A_1$. To differentiate this amplitude from its previous value, we name it $\beta_{b,2}$.
 
\end{enumerate}

\subsection{Indistinguishability of the $\utilde$ and $U_\bot$ worlds}

Let us denote the components in state over registers $\reg{a,b,m,aux,adv}$ where $H(a) = 1$ in register $\reg{a}$. %%%%%%%and $\reg{b} = \reg{m}$ as the "good branch".

\begin{claim}
The state in the good branch are identical in the following two worlds for the same polynomial $k$:
\begin{enumerate}
    \item World $\utilde$: $\simulator$ calls $\utilde$ and $\utilde^\dagger$ alternatively, for $k$ times and $(k-1)$-times respectively. We denote $\utilde^{(i)}$ and $\utilde^{\dagger,(i)}$ as the $i$-th time of calling $\utilde$ and $\utilde^{\dagger}$ respectively.
    $$\utilde^{(1)}, \utilde^{\dagger,(1)}, \utilde^{(2)}, \utilde^{\dagger,(2)}, \cdots, \utilde^{\dagger,(k-1)}, \utilde^{(k)}$$

    \item World $U_\bot$: $\simulator$ first calls $\utilde$, and then calls $U_\bot^\dagger$  and $U_\bot$ and alternatively, for $(k-1)$-times respectively. 
    
    We denote $U_\bot^{(i)}$ and $U_\bot^{\dagger,(i)}$ as the $i$-th time of calling $U_\bot$ and $U_\bot^{\dagger}$ respectively (note that $U_\bot^{(i)}$ begins with $i = 2$.
    $$\utilde^{(1)}, U_\bot^{\dagger,(1)}, U_\bot^{(2)}, U_\bot^{\dagger,(2)}, \cdots, U_\bot^{\dagger,(k-1)}, U_\bot^{(k)}$$, we
    
\end{enumerate} 
\end{claim}

\begin{proof}
We prove by induction.

\jiahui{be careful defining what's the base case}

\textbf{The base case}, we have already shown in the previous two sections \ref{sec:sim_view_utilde}, \ref{sec:sim_view_udummy}: after calling $\utilde^{(1)}, \utilde^{\dagger,(1)}, \utilde^{(2)}$ or calling $\utilde^{(1)}, U_\bot^{\dagger,(1)}, U_\bot^{(2)}$, we obtain the same state $\gamma_{a}\ket{a}_{\reg{a}}  \sum_{b} \beta_{b,2} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,2}}_\reg{w} \ket{\advstate_{a,b,b,2}}_{\reg{adv}}$. 


\textbf{ $k \to (k+1)$ Case}: Suppose that, in the $\utilde$-world, after calling $\utilde^{(1)}, \utilde^{\dagger,(1)}, \utilde^{(2)}, \utilde^{\dagger,(2)}, \cdots, \utilde^{\dagger,(k-1)}, \utilde^{(k)}$, and in the $U_\bot$-world, after calling $\utilde^{(1)}, U_\bot^{\dagger,(1)}, U_\bot^{(2)}, U_\bot^{\dagger,(2)}, \cdots, U_\bot^{\dagger,(k-1)}, U_\bot^{(k)}$, we have the good branch as follows for both worlds: 

\begin{align}
\label[state_down:k]{QCCC:V:down:k}
& \gamma_{a, (k)}\ket{a}_{\reg{a}}   \sum_{b} \beta_{b,(k)} \ket{b}_{\reg{b}}  \ket{b}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,k}}_\reg{w} \ket{\advstate_{a,b,b,k}}_{\reg{adv}}
 \end{align}

Then in the $\utilde$-world, we call $\utilde^\dagger$ and $\utilde$ again. We analyze the evolution of the state:
\begin{itemize}
    \item First $\utilde^\dagger$ applies the controlled CNOT: conditioned on that $H(a) = 1$, copying register
$\reg{b}$ into register $\reg{m}$. Since we only consider the good branch, we have:
\begin{align}
\label[state_rewind:k.1]{QCCC:V:rewind:k}
& \gamma_{a, (k)}\ket{a}_{\reg{a}}   \sum_{b} \beta_{b,(k)} \ket{b}_{\reg{b}}  \ket{\vec{0}}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,k}}_\reg{w} \ket{\advstate_{a,b,b,k}}_{\reg{adv}}
 \end{align}

 \item Next $\utilde^\dagger$ applies the honest verifier's $U^\dagger$ ($U^\dagger_a$ in our setting) conditioned on $H(a) = 1$:
 \begin{align}
\label[state_rewind:k]{QCCC:V:rewind:k}
& \gamma_{a, (k)}\ket{a}_{\reg{a}} U_a^\dagger  \sum_{b} \beta_{b,(k)}
 \ket{b}_{\reg{b}}  \ket{\vec{0}}_{\reg{m}}
\ket{H}_{\reg{aux}}\ket{\psi_{a,b,k}}_\reg{w} \ket{\advstate_{a,b,b,k}}_{\reg{adv}}
 \end{align}

 


\end{itemize}

\end{proof}

\UpdateLine 

\xiao{to do...}





==> sections/CPM-babycase-simplified-part-2.tex <==
\section{Soundness Reduction (Part 1/2)}
\label{sec:CPM-3ZK:decider:lem:soundness:proof}

In this section, we prove \Cref{CPM-3ZK:decider:lem:soundness}. 

At a high level, we assume for contradiction that  \Cref{CPM-3ZK:decider:lem:soundness} is false and show how to construct a malicious prover $\tilde{\Prover}$ breaking the soundness of the original LOCC ZK protocol. Toward that, we first need to make some modifications to the machine $\mcal{B}$ and the MnR game $\Sim^{\tilde{\Verifier}}$, making use of some particular properties of the $\tilde{\Verifier}$ we defined earlier. This is done in \xiao{cref}. Next, we will present the malicious prover $\tilde{\Prover}$ and prver that it can indeed break the soundness. This is done in \xiao{cref}.


\subsection{Cleaning the MnR Game}
In \Cref{CPM-3ZK:MnR:game:modify:1}, we present a modified version of the MnR game $\Sim^{\tilde{\Verifier}}[H, \vb{y}]$ defined in \Cref{CPM-3ZK:MnR:game}. Since we will be interested only in the case $H = H_0$ and $\vb{y} = \vb{1} = (1, 1)$, we present this case only. We highlight its difference with \Cref{CPM-3ZK:MnR:game} in \red{red color}.


\begin{GameBox}[label={CPM-3ZK:MnR:game:modify:1}]{Measure-and-Reprogram Game \textnormal{$\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$}}
 It works as follows
\begin{enumerate}
\item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:1}
For each $i\in[K]$, uniformly pick \dlt{$(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$} \red{$j_i \in [q] \cup \Set{\bot}$} conditioned on that there exists at most one $i\in [K]$ such that $j_i=j^*$  for all $j^*\in [q]$. 

\item
 Let $s$ denote the number of $j_i$'s in $\Set{j_i}_{i \in [k]}$ that are not $\bot$.  We re-label the indices $i$ for \dlt{pairs $\Set{(j_i, b_i)}_{i \in [K]}$} \red{$\Set{(j_i)}_{i \in [K]}$} so that $j_1 < j_2 < \ldots < j_s$ and $j_{s+1} = j_{s+2} =\ldots = j_K = \bot$.

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes \red{$H_0$}, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:4:a} 
      If $j=j_i$ for some $i\in[s]$, measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, z_i})$ where $z_i \in [K]$ is determined by the measurement outcome, 
      \red{\begin{itemize}
      \item
      {\bf Defining $\msf{sq}(i)$:} Note that the $j_i$-th query to $\mcal{O}$ must be invoked by $\Sim$'s query to verifier $\tilde{\Verifier}$. We will call this $\Sim$'s query (that invokes the $j_i$-th query to $\mcal{O}$) as the $i$-th special query and denote it by $\msf{sq}(i)$. 
      % We establish certain properties of $\msf{sq}(i)$ in \Cref{CPM-3ZK:MnR:game:modify:1:lem}, which will be useful later. 
      \end{itemize}
      }

      It then behaves \dlt{according to the value $b_i$} as follows:
        \begin{enumerate}
        \item 
        \dlt{If $b_i=0$:} First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$, and then answer the $j_i$-th query using the reprogrammed oracle.
        \item 
        \dlt{If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$.} 
        \end{enumerate}
    \item 
    Otherwise (i.e., $j \ne j_i$ $\forall i \in [s]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, \ldots, p^*_K), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{CPM-3ZK:MnR:notation:item:2}).

\item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:4}
For all $i \in \Set{s+1, s+2, \ldots, K}$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}^*_i \coloneqq (p^*_1, \ldots, p^*_i)$. 

\item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:5}
{\bf Output:}   The output of this game is defined as follows
\begin{itemize}
\item
If it holds for all $i \in [K]$ that $\vb{p}_i$ is a prefix of $\vb{p}_K$, then output $(\vb{p}_K, \rho_{\msf{out}})$;

\item
Otherwise, output $(\bot, \bot)$.
\end{itemize}
\end{enumerate}
\end{GameBox}

\begin{lemma}\label{CPM-3ZK:MnR:game:modify:1:lem}
For the $\dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ defined in \Cref{CPM-3ZK:MnR:game:modify:1} and the $\mcal{B}(x)$ defined in \Cref{CPM-3ZK:BQP-decider}, it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]]\ge \frac{1}{2^k} \cdot \Pr[\mcal{B}(x) = 1].$$
\end{lemma}
\begin{proof}[Proof of \Cref{CPM-3ZK:MnR:game:modify:1:lem}]
First, recall that by the definition of $\mcal{B}(x)$ (see \Cref{CPM-3ZK:BQP-decider}), it holds that
$$\Pr[\mcal{B}(x) = 1 ] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la {\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]].$$ 
Thus, proving \Cref{CPM-3ZK:MnR:game:modify:1:lem} is all about comparing \Cref{CPM-3ZK:MnR:game:modify:1} with the game ${\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ (i.e., \Cref{CPM-3ZK:MnR:game} with $H =  H_0$ and $\vb{y} = \vb{1}$).

Next, note that \Cref{CPM-3ZK:MnR:game:modify:1} is identical to  ${\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ conditioned on the event that none of the $b_i$'s is $1$ in the latter. Moreover, from the description in \Cref{CPM-3ZK:MnR:game:modify:1:step:1}, this event happens with probabiity at least $\frac{1}{2^k}$. Thus, the inequality in \Cref{CPM-3ZK:MnR:game:modify:1:lem} holds.  

(We remark that the definition of $\msf{sq}(i)$ in \Cref{CPM-3ZK:MnR:game:modify:1:step:4:a} does not affect the game as all, because just a definition. Also note that the game does not make use of the $b_i$'s. Thus, we do not sample them anymore.)


This completes the proof of \Cref{CPM-3ZK:MnR:game:modify:1:lem}.

\end{proof}

\para{Structure of $z_i$'s.}
\xiao{we prove some properties of the $z_i$'s defined in \Cref{CPM-3ZK:MnR:game:modify:1:step:4:a} in \Cref{CPM-3ZK:MnR:game:modify:1}.}

\begin{lemma}\label{MnR:game:modify:1:z:non-devreasing:lemma}
For the $s$ and $\Set{z_t}_{t \in [s]}$ defined in \Cref{CPM-3ZK:MnR:game:modify:1}, it holds that\footnote{In \Cref{MnR:game:modify:1:z:non-devreasing:lemma} and its proof, for the corner case $t= 1$, the $\max$ is taken over $\emptyset$. We naturally define $\max(\emptyset) = 0$. }
$$\forall t \in [s],~ z_t \le \max\{z_1, z_2 \ldots, z_{t-1}\} + 1. ~~(\text{In particular, $z_1 = 1$ if $s\ge 1$.})$$
\end{lemma}
\begin{proof}
In the following proof, (arbitrarily) fix a $t \in [s]$.
 
Consider the moment of the execution when $\Sim$ is about to make the $\msf{sq}(t)$ query (i.e., the query that will invoke the measurement of $z_t$). Let us denote the overall state across all the registers as $\rho$. Let us denote $z \coloneqq \max\{z_1, z_2, \ldots, z_{t-1}\}$.

 At this moment, we know by definition of \Cref{CPM-3ZK:MnR:game:modify:1} that the oracle $H_0$ has been re-programmed to output 1 for input vectors of length {\em at most $z$}. In particular, if we denote the oracle at this moment as $\hat{H}$, then it outputs $0$ on all vectors $(p_1, \ldots, p_{z+1})$ of length $z+1$.

Next, we claim that 
$$
\forall v \in\Set{z+1, z+2, \ldots, K},~ \Tr[\ketbra{v}_{\reg{lc}} \rho] = 0,
$$ 
where $\ketbra{v}_{\reg{lc}}$ is the projector that projects register $\reg{lc}$ to value $v$. That is, we claim that the $\reg{lc}$ register of state $\rho$ does not have any weights on value $v \ge z+1$. This is because:
\begin{enumerate}
 \item
 by the definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}), for $\reg{lc}$ to contain the value $z+1$ or greater, it is necessary that there exists some $(p_1, \ldots, p_{z+1})$ such that $H(p_1, \ldots, p_{z+1}) = 1$;
 \item
 as we just argued, it holds for the current oracle $\hat{H}$ that $\hat{H}(p_1, \ldots, p_{z+1}) = 0$ for all possible $(p_1, \ldots, p_{z+1})$.
 \end{enumerate}

Now, let us consider the $\msf{sq}(t)$ query. We first claim that at this moment, the (classical)\footnote{Recall from \Cref{item:fact:gc} that the the global counter is always classical throughout the execution.} global counter value $g$ must satisfy $g \le z$. If not (i.e., $g \ge z+1$), then by definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}) and the fact that the $\reg{lc}$ register does not have any weights on $z+1$ or greater, this query will not invoke the measurement of any $\reg{p_i}$ registers simply because it falls into the ``{\bf Case} ($i \ne j$)'' in \Cref{CPM-3ZK:V:unitary}. This contradicts the fact that the current query is the $\msf{sq}(t)$ query (which must invoke the measurement of some $\reg{p_i}$ registers.)

Therefore, the only possibility is the that global counter value $g \le z$. In this case, by definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}), the $\msf{sq}(t)$ query will invoke the measurement of at most $\reg{p_1, \ldots, p_{g+1}}$ (i.e., the length of measured  registers will not exceed $g+1$). In this case, $z_t \le g+1$ and thus $z_t \le z + 1$, satisfying the requirement of \Cref{MnR:game:modify:1:z:non-devreasing:lemma}.

Finally, we remark that the above argument implies $z_1 \le 1$ as a particular case. On the other hand, if $s \ge 1$, then $z_1$ by definition lies in $[K]$. Thus, it follows that $z_1 = 1$. 

This completes the proof of \Cref{MnR:game:modify:1:z:non-devreasing:lemma}.

\end{proof}


\xiao{Excluding bad events}
We next show in \Cref{MnR:game:modify:1:z:non-devreasing:cor} a powerful corollary of \Cref{MnR:game:modify:1:z:non-devreasing:lemma}. 
\begin{corollary}[of \Cref{MnR:game:modify:1:z:non-devreasing:lemma}]\label{MnR:game:modify:1:z:non-devreasing:cor}
For \Cref{CPM-3ZK:MnR:game:modify:1}, define the following event $E_\msf{bad}$
$$E_\msf{Bad} \coloneqq (s \ne K) \vee (z_1 \ne 1) \vee (z_2 \ne 2) \vee \ldots \vee (z_K \ne K).$$
It then follows that
$$\Pr[\msf{Pred}(\rho) = 1 ~\wedge~E_\msf{Bad} ~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] = 0.$$
\end{corollary}
\begin{proof}[Proof of \Cref{MnR:game:modify:1:z:non-devreasing:cor}]
We first define another ``bad'' event $\tilde{E}_{\msf{Bad}}$
$$\tilde{E}_{\msf{Bad}} \coloneqq \big(\max\{z_1, \ldots, z_s\} < K\big).$$
Then, by \Cref{MnR:game:modify:1:z:non-devreasing:lemma}, it is not hard to see that the event that ``$\tilde{E}_{\msf{Bad}}$ happens'' implies the event that ``$E_\msf{Bad}$ happens.''

Therefore, to prove \Cref{MnR:game:modify:1:z:non-devreasing:cor}, it suffices to prove the following inequality:
\begin{equation}\label[Inequality]{MnR:game:modify:1:z:non-devreasing:cor:inter:ineq}
\Pr[\msf{Pred}(\rho) = 1 ~\wedge~\tilde{E}_\msf{Bad} ~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] = 0
\end{equation}
The proof for \Cref{MnR:game:modify:1:z:non-devreasing:cor:inter:ineq} is very similar to that for \Cref{MnR:game:modify:1:z:non-devreasing:lemma}. We include it below for the sake of completeness.   

Let $z \coloneqq \max\{z_1, \ldots, z_s\}$. If event $\tilde{E}_{\msf{Bad}}$ happens, we know that $z < K$. Now, consider the moment when the $\Sim$ halts. At this moment, we know by definition of \Cref{CPM-3ZK:MnR:game:modify:1} that the oracle $H_0$ has been re-programmed to output 1 for input vectors of length {\em at most $z < K$}. In particular, if we denote the oracle at this moment as $\hat{H}$, then it outputs $0$ on all vectors $(p_1, \ldots, p_{K})$ of length $K$.

Next, we claim that 
\begin{equation}\label{MnR:game:modify:1:z:non-devreasing:cor:eq:K:weights}
\Tr[\ketbra{K}_{\reg{lc}} \rho] = 0,
\end{equation}
where $\ketbra{K}_{\reg{lc}}$ is the projector that projects register $\reg{lc}$ to value $K$. That is, we claim that the $\reg{lc}$ register of the final state $\rho$ at $\Sim$'s halt does not have any weights on value $K$. This is because:
\begin{enumerate}
 \item
 by the definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}), for $\reg{lc}$ to contain the value $K$, it is necessary that there exists some $(p_1, \ldots, p_K)$ such that $H(p_1, \ldots, p_K) = 1$;
 \item
 as we just argued, it holds for the current oracle $\hat{H}$ that $\hat{H}(p_1, \ldots, p_K) = 0$ for all possible $(p_1, \ldots, p_K)$.
 \end{enumerate}
In this case, \Cref{MnR:game:modify:1:z:non-devreasing:cor:eq:K:weights} implies that $\msf{Pred}(\rho) = 0$ (recall the definition of $\msf{Pred}$ in \Cref{CPM-3ZK:BQP-decider}). 

This completes the proof of \Cref{MnR:game:modify:1:z:non-devreasing:cor}.

\end{proof}


\Cref{MnR:game:modify:1:z:non-devreasing:cor} is powerful in the sense that it allows us to further clean the game $\dot{S}^{\tilde{V}}[H_0, \vb{1}]$ (i.e., \Cref{CPM-3ZK:MnR:game:modify:1}) in the following manner: during the execution of \Cref{CPM-3ZK:MnR:game:modify:1}, once the event $E_\msf{Bad}$ occurs, we can immediately abort the execution (possibly prematurely), without reducing the probability of $\msf{Pred}(\rho) = 1$. We formalize this observation as the following 
\Cref{CPM-3ZK:MnR:game:modify:2} (where we highlight its difference with \Cref{CPM-3ZK:MnR:game:modify:1} in \red{red color}) and \Cref{MnR:game:modify:2:cor}.


\begin{GameBox}[label={CPM-3ZK:MnR:game:modify:2}]{Measure-and-Reprogram Game \textnormal{$\ddot{\Sim}^{\tilde{\Verifier}}[H_0, \vb{1}]$}}
 It works as follows
\begin{enumerate}
\item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:1}
For each $i\in[K]$, uniformly pick $j_i \in [q]$ \dlt{$\cup \Set{\bot}$} conditioned on that there exists at most one $i\in [K]$ such that $j_i=j^*$  for all $j^*\in [q]$. 

\item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:2}
 \dlt{Let $s$ denote the number of $j_i$'s in $\Set{j_i}_{i \in [k]}$ that are not $\bot$.  We re-label the indices $i$ for $\Set{(j_i)}_{i \in [K]}$ so that $j_1 < j_2 < \ldots < j_s$ and $j_{s+1} = j_{s+2} =\ldots = j_K = \bot$.}

\red{We re-label the indices $i$ for $\Set{(j_i)}_{i \in [K]}$  so that $j_1 < j_2 < \ldots < j_K$.}

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes $H_0$, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:4:a} 
      If $j=j_i$ for some $i\in[\red{K}]$, measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, z_i})$ where $z_i \in [K]$ is determined by the measurement outcome. \red{It halts immediately and outputs $(\bot, \bot)$ if any of the following events happen:
      \begin{enumerate}
        \item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:3:a:i} 
        $z_i \ne i$, {\em or}
      \item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:3:a:ii} 
        $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$. 
      \end{enumerate}
      } 
      (The $\msf{sq}(i)$ queries are defined in the same manner as in \Cref{CPM-3ZK:MnR:game:modify:1}.)
      

      It then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, 1)$ and then answer the $j_i$-th query using the reprogrammed oracle.
        
    \item 
    Otherwise (i.e., $j \ne j_i$ $\forall i \in [\red{K}]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, \ldots, p^*_K), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{CPM-3ZK:MnR:notation:item:2}).

\item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:5}
\dlt{For all $i \in \Set{s+1, s+2, \ldots, K}$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}^*_i \coloneqq (p^*_1, \ldots, p^*_i)$.} 

\item \label[Step]{CPM-3ZK:MnR:game:modify:2:step:6}
{\bf Output:}   \red{directly output $(\vb{p}_K, \rho_{\msf{out}})$} 
\dlt{The output of this game is defined as follows}
\begin{itemize}
\item
\dlt{If it holds for all $i \in [K]$ that $\vb{p}_i$ is a prefix of $\vb{p}_K$, then output $(\vb{p}_K, \rho_{\msf{out}})$;}

\item
\dlt{Otherwise, output $(\bot, \bot)$.}
\end{itemize}

\end{enumerate}
\end{GameBox}

\begin{corollary}[of \Cref{MnR:game:modify:1:z:non-devreasing:cor}]\label{MnR:game:modify:2:cor}
For the $\dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ defined in \Cref{CPM-3ZK:MnR:game:modify:1} and the $\ddot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ defined in \Cref{CPM-3ZK:MnR:game:modify:2} , it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \ddot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] \ge \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]].$$
\end{corollary}
\begin{proof}[Proof of \Cref{MnR:game:modify:2:cor}]
We prove this corollary by considering the \red{red-color} changes in \Cref{CPM-3ZK:MnR:game:modify:2} one by one.

In \Cref{CPM-3ZK:MnR:game:modify:2:step:1}, we simply prevent the value $j_i$ from taking the value $\bot$. This follows immediately from \Cref{MnR:game:modify:1:z:non-devreasing:cor}---if there exists some $j_i = \bot$, then it must follow that $s \ne K$, which is a part of the $E_{\msf{Bad}}$ defined in  \Cref{MnR:game:modify:1:z:non-devreasing:cor}. Thus, we can safely ignore this case without reducing the probability of $\msf{Pred}(\rho) = 1$.

The changes made in \Cref{CPM-3ZK:MnR:game:modify:2:step:2,CPM-3ZK:MnR:game:modify:2:step:5} are direct consequences of the adjustment made in \Cref{CPM-3ZK:MnR:game:modify:2:step:1}.

The introduction of \Cref{CPM-3ZK:MnR:game:modify:2:step:3:a:i} can also be elucidated by \Cref{MnR:game:modify:1:z:non-devreasing:cor}. Specifically, the occurrence of the event $z_i \neq i$ is encompassed within the definition of $E_{\msf{Bad}}$ outlined in \Cref{MnR:game:modify:1:z:non-devreasing:cor}. Consequently, we can safely disregard this scenario without diminishing the probability of $\msf{Pred}(\rho) = 1$.

The inclusion of \Cref{CPM-3ZK:MnR:game:modify:2:step:3:a:ii} essentially involves relocating the checks conducted in the original \Cref{CPM-3ZK:MnR:game:modify:2:step:6} to an earlier stage, specifically within the current \Cref{CPM-3ZK:MnR:game:modify:2:step:3:a:ii}.

This finishes the proof of \Cref{MnR:game:modify:2:cor}.

\end{proof}

\begin{remark}[The Type of $\msf{sq}(i)$ Query]\label{rmk:sq:type} 
We remark that in \Cref{CPM-3ZK:MnR:game:modify:2}, the $\msf{sq}(i)$ query must be a $\tilde{V}$ query (instead of being  a $\tilde{V}^\dagger$ query). This follows from a similar argument as we did in the proof of \Cref{MnR:game:modify:1:z:non-devreasing:lemma}. In more detail, note that the $\msf{sq}(i)$ query by definition invokes the measurement of $\reg{p_1\ldots p_i}$. If it is invoked by a $\tilde{V}^\dagger$ query, then by the definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}),  both the global counter and the local counter must be of the same value $i$ {\em right before this query}. However, this is simply impossible---using the argument as we did in the proof of \Cref{MnR:game:modify:1:z:non-devreasing:lemma}, the $\reg{lc}$ register has zero weights on value $i$ before the $\msf{sq}(i)$ query is processed. Therefore, the $\msf{sq}(i)$ query must be a $\tilde{V}$ query. 
\end{remark}


\subsubsection{Simplification Assumptions} 
Henceforth, we make three assumptions regarding the behavior of the simulator $\Sim$  that would greatly simplify the remainder of our proof. We first present two assumptions which are easy to state and validate.
\begin{itemize}
\item 
\hypertarget{CPM-3ZK:simp-assumption:1}{{\bf Assumption 1:}} When the global counter is $\ket{0}_{\reg{gc}}$,\footnote{Note that due to \Cref{item:fact:gc}, we do not need to consider the case where the global counter is a superposition.} $\Sim$ will not make a $\tilde{V}^\dagger$ query.

\item 
\hypertarget{CPM-3ZK:simp-assumption:2}{{\bf Assumption 2:}} When the global counter is $\ket{K}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ query.
\end{itemize}
We argue that these assumptions will not decrease the probability of $\msf{Pred}(\rho) = 1$ for \Cref{CPM-3ZK:MnR:game:modify:2}. To see that, consider that scenario where the $\Sim$ makes a $\tilde{V}^\dagger$ (resp.\ $\tilde{V}$) query when global counter is $\ket{0}_{\reg{gc}}$ (resp.\ $\ket{K}_{\reg{gc}}$). By the definition in \Cref{CPM-3ZK:V:unitary}, the effect of this $\tilde{V}^\dagger$ (resp.\ $\tilde{V}$) query is to apply the identity operator (i.e., do nothing). Thus, such a query has no effects on the overall states at all and can be ignored. More accurately, one can define another machine $\Sim^*$ that behaves identically to $\Sim$ except that when $\Sim$ tries to make a $\tilde{V}^\dagger$ (resp.\ $\tilde{V}$) query at $\ket{0}_{\reg{gc}}$ (resp.\ $\ket{K}_{\reg{gc}}$), $\Sim^*$ does not do anything and pretend that this query has been answered. The probability of $\msf{Pred}(\rho) = 1$ for \Cref{CPM-3ZK:MnR:game:modify:2} w.r.t.\ this new $\Sim^*$ is then identical to that of the original \Cref{CPM-3ZK:MnR:game:modify:2}. 

Next, we state and validate the third assumption.
\begin{itemize}
\item 
\hypertarget{CPM-3ZK:simp-assumption:3}{{\bf Assumption 3:}} For each $i \in [K]$, {\em before the $\msf{sq}(i)$ query is made}, we allow $\Sim$ to operate directly on registers $\reg{t_j}$ for all $j \in \Set{i+1, i+2, \ldots, K}$. Then, for each $i \in [K]$, before the $\msf{sq}(i)$ query is made, $\Sim$ will not try to make a $\tilde{V}$-query when the global counter is $\ket{i}_{\reg{gc}}$.
\end{itemize}
We now argue that \hyperlink{CPM-3ZK:simp-assumption:3}{{\bf Assumption 3}} will not decrease the probability of $\msf{Pred}(\rho) = 1$ for \Cref{CPM-3ZK:MnR:game:modify:2}.
Consider the scenario where before the $\msf{sq}(i)$ query is made, $\Sim$ makes a $\tilde{V}$ when the global counter is $\ket{i}_{\reg{gc}}$. At this moment, via the same argument as in the proof of \Cref{MnR:game:modify:1:z:non-devreasing:lemma} and \Cref{MnR:game:modify:1:z:non-devreasing:cor}, we know that the local counter register does not have any weights on value $i$. Therefore, this $\tilde{V}$ query falls into the ``{\bf Case $(i\ne j)$}'' category in \Cref{CPM-3ZK:V:unitary} and thus the operator $C'_{i+1}A_{i+1}$ will be applied. From $\Sim$'s view point, the only effect of $C'_{i+1}A_{i+1}$ is to move the contents of $\reg{t_{i+1}}$ to the $\reg{m}$ register, which can be seen and modified by $\Sim$. Moreover, note that after this query, the global counter has been increase to the value $i+1$ while the global counter does not increase at all. Therefore, future $\tilde{V}$ queries (before $\msf{sq}(i)$) will always been answered by $C'_{j}A_{j}$ according to the global counter value $j$, {\em until $\Sim$ makes enough $\tilde{V}^\dagger$ queries to bring the global counter back to value $i$}. Therefore, instead of allowing $\Sim$ to perform these queries, one can define another machine $\Sim^*$ that behaves identically to $\Sim$ except that when $\Sim$ tries to make a $\tilde{V}$ query at $\ket{i}_{\reg{gc}}$ before the $\msf{sq}(i)$ query, $\Sim^*$ dose not make this query; instead it operates directly on register $\reg{t_{j+1}}$ if the global operator before this query was $\ket{j}_{\reg{gc}}$. The probability of $\msf{Pred}(\rho) = 1$ for \Cref{CPM-3ZK:MnR:game:modify:2} w.r.t.\ this new $\Sim^*$ is then identical to that of the original \Cref{CPM-3ZK:MnR:game:modify:2}. This is exactly what we allowed in \hyperlink{CPM-3ZK:simp-assumption:3}{{\bf Assumption 3}}.


\subsection{Defining the Real Game} 

\xiao{add intuitive explanations.}

\para{Looking into $\Sim^{\tilde{\Verifier}}$.} Next, we re-state the game $\ddot{\Sim}^{\tilde{\Verifier}}[H_0, \vb{1}]$ defined in \Cref{CPM-3ZK:MnR:game:modify:2}. This time, we will look into the execution of $\Sim^{\tilde{\Verifier}}$ and their registers. This is different from previous games where we always treat $\Sim^{\tilde{\Verifier}}$ as a ``black-box'' and only focus on how it accesses the oracle $H_0$. We denote this game as $\msf{Real}(\Sim, \tilde{\Verifier})$ and present it in \Cref{CPM-3ZK:MnR:game:real}.       

It is straightforward that \Cref{CPM-3ZK:MnR:game:real} is identical to \Cref{CPM-3ZK:MnR:game:modify:2} with only cosmetic changes. Therefore, it holds that
\begin{equation}\label{CPM-3ZK:MnR:to:real:ind-eq}
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \ddot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].
\end{equation}



\begin{GameBox}[label={CPM-3ZK:MnR:game:real}]{Game \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier})$}}
For each $i\in[K]$, uniformly pick $j_i\in [q]$ conditioned on that there exists at most one $i\in [K]$ such that $j_i=j^*$ for all $j^*\in [q]$. We re-label the indices $i$ for $\Set{(j_i)}_{i \in [K]}$  so that $j_1 < j_2 < \ldots < j_K$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner: For each $i \in [K]$, 

\para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with $\tilde{V}$ and $\tilde{V}^\dagger$ accordingly, where $\tilde{\Verifier}$ uses $H^{(i-1)}_0$ as the oracle. (see below for the definitions of $H^{(i-1)}_0$ for $i\ge 2$.)


\para{For Query $\msf{sq}(i)$:} Note that by definition (and \Cref{rmk:sq:type}), the $\msf{sq}(i)$ query is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.   Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and applies $\tilde{V}$ using $H^{(i)}_0$ as the oracle.


\para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Real}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_K, \rho_{\msf{out}})$.

\end{GameBox}



\subsection{Defining the Dummy Game} 

\para{A Dummy Version of $\tilde{\Verifier}$.} We first define a unitary $\ddot{V}$, which should be treated as the ``dummy version'' of $\tilde{\Verifier}$'s unitary $\tilde{V}$. We present it in \Cref{CPM-3ZK:V-dummy}, highlighting its difference with $\tilde{V}$ (defined in \Cref{CPM-3ZK:V:unitary}) in \red{red color}.
\begin{AlgorithmBox}[label={CPM-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}
{\bf Helper Unitaries.} We first define additional helper unitaries. For each $i \in [2]$:
\begin{itemize}
 \item
{\bf $\ddot{C}_i$: swap $\reg{m}$ and $\reg{t_i}$.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, \red{then do nothing}. 
\item
If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{t_i}$ and $\reg{m}$.
\end{itemize}
 \end{itemize} 

\para{Unitary $\ddot{V}$.} On each query, it compares the global counter value $i$ with the local counter value $j$ and behaves accordingly. In particular:
\begin{description}
\item[Case $(i = j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $D_i\red{\ddot{C}_i}A_i$, where $A_i$ and $D_i$ is  defined in \Cref{CPM-3ZK:V:unitary} and $\ddot{C}_i$ is defined above.
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}

\item[Case $(i \ne j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $C'_iA_i$, where $A_i$ and $C_i$ is  defined in \Cref{CPM-3ZK:V:unitary}
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}
\end{description}
\end{AlgorithmBox}




% \begin{AlgorithmBox}[label={CPM-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}


% \para{Compare Counters.} On each query, check if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% \begin{itemize}
% \item
% If $i \ne j$, then apply $U_{gc}$ to increase the global counter, and do nothing else.
% \item
% If $i = j$, then first apply $U_{gc}$ to increase the global counter, and then behave differently according to the value of the global counter $i$. We describe it in the following.
% \end{itemize}

% \para{Global Counter $i = 1$.} Apply $\ddot{V}_1 \coloneqq D_1 \red{\ddot{C}_1} A_1$, where $D_1$ and $A_1$ are the same as for $\tilde{V}$ and $\ddot{C}_1$ is defined as follows:
% \begin{itemize}
% \item
% {\bf ($\ddot{C}_1$: Swap $\reg{m}$ and $\reg{t_1}$.)} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% \item
% If $H(p_1) = 1$, \red{then do nothing}. 
% \end{itemize}

% \end{itemize}


% \para{Global Counter $i = 2$.} Apply $\ddot{V}_2 \coloneqq D_2 \red{\ddot{C}_2} A_2$,
% where $D_2$ and $A_2$ are the same as for $\tilde{V}$ and $\ddot{C}_2$ is defined as follows:
% \begin{itemize}

% \item 
% {\bf ($\ddot{C}_2$: Swap $\reg{m}$ and $\reg{t_2}$.)} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% \item
% If $H(p_1, p_2) = 1$, \red{then do nothing}. 
% \end{itemize}

% \end{itemize}

% \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.

% \end{AlgorithmBox}


\para{A Dummy MnR Game.} We now define another game $\msf{Dummy}(\Sim, \tilde{\Verifier})$. This game will essentially serve as a malicious prover $\tilde{\Prover}$ that could break the soundness of the original ZK protocol, leading to our desired contradiction. Intuitively, $\msf{Dummy}(\Sim, \tilde{\Verifier})$ behaves identical to $\msf{Real}(\Sim, \tilde{\Verifier})$ except for that it answers $\Sim$'s queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$ using the dummy version of $\tilde{\Verifier}$ as we defined in \Cref{CPM-3ZK:V-dummy}. We present the game in \Cref{CPM-3ZK:MnR:game:dummy} and highlight its difference $\msf{Real}(\Sim, \tilde{\Verifier})$ (in \Cref{CPM-3ZK:MnR:game:real}) in \red{red color}. 
\begin{GameBox}[label={CPM-3ZK:MnR:game:dummy}]{Game \textnormal{$\msf{Dummy}(\Sim, \tilde{\Verifier})$}}
For each $i\in[K]$, uniformly pick $j_i\in [q]$ conditioned on that there exists at most one $i\in [K]$ such that $j_i=j^*$ for all $j^*\in [q]$. We re-label the indices $i$ for $\Set{(j_i)}_{i \in [K]}$  so that $j_1 < j_2 < \ldots < j_K$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner: For each $i \in [K]$, 

\para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with \red{$\ddot{V}$} and \red{$\ddot{V}^\dagger$} accordingly, using $H^{(i-1)}_0$ as the oracle. (Note that \red{$\ddot{V}$} is defined in \Cref{CPM-3ZK:V-dummy}.)


\para{For Query $\msf{sq}(i)$:} Answered in the same manner as in \Cref{CPM-3ZK:MnR:game:real}.


\para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Dummy}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_K, \rho_{\msf{out}})$.

\end{GameBox}
The following is the most involved lemma. We defer its proof to \xiao{Cref}, before which we first show (in \xiao{Cref}) how to finish the current proof of \Cref{CPM-3ZK:decider:lem:soundness} assuming that \Cref{CPM-3ZK:MnR:game:dummy:lem} holds.


\begin{lemma}\label{CPM-3ZK:MnR:game:dummy:lem}
For the $\msf{Dummy}(\Sim, \tilde{\Verifier})$ defined in \Cref{CPM-3ZK:MnR:game:dummy} and the $\msf{Real}(\Sim, \tilde{\Verifier})$ defined in \Cref{CPM-3ZK:MnR:game:real}, it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].$$
\end{lemma}






\subsection{Finishing the Proof of \Cref{CPM-3ZK:decider:lem:soundness}}
In this part, we finish the proof of \Cref{CPM-3ZK:decider:lem:soundness} assuming that \Cref{CPM-3ZK:MnR:game:dummy:lem} holds. 

\xiao{Add some intitive explanation. }



\begin{AlgorithmBox}[label={malicious-Prover}]{Malicious Prover $\tilde{\Prover}(x)$}
On input $x$, $\tilde{\Prover}(x)$ internally emulates \Cref{CPM-3ZK:MnR:game:dummy} with the help of an external honest verifier $\Verifier$ in the following manner.

\para{Registers:} Note that to emulate \Cref{CPM-3ZK:MnR:game:dummy}, $\tilde{\Prover}$ needs to prepare registers as in \Cref{2-LOCC:V:inital:expr}. To do that, $\tilde{\Prover}$ prepares the following registers
\begin{equation}\label[Expression]{malicious-P:inital:expr}
\ket{x}_{\reg{ins}} 
\ket{0}_{\reg{gc}}
\ket{0}_{\reg{lc}} 
\ket{\vb{0}}_{\reg{p_1}}
\ldots
\ket{\vb{0}}_{\reg{p_K}}
\ket{\vb{0}}_{\reg{m}} 
\ket{\bot}_{\reg{t_1}}
\ldots
\ket{\bot}_{\reg{t_K}}  
\ket{H_0}_{\reg{aux}} 
\end{equation}
Comparing \Cref{malicious-P:inital:expr} with \Cref{2-LOCC:V:inital:expr}, one can see that registers $\reg{v_1\ldots v_K}$ and $\reg{w}$ are missing. As we will explain shortly, these registers can be think of being held by the external honest verifier $\Verifier$.

\para{Execution:} $\tilde{\Prover}$ emulates \Cref{CPM-3ZK:MnR:game:dummy} in the following manner. For each $i \in [K]$,
\begin{itemize}
\item
{\bf For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} $\tilde{\Prover}$ answers such queries with in exactly the same manner as \Cref{CPM-3ZK:MnR:game:dummy}. We emphasize that such queries will be answered using the $\ddot{V}$ or $\ddot{V}^\dagger$. Note that $\ddot{V}$ by definition (see \Cref{CPM-3ZK:V-dummy}) will only make use of the registers shown in \Cref{malicious-P:inital:expr}. Therefore, $\tilde{\Prover}$ could emulate them internally, without touching upon the external honest $\Verifier$'s registers.

\item
{\bf For Query $\msf{sq}(i)$:} $\tilde{\Prover}$ first behaves in the same manner as \Cref{CPM-3ZK:MnR:game:dummy} until she obtains the measurement outcome $\vb{p}_i = (p_{1}, \ldots, p_i)$. Also, same as \Cref{CPM-3ZK:MnR:game:dummy}, if the value  $\vb{p}_{i-1}$ obtained earlier is not a prefix of the current $\vb{p}_i$, $\tilde{\Prover}$ aborts the execution directly.

If the execution has not been aborted so far, the next step in \Cref{CPM-3ZK:MnR:game:dummy} is to apply the unitary $\tilde{V}$. We emphasize that this is the (only) step that $\tilde{\Prover}$ cannot finish by herself internally, because the $\tilde{V}$ operator defined in \Cref{CPM-3ZK:V:unitary} (in particular, the operator $B_i$) needs to work on the external honest $\Verifier$'s registers $\reg{v_i}$ and $\reg{w}$. To do that, $\tilde{\Prover}$ simply puts $p_i$ in to the $\reg{m}$ register and sends it to the external $\Verifier$ (note that $p_i$ is a classical message). Then, by definition, the honest $\Verifier$ will compute the (possibly quantum) response $v_2$, put it in the $\reg{m}$ register, and send $\reg{m}$ back to $\tilde{\Prover}$. Using this returned $\reg{m}$ register, $\tilde{\Prover}$ can easily finish the remaining steps in exactly the same manner as \Cref{CPM-3ZK:MnR:game:dummy}.
\end{itemize}

\para{Output:} We do not define any output for $\tilde{\Prover}$. (In \Cref{CPM-3ZK:MnR:game:dummy}, the $\rho_{\msf{out}}$ part in the output is on the register $\reg{w}$. But this register is held by the external honest $\Verifier$ in the current game.)
\end{AlgorithmBox}

From the above description, it is easy to see that the view of $\Sim$ in \Cref{malicious-Prover} is identical to that in \Cref{CPM-3ZK:MnR:game:dummy}. Thus, during the execution $\langle \tilde{\Prover}, \Verifier\rangle(x)$, the overall state across the joint registers held by both the malicious $\tilde{\Prover}$ (as defined in \Cref{malicious-Prover}) and the honest $\Verifier$ evolves in exactly the same manner as in \Cref{CPM-3ZK:MnR:game:dummy}. Therefore, it follows that
\begin{equation}\label[Inequality]{eq:malicious-P:dummy}
\Pr[d = 1~:~ d \la \msf{Out}_{\Verifier}\big(\langle \tilde{\Prover}, \Verifier\rangle(x)\big)] 
\ge \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})]
,\end{equation}
where the `$>$' part in the ``$\ge$'' sign in \Cref{eq:malicious-P:dummy} is due to the following reason: Note that the predicate $\msf{Pred}$ checks if the $\reg{lc}$ register contains $K$ {\em in addition to the check that the verifier's decision bit is 1} (see \Cref{CPM-3ZK:BQP-decider}); however, the LHS in \Cref{eq:malicious-P:dummy} only checks if the  verifier's decision bit is 1.



\para{Deriving the Final Contradiction.} Now, we are ready to finish the proof of \Cref{CPM-3ZK:decider:lem:soundness}. Toward that, we assume for contradiction that \Cref{CPM-3ZK:decider:lem:soundness} does not hold. Formally, we assume that there exist a $\Lang \in \BQP$, a $x \in \bits^{\secpar} \setminus \Lang$, and a polynomial $\delta(\cdot)$ so that for infinitely many $\secpar$ it holds that  
\begin{equation}\label[Inequality]{decider:lem:soundness:proof:eq:contradiction}
\Pr[\mcal{B}(x) = 1] \ge  \frac{1}{\delta(\secpar)}.
\end{equation}

It then follows that
\begin{align}
\Pr[d = 1~:~ d \la \msf{Out}_{\Verifier}\big(\langle \tilde{\Prover}, \Verifier\rangle(x)\big)] 
& \ge 
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})]
\label[Inequality]{decider:lem:soundness:proof:eq:final:1} \\ 
& =
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})]
\label{decider:lem:soundness:proof:eq:final:2} \\ 
& =
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \ddot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]]
\label{decider:lem:soundness:proof:eq:final:3} \\ 
& \ge 
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]]
\label[Inequality]{decider:lem:soundness:proof:eq:final:4} \\ 
& \ge
\frac{1}{2^K} \cdot \Pr[\mcal{B}(x) = 1] 
\label[Inequality]{decider:lem:soundness:proof:eq:final:5} \\ 
& \ge
\frac{1}{2^K \delta(\secpar)}
\label[Inequality]{decider:lem:soundness:proof:eq:final:6} 
,\end{align}
where \Cref{decider:lem:soundness:proof:eq:final:1} follows form \Cref{eq:malicious-P:dummy}, \Cref{decider:lem:soundness:proof:eq:final:2} follows from \Cref{CPM-3ZK:MnR:game:dummy:lem}, \Cref{decider:lem:soundness:proof:eq:final:3} follows from \Cref{CPM-3ZK:MnR:to:real:ind-eq}, \Cref{decider:lem:soundness:proof:eq:final:4} follows from \Cref{MnR:game:modify:2:cor}, \Cref{decider:lem:soundness:proof:eq:final:5} follows from \Cref{CPM-3ZK:MnR:game:modify:1:lem}, and \Cref{decider:lem:soundness:proof:eq:final:6} follows from \Cref{decider:lem:soundness:proof:eq:contradiction}.

Now, recall that $K$ is a constant. Thus, $2^K \delta(\secpar)$ is a polynomial on the security parameter $\secpar$. Thus, \Cref{decider:lem:soundness:proof:eq:final:6} contradicts the soundness of the ZK protocol $\langle \Prover, \Verifier \rangle$.

\vspace{1em}
This eventually completes the proof of \Cref{CPM-3ZK:decider:lem:soundness}. 

==> sections/CPM-babycase-simplified-part-3.tex <==

\section{Warm Up: Three-Round BBZK in the CPM Model (Part 3/3)}


% \subsection{Branch-Wise Equivalence Suffices}
% We first notice that \Cref{CPM-3ZK:MnR:game:real} can be treated as a sequence of alternating unitaries and measurements. In particular, there are 3 types of measurements (and $(q+4)$ measurements are made in total):
% \begin{enumerate}
% \item
% \label[Type]{CPM-3ZK:branchwise:measure:type:1}
% {\bf Type-1:} The simulator $\Sim$ simply alternates between her local unitary $S$ and the measurement on register $\reg{u}$, which determines the type of her next query (i.e., either $\tilde{V}$ or $\tilde{V}^\dagger$). Note that there are $q$ such measurements since $\Sim$ makes $q$ queries in total.
% \item
% \label[Type]{CPM-3ZK:branchwise:measure:type:2}
% {\bf Type-2:}
% When $\Sim$ makes the $\msf{sq}(i)$-th query, it triggers a measurement on registers $\reg{p_1}, \ldots, \reg{p_i}$. Note that there are $k =2$ such measurements.

% \item
% \label[Type]{CPM-3ZK:branchwise:measure:type:3}
% {\bf Type-3:}
% The $\msf{sq}(i)$-th query is answered according to a random bit $b_i$ sampled at the beginning. This can be equivalently understood as preparing a qubit $\ket{\psi}_{\reg{b_i}} = \frac{1}{\sqrt{2}} (\ket{0} + \ket{1})$ at the beginning and measuring it to define the classical bit $b_i$ used to answer the $\msf{sq}(i)$-th query. Note that there are $k =2$ such measurements as well.
% \end{enumerate}
% Also, notice that in \Cref{CPM-3ZK:MnR:game:real}, the values $\Set{j_i}_{i \in [2]}$ are sampled at the very beginning and after that the timing of all the measurements are fixed. It then follows from \Cref{branchwise:lem} that the accepting probability $\Pr[\msf{Pred}(\rho)]$ w.r.t.\  \Cref{CPM-3ZK:MnR:game:real} can be equivalently expressed as the summation of all accepting probabilities w.r.t.\ a ``sub-normalized'' version of \Cref{CPM-3ZK:MnR:game:real} where all the $(q+4)$ measurements are replaced with projections. Formally, we defined the ``sub-normalized'' \Cref{CPM-3ZK:MnR:game:real} (and similarly for \Cref{CPM-3ZK:MnR:game:dummy}) in \Cref{CPM-3ZK:MnR:game:subnormalized}.

% \begin{FigureBox}[label={CPM-3ZK:MnR:game:subnormalized}]{Sub-Normalized Games \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$} and \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$}}
% {\bf Parameters.} Fix $J = (j_1, j_2)$ such that $j_1, j_2 \in [q]$ and $j_1 < j_2$. Also fix a classical string of $(q+4)$ symbols $\msf{pat} = (u_1, \ldots, u_q, p_1, b_{1}, p_1p_2,   b_2)$ with  $u_i \in \Set{\uparrow, \downarrow}$, $p_1 \in \Set{0, 1}^{\ell}$, $p_1p_2 \in \Set{0, 1}^{2\ell}$, and $b_1, b_2 \in\bits$. The following games are parameterized by $(J, \msf{pat})$.

% \para{Game $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} It behaves identically to \Cref{CPM-3ZK:MnR:game:real} except for the following differences: 
% \begin{enumerate}
% 	\item
% 	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

% \item
% When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
% \item
% When the measurement on $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$) is triggered (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1}$ (resp.\ $\ketbra{p_1,p_2}$) to register $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$); 
% \item
% When it needs $b_i$ (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:3} above), it applies the projector $\ketbra{b_i}$ to register $\reg{b_i}$. 
% \end{enumerate}

% \para{Game $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} This is defined in a similar way w.r.t.\ \Cref{CPM-3ZK:MnR:game:dummy}. Namely, It behaves identically to \Cref{CPM-3ZK:MnR:game:dummy} except for the following differences: 
% \begin{enumerate}
% 	\item
% 	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

% \item
% When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
% \item
% When the measurement on $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$) is triggered (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1}$ (resp.\ $\ketbra{p_1,p_2}$) to register $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$); 
% \item
% When it needs $b_i$ (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:3} above), it applies the projector $\ketbra{b_i}$ to register $\reg{b_i}$. 
% \end{enumerate}
% \end{FigureBox}

% It then follows from \Cref{branchwise:lem} that
% \begin{align*}
% \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})] 
% & = 
% \frac{2!}{\binom{q}{2}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] \\
% \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] 
% & = 
% \frac{2!}{\binom{q}{2}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})],
% \end{align*}
% where the summations are taken over all possible $J$ and $\msf{pat}$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}. 

% Therefore, to prove \Cref{CPM-3ZK:MnR:game:dummy:lem}, it suffices to prove the following \Cref{CPM-3ZK:branch-wise:suffices}.
% \begin{lemma}[Branch-Wise Equivalence Suffices]\label{CPM-3ZK:branch-wise:suffices}
% For all $(J, \msf{pat})$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}, it holds that 
% $$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})].$$
% \end{lemma}


\subsection{Proving \Cref{CPM-3ZK:branch-wise:suffices}}
In this proof, we consider an (arbitrarily) fixed $J$ and $\msf{pat}$ that satisfy the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}.

\para{Simplification Assumptions.} We first make three assumptions regarding the behavior of $\Sim$. As we will show, these assumptions will not affect the accepting probability of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ and $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$, but it will simplify the notation and ease the presentation of the current proof.
\begin{itemize}
\item 
\hypertarget{CPM-3ZK:simp-assumption:1}{{\bf Assumption 1:}} When the global counter is $\ket{0}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}^\dagger$ (resp.\ $\ddot{V}^\dagger$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$).

\item 
\hypertarget{CPM-3ZK:simp-assumption:2}{{\bf Assumption 2:}} When the global counter is $\ket{2}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ (resp.\ $\ddot{V}$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$).

\item 
\hypertarget{CPM-3ZK:simp-assumption:3}{{\bf Assumption 3:}} For each $i \in [2]$, before the $\msf{sq}(i)$-th query is made, when the global counter is $\ket{i-1}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ (resp.\ $\ddot{V}$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$) 
\end{itemize}
\xiao{We argue that we can indeed make these assumptions when proving \Cref{CPM-3ZK:branch-wise:suffices}. to do... 
} \xiao{A caveat is:} to make \hyperlink{CPM-3ZK:simp-assumption:3}{Assumption 3}, we need to additionally assume that before the $\msf{sq}(i)$-th query is made, $\Sim$'s local operator may modify register $\reg{t_i}$. But we claim that this will not affect our proof of \Cref{CPM-3ZK:branch-wise:suffices}. 




Next, we define a sequence of hybrids $H_0$, $H_1$, and $H_2$. To better illustrate these hybrids, we provide pictures in \Cref{figure:CPM-3ZK:hybrids}.

\para{Hybrid $H_0$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H0}.) This is exactly the execution of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. 

\xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H0}. 
Point out the position of $\msf{sq}(1)$ and $\msf{sq}(2)$. Also exaplain how the assumptions made above are reflected in this figure.}
\xiao{Also, this is the moment to introduce the notation of $\uparrow$-query and $\downarrow$-query.}

Therefore, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$




\para{Hybrid $H_1$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H1}.) This hybrid is identical to the previous one except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (i.e., query $\msf{sq}(1)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (resp.\ from $\ket{1}_{\reg{gc}}$ to $\ket{0}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}
This is best illustrated by the \red{red-color} symbols in \Cref{figure:CPM-3ZK:hybrids:H1} \xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H1}} 

\para{Hybrid $H_2$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H2}.) This hybrid is identical to the previous one except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (i.e., query $\msf{sq}(2)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (resp.\ from $\ket{2}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}
This is best illustrated by the \red{red-color} symbols in \Cref{figure:CPM-3ZK:hybrids:H2} \xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H2}} 

It is straightforward that hybrid $H_2$ is exactly the execution of $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. Therefore, it holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_2 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$


\begin{figure}[!tb]
\centering
     \begin{subfigure}[t]{0.47\textwidth}
         \fbox{
         \includegraphics[width=\textwidth,page=1]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H0}
     \end{subfigure}
     \hspace{15pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=2]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H1}
     \end{subfigure}
     
     \centering\vspace{1em}
     \begin{subfigure}[t]{0.47\textwidth}
         
         \fbox{
         \includegraphics[width=\textwidth,page=3]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H2}
     \end{subfigure}
     \caption{Illustration of Hbyrids $H_0$, $H_1$, and $H_2$}
     \label{figure:CPM-3ZK:hybrids}
\end{figure}

With the above hybrids, to prove \Cref{CPM-3ZK:branch-wise:suffices}, it now suffices to establish the following \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. 
\begin{lemma}\label{lem:CPM-3ZK:H01}
It holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_1 \big].$$
\end{lemma}

\begin{lemma}\label{lem:CPM-3ZK:H12}
It holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_1 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_2 \big].$$
\end{lemma}

\para{Preparation for the proofs of \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}.} In the sequel (\xiao{crefxxx}), we prove \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. Before we start, we first do some preparation work and set up some notations that will ease our presentation later.

First, recall from \Cref{CPM-3ZK:MnR:game:real} that after the $\msf{sq}(i)$-th query is made, the malicious verifier $\tilde{\Verifier}$ will use $H^{\vb{p}_i, \vb{1}}_0$ as its oracle. Also, note that the above hybrids are defined w.r.t.\ a fixed $(J,\msf{pat})$. Therefore, we could re-write some of $\tilde{\Verifier}$'s unitaries in \Cref{CPM-3ZK:V:unitary}, whose behavior depend on the value $H(p_1, \ldots, p_i)$, into a format that uses the $p_i$'s contained in (the a prior fixed) $\msf{pat}$ as a controlled unitary. 

In particular, for the $(p_1, p_2)$ contained in the fixed $\msf{pat}$, we keep the $U_{gc}$, $U_{lc}$, $A_i$ and $D_i$ the same as in \Cref{CPM-3ZK:V:unitary}, but we re-write the unitaries $B_i$, $C_i$, and $\ddot{C}_i$ ($\forall i \in [2]$) in the following format:
\begin{enumerate}
\item \label{CPM-3ZK:renaming:B1}
Let $B_1 = \ketbra{p_1}_{\reg{p_1}} \tensor B_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor I$. Note that $B_{1,1}$ is exactly the $V_{p_1}$ in \Cref{CPM-3ZK:V:unitary}, and it acts non-trivially only on $\reg{v_1}$ and $\reg{w}$, and works as identity on other registers. 

\item \label{CPM-3ZK:renaming:C1}
Let $C_1 = \ketbra{p_1}_{\reg{p_1}} \tensor C_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor C_{1,0}$. Note that $C_{1,1}$ is the swap operator between $\reg{v_1}$ and $\reg{m}$, and $C_{1,0}$ is the swap operator between $\reg{t_1}$ and $\reg{m}$.

\item \label{CPM-3ZK:renaming:ddotC1}
Let $\ddot{C}_1 = \ketbra{p_1}_{\reg{p_1}} \tensor I + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor C_{1,0}$. (Recall the definition of $\ddot{C}_1$ from \Cref{CPM-3ZK:V-dummy}.)

\item \label{CPM-3ZK:renaming:D1}
Let $D_1 = \ketbra{p_1}_{\reg{p_1}} \tensor D_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor I$. Note that $D_{1,1}$ is exactly the local-counter increasing unitary $U_{lc}$, which acts non-trivially only on $\reg{lc}$. 

\item \label{CPM-3ZK:renaming:B2}
Let $B_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor B_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor I$. Note that $B_{2,1}$ is exactly the $V_{p_2}$ in \Cref{CPM-3ZK:V:unitary}, which acts non-trivially only on $\reg{v_2}$ and $\reg{w}$, and works as identity on other registers.

\item \label{CPM-3ZK:renaming:C2}
Let $C_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0}$. Note that $C_{2,1}$ is the swap operator between $\reg{m}$ and $\reg{v_2}$, and $C_{2,0}$ is the swap operator between $\reg{t_2}$ and $\reg{m}$.

\item \label{CPM-3ZK:renaming:ddotC2}
Let $\ddot{C}_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor I + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0}$. (Recall the definition of $\ddot{C}_2$ from \Cref{CPM-3ZK:V-dummy}.)

\item \label{CPM-3ZK:renaming:D2}
Let $D_2= \ketbra{p_1, p_2}_{\reg{p_1p_2}} \tensor D_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}} \ketbra{p'_1,p'_2}_{\reg{p_1p_2}} \tensor I$. Note that $D_{2,1}$ is exactly the local-counter increasing unitary $U_{lc}$ (i.e., same as $D_{1,1}$), which acts non-trivially only on $\reg{lc}$. 
\end{enumerate}
It will be helpful to keep track of the registers on which the unitaries acts on {\em non-trivially}. For the reader's convenience, we summarize it in \Cref{CPM-3ZK:non-trivial-registers:table}. For a unitary shown in the table, it acts as the identity on registers not shown in its row.


\begin{table}[!htb]
\centering
\caption{Registers on which the unitaries acts non-trivially}
\label{CPM-3ZK:non-trivial-registers:table}
\vspace{0.5em}
\begin{tabular}{C{50pt} C{70pt} c C{50pt} C{70pt}}
\toprule
Unitary operators & Non-trivial registers & \phantom{abcde}  & Unitary operators & Non-trivial registers \\ 
\cmidrule{1-2} \cmidrule{4-5}
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$A_1$    	& $\reg{p_1}, \reg{m}$ & & 
$A_2$ 		& $\reg{p_2}, \reg{m}$ \\ 
\addlinespace[0.3em]
$B_1$ 		& $\reg{p_1}$, $\reg{v_1}$, $\reg{w}$   & & 
$B_2$ 		& $\reg{p_1}$, $\reg{p_2}$, $\reg{v_2}$, $\reg{w}$ \\
\addlinespace[0.3em]
$B_{1,1}$ 	& $\reg{v_1}$, $\reg{w}$  & & 
$B_{2,1}$ 	& $\reg{v_2}$, $\reg{w}$ \\ 
\addlinespace[0.3em]
$C_1$    	&  $\reg{p_1}$, $\reg{v_1}$, $\reg{t_1}$, $\reg{m}$ & & 
$C_2$    	&  $\reg{p_1}$, $\reg{p_2}$, $\reg{v_2}$, $\reg{t_2}$, $\reg{m}$  \\ 
\addlinespace[0.3em]
$C_{1,1}$   & $\reg{v_1}$, $\reg{m}$  & & 
$C_{2,1}$   & $\reg{v_2}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$C_{1,0}$  	& $\reg{t_1}$, $\reg{m}$ & & 
$C_{2,0}$  	& $\reg{t_2}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$\ddot{C}_1$    	&  $\reg{p_1}$,  $\reg{t_1}$, $\reg{m}$ & & 
$\ddot{C}_2$    	&  $\reg{p_1}$, $\reg{p_2}$,  $\reg{t_2}$, $\reg{m}$  \\ 
\addlinespace[0.3em]
$D_1$		& $\reg{p_1}$, $\reg{lc}$  & & 
$D_2$		& $\reg{p_1}$, $\reg{p_2}$, $\reg{lc}$ \\ 
\addlinespace[0.3em]
$D_{1,1}$		& $\reg{lc}$  & & 
$D_{2,1}$		& $\reg{lc}$ \\ 
\addlinespace[0.3em]
$U_{gc}$ & $\reg{gc}$ & &   $S$ 		& $\reg{m}$, $\reg{u}$, $\reg{s}$  \\   
\bottomrule
\end{tabular}
\end{table}


\xiao{The following proof does not take care of the value $b_1$ and $b_2$. Need to add some argument to say that we can assume  w.l.o.g.\ that $b_1 = b_2 =1$.}



\subsection{Structure of the Counters} 
\label{CPM-3ZK:counter-structure:section}
We need to show that the counters are in a particular structure. by the following lemma
% \begin{lemma}[Counter Structure.]\label{CPM-3ZK:counter-structure:lemma}
% Under the above assumptions 1 2 and 3. At layer $k \in \Set{0,1,2}$, the overall state is of the format:
% % \begin{align*}
% % & \ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(k)}_{p_1, \ldots, p_k}} +  \\ 
% % & \hspace{3em}
% % \ket{k}_{\reg{gc}} \sum^{k}_{j = 1} \ket{k-j}_{\reg{lc}} \ket{p_1, \ldots, p_{k-j}} \sum_{p'_{k-j+1}, \ldots, p'_{k}}\ket{p'_{k-j+1}, \ldots, p'_{k}} \ket{\rho^{(k)}_{p_1, \ldots, p_{k-j}, p'_{k-j+1}, \ldots, p'_{k}}}
% % \end{align*}
% % where the summation over $(p'_1, \ldots, p'_j)$ meaning to take the summation over all $(p'_1, \ldots, p'_j) \ne (p_1, \ldots, p_j)$.

% \begin{align*}
% & \ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(k)}_{p_1, \ldots, p_k}} +  \\ 
% & \hspace{3em}
% \ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j} \sum_{p'_{j+1}, \ldots, p'_{k}}\ket{p'_{j+1}, \ldots, p'_{k}} \ket{\rho^{(k)}_{p_1, \ldots, p_{j}, p'_{j+1}, \ldots, p'_{k}}}
% \end{align*}
% where the summation over $(p'_{j+1}, \ldots, p'_k)$ meaning to take the summation over all $(p'_{j+1}, \ldots, p'_k)$ conditioned on that 
% $$\wedge^{k}_{i = j+1}(p'_i \ne p_i).$$

% \xiao{they above two terms can be merged into 1 if let $j$ starts from $0$. I may do that later if it does not hurt readability.}	

% For readability, I expand the above succinct expression:
% \begin{align*}
% & 
% \ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(k)}_{p_1, \ldots, p_k}} ~+  \\ 
% &
% \ket{k}_{\reg{gc}} \ket{k-1}_{\reg{lc}} \ket{p_1, \ldots, p_{k-1}}_{\reg{p_1, \ldots, p_{k-1}}} \sum_{p'_k} \ket{p'_k} \ket{\rho^{(k)}_{p_1, \ldots, p_{k-1}, p'_k}} ~+  \\ 
% &
% \ket{k}_{\reg{gc}} \ket{k-2}_{\reg{lc}} \ket{p_1, \ldots, p_{k-2}}_{\reg{p_1, \ldots, p_{k-2}}} \sum_{p'_{k-1}, p'_k} \ket{p'_{k-1}, p'_k} \ket{\rho^{(k)}_{p_1, \ldots, p_{k-2}, p'_{k-1},  p'_k}} ~+  \\ 
% & \cdots \\ 
% &
% \ket{k}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \sum_{p'_{2}, \ldots,  p'_k} \ket{p'_2, \ldots,  p'_k} \ket{\rho^{(k)}_{p_1, p'_2, \ldots,  p'_k}} ~+  \\ 
% &
% \ket{k}_{\reg{gc}} \ket{0}_{\reg{lc}} \sum_{p'_{1}, \ldots,  p'_k} \ket{p'_1, \ldots,  p'_k} \ket{\rho^{(k)}_{p'_1,  \ldots,  p'_k}} 
% \end{align*}
% \end{lemma}


\begin{lemma}[Counter Structure.]
Under the above assumptions 1 2 and 3. For each $k \in \Set{0,1,2}$, at the global couonter's $t$-th arrival at value $k$, the overall state is of the following format:
\begin{align*}
\ket{\phi^{(t,k)}} 
& =  
\ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(t,k)}} ~+  \\
& \hspace{8em} 
\ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(t,k)}_{p'_{j+1}}}
\numberthis \label{CPM-3ZK:counter-strucutre:expression}
\end{align*}
where the summation over $p'_{j+1}, \ne, p_{j+1}$ means to take the summation over $p'_{j+1} \in \bits^\ell \setminus \Set{p_{j+1}}$.

For readability, we expand the above succinct \Cref{CPM-3ZK:counter-strucutre:expression}:
\begin{align*}
\ket{\phi^{(t,k)}}
= & 
\ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(t,k)}} ~+  \\ 
&
\ket{k}_{\reg{gc}} \ket{k-1}_{\reg{lc}} \ket{p_1, \ldots, p_{k-1}}_{\reg{p_1, \ldots, p_{k-1}}} \sum_{p'_k \ne p_k} \ket{p'_k}_{\reg{p_k}} \ket{\rho^{(t,k)}_{ p'_k}} ~+  \\ 
&
\ket{k}_{\reg{gc}} \ket{k-2}_{\reg{lc}} \ket{p_1, \ldots, p_{k-2}}_{\reg{p_1, \ldots, p_{k-2}}} \sum_{p'_{k-1} \ne p_{k-1}} \ket{p'_{k-1}}_{\reg{p_{k-1}}} \ket{\rho^{(t,k)}_{p'_{k-1}}} ~+  \\ 
& \cdots \\ 
&
\ket{k}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \sum_{p'_{2} \ne p_2} \ket{p'_2}_{\reg{p_2}} \ket{\rho^{(t,k)}_{p'_2}} ~+  \\ 
&
\ket{k}_{\reg{gc}} \ket{0}_{\reg{lc}} \sum_{p'_{1}} \ket{p'_1}_{\reg{p_1}} \ket{\rho^{(t,k)}_{p'_1 \ne p_1}} 
\end{align*}
\end{lemma}
\begin{proof}[Proof of \Cref{CPM-3ZK:counter-structure:lemma}]
We prove this lemma via mathematical induction over the queries of the simulator. That is, we first prove that the initial state at the very beginning of the MnR game is of the format shown in \Cref{CPM-3ZK:counter-strucutre:expression} (i.e., the base case), and then show that each query made by the simulator will lead to a new state of the same format shown in \Cref{CPM-3ZK:counter-strucutre:expression} as well (i.e., the induction step).

\para{Base Case.} This corresponds to the state at the very beginning of the MnR game. By definition, the initial sate is of the format $\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}$. It satisfies the format shown in \Cref{CPM-3ZK:counter-strucutre:expression} (by setting $\ket{\rho^{(0,0)}} \coloneqq \ket{\rho}$).

\para{Induction Step.} We assume that the lemma is true for the global counter's $t$-th arrival at value $k$. We prove that the simulator's next query, no matter what this query is, will lead to a new state that satisfies the format shown in \Cref{CPM-3ZK:counter-strucutre:expression} as well.

\xiao{The main bulk of the proof is shown below. Still need to polish the language and add crefs. To do...}

\subpara{Case $\tilde{V}$:} Assume this is the global counter's $z$-th arrival at value $k+1$
\begin{align*}
\tilde{V}S \ket{\phi^{t,k}}
& = 
\tilde{V}S 
\bigg(
\ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(t,k)}} ~+  \\
& \hspace{8em} 
\ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(t,k)}_{p'_{j+1}}}
\bigg) \\ 
& =
\tilde{V}
\bigg(\ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} S\ket{\rho^{(t,k)}} ~+  \\
& \hspace{8em} 
\ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} S \ket{\rho^{(t,k)}_{p'_{j+1}}}
\bigg) \\ 
& =
D_{k+1}C_{k+1}B_{k+1}A_{k+1}\ket{k+1}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} \sum_{p'_{k+1} \ne p_{k+1}}\ket{p'_{k+1}}_{\reg{p_{k+1}}} S \ket{\rho^{(t,k)}_{p'_{k+1}}}
+ \\ 
& \hspace{10em}
C_{k+1}A_{k+1}\ket{k+1}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} S \ket{\rho^{(t,k)}_{p'_{j+1}}} \\ 
& =
\ket{k+1}_{\reg{gc}} D_{k+1} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} \sum_{p'_{k+1} \ne p_{k+1}} C_{k+1,1} B_{k+1,1} A_{k+1}\ket{p'_{k+1}}_{\reg{p_{k+1}}} S \ket{\rho^{(t,k)}_{p'_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k+1}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} C_{k+1,0} A_{k+1}S \ket{\rho^{(t,k)}_{p'_{j+1}}} \\ 
& =
\ket{k+1}_{\reg{gc}} D_{k+1} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} \sum_{p'_{k+1} \in \bits^\ell} \ket{p'_{k+1}}_{\reg{p_{k+1}}} \ket{\dot{\rho}_{p'_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k+1}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\dot{\rho}_{p'_{j+1}}} \\ 
& =
\ket{k+1}_{\reg{gc}} \ket{k+1}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}   \ket{p_{k+1}}_{\reg{p_{k+1}}} \ket{\dot{\rho}_{p_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k+1}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} \sum_{p'_{k+1} \ne p_{k+1}} \ket{p'_{k+1}}_{\reg{p_{k+1}}} \ket{\dot{\rho}_{p'_{k+1}}}
+ \\
& \hspace{10em}
\ket{k+1}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\dot{\rho}_{p'_{j+1}}} \\ 
& =
\ket{k+1}_{\reg{gc}} \ket{k+1}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}   \ket{p_{k+1}}_{\reg{p_{k+1}}} \ket{\dot{\rho}_{p_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k+1}_{\reg{gc}} \sum^{k}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\dot{\rho}_{p'_{j+1}}} \\ 
& =
\ket{k+1}_{\reg{gc}} \ket{k+1}_{\reg{lc}} \ket{p_1, \ldots, p_{k+1}}_{\reg{p_1, \ldots, p_{k+1}}} \ket{\rho^{(z,k+1)}_{p_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k+1}_{\reg{gc}} \sum^{k}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(z,k+1)}_{p'_{j+1}}}
\end{align*}

\subpara{Case $\tilde{V}^\dagger$:} Assume this is the global counter's $z$-th arrival at value $k-1$.
\begin{align*}
\tilde{V}^\dagger S \ket{\phi^{t,k}}
& = 
\tilde{V}^\dagger S 
\bigg(
\ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}}\ket{\rho^{(t,k)}} ~+  \\
& \hspace{8em} 
\ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(t,k)}_{p'_{j+1}}}
\bigg) \\ 
& =
\tilde{V}^\dagger
\bigg(
\ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} S\ket{\rho^{(t,k)}} ~+  \\
& \hspace{8em} 
\ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}}  S\ket{\rho^{(t,k)}_{p'_{j+1}}}
\bigg) \\ 
& =
U^\dagger_{gc} A^\dagger_{k} B^\dagger_{k} C^\dagger_{k} D^\dagger_{k} \ket{k}_{\reg{gc}} \ket{k}_{\reg{lc}} \ket{p_1, \ldots, p_k}_{\reg{p_1, \ldots, p_k}} \sum_{p'_{k+1} \ne p_{k+1}}\ket{p'_{k+1}}_{\reg{p_{k+1}}} S \ket{\rho^{(t,k)}_{p'_{k+1}}}
+ \\ 
& \hspace{10em}
U^\dagger_{gc} A^\dagger_{k}  C^\dagger_{k} \ket{k}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} S \ket{\rho^{(t,k)}_{p'_{j+1}}} \\ 
& =
\ket{k-1}_{\reg{gc}} \ket{k-1}_{\reg{lc}} \ket{p_1, \ldots, p_{k-1}}_{\reg{p_1, \ldots, p_{k-1}}} A^\dagger_{k}  \ket{p_k}_{\reg{p_k}} B^\dagger_{k,1} C^\dagger_{k,1}\sum_{p'_{k+1} \ne p_{k+1}}\ket{p'_{k+1}}_{\reg{p_{k+1}}} S \ket{\rho^{(t,k)}_{p'_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k-1}_{\reg{gc}} \sum^{k-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}} A^\dagger_{k} \ket{p'_{j+1}}_{\reg{p_{j+1}}} C^\dagger_{k,0}  S \ket{\rho^{(t,k)}_{p'_{j+1}}} \\ 
& =
\ket{k-1}_{\reg{gc}} \ket{k-1}_{\reg{lc}} \ket{p_1, \ldots, p_{k-1}}_{\reg{p_1, \ldots, p_{k-1}}} A^\dagger_{k}  \ket{p_k}_{\reg{p_k}} B^\dagger_{k,1} C^\dagger_{k,1}\sum_{p'_{k+1} \ne p_{k+1}}\ket{p'_{k+1}}_{\reg{p_{k+1}}} S \ket{\rho^{(t,k)}_{p'_{k+1}}}
+ \\ 
& \hspace{10em}
\ket{k-1}_{\reg{gc}}  \ket{k-1}_{\reg{lc}} \ket{p_1, \ldots, p_{k-1}}_{\reg{p_1, \ldots, p_{k-1}}} \sum_{p'_{k} \ne p_{k}} A^\dagger_{k} \ket{p'_{k}}_{\reg{p_{k}}} C^\dagger_{k,0}  S \ket{\rho^{(t,k)}_{p'_{k}}} 
+ \\
& \hspace{10em}
\ket{k-1}_{\reg{gc}} \sum^{k-2}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}  \ket{p'_{j+1}}_{\reg{p_{j+1}}} A^\dagger_{k} C^\dagger_{k,0}  S \ket{\rho^{(t,k)}_{p'_{j+1}}} \\ 
& =
\ket{k-1}_{\reg{gc}} \ket{k-1}_{\reg{lc}} \ket{p_1, \ldots, p_{k-1}}_{\reg{p_1, \ldots, p_{k-1}}} \ket{\rho^{(z,k-1)}}
+ \\ 
& \hspace{10em}
\ket{k-1}_{\reg{gc}} \sum^{k-2}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}  \ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(z,k-1)}_{p'_{j+1}}} 
\end{align*}

\xiao{Also need to consider the cases of the $\msf{sq}(i)$ query. But that is almost identical to the above. Say that we omit the details.} 

\UpdateLine 

This finishes the proof of \Cref{CPM-3ZK:counter-structure:lemma}.

\end{proof}

The effect of \Cref{CPM-3ZK:counter-structure:lemma} is to allow us to talk about the hybrids in the following manner (without track the counters anymore), and at the end check the predicate on the branch $\ket{p_1, \ldots, p_K}$ only.
\begin{itemize}
\item
When $\tilde{V}$ (\xiao{$\tilde{V}^\dagger$ is simply the inverse of the following}) is made between Layer-$(k-1)$ and Layer-$k$, simply apply $D_kC_kB_kA_kU_{gc}$ \xiao{Also, the $\msf{sq}(i)$ query needs to insert a projection $\ketbra{p_1, \ldots, p_i}$ here. Will do it later.}:


\item
When $\ddot{V}$ (\xiao{$\ddot{V}^\dagger$ is simply the inverse of the following}) is made between Layer-$(k-1)$ and Layer-$k$, simply apply $D_k\ddot{C}_kA_kU_{gc}$
\end{itemize}



\subsection{Proving \Cref{lem:CPM-3ZK:H01}}
\label{sec:lem:CPM-3ZK:H01:proof}

We first present the following \xiao{lemma}.
\xiao{add some intuitive explanation.}

\begin{lemma}[Invariance in $H_0$ and $H_1$]\label{lem:CPM-3ZK-hyb01:proof:invariant}
Assume that during the execution of $H_0$ (and $H_1$), the global counter reaches value $1$ for $T$ times in total. For each $t \in [T]$, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds: in hybrid $H_0$ (resp.\ $H_1$), when the global counter reaches value $1$ for the $t$-th time, the overall state can be written as $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows
\begin{align}
\ket{\phi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}}, \label{lem:CPM-3ZK-hyb01:proof:target-format:H0}\\ 
\ket{\psi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{C_{1,0}} \ket{\rho^{(t)}_{p'_1}}. \label{lem:CPM-3ZK-hyb01:proof:target-format:H1}
\end{align}
where the unitaries $B_{1,1}$, $C_{1,0}$, and $C_{1,1}$  are as defined in \Cref{CPM-3ZK:renaming:B1,CPM-3ZK:renaming:C1}.
\end{lemma}


\para{Finishing the proof of \Cref{lem:CPM-3ZK:H01}}. Let us consider the last time when the global counter reaches value $1$. By \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, the overall states in $H_0$ and $H_1$ would be of the format respectively
\begin{align}
\ket{\phi^{(T)}} 
& = 
\overbrace{
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}} ,\\ 
\ket{\psi^{(T)}}
& = 
\overbrace{
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}}. 
\end{align}
Since this is the last time the global counter reaches value $1$, the two hybrids $H_0$ and $H_1$ by definition behave identically after that. That is, the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ will go through the same quantum procedure (let us denote it by $\mcal{F}$) and finally measured by the predicate $\msf{Pred}$.	

Next, note that the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the identical ``branch'' corresponding to $\ket{p_1}_{\reg{p_1}}$ (labeled as $\msf{Good}$ in the above equations). Also, the $\msf{Bad}$ branch will not contribute any shares to the accepting probability of the predicate $\msf{Pred}$---this is because the quantum procedure $\mcal{F}$ will not change the fact that $p'_1 \ne p_1$ for the $\msf{Bad}$ branch, and recall that $\msf{Pred}$ will output $0$ if a branch in the superposition does not have any non-zero amplitude for $\ket{p_1}$.	

In summary, only the $\msf{Good}$ branch matters for the remaining execution (after the last time when the global counter reaches value 1), contributing to the event $\msf{Pred}(\rho) = 1$. Therefore, \Cref{lem:CPM-3ZK:H01} holds because $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the same $\msf{Good}$ branch.

\para{Proving \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.} Now, the only thing left is to prove \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. We establish this lemma by a mathematical induction on the number $t \in [T]$ indicating it is which time the global counter reaches value $1$. We will keep track of how the overall states evolve in both $H_0$ and $H_1$ simultaneously.

\subsubsection{Base Case ($t = 1$)}
\label{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:base:sec} 

This corresponds to the very first time the global counter reaches $1$. By definition, this is due to $\Sim$'s query $\msf{sq}(1)$. 

We first derive how the overall state evolves in $H_0$. Formally, $\Sim$'s local operation $S$ is applied to the initial state, preparing a superposition in register $\reg{m}$. Then, the first $\tilde{V}$-query (i.e., the query $\msf{sq}(1)$) is made. Note that at this moment, both the global and local values are of the value $0$. Thus, according to \xiao{our discussion in \Cref{CPM-3ZK:counter-structure:section}}, the operator $D_1C_1B_1\ketbra{p_1}_{\reg{p_1}}A_1U_{gc}$. 

In summary, if we assume that the initial state across all the registers are $\ket{\rho}$, then the state $\ket{\phi^{(1)}}$ will be as follows:
% \begin{enumerate}
% \item
% $U_{gc}$ increases the global counter from $0$ to $1$. Note that currently, the global counter and local counter are of the form $\ket{1}_{\reg{gc}}\ket{0}_{\reg{gc}}$. 

% \item
% The unitary $A_1$ is applied

% \item
% The $\reg{p_1}$ register is projected to $\ketbra{p_1}_{\reg{p_1}}$.
% \item
% The unitary $D_1C_1B_1$ is then applied.
% \end{enumerate}
% In summary, the state $\ket{\phi^{(1)}}$ is obtained by applying the operator $D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}S$ is applied to the initial state. If we assume the initial state across all the registers are $\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}$, then it holds that:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}S  
\ket{\rho}
\\
& =
D_1C_1B_1  
 \ket{p_1}_{\reg{p_1}} \ket{\rho_{p_1}} 
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:4} \\ 
& =  
 \ket{p_1}_{\reg{p_1}}  D_{1,1}  C_{1,1}B_{1,1} \ket{\rho_{p_1}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:5} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} 
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:4} follows by defining $\ket{\rho_{p_1}} \coloneqq \bra{p_1}_{\reg{p_1}} A_1 U_{gc}S  
\ket{\rho}$;
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:5} follows from the definition of $B_1$  $C_1$, and $D_1$ (see \Cref{CPM-3ZK:renaming:B1,CPM-3ZK:renaming:C1,CPM-3ZK:renaming:D1});
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} follows by defining $\ket{\rho^{(1)}_{p_1}} \coloneqq D_{1,1} C_{1,1}B_{1,1} \ket{\rho_{p_1}}$.
\end{itemize}
% Obviously, $\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7}$ is a special case of \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} when $t = 1$.
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} satisfies the format shown in \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} when $t = 1$.


Also, note that the game $H_0$ and $H_1$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} that 
$$\ket{\psi^{(1)}} =  \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} .$$ Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.



\subsubsection{Induction Step ($t \ge 2$)} 
\label{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:sec} 


We assume $\ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t-1)}}$ satisfies \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, and show in the following that \Cref{lem:CPM-3ZK-hyb01:proof:invariant} holds when the global counter reaches $1$ for the $t$-th time.

We establish this claim by considering the following MECE (mutually exclusive and collectively exhaustive) cases:
\begin{enumerate}
\item \label[Case]{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}
{\bf Case 1:} The $t$-th arrival at value $1$ is due to an immediate $\uparrow \downarrow$ after the $(t-1)$-th arrival. That is, after the $(t-1)$-th arrival, $\Sim$ first makes a $\uparrow$ query, bringing the global counter to $0$, and then makes an $\downarrow$ query, bringing the global counter back to $1$. 
\item \label[Case]{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}
{\bf Case 2:} The $t$-th arrival at value $1$  is due to an immediate $\downarrow \uparrow $ after the $(t-1)$-th arrival. That is, after the $(t-1)$-th arrival, $\Sim$ first makes a $\downarrow$ query, bringing the global counter to $2$, and then makes an $\uparrow$ query, bringing the global counter back to $1$. 
\end{enumerate}


\subsubsubsection{Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}} 

We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) in \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}:
\begin{enumerate}
 \item
$\Sim$'s local unitary $S$ is applied. Note that this step is identical for both $H_0$ and $H_1$. 

\item
An $\uparrow$-query is made, bringing the global counter from 1 to 0.  \xiao{According to our notation in \Cref{CPM-3ZK:counter-structure:section}}: 
\begin{itemize}
    \item
    In $H_0$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1$; 
    \item
    In $H_1$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1$. 
\end{itemize}
\item
$\Sim$ will apply her local operation $S$ again. Note that this step is again identical for both $H_0$ and $H_1$.
\item
An $\downarrow$-query is made, bringing the global counter from 0 back to 1, which is the global counter's $t$-th arrival at value 1. \xiao{According to our notation in \Cref{CPM-3ZK:counter-structure:section}}: 
\begin{itemize}
    \item
    In $H_0$, this corresponds to applying $D_1C_1B_1A_1U_{gc}$; 
    \item
    In $H_1$, this corresponds to applying $D_1\ddot{C}_1A_1U_{gc}$. 
\end{itemize} 
\end{enumerate}
It follows from the above description that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
\begin{align}
\ket{\phi^{(t)}}
& = D_1C_1B_1A_1U_{gc} S U^{\dagger}_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1 S  \ket{\phi^{(t-1)}}, \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}\\ 
\ket{\psi^{(t)}}
& = D_1 \ddot{C}_1A_1U_{gc} S  U^{\dagger}_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1 S \ket{\psi^{(t-1)}}. \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}
\end{align}

% We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) in  \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}:
% \begin{enumerate}
%  \item
% $\Sim$'s local unitary $S$ is applied. Note that this step is identical for both $H_0$ and $H_1$. 
% \item
% An $\uparrow$-query is made, bringing the global counter from $1$ to $0$. 
% \begin{itemize}
%     \item
%     In $H_0$, this corresponds to applying $\tilde{V}^\dagger$; 
%     \item
%     In $H_1$, this corresponds to applying $\ddot{V}^\dagger$. 
% \end{itemize}
% \item
% The local operation $S$ is applied. Note that this step is identical for both $H_0$ and $H_1$ as well.
% \item
% An $\downarrow$-query is made, resulting in the global counter's $t$-th arrive to $1$.
% \begin{itemize}
%     \item
%     In $H_0$, this corresponds to applying $\tilde{V}$; 
%     \item
%     In $H_1$, this corresponds to applying $\ddot{V}$. 
% \end{itemize} 
% \end{enumerate}
% It follows from the above description that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
% \begin{align}
% \ket{\phi^{(t)}}
% & = \tilde{V} S \tilde{V}^\dagger S  \ket{\phi^{(t-1)}}, \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}\\ 
% \ket{\psi^{(t)}}
% & = \ddot{V} S \ddot{V}^\dagger S \ket{\psi^{(t-1)}}. \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}
% \end{align}

\begin{remark}[High-Level Idea for the Sequel]
Recall that our eventual goal is to prove that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ are of the format shown in \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0,lem:CPM-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}. But we first need to perform some preparation work, putting \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. Then, we show on \Cpageref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} how to use \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} to complete the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}. 
\end{remark}



\begin{MyClaim}\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}
There exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ so that the following holds
\begin{align}
\ket{\phi^{(t)}}
& =  
D_1C_1 B_1 U_{gc} S^{\reg{p_1}/\reg{m}} U^\dagger_{gc} B^\dagger_1 C^\dagger_1
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\bigg) \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(t)}}
& = 
D_1\ddot{C}_1 U_{gc} S^{\reg{p_1}/\reg{m}} U^\dagger_{gc}   \ddot{C}^\dagger_1 
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\bigg) 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} 
\end{align}
where $S^{\reg{p_1}/\reg{m}}$ is identical to $S$ except that it treats register $\reg{p_1}$ as $\reg{m}$.
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}]

First, notice that  
\begin{align*}
 A_1 U_{gc} S U^\dagger_{gc} A^\dagger_1 
 & = 
 A_1 U_{gc} S A^\dagger_1 U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:1} \\ 
 & = 
 A_1 U_{gc} A^\dagger_1 S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:2} \\
  & = 
 A_1 A^\dagger_1 U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:3} \\
 & = 
U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:1,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:3} follows from the fact that $U_{gc}$ acts non-trivially on different registers from $A_2$;

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:2} from the fact that $S$ acts as the identity operator on $\reg{p_1}$ and that $A_1$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_1}$ (see \Cref{CPM-3ZK:V:unitary}). 
\end{itemize}

% \UpdateLine
% First, notice that  
% \begin{align*}
%  A_1 U_{gc} S U^\dagger_{gc} A^\dagger_1 
%  & = 
%  A_1 S U_{gc} U^\dagger_{gc} A^\dagger_1 
%  \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:1} \\
%  & = 
%  A_1 S A^\dagger_1 \\
%  & =  
%  A_1 A^\dagger_1  S^{\reg{p_1}/\reg{m}} 
%  \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:2} \\ 
%  & = 
%  S^{\reg{p_1}/\reg{m}}
%  \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S} 
% ,\end{align*}
% where \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:1} follows from the fact that $U_{gc}$ acts non-trivially on different registers from $S$, and  \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:2}  follows from the fact that $S$ acts as the identity operator on $\reg{p_1}$ and that $A_1$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}). 

\subpara{Proving \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(t)}}$:
\begin{align*}
\ket{\phi^{(t)}}
& =
D_1C_1B_1A_1U_{gc} S U^{\dagger}_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:0} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1 D^\dagger_1  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1 D^\dagger_1 S 
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  +
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1 D^\dagger_1  
\bigg(
\ket{p_1}_{\reg{p_1}} S \ket{\rho^{(t-1)}_{p_1}}  +
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} S C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1  
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  +
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} S C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} \\
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  B^\dagger_1 C^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  + \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} S^{\reg{t_1}/\reg{m}} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  B^\dagger_1 C^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  + \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  B^\dagger_1 C^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0};

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S};

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} follows from our induction assumption;

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} from  from the fact that $S$ acts as the identity operator on $\reg{p_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} from  from the definition of $D_1$ (see \Cref{CPM-3ZK:renaming:D1});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} from the fact that $S$ acts as the identity operator on $\reg{t_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}) and $C_{1,0}$ is nothing but a swap operator between $\reg{t_1}$ and $\reg{m}$ (see \Cref{CPM-3ZK:renaming:C1}); (Note that $S^{\reg{t_1}/\reg{m}}$ is defined to be an operator that is identical to $S$ except that it treats $\reg{t_1}$ as $\reg{m}$.)

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} follows from the fact that $S^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $C_{1,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} follows by defining 
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}
\ket{\dot{\rho}^{(t-1)}_{p_1}}   \coloneqq D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}} ~~~\text{and}~~~
\ket{\dot{\rho}^{(t-1)}_{p'_1}}  \coloneqq S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}).
\end{equation}
\end{itemize}
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\subpara{Proving \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi}.} We now show the derivatino for $\ket{\psi^{(t)}}$. This is almost identical to the above proof for \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align*}
\ket{\psi^{(t)}}
& =
D_1 \ddot{C}_1 A_1U_{gc} S U^{\dagger}_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:0} \\ 
& =
D_1 \ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1 D^\dagger_1  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} \\ 
& =
D_1 \ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1 D^\dagger_1  S  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2} \\ 
& =
D_1\ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  ~+~ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0}  S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:6} \\ 
& =
D_1\ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1};

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S};


\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2}  follows from our induction assumption;


\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:6} follows from a similar argument as we did to derive \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2};


\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} follows from {\em the same definitions} of $\ket{\dot{\rho}^{(t-1)}_{p_1}}$ and $\ket{\dot{\rho}^{(t-1)}_{p'_1}}$ as shown in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}.
\end{itemize}
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\vspace{1em}
This completes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\end{proof}

\vspace{1em}

\begin{MyClaim}\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}
Let $S^{\reg{p_1}/\reg{m}}$ and $\Set{\dot{\rho}^{(t-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ be as defined in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}. Let
\begin{align}
\ket{\gamma^{(t-1)}_0} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:0} \\ 
\ket{\gamma^{(t-1)}_1} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:1} \\ 
\ket{\gamma^{(t)}_0} 
& \coloneqq 
C_1 B_1 U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}    B^\dagger_1 C^\dagger_1 \ket{\gamma^{(t-1)}_0} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0} \\ 
\ket{\gamma^{(t)}_1}
& \coloneqq 
\ddot{C}_1 U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}   \ddot{C}^\dagger_1  \ket{\gamma^{(t-1)}_1}
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1} 
.\end{align}
Then, there exist (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds:
\begin{align}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} 
.\end{align}
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}]
This claim follows from an application of \Cref{lem:err-inv-com}, with the notation correspondence listed in \Cref{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}}
\label{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}  \\ 
\midrule
\addlinespace[0.3em]
$\reg{a}$   & $\reg{p_1}$ & & $W_1$ & $C_{1,1}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_0$ & $C_{1,0}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_1}$ & & $W$   & $C_{1}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u}$, $\reg{s}$, $\reg{gc}$ & & $\tilde{W}$ & $\ddot{C}_1$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p'_1}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_1$ & $B_{1,1}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & $\ket{\gamma^{(t-1)}_0}$ \\ 
\addlinespace[0.3em]
   & & & $U$   & $B_1$ & & $\ket{\eta^{(\msf{in})}_1}$ & $\ket{\gamma^{(t-1)}_1}$  \\ 
\addlinespace[0.3em]
 &  & &   $S$   & $U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}$ & &  $\ket{\rho^{(\msf{out})}_a}_\reg{mtso}$    & $\ket{\dot{\rho}^{(t)}_{p_1}}$  \\ 
\addlinespace[0.3em]
  &  & &   &  & &  $\ket{\rho^{(\msf{out})}_{a'}}_\reg{mtso}$     & $\ket{\dot{\rho}^{(t)}_{p'_1}}$  \\  
  \addlinespace[0.3em]
 &  & & & & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\gamma^{(t)}_0}$  \\
\addlinespace[0.3em] 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\gamma^{(t)}_1}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_1$ should work as the identity operator on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{1,1}$ (playing the role of $W_1$) who works as identity on registers $\reg{u}$, $\reg{s}$, and $\reg{gc}$ (playing the role of registers $\reg{s}$). (Recall $C_{1,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
\Cref{lem:err-inv-com} requires that $W_0$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{1,0}$ (playing the role of $W_0$), who is a swap operator between registers $\reg{m}$ and $\reg{t_1}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively). (Recall $C_{1,0}$ from \Cref{CPM-3ZK:renaming:C1}.)

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_0$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $\ddot{C}_1$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $C_{1,0}$ (playing the role of $W_0$) on branches $\ket{p'_1}_{\reg{p_1}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $p'_1 \ne p_1$. (Recall $\ddot{C}_1$ from \Cref{CPM-3ZK:renaming:ddotC1})

\item
 \Cref{lem:err-inv-com} requires that $U_1$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $B_{1,1}$ (playing the role of $U_1$), who works as identity on registers $\reg{u}$, $\reg{s}$, and $\reg{gc}$ (playing the role of register $\reg{s}$). (Recall $B_{1,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $U_{gc}S^{\reg{p_1}/\reg{m}}U^\dagger_{gc}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{u}$, $\reg{s}$, and $\reg{gc}$ (playing the role of registers $\reg{a}$ and $\reg{s}$). (Recall $S$ from \Cref{CPM-3ZK:non-trivial-registers:table} and the fact that $S^{\reg{p_1}/\reg{m}}$ is identical to $S$ except that it treats $\reg{p_1}$ as $\reg{m}$.)
\end{itemize}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}) to the $\ket{\gamma^{(t-1)}_0}$ and $\ket{\gamma^{(t-1)}_1}$ defined in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1}  (playing the role of $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ in \Cref{lem:err-inv-com}). This implies the existence of (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1}}}_{p'_1\in\bits^\ell }$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\gamma^{(t)}_0} 
& = \ket{p_1}_{\reg{p_1}}\ket{\dot{\rho}^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\dot{\rho}^{(t)}_{p'_1}} \\ 
\ket{\gamma^{(t)}_1} 
& = \ket{p_1}_{\reg{p_1}}\ket{\dot{\rho}^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\dot{\rho}^{(t)}_{p'_1}} 
,\end{align*}
which are exactly \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} in  \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. 






This completes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}.

\end{proof}

\para{Finishing the Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}.}\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} With \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} at hand, we now finish the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}.

\subpara{Proof for \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}.} We first establish \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}:
\begin{align}
\ket{\phi^{(t)}} 
& = D_1 \ket{\gamma^{(t)}_0} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:1} \\ 
& = D_1 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\bigg) 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} D_{1,1}\ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\rho^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:2} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} follows from the definition of $D_1$ (see \Cref{CPM-3ZK:renaming:D1});

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:4} follows by defining
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho}
\ket{\rho^{(t)}_{p_1}}   \coloneqq D_{1,1} \ket{\dot{\rho}^{(t)}_{p_1}} ~~~\text{and}~~~
\ket{\rho^{(t)}_{p'_1}}  \coloneqq \ket{\dot{\rho}^{(t)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}).
\end{equation}
\end{itemize}
Note that \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. 


\subpara{Proof for \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}.}  Next, we establish \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}:


\begin{align}
\ket{\psi^{(t)}} 
& = D_1 \ket{\gamma^{(t)}_1} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:1} \\ 
& = D_1 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t)}_{p'_1}} 
\bigg) 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} D_{1,1}\ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:2} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} follows from the definition of $D_1$ (see \Cref{CPM-3ZK:renaming:D1});

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:4} follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1}}$ and $\ket{\rho^{(t)}_{p'_1}}$ in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho}.
\end{itemize}
Note that \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. 

~\\ 
This eventually completes the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}.




\subsubsubsection{Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}} 
We first remark that in \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}, the computation that brings $\ket{\phi^{(t-1)}}$ to $\ket{\phi^{(t)}}$ is identical to that brings $\ket{\psi^{(t-1)}}$ to $\ket{\psi^{(t)}}$, because $H_0$ and $H_1$ are identical when the global counter ``jumps'' between $1$ and $2$. (This can be also seen pictorially by comparing \Cref{figure:CPM-3ZK:hybrids:H0} and \Cref{figure:CPM-3ZK:hybrids:H1}.) In the following, we refer to this computation as $\Lambda$. That is, we have 
\begin{align}
\ket{\phi^{(t)}} 
& = 
\Lambda \ket{\phi^{(t-1)}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi} \\ 
\ket{\psi^{(t)}} 
& = 
\Lambda \ket{\psi^{(t-1)}}
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi}
.\end{align} 

\para{Structure of $\Lambda$.} While the exact format of $\Lambda$ will not be substantial, our proof of \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2} will rely on certain properties of $\Lambda$, which we formalize in the following \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.

\begin{MyClaim}\label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}
For the operator $\Lambda$ defined above, there exist two operators $\Lambda_0$ and $\Lambda_1$ so that
\begin{itemize}
\item
both  $\Lambda_1$ and $\Lambda_0$ act as the identity operator on $\reg{p_1}$;
\item
$\Lambda_0$ acts as the identity operator on $\reg{t_1}$;
\end{itemize}
and the following holds
\begin{align}
& 
\Lambda = \ketbra{p_1}_{\reg{p_1}} \tensor \Lambda_1 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Lambda_0, \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} \\ 
& 
\Lambda_0 C_{1,0}  = C_{1,0} \Lambda^{\reg{t_1}/\reg{m}}_0, \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} \\ 
& 
\Lambda_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Lambda^{\reg{t_1}/\reg{m}}_0 \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} 
,\end{align}
where $\Lambda^{\reg{t_1}/\reg{m_1}}_1$ is identical to $\Lambda_1$ except that it treats $\reg{t_1}$ as $\reg{m_1}$.  
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}]

First, note that $\Lambda$ can be written as $\Lambda = \Gamma_z \Gamma_{z-1} \cdots \Gamma_1$ (for some integer $z$), where each $\Gamma_i$ ($i \in [z]$) comes from the set of operators $\Set{S, A_2, B_2, C_2, D_2, U_{gc}, \ketbra{p_1, p_2}_{\reg{p_1p_2}}}$. This is because $\Lambda$ only corresponds to the operations that happen when the global counter is no less than value $1$---\xiao{according to our notation in \Cref{CPM-3ZK:counter-structure:section}, only the  ``Layer-2'' operators will be applied.}

Therefore, to prove \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, it suffices to show that for each operator $\Gamma \in \Set{\ketbra{p_1, p_2}_{\reg{p_1p_2}}, U_{gc}, S, A_2, B_2, C_2, D_2}$, there exist two operators $\Gamma_0$ and $\Gamma_1$ so that
\begin{itemize}
\item
both  $\Gamma_1$ and $\Gamma_0$ act as the identity operator on $\reg{p_1}$;
\item
$\Gamma_0$ acts as the identity operator on $\reg{t_1}$;
\end{itemize}
and the following holds
\begin{align*}
& 
\Gamma = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_1 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_0,\\ 
& 
\Gamma_0 C_{1,0}  = C_{1,0} \Gamma^{\reg{t_1}/\reg{m}}_0, \\ 
& 
\Gamma_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Gamma^{\reg{t_1}/\reg{m}}_0 
.\end{align*}
In the following, we prove it for each possible $\Gamma$.

First, notice that the above is true for $\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}}$, simply because such a $\Gamma$ can be written in the following format:
$$\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_1  + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_0,$$
with $\Gamma_1  \coloneqq \ketbra{p_2}_{\reg{p_2}}$ and $\Gamma_0  \coloneqq I$, and such a $\Gamma_0$ vacuously satisfies the requires $\Gamma_0 C_{1,0}  = C_{1,0} \Gamma^{\reg{t_1}/\reg{m}}_0$ and $\Gamma_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Gamma^{\reg{t_1}/\reg{m}}_0$.

The above is true for $\Gamma = U_{gc}$ as well, because $U_{gc}$ acts non-trivially only on register $\reg{gc}$.


The above is also true for $\Gamma = S$ because (1) $S$ does not act on $\reg{p_1}$, (2) $S$ does not work on $\reg{t_1}$ and $C_{1,0}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_1}$, and (3) $S^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $C_{1,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}).

The above is true for $\Gamma = A_2$ as well, because $A_2$ is nothing but the swap operator between registers $\reg{p_2}$ and $\reg{m}$.

The only  cases left are $\Gamma \in \Set{B_2, C_2, D_2}$. The proof for these cases are (almost) identical. In the following, we only prove it for $\Gamma = C_2$.
\begin{align*}
\Gamma = C_2 
& = 
\ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0} \numberthis \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:1} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor C_{2,1}
+ 
\sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1}_{\reg{p_1}} \tensor \ketbra{p'_2}_{\reg{p_2}} \tensor C_{2,0} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor C_{2,1} 
+ \ketbra{p_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0} \\ 
& \hspace{15em} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0} \\ 
& = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_1 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_0 \numberthis \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:2}
,\end{align*}
where \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:1} follows from the definition of $C_2$ (see \Cref{CPM-3ZK:renaming:C2}), and \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:2} follows by defining $\Gamma_0$ and $\Gamma_1$ as follows 
\begin{align*}
 \Gamma_1 & \coloneqq \ketbra{p_2}_{\reg{p_2}} \tensor C_{2,1} 
+ \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0} \\ 
 \Gamma_0 & \coloneqq \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0}.
\end{align*} 
Clearly, such a $\Gamma_0$ satisfies the requires $\Gamma_0 C_{1,0}  = C_{1,0} \Gamma^{\reg{t_1}/\reg{m}}_0$ and $\Gamma_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Gamma^{\reg{t_1}/\reg{m}}_0$, because (1) $C_{2,0}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_2}$, and (2) $C_{2,0}^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $ C_{1,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}).


This finishes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.	

\end{proof}





\para{Finishing the Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}.} With \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute} in hand, we now show how to finish the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}.

\subpara{Proof of \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}.} First, we establish \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}:
\begin{align}
 \ket{\phi^{(t)}} 
 & = 
 \Lambda  \ket{\phi^{(t-1)}}  
 \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:0}\\ 
& = 
\Lambda  
  \bigg(
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
  \bigg)  
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:1}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \Lambda_0 C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:2}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \Lambda^{\reg{t_1}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:3}\\ 
    & =  
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:4}
,\end{align}
where  
\begin{itemize}
\item

\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi}, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:1} follows from our induction assumption, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:2}  follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:3} follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, 

\item 
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:4} follows by defining
\begin{equation}\label[Expression]{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:def:rho-t}
\ket{\rho^{(t)}_{p_1}} 
\coloneqq 
 \Lambda_1 \ket{\rho^{(t-1)}_{p_1}} ~~~\text{and}~~~ 
\ket{\rho^{(t)}_{p'_1}} 
\coloneqq 
\Lambda^{\reg{t_1}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}). 
\end{equation}
\end{itemize}
Clearly, \Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:4} is of the same format as \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.

\subpara{Proof of \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}.} Next, we present the derivation for  \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}:
\begin{align}
 \ket{\psi^{(t)}} 
 & = 
 \Lambda  \ket{\psi^{(t-1)}}  
 \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0}\\ 
& = 
\Lambda  
  \bigg(
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0}  \ket{\rho^{(t-1)}_{p'_1}}
  \bigg)  
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \Lambda_0 C_{1,0}  \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \Lambda^{\reg{t_1}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3}\\ 
    & =  
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4}
,\end{align}
where  
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi}, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1} follows from our induction assumption, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2}  follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3} follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, 

\item 
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1}}$ and $\ket{\rho^{(t)}_{p'_1}}$ as shown in \Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:def:rho-t}.
\end{itemize}
Clearly, \Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} is of the same format as \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.



This finishes the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}.


\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:sec} together finish the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, which in turn finishes the proof of \Cref{lem:CPM-3ZK:H01} eventually.



\subsection{Proof of \Cref{lem:CPM-3ZK:H12}}

Due to a similar argument as we did at the beginning of \Cref{sec:lem:CPM-3ZK:H01:proof}, we claim that: to prove \Cref{lem:CPM-3ZK:H12}, it suffices to establish the following \Cref{lem:CPM-3ZK-hyb12:proof:invariant}.

\begin{lemma}[Invariance in $H_1$ and $H_2$]\label{lem:CPM-3ZK-hyb12:proof:invariant}
Assume that during the execution of $H_1$ (and $H_2$), the global counter reaches value $2$ for $T$ times in total. For each $t \in [T]$, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1, p'_2}}}_{p'_1, p'_2 \in \bits^\ell \times \bits^\ell}$ so that the following holds: in hybrid $H_1$ (resp.\ $H_2$), when the global counter reaches value $2$ for the $t$-th time, the overall state can be written as $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows
\begin{align}
\ket{\phi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1, p_2}}  ~+~
   \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t)}_{p'_1, p'_2}}, \label{lem:CPM-3ZK-hyb12:proof:target-format:H1}\\ 
\ket{\psi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1, p_2}}  ~+~
 \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \red{C_{2,0}} \ket{\rho^{(t)}_{p'_1, p'_2}}. \label{lem:CPM-3ZK-hyb12:proof:target-format:H2}
\end{align}
where the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above), and the unitaries $B_{2,1}$, $C_{2,0}$, and $C_{2,1}$  are as defined in \Cref{CPM-3ZK:renaming:B2,CPM-3ZK:renaming:C2}.
\end{lemma}

\para{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant}.} Similar as the proof for \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, 
we establish \Cref{lem:CPM-3ZK-hyb12:proof:invariant} by a mathematical induction on the number $t \in [T]$  indicating it is which time the global counter reaches value 2. We will keep
track of how the overall states evolve in both $H_1$ and $H_2$ simultaneously.







\subsubsection{Base Case ($t = 1$)}
\label{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec} 

This corresponds to the very first time the global counter reaches $2$. By definition, this is due to $\Sim$'s query $\msf{sq}(2)$. 

We first derive how the overall state evolves in $H_1$. Formally, $\Sim$'s local operation $S$ is applied to the initial state, preparing a superposition in register $\reg{m}$. Then, the first $\tilde{V}$-query (i.e., the query $\msf{sq}(1)$) is made.  According to \xiao{our discussion in \Cref{CPM-3ZK:counter-structure:section}}, the operator $D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}A_2U_{gc}$ will be applied. 

Also, note that the state right before this query has global counter 1. It follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant} that the state must be of the format  $\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho_{p'_1}}$. 

In summary, the state $\ket{\phi^{(1)}}$ in $H_1$ can be written as follows:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}A_2U_{gc} S   
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho_{p'_1}}
\bigg)
\\
& =  
D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}   
\bigg(
\ket{p_1}_{\reg{p_1}} A_2U_{gc} S \ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  A_2U_{gc}S C_{1,0}\ket{\rho_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:1}\\
& =  
D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}   
\bigg(
\ket{p_1}_{\reg{p_1}} \sum_{p'_2 \in \bits^\ell} \ket{p'_2}_{\reg{p_2}} \ket{\rho_{p_1, p'_2}} + \\ 
& \hspace{18em}
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \sum_{p'_2 \in \bits^\ell} \ket{p'_2}_{\reg{p_2}} \ket{\rho_{p_1, p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:2}\\ 
& =  
D_2C_2B_2\ket{p_1, p_2}_{\reg{p_1p_2}} \ket{\rho_{p_1, p_2}} \\ 
& =  
\ket{p_1, p_2}_{\reg{p_1p_2}}D_{2,1}C_{2,1}B_{2,1}\ket{\rho_{p_1, p_2}} 
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3}\\ 
& =  
\ket{p_1, p_2}_{\reg{p_1p_2}}\ket{\rho^{(1)}_{p_1, p_2}} 
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:4}
,\end{align*}
where
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:1} follows from the fact that $A_2$, $U_{gc}$  and $S$ act as the identity operator on $\reg{p_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:2} follows from decomposing the $\reg{p_2}$ register in the computational basis for states $A_2U_{gc} S \ket{\rho_{p_1}}$ and $A_2U_{gc} S C_{1,0} \ket{\rho_{p'_1}}$;

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3} follows from the definitions of $B_2$, $C_2$, and $D_2$ (see \Cref{CPM-3ZK:renaming:B2,CPM-3ZK:renaming:C2,CPM-3ZK:renaming:D2});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:4} follows by defining $\ket{\rho^{(1)}_{p_1, p_2}} \coloneqq D_{2,1}C_{2,1}B_{2,1}\ket{\rho_{p_1, p_2}}$.
\end{itemize}
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:4} satisfies the format shown in \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1} when $t = 1$.

Also, note that the game $H_1$ and $H_2$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:4} that 
$$\ket{\psi^{(1)}} =  \ket{p_1, p_2}_{\reg{p_1p_2}} \ket{\rho^{(1)}_{p_1,p_2}}.$$ Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.


\subsubsection{Induction Step ($t \ge 2$)} 
\label{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec} 

We assume $\ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t-1)}}$ satisfies \Cref{lem:CPM-3ZK-hyb12:proof:invariant}, and show in the following that \Cref{lem:CPM-3ZK-hyb12:proof:invariant} holds when the global counter reaches $2$ for the $t$-th time.

We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$):
\begin{enumerate}
 \item
$\Sim$'s local unitary $S$ is applied. Note that this step is identical for both $H_1$ and $H_2$. 

\item
An $\uparrow$-query is made, bringing the global counter from 2 to 1.  \xiao{According to our notation in \Cref{CPM-3ZK:counter-structure:section}}: 
\begin{itemize}
    \item
    In $H_1$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_2 B^\dagger_2 C^\dagger_2 D^\dagger_2$; 
    \item
    In $H_2$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_2 \ddot{C}^\dagger_2 D^\dagger_2$. 
\end{itemize}
\item \label[Step]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:description:def:lambda}
At this point, there are two cases to consider: 
\begin{enumerate}
\item \label[Case]{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-1}
 $\Sim$ can make a $\downarrow$-query immediately, bringing the global counter back to $2$; {\em or } 
\item \label[Case]{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-2}
 $\Sim$ can rewind $\tilde{V}$ further, bringing the global counter to $0$.  
\end{enumerate}
Looking ahead, our proof can handle these two cases at one stroke. To do that, we denote the execution from this point until (exclusively) {\em the next $\downarrow$ query that brings the global counter to value $2$} (i.e., the exact query that yields the global counter's $t$-th arrival at value $2$) as an operator $\Lambda$. $\Lambda$ might be $\Sim$ local operator $S$ {\em only}, corresponding to \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-1}; $\Lambda$ might also be the combonation of some other operators, representing the operations performed in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-2} before the global counter's next arrival at value 2. 

\item
After the application of the operator $\Lambda$ defined above, an $\downarrow$-query is made, bringing the global counter from 1 back to 2, which is the global counter's $t$-th arrival at value 2. \xiao{According to our notation in \Cref{CPM-3ZK:counter-structure:section}}: 
\begin{itemize}
    \item
    In $H_0$, this corresponds to applying $D_2C_2B_2A_2U_{gc}$; 
    \item
    In $H_1$, this corresponds to applying $D_2\ddot{C}_2A_2U_{gc}$. 
\end{itemize} 
\end{enumerate}
It follows from the above description that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
\begin{align}
\ket{\phi^{(t)}}
& = D_2C_2B_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 B^\dagger_2 C^\dagger_2 D^\dagger_2 S  \ket{\phi^{(t-1)}}, \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1}\\ 
\ket{\psi^{(t)}}
& = D_2 \ddot{C}_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 \ddot{C}^\dagger_2 D^\dagger_2 S \ket{\psi^{(t-1)}}. \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2}
\end{align}

We first make a useful claim that specifies the registers on which the $\Lambda$ defined above act non-trivially. 
\begin{MyClaim}[Non-Trivial Registers for $\Lambda$]\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}
The $\Lambda$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:description:def:lambda} acts non-trivially only on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$ (i.e., it works as the identity operator on the other registers). 
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}]

By definition, $\Lambda$ only contains operations that happen when the global counter is $1$ or smaller. This is best illustrated by \Cref{figure:CPM-3ZK:hybrids:H1}---$\Lambda$ only contains operations that happen in between the line corresponding to $\ket{0}_{\reg{gc}}$ and the line corresponding to $\ket{1}_{\reg{gc}}$ (except for the $\tilde{V}$ corresponding $\msf{sq}(1)$). 

Therefore, $\Lambda$ can be written as $\Lambda = \Gamma_z \Gamma_{z-1} \cdots \Gamma_1$ (for some integer $z$), where each $\Gamma_i$ ($i \in [z]$) comes from the set of operators $\Set{S, A_1,  \ddot{C}_1, D_1, U_{gc}}$. It then follows from \Cref{CPM-3ZK:non-trivial-registers:table} that $\Lambda$ works non-trivially only on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$.

This finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}.

\end{proof}

\begin{remark}[High-Level Idea for the Sequel]
Recall that our eventual goal is to prove that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ are of the format shown in \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1,lem:CPM-3ZK-hyb12:proof:target-format:H2} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2}. But we first need to perform some preparation work, putting \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}. Then, we show on \Cpageref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish} how to use \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} to complete the proof for the induction step. 
\end{remark}




The following \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} can be viewed as an analog of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.
\begin{MyClaim}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}
There exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds
\begin{align*}
\ket{\phi^{(t)}}
& =  
D_2C_2 B_2 U_{gc} \Lambda^{\reg{p_2}/\reg{m}} U_{gc}^\dagger   B^\dagger_2 C^\dagger_2
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}  
+ \\ 
& \hspace{16em} 
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\bigg) \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(t)}}
& = 
D_2\ddot{C}_2 U_{gc}\Lambda^{\reg{p_2}/\reg{m}}  U_{gc}^\dagger \ddot{C}^\dagger_2 
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}   +  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\bigg) 
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} 
\end{align*}
where $\Lambda^{\reg{p_2}/\reg{m}}$ is identical to the $\Lambda$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:description:def:lambda}, except that it treats register $\reg{p_2}$ as $\reg{m}$, and the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}]
First, notice that  
\begin{align*}
 A_2 U_{gc} \Lambda U^\dagger_{gc} A^\dagger_2 
 & = 
 A_2 U_{gc} \Lambda A^\dagger_2 U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:1} \\ 
 & = 
 A_2 U_{gc} A^\dagger_2 \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:2} \\
  & = 
 A_2 A^\dagger_2 U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:3} \\
 & = 
U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:1,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:3} follows from the fact that $U_{gc}$ acts non-trivially on different registers from $A_2$;

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:2} from the fact that $\Lambda$ acts as the identity operator on $\reg{p_2}$ (see \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}) and that $A_2$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_2}$ (see \Cref{CPM-3ZK:V:unitary}). 
\end{itemize}

\subpara{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(t)}}$:
\begin{align*}
\ket{\phi^{(t)}}
& =
D_2C_2B_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 B^\dagger_2 C^\dagger_2 D^\dagger_2  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:0} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2 D^\dagger_2  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:1} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2 D^\dagger_2 S 
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:2} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2 D^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} SC_{2,0} B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:3} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} S C_{2,0}  B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:4} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} S^{\reg{t_2}/\reg{m}}  B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:5} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  S^{\reg{t_2}/\reg{m}}  \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:6} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}     \ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1};

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S};

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:2} follows from our induction assumption;

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:3} from  from the fact that $S$ acts as the identity operator on $\reg{p_1}$ and $\reg{p_2}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:4} from the definition of $D_2$ (see \Cref{CPM-3ZK:renaming:D2});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:5} from the fact that $S$ acts as the identity operator on $\reg{t_2}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}) and $C_{2,0}$ is nothing but a swap operator between $\reg{t_2}$ and $\reg{m}$ (see \Cref{CPM-3ZK:renaming:C2}); (Note that $S^{\reg{t_2}/\reg{m}}$ is defined to be an operator that is identical to $S$ except that it treats $\reg{t_2}$ as $\reg{m}$.)

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:6} follows from the fact that $S^{\reg{t_2}/\reg{m}}$ acts non-trivially on different registers from $B_{2,1}$ and $C_{2,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:7} follows by defining 
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho-dot}
\ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}   \coloneqq D^\dagger_{2,1} S \ket{\rho^{(t-1)}_{p_1,p_2}} ~~~\text{and}~~~
\ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}  \coloneqq S^{\reg{t_2}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1,p'_2}} ~~\big(\forall (p'_1,p'_2) \in \big(\bits^\ell \times \bits^\ell\big) \setminus \Set{(p_1,p_2)}\big).
\end{equation}
\end{itemize}
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\subpara{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi}.} We now show the derivation for $\ket{\psi^{(t)}}$. This is almost identical to the above proof for \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.


\begin{align*}
\ket{\psi^{(t)}}
& =
D_2\ddot{C}_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 \ddot{C}^\dagger_2 D^\dagger_2  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:0} \\ 
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} \ddot{C}^\dagger_2 D^\dagger_2  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:1} \\ 
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} \ddot{C}^\dagger_2 D^\dagger_2 S 
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(t-1)}_{p_1,p_2}} 
+
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} C_{2,0} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:2} \\  
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} \ddot{C}^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  
+ 
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}  S^{\reg{t_2}/\reg{m}}  \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:6} \\ 
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1,p_2}} 
+
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2};

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S};


\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:2}  follows from our induction assumption;


\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:6} follows from a similar argument as we did to derive \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:6} from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:2};


\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:7} follows from {\em the same definitions} of $\ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}$ and $\ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}$ as shown in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho-dot}.
\end{itemize}
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\vspace{1em}
This finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\end{proof}

The following \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} can be treated as an analog of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. 
\begin{MyClaim}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}
Let $\Lambda^{\reg{p_2}/\reg{m}}$ and $\Set{\dot{\rho}^{(t-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ be as defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}. Let
\begin{align}
\ket{\gamma^{(t-1)}_0} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:in:0} \\ 
\ket{\gamma^{(t-1)}_1} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}   \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:in:1} \\ 
\ket{\gamma^{(t)}_0} 
& \coloneqq 
C_2 B_2 U_{gc} \Lambda^{\reg{p_2}/\reg{m}} U_{gc}^\dagger   B^\dagger_2 C^\dagger_2 \ket{\gamma^{(t-1)}_0} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:0} \\ 
\ket{\gamma^{(t)}_1}
& \coloneqq 
\ddot{C}_2 U_{gc}\Lambda^{\reg{p_2}/\reg{m}}  U_{gc}^\dagger \ddot{C}^\dagger_2 
 \ket{\gamma^{(t-1)}_1}
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:1} 
.\end{align}
Then, there exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds:
\begin{align}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:0} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}   \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:1} 
.\end{align}
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}]
This claim follows from an application of \Cref{lem:err-inv-com}, with the notation correspondence listed in \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}}
\label{lem:CPM-3ZK-hyb12:proof:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1}$, $\reg{p_2}$ & & $W_1$ & $C_{2,1}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1,p_2}_{\reg{p_1p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_0$ & $C_{2,0}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1,p'_2}_{\reg{p_1p_2}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_2}$ & & $W$   & $C_{2}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u}$, $\reg{s}$, $\reg{t_1}$, $\reg{gc}$, $\reg{lc}$ & & $\tilde{W}$ & $\ddot{C}_2$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_1$ & $B_{2,1}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & $\ket{\gamma^{(t-1)}_0}$ \\ 
\addlinespace[0.3em]
   & & & $U$   & $B_2$ & & $\ket{\eta^{(\msf{in})}_1}$ & $\ket{\gamma^{(t-1)}_1}$  \\ 
\addlinespace[0.3em]
 &  & &   $S$   & $U_{gc}\Lambda^{\reg{p_2}/\reg{m}}U^\dagger_{gc}$ & &  $\ket{\rho^{(\msf{out})}_a}_\reg{mtso}$    & $\ket{\dot{\rho}^{(t)}_{p_1,p_2}}$  \\ 
\addlinespace[0.3em]
  &  & &   &  & &  $\ket{\rho^{(\msf{out})}_{a'}}_\reg{mtso}$     & $\ket{\dot{\rho}^{(t)}_{p'_1,p'_2}}$  \\  
  \addlinespace[0.3em]
 &  & & & & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\gamma^{(t)}_0}$  \\
\addlinespace[0.3em] 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\gamma^{(t)}_1}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_1$ should work as the identity operator on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{2,1}$ (playing the role of $W_1$) who works as identity on registers $\reg{u}$, $\reg{s}$, $\reg{t_1}$, $\reg{gc}$, and $\reg{lc}$ (playing the role of registers $\reg{s}$). (Recall $C_{2,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
\Cref{lem:err-inv-com} requires that $W_0$ should be the swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{2,0}$ (playing the role of $W_0$), who is the swap operator between registers $\reg{m}$ and $\reg{t_2}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively). (Recall $C_{2,0}$ from \Cref{CPM-3ZK:renaming:C2}.)

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_0$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $\ddot{C}_2$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1, p_2}_{\reg{p_1p_2}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $C_{2,0}$ (playing the role of $W_0$) on branches $\ket{p'_1, p'_2}_{\reg{p_1p_2}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, p'_2) \ne (p_1, p_2)$. (Recall $\ddot{C}_2$ from \Cref{CPM-3ZK:renaming:ddotC2})

\item
 \Cref{lem:err-inv-com} requires that $U_1$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $B_{2,1}$ (playing the role of $U_1$), who works as identity on registers $\reg{u}$, $\reg{s}$, $\reg{t_1}$, $\reg{gc}$, and $\reg{lc}$ (playing the role of register $\reg{s}$). (Recall $B_{2,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $U_{gc}\Lambda^{\reg{p_2}/\reg{m}}U^\dagger_{gc}$ (playing the role of $S$)---recall from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim} that $\Lambda$ acts non-trivially on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$. Thus, $U_{gc}\Lambda^{\reg{p_2}/\reg{m}}U^\dagger_{gc}$ acts non-trivially on registers $\reg{p_2}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$, which constitute registers $\reg{a}$ and $\reg{s}$ (see \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}). 
\end{itemize}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}) to the $\ket{\gamma^{(t-1)}_0}$ and $\ket{\gamma^{(t-1)}_1}$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:0,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:1}  (playing the role of $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ in \Cref{lem:err-inv-com}). This implies the existence of (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1,p'_2}}}_{(p'_1, p'_2)\in\bits^\ell \times \bits^\ell}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}   \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}   \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}}  
,\end{align*}
which are exactly \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:0,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:1} in  \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}. 






This completes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}.

\end{proof}





% \begin{MyClaim}
% % \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}
% There exist (potentially sub-normalized) pure states $\Set{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds
% \begin{align}
% \ket{\phi^{(k)}}
% & = \tilde{U}_6 \tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}}   \tilde{U}^\dagger_5 \tilde{U}^\dagger_6
% \bigg( 
% \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} \\ 
% \ket{\psi^{(k)}}
% & = 
% B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}}  B^\dagger_{\msf{dmy}}
% \bigg( 
% \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} 
% \end{align}
% where $\Lambda^{\reg{p_2}/\reg{m}}$ is identical to $\Lambda$ except that it treats register $\reg{p_2}$ as $\reg{m}$, and the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
% \end{MyClaim}
% \begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}]
% First, notice that
% \begin{equation}\label{lem:CPM-3ZK-hyb12:proof:case-2:eq:swap-Lambda} 
% \tilde{U}_4 \Lambda \tilde{U}^\dagger_4 = \tilde{U}_4  \tilde{U}^\dagger_4 \Lambda^{\reg{p_2}/\reg{m}} = \Lambda^{\reg{p_2}/\reg{m}},
% \end{equation}
% where the first equality follows from the fact that $\Lambda^{\reg{p_2}/\reg{m}}$ does not operate on $\reg{p_2}$ and $\tilde{U}^\dagger_4$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_2}$.

% \para{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(k)}}$:

% \begin{align*}
% \ket{\phi^{(k)}}
% & = 
% \tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \ket{\phi^{(k-1)}} \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1} \\
% & = 
% \tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} S_j \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}
% ,\end{align*}
% where \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1}  follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi}, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} follows from our induction assumption, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3} follows from \Cref{lem:CPM-3ZK-hyb12:proof:case-2:eq:swap-Lambda}, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  follows from the fact that $S_j$ works as identity on registers $\reg{p_1}$ and $\reg{p_2}$ (see \Cref{CPM-3ZK:table:non-trivial-registers}), \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  follows from the definitions of $\tilde{U}_{6,1}$ and $S^{\reg{t_2}/\reg{m}}_j$, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  follows from the fact that $S^{\reg{t_2}/\reg{m}}_j$ and $\tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} $ act non-trivially on different registers (see \Cref{CPM-3ZK:table:non-trivial-registers}), and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  follows by defining
% \begin{equation}
% \label[Expression]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}
% \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}} \coloneqq S_j \ket{\rho^{(k-1)}_{p_1, p_2}} ~~~\text{and}~~~ \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \coloneqq S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}~~~(\forall (p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}).
% \end{equation}
% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

% \para{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi}.} This proof is almost identical to the above proof for \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
% \begin{align*}
% \ket{\psi^{(k)}}
% & = 
% B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \ket{\psi^{(k-1)}} \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} \\
% & = 
% B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1}  \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2} \\ 
% & =
% B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}} B^\dagger_{\msf{dmy}} \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}
% ,\end{align*}
% where \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2}  follows from our induction assumption, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} follows from a similar argument as we did to \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6} from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2}, and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4} follows from the same definition of $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$ and $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ as shown in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}

% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}  finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.


% This eventually finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

% \end{proof}


% \para{Finishing the Induction Step.}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish} 
%  With the above \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} in hand, we can finish the induction step by applying \Cref{lem:err-inv-com}. Formally, we apply \Cref{lem:err-inv-com} to the states and operators in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}, with the notation correspondence listed in \Cref{lem:CPM-3ZK-hyb12:proof:induction:cor-table}. We provide a detailed explanation below.
% \begin{table}[!htb]
% \centering
% \caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}}
% \label{lem:CPM-3ZK-hyb12:proof:induction:cor-table}
% \vspace{0.5em}
% \begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
% \toprule
%  \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
% \phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
% In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}  \\ 
% \midrule
% % \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
% \addlinespace[0.3em]
% $\reg{a}$    & $\reg{p_1}$, $\reg{p_2}$ & & $W_0$ & $\tilde{U}_{6,0}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$  \\ 
% \addlinespace[0.3em]
% $\reg{m}$    & $\reg{m}$ & & $W_1$ & $\tilde{U}_{6,1}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$  \\
% \addlinespace[0.3em]
% $\reg{t}$    & $\reg{t_2}$ & & $W$   & $\tilde{U}_{6}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$  \\ 
% \addlinespace[0.3em]
% $\reg{s}$    & $\reg{t_1}$,  $\reg{u}$, $\reg{s}$ & & $\tilde{W}$ & $B_{\msf{dmy}}$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ \\ 
% \addlinespace[0.3em]
% $\reg{o}$    & other registers & & $U_0$ & $\tilde{U}_{5,0}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0} \\ 
% \addlinespace[0.3em]
%    & & & $U$   & $\tilde{U}_{5}$ & & $\ket{\eta^{(\msf{in})}_1}$ & \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}  \\ 
%    \addlinespace[0.3em]
%  &  & & $S$   & $\Lambda^{\reg{p_2}/\reg{m}}$ & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\phi^{(\msf{k})}}$  \\ 
%   &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\psi^{(\msf{k})}}$  \\   
% \bottomrule
% \end{tabular}
% \end{table}

% First, we argue that the premises of \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:CPM-3ZK-hyb12:proof:induction:cor-table}:
% \begin{itemize}
% \item
% \Cref{lem:err-inv-com} requires that $W_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,0}$ (playing the role of $W_0$) who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$ (playing the role of registers $\reg{s}$).

% \item
% \Cref{lem:err-inv-com} requires that $W_1$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,1}$ (playing the role of $W_1$), who is a swap operator between registers $\reg{m}$ and $\reg{t_2}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively).

% \item
% \Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_1$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $B_{\msf{dmy}}$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $\tilde{U}_{6,1}$ (playing the role of $W_1$) on branches $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, p'_2) \ne (p_1, p_2)$.

% \item
%  \Cref{lem:err-inv-com} requires that $U_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{5,0}$ (playing the role of $U_0$), who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of register $\reg{s}$).

% \item
%  \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\Lambda^{\reg{p_2}/\reg{m}}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{p_2}$,  $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of registers $\reg{a}$ and $\reg{s}$).
% \end{itemize}

% Next, using the above notation, we could define
% \begin{align}
% \ket{\eta^{(\msf{in})}_0}
% & \coloneqq 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}   \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{4,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}, \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0}  \\ 
% \ket{\eta^{(\msf{in})}_1}
% & \coloneqq 
%  \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}.  \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}   
% \end{align}

% Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:CPM-3ZK-hyb12:proof:induction:cor-table}) to the $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}. This implies the existence of (potentially non-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1, p'_2}}}_{(p'_1, p'_2) \in\bits^\ell \times \bits^\ell}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
% \begin{align*}
% \ket{\phi^{(k)}} 
% & = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k)}_{p'_1,p'_2}} \\ 
% \ket{\psi^{(k)}} 
% & = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\rho^{(k)}_{p'_1,p'_2}} 
% ,\end{align*}
% which are exactly \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1,lem:CPM-3ZK-hyb12:proof:target-format:H2} in  \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. 

% This finishes the induction step.


% \vspace{1em}
% Finally, we remark that our proof for the base case in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec}   together finish the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant} eventually.




\para{Finishing the Proof for the Induction Step.}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish} With \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} at hand, we now finish the proof for the induction Step.

\subpara{Proof for \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1}.} We first establish \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1}:
\begin{align}
\ket{\phi^{(t)}} 
& = D_2 \ket{\gamma^{(t)}_0} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:1} \\ 
& = D_2 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\bigg) 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} D_{2,1} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\rho^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:0} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:2} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:0} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:3} follows from the definition of $D_2$ (see \Cref{CPM-3ZK:renaming:D2});

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:4} follows by defining
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho}
\ket{\rho^{(t)}_{p_1,p_2}}   \coloneqq D_{2,1} \ket{\dot{\rho}^{(t)}_{p_1,p_2}} ~~~\text{and}~~~
\ket{\rho^{(t)}_{p'_1,p'_2}}  \coloneqq \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} ~~\big(\forall (p'_1, p'_2) \in \big(\bits^\ell \times \bits^\ell\big) \setminus \Set{(p_1,p_2)}\big).
\end{equation}
\end{itemize}
Note that \Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. 


\subpara{Proof for \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2}.} We next establish \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2}:
\begin{align}
\ket{\psi^{(t)}} 
& = D_2 \ket{\gamma^{(t)}_1} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:1} \\ 
& = D_2 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\bigg) 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} D_{2,1} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}   \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}  \ket{\rho^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:1} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:2} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:1} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:3} follows from the definition of $D_2$ (see \Cref{CPM-3ZK:renaming:D2});

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:4} follows follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1, p_2}}$ and $\ket{\rho^{(t)}_{p'_1, p'_2}}$ in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho}.
\end{itemize}
Note that \Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. 

This finishes the proof of the induction step of \Cref{lem:CPM-3ZK-hyb12:proof:invariant}.

\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec} together finish the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant}, which in turn finishes the proof of \Cref{lem:CPM-3ZK:H12} eventually.


==> sections/CPM-babycase-simplified.tex <==
\section{Impossibility of Constant-Round Black-Box Quantum Zero-Knowledge}


\xiao{I change the model to a classical-prover-message (CPM) model. This is to reflect the final soundness reduction, where we have to receive unmeasured Verifier's messages from the external verifier. Only in this way can we ensure that the view of the simulator is identical to that in our dummy up-and-down game.}


In this section, we show as a warm-up example that three-round ZK in the CPM model is impossible. This proof already illustrate the main ideas behind our general impossibility for the constant-round case. \xiao{Note that even such a result is not known yet.}






\subsection{The Model}

\subsubsection{Protocol Structure}
 We consider a three-round protocol where the prover $\Prover$ and verifier $\Verifier$ takes a statement $x \in \Lang$ and the security parameter $\secpar$ as the comment input. $\Prover$ additional takes a witness $w \in \Relation_\Lang(x)$ as the private input. $\Prover$ sends the first message $p_1$; $\Verifier$ responds with the second message $v_1$; then, $\Prover$ sends the final message $p_2$. W.l.o.g., we assume that all these massages are of the same length $\ell(\secpar)$, which is a polynomial in $\secpar$. Since we are in the CMP model, the messages $(p_1, p_2)$ are all classical, but the message $v_2$ could be quantum. 

 \xiao{from now one, we append one more message $v_2$ (possibly quantum) at the end of the execution. This message is just that the honest verifier let $P$ know if the execution is accepted or not. Not that this can only make our impossibility stronger! So, the protocol now has four rounds, i.e., $(p_1, v_1, p_2, v_2)$. And we will keep calling it four-round CPM BBZK.}

\para{Honest Verifier}  \xiao{need to explain to specify the model.}





\subsubsection{Generic Malicious Verifier}

\begin{xiaoenv}{Generic Malicious Verifier}
A malicious verifier $\tilde{\Verifier}$ could differ from the honest $\Verifier$ in the following way:
\begin{itemize}
\item
Its work space $\reg{w}$ could be larger than $\Verifier$;
\item
It make take an auxiliary input $\ket{\rho}$ of polynomial size, stored in some part in $\reg{w}$ at the beginning of the protocol;
\item
It may use a different unitary $V^*$ (can be implemented by poly-size quantum circuits) from the honest $\Verifier$.
\end{itemize}
Other than the above, it behaves in the same way as the honest $\Verifier$.
\end{xiaoenv}

 


\subsubsection{ZK Simulator}
 We now describe formally how the simulator $\Sim$ interacts with a generic malicious verifier $\tilde{\Verifier}$. Once again, there are multiple ways to do so and we choose the following one without loss of generality, which is particularly suitable for our proof of impossibility.

Note that we focus on black-box simulation. Thus, $\Sim$ can only query $\tilde{\Verifier}$ via its unitary $\tilde{V}$ and its inverse $\tilde{V}^\dagger$, but does not get to see the internal register $\reg{w}$ of $\tilde{\Verifier}$. 


Also, recall that $\reg{m}$ is used to exchange messages, and as explained above, it is always measured when a party is about to send message in the real execution (as we are in the LOCC setting). However, it is worth noticing that for simulation, $\reg{m}$ is considered as being held by $\Sim$, who could choose {\em not} to measure it. 

In more detail, a black-box simulator $\Sim$ is defined by a ``local'' unitary $S$. It is granted oracle access to $\tilde{V}$ and $\tilde{V}^\dagger$. It makes use of the following registers
\begin{itemize}
\item
Register $\reg{m}$ to exchange messages with the malicious verifier $\tilde{V}$;
\item
Register $\reg{s}$ which is her ``local'' work space;
\item
A query register $\reg{u}$ in a $2$-dimension Hilbert space spanned by the basis $\Set{ \ket{\downarrow}_{\reg{u}}, \ket{\uparrow}_{\reg{u}}}$ (explained shortly).
\end{itemize}
$\Sim$ behavior is nothing but iterations of the following three steps:
\begin{enumerate}
\item
Apply the local operator $S$ on registers $\reg{m}$, $\reg{u}$, and $\reg{s}$;
\item
Measure the $\reg{u}$ register to learn the type of the next query (see the next bullet);
\item
Make the oracle query according to the measurement outcome from the last step---if the measurement outcome is $\ket{\uparrow}$, it query the $\tilde{V}$ oracle on $\reg{m}$; otherwise (i.e., the measurement outcome is $\ket{\uparrow}$), it query the $\tilde{V}^\dagger$ oracle on $\reg{m}$.
\end{enumerate}
$\Sim$ keeps repeating the above three steps until she decides to stop. At that moment, the internal state of $\tilde{V}$ is defined to be the simulation output.



% \para{Formal Description of $\Sim^{\tilde{V}(x, \ket{\rho})}$.} With the above intuitive explanation, we proceed to present the formal description of the interaction between $\Sim$ and a malicious verifier $\tilde{V}(x, \ket{\rho})$. 

% The execution starts by initializing the following state:
% \begin{equation}\label{2-LOCC:S:inital:expr}
% \ket{\eta_0} \coloneqq \ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{\phi}_{\reg{o}} \ket{\downarrow_1}_{\reg{u_1}} \ldots \ket{\downarrow_1}_{\reg{u_q}} \ket{\rho}_{\reg{s}},
% \end{equation}





% \para{$\Sim$'s Behavior.} 
% \begin{xiaoenv}{}
% Start with the intermediate measurement. And then say that all the measurements on $\reg{u_j}$'s can be deferred, because a consequence of deferred measurement principle is:
% \begin{quote}
% {\em If after a measurement a qubit is used as a control qubit only, then the
% measurement can be deferred.}
% \end{quote}
% \end{xiaoenv}
% The behavior of a  $q$-query simulator can be described as follows. For $j \in [q]$, 
% \begin{itemize}
% \item
% Apply the local unitary $S_j$. $S_j$ is a unitary that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$; Intuitively, it represents the local operation $\Sim$ performs between two oracle queries. In particular, it computes and stores the type of the $j$-th query in register $\reg{u_j}$, possibly in superposition.
% \item
% Measure $\reg{u_j}$;
% \item
% Make the $j$-th oracle query according to the measurement outcome from the last step. Formally, we define this step as a unitary$O_{j}$ that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$ and $\reg{o}$. We present the formal definition of $O_{j}$ in \Cref{figbox:LOCC:3ZK:oracle}.
% \end{itemize}


% \begin{FigureBox}[label={figbox:LOCC:3ZK:oracle}]{Description of Unitary $O_j$}
% Each $O_j$ can be understood as unitary controlled on register $\reg{u_j}$. Formally, for each $j \in [q]$, $O_j$ is defined as follows 
% \begin{itemize}
% \item
% If $\reg{u_j}$ is of the form $\ket{\downarrow_1}_{\reg{u_j}}$, it applies $\tilde{U}_1$ on $\reg{m_1}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\uparrow_1}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_1$ on $\reg{m_1}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\downarrow_2}_{\reg{u_j}}$, it applies $\tilde{U}_2$ on $\reg{m_2}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\uparrow_2}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_2$ on $\reg{m_2}$ and $\reg{o}$.
% \end{itemize}
% \end{FigureBox}

% % is defined by a sequence of $q$ unitary operators $\Set{S_1,  \ldots, S_q}$. It proceeds as follows:
% % \begin{itemize}
% % \item
% % {\bf (First $q$ queries)} For $j\in [q]$, $\Sim$ repeats the following steps:
% % \begin{itemize}
% %  \item
% %  $\Sim$ first applies the ``local'' unitary $S_j$, which operates non-trivially on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$. 
% %  \item
% %  Then, controlled on the query type (possibly in superposition) stored in $\reg{u_j}$, the corresponding unitary is applied according to the rule described in \Cref{figbox:LOCC:3ZK:oracle}.
% %  \end{itemize} 

% % \item
% % {\bf (Final output.)} We denote by $\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho)$ the above execution; We denote by $\OUT(\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho))$ the output of $\tilde{\Verifier}$, i.e., final state in $\reg{out}$ tracing out all other registers after the execution
% % \end{itemize}
% \xiao{add a remark explaining two things: (1) $S_{j}$ only need to work on $\reg{u}_j$ and does not touch other $\reg{u}$ registers; (2) There's no need to add $S_{q+1}$ for $\Sim$'s post-processing, as the output will anyway trace $\Sim$'s registers out.}


% \subpara{$\Sim$ with Deferred Measurements.} Recall that a consequence of the deferred measurement principle is that {\em If after a measurement a qubit is used as a control qubit only, then the measurement can be deferred.} Also, observe in the above description of $\Sim$'s behavior that each $\reg{u_j}$ register is used {\em only} as a controlled register to determine the type of $O_j$. Thus, by the deferred measurement principle, we can equivalently describe $\Sim$ as the following two steps (assuming the starting state is $\ket{\eta_0}$):
% \begin{enumerate}
% \item
% Compute $\ket{\eta_q} \coloneqq O_q S_q O_{q-1} S_{q-1} \cdots O_1 S_1\cdot \ket{\eta_0}$.
% \item
% Measure registers $\reg{u_1},\ldots, \reg{u_q}$.
% \end{enumerate}
% From now on, we will use this deferred-measurement description of the simulator $\Sim$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comment some old materials
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% At a high-level, $\Sim$ can run $\tilde{\mathcal{V}}$ as a real prover, i.e., sending a message to $\tilde{\Verifier}$ and expecting $\tilde{\Verifier}$'s response (dubbed as ``down-queries''), or rewind $\tilde{\Verifier}$ (dubbed ``up-queries''). In the following, we formally define $\Sim$'s behavior. We also show in \Cref{figure:Sim-query:3-round} an exemplary execution of $\Sim$ where she makes 17 queries in total. We find it helpful to trace this concrete example while trying to understand the behavior of $\Sim$.
% \begin{figure}[!thb]
% \centering{
%     \fbox{
%          \includegraphics[width=0.5\textwidth]{figures/Three-round-real.jpg}
%     }         
% }
% \caption{An exemplary Query Pattern of $\Sim$}
% \label{figure:Sim-query:3-round}
% \end{figure}

% \subpara{Initialize $p_1$:} $\Sim$ starts by preparing a state in register $\reg{m_1}$ as her first message $p_1$. Formally, $\Sim$ applies a ``local'' unitary $S_0$ that works non-trivially on register $\reg{m_1}$ and $\reg{s}$. This yields a quantum state $p_1$ in $\reg{m_1}$ together with some residual internal state of $\Sim$ in $\reg{s}$. 


% \subpara{Obtain $v_1$:} $\Sim$ then queries $\tilde{\Verifier}$ to learn the response $v_1$. Formally, $\tilde{V}$ applies the unitary $\tilde{U}_3\tilde{U}_2\tilde{U}_1$ as defined earlier, which yields a state $v_1$ in register $\reg{m_1}$. This step is illustrated as the $\downarrow$ labeled by $\circled{1}$ in \Cref{figure:Sim-query:3-round}, and we say that the execution moves from Layer-1 to Layer-2.\footnote{It is worth noting that although both $p_1$ and $v_1$ are classical strings in the real execution, the simulator $\Sim$ may put a quantum state in $\reg{m_1}$ as her first message, and in that case, $\tilde{V}$'s response $v_1$ may also be a quantum state.} 


% \subpara{Subsequent Queries:} From now on, $\Sim$ can freely ask $\tilde{V}$ to perform $\tilde{U}$ or $\tilde{U}^\dagger$, and may modify the contains of $\reg{m_1}$ and $\reg{m_2}$ in between using her unitaries $S_1$, $S_2$, and $S_3$. Formally, $\Sim$ repeats the following procedure
% \begin{itemize}
% \item
% if the execution reaches Layer-$i$ (for $i \in [3]$), $\Sim$ will first apply the unitary $S_i$, and then measure the single-qubit register $\reg{q}$ \xiao{add this register when explaining $\Sim$'s registers} to decide if she wants to make a $\tilde{U}$ query or a $\tilde{U}^\dagger$ query. Depending on the query made, the execution will either move to Layer-$(i-1)$ (if a $\tilde{U}^\dagger$ query is made) or Layer-$(i+1)$ (if a $\tilde{U}$ query is made). 

% W.l.o.g., we use the following conventions. When the execution is at Layer-1 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\uparrow}$, then $\Sim$ aborts the execution immediately. Intuitively, this is because the execution is already rewound to the very beginning and it does not make sense to rewind it further; we simply view this as a failed simulation. Also, when the execution is at Layer-3 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\downarrow}$, then $\Sim$ terminates and announces the end of the simulation. Intuitively, Layer-3 represents the very end of the protocol and it does not make sense to continue to the next round; we simply view this as $\Sim$'s signal for the end of the simulation.
% \end{itemize}
% This procedure is best understood by tracing the example shown in \Cref{figure:Sim-query:3-round}. Consider the status of the execution right after the arrow $\circled{1}$. $\Sim$ then applies $S_2$ on $\reg{m_1}$ and $\reg{s}$ \xiao{probably on $\reg{m_2}$ as well?}, and measures $\reg{d}$. The situation shown in  \Cref{figure:Sim-query:3-round} corresponds to $\Sim$ decides to make a $\tilde{U}^\dagger$-query next (represented by arrow $\circled{2}$), which brings the execution back to Layer-1. $\Sim$ then applies $S_1$ on $\reg{m_1}$ and $\reg{s}$, and measures $\reg{d}$. By the assumption made above, $\Sim$ will make a $\tilde{U}$-query next, which brings the execution to Layer-2 (represented by arrow $\circled{3}$). 

% Another set of queries that deserve a closer look is from arrow $\circled{11}$ to arrow $\circled{12}$. They represent the following steps: Right after the $\tilde{U}$-query labeled by $\circled{10}$, $\Sim$ applies $S_3$ on $\reg{m_2}$ and $\reg{s}$, measures $\reg{q}$, and decides to make the  $\tilde{U}^\dagger$-query labeled by $\circled{11}$. This brings the execution to Layer-2. Then, $\Sim$ further rewinds the execution back to Layer-1 and ``jumps'' between Layer-1 and Layer-2 twice (as represented by arrow $\circled{12}$ to arrow $\circled{15}$). After that, $\Sim$ decides to go to Layer-3 as represented by arrow $\circled{16}$, which is the last query made by $\Sim$. That is, after applying $\circled{16}$, the measurement of $\reg{q}$ returns $\ket{\downarrow}$, indicating the end of the execution as we explained above. 


\subsection{Theorem Statement and Proof Outline}

\xiao{to do... As the title of the subsection indicates..}


\UpdateLine







\subsection{A Particular Malicious Verifier}
\label{sec:particular-mal-V}




\xiao{may need to explain the high-level picture: why are we defining $\tilde{V}$?} Similar as \cite{FOCS:CCLY21}, we first show the impossibility result with an inefficient $\tilde{V}$. The inefficiency is only due to a random function $H$ hard-wired in $\tilde{V}$. Jumping ahead, we will make $\tilde{V}$ efficient later (\xiao{Cref to sec}) by replacing $H$ with a $q$-wise independent hash.

\subsubsection{$\tilde{\Verifier}$'s registers}
\label{sec:CPM-3ZK:Vtil:registers} 
$\tilde{\Verifier}$ starts by initializing the following registers (see \Cref{figure:2-LOCC-V:registers} for an explanation \xiao{add a figure explaining the meaning fo the registers.}):
\begin{equation}\label[Expression]{2-LOCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{\vb{0}}_{\reg{p_1}}\ket{\vb{0}}_{\reg{v_1}}\ket{\vb{0}}_{\reg{p_2}}\ket{\vb{0}}_{\reg{v_2}} \ket{\vb{0}}_{\reg{m}} \ket{\bot}_{\reg{t_1}}\ket{\bot}_{\reg{t_2}} \ket{0}_{\reg{d}} \ket{\vb{0}}_\reg{w} \ket{H}_{\reg{aux}} 
\end{equation}








% In the impossibility result, we construct a BQP algorithm that runs both the simulator $\simulator$ and verifier $V$.
% Our entire purified view therefore consists of all above registers $\reg{ins, a,b,m,aux,w,adv}$. 


\subsubsection{$\tilde{V}$'s Unitary.} 
\label{sec:CPM-3ZK:Vtil:unitaries} 




\begin{xiaoenv}{Define the Counter}
Define the Counter

Both $\reg{gc}$ and $\reg{lc}$ registers are initialized to $0$. We set $C = 2^\secpar$,\footnote{We note that it suffices to set $C$ to any super-polynomial function on $\secpar$. We choose $2^\secpar$ only for concreteness.} and define the unitary $U_{gc}$ as the following mapping
 $$U_{gc} : 	\ket{i}_{\reg{gc}} \mapsto \ket{i+1 \mod C}_{\reg{gc}}.$$

 We also define the unitary to increase the local counter $U_{lc}$ as follows:
 $$U_{lc} : 	\ket{i}_{\reg{lc}} \mapsto \ket{i+1 \mod 4}_{\reg{lc}}.$$
 Note that modulus 4 is good enough for us, because we will show later that the local counter will always be in $\Set{1,2,3}$.
\end{xiaoenv}



We now desribe $\tilde{\Verifier}$'s unitary $\tilde{V}$. 


\begin{AlgorithmBox}[label={CPM-3ZK:V:unitary}]{Unitary \textnormal{$\tilde{V}$} for the Malicious Verifier \textnormal{$\tilde{\Verifier}$}}

{\bf Helper Unitaries.} Before we described $\tilde{V}$, we first define some helper unitaries. For each $i \in [2]$:
\begin{itemize}	
\item 
{\bf $A_i$: swap $\reg{p_i}$ and $\reg{m}$.} This unitary swaps the contents of $\reg{p_i}$ and $\reg{m}$.

\item 
{\bf $B_i$: apply $V$'s unitary.}
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then apply $V_{p_1, \ldots, p_i}$, which is the honest $\Verifier$'s unitary to generate $v_i$ from $p_i$.
\item
If $H(p_1, \ldots, p_i) = 0$, then do nothing; 
\end{itemize}


\item 
{\bf $C_i$: deliver $v_i$.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_i}$.
\item
If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_i}$.
\end{itemize}

\item 
{\bf $C'_i$: swap $\reg{m}$ and $\reg{t_i}$.} 
This unitary is the swap operator between registers $\reg{m}$ and $\reg{t_i}$.
% \item
% {\bf $C'_i$: swap $\reg{t_i}$ and $\reg{m}$.} This unitary swaps the contents of $\reg{t_i}$ and $\reg{m}$.

\item 
{\bf $D_i$: increase local counter.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
\item
If $H(p_1, \ldots, p_i) = 0$, then do nothing.
\end{itemize}
\end{itemize}

\para{$\tilde{\Verifier}$'s Unitary $\tilde{V}$.} On each query, it compares the global counter value $i$ with the local counter value $j$ and behaves accordingly. In particular:
\begin{description}
\item[Case $i = j$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $D_iC_iB_iA_i$ as defined above.
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}

\item[Case $(i \ne j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $C'_iA_i$ as defined above.
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}
\end{description}
\end{AlgorithmBox}

We first claim a fact regarding the global counter register.
\begin{enumerate}
\item \label[Fact]{item:fact:gc}
{\bf Fact 1:} Throughout the execution of $\Sim^{\tilde{\Verifier}}$, the global counter register will always contain a classical value.
\end{enumerate}
\xiao{add argument for \Cref{item:fact:gc}.}

% \para{Compare Counters.} On each query, $\tilde{\Verifier}$ first checks if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% \begin{enumerate}
% \item
% If $i \ne j$, then $\tilde{\Verifier}$ only applies $U_{gc}$ to increase the global counter, and does nothing else.
% \item
% If $i = j$, then $\tilde{\Verifier}$ first applies $U_{gc}$ to increase the global counter, and then behaves differently according to the value of the global counter $i$. We describe it in the following.
% \end{enumerate}

% \para{Global Counter $i = 1$.} This corresponds to $\tilde{\Verifier}$'s behavior for the 1st slot, namely generating $v_1$ as the response to the $p_1$ she just received form the $\Prover$. $\tilde{\Verifier}$ applies $\tilde{V}_1$, which is defined as follows
% $$\tilde{V}_1 \coloneqq D_1 C_1 B_1 A_1, $$
% \xiao{old name: $\tilde{V}_1 \coloneqq \tilde{U}_3 \tilde{U}_2 \tilde{U}_1,$}
% with the unitaries defined as follows:
% \begin{enumerate}
% % \item
% % {\bf ($\tilde{U}_{\msf{c}}$: Increase the Counter.)} This unitary maps $\ket{i}_{\reg{count}}$ to $\ket{i+1 \mod 2}_{\reg{count}}$.

% \item \label{item:Vtil:unitary:1-1}
% {\bf ($A_1$: Swap $\reg{p_1}$ and $\reg{m}$.)} This unitary swaps the contents of $\reg{p_1}$ and $\reg{m}$ registers.
% \begin{MyComment}
% In the real execution, this steps is for $\tilde{V}$ to move the first message it received from the prover (in the $\reg{m_1}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_1}$), so that it can perform computation in subsequent steps.
% \end{MyComment}

% \item \label{item:Vtil:unitary:1-2}
% {\bf ($B_1$: Apply $V$'s Unitary.)}
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then do nothing; \xiao{need to recall where $p_1$ is stored.}
% \item
% If $H(p_1) = 1$, then apply $\sum_{p_1} \ketbra{p_1} \tensor V_{p_1}$, which is the honest $\Verifier$'s unitary to generate $v_1$ from $p_1$.
% \end{enumerate}
% \begin{MyComment}
% Recall \xiao{from XXX} that $U$ can be written in the form of $\sum_{p_1} \ketbra{p_1}\tensor U_{p_1}$ because the concerned protocol is LOCC. $V_{p_1}$ works non-trivially on registers $\reg{ins}$, $\reg{v_2}$, and $\reg{w}$. In particular, it generates $V$'s message $v_1$ in register $\reg{v_1}$ (together with some residual state on $\reg{w}$).
% \end{MyComment}


% \item \label{item:Vtil:unitary:1-3}
% {\bf ($C_1$: Deliver $v_1$.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% \item
% If $H(p_1) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_1}$.
% % set the content in register $\reg{m}$ to $\ket{v_1 \xor m}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_1$ is the content in register $\reg{v_1}$. 
% \end{enumerate}


% \item \label{item:Vtil:unitary:1-4}
% {\bf ($D_1$: Increase Local Counter.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then do nothing.

% \item
% If $H(p_1) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
% \end{enumerate}
% \end{enumerate}


% \para{Global Counter $i = 2$.} This corresponds to $\tilde{\Verifier}$'s behavior for the 2nd slot, namely generating $v_2$ as the response to the $p_2$ she just received form the $\Prover$. $\tilde{\Verifier}$ applies $\tilde{V}_2$, which is defined as follows
% $$\tilde{V}_2 \coloneqq D_2C_2B_2A_2, $$
% \xiao{old name: $\tilde{V}_2 \coloneqq \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,$}
% with the unitaries defined as follows:

% % This corresponds to $\tilde{\Verifier}$'s behavior for the 2nd slot, namely generating $v_2$ as the response to the $p_2$ she just received form the $\Prover$. This case is different from the above case of the 1st slot---$\tilde{\Verifier}$ will first query the oracle $H$ on input $p_1$ stored in the register $\reg{p_1}$, and behaves differently according to the answer from $H$. \xiao{(need to add a remark: technically, we need to first compute the output of $H$, then do the following computation, and then un-compute $H$?)} In particular, we need to consider the following two sub-cases:
% % \begin{enumerate}
% % \item \label[Case]{item:CPM-3ZK:Vtil:slot-2:bad}
% % If $H(p_1) = 0$, then $\tilde{\Verifier}$ does not do anything. Equivalently, $\tilde{V}_2$ is defined as
% %  $$\tilde{V}_2 \coloneqq I.$$

% % \item \label[Case]{item:CPM-3ZK:Vtil:slot-2:good}
% % Otherwise (i.e., $H(p_1) = 1$), then $\tilde{V}_2$ is defined as
% % $$\tilde{V}_2 \coloneqq \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,$$ 
% % with the unitaries defiend as follows:

% % \end{enumerate}
% \begin{enumerate}
% \item \label{item:Vtil:unitary:2-1}
% {\bf ($A_2$: Swap $\reg{p_2}$ and $\reg{m}$.)} This unitary swaps the contents of $\reg{p_2}$ and $\reg{m}$ registers.

% \begin{MyComment}
% In the real execution, this steps is for $\tilde{V}$ to move the $p_2$ message it received from the prover (in the $\reg{m_2}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_2}$), so that it can perform computation in the next step.
% \end{MyComment}

% \item \label{item:Vtil:unitary:2-2}
% {\bf ($B_2$: $\tilde{\Verifier}$'s Decision.)} This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then do nothing. \xiao{need to recall where $(p_1,p_2)$ are stored.}

% \item
% If $H(p_1, p_2) = 1$, then apply $\sum_{p_2} \ketbra{p_2} \tensor V_{p_2}$, which is the honest $\Verifier$'s unitary to generate $v_2$ from $p_2$.
%  % it applies $U_\msf{d}$, where  $U_\msf{d}$ is the honest verifier's decision unitary. \xiao{If necessary, we can decompose $U_\msf{d}$ as $U_{\msf{d}} \coloneqq \sum_{p_1, v_1, p_2}\ketbra{p_1, v_1, p_2} \tensor U_{p_1, v_1, p_2}$.}
% \end{enumerate}
% % \begin{MyComment}
% % Recall that $U_\msf{d}$ works non-trivially on registers $\reg{ins}$, $\reg{p_1}$, $\reg{v_1}$, $\reg{p_2}$, $\reg{d}$, and $\reg{w}$. In particular, it generates $V$'s final decision bit in register $\reg{d}$ (together with some residual state on $\reg{w}$).
% % \end{MyComment}



% \item \label{item:Vtil:unitary:2-3}
% \xiao{Add this to make the writing of my proof consistent event at the `last layer' (i.e., \Cref{lem:CPM-3ZK-hyb02:proof:invariant}). This essentially allows Sim to see the verifier's final decision bit, which is a weaker notion of ZK. this makes our impossibility result stronger.} 

% {\bf ($C_2$:  Deliver $v_2$.)} This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% \item
% If $H(p_1, p_2) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_2}$.
% % set the content in register $\reg{m}$ to $\ket{v_2 \xor m}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_2$ is the content in register $\reg{v_2}$. 
% % then sets the content in register $\reg{m_2}$ to $\ket{d \xor m}_{\reg{m_2}}$, where $m$ is the original content in register $\reg{m_2}$ and $d$ is the content in register $\reg{d}$.
% \end{enumerate}

% \item \label{item:Vtil:unitary:2-4}
% {\bf ($D_2$: Increase Local Counter.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then do nothing.

% \item
% If $H(p_1, p_2) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
% \end{enumerate}

% \end{enumerate}



% \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.



\xiao{Add a lemma stating that for all $x\in \Lang$, the execution between the honest $\Prover$ and $\tilde{\Verifier}$ will lead to acceptance with probability $\epsilon^2$. This proof is simply, but it helps the reader to understand our model. Also, I want to high-light that in the real execution, \Cref{item:CPM-3ZK:Vtil:slot-2:good} will always be triggered.	}






\subsection{$\BQP$ Decider}

\para{MnR Game with ZK Simulator.} We first define the measure-and-reprogram (MnR) game w.r.t. the simulator $\Sim$ and $\tilde{\Verifier}(x)$ defined in previous sections. This game is simply an instantiation of MnR game defined in \Cref{MnR:lem:game} with the following notation: 
\begin{enumerate}
\item \label{CPM-3ZK:MnR:notation:item:1}
We treat the execution of the simulator (with oracle access to $\tilde{V}$ and $\tilde{V}^\dagger$) as an oracle machine $\Sim^{\tilde{\Verifier}}$ that has quantum oracle access to a random function $H: \mcal{X}^{\le 2} \rightarrow \mcal{Y}$, where $\mcal{X}=\bits^\ell$ and $\mcal{Y} = \bits$. Let $\vb{y} = (y_1, y_2) \in \mcal{Y}^2$.

\item \label{CPM-3ZK:MnR:notation:item:2}
Recall that the output of  $\Sim^{\tilde{\Verifier}}$ is defined to be the output $\tilde{\Verifier}$ at halt, which is in turn defined to be all the internal registers of $\tilde{\Verifier}$. We will split $\tilde{\Verifier}$'s output as $(\vb{p} = (p_1, p_2), \rho_{\msf{out}})$,  where $\vb{p}$ is the string contained in the $\reg{p_1}$ and $\reg{p_2}$ registers, and $\rho_{\msf{out}}$ is the remaining state tracing out $\reg{p_1}$ and $\reg{p_2}$. In particular, $\rho$ contains the global counter register $\reg{gc}$ and register $\reg{d}$ that contains $\tilde{\Verifier}$'s final decision (qu)bit. 

\item \label{CPM-3ZK:MnR:notation:item:3}
We assume that $\Sim^{\tilde{\Verifier}}$ as an oracle machine makes $q$ queries to $H$ in total.
\end{enumerate}

Since this game will be particularly important for the sequel sections, we choose to present it in full detail in \Cref{CPM-3ZK:MnR:game}.


\begin{GameBox}[label={CPM-3ZK:MnR:game}]{Measure-and-Reprogram Game \textnormal{$\Sim^{\tilde{\Verifier}}[H, \vb{y}]$}}
 It works as follows
\begin{enumerate}
\item \label[Step]{CPM-3ZK:MnR:game:step:1}
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$  conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$.

\item \label[Step]{CPM-3ZK:MnR:game:step:2}
    Let $s$ denote the number of $j_i$'s in $\Set{j_i}_{i \in [k]}$ that are not $\bot$.  We re-label the indices $i$ for pairs $\Set{(j_i, b_i)}_{i \in [k]}$ so that $j_1 < j_2 < \ldots < j_s$ and $j_{s+1} = j_{s+2} =\ldots = j_k = \bot$.

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes $H$, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item If $j=j_i$ for some $i\in[2]$, measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, 2_i})$ where $2_i\leq 2$ is determined by the measurement outcome, and then behaves according to the value $b_i$ as follows:
        \begin{enumerate}
        \item 
        If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$, and then answer the $j_i$-th query using the reprogrammed oracle. 
        \item 
        If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$. 
        \end{enumerate}
    \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [2]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{CPM-3ZK:MnR:notation:item:2}).

\item
For all $i \in [2]$ such that $j_i = \bot$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}_i \coloneqq (p^*_1, \ldots, p^*_i)$. 

\item
{\bf Output:} The output of this game is defined as follows
\begin{itemize}
\item
If it holds for all $i \in [2]$ that $\vb{p}_i$ is a prefix of $\vb{p}_2$, then output $(\vb{p}_2, \rho_{\msf{out}})$;

\item
Otherwise, output $(\bot, \bot)$.
\end{itemize}
\end{enumerate}
\end{GameBox}

\para{Decider for $\BQP$.} We now define the $\BQP$ decider $\mcal{B}$ in \Cref{CPM-3ZK:BQP-decider}.
\begin{AlgorithmBox}[label={CPM-3ZK:BQP-decider}]{\textnormal{$\BQP$} Decider $\mcal{B}(x)$}
On input a classical string $x$, machine $\mcal{B}(x)$ works as follows:
\begin{enumerate}
\item
{\bf (Parameter Setting.)}
Let $\vb{1} \coloneqq (1,1)$. Let $\mcal{M} \coloneqq \bits^{\ell}$ and $H_0 :\mcal{M}^{\le 2} \ra \bits$ be the zero-function, i.e., $H_0(p_1, \ldots, p_i) = 0$ for all $(p_1, \ldots, p_i) \in \mcal{M}^{\le 2}$.

\item
{\bf (MnR Game with $\Sim^{\tilde{V}}$.)} Execute $(\vb{p} = (p_1, p_2), \rho) \la \Sim^{\tilde{V}}[H_0, \vb{1}]$ as per \Cref{CPM-3ZK:MnR:game}. 
% and let $\hat{H}_0$ denote the oracle at halt (i.e., the re-programmed oracle). 
 That is, $\mcal{B}(x)$ executes \Cref{CPM-3ZK:MnR:game} with $H \coloneqq H_0$ and $\vb{y} \coloneqq (1,1)$ and  denotes the output of this procedure as $(\vb{p} = (p_1, p_2), \rho)$.
% , and denotes the oracle at the end of the MnR game as $\hat{H}_0$.
 Note that in this step, $\mcal{B}$ makes use of its input $x$, which is used as the input instance to $\tilde{V}$ (though we did not include it in the notation explicitly).

\item
{\bf (Output.)} It outputs 1 if and only if $\msf{Pred}(\rho) = 1$, where $\msf{Pred}(\rho)$ is a (quantum) predicate that outputs 1 if and only if all of the following conditions hold:
\begin{enumerate}
% \item
% $\hat{H}_0(p_1) = 1$ and $\hat{H}_0(p_1, p_2) = 1$. (Recall that $p_1$ and $p_2$ are contained in $\vb{p}$.)

\item
% The value contained in the global counter register $\reg{gc}$ is 2. (Recall that the $\reg{gc}$ register is contained in $\rho$ and remains classical throughout the whole execution.)
Measure the local counter register $\reg{lc}$ in the computational basis and the measurement outcome is 1. (Recall that the $\reg{lc}$ register is contained in $\rho$.)
\item
Measure register $\reg{d}$ in the computational basis and the measurement outcome is 1. (Recall that the $\reg{d}$ register is also contained in $\rho$.)
\end{enumerate}
\end{enumerate}
\end{AlgorithmBox}


Next, we argue that $\mcal{B}$ is a valid $\BQP$ decider. Toward that, it suffices to establish the following \Cref{CPM-3ZK:decider:lem:completeness,CPM-3ZK:decider:lem:soundness}.

\begin{lemma}[Completeness]\label{CPM-3ZK:decider:lem:completeness}
\xiao{(need to talk about $\epsilon \le \epsilon_q = \frac{1}{256k^2q^2(4kq+1)^{2k}}$ in this lemma.)}
For all $\Lang \in \BQP$ and all $x \in \Lang \cap \bits^{\secpar}$, it holds for the $\mcal{B}$ defined in \Cref{CPM-3ZK:BQP-decider} that
$$\Pr[\mcal{B}(x) = 1] \ge \frac{1}{8 \cdot (4kq + 1)^{2k}} -\negl(\secpar).$$
\xiao{need to change $k$ to 2 in this special case.}
\end{lemma}


\begin{lemma}[Soundness]\label{CPM-3ZK:decider:lem:soundness}
For all $\Lang \in \BQP$ and all $x \in \bits^{\secpar} \setminus \Lang$, it holds for the $\mcal{B}$ defined in \Cref{CPM-3ZK:BQP-decider} that
$$\Pr[\mcal{B}(x) = 1] = \negl(\secpar).$$
\xiao{need to change $k$ to 2 in this special case.}
\end{lemma}

We present the proof for \Cref{CPM-3ZK:decider:lem:completeness} in \Cref{sec:CPM-3ZK:decider:lem:completeness:proof}. 

The proof for \Cref{CPM-3ZK:decider:lem:soundness} is one of the most technically involved part of this work, and thus we put it in a separate section in \Cref{sec:CPM-3ZK:decider:lem:soundness:proof}.


\subsection{Proof of Completeness}
\label{sec:CPM-3ZK:decider:lem:completeness:proof}

\xiao{need to modify $k$ to $2$.}

In this subsection, we prove \Cref{CPM-3ZK:decider:lem:completeness}.

First, notice that 
\begin{align}
\Pr[\mcal{B}(x) = 1] 
& = 
\Pr[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_0, \vb{1}]] \label{CPM-3ZK:decider:lem:completeness:proof:sparsity:1} \\ 
& \ge 
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]] - 32k^2q^2\epsilon \label[Inequality]{CPM-3ZK:decider:lem:completeness:proof:sparsity:2} 
\end{align}
where \Cref{CPM-3ZK:decider:lem:completeness:proof:sparsity:1} follows from the definition and notation in \Cref{CPM-3ZK:BQP-decider}, and \Cref{CPM-3ZK:decider:lem:completeness:proof:sparsity:2} follows from \Cref{lem:ind-sparse-and-zero}. 
% (In \Cref{CPM-3ZK:decider:lem:completeness:proof:sparsity:2}, the predicate $\msf{Pred}^{\hat{H}_\epsilon}$ works in the same manner as the $\msf{Pred}^{\hat{H}_0}$ defined in \xiao{Cref} , except that it replaces $\hat{H}_0$ with $\hat{H}_\epsilon$.)

\subpara{Additional Notation.} In the following, we make use of the following notation:
\begin{itemize}
\item
For any classical oracle $H$, we use $\msf{SIM}^{H}$ to refer to the execution of $\Sim^{\tilde{\Verifier}}$ where $\tilde{\Verifier}$ uses $H$ as the oracle. 

\item
When we write $\bs{\beta}$ in the subscribe of the $\Pr$ symbol, it means we sample $\bs{\beta}$ from a distribution $D_\epsilon$ over $\bits^2$, whose each coordinate takes 1 with probability $\epsilon$ independently. 

\item
For a function $H: \mcal{M}^{\le 2} \ra \mcal{Y}$ and a vector $\vb{p} = (p_1, p_2) \in \mcal{M}^2$,  let $\bar{H}(\vb{p}) \coloneqq  \big(H(p_1), H(p_1, p_2) \big)$.

\item
The bold-face $\vb{1}$ is defined to be $(1, 1)$.
\end{itemize}
With the above notation, it holds that:
\begin{align*}
& \Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]] \\  
=~&  
\sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}   \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]]  \numberthis \label{CPM-3ZK:decider:lem:completeness:proof:final:1} \\ 
\ge~& 
\frac{1}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \msf{SIM}^{H^{\vb{p}^*, \vb{1}}_\epsilon}] \numberthis \label{CPM-3ZK:decider:lem:completeness:proof:final:2} \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon, \bs{\beta}}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 \wedge \bs{\beta} = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H^{\vb{p}^*, \bs{\beta}}_\epsilon}] \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \Pr_{H_\epsilon}[ \msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \numberthis \label{CPM-3ZK:decider:lem:completeness:proof:final:3} 
,\end{align*}
where \Cref{CPM-3ZK:decider:lem:completeness:proof:final:1} follows from the Law of Total Probability, \Cref{CPM-3ZK:decider:lem:completeness:proof:final:2} follows from \Cref{MnR:lem},  and \Cref{CPM-3ZK:decider:lem:completeness:proof:final:3} follows again from the Law of Total Probability.

Next, we bound the RHS of \Cref{CPM-3ZK:decider:lem:completeness:proof:final:3} via the ZK guarantee for simulator $\Sim$. First, recall that \xiao{This probably should be a lemma appeared earlier.} the honest $\Prover$ will make $\tilde{\Verifier}^{H_\epsilon}$ accept with probability $\epsilon^k$. That is,
\begin{equation}\label{CPM-3ZK:decider:lem:completeness:proof:final:4}
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1}~:~ (\vb{p}, \rho) \la \msf{OUT}_{\tilde{\Verifier}}\big(\langle \Prover(w), \tilde{\Verifier}^{H_\epsilon} \rangle(x)\big)] = \epsilon^k,
\end{equation}
where we used the fact that by definition,  $\tilde{\Verifier}^{H_\epsilon}$ accepts if the $\reg{lc}$ register contains 2, the decision register $\reg{d}$ contains 1, and the transcript $(p_1, p_2)$ satisfies $H_\epsilon(p_1) = 1$ and $H_\epsilon(p_1, p_2) = 1$. 

It then follows from \Cref{CPM-3ZK:decider:lem:completeness:proof:final:4} and the ZK property that 
\begin{equation}\label{CPM-3ZK:decider:lem:completeness:proof:final:5}
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1}~:~ (\vb{p}, \rho) \la (\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \ge \epsilon^k - \negl(\secpar) \ge \frac{\epsilon^k}{4} - \negl(\secpar).
\end{equation}

In summary, it holds that 
\begin{align*}
\Pr[\mcal{B}(x) = 1] 
& \ge 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \bigg(\frac{\epsilon^k}{4} - \negl(\secpar) \bigg) - 32k^2q^2\epsilon \numberthis \label[Inequality]{CPM-3ZK:decider:lem:completeness:proof:final:6} \\ 
& \ge 
\frac{1}{4(4kq+1)^{2k}} - \negl(\secpar) - 32k^2q^2\epsilon \numberthis \label[Inequality]{CPM-3ZK:decider:lem:completeness:proof:final:7} \\ 
& \ge
\frac{1}{8(4kq+1)^{2k}} - \negl(\secpar) 
,\end{align*}
where \Cref{CPM-3ZK:decider:lem:completeness:proof:final:6} follows from  \Cref{CPM-3ZK:decider:lem:completeness:proof:sparsity:2}, \Cref{CPM-3ZK:decider:lem:completeness:proof:final:3}, and \Cref{CPM-3ZK:decider:lem:completeness:proof:final:5}, and \Cref{CPM-3ZK:decider:lem:completeness:proof:final:7} follows from our parameter setting that $\epsilon \le \epsilon_q = \frac{1}{256k^2q^2(4kq+1)^{2k}}$. \xiao{need to talk about $\epsilon_q$ in the lemma.}

This completes the proof of \Cref{CPM-3ZK:decider:lem:completeness}.







% \section{Warm Up: Three-Round BBZK in the CPM Model (Part 2/3)  (Old Version)}
% \label{sec:CPM-3ZK:decider:lem:soundness:proof}

% In this section, we prove \Cref{CPM-3ZK:decider:lem:soundness}. 

% At a high level, we assume for contradiction that  \Cref{CPM-3ZK:decider:lem:soundness} is false and show how to construct a malicious prover $\tilde{\Prover}$ breaking the soundness of the original LOCC ZK protocol. Toward that, we first need to make some modifications to the machine $\mcal{B}$ and the MnR game $\Sim^{\tilde{\Verifier}}$, making use of some particular properties of the $\tilde{\Verifier}$ we defined earlier. This is done in \xiao{cref}. Next, we will present the malicious prover $\tilde{\Prover}$ and prver that it can indeed break the soundness. This is done in \xiao{cref}.

% \subsection{Preparation}
% \subsubsection{Restating the MnR Game}
% In \Cref{CPM-3ZK:MnR:game:modify:1}, we present a modified version of the MnR game $\Sim^{\tilde{\Verifier}}[H, \vb{y}]$ defined in \Cref{CPM-3ZK:MnR:game}. Since we will be interested only in the case $H = H_0$ and $\vb{y} = \vb{1} = (1, 1)$, we present this case only. We highlight its difference with \Cref{CPM-3ZK:MnR:game} in \red{red color}.


% \begin{GameBox}[label={CPM-3ZK:MnR:game:modify:1}]{Measure-and-Reprogram Game \textnormal{$\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$}}
%  It works as follows
% \begin{enumerate}
% \item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:1}
% For each $i\in[2]$, uniformly pick \dlt{$(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$} \red{$(j_i,b_i)\in [q]\times \bits$} conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. \red{It re-label the tuples $\Set{(j_i, b_i)}_{i \in [2]}$ to make sure that $j_1 < j_2$.} \red{It also defines an empty vector $\vb{p}_0 = \emptyset$.}

% \item
% Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes \red{$H_0$}, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
% \begin{enumerate}
%       \item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:2:a} 
%       If $j=j_i$ for some $i\in[2]$, \dlt{measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, 2_i})$ where $2_i\leq 2$ is determined by the measurement outcome,} \red{measure this query to obtain  $\vb{p}_i=(p_{i,1}, \ldots,p_{i, i})$.} \red{If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_i$, the execution halts immediately and outputs $(\bot, \bot)$.}
%       \red{\begin{itemize}
%       \item
      
%       {\bf Defining $\msf{sq}(i)$:} Note that the $j_i$-th query to $\mcal{O}$ must be invoked by $\Sim$'s query to $\tilde{\Verifier}$. We will call this $\Sim$'s query (that invokes the $j_i$-th query to $\mcal{O}$) as the $i$-th special query and denote it by $\msf{sq}(i)$. We establish certain properties of $\msf{sq}(i)$ in \Cref{CPM-3ZK:MnR:game:modify:1:lem}, which will be useful later. 
%       \end{itemize}
%       }

%       It then behaves according to the value $b_i$ as follows:
%         \begin{enumerate}
%         \item 
%         If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$, and then answer the $j_i$-th query using the reprogrammed oracle. 
%         \item 
%         If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$. 
%         \end{enumerate}
%     \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [2]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
%     \end{enumerate}

% \item
% Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{CPM-3ZK:MnR:notation:item:2}).

% \item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:4}
% \dlt{For all $i \in [2]$ such that $j_i = \bot$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}^*_i \coloneqq (p^*_1, \ldots, p^*_i)$.} 

% \item \label[Step]{CPM-3ZK:MnR:game:modify:1:step:5}
% {\bf Output:}  \red{Output $(\vb{p}_2, \rho_{\msf{out}})$.}
% \begin{itemize}
% \item
% \dlt{If it holds for all $i \in [2]$ that $\vb{p}_i$ is a prefix of $\vb{p}_2$, then output $(\vb{p}_2, \rho_{\msf{out}})$;}

% \item
% \dlt{Otherwise, output $(\bot, \bot)$.}
% \end{itemize}
% \end{enumerate}
% \end{GameBox}

% \begin{lemma}\label{CPM-3ZK:MnR:game:modify:1:lem}
% For the $\dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ defined in \Cref{CPM-3ZK:MnR:game:modify:1} and the $\mcal{B}(x)$ defined in \Cref{CPM-3ZK:BQP-decider}, it holds that
% $$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]]\ge \Pr[\mcal{B}(x) = 1].$$
% Moreover, for the $\msf{sq}(i)$ $(\forall i \in [2])$ defined in \Cref{CPM-3ZK:MnR:game:modify:1:step:2:a}, it enjoys the following properties:
% \begin{itemize}
% \item
% Query $\msf{sq}(i)$ is a $\tilde{V}$-query (instead of being a $\tilde{V}^\dagger$-query).
% \item
% \xiao{to be added as needed.}
% \end{itemize}
% \end{lemma}
% \begin{proof}
% 	\begin{xiaoenv}{Polish the language}
% 	The proof of this lemma follows from the way we set counters.

% 	Need to explain the order $j_1 < j_2$.

% 	Next, we argue that the change in \Cref{CPM-3ZK:MnR:game:modify:1:step:1} does not decrease the accepting probability of the predicate. To see that, notice that we start with an all-$0$ function $H_0$, and the whole MnR game $\Sim^{\tilde{\Verifier}}[H_0, \vb{1}]$ measures at most 2 queries in total. Therefore, if there is a tuple $(j_i, b_i) = (\bot, \bot)$, then at most one query can be measured. Also, due to the way we set the global and local counters, it is clear that the measurement will not output $(p_1, p_2)$ unless an ealier measurement has output $(p_1)$. That is, the measured queries will appear in a length-increasing order. Thus, if only one query corresponds to $H_0$ being programmed at (at most) a single point $p_1$ (to output 1). This cannot bring the local counter to $2$. In this case, $\msf{Pred}(\rho)$ will always output 0. Thus, it will not decrease the winning probability by delete $\Set{(\bot, \bot)}$ from the support of $(j_i, b_i)$. 

% 	Also, note that if $(j_i, b_i)$ does not take the value $(\bot, \bot)$, the condition in \Cref{CPM-3ZK:MnR:game:modify:1:step:4} will never be satisfied. Thus, we can safely delete  \Cref{CPM-3ZK:MnR:game:modify:1:step:4} as well.

% 	The modification in \Cref{CPM-3ZK:MnR:game:modify:1:step:2:a} is simply to say that the first measurement generate $(p'_1)$ and the second measurement generate $(p'_1, p'_2)$. We have argued this in the above.

% 	Also, as long as the measured queries appear in a length-increasing order, the modification in	\Cref{CPM-3ZK:MnR:game:modify:1:step:5} becomes only cosmetic.
% 	\end{xiaoenv}

% This completes the proof of \Cref{CPM-3ZK:MnR:game:modify:1:lem}.

% \end{proof}


% \para{Looking into $\Sim^{\tilde{\Verifier}}$.} Next, we re-state the game $\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$ defined in \Cref{CPM-3ZK:MnR:game}. This time, we will look into the execution of $\Sim^{\tilde{\Verifier}}$ and their registers. This is different from previous games where we always treat $\Sim^{\tilde{\Verifier}}$ as a ``black-box'' and only focus on how it accesses the oracle $H_0$. We denote this game as $\msf{Real}(\Sim, \tilde{\Verifier})$ and present it in \Cref{CPM-3ZK:MnR:game:real}.	

% It is straightforward that \Cref{CPM-3ZK:MnR:game:real} is identical to \Cref{CPM-3ZK:MnR:game} with only cosmetic changes. Therefore, it holds that
% \begin{equation}\label{CPM-3ZK:MnR:to:real:ind-eq}
% \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].
% \end{equation}



% \begin{GameBox}[label={CPM-3ZK:MnR:game:real}]{Game \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier})$}}
% For each $i\in[2]$, uniformly pick $(j_i,b_i)\in [q]\times \bits$ conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. W.l.o.g., we assume that $j_1 < j_2$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner for each $i \in [2]$. 

% \para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with $\tilde{V}$ and $\tilde{V}^\dagger$ accordingly, where $\tilde{\Verifier}$ uses $H^{(i-1)}_0$ as the oracle.


% \para{For Query $\msf{sq}(i)$:} Note that by \Cref{CPM-3ZK:MnR:game:modify:1:lem}, $\msf{sq}(i)$ is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.	Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and behaves according to the value $b_i$ as follows:
% \begin{enumerate}
% \item 
%         If $b_i=0$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i)}_0$ as the oracle.
% . 

% \item 
%         If $b_i=1$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i-1)}_0$ as the oracle.
% \end{enumerate}


% \para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Real}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_2, \rho_{\msf{out}})$.

% \end{GameBox}


% \subsubsection{A Dummy Game} 

% \para{A Dummy Version of $\tilde{\Verifier}$.} We first define a unitary $\ddot{V}$, which should be treated as the ``dummy version'' of $\tilde{\Verifier}$'s unitary $\tilde{V}$. We present it in \Cref{CPM-3ZK:V-dummy}, highlighting its difference with $\tilde{V}$ (defined in \Cref{CPM-3ZK:V:unitary}) in \red{red color}.
% \begin{AlgorithmBox}[label={CPM-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}
% {\bf Helper Unitaries.} We first define additional helper unitaries. For each $i \in [2]$:
% \begin{itemize}
%  \item
% {\bf $\ddot{C}_i$: swap $\reg{m}$ and $\reg{t_i}$.} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1, \ldots, p_i) = 1$, \red{then do nothing}. 
% \item
% If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{t_i}$ and $\reg{m}$.
% \end{itemize}
%  \end{itemize} 

% \para{Unitary $\ddot{V}$.} On each query, it compares the global counter value $i$ with the local counter value $j$ and behaves accordingly. In particular:
% \begin{description}
% \item[Case $(i = j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
% \begin{itemize}
% \item
% If $i \in [2]$, then it applies $D_i\red{\ddot{C}_i}A_i$, where $A_i$ and $D_i$ is  defined in \Cref{CPM-3ZK:V:unitary} and $\ddot{C}_i$ is defined above.
% \item
% Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
% \end{itemize}

% \item[Case $(i \ne j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
% \begin{itemize}
% \item
% If $i \in [2]$, then it applies $C_iA_i$, where $A_i$ and $C_i$ is  defined in \Cref{CPM-3ZK:V:unitary}
% \item
% Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
% \end{itemize}
% \end{description}
% \end{AlgorithmBox}




% % \begin{AlgorithmBox}[label={CPM-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}


% % \para{Compare Counters.} On each query, check if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% % \begin{itemize}
% % \item
% % If $i \ne j$, then apply $U_{gc}$ to increase the global counter, and do nothing else.
% % \item
% % If $i = j$, then first apply $U_{gc}$ to increase the global counter, and then behave differently according to the value of the global counter $i$. We describe it in the following.
% % \end{itemize}

% % \para{Global Counter $i = 1$.} Apply $\ddot{V}_1 \coloneqq D_1 \red{\ddot{C}_1} A_1$, where $D_1$ and $A_1$ are the same as for $\tilde{V}$ and $\ddot{C}_1$ is defined as follows:
% % \begin{itemize}
% % \item
% % {\bf ($\ddot{C}_1$: Swap $\reg{m}$ and $\reg{t_1}$.)} 
% % This unitary perform the following operation in superposition:
% % \begin{itemize}
% % \item
% % If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% % \item
% % If $H(p_1) = 1$, \red{then do nothing}. 
% % \end{itemize}

% % \end{itemize}


% % \para{Global Counter $i = 2$.} Apply $\ddot{V}_2 \coloneqq D_2 \red{\ddot{C}_2} A_2$,
% % where $D_2$ and $A_2$ are the same as for $\tilde{V}$ and $\ddot{C}_2$ is defined as follows:
% % \begin{itemize}

% % \item 
% % {\bf ($\ddot{C}_2$: Swap $\reg{m}$ and $\reg{t_2}$.)} 
% % This unitary perform the following operation in superposition:
% % \begin{itemize}
% % \item
% % If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% % \item
% % If $H(p_1, p_2) = 1$, \red{then do nothing}. 
% % \end{itemize}

% % \end{itemize}

% % \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.

% % \end{AlgorithmBox}


% \para{A Dummy MnR Game.} We now define another game $\msf{Dummy}(\Sim, \tilde{\Verifier})$. This game will essentially serve as a malicious prover $\tilde{\Prover}$ that could break the soundness of the original ZK protocol, leading to our desired contradiction. Intuitively, $\msf{Dummy}(\Sim, \tilde{\Verifier})$ behaves identical to $\msf{Real}(\Sim, \tilde{\Verifier})$ except for that it answers $\Sim$'s queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$ using the dummy version of $\tilde{\Verifier}$ as we defined in \Cref{CPM-3ZK:V-dummy}. We present the game in \Cref{CPM-3ZK:MnR:game:dummy} and highlight its difference $\msf{Real}(\Sim, \tilde{\Verifier})$ (in \Cref{CPM-3ZK:MnR:game:real}) in \red{red color}. 
% \begin{GameBox}[label={CPM-3ZK:MnR:game:dummy}]{Game \textnormal{$\msf{Dummy}(\Sim, \tilde{\Verifier})$}}
% For each $i\in[2]$, uniformly pick $(j_i,b_i)\in [q]\times \bits$ conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. W.l.o.g., we assume that $j_1 < j_2$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner for each $i \in [2]$. 

% \para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with \red{$\ddot{V}$} and \red{$\ddot{V}^\dagger$} accordingly, using $H^{(i-1)}_0$ as the oracle. (Note that \red{$\ddot{V}$} is defined in \Cref{CPM-3ZK:V-dummy}.)


% \para{For Query $\msf{sq}(i)$:} Note that by \Cref{CPM-3ZK:MnR:game:modify:1:lem}, $\msf{sq}(i)$ is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.	Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and behaves according to the value $b_i$ as follows:
% \begin{enumerate}
% \item 
%         If $b_i=0$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i)}_0$ as the oracle.
% . 

% \item 
%         If $b_i=1$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i-1)}_0$ as the oracle.
% \end{enumerate}


% \para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Dummy}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_2, \rho_{\msf{out}})$.

% \end{GameBox}
% The following is the most involved lemma in this section. We defer its proof to \xiao{Cref}, before which we first show (in \xiao{Cref}) how to finish the current proof of \Cref{CPM-3ZK:decider:lem:soundness} assuming that \Cref{CPM-3ZK:MnR:game:dummy:lem} holds.


% \begin{lemma}\label{CPM-3ZK:MnR:game:dummy:lem}
% For the $\msf{Dummy}(\Sim, \tilde{\Verifier})$ defined in \Cref{CPM-3ZK:MnR:game:dummy} and the $\msf{Real}(\Sim, \tilde{\Verifier})$ defined in \Cref{CPM-3ZK:MnR:game:real}, it holds that
% $$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].$$
% \end{lemma}

% \subsection{Finishing the Proof of \Cref{CPM-3ZK:decider:lem:soundness}}
% \xiao{In this part, we finish the proof of \Cref{CPM-3ZK:decider:lem:soundness} assuming that \Cref{CPM-3ZK:MnR:game:dummy:lem} holds. This step is simple. I'll do it later.}




    





==> sections/CPM-babycase.tex <==

\section{Warm Up: Three-Round BBZK in the CPM Model (Part 1/2)}


\xiao{I change the model to a classical-prover-message (CPM) model. This is to reflect the final soundness reduction, where we have to receive unmeasured Verifier's messages from the external verifier. Only in this way can we ensure that the view of the simulator is identical to that in our dummy up-and-down game.}


In this section, we show as a warm-up example that three-round ZK in the CPM model is impossible. This proof already illustrate the main ideas behind our general impossibility for the constant-round case. \xiao{Note that even such a result is not known yet.}






\subsection{The Model}

\subsubsection{Protocol Structure}
 We consider a three-round protocol where the prover $\Prover$ and verifier $\Verifier$ takes a statement $x \in \Lang$ and the security parameter $\secpar$ as the comment input. $\Prover$ additional takes a witness $w \in \Relation_\Lang(x)$ as the private input. $\Prover$ sends the first message $p_1$; $\Verifier$ responds with the second message $v_1$; then, $\Prover$ sends the final message $p_2$. W.l.o.g., we assume that all these massages are of the same length $\ell(\secpar)$, which is a polynomial in $\secpar$. Since we are in the CMP model, the messages $(p_1, p_2)$ are all classical, but the message $v_2$ could be quantum. 

 \xiao{from now one, we append one more message $v_2$ (possibly quantum) at the end of the execution. This message is just that the honest verifier let $P$ know if the execution is accepted or not. Not that this can only make our impossibility stronger! So, the protocol now has four rounds, i.e., $(p_1, v_1, p_2, v_2)$. And we will keep calling it four-round CPM BBZK.}

\para{Honest Verifier}  \xiao{need to explain to specify the model.}





\subsubsection{Generic Malicious Verifier}

\begin{xiaoenv}{Generic Malicious Verifier}
A malicious verifier $\tilde{\Verifier}$ could differ from the honest $\Verifier$ in the following way:
\begin{itemize}
\item
Its work space $\reg{w}$ could be larger than $\Verifier$;
\item
It make take an auxiliary input $\ket{\rho}$ of polynomial size, stored in some part in $\reg{w}$ at the beginning of the protocol;
\item
It may use a different unitary $V^*$ (can be implemented by poly-size quantum circuits) from the honest $\Verifier$.
\end{itemize}
Other than the above, it behaves in the same way as the honest $\Verifier$.
\end{xiaoenv}

 


\subsubsection{ZK Simulator}
 We now describe formally how the simulator $\Sim$ interacts with a generic malicious verifier $\tilde{\Verifier}$. Once again, there are multiple ways to do so and we choose the following one without loss of generality, which is particularly suitable for our proof of impossibility.

Note that we focus on black-box simulation. Thus, $\Sim$ can only query $\tilde{\Verifier}$ via its unitary $\tilde{V}$ and its inverse $\tilde{V}^\dagger$, but does not get to see the internal register $\reg{w}$ of $\tilde{\Verifier}$. 


Also, recall that $\reg{m}$ is used to exchange messages, and as explained above, it is always measured when a party is about to send message in the real execution (as we are in the LOCC setting). However, it is worth noticing that for simulation, $\reg{m}$ is considered as being held by $\Sim$, who could choose {\em not} to measure it. 

In more detail, a black-box simulator $\Sim$ is defined by a ``local'' unitary $S$. It is granted oracle access to $\tilde{V}$ and $\tilde{V}^\dagger$. It makes use of the following registers
\begin{itemize}
\item
Register $\reg{m}$ to exchange messages with the malicious verifier $\tilde{V}$;
\item
Register $\reg{s}$ which is her ``local'' work space;
\item
A query register $\reg{u}$ in a $2$-dimension Hilbert space spanned by the basis $\Set{ \ket{\downarrow}_{\reg{u}}, \ket{\uparrow}_{\reg{u}}}$ (explained shortly).
\end{itemize}
$\Sim$ behavior is nothing but iterations of the following three steps:
\begin{enumerate}
\item
Apply the local operator $S$ on registers $\reg{m}$, $\reg{u}$, and $\reg{s}$;
\item
Measure the $\reg{u}$ register to learn the type of the next query (see the next bullet);
\item
Make the oracle query according to the measurement outcome from the last step---if the measurement outcome is $\ket{\uparrow}$, it query the $\tilde{V}$ oracle on $\reg{m}$; otherwise (i.e., the measurement outcome is $\ket{\uparrow}$), it query the $\tilde{V}^\dagger$ oracle on $\reg{m}$.
\end{enumerate}
$\Sim$ keeps repeating the above three steps until she decides to stop. At that moment, the internal state of $\tilde{V}$ is defined to be the simulation output.



% \para{Formal Description of $\Sim^{\tilde{V}(x, \ket{\rho})}$.} With the above intuitive explanation, we proceed to present the formal description of the interaction between $\Sim$ and a malicious verifier $\tilde{V}(x, \ket{\rho})$. 

% The execution starts by initializing the following state:
% \begin{equation}\label{2-LOCC:S:inital:expr}
% \ket{\eta_0} \coloneqq \ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{m_1}} \ket{\vb{0}}_{\reg{m_2}} \ket{\phi}_{\reg{o}} \ket{\downarrow_1}_{\reg{u_1}} \ldots \ket{\downarrow_1}_{\reg{u_q}} \ket{\rho}_{\reg{s}},
% \end{equation}





% \para{$\Sim$'s Behavior.} 
% \begin{xiaoenv}{}
% Start with the intermediate measurement. And then say that all the measurements on $\reg{u_j}$'s can be deferred, because a consequence of deferred measurement principle is:
% \begin{quote}
% {\em If after a measurement a qubit is used as a control qubit only, then the
% measurement can be deferred.}
% \end{quote}
% \end{xiaoenv}
% The behavior of a  $q$-query simulator can be described as follows. For $j \in [q]$, 
% \begin{itemize}
% \item
% Apply the local unitary $S_j$. $S_j$ is a unitary that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$; Intuitively, it represents the local operation $\Sim$ performs between two oracle queries. In particular, it computes and stores the type of the $j$-th query in register $\reg{u_j}$, possibly in superposition.
% \item
% Measure $\reg{u_j}$;
% \item
% Make the $j$-th oracle query according to the measurement outcome from the last step. Formally, we define this step as a unitary$O_{j}$ that operates non-trivially only on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$ and $\reg{o}$. We present the formal definition of $O_{j}$ in \Cref{figbox:LOCC:3ZK:oracle}.
% \end{itemize}


% \begin{FigureBox}[label={figbox:LOCC:3ZK:oracle}]{Description of Unitary $O_j$}
% Each $O_j$ can be understood as unitary controlled on register $\reg{u_j}$. Formally, for each $j \in [q]$, $O_j$ is defined as follows 
% \begin{itemize}
% \item
% If $\reg{u_j}$ is of the form $\ket{\downarrow_1}_{\reg{u_j}}$, it applies $\tilde{U}_1$ on $\reg{m_1}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\uparrow_1}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_1$ on $\reg{m_1}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\downarrow_2}_{\reg{u_j}}$, it applies $\tilde{U}_2$ on $\reg{m_2}$ and $\reg{o}$.
% \item
% If $\reg{u_j}$ is of the form $\ket{\uparrow_2}_{\reg{u_j}}$, it applies $\tilde{U}^\dagger_2$ on $\reg{m_2}$ and $\reg{o}$.
% \end{itemize}
% \end{FigureBox}

% % is defined by a sequence of $q$ unitary operators $\Set{S_1,  \ldots, S_q}$. It proceeds as follows:
% % \begin{itemize}
% % \item
% % {\bf (First $q$ queries)} For $j\in [q]$, $\Sim$ repeats the following steps:
% % \begin{itemize}
% %  \item
% %  $\Sim$ first applies the ``local'' unitary $S_j$, which operates non-trivially on registers $\reg{m_1}$, $\reg{m_2}$, $\reg{u_j}$, and $\reg{s}$. 
% %  \item
% %  Then, controlled on the query type (possibly in superposition) stored in $\reg{u_j}$, the corresponding unitary is applied according to the rule described in \Cref{figbox:LOCC:3ZK:oracle}.
% %  \end{itemize} 

% % \item
% % {\bf (Final output.)} We denote by $\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho)$ the above execution; We denote by $\OUT(\Sim^{\tilde{\Verifier}(x; \phi)}(x; \rho))$ the output of $\tilde{\Verifier}$, i.e., final state in $\reg{out}$ tracing out all other registers after the execution
% % \end{itemize}
% \xiao{add a remark explaining two things: (1) $S_{j}$ only need to work on $\reg{u}_j$ and does not touch other $\reg{u}$ registers; (2) There's no need to add $S_{q+1}$ for $\Sim$'s post-processing, as the output will anyway trace $\Sim$'s registers out.}


% \subpara{$\Sim$ with Deferred Measurements.} Recall that a consequence of the deferred measurement principle is that {\em If after a measurement a qubit is used as a control qubit only, then the measurement can be deferred.} Also, observe in the above description of $\Sim$'s behavior that each $\reg{u_j}$ register is used {\em only} as a controlled register to determine the type of $O_j$. Thus, by the deferred measurement principle, we can equivalently describe $\Sim$ as the following two steps (assuming the starting state is $\ket{\eta_0}$):
% \begin{enumerate}
% \item
% Compute $\ket{\eta_q} \coloneqq O_q S_q O_{q-1} S_{q-1} \cdots O_1 S_1\cdot \ket{\eta_0}$.
% \item
% Measure registers $\reg{u_1},\ldots, \reg{u_q}$.
% \end{enumerate}
% From now on, we will use this deferred-measurement description of the simulator $\Sim$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comment some old materials
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% At a high-level, $\Sim$ can run $\tilde{\mathcal{V}}$ as a real prover, i.e., sending a message to $\tilde{\Verifier}$ and expecting $\tilde{\Verifier}$'s response (dubbed as ``down-queries''), or rewind $\tilde{\Verifier}$ (dubbed ``up-queries''). In the following, we formally define $\Sim$'s behavior. We also show in \Cref{figure:Sim-query:3-round} an exemplary execution of $\Sim$ where she makes 17 queries in total. We find it helpful to trace this concrete example while trying to understand the behavior of $\Sim$.
% \begin{figure}[!thb]
% \centering{
%     \fbox{
%          \includegraphics[width=0.5\textwidth]{figures/Three-round-real.jpg}
%     }         
% }
% \caption{An exemplary Query Pattern of $\Sim$}
% \label{figure:Sim-query:3-round}
% \end{figure}

% \subpara{Initialize $p_1$:} $\Sim$ starts by preparing a state in register $\reg{m_1}$ as her first message $p_1$. Formally, $\Sim$ applies a ``local'' unitary $S_0$ that works non-trivially on register $\reg{m_1}$ and $\reg{s}$. This yields a quantum state $p_1$ in $\reg{m_1}$ together with some residual internal state of $\Sim$ in $\reg{s}$. 


% \subpara{Obtain $v_1$:} $\Sim$ then queries $\tilde{\Verifier}$ to learn the response $v_1$. Formally, $\tilde{V}$ applies the unitary $\tilde{U}_3\tilde{U}_2\tilde{U}_1$ as defined earlier, which yields a state $v_1$ in register $\reg{m_1}$. This step is illustrated as the $\downarrow$ labeled by $\circled{1}$ in \Cref{figure:Sim-query:3-round}, and we say that the execution moves from Layer-1 to Layer-2.\footnote{It is worth noting that although both $p_1$ and $v_1$ are classical strings in the real execution, the simulator $\Sim$ may put a quantum state in $\reg{m_1}$ as her first message, and in that case, $\tilde{V}$'s response $v_1$ may also be a quantum state.} 


% \subpara{Subsequent Queries:} From now on, $\Sim$ can freely ask $\tilde{V}$ to perform $\tilde{U}$ or $\tilde{U}^\dagger$, and may modify the contains of $\reg{m_1}$ and $\reg{m_2}$ in between using her unitaries $S_1$, $S_2$, and $S_3$. Formally, $\Sim$ repeats the following procedure
% \begin{itemize}
% \item
% if the execution reaches Layer-$i$ (for $i \in [3]$), $\Sim$ will first apply the unitary $S_i$, and then measure the single-qubit register $\reg{q}$ \xiao{add this register when explaining $\Sim$'s registers} to decide if she wants to make a $\tilde{U}$ query or a $\tilde{U}^\dagger$ query. Depending on the query made, the execution will either move to Layer-$(i-1)$ (if a $\tilde{U}^\dagger$ query is made) or Layer-$(i+1)$ (if a $\tilde{U}$ query is made). 

% W.l.o.g., we use the following conventions. When the execution is at Layer-1 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\uparrow}$, then $\Sim$ aborts the execution immediately. Intuitively, this is because the execution is already rewound to the very beginning and it does not make sense to rewind it further; we simply view this as a failed simulation. Also, when the execution is at Layer-3 and $\Sim$'s measurement of $\reg{q}$ leads to $\ket{\downarrow}$, then $\Sim$ terminates and announces the end of the simulation. Intuitively, Layer-3 represents the very end of the protocol and it does not make sense to continue to the next round; we simply view this as $\Sim$'s signal for the end of the simulation.
% \end{itemize}
% This procedure is best understood by tracing the example shown in \Cref{figure:Sim-query:3-round}. Consider the status of the execution right after the arrow $\circled{1}$. $\Sim$ then applies $S_2$ on $\reg{m_1}$ and $\reg{s}$ \xiao{probably on $\reg{m_2}$ as well?}, and measures $\reg{d}$. The situation shown in  \Cref{figure:Sim-query:3-round} corresponds to $\Sim$ decides to make a $\tilde{U}^\dagger$-query next (represented by arrow $\circled{2}$), which brings the execution back to Layer-1. $\Sim$ then applies $S_1$ on $\reg{m_1}$ and $\reg{s}$, and measures $\reg{d}$. By the assumption made above, $\Sim$ will make a $\tilde{U}$-query next, which brings the execution to Layer-2 (represented by arrow $\circled{3}$). 

% Another set of queries that deserve a closer look is from arrow $\circled{11}$ to arrow $\circled{12}$. They represent the following steps: Right after the $\tilde{U}$-query labeled by $\circled{10}$, $\Sim$ applies $S_3$ on $\reg{m_2}$ and $\reg{s}$, measures $\reg{q}$, and decides to make the  $\tilde{U}^\dagger$-query labeled by $\circled{11}$. This brings the execution to Layer-2. Then, $\Sim$ further rewinds the execution back to Layer-1 and ``jumps'' between Layer-1 and Layer-2 twice (as represented by arrow $\circled{12}$ to arrow $\circled{15}$). After that, $\Sim$ decides to go to Layer-3 as represented by arrow $\circled{16}$, which is the last query made by $\Sim$. That is, after applying $\circled{16}$, the measurement of $\reg{q}$ returns $\ket{\downarrow}$, indicating the end of the execution as we explained above. 


\subsection{Theorem Statement and Proof Outline}

\xiao{to do... As the title of the subsection indicates..}


\UpdateLine







\subsection{A Particular Malicious Verifier}
\label{sec:particular-mal-V}




\xiao{may need to explain the high-level picture: why are we defining $\tilde{V}$?} Similar as \cite{FOCS:CCLY21}, we first show the impossibility result with an inefficient $\tilde{V}$. The inefficiency is only due to a random function $H$ hard-wired in $\tilde{V}$. Jumping ahead, we will make $\tilde{V}$ efficient later (\xiao{Cref to sec}) by replacing $H$ with a $q$-wise independent hash.

\subsubsection{$\tilde{\Verifier}$'s registers}
\label{sec:LOCC-3ZK:Vtil:registers} 
$\tilde{\Verifier}$ starts by initializing the following registers (see \Cref{figure:2-LOCC-V:registers} for an explanation \xiao{add a figure explaining the meaning fo the registers.}):
\begin{equation}\label[Expression]{2-LOCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{\vb{0}}_{\reg{p_1}}\ket{\vb{0}}_{\reg{v_1}}\ket{\vb{0}}_{\reg{p_2}}\ket{\vb{0}}_{\reg{v_2}} \ket{\vb{0}}_{\reg{m}} \ket{\bot}_{\reg{t_1}}\ket{\bot}_{\reg{t_2}} \ket{0}_{\reg{d}} \ket{\vb{0}}_\reg{w} \ket{H}_{\reg{aux}} 
\end{equation}








% In the impossibility result, we construct a BQP algorithm that runs both the simulator $\simulator$ and verifier $V$.
% Our entire purified view therefore consists of all above registers $\reg{ins, a,b,m,aux,w,adv}$. 


\subsubsection{$\tilde{V}$'s Unitary.} 
\label{sec:LOCC-3ZK:Vtil:unitaries} 




\begin{xiaoenv}{Define the Counter}
Define the Counter

Both $\reg{gc}$ and $\reg{lc}$ registers are initialized to $0$. We set $C = 2^\secpar$,\footnote{We note that it suffices to set $C$ to any super-polynomial function on $\secpar$. We choose $2^\secpar$ only for concreteness.} and define the unitary $U_{gc}$ as the following mapping
 $$U_{gc} : 	\ket{i}_{\reg{gc}} \mapsto \ket{i+1 \mod C}_{\reg{gc}}.$$

 We also define the unitary to increase the local counter $U_{lc}$ as follows:
 $$U_{lc} : 	\ket{i}_{\reg{lc}} \mapsto \ket{i+1 \mod 4}_{\reg{lc}}.$$
 Note that modulus 4 is good enough for us, because we will show later that the local counter will always be in $\Set{1,2,3}$.
\end{xiaoenv}



We now desribe $\tilde{\Verifier}$'s unitary $\tilde{V}$. 


\begin{AlgorithmBox}[label={LOCC-3ZK:V:unitary}]{Unitary \textnormal{$\tilde{V}$} for the Malicious Verifier \textnormal{$\tilde{\Verifier}$}}

{\bf Helper Unitaries.} Before we described $\tilde{V}$, we first define some helper unitaries. For each $i \in [2]$:
\begin{itemize}	
\item 
{\bf $A_i$: swap $\reg{p_i}$ and $\reg{m}$.} This unitary swaps the contents of $\reg{p_i}$ and $\reg{m}$.

\item 
{\bf $B_i$: apply $V$'s unitary.}
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then apply $\sum_{p_i} \ketbra{p_i} \tensor V_{p_i}$, which is the honest $\Verifier$'s unitary to generate $v_i$ from $p_i$.
\item
If $H(p_1, \ldots, p_i) = 0$, then do nothing; 
\end{itemize}


\item 
{\bf $C_i$: deliver $v_i$.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_i}$.
\item
If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_i}$.
\end{itemize}

\item
{\bf $C'_i$: swap $\reg{t_i}$ and $\reg{m}$.} This unitary swaps the contents of $\reg{t_i}$ and $\reg{m}$.

\item 
{\bf $D_i$: increase local counter.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
\item
If $H(p_1, \ldots, p_i) = 0$, then do nothing.
\end{itemize}
\end{itemize}

\para{$\tilde{\Verifier}$'s Unitary $\tilde{V}$.} On each query, it compares the global counter value $i$ with the local counter value $j$ and behaves accordingly. In particular:
\begin{description}
\item[Case $i = j$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $D_iC_iB_iA_i$ as defined above.
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}

\item[Case $(i \ne j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $C'_iA_i$ as defined above.
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}
\end{description}
\end{AlgorithmBox}



% \para{Compare Counters.} On each query, $\tilde{\Verifier}$ first checks if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% \begin{enumerate}
% \item
% If $i \ne j$, then $\tilde{\Verifier}$ only applies $U_{gc}$ to increase the global counter, and does nothing else.
% \item
% If $i = j$, then $\tilde{\Verifier}$ first applies $U_{gc}$ to increase the global counter, and then behaves differently according to the value of the global counter $i$. We describe it in the following.
% \end{enumerate}

% \para{Global Counter $i = 1$.} This corresponds to $\tilde{\Verifier}$'s behavior for the 1st slot, namely generating $v_1$ as the response to the $p_1$ she just received form the $\Prover$. $\tilde{\Verifier}$ applies $\tilde{V}_1$, which is defined as follows
% $$\tilde{V}_1 \coloneqq D_1 C_1 B_1 A_1, $$
% \xiao{old name: $\tilde{V}_1 \coloneqq \tilde{U}_3 \tilde{U}_2 \tilde{U}_1,$}
% with the unitaries defined as follows:
% \begin{enumerate}
% % \item
% % {\bf ($\tilde{U}_{\msf{c}}$: Increase the Counter.)} This unitary maps $\ket{i}_{\reg{count}}$ to $\ket{i+1 \mod 2}_{\reg{count}}$.

% \item \label{item:Vtil:unitary:1-1}
% {\bf ($A_1$: Swap $\reg{p_1}$ and $\reg{m}$.)} This unitary swaps the contents of $\reg{p_1}$ and $\reg{m}$ registers.
% \begin{MyComment}
% In the real execution, this steps is for $\tilde{V}$ to move the first message it received from the prover (in the $\reg{m_1}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_1}$), so that it can perform computation in subsequent steps.
% \end{MyComment}

% \item \label{item:Vtil:unitary:1-2}
% {\bf ($B_1$: Apply $V$'s Unitary.)}
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then do nothing; \xiao{need to recall where $p_1$ is stored.}
% \item
% If $H(p_1) = 1$, then apply $\sum_{p_1} \ketbra{p_1} \tensor V_{p_1}$, which is the honest $\Verifier$'s unitary to generate $v_1$ from $p_1$.
% \end{enumerate}
% \begin{MyComment}
% Recall \xiao{from XXX} that $U$ can be written in the form of $\sum_{p_1} \ketbra{p_1}\tensor U_{p_1}$ because the concerned protocol is LOCC. $V_{p_1}$ works non-trivially on registers $\reg{ins}$, $\reg{v_2}$, and $\reg{w}$. In particular, it generates $V$'s message $v_1$ in register $\reg{v_1}$ (together with some residual state on $\reg{w}$).
% \end{MyComment}


% \item \label{item:Vtil:unitary:1-3}
% {\bf ($C_1$: Deliver $v_1$.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% \item
% If $H(p_1) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_1}$.
% % set the content in register $\reg{m}$ to $\ket{v_1 \xor m}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_1$ is the content in register $\reg{v_1}$. 
% \end{enumerate}


% \item \label{item:Vtil:unitary:1-4}
% {\bf ($D_1$: Increase Local Counter.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1) = 0$, then do nothing.

% \item
% If $H(p_1) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
% \end{enumerate}
% \end{enumerate}


% \para{Global Counter $i = 2$.} This corresponds to $\tilde{\Verifier}$'s behavior for the 2nd slot, namely generating $v_2$ as the response to the $p_2$ she just received form the $\Prover$. $\tilde{\Verifier}$ applies $\tilde{V}_2$, which is defined as follows
% $$\tilde{V}_2 \coloneqq D_2C_2B_2A_2, $$
% \xiao{old name: $\tilde{V}_2 \coloneqq \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,$}
% with the unitaries defined as follows:

% % This corresponds to $\tilde{\Verifier}$'s behavior for the 2nd slot, namely generating $v_2$ as the response to the $p_2$ she just received form the $\Prover$. This case is different from the above case of the 1st slot---$\tilde{\Verifier}$ will first query the oracle $H$ on input $p_1$ stored in the register $\reg{p_1}$, and behaves differently according to the answer from $H$. \xiao{(need to add a remark: technically, we need to first compute the output of $H$, then do the following computation, and then un-compute $H$?)} In particular, we need to consider the following two sub-cases:
% % \begin{enumerate}
% % \item \label[Case]{item:LOCC-3ZK:Vtil:slot-2:bad}
% % If $H(p_1) = 0$, then $\tilde{\Verifier}$ does not do anything. Equivalently, $\tilde{V}_2$ is defined as
% %  $$\tilde{V}_2 \coloneqq I.$$

% % \item \label[Case]{item:LOCC-3ZK:Vtil:slot-2:good}
% % Otherwise (i.e., $H(p_1) = 1$), then $\tilde{V}_2$ is defined as
% % $$\tilde{V}_2 \coloneqq \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,$$ 
% % with the unitaries defiend as follows:

% % \end{enumerate}
% \begin{enumerate}
% \item \label{item:Vtil:unitary:2-1}
% {\bf ($A_2$: Swap $\reg{p_2}$ and $\reg{m}$.)} This unitary swaps the contents of $\reg{p_2}$ and $\reg{m}$ registers.

% \begin{MyComment}
% In the real execution, this steps is for $\tilde{V}$ to move the $p_2$ message it received from the prover (in the $\reg{m_2}$ register) to its internal register that is supposed to store this message (i.e., $\reg{p_2}$), so that it can perform computation in the next step.
% \end{MyComment}

% \item \label{item:Vtil:unitary:2-2}
% {\bf ($B_2$: $\tilde{\Verifier}$'s Decision.)} This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then do nothing. \xiao{need to recall where $(p_1,p_2)$ are stored.}

% \item
% If $H(p_1, p_2) = 1$, then apply $\sum_{p_2} \ketbra{p_2} \tensor V_{p_2}$, which is the honest $\Verifier$'s unitary to generate $v_2$ from $p_2$.
%  % it applies $U_\msf{d}$, where  $U_\msf{d}$ is the honest verifier's decision unitary. \xiao{If necessary, we can decompose $U_\msf{d}$ as $U_{\msf{d}} \coloneqq \sum_{p_1, v_1, p_2}\ketbra{p_1, v_1, p_2} \tensor U_{p_1, v_1, p_2}$.}
% \end{enumerate}
% % \begin{MyComment}
% % Recall that $U_\msf{d}$ works non-trivially on registers $\reg{ins}$, $\reg{p_1}$, $\reg{v_1}$, $\reg{p_2}$, $\reg{d}$, and $\reg{w}$. In particular, it generates $V$'s final decision bit in register $\reg{d}$ (together with some residual state on $\reg{w}$).
% % \end{MyComment}



% \item \label{item:Vtil:unitary:2-3}
% \xiao{Add this to make the writing of my proof consistent event at the `last layer' (i.e., \Cref{lem:LOCC-3ZK-hyb02:proof:invariant}). This essentially allows Sim to see the verifier's final decision bit, which is a weaker notion of ZK. this makes our impossibility result stronger.} 

% {\bf ($C_2$:  Deliver $v_2$.)} This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% \item
% If $H(p_1, p_2) = 1$, then swap the contents of registers $\reg{m}$ and $\reg{v_2}$.
% % set the content in register $\reg{m}$ to $\ket{v_2 \xor m}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_2$ is the content in register $\reg{v_2}$. 
% % then sets the content in register $\reg{m_2}$ to $\ket{d \xor m}_{\reg{m_2}}$, where $m$ is the original content in register $\reg{m_2}$ and $d$ is the content in register $\reg{d}$.
% \end{enumerate}

% \item \label{item:Vtil:unitary:2-4}
% {\bf ($D_2$: Increase Local Counter.)} 
% This unitary perform the following operation in superposition:
% \begin{enumerate}
% \item
% If $H(p_1, p_2) = 0$, then do nothing.

% \item
% If $H(p_1, p_2) = 1$, then apply the unitary $U_{lc}$ to increase the local counter by 1. 
% \end{enumerate}

% \end{enumerate}



% \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.



\xiao{Add a lemma stating that for all $x\in \Lang$, the execution between the honest $\Prover$ and $\tilde{\Verifier}$ will lead to acceptance with probability $\epsilon^2$. This proof is simply, but it helps the reader to understand our model. Also, I want to high-light that in the real execution, \Cref{item:LOCC-3ZK:Vtil:slot-2:good} will always be triggered.	}






\subsection{$\BQP$ Decider}

\para{MnR Game with ZK Simulator.} We first define the measure-and-reprogram (MnR) game w.r.t. the simulator $\Sim$ and $\tilde{\Verifier}(x)$ defined in previous sections. This game is simply an instantiation of MnR game defined in \Cref{MnR:lem:game} with the following notation: 
\begin{enumerate}
\item \label{LOCC-3ZK:MnR:notation:item:1}
We treat the execution of the simulator (with oracle access to $\tilde{V}$ and $\tilde{V}^\dagger$) as an oracle machine $\Sim^{\tilde{\Verifier}}$ that has quantum oracle access to a random function $H: \mcal{X}^{\le 2} \rightarrow \mcal{Y}$, where $\mcal{X}=\bits^\ell$ and $\mcal{Y} = \bits$. Let $\vb{y} = (y_1, y_2) \in \mcal{Y}^2$.

\item \label{LOCC-3ZK:MnR:notation:item:2}
Recall that the output of  $\Sim^{\tilde{\Verifier}}$ is defined to be the output $\tilde{\Verifier}$ at halt, which is in turn defined to be all the internal registers of $\tilde{\Verifier}$. We will split $\tilde{\Verifier}$'s output as $(\vb{p} = (p_1, p_2), \rho_{\msf{out}})$,  where $\vb{p}$ is the string contained in the $\reg{p_1}$ and $\reg{p_2}$ registers, and $\rho_{\msf{out}}$ is the remaining state tracing out $\reg{p_1}$ and $\reg{p_2}$. In particular, $\rho$ contains the global counter register $\reg{gc}$ and register $\reg{d}$ that contains $\tilde{\Verifier}$'s final decision (qu)bit. 

\item \label{LOCC-3ZK:MnR:notation:item:3}
We assume that $\Sim^{\tilde{\Verifier}}$ as an oracle machine makes $q$ queries to $H$ in total.
\end{enumerate}

Since this game will be particularly important for the sequel sections, we choose to present it in full detail in \Cref{LOCC-3ZK:MnR:game}.


\begin{GameBox}[label={LOCC-3ZK:MnR:game}]{Measure-and-Reprogram Game \textnormal{$\Sim^{\tilde{\Verifier}}[H, \vb{y}]$}}
 It works as follows
\begin{enumerate}
\item
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$  conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$.

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes $H$, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item If $j=j_i$ for some $i\in[2]$, measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, 2_i})$ where $2_i\leq 2$ is determined by the measurement outcome, and then behaves according to the value $b_i$ as follows:
        \begin{enumerate}
        \item 
        If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$, and then answer the $j_i$-th query using the reprogrammed oracle. 
        \item 
        If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$. 
        \end{enumerate}
    \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [2]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{LOCC-3ZK:MnR:notation:item:2}).

\item
For all $i \in [2]$ such that $j_i = \bot$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}_i \coloneqq (p^*_1, \ldots, p^*_i)$. 

\item
{\bf Output:} The output of this game is defined as follows
\begin{itemize}
\item
If it holds for all $i \in [2]$ that $\vb{p}_i$ is a prefix of $\vb{p}_2$, then output $(\vb{p}_2, \rho_{\msf{out}})$;

\item
Otherwise, output $(\bot, \bot)$.
\end{itemize}
\end{enumerate}
\end{GameBox}

\para{Decider for $\BQP$.} We now define the $\BQP$ decider $\mcal{B}$ in \Cref{LOCC-3ZK:BQP-decider}.
\begin{AlgorithmBox}[label={LOCC-3ZK:BQP-decider}]{\textnormal{$\BQP$} Decider $\mcal{B}(x)$}
On input a classical string $x$, machine $\mcal{B}(x)$ works as follows:
\begin{enumerate}
\item
{\bf (Parameter Setting.)}
Let $\vb{1} \coloneqq (1,1)$. Let $\mcal{M} \coloneqq \bits^{\ell}$ and $H_0 :\mcal{M}^{\le 2} \ra \bits$ be the zero-function, i.e., $H_0(p_1, \ldots, p_i) = 0$ for all $(p_1, \ldots, p_i) \in \mcal{M}^{\le 2}$.

\item
{\bf (MnP Game with $\Sim^{\tilde{V}}$.)} Execute $(\vb{p} = (p_1, p_2), \rho) \la \Sim^{\tilde{V}}[H_0, \vb{1}]$ as per \Cref{LOCC-3ZK:MnR:game}. 
% and let $\hat{H}_0$ denote the oracle at halt (i.e., the re-programmed oracle). 
 That is, $\mcal{B}(x)$ executes \Cref{LOCC-3ZK:MnR:game} with $H \coloneqq H_0$ and $\vb{y} = (1,1)$ and  denotes the output of this procedure as $(\vb{p} = (p_1, p_2), \rho)$.
% , and denotes the oracle at the end of the MnR game as $\hat{H}_0$.
 Note that in this step, $\mcal{B}$ makes use of its input $x$, which is used as the input instance to $\tilde{V}$ (though we did not include it in the notation explicitly).

\item
{\bf (Output.)} It outputs 1 if and only if $\msf{Pred}(\rho) = 1$, where $\msf{Pred}(\rho)$ is a (quantum) predicate that outputs 1 if and only if all of the following conditions hold:
\begin{enumerate}
% \item
% $\hat{H}_0(p_1) = 1$ and $\hat{H}_0(p_1, p_2) = 1$. (Recall that $p_1$ and $p_2$ are contained in $\vb{p}$.)

\item
% The value contained in the global counter register $\reg{gc}$ is 2. (Recall that the $\reg{gc}$ register is contained in $\rho$ and remains classical throughout the whole execution.)
Measure the local counter register $\reg{lc}$ in the computational basis and the measurement outcome is 1. (Recall that the $\reg{lc}$ register is contained in $\rho$.)
\item
Measure register $\reg{d}$ in the computational basis and the measurement outcome is 1. (Recall that the $\reg{d}$ register is also contained in $\rho$.)
\end{enumerate}
\end{enumerate}
\end{AlgorithmBox}


Next, we argue that $\mcal{B}$ is a valid $\BQP$ decider. Toward that, it suffices to establish the following \Cref{LOCC-3ZK:decider:lem:completeness,LOCC-3ZK:decider:lem:soundness}.

\begin{lemma}[Completeness]\label{LOCC-3ZK:decider:lem:completeness}
\xiao{(need to talk about $\epsilon \le \epsilon_q = \frac{1}{256k^2q^2(4kq+1)^{2k}}$ in this lemma.)}
For all $\Lang \in \BQP$ and all $x \in \Lang \cap \bits^{\secpar}$, it holds for the $\mcal{B}$ defined in \Cref{LOCC-3ZK:BQP-decider} that
$$\Pr[\mcal{B}(x) = 1] \ge \frac{1}{8 \cdot (4kq + 1)^{2k}} -\negl(\secpar).$$
\xiao{need to change $k$ to 2 in this special case.}
\end{lemma}


\begin{lemma}[Soundness]\label{LOCC-3ZK:decider:lem:soundness}
For all $\Lang \in \BQP$ and all $x \in \bits^{\secpar} \setminus \Lang$, it holds for the $\mcal{B}$ defined in \Cref{LOCC-3ZK:BQP-decider} that
$$\Pr[\mcal{B}(x) = 1] = \negl(\secpar).$$
\xiao{need to change $k$ to 2 in this special case.}
\end{lemma}

We present the proof for \Cref{LOCC-3ZK:decider:lem:completeness} in \Cref{sec:LOCC-3ZK:decider:lem:completeness:proof}. 

The proof for \Cref{LOCC-3ZK:decider:lem:soundness} is one of the most technically involved part of this work, and thus we put it in a separate section in \Cref{sec:LOCC-3ZK:decider:lem:soundness:proof}.


\subsection{Proof of Completeness}
\label{sec:LOCC-3ZK:decider:lem:completeness:proof}

\xiao{need to modify $k$ to $2$.}

In this subsection, we prove \Cref{LOCC-3ZK:decider:lem:completeness}.

First, notice that 
\begin{align}
\Pr[\mcal{B}(x) = 1] 
& = 
\Pr[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_0, \vb{1}]] \label{LOCC-3ZK:decider:lem:completeness:proof:sparsity:1} \\ 
& \ge 
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]] - 32k^2q^2\epsilon \label[Inequality]{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2} 
\end{align}
where \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:1} follows from the definition and notation in \Cref{LOCC-3ZK:BQP-decider}, and \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2} follows from \Cref{lem:ind-sparse-and-zero}. 
% (In \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2}, the predicate $\msf{Pred}^{\hat{H}_\epsilon}$ works in the same manner as the $\msf{Pred}^{\hat{H}_0}$ defined in \xiao{Cref} , except that it replaces $\hat{H}_0$ with $\hat{H}_\epsilon$.)

\subpara{Additional Notation.} In the following, we make use of the following notation:
\begin{itemize}
\item
For any classical oracle $H$, we use $\msf{SIM}^{H}$ to refer to the execution of $\Sim^{\tilde{\Verifier}}$ where $\tilde{\Verifier}$ uses $H$ as the oracle. 

\item
When we write $\bs{\beta}$ in the subscribe of the $\Pr$ symbol, it means we sample $\bs{\beta}$ from a distribution $D_\epsilon$ over $\bits^2$, whose each coordinate takes 1 with probability $\epsilon$ independently. 

\item
For a function $H: \mcal{M}^{\le 2} \ra \mcal{Y}$ and a vector $\vb{p} = (p_1, p_2) \in \mcal{M}^2$,  let $\bar{H}(\vb{p}) \coloneqq  \big(H(p_1), H(p_1, p_2) \big)$.

\item
The bold-face $\vb{1}$ is defined to be $(1, 1)$.
\end{itemize}
With the above notation, it holds that:
\begin{align*}
& \Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]] \\  
=~&  
\sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}   \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \Sim^{\tilde{V}}[H_\epsilon, \vb{1}]]  \numberthis \label{LOCC-3ZK:decider:lem:completeness:proof:final:1} \\ 
\ge~& 
\frac{1}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 ~:~(\vb{p}, \rho) \la \msf{SIM}^{H^{\vb{p}^*, \vb{1}}_\epsilon}] \numberthis \label{LOCC-3ZK:decider:lem:completeness:proof:final:2} \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon, \bs{\beta}}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 \wedge \bs{\beta} = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H^{\vb{p}^*, \bs{\beta}}_\epsilon}] \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{\vb{p}^* \in (\bits^{\ell} \times \bits^{\ell}) \cup \Set{(\bot,\bot)}}  \Pr_{H_\epsilon}[\vb{p} = \vb{p}^* \wedge \msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \\
=~& 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \Pr_{H_\epsilon}[ \msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1} ~:~(\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \numberthis \label{LOCC-3ZK:decider:lem:completeness:proof:final:3} 
,\end{align*}
where \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:1} follows from the Law of Total Probability, \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:2} follows from \Cref{MnR:lem},  and \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:3} follows again from the Law of Total Probability.

Next, we bound the RHS of \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:3} via the ZK guarantee for simulator $\Sim$. First, recall that \xiao{This probably should be a lemma appeared earlier.} the honest $\Prover$ will make $\tilde{\Verifier}^{H_\epsilon}$ accept with probability $\epsilon^k$. That is,
\begin{equation}\label{LOCC-3ZK:decider:lem:completeness:proof:final:4}
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1}~:~ (\vb{p}, \rho) \la \msf{OUT}_{\tilde{\Verifier}}\big(\langle \Prover(w), \tilde{\Verifier}^{H_\epsilon} \rangle(x)\big)] = \epsilon^k,
\end{equation}
where we used the fact that by definition,  $\tilde{\Verifier}^{H_\epsilon}$ accepts if the $\reg{lc}$ register contains 2, the decision register $\reg{d}$ contains 1, and the transcript $(p_1, p_2)$ satisfies $H_\epsilon(p_1) = 1$ and $H_\epsilon(p_1, p_2) = 1$. 

It then follows from \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:4} and the ZK property that 
\begin{equation}\label{LOCC-3ZK:decider:lem:completeness:proof:final:5}
\Pr_{H_\epsilon}[\msf{Pred}(\rho) = 1 \wedge \bar{H}_\epsilon(\vb{p}) = \vb{1}~:~ (\vb{p}, \rho) \la (\vb{p}, \rho) \la \msf{SIM}^{H_\epsilon}] \ge \epsilon^k - \negl(\secpar) \ge \frac{\epsilon^k}{4} - \negl(\secpar).
\end{equation}

In summary, it holds that 
\begin{align*}
\Pr[\mcal{B}(x) = 1] 
& \ge 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \bigg(\frac{\epsilon^k}{4} - \negl(\secpar) \bigg) - 32k^2q^2\epsilon \numberthis \label[Inequality]{LOCC-3ZK:decider:lem:completeness:proof:final:6} \\ 
& \ge 
\frac{1}{4(4kq+1)^{2k}} - \negl(\secpar) - 32k^2q^2\epsilon \numberthis \label[Inequality]{LOCC-3ZK:decider:lem:completeness:proof:final:7} \\ 
& \ge
\frac{1}{8(4kq+1)^{2k}} - \negl(\secpar) 
,\end{align*}
where \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:6} follows from  \Cref{LOCC-3ZK:decider:lem:completeness:proof:sparsity:2}, \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:3}, and \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:5}, and \Cref{LOCC-3ZK:decider:lem:completeness:proof:final:7} follows from our parameter setting that $\epsilon \le \epsilon_q = \frac{1}{256k^2q^2(4kq+1)^{2k}}$. \xiao{need to talk about $\epsilon_q$ in the lemma.}

This completes the proof of \Cref{LOCC-3ZK:decider:lem:completeness}.







\section{Warm Up: Three-Round BBZK in the CPM Model (Part 2/2)}
\label{sec:LOCC-3ZK:decider:lem:soundness:proof}

In this section, we prove \Cref{LOCC-3ZK:decider:lem:soundness}. 

At a high level, we assume for contradiction that  \Cref{LOCC-3ZK:decider:lem:soundness} is false and show how to construct a malicious prover $\tilde{\Prover}$ breaking the soundness of the original LOCC ZK protocol. Toward that, we first need to make some modifications to the machine $\mcal{B}$ and the MnR game $\Sim^{\tilde{\Verifier}}$, making use of some particular properties of the $\tilde{\Verifier}$ we defined earlier. This is done in \xiao{cref}. Next, we will present the malicious prover $\tilde{\Prover}$ and prver that it can indeed break the soundness. This is done in \xiao{cref}.

\subsection{Preparation}
\subsubsection{Restating the MnR Game}
In \Cref{LOCC-3ZK:MnR:game:modify:1}, we present a modified version of the MnR game $\Sim^{\tilde{\Verifier}}[H, \vb{y}]$ defined in \Cref{LOCC-3ZK:MnR:game}. Since we will be interested only in the case $H = H_0$ and $\vb{y} = \vb{1} = (1, 1)$, we present this case only. We highlight its difference with \Cref{LOCC-3ZK:MnR:game} in \red{red color}.


\begin{GameBox}[label={LOCC-3ZK:MnR:game:modify:1}]{Measure-and-Reprogram Game \textnormal{$\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$}}
 It works as follows
\begin{enumerate}
\item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:1}
For each $i\in[2]$, uniformly pick \dlt{$(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$} \red{$(j_i,b_i)\in [q]\times \bits$} conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. \red{It re-label the tuples $\Set{(j_i, b_i)}_{i \in [2]}$ to make sure that $j_1 < j_2$.} \red{It also defines an empty vector $\vb{p}_0 = \emptyset$.}

\item
Run the oracle machine $\Sim^{\tilde{\Verifier}}$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes \red{$H_0$}, and when $\Sim^{\tilde{\Verifier}}$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:2:a} 
      If $j=j_i$ for some $i\in[2]$, \dlt{measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, 2_i})$ where $2_i\leq 2$ is determined by the measurement outcome,} \red{measure this query to obtain  $\vb{p}_i=(p_{i,1}, \ldots,p_{i, i})$.} \red{If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_i$, the execution halts immediately and outputs $(\bot, \bot)$.}
      \red{\begin{itemize}
      \item
      
      {\bf Defining $\msf{sq}(i)$:} Note that the $j_i$-th query to $\mcal{O}$ must be invoked by $\Sim$'s query to $\tilde{\Verifier}$. We will call this $\Sim$'s query (that invokes the $j_i$-th query to $\mcal{O}$) as the $i$-th special query and denote it by $\msf{sq}(i)$. We establish certain properties of $\msf{sq}(i)$ in \Cref{LOCC-3ZK:MnR:game:modify:1:lem}, which will be useful later. 
      \end{itemize}
      }

      It then behaves according to the value $b_i$ as follows:
        \begin{enumerate}
        \item 
        If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$, and then answer the $j_i$-th query using the reprogrammed oracle. 
        \item 
        If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i, \red{1})$. 
        \end{enumerate}
    \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [2]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{LOCC-3ZK:MnR:notation:item:2}).

\item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:4}
\dlt{For all $i \in [2]$ such that $j_i = \bot$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}^*_i \coloneqq (p^*_1, \ldots, p^*_i)$.} 

\item \label[Step]{LOCC-3ZK:MnR:game:modify:1:step:5}
{\bf Output:}  \red{Output $(\vb{p}_2, \rho_{\msf{out}})$.}
\begin{itemize}
\item
\dlt{If it holds for all $i \in [2]$ that $\vb{p}_i$ is a prefix of $\vb{p}_2$, then output $(\vb{p}_2, \rho_{\msf{out}})$;}

\item
\dlt{Otherwise, output $(\bot, \bot)$.}
\end{itemize}
\end{enumerate}
\end{GameBox}

\begin{lemma}\label{LOCC-3ZK:MnR:game:modify:1:lem}
For the $\dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]$ defined in \Cref{LOCC-3ZK:MnR:game:modify:1} and the $\mcal{B}(x)$ defined in \Cref{LOCC-3ZK:BQP-decider}, it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]]\ge \Pr[\mcal{B}(x) = 1].$$
Moreover, for the $\msf{sq}(i)$ $(\forall i \in [2])$ defined in \Cref{LOCC-3ZK:MnR:game:modify:1:step:2:a}, it enjoys the following properties:
\begin{itemize}
\item
Query $\msf{sq}(i)$ is a $\tilde{V}$-query (instead of being a $\tilde{V}^\dagger$-query).
\item
\xiao{to be added as needed.}
\end{itemize}
\end{lemma}
\begin{proof}
	\begin{xiaoenv}{Polish the language}
	The proof of this lemma follows from the way we set counters.

	Need to explain the order $j_1 < j_2$.

	Next, we argue that the change in \Cref{LOCC-3ZK:MnR:game:modify:1:step:1} does not decrease the accepting probability of the predicate. To see that, notice that we start with an all-$0$ function $H_0$, and the whole MnR game $\Sim^{\tilde{\Verifier}}[H_0, \vb{1}]$ measures at most 2 queries in total. Therefore, if there is a tuple $(j_i, b_i) = (\bot, \bot)$, then at most one query can be measured. Also, due to the way we set the global and local counters, it is clear that the measurement will not output $(p_1, p_2)$ unless an ealier measurement has output $(p_1)$. That is, the measured queries will appear in a length-increasing order. Thus, if only one query corresponds to $H_0$ being programmed at (at most) a single point $p_1$ (to output 1). This cannot bring the local counter to $2$. In this case, $\msf{Pred}(\rho)$ will always output 0. Thus, it will not decrease the winning probability by delete $\Set{(\bot, \bot)}$ from the support of $(j_i, b_i)$. 

	Also, note that if $(j_i, b_i)$ does not take the value $(\bot, \bot)$, the condition in \Cref{LOCC-3ZK:MnR:game:modify:1:step:4} will never be satisfied. Thus, we can safely delete  \Cref{LOCC-3ZK:MnR:game:modify:1:step:4} as well.

	The modification in \Cref{LOCC-3ZK:MnR:game:modify:1:step:2:a} is simply to say that the first measurement generate $(p'_1)$ and the second measurement generate $(p'_1, p'_2)$. We have argued this in the above.

	Also, as long as the measured queries appear in a length-increasing order, the modification in	\Cref{LOCC-3ZK:MnR:game:modify:1:step:5} becomes only cosmetic.
	\end{xiaoenv}

This completes the proof of \Cref{LOCC-3ZK:MnR:game:modify:1:lem}.

\end{proof}


\para{Looking into $\Sim^{\tilde{\Verifier}}$.} Next, we re-state the game $\dot{\Sim}^{\tilde{\Verifier}}[\red{H_0}, \red{\vb{1}}]$ defined in \Cref{LOCC-3ZK:MnR:game}. This time, we will look into the execution of $\Sim^{\tilde{\Verifier}}$ and their registers. This is different from previous games where we always treat $\Sim^{\tilde{\Verifier}}$ as a ``black-box'' and only focus on how it accesses the oracle $H_0$. We denote this game as $\msf{Real}(\Sim, \tilde{\Verifier})$ and present it in \Cref{LOCC-3ZK:MnR:game:real}.	

It is straightforward that \Cref{LOCC-3ZK:MnR:game:real} is identical to \Cref{LOCC-3ZK:MnR:game} with only cosmetic changes. Therefore, it holds that
\begin{equation}\label{LOCC-3ZK:MnR:to:real:ind-eq}
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \dot{\Sim}^{\tilde{\Verifier}}[{H_0}, {\vb{1}}]] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].
\end{equation}



\begin{GameBox}[label={LOCC-3ZK:MnR:game:real}]{Game \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier})$}}
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in [q]\times \bits$ conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. W.l.o.g., we assume that $j_1 < j_2$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner for each $i \in [2]$. 

\para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with $\tilde{V}$ and $\tilde{V}^\dagger$ accordingly, where $\tilde{\Verifier}$ uses $H^{(i-1)}_0$ as the oracle.


\para{For Query $\msf{sq}(i)$:} Note that by \Cref{LOCC-3ZK:MnR:game:modify:1:lem}, $\msf{sq}(i)$ is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.	Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and behaves according to the value $b_i$ as follows:
\begin{enumerate}
\item 
        If $b_i=0$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i)}_0$ as the oracle.
. 

\item 
        If $b_i=1$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i-1)}_0$ as the oracle.
\end{enumerate}


\para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Real}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_2, \rho_{\msf{out}})$.

\end{GameBox}


\subsubsection{A Dummy Game} 

\para{A Dummy Version of $\tilde{\Verifier}$.} We first define a unitary $\ddot{V}$, which should be treated as the ``dummy version'' of $\tilde{\Verifier}$'s unitary $\tilde{V}$. We present it in \Cref{LOCC-3ZK:V-dummy}, highlighting its difference with $\tilde{V}$ (defined in \Cref{LOCC-3ZK:V:unitary}) in \red{red color}.
\begin{AlgorithmBox}[label={LOCC-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}
{\bf Helper Unitaries.} We first define additional helper unitaries. For each $i \in [2]$:
\begin{itemize}
 \item
{\bf $\ddot{C}_i$: swap $\reg{m}$ and $\reg{t_i}$.} 
This unitary perform the following operation in superposition:
\begin{itemize}
\item
If $H(p_1, \ldots, p_i) = 1$, \red{then do nothing}. 
\item
If $H(p_1, \ldots, p_i) = 0$, then swap the contents of registers $\reg{t_i}$ and $\reg{m}$.
\end{itemize}
 \end{itemize} 

\para{Unitary $\ddot{V}$.} On each query, it compares the global counter value $i$ with the local counter value $j$ and behaves accordingly. In particular:
\begin{description}
\item[Case $(i = j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $D_i\red{\ddot{C}_i}A_i$, where $A_i$ and $D_i$ is  defined in \Cref{LOCC-3ZK:V:unitary} and $\ddot{C}_i$ is defined above.
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}

\item[Case $(i \ne j)$:] It first applies the unitary $U_{gc}$ to increase the global counter by 1, and then behaves according to the (increased) global counter. In particular:
\begin{itemize}
\item
If $i \in [2]$, then it applies $C'_iA_i$, where $A_i$ and $C'_i$ is  defined in \Cref{LOCC-3ZK:V:unitary}
\item
Otherwise (i.e., $i \notin[2]$), it does nothing (i.e., applies the identity operator).
\end{itemize}
\end{description}
\end{AlgorithmBox}




% \begin{AlgorithmBox}[label={LOCC-3ZK:V-dummy}]{Unitary \textnormal{$\ddot{V}$} for a Dummy-Version of \textnormal{$\tilde{\Verifier}$}}


% \para{Compare Counters.} On each query, check if the value $i$ contained in $\ket{i}_{\reg{gc}}$ is equal to the value $j$ contained in $\ket{j}_{\reg{lc}}$,
% \begin{itemize}
% \item
% If $i \ne j$, then apply $U_{gc}$ to increase the global counter, and do nothing else.
% \item
% If $i = j$, then first apply $U_{gc}$ to increase the global counter, and then behave differently according to the value of the global counter $i$. We describe it in the following.
% \end{itemize}

% \para{Global Counter $i = 1$.} Apply $\ddot{V}_1 \coloneqq D_1 \red{\ddot{C}_1} A_1$, where $D_1$ and $A_1$ are the same as for $\tilde{V}$ and $\ddot{C}_1$ is defined as follows:
% \begin{itemize}
% \item
% {\bf ($\ddot{C}_1$: Swap $\reg{m}$ and $\reg{t_1}$.)} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_1}$.

% \item
% If $H(p_1) = 1$, \red{then do nothing}. 
% \end{itemize}

% \end{itemize}


% \para{Global Counter $i = 2$.} Apply $\ddot{V}_2 \coloneqq D_2 \red{\ddot{C}_2} A_2$,
% where $D_2$ and $A_2$ are the same as for $\tilde{V}$ and $\ddot{C}_2$ is defined as follows:
% \begin{itemize}

% \item 
% {\bf ($\ddot{C}_2$: Swap $\reg{m}$ and $\reg{t_2}$.)} 
% This unitary perform the following operation in superposition:
% \begin{itemize}
% \item
% If $H(p_1, p_2) = 0$, then swap the contents of registers $\reg{m}$ and $\reg{t_2}$.

% \item
% If $H(p_1, p_2) = 1$, \red{then do nothing}. 
% \end{itemize}

% \end{itemize}

% \para{Other Cases.} If the global counter $i=0$ or $i \ge 3$, then do nothing.

% \end{AlgorithmBox}


\para{A Dummy MnR Game.} We now define another game $\msf{Dummy}(\Sim, \tilde{\Verifier})$. This game will essentially serve as a malicious prover $\tilde{\Prover}$ that could break the soundness of the original ZK protocol, leading to our desired contradiction. Intuitively, $\msf{Dummy}(\Sim, \tilde{\Verifier})$ behaves identical to $\msf{Real}(\Sim, \tilde{\Verifier})$ except for that it answers $\Sim$'s queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$ using the dummy version of $\tilde{\Verifier}$ as we defined in \Cref{LOCC-3ZK:V-dummy}. We present the game in \Cref{LOCC-3ZK:MnR:game:dummy} and highlight its difference $\msf{Real}(\Sim, \tilde{\Verifier})$ (in \Cref{LOCC-3ZK:MnR:game:real}) in \red{red color}. 
\begin{GameBox}[label={LOCC-3ZK:MnR:game:dummy}]{Game \textnormal{$\msf{Dummy}(\Sim, \tilde{\Verifier})$}}
For each $i\in[2]$, uniformly pick $(j_i,b_i)\in [q]\times \bits$ conditioned on that there exists at most one $i\in [2]$ such that $j_i=j^*$  for all $j^*\in [q]$. W.l.o.g., we assume that $j_1 < j_2$. Initialize $H^{(0)}_0 \coloneqq H_0$ and $\vb{p}_0 = \emptyset$ and run the oracle machine $\Sim^{\tilde{\Verifier}}$ in the following manner for each $i \in [2]$. 

\para{For $\Sim$'s Queries between $\msf{sq}(i-1)$ and $\msf{sq}(i)$:} Answer such queries with \red{$\ddot{V}$} and \red{$\ddot{V}^\dagger$} accordingly, using $H^{(i-1)}_0$ as the oracle. (Note that \red{$\ddot{V}$} is defined in \Cref{LOCC-3ZK:V-dummy}.)


\para{For Query $\msf{sq}(i)$:} Note that by \Cref{LOCC-3ZK:MnR:game:modify:1:lem}, $\msf{sq}(i)$ is a $\tilde{V}$-query and it invokes a measurement over registers $\reg{p_1}\ldots \reg{p_i}$, resulting in the measurement outcome $\vb{p}_i = (p_1, \ldots, p_i)$. If $\vb{p}_{i-1}$ is not a prefix of $\vb{p}_{i}$, the execution halts immediately with output $(\bot, \bot)$.	Otherwise, it defines $H^{(i)}_0 \coloneqq H^{\vb{p}_i, \vb{1}}_0$, and behaves according to the value $b_i$ as follows:
\begin{enumerate}
\item 
        If $b_i=0$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i)}_0$ as the oracle.
. 

\item 
        If $b_i=1$: apply $\tilde{V}$ with $\tilde{\Verifier}$ using $H^{(i-1)}_0$ as the oracle.
\end{enumerate}


\para{Output:} Let $(\vb{p}^*, \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt. This game $\msf{Dummy}(\Sim, \tilde{\Verifier})$ outputs $(\vb{p}_2, \rho_{\msf{out}})$.

\end{GameBox}
The following is the most involved lemma in this section. We defer its proof to \xiao{Cref}, before which we first show (in \xiao{Cref}) how to finish the current proof of \Cref{LOCC-3ZK:decider:lem:soundness} assuming that \Cref{LOCC-3ZK:MnR:game:dummy:lem} holds.


\begin{lemma}\label{LOCC-3ZK:MnR:game:dummy:lem}
For the $\msf{Dummy}(\Sim, \tilde{\Verifier})$ defined in \Cref{LOCC-3ZK:MnR:game:dummy} and the $\msf{Real}(\Sim, \tilde{\Verifier})$ defined in \Cref{LOCC-3ZK:MnR:game:real}, it holds that
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})].$$
\end{lemma}

\subsection{Finishing the Proof of \Cref{LOCC-3ZK:decider:lem:soundness}}
\xiao{In this part, we finish the proof of \Cref{LOCC-3ZK:decider:lem:soundness} assuming that \Cref{LOCC-3ZK:MnR:game:dummy:lem} holds. This step is simple. I'll do it later.}



\subsection{Branch-Wise Equivalence Suffices}
We first notice that \Cref{LOCC-3ZK:MnR:game:real} can be treated as a sequence of alternating unitaries and measurements. In particular, there are 3 types of measurements (and $(q+4)$ measurements are made in total):
\begin{enumerate}
\item
\label[Type]{LOCC-3ZK:branchwise:measure:type:1}
{\bf Type-1:} The simulator $\Sim$ simply alternates between her local unitary $S$ and the measurement on register $\reg{u}$, which determines the type of her next query (i.e., either $\tilde{V}$ or $\tilde{V}^\dagger$). Note that there are $q$ such measurements since $\Sim$ makes $q$ queries in total.
\item
\label[Type]{LOCC-3ZK:branchwise:measure:type:2}
{\bf Type-2:}
When $\Sim$ makes the $\msf{sq}(i)$-th query, it triggers a measurement on registers $\reg{p_1}, \ldots, \reg{p_i}$. Note that there are $k =2$ such measurements.

\item
\label[Type]{LOCC-3ZK:branchwise:measure:type:3}
{\bf Type-3:}
The $\msf{sq}(i)$-th query is answered according to a random bit $b_i$ sampled at the beginning. This can be equivalently understood as preparing a qubit $\ket{\psi}_{\reg{b_i}} = \frac{1}{\sqrt{2}} (\ket{0} + \ket{1})$ at the beginning and measuring it to define the classical bit $b_i$ used to answer the $\msf{sq}(i)$-th query. Note that there are $k =2$ such measurements as well.
\end{enumerate}
Also, notice that in \Cref{LOCC-3ZK:MnR:game:real}, the values $\Set{j_i}_{i \in [2]}$ are sampled at the very beginning and after that the timing of all the measurements are fixed. It then follows from \Cref{lem:branchwise:preparation} that the accepting probability $\Pr[\msf{Pred}(\rho)]$ w.r.t.\  \Cref{LOCC-3ZK:MnR:game:real} can be equivalently expressed as the summation of all accepting probabilities w.r.t.\ a ``sub-normalized'' version of \Cref{LOCC-3ZK:MnR:game:real} where all the $(q+4)$ measurements are replaced with projections. Formally, we defined the ``sub-normalized'' \Cref{LOCC-3ZK:MnR:game:real} (and similarly for \Cref{LOCC-3ZK:MnR:game:dummy}) in \Cref{LOCC-3ZK:MnR:game:subnormalized}.

\begin{FigureBox}[label={LOCC-3ZK:MnR:game:subnormalized}]{Sub-Normalized Games \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$} and \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$}}
{\bf Parameters.} Fix $J = (j_1, j_2)$ such that $j_1, j_2 \in [q]$ and $j_1 < j_2$. Also fix a classical string of $(q+4)$ symbols $\msf{pat} = (u_1, \ldots, u_q, p_1, b_{1}, p_1p_2,   b_2)$ with  $u_i \in \Set{\uparrow, \downarrow}$, $p_1 \in \Set{0, 1}^{\ell}$, $p_1p_2 \in \Set{0, 1}^{2\ell}$, and $b_1, b_2 \in\bits$. The following games are parameterized by $(J, \msf{pat})$.

\para{Game $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} It behaves identically to \Cref{LOCC-3ZK:MnR:game:real} except for the following differences: 
\begin{enumerate}
	\item
	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

\item
When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
\item
When the measurement on $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$) is triggered (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1}$ (resp.\ $\ketbra{p_1,p_2}$) to register $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$); 
\item
When it needs $b_i$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:3} above), it applies the projector $\ketbra{b_i}$ to register $\reg{b_i}$. 
\end{enumerate}

\para{Game $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} This is defined in a similar way w.r.t.\ \Cref{LOCC-3ZK:MnR:game:dummy}. Namely, It behaves identically to \Cref{LOCC-3ZK:MnR:game:dummy} except for the following differences: 
\begin{enumerate}
	\item
	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

\item
When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
\item
When the measurement on $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$) is triggered (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1}$ (resp.\ $\ketbra{p_1,p_2}$) to register $\reg{p_1}$ (resp.\ $\reg{p_1p_2}$); 
\item
When it needs $b_i$ (corresponding to \Cref{LOCC-3ZK:branchwise:measure:type:3} above), it applies the projector $\ketbra{b_i}$ to register $\reg{b_i}$. 
\end{enumerate}
\end{FigureBox}

It then follows from \Cref{lem:branchwise:preparation} that
\begin{align*}
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})] 
& = 
\frac{2!}{\binom{q}{2}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] \\
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] 
& = 
\frac{2!}{\binom{q}{2}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})],
\end{align*}
where the summations are taken over all possible $J$ and $\msf{pat}$ satisfying the requirements in \Cref{LOCC-3ZK:MnR:game:subnormalized}. 

Therefore, to prove \Cref{LOCC-3ZK:MnR:game:dummy:lem}, it suffices to prove the following \Cref{LOCC-3ZK:branch-wise:suffices}.
\begin{lemma}[Branch-Wise Equivalence Suffices]\label{LOCC-3ZK:branch-wise:suffices}
For all $(J, \msf{pat})$ satisfying the requirements in \Cref{LOCC-3ZK:MnR:game:subnormalized}, it holds that 
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})].$$
\end{lemma}


\subsection{Proving \Cref{LOCC-3ZK:branch-wise:suffices}}
In this proof, we consider an (arbitrarily) fixed $J$ and $\msf{pat}$ that satisfy the requirements in \Cref{LOCC-3ZK:MnR:game:subnormalized}.

\para{Simplification Assumptions.} We first make three assumptions regarding the behavior of $\Sim$. As we will show, these assumptions will not affect the accepting probability of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ and $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$, but it will simplify the notation and ease the presentation of the current proof.
\begin{itemize}
\item 
\hypertarget{LOCC-3ZK:simp-assumption:1}{{\bf Assumption 1:}} When the global counter is $\ket{0}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}^\dagger$ (resp.\ $\ddot{V}^\dagger$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$).

\item 
\hypertarget{LOCC-3ZK:simp-assumption:2}{{\bf Assumption 2:}} When the global counter is $\ket{2}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ (resp.\ $\ddot{V}$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$).

\item 
\hypertarget{LOCC-3ZK:simp-assumption:3}{{\bf Assumption 3:}} For each $i \in [2]$, before the $\msf{sq}(i)$-th query is made, when the global counter is $\ket{i-1}_{\reg{gc}}$, $\Sim$ will not make a $\tilde{V}$ (resp.\ $\ddot{V}$) query in $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$ (resp.\ $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$) 
\end{itemize}
\xiao{We argue that we can indeed make these assumptions when proving \Cref{LOCC-3ZK:branch-wise:suffices}. to do... 
} \xiao{A caveat is:} to make \hyperlink{LOCC-3ZK:simp-assumption:3}{Assumption 3}, we need to additionally assume that before the $\msf{sq}(i)$-th query is made, $\Sim$'s local operator may modify register $\reg{t_i}$. But we claim that this will not affect our proof of \Cref{LOCC-3ZK:branch-wise:suffices}. 




Next, we define a sequence of hybrids $H_0$, $H_1$, and $H_2$. To better illustrate these hybrids, we provide pictures in \Cref{figure:CPM-3ZK:hybrids}.

\para{Hybrid $H_0$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H0}.) This is exactly the execution of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. 

\xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H0}. 
Point out the position of $\msf{sq}(1)$ and $\msf{sq}(2)$. Also exaplain how the assumptions made above are reflected in this figure.}
\xiao{Also, this is the moment to introduce the notation of $\uparrow$-query and $\downarrow$-query.}

Therefore, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$




\para{Hybrid $H_1$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H1}.) This hybrid is identical to the previous one except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (i.e., query $\msf{sq}(1)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (resp.\ from $\ket{1}_{\reg{gc}}$ to $\ket{0}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}
This is best illustrated by the \red{red-color} symbols in \Cref{figure:CPM-3ZK:hybrids:H1} \xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H1}} 

\para{Hybrid $H_2$.} (Illustrated in \Cref{figure:CPM-3ZK:hybrids:H2}.) This hybrid is identical to the previous one except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (i.e., query $\msf{sq}(2)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (resp.\ from $\ket{2}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}
This is best illustrated by the \red{red-color} symbols in \Cref{figure:CPM-3ZK:hybrids:H2} \xiao{add more explanation. Also, tell the reader how to read \Cref{figure:CPM-3ZK:hybrids:H2}} 

It is straightforward that hybrid $H_2$ is exactly the execution of $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. Therefore, it holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_2 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$


\begin{figure}[!tb]
\centering
     \begin{subfigure}[t]{0.47\textwidth}
         \fbox{
         \includegraphics[width=\textwidth,page=1]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H0}
     \end{subfigure}
     \hspace{15pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=2]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H1}
     \end{subfigure}
     
     \centering\vspace{1em}
     \begin{subfigure}[t]{0.47\textwidth}
         
         \fbox{
         \includegraphics[width=\textwidth,page=3]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H2}
     \end{subfigure}
     \caption{Illustration of Hbyrids $H_0$, $H_1$, and $H_2$}
     \label{figure:CPM-3ZK:hybrids}
\end{figure}

With the above hybrids, to prove \Cref{LOCC-3ZK:branch-wise:suffices}, it now suffices to establish the following \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. 
\begin{lemma}\label{lem:CPM-3ZK:H01}
It holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_1 \big].$$
\end{lemma}

\begin{lemma}\label{lem:CPM-3ZK:H12}
It holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_1 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_2 \big].$$
\end{lemma}

\para{Preparation for the proofs of \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}.} In the sequel (\xiao{crefxxx}), we prove \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. Before we start, we first do some preparation work and set up some notations that will ease our presentation later.

First, recall from \Cref{LOCC-3ZK:MnR:game:real} that after the $\msf{sq}(i)$-th query is made, the malicious verifier $\tilde{\Verifier}$ will use $H^{\vb{p}_i, \vb{1}}_0$ as its oracle. Also, note that the above hybrids are defined w.r.t.\ a fixed $(J,\msf{pat})$. Therefore, we could re-write some of $\tilde{\Verifier}$'s unitaries in \Cref{LOCC-3ZK:V:unitary}, whose behavior depend on the value $H(p_1, \ldots, p_i)$, into a format that uses the $p_i$'s contained in (the a prior fixed) $\msf{pat}$ as a controlled unitary. 

In particular, for the $(p_1, p_2)$ contained in the fixed $\msf{pat}$, we keep the $U_{gc}$, $U_{lc}$, $A_i$ and $D_i$ the same as in \Cref{LOCC-3ZK:V:unitary}, but we re-write the unitaries $B_i$, $C_i$, and $\ddot{C}_i$ ($\forall i \in [2]$) in the following format:
\begin{enumerate}
\item \label{LOCC-3ZK:renaming:B1}
Let $B_1 = \ketbra{p_1}_{\reg{p_1}} \tensor B_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor I$. Note that $B_{1,1}$ is exactly the $V_{p_1}$ in \Cref{LOCC-3ZK:V:unitary}, and it acts non-trivially only on $\reg{v_1}$ and $\reg{w}$, and works as identity on other registers. 

\item \label{LOCC-3ZK:renaming:C1}
Let $C_1 = \ketbra{p_1}_{\reg{p_1}} \tensor C_{1,1} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor C_{1,0}$. Note that $C_{1,1}$ is the swap operator between $\reg{v_1}$ and $\reg{m}$; $C_{1,0}$ is the swap operator between  $\reg{t_1}$ and $\reg{m}$.

\item \label{LOCC-3ZK:renaming:ddotC1}
Let $\ddot{C}_1 = \ketbra{p_1}_{\reg{p_1}} \tensor I + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor C_{1,0}$. Note that $C_{1,0}$ is the swap operator between  $\reg{t_1}$ and $\reg{m}$.

\item \label{LOCC-3ZK:renaming:B2}
Let $B_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor B_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor I$. Note that $B_{2,1}$ is exactly the $V_{p_2}$ in \Cref{LOCC-3ZK:V:unitary}, which acts non-trivially only on $\reg{v_2}$ and $\reg{w}$, and works as identity on other registers.

\item \label{LOCC-3ZK:renaming:C2}
Let $C_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0}$. Note that $C_{2,1}$ is the swap operator between $\reg{m}$ and $\reg{v_2}$; $C_{2,0}$ is the swap operator between $\reg{m}$ and $\reg{t_2}$.

\item \label{LOCC-3ZK:renaming:ddotC2}
Let $\ddot{C}_2 = \ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor I + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0}$. Note that $C_{2,0}$ is the swap operator between $\reg{m}$ and $\reg{t_2}$.
\end{enumerate}
It will be helpful to keep track of the registers on which the unitaries acts on {\em non-trivially}. For the reader's convenience, we summarize it in \Cref{LOCC-3ZK:non-trivial-registers:table}. For a unitary shown in the table, it acts as the identity on registers not shown in its row.

\xiao{add $C'_1$, $C'_2$? not sure if necessary}
\begin{table}[!htb]
\centering
\caption{Registers on which the unitaries acts non-trivially}
\label{LOCC-3ZK:non-trivial-registers:table}
\vspace{0.5em}
\begin{tabular}{C{50pt} C{70pt} c C{50pt} C{70pt}}
\toprule
Unitary operators & Non-trivial registers & \phantom{abcde}  & Unitary operators & Non-trivial registers \\ 
\cmidrule{1-2} \cmidrule{4-5}
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$A_1$    	& $\reg{p_1}, \reg{m}$ & & 
$A_2$ 		& $\reg{p_2}, \reg{m}$ \\ 
\addlinespace[0.3em]
$B_1$ 		& $\reg{p_1}$, $\reg{v_1}$, $\reg{w}$   & & 
$B_2$ 		& $\reg{p_1}$, $\reg{p_2}$, $\reg{v_2}$, $\reg{w}$ \\
\addlinespace[0.3em]
$B_{1,1}$ 	& $\reg{v_1}$, $\reg{w}$  & & 
$B_{2,1}$ 	& $\reg{v_2}$, $\reg{w}$ \\ 
\addlinespace[0.3em]
$C_1$    	&  $\reg{p_1}$, $\reg{v_1}$, $\reg{t_1}$, $\reg{m}$ & & 
$C_2$    	&  $\reg{p_1}$, $\reg{p_2}$, $\reg{v_2}$, $\reg{t_2}$, $\reg{m}$  \\ 
\addlinespace[0.3em]
$C_{1,1}$   & $\reg{v_1}$, $\reg{m}$  & & 
$C_{2,1}$   & $\reg{v_2}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$C_{1,0}$  	& $\reg{t_1}$, $\reg{m}$ & & 
$C_{2,0}$  	& $\reg{t_2}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$\ddot{C}_1$    	&  $\reg{p_1}$,  $\reg{t_1}$, $\reg{m}$ & & 
$\ddot{C}_2$    	&  $\reg{p_1}$, $\reg{p_2}$,  $\reg{t_2}$, $\reg{m}$  \\ 
\addlinespace[0.3em]
$D_1$		& $\reg{p_1}$, $\reg{lc}$  & & 
$D_2$		& $\reg{p_1}$, $\reg{p_2}$, $\reg{lc}$ \\ 
\addlinespace[0.3em]
& & &   $S$ 		& $\reg{m}$, $\reg{u}$, $\reg{s}$  \\   
\bottomrule
\end{tabular}
\end{table}


\xiao{The following proof does not take care of the value $b_1$ and $b_2$. Need to add some argument to say that we can assume  w.l.o.g.\ that $b_1 = b_2 =1$.}

\subsection{Proving \Cref{lem:CPM-3ZK:H01}}

We first present the following \xiao{lemma}.
\xiao{add some intuitive explanation.}

\begin{lemma}[Invariance in $H_0$ and $H_1$]\label{lem:LOCC-3ZK-hyb01:proof:invariant}
Assume that during the execution of $H_0$ (and $H_1$), the global counter reaches value $1$ for $T$ times in total. For each $t \in [T]$, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds: in hybrid $H_0$ (resp.\ $H_1$), when the global counter reaches value $1$ for the $t$-th time, the overall state can be written as $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows
\begin{align}
\ket{\phi^{(t)}} 
& = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}}, \label{lem:LOCC-3ZK-hyb01:proof:target-format:H0}\\ 
\ket{\psi^{(t)}} 
& = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{C_{1,0}} \ket{\rho^{(t)}_{p'_1}}. \label{lem:LOCC-3ZK-hyb01:proof:target-format:H1}
\end{align}
where the unitaries $B_{1,1}$, $C_{1,0}$, and $C_{1,1}$  are as defined in \Cref{LOCC-3ZK:non-trivial-registers:table}.
\end{lemma}


\para{Finishing the proof of \Cref{lem:CPM-3ZK:H01}}. Let us consider the last time when the global counter reaches value $1$. By \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}, the overall states in $H_0$ and $H_1$ would be of the format 
\begin{align}
\ket{\phi^{(T)}} 
& = 
\overbrace{
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}} ,\\ 
\ket{\psi^{(T)}}
& = 
\overbrace{
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{C_{1,0}} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}}. 
\end{align}
Since this is the last time the global counter reaches value $1$, the two hybrids $H_0$ and $H_1$ by definition behave identically after that. That is, the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ will go through the same quantum procedure (let us denote it by $\mcal{F}$) and finally measured by the predicate $\msf{Pred}$.	

Next, note that the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the identical ``branch'' corresponding to $\ket{p_1}_{\reg{p_1}}$ (labeled as $\msf{Good}$ in the above equations). Also, the $\msf{Bad}$ branch will not contribute any shares to the accepting probability of the predicate $\msf{Pred}$---this is because the quantum procedure $\mcal{F}$ will never change the local counter for the $\msf{Bad}$ branch, and $\msf{Pred}$ will output $0$ if the local counter is not $\ket{2}_{\reg{lc}}$.	

In summary, only the $\msf{Good}$ branch matters for the remaining execution to contribute to the event $\msf{Pred}(\rho) = 1$. Therefore, \Cref{lem:CPM-3ZK:H01} holds because $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the same $\msf{Good}$ branch.

\para{Proving \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.} Now, the only thing left is to prove \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}. We establish this lemma by a mathematical induction on the number $t \in [T]$ indicating it is which time global counter reaches value $1$. We will keep track of how the overall states evolve in both $H_0$ and $H_1$ simultaneously.

\subsubsection{Base Case ($t = 1$)}
\label{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:sec} 

This corresponds to the very first time the global counter reaches $1$. By definition, this is due to $\Sim$'s query $\msf{sq}(1)$. 

We first derive how the overall state evolves in $H_0$. Formally, $\Sim$'s local operation $S$ is applied to the initial state, preparing a superposition in register $\reg{m}$. Then, the first $\tilde{V}$-query (i.e., the query $\msf{sq}(1)$) is made. Note that at this moment, both the global and local values are of the value $0$. Thus, according to \Cref{LOCC-3ZK:V:unitary} and \Cref{LOCC-3ZK:MnR:game:subnormalized}, the state will evolves as follows:
\begin{enumerate}
\item
$U_{gc}$ increases the global counter from $0$ to $1$. Note that currently, the global counter and local counter are of the form $\ket{1}_{\reg{gc}}\ket{0}_{\reg{gc}}$. 

\item
The unitary $A_1$ is applied

\item
The $\reg{p_1}$ register is projected to $\ketbra{p_1}_{\reg{p_1}}$.
\item
The unitary $D_1C_1B_1$ is then applied.
\end{enumerate}
In summary, the state $\ket{\phi^{(1)}}$ is obtained by applying the operator $D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}S$ is applied to the initial state. If we assume the initial state across all the registers are $\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}$, then it holds that:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}S  
\big(
\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}
\big) \\
& = 
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}  
\big( 
\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}} S \ket{\rho}
\big)
 \numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:1} \\ 
& = 
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 
\big(
\ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} S \ket{\rho} 
\big) 
\\
& = 
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} 
\big(
 \ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} A_1 S \ket{\rho} 
 \big)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:2} \\ 
& = 
D_1C_1B_1  
\big(
 \ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} \ketbra{p_1}_{\reg{p_1}}  A_1 S \ket{\rho} 
 \big)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:3} \\ 
& = 
D_1C_1B_1  
\big(
\ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\rho_{p_1}} 
\big)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:4} \\ 
& = 
D_1  
\big(
 \ket{1}_{\reg{gc}}\ket{0}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} C_{1,1}B_{1,1} \ket{\rho_{p_1}}
 \big) 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:5} \\ 
& = 
 \ket{1}_{\reg{gc}}\ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} C_{1,1}B_{1,1} \ket{\rho_{p_1}} 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:6} \\ 
& = 
 \ket{1}_{\reg{gc}}\ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:1} follows from the fact $S$ acts as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:2} follows from the fact $A_1$ acts as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:3} follows from the fact that the projector $\ketbra{p_1}_{\reg{p_1}}$ has no effects on $\reg{gc}$ and $\reg{lc}$;
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:4} follows by defining the (sub-normalized) state $\ket{\rho_{p_1}} \coloneqq \bra{p_1}_{\reg{p_1}}  A_1 S \ket{\rho}$;
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:5} follows from the definition of $B_{1,1}$ and $C_{1,1}$ (see \Cref{LOCC-3ZK:renaming:B1,LOCC-3ZK:renaming:C1});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:6}  follows from the definition of $D_1$ (see \Cref{LOCC-3ZK:V:unitary});
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} follows by defining $\ket{\rho^{(1)}_{p_1}} \coloneqq C_{1,1}B_{1,1} \ket{\rho_{p_1}}$.
\end{itemize}
% Obviously, $\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7}$ is a special case of \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} when $t = 1$.
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} satisfies the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} when $t = 1$.


Also, note that the game $H_0$ and $H_1$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:eq:7} that 
$$\ket{\psi^{(1)}} =  \ket{1}_{\reg{gc}}\ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} .$$ Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.



\subsubsection{Induction Step ($t \ge 2$)} 
\label{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:sec} 


We assume $\ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t-1)}}$ satisfies \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}, and prove in the following that \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} holds when the global counter reaches $1$ for the $t$-th time.

We establish this claim by considering the following MECE (mutually exclusive and collectively exhaustive) cases:
\begin{enumerate}
\item \label[Case]{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}
{\bf Case 1:} The $t$-th arrival at value $1$ is due to an immediate $\uparrow \downarrow$ after the $(t-1)$-th arrival. That is, after the $(t-1)$-th arrival, $\Sim$ first makes a $\uparrow$ query, bringing the global counter to $0$, and then makes an $\downarrow$ query, bringing the global counter back to $1$. 
\item \label[Case]{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}
{\bf Case 2:} The $t$-th arrival at value $1$  is due to an immediate $\downarrow \uparrow $ after the $(t-1)$-th arrival. That is, after the $(t-1)$-th arrival, $\Sim$ first makes a $\downarrow$ query, bringing the global counter to $2$, and then makes an $\uparrow$ query, bringing the global counter back to $1$. 
\end{enumerate}


\subsubsubsection{Proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}} 
We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) in  \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}:
\begin{enumerate}
 \item
$\Sim$'s local unitary $S$ is applied. Note that this step is identical for both $H_0$ and $H_1$. 
\item
An $\uparrow$-query is made, bringing the global counter from $1$ to $0$. 
\begin{itemize}
    \item
    In $H_0$, this corresponds to applying $\tilde{V}^\dagger$; 
    \item
    In $H_1$, this corresponds to applying $\ddot{V}^\dagger$. 
\end{itemize}
\item
The local operation $S$ is applied. Note that this step is identical for both $H_0$ and $H_1$ as well.
\item
An $\downarrow$-query is made, resulting in the global counter's $t$-th arrive to $1$.
\begin{itemize}
    \item
    In $H_0$, this corresponds to applying $\tilde{V}$; 
    \item
    In $H_1$, this corresponds to applying $\ddot{V}$. 
\end{itemize} 
\end{enumerate}
It follows from the above description that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
\begin{align}
\ket{\phi^{(t)}}
& = \tilde{V} S \tilde{V}^\dagger S  \ket{\phi^{(t-1)}}, \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}\\ 
\ket{\psi^{(t)}}
& = \ddot{V} S \ddot{V}^\dagger S \ket{\psi^{(t-1)}}. \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}
\end{align}

\begin{remark}[High-Level Idea for the Sequel]
Recall that our eventual goal is to prove that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ are of the format shown in \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0,lem:LOCC-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}. But we first need to perform some preparation work, putting \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. Then, we show on \Cpageref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} how to use \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} to complete the proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}. 
\end{remark}



\begin{MyClaim}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}
There exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ so that the following holds
\begin{align}
\ket{\phi^{(t)}}
& = 
D_1 \bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  
C_1 B_1 S^{\reg{p_1}/\reg{m}}   B^\dagger_1 C^\dagger_1
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\bigg)
\bigg) \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(t)}}
& = 
D_1 
\bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} 
\ddot{C}_1 S^{\reg{p_1}/\reg{m}}  \ddot{C}^\dagger_1 
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\bigg) 
\bigg)
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} 
\end{align}
where $S^{\reg{p_1}/\reg{m}}$ is identical to $S$ except that it treats register $\reg{p_1}$ as $\reg{m}$.
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}]
First, notice that  
\begin{equation}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S} 
A_1 S A^\dagger_1 =  A_1 A^\dagger_1  S^{\reg{p_1}/\reg{m}} = S^{\reg{p_1}/\reg{m}},
\end{equation}
where the first equality follows from the fact that $S$ as the identity operator on $\reg{p_1}$ and $A_1$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_1}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table}). 

\para{Proving \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(t)}}$:
\begin{align*}
\ket{\phi^{(t)}}
& =
\tilde{V} S \tilde{V}^\dagger S  \ket{\phi^{(t-1)}} 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} \\ 
& =
\tilde{V} S \tilde{V}^\dagger S  
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} \\ 
& =
\tilde{V} S \tilde{V}^\dagger   
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} S\ket{\rho^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} S C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} \\ 
& =
\tilde{V} S \tilde{V}^\dagger   
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} S\ket{\rho^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0} S^{\reg{t_1}/\reg{m}} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} \\
& =
\tilde{V} S \tilde{V}^\dagger   
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} S\ket{\rho^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} \\
& =
\tilde{V} S \tilde{V}^\dagger   
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} \\
& =
\tilde{V} S 
\bigg(
U^\dagger_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1 \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ \\ 
& \hspace{8em}  
U^\dagger_{gc} A^\dagger_1 C'^\dagger_1  \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} \\ 
& =
\tilde{V} S 
\bigg(
\ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}} A^\dagger_1 B^\dagger_1 C^\dagger_1   \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ \\ 
& \hspace{8em}  
 \ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}}  A^\dagger_1 C'^\dagger_1  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:8} \\ 
& =
\tilde{V} S 
\bigg(
\ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}} A^\dagger_1 B^\dagger_1 C^\dagger_1   \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ \\ 
& \hspace{8em}  
 \ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}}  A^\dagger_1 B^\dagger_1 C^\dagger_1  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:9} \\ 
& =
\tilde{V}  
\bigg(
\ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}} S A^\dagger_1 B^\dagger_1 C^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
~+~ 
  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:10} \\ 
& =
D_1C_1B_1A_1  
\bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} S A^\dagger_1 B^\dagger_1 C^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
~+~ \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:11} \\ 
& =
D_1  
\bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} C_1B_1A_1 S A^\dagger_1 B^\dagger_1 C^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
~+~ \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:12} \\ 
& =
D_1  
\bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} C_1B_1 S^{\reg{p_1}/\reg{m}} B^\dagger_1 C^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:13} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0};

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} follows from our induction assumption;

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} follows from the fact that $S$ acts as the identity operator on $\reg{gc}$, $\reg{lc}$, and $\reg{p_1}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} follows from the fact that $S$ acts as the identity operator on $\reg{t_1}$ and $C_{1,0}$ is nothing but a swap operator between $\reg{t_1}$ and $\reg{m}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table}); (Note that $S^{\reg{t_1}/\reg{m}}$ is defined to be an operator that is identical to $S$ except that it treats $\reg{t_1}$ as $\reg{m}$.)

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} follows from the fact that $S^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $C_{1,1}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} follows by setting 
\begin{equation}
\label[Expression]{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}
\ket{\dot{\rho}^{(t-1)}_{p_1}}   \coloneqq S_j \ket{\rho^{(t-1)}_{p_1}} ~~~\text{and}~~~
\ket{\dot{\rho}^{(t-1)}_{p'_1}}  \coloneqq S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1});
\end{equation}

\item
both \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:11} follows from the definition of $\tilde{V}$ (see  \Cref{LOCC-3ZK:V:unitary});

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:8} follows from the definition of $D_1$ (see  \Cref{LOCC-3ZK:V:unitary}), the fact that $A_1$, $B_1$, $C_1$, and $C'_1$ work as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table}), and the definition of $U_{gc}$;

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:9} follows from the fact that the operator $C'_1$ (see \Cref{LOCC-3ZK:V:unitary}) is identical to $C_1B_1$ (see \Cref{LOCC-3ZK:renaming:B1,LOCC-3ZK:renaming:C1}) {\em when register $\reg{p_1}$ contains values $p'_1 \ne p_1$};


\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:10} follows from the fact that $S$ acts as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table});

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:12} follows from the fact that $A_1$, $B_1$, and $C_1$ as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table}); 

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:13} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S}.
\end{itemize}
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:13} finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\para{Proving \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi}.} This proof is almost identical to the above proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align*}
\ket{\psi^{(t)}}
& =
\ddot{V} S \ddot{V}^\dagger S  \ket{\psi^{(t-1)}} 
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} \\ 
& =
\ddot{V} S \ddot{V}^\dagger S  
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2} \\ 
& =
\ddot{V} S \ddot{V}^\dagger   
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} S\ket{\rho^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0} S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:5} \\ 
& =
\ddot{V} S \ddot{V}^\dagger   
\bigg(
\ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:6} \\ 
& =
\ddot{V} S 
\bigg(
U^\dagger_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1 \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
~+~ \\
& \hspace{8em} 
U^\dagger_{gc} A^\dagger_1 C'^\dagger_1  \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}   \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} \\ 
& =
\ddot{V} S 
\bigg(
\ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}} A^\dagger_1 \ddot{C}^\dagger_1   \ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ \\ 
& \hspace{8em}  
 \ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}}  A^\dagger_1 C'^\dagger_1  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:8} \\
& =
\ddot{V}  
\bigg(
\ket{0}_{\reg{gc}} \ket{0}_{\reg{lc}} S A^\dagger_1  \ddot{C}^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
~+~ 
  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:10} \\ 
& =
D_1\ddot{C}_1 A_1 
\bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} S A^\dagger_1  \ddot{C}^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
~+~ \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}   \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:11} \\  
& =
D_1  
\bigg(
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} \ddot{C}_1  S^{\reg{p_1}/\reg{m}}  \ddot{C}^\dagger_1   
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  C_{1,0}    \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\bigg)
\numberthis \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:13} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1};

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2}  follows from our induction assumption;

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:5} follows from a similar argument as we did to derive \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2};

\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:6} follows from {\em the same definitions} of $\ket{\dot{\rho}^{(k-1)}_{p_1}}$ and $\ket{\dot{\rho}^{(k-1)}_{p'_1}}$ as shown in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot};

\item
both \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:11} follows from the definition of $\ddot{V}$ (see \Cref{LOCC-3ZK:V-dummy});



\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:8} follows from the definition of $D_1$ (see  \Cref{LOCC-3ZK:V:unitary}), the fact that $A_1$, $\ddot{C}_1$, and $C'_1$ work as the identity operator on $\reg{gc}$ and $\reg{lc}$ (see \Cref{LOCC-3ZK:non-trivial-registers:table}), and the definition of $U_{gc}$;



\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:10} follows  from a similar argument as we did to derive \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:10} from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:8};


\item
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:13} follows  from a similar argument as we did to derive \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:13} from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:11};

\end{itemize}
\Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:13} finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

This completes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\end{proof}




\begin{MyClaim}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}
Let $S^{\reg{p_1}/\reg{m}}$ and $\Set{\dot{\rho}^{(t-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ be as defined in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}. Let
\begin{align}
\ket{\gamma^{(t-1)}_0} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:0} \\ 
\ket{\gamma^{(t-1)}_1} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:1} \\ 
\ket{\gamma^{(t)}_0} 
& \coloneqq 
C_1 B_1 S^{\reg{p_1}/\reg{m}}   B^\dagger_1 C^\dagger_1 \ket{\gamma^{(t-1)}_0} 
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0} \\ 
\ket{\gamma^{(t)}_1}
& \coloneqq 
\ddot{C}_1 S^{\reg{p_1}/\reg{m}}  \ddot{C}^\dagger_1  \ket{\gamma^{(t-1)}_1}
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1} 
.\end{align}
Then, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds:
\begin{align}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\rho^{(t)}_{p'_1}} 
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} 
.\end{align}
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}]
This claim follows from an application of \Cref{lem:err-inv-com}, with the notation correspondence listed in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}}
\label{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1}$ & & $W_1$ & $C_{1,1}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_0$ & $C_{1,0}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_1}$ & & $W$   & $C_{1}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u}$, $\reg{s}$ & & $\tilde{W}$ & $\ddot{C}_1$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p'_1}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_1$ & $B_{1,1}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & $\ket{\gamma^{(t-1)}_0}$ \\ 
\addlinespace[0.3em]
   & & & $U$   & $B_1$ & & $\ket{\eta^{(\msf{in})}_1}$ & $\ket{\gamma^{(t-1)}_1}$  \\ 
   \addlinespace[0.3em]
 &  & & $S$   & $S^{\reg{p_1}/\reg{m_1}}$ & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\gamma^{(t)}_0}$  \\ 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\gamma^{(t)}_1}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_1$ should work as the identity operator on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{1,1}$ (playing the role of $W_1$) who works as identity on registers $\reg{u}$ and $\reg{s}$ (playing the role of registers $\reg{s}$). (Recall $C_{1,1}$ from \Cref{LOCC-3ZK:non-trivial-registers:table}.)

\item
\Cref{lem:err-inv-com} requires that $W_0$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{1,0}$ (playing the role of $W_0$), who is a swap operator between registers $\reg{m}$ and $\reg{t_1}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively). (Recall $C_{1,0}$ from \Cref{LOCC-3ZK:non-trivial-registers:table}.)

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_0$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $\ddot{C}_1$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $C_{1,0}$ (playing the role of $W_0$) on branches $\ket{p'_1}_{\reg{p_1}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $p'_1 \ne p_1$. (Recall $\ddot{C}_1$ from \Cref{LOCC-3ZK:renaming:ddotC1})

\item
 \Cref{lem:err-inv-com} requires that $U_1$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $B_{1,1}$ (playing the role of $U_1$), who works as identity on registers $\reg{u}$ and $\reg{s}$ (playing the role of register $\reg{s}$). (Recall $B_{1,1}$ from \Cref{LOCC-3ZK:non-trivial-registers:table}.)

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $S^{\reg{p_1}/\reg{m}}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{u}$ and $\reg{s}$ (playing the role of registers $\reg{a}$ and $\reg{s}$). (Recall $S$ from \Cref{LOCC-3ZK:non-trivial-registers:table} and the fact that $S^{\reg{p_1}/\reg{m}}$ is identical to $S$ except that it treats $\reg{p_1}$ as $\reg{m}$.)
\end{itemize}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:LOCC-3ZK-hyb01:proof:case-1:cor-table}) to the $\ket{\gamma^{(t-1)}_0}$ and $\ket{\gamma^{(t-1)}_1}$ defined in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1}  (playing the role of $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ in \Cref{lem:err-inv-com}). This implies the existence of (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1\in\bits^\ell }$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\gamma^{(t)}_0} 
& = \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}} \\ 
\ket{\gamma^{(t)}_1} 
& = \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
,\end{align*}
which are exactly \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} in  \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. 






This completes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}.

\end{proof}

\para{Finishing the Proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}.}\label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} With \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} at hand, we now finish the proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}.

We first establish \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0}:
\begin{align}
\ket{\phi^{(t)}} 
& = D_1 \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} \ket{\gamma^{(t)}_0} 
\label{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:1} \\ 
& = D_1 \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\rho^{(t)}_{p'_1}} 
\bigg) 
\label{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:2} \\ 
& = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(t)}_{p_1}}  
+ 
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\rho^{(t)}_{p'_1}} 
\label{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}; 

\item
\Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:2} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2};

\item
\Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} follows from the definition of $D_1$ (see \Cref{LOCC-3ZK:V:unitary}).
\end{itemize}
Note that \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} is exactly 
\Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}. 


Next, we establish \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1}:
\begin{align}
\ket{\psi^{(t)}} 
& = D_1 \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} \ket{\gamma^{(t)}_1} 
\label{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:1} \\ 
& = D_1 \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}} 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
\bigg) 
\label{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:2} \\ 
& = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(t)}_{p_1}}  
+ 
\ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0}  \ket{\rho^{(t)}_{p'_1}} 
\label{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:1} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}; 

\item
\Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:2} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2};

\item
\Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} follows from the definition of $D_1$ (see \Cref{LOCC-3ZK:V:unitary}).
\end{itemize}
Note that \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} is exactly 
\Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.

~\\ 
This eventually completes the proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-1}.









\subsubsubsection{Proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}} 
We first remark that in \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}, the computation that brings $\ket{\phi^{(t-1)}}$ to $\ket{\phi^{(t)}}$ is identical to that brings $\ket{\psi^{(t-1)}}$ to $\ket{\psi^{(t)}}$, because $H_0$ and $H_1$ are identical when the global counter ``jumps'' between $1$ and $2$. (This can be also seen pictorially by comparing \Cref{figure:CPM-3ZK:hybrids:H0} and \Cref{figure:CPM-3ZK:hybrids:H1}.) In the following, we refer to this computation as $\Lambda$. That is, we have $\ket{\phi^{(t)}} = \Lambda \ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t)}} = \Lambda \ket{\psi^{(t-1)}}$. It then follows from our induction assumption
\begin{align*}
\ket{\phi^{(t)}} 
& = \Lambda \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  +
\Lambda \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}, \\ 
\ket{\psi^{(t)}} 
& = \Lambda \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  +
\Lambda \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t-1)}_{p'_1}}.
\end{align*}
Therefore, to finish the proof for \Cref{LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}, it suffices to establish the following \Cref{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:1,LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:2}.

\begin{MyClaim}\label{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:1}
There exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell \setminus \Set{p_1}}$ so that the following holds
\begin{align}
 \Lambda \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}} 
 & = 
 \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}}  
 \label{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:1:eq:1}\\
 \Lambda \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t-1)}_{p'_1}}
 & = \ket{1}_{\reg{gc}} \ket{0}_{\reg{lc}}  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
  \label{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:1:eq:2}
.\end{align} 
\end{MyClaim}

\begin{MyClaim}\label{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:2}
There exists a (possibly sub-normalized) pure state $\ket{\rho^{(t)}_{p_1}}$ so that the following holds
$$\Lambda \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}} = \ket{1}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}.$$
\end{MyClaim}
Now, this only thing left is to finish the proof of the above two claims, which we do in 
\Cref{LOCC-3ZK-hyb01:invariant:induction:case-2:claim:1:proof:sec,LOCC-3ZK-hyb01:invariant:induction:case-2:claim:2:proof:sec} respectively.


\subsubsubsection{Proof of \Cref{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:1}} 
\label{LOCC-3ZK-hyb01:invariant:induction:case-2:claim:1:proof:sec}



\UpdateLine{}

\subsubsubsection{Proof of \Cref{LOCC-3ZK-hyb01:proof:invariant:induction:case-2:claim:2}} 
\label{LOCC-3ZK-hyb01:invariant:induction:case-2:claim:2:proof:sec}

\xiao{to do...}

\UpdateLine{}


We now describe formally how $\ket{\phi^{(t-1)}}$ (and thus $\ket{\psi^{(t-1)}}$) evolves in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}. 
\begin{enumerate}
\item
$\Sim$'s local operator $S$ is applied
\item
An $\downarrow$-query is made, bringing the global counter to $2$. Here are two sub-cases to consider, depending if the $\downarrow$ query represents the first time the global counter arrives at $2$.
\begin{enumerate}
\item \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-1}
If it is the first time the global counter arrives at $2$ (i.e., the $\msf{sq}(2)$ query), then, by the definition of $\tilde{V}$ (see \Cref{LOCC-3ZK:V:unitary}),  the operator  $\tilde{U}_6 \tilde{U}_5 \ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} \tilde{U}_4$ will be applied;
\item \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-2}
Otherwise, the operator $\tilde{U}_6 \tilde{U}_5 \tilde{U}_4$ will be applied.   
\end{enumerate}
\item 
The $(j + 1)$-th local operation $S_{j+1}$ is applied. 
\item
An $\uparrow$-query is made, bringing the execution to Layer-2 for the $k$-th time. This corresponds to applying $\tilde{U}^\dagger_4\tilde{U}^\dagger_5 \tilde{U}^\dagger_6$.
\end{enumerate}
In summary, the evolution in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2} could be expressed as 
\begin{align}
\ket{\phi^{(k)}} &= \Lambda S_j \cdot \ket{\phi^{(k-1)}} \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi}\\ 
\ket{\psi^{(k)}} &= \Lambda S_j \cdot \ket{\psi^{(k-1)}} \label{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi},
\end{align}
where $\Lambda$ is defined to be {\em either}
\begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:def:Lambda}
\Lambda \coloneqq \tilde{U}^\dagger_4\tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_{j+1} \tilde{U}_6 \tilde{U}_5 \ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} \tilde{U}_4~~~\text{or}~~~\Lambda \coloneqq \tilde{U}^\dagger_4\tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_{j+1} \tilde{U}_6 \tilde{U}_5 \tilde{U}_4,
\end{equation}
depending on which sub-case between \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-1,lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2-2} we are talking about.

Fortunately, we can finish the proof for both of these two sub-cases (i.e., the two versions of $\Lambda$) at one stroke. To do that, we first establish a claim regarding the operator $\Lambda$.
\begin{MyClaim}\label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}
The following holds for both forms of $\Lambda$ as defined in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:def:Lambda}. There exist two operators $\Lambda_0$ and $\Lambda_1$ operating on registers other than $\reg{p_1}$ so that the following holds
\begin{align}
& 
\Lambda = \ketbra{p_1}_{\reg{p_1}} \tensor \Lambda_0 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Lambda_1, \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} \\ 
& 
\Lambda_1 \tilde{U}_{3,1}  = \tilde{U}_{3,1} \Lambda^{\reg{t_1}/\reg{m}}_1, ~\text{and} \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} \\ 
& 
\Lambda_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Lambda^{\reg{t_1}/\reg{m}}_1 \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} 
,\end{align}
where $\Lambda^{\reg{t_1}/\reg{m_1}}_1$ is identical to $\Lambda_1$ except that it treats $\reg{t_1}$ as $\reg{m_1}$.  
\end{MyClaim}

\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}]
To prove \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, it suffices to show that for each operator $\Gamma \in \Set{S_{j+1}, \tilde{U}_6, \tilde{U}_5, \ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}},\tilde{U}_4}$, there exist operators $\Gamma_0$ and $\Gamma_1$ so that $\Gamma$ can be written as 
$$\Gamma = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_0 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_1$$
and it holds that $\Gamma_1 \tilde{U}_{3,1}  = \tilde{U}_{3,1} \Gamma^{\reg{t_1}/\reg{m}}_1$ and $\Gamma_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Gamma^{\reg{t_1}/\reg{m}}_1$.

Obviously, the above is true for $\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}}$, simply because such a $\Gamma$ can be written in the following format:
$$\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_0  + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor I,$$
with $\Gamma_0  \coloneqq \ketbra{p_2}_{\reg{p_2}}$ and $\Gamma_1  \coloneqq I$, and thus $\Gamma_1$ vacuously satisfies the requires $\Gamma_1 \tilde{U}_{3,1}  = \tilde{U}_{3,1} \Gamma^{\reg{t_1}/\reg{m}}_1$ and $\Gamma_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Gamma^{\reg{t_1}/\reg{m}}_1$.


% acts on neither $\reg{p_1}$ nor $\reg{m}$, and it acts non-trivially on different registers from that of $\tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}).

The above is true for $\Gamma =\tilde{U}_4$ as well, because $\tilde{U}_4$ is nothing but the swap operator between registers $\reg{p_2}$ and $\reg{m}$.

The above is also true for $\Gamma = S_{j+1}$ because (1) $S_{j+1}$ does not act on $\reg{p_1}$, (2) $S_{j+1}$ does not work on $\reg{t_1}$ and $\tilde{U}_{3,1}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_1}$, and (3) $S^{\reg{t_1}/\reg{m}}_{j+1}$ acts non-trivially on different registers from $\tilde{U}_{2,0}$ and $\tilde{U}_{3,0}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}).



% is easy to see (from \Cref{LOCC-3ZK:table:non-trivial-registers}) that $S_{j+1} \tilde{U}_{3,1}  = \tilde{U}_{3,1}   S^{\reg{t_1}/\reg{m_1}}_{j+1}$ and  $S_{j+1} \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m_1}}_{j+1}$.


The only  cases left are $\Gamma \in \Set{\tilde{U}_5, \tilde{U}_6}$. These two cases are a little trickier than the previous cases because they use $\reg{p_1}$ (and $\reg{p_2}$) as a control register (see \Cref{LOCC-3ZK:renaming:3,LOCC-3ZK:renaming:4}). In the following, we only prove it for $\Gamma = \tilde{U}_6$; the other case (i.e., $\Gamma = \tilde{U}_5$) follows from a similar argument.
\begin{align*}
\Gamma = \tilde{U}_6 
& = 
\ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{6,0} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor \tilde{U}_{6,1} \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:1} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor \tilde{U}_{6,0} 
+ 
\sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1}_{\reg{p_1}} \tensor \ketbra{p'_2}_{\reg{p_2}} \tensor \tilde{U}_{6,1} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor \tilde{U}_{6,0} 
+ \ketbra{p_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1} \\ 
& \hspace{15em} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1} \\ 
& = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_0 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_1 \numberthis \label{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:2}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:1} follows from the definition of $\tilde{U}_6$ from \Cref{LOCC-3ZK:renaming:4}, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:U6:2} follows from defining $\Gamma_0$ and $\Gamma_1$ as follows 
\begin{align*}
 \Gamma_0 & \coloneqq \ketbra{p_2}_{\reg{p_2}} \tensor \tilde{U}_{6,0} 
+ \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1} \\ 
 \Gamma_1 & \coloneqq \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor \tilde{U}_{6,1}.
\end{align*} 
Clearly, such a $\Gamma_1$ also satisfies $\Gamma_1 \tilde{U}_{3,1}   = \tilde{U}_{3,1}  \Gamma_1^{\reg{t_1}/\reg{m}}$ and $\Gamma_1 \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} = \tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Gamma_1^{\reg{t_1}/\reg{m}}$, because (1) such a $\Gamma_1$ does not operates on $\reg{t_1}$, (2) $\tilde{U}_{3,1}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_1}$, and (3) $\Gamma^{\reg{t_1}/\reg{m}}_1$ acts non-trivially on different registers from $\tilde{U}_{2,0}$ and $\tilde{U}_{3,0}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}).
% $\Gamma_1$ operates on different registers from $\tilde{U}_{3,1}  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ and $\Gamma_1$ does not work on $\reg{m_1}$ (therefore it is vacuously true that $\Gamma_1 = \Gamma^{\reg{t_1}/\reg{m_1}}_1$).


This finishes the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.

\end{proof}



\para{Finishing the Proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}.} In the following, we show how to finish the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2} using \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.

First, we present the derivation for $\ket{\phi^{(k)}}$:
\begin{align}
 \ket{\phi^{(k)}} & = \Lambda S_j \cdot \ket{\phi^{(k-1)}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:0}\\ 
 & =  
\Lambda  S_j \cdot
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}}
\bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:1} \\ 
& = 
\Lambda \cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  S_j \tilde{U}_{3,1} \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:2} \\
& = 
\Lambda \cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1} S^{\reg{t_1}/\reg{m}}_j  \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:3} \\ 
& = 
\Lambda \cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} \bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:4} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \Lambda_1 \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:5} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \Lambda^{\reg{t_1}/\reg{m}}_1 S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:6} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}   \tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0} \ket{\rho^{(k)}_{p'_1}},  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:7} 
\end{align}
where  \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:0} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:1} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:2}  follows from the fact that $S_j$ does not act on register $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:3} follows from the definition of $S_j$ and $\tilde{U}_{3,1}$, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:4} follows from the fact that $S^{\reg{t_1}/\reg{m}}_j$ and $\tilde{U}^\dagger_{2,0} \tilde{U}^\dagger_{3,0}$ operate non-trivially on different registers (see \Cref{LOCC-3ZK:table:non-trivial-registers}), \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:5} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:6} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:7} follows by defining
\begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:def:rho-k}
\ket{\rho^{(k)}_{p_1}} 
\coloneqq 
 \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}} ~~~\text{and}~~~ 
\ket{\rho^{(k)}_{p'_1}} 
\coloneqq 
\Lambda^{\reg{t_1}/\reg{m}}_1 S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}). 
\end{equation}
Clearly, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:7} is of the same format as \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.


Next, we present the derivation for $\ket{\psi^{(k)}}$:
\begin{align}
 \ket{\psi^{(k)}} & = \Lambda S_j \cdot \ket{\psi^{(k-1)}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0}\\ 
 & =  
\Lambda  S_j \cdot
\bigg( 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \ket{\rho^{(k-1)}_{p'_1}}
\bigg) \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \Lambda_1 \tilde{U}_{3,1}     S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2} \\
& = 
\ket{p_1}_{\reg{p_1}} \Lambda_0 S_j \ket{\rho^{(k-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}    \Lambda^{\reg{t_1}/\reg{m}}_1 S^{\reg{t_1}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1}}  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3} \\  
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(k)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}   \tilde{U}_{3,1}    \ket{\rho^{(k)}_{p'_1}},  \label{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} 
,\end{align}
where \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi}, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2} follows from a similar argument as we derived \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:5} (from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:eq:1}), \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3} follows from \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, and \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} follows from the same definitions of $\ket{\rho^{(k)}_{p_1}}$ and $\ket{\rho^{(k)}_{p'_1}}$ as shown in \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:def:rho-k}.

Clearly, \Cref{lem:LOCC-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} is of the same format as \Cref{lem:LOCC-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:LOCC-3ZK-hyb01:proof:invariant}.

This finishes the proof for \Cref{lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:case-2}.


\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof:induction:sec} together finish the proof of \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} eventually.





\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb12}}

\xiao{almost copy the proof for \Cref{lem:LOCC-3ZK-hyb01}. Include it for demonstration of the 4-round baby case. In the final constant-round case, such a lemma is indeed generic reduciton step between $H'_{i-1}$ and $H'_{i}$.}

\begin{lemma}\label{lem:LOCC-3ZK-hyb12:proof:invariant}
Assume that the execution of $H'_1$ (and $H'_2$) \xiao{I think $H'_1$ is defined for fixed $p_1, p_2, u$} reaches Layer-3 for $K$ times in total. For each $k \in [K]$, there exist (potentially sub-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1, p'_2}}}_{(p'_1, p'_2) \in \bits^\ell\times\bits^\ell}$ so that the following holds: in hybrid $H'_1$ (resp.\ $H'_2$), when execution reaches Layer-3 for the $k$-th time, the overall state can be written as $\ket{\phi^{(k)}}$ (resp.\ $\ket{\psi^{(k)}}$) defined as follows
\begin{align}
\ket{\phi^{(k)}} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \red{\tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0}} \ket{\rho^{(k)}_{p'_1, p'_2}}, \label{lem:LOCC-3ZK-hyb12:proof:target-format:H1}
\\ 
\ket{\psi^{(k)}} 
& = 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p'_2}}\red{\tilde{U}_{6,1}} \ket{\rho^{(k)}_{p'_1, p'_2}}, \label{lem:LOCC-3ZK-hyb12:proof:target-format:H2}
\end{align}
where the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
\end{lemma}

\xiao{finish the proof of \Cref{lem:LOCC-3ZK-hyb12} using \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}.}







\subsection{Proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}}

Similar as in the proof of \Cref{sec:lem:LOCC-3ZK-hyb01:proof:invariant:proof}, 
we establish \Cref{lem:LOCC-3ZK-hyb12:proof:invariant} by a mathematical induction on the number $k \in [K]$ indicating it is which time the execution reaches Layer-3. We will keep track of how the overall states evolve in both $H'_1$ and $H'_2$ simultaneously.







\subsubsection{Base Case ($k = 1$)}
\label{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:sec} 


This corresponds to the very first time the execution reaches Layer-3. 

Notice that the execution has to reach Layer-2 before it reaches Layer-3. Notation-wise, let $\ket{\eta}$ denote the overall state at this particular arrival at Layer-2 (i.e., the one right before it reaches Layer-3 for the first time). It then follows from \Cref{lem:LOCC-3ZK-hyb01:proof:invariant} that $\ket{\eta}$ in game $H'_1$ can be written as
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:initial-state}
\ket{\eta} = \ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1} \ket{\rho_{p'_1}}.
\end{equation}
Moreover, this $\ket{\eta}$ is also the overall state at the same time point {\em in game $H'_2$}, simply because the games $H'_1$ and $H'_2$ are identical so far. Also, $\ket{\eta}$ will evolve in an identical manner in $H'_1$ and $H'_2$ until the first arrival at Layer. Formally, in both games, $\Sim$'s local operation $S_j$ is applied to $\ket{\eta}$. Then, the operator $\tilde{U}_6\tilde{U}_5\ketbra{p_1, p_2}_{\reg{p_1p_2}}\tilde{U}_4$ is applied, bringing the execution to Layer-3 for the first time. In summary, it holds that
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi-psi-equal}
\ket{\phi^{(1)}} = \ket{\psi^{(1)}} = \tilde{U}_6\tilde{U}_5\ketbra{p_1, p_2}_{\reg{p_1p_2}}\tilde{U}_4 S_j \cdot \ket{\eta}.
\end{equation}

In the following, we show that such a $\ket{\phi^{(1)}}$ (resp.\ $\ket{\psi^{(1)}}$) indeed satisfies the requirement as stipulated by  \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1} (resp.\ \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H2}) in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}.


\xiao{Check with @Nai-Hui if a sub-normalized state can be decomposed as in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:4}...}

\begin{align*}
\ket{\phi^{(1)}}
& = 
\tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}\tilde{U}_4 S_j \cdot \ket{\eta} \\
& =
 \tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}\tilde{U}_4  S_j 
\cdot \bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1}  \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:1} \\ 
& =
 \tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}\tilde{U}_4  
\cdot \bigg(
\ket{p_1}_{\reg{p_1}} S_j \ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_{3,1}  S^{\reg{t_1}/\reg{m}}_j \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:2} \\ 
& =
\tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}
\cdot \bigg(
\ket{p_1}_{\reg{p_1}} \tilde{U}_4 S_j \ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \tilde{U}_4 \tilde{U}_{3,1}  S^{\reg{t_1}/\reg{m}}_j \ket{\rho_{p'_1}}
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:3} \\ 
& =
\tilde{U}_6\tilde{U}_5\ketbra{p_1,p_2}_{\reg{p_1p_2}}
\cdot \bigg(
\ket{p_1}_{\reg{p_1}} \sum_{p'_2 \in \bits^{\ell}}\ket{p'_2}_{\reg{p_2}} \ket{\rho_{p_1, p'_2}} + \\
& \hspace{19em} 
\sum_{p'_1 \in \bits^{\ell} \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \sum_{p'_2 \in \bits^{\ell}}\ket{p'_2}_{\reg{p_2}} \ket{\rho_{p'_1, p'_2}} 
\bigg) \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:4} \\ 
& =
\tilde{U}_6\tilde{U}_5
\cdot 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho_{p_1, p_2}}  
\\ 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \tilde{U}_{6,0}\tilde{U}_{5,0} \ket{\rho_{p_1, p_2}} 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:5} \\ 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(1)}_{p_1, p_2}} 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:1} follows from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:initial-state}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:2} follows from the definitions of $S_j$ and $\tilde{U}_{3,1}$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:3} follows from the fact that $\tilde{U}_4$ works as identity on register $\reg{p_1}$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:4} follows from decomposing the $\reg{p_2}$ register in the computational basis for states $\tilde{U}_4 S_j \ket{\rho_{p_1}}$ and $\tilde{U}_4 \tilde{U}_{3,1}  S^{\reg{t_1}/\reg{m}}_j \ket{\rho_{p'_1}}$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:5} follows from the definitions of $\tilde{U}_5$ and $\tilde{U}_6$, and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6} follows by defining $\ket{\rho^{(1)}_{p_1, p_2}}  \coloneqq \tilde{U}_{6,0}\tilde{U}_{5,0} \ket{\rho_{p_1, p_2}}$.
% \begin{equation}\label[Expression]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:7}
% \forall p'_1 \in \bits^{\ell}, ~~\ket{\rho^{(1)}_{p'_1, p_2}}  \coloneqq \tilde{U}_{6,0}\tilde{U}_{5,0} \ket{\rho_{p'_1, p_2}}.
% \end{equation}

It is straightforward that \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6} is a special case of \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1} with $k=1$, as stipulated by \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. 

Also, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi-psi-equal,lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:phi:derivation:6} together imply that 
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:psi:derivation:1}
 \ket{\psi^{(1)}} = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(1)}_{p_1, p_2}}.
\end{equation}
Clearly, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:psi:derivation:1} is a special case of \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H2} with $k=1$, as stipulated by \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. 

This finishes the proof for the base case $k =1$.






\subsubsection{Induction Step ($k\ge 2$)} 
\label{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:sec} 

We assume $\ket{\phi^{(k-1)}}$ and $\ket{\psi^{(k-1)}}$ satisfies \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}, and prove in the following that \Cref{lem:LOCC-3ZK-hyb12:proof:invariant} holds when the execution reaches Layer-2 for the $k$-th time.





Consider the execution between the $(k-1)$-th arrival and $k$-th arrival at Layer-3. It can be described as follows:
\begin{enumerate}
\item
 $\Sim$ first applies the local operator $S_j$. Note that this step is identical for both $H'_1$ and $H'_2$.
 \item
An $\uparrow$-query is made, bringing the execution to Layer-2. 
\begin{itemize}
\item
In $H'_1$, this corresponds to applying $\tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6$;
\item
In $H'_2$, this corresponds to applying $\tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}} $ (as per \Cref{eq:B-dummy}). 
\end{itemize}

\item
The $(j+1)$-th local operation $S_{j+1}$ is applied. Note that this step is identical for both $H'_1$ and $H'_2$ as well.

\item
At this point, there are two cases to consider: 
\begin{enumerate}
\item \label[Case]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-1}
 $\Sim$ can make a $\downarrow$-query immediately, bringing the execution back to Layer-3; {\em or } 
\item \label[Case]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-2}
 $\Sim$ can rewind $\tilde{V}$ further, bringing the execution to Layer-1.  
\end{enumerate}
Fortunately, our proof (to appear shortly) can handle these two cases at one stroke. To do that, we denote the execution from this point until (exclusively) {\em the next $\downarrow$ query  from Layer-2 to Layer-3} (i.e., the exact query that yields the $k$-th arrival at Layer-3) as an operator $\Lambda$. $\Lambda$ might be the $(j+1)$-th local operator $S_{j+1}$ {\em only}, corresponding to \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-1}; $\Lambda$ might also be some non-identity operator, representing the operations performed in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-2} before the next arrival at Layer-3. We do not specify the exact form of $\Lambda$. But we high-light an important fact:
\begin{itemize}
 \item
 {\bf Fact:} for both \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-1,lem:LOCC-3ZK-hyb12:proof:invariant:proof:case-2-2}, $\Lambda$ works non-trivially only on registers $\reg{p_1}$, $\reg{m}$, $\reg{t_1}$, $\reg{s}$, $\reg{u}$'s  \xiao{This is true because the execution between Layer-1 and Layer-2 have already been replaced with dummy up-and-downs, which involves only swapping operations between $\reg{m}$ and $\reg{t}_1$. Need to provide a detailed explanation of this fact. Importantly, $\Lambda$ does not touch $\reg{p_2}$, $\reg{t_2}$, and $\reg{w}$.}  (i.e., it works as identity on other registers). 
 \end{itemize} 

\item
Finally, an $\downarrow$-query is made, bringing the execution back to Layer-3. 
\begin{itemize}
\item
In $H'_1$, this corresponds to applying $\tilde{U}_6 \tilde{U}_5 \tilde{U}_4$;
\item
In $H'_2$, this corresponds to applying $B_{\msf{dmy}} \tilde{U}_4$. 
\end{itemize}
\end{enumerate}

It follows from the above description that the states $\ket{\phi^{(k)}}$ and $\ket{\psi^{(k)}}$ can be written as:
\begin{align}
\ket{\phi^{(k)}}
& = \tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \ket{\phi^{(k-1)}}, \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi}\\ 
\ket{\psi^{(k)}}
& = B_{\msf{dmy}}\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}} S_j \cdot \ket{\psi^{(k-1)}}. \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}
\end{align}

\begin{remark}[High-Level Idea for the Sequel]
Recall that our eventual goal is to prove that the states $\ket{\phi^{(k)}}$ and $\ket{\psi^{(k)}}$ defined above can indeed be written in the format shown in \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1,lem:LOCC-3ZK-hyb12:proof:target-format:H2} in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. At a high level, we will prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi,lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}. But we first need to perform some preparation work, putting \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi,lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}. Then, we show on \Cpageref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish} how to combine \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} and \Cref{lem:err-inv-com} to complete the proof for the induction step. 
\end{remark}



\begin{MyClaim}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}
There exist (potentially sub-normalized) pure states $\Set{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds
\begin{align}
\ket{\phi^{(k)}}
& = \tilde{U}_6 \tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}}   \tilde{U}^\dagger_5 \tilde{U}^\dagger_6
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(k)}}
& = 
B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}}  B^\dagger_{\msf{dmy}}
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} 
\end{align}
where $\Lambda^{\reg{p_2}/\reg{m}}$ is identical to $\Lambda$ except that it treats register $\reg{p_2}$ as $\reg{m}$, and the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}]
First, notice that
\begin{equation}\label{lem:LOCC-3ZK-hyb12:proof:case-2:eq:swap-Lambda} 
\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 = \tilde{U}_4  \tilde{U}^\dagger_4 \Lambda^{\reg{p_2}/\reg{m}} = \Lambda^{\reg{p_2}/\reg{m}},
\end{equation}
where the first equality follows from the fact that $\Lambda^{\reg{p_2}/\reg{m}}$ does not operate on $\reg{p_2}$ and $\tilde{U}^\dagger_4$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_2}$.

\para{Proving \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(k)}}$:

\begin{align*}
\ket{\phi^{(k)}}
& = 
\tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \ket{\phi^{(k-1)}} \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1} \\
& = 
\tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} S_j \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1}  follows from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3} follows from \Cref{lem:LOCC-3ZK-hyb12:proof:case-2:eq:swap-Lambda}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  follows from the fact that $S_j$ works as identity on registers $\reg{p_1}$ and $\reg{p_2}$ (see \Cref{LOCC-3ZK:table:non-trivial-registers}), \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  follows from the definitions of $\tilde{U}_{6,1}$ and $S^{\reg{t_2}/\reg{m}}_j$, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  follows from the fact that $S^{\reg{t_2}/\reg{m}}_j$ and $\tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} $ act non-trivially on different registers (see \Cref{LOCC-3ZK:table:non-trivial-registers}), and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  follows by defining
\begin{equation}
\label[Expression]{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}
\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}} \coloneqq S_j \ket{\rho^{(k-1)}_{p_1, p_2}} ~~~\text{and}~~~ \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \coloneqq S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}~~~(\forall (p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}).
\end{equation}
\Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  finishes the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\para{Proving \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi}.} This proof is almost identical to the above proof for \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align*}
\ket{\psi^{(k)}}
& = 
B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \ket{\psi^{(k-1)}} \numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} \\
& = 
B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1}  \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2} \\ 
& =
B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}} B^\dagger_{\msf{dmy}} \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} \\ 
& =
\tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
\bigg) 
\numberthis \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}
,\end{align*}
where \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} follows from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2}  follows from our induction assumption, \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} follows from a similar argument as we did to \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6} from \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2}, and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4} follows from the same definition of $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$ and $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ as shown in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}

\Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}  finishes the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.


This eventually finishes the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\end{proof}


\para{Finishing the Induction Step.}\label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish} 
 With the above \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} in hand, we can finish the induction step by applying \Cref{lem:err-inv-com}. Formally, we apply \Cref{lem:err-inv-com} to the states and operators in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}, with the notation correspondence listed in \Cref{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}}
\label{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1}$, $\reg{p_2}$ & & $W_0$ & $\tilde{U}_{6,0}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_1$ & $\tilde{U}_{6,1}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_2}$ & & $W$   & $\tilde{U}_{6}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{t_1}$,  $\reg{u}$, $\reg{s}$ & & $\tilde{W}$ & $B_{\msf{dmy}}$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_0$ & $\tilde{U}_{5,0}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0} \\ 
\addlinespace[0.3em]
   & & & $U$   & $\tilde{U}_{5}$ & & $\ket{\eta^{(\msf{in})}_1}$ & \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}  \\ 
   \addlinespace[0.3em]
 &  & & $S$   & $\Lambda^{\reg{p_2}/\reg{m}}$ & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\phi^{(\msf{k})}}$  \\ 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\psi^{(\msf{k})}}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises of \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,0}$ (playing the role of $W_0$) who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$ (playing the role of registers $\reg{s}$).

\item
\Cref{lem:err-inv-com} requires that $W_1$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,1}$ (playing the role of $W_1$), who is a swap operator between registers $\reg{m}$ and $\reg{t_2}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively).

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_1$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $B_{\msf{dmy}}$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $\tilde{U}_{6,1}$ (playing the role of $W_1$) on branches $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, p'_2) \ne (p_1, p_2)$.

\item
 \Cref{lem:err-inv-com} requires that $U_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{5,0}$ (playing the role of $U_0$), who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of register $\reg{s}$).

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\Lambda^{\reg{p_2}/\reg{m}}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{p_2}$,  $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of registers $\reg{a}$ and $\reg{s}$).
\end{itemize}

Next, using the above notation, we could define
\begin{align}
\ket{\eta^{(\msf{in})}_0}
& \coloneqq 
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}   \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{4,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}, \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0}  \\ 
\ket{\eta^{(\msf{in})}_1}
& \coloneqq 
 \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}.  \label{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}   
\end{align}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:LOCC-3ZK-hyb12:proof:induction:cor-table}) to the $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ defined in \Cref{lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0,lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}. This implies the existence of (potentially non-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1, p'_2}}}_{(p'_1, p'_2) \in\bits^\ell \times \bits^\ell}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\phi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k)}_{p'_1,p'_2}} \\ 
\ket{\psi^{(k)}} 
& = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\rho^{(k)}_{p'_1,p'_2}} 
,\end{align*}
which are exactly \Cref{lem:LOCC-3ZK-hyb12:proof:target-format:H1,lem:LOCC-3ZK-hyb12:proof:target-format:H2} in  \Cref{lem:LOCC-3ZK-hyb12:proof:invariant}. 

This finishes the induction step.


\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:LOCC-3ZK-hyb12:proof:invariant:proof:induction:sec}   together finish the proof of \Cref{lem:LOCC-3ZK-hyb12:proof:invariant} eventually.






\UpdateLine
    











==> sections/CPM-full.tex <==

\section{CPM: Full Version}

In this section, we provide the proof of \Cref{lem:H:IND} for the general case (in contrast to the warm-up case $K =2$ shown in \Cref{sec:CMP:warm-up}).

Due to a similar argument as we did at the beginning of \Cref{sec:lem:CPM-3ZK:H01:proof}, we claim that: to prove \Cref{lem:H:IND}, it suffices to establish the following \Cref{lem:H:IND:proof:invariant}.
\begin{lemma}[Invariance in $H^{(J, \msf{pat})}_{k-1}$ and $H^{(J, \msf{pat})}_{k}$]
\label{lem:H:IND:proof:invariant}
For a $(J, \msf{pat})$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized} and a $k \in [K]$, assume that during the execution of $H^{(J, \msf{pat})}_{k-1}$ (and $H^{(J, \msf{pat})}_{k}$), the global counter reaches value $k$ for $T$ times in total. For each $t \in [T]$, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}}_{p'_1, \ldots, p'_k \in \bits^{k\ell}}$ so that the following holds: in hybrid $H^{(J, \msf{pat})}_{k-1}$ (resp.\ $H^{(J, \msf{pat})}_{k}$), when the global counter reaches value $k$ for the $t$-th time, the overall state can be written as the $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows:
\begin{align}
\ket{\phi^{(t)}} 
& =  
\ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \ket{\rho^{(t)}_{p_1, \ldots, p_k}}  ~+~
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1} \ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}, 
   \label{lem:H:IND:proof:invariant:target-format:Hk-1}\\ 
\ket{\psi^{(t)}} 
& =  
\ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \ket{\rho^{(t)}_{p_1, \ldots, p_k}}  ~+~
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}  \red{C_{k,0}} \ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}
 \label{lem:H:IND:proof:invariant:target-format:Hk}
,\end{align}
where the summations are taken over all $(p'_1, \ldots, p'_k) \in \bits^{k\ell} \setminus \Set{(p_1, \ldots, p_k)}$ (abbreviated as $(p'_1, \ldots, p'_k) \ne (p_1, \ldots, p_k)$ in the above), the $(p_1, \ldots, p_k)$ are defined in $\msf{pat}$, and the unitaries $B_{k,1}$, $C_{k,0}$, and $C_{k,1}$  are as defined in \Cref{re-define:unitaries}. 
\end{lemma}



\para{Proving \Cref{lem:H:IND:proof:invariant}.} Similar as the proofs for \Cref{lem:CPM-3ZK-hyb01:proof:invariant,lem:CPM-3ZK-hyb12:proof:invariant}, 
we establish \Cref{lem:H:IND:proof:invariant} through mathematical induction on the number $t \in [T]$, indicating the time at which the global counter reaches the value $k$. Throughout this proof, we will monitor the evolution of the overall states in both $H^{(J, \msf{pat})}_1$ and $H^{(J, \msf{pat})}_2$ simultaneously. This is done in \Cref{sec:lem:H:IND:proof:invariant:base,sec:lem:H:IND:proof:invariant:induction} respective.





\subsection{Base Case ($t = 1$)}
\label{sec:lem:H:IND:proof:invariant:base}

We first derive how the overall state evolves in $H^{(J, \msf{pat})}_{k-1}$. 

This base case corresponds to the very first time the global counter reaches value $k$. By definition, this is due to the $\msf{sq}(k)$ query. 


We assume w.l.o.g.\ that the overall state right before this query is some pure state $\ket{\rho}$. Then, by definition, the $\msf{sq}(k)$ query corresponds to the following procedure: $\Sim$ first applies her local unitary $S$ (followed by the projector $\ketbra{\downarrow}_{\reg{u}}$ which we hide as per \Cref{rmk:CPM-3ZK:hid-proj-u}). Next, according to the notation in \Cref{MnR:game:redefine:hybrids}, the operator $D_kC_kB_k \ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} A_k U_{gc}$ will be applied. In summary, the state $\ket{\phi^{(1)}}$ in $H^{(J, \msf{pat})}_1$ can be written as follows:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_kC_kB_k \ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} A_k U_{gc} S   
\ket{\rho}
\\
& =  
D_kC_kB_k \ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} 
\ket{\dot{\rho}_{p_1, \ldots, p_k}}  
\numberthis \label{H:IND:proof:invariant:base:eq:1}\\
& =  
 \ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} 
D_{k,1} C_{k,1} B_{k,1} \ket{\rho_{p_1, \ldots, p_k}}  
\numberthis \label{H:IND:proof:invariant:base:eq:2}\\
& =  
 \ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} 
 \ket{\rho^{(1)}_{p_1, \ldots, p_k}}  
\numberthis \label{H:IND:proof:invariant:base:eq:3}
,\end{align*}
where
\begin{itemize}
\item
\Cref{H:IND:proof:invariant:base:eq:1} follows by defining
$
\ket{\rho_{p_1, \ldots, p_k}} 
\coloneqq 
\bra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} A_k U_{gc} S \ket{\rho}  
$;

\item 
\Cref{H:IND:proof:invariant:base:eq:2} follows from the definitions of $B_k$, $C_k$, and $D_k$ (see \Cref{re-define:unitaries});

\item 
\Cref{H:IND:proof:invariant:base:eq:3} follows by defining $ \ket{\rho^{(1)}_{p_1, \ldots, p_k}}  \coloneqq D_{k,1} C_{k,1} B_{k,1} \ket{\rho_{p_1, \ldots, p_k}}$.	
\end{itemize}
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{H:IND:proof:invariant:base:eq:3} satisfies the format shown in \Cref{lem:H:IND:proof:invariant:target-format:Hk-1} when $t = 1$.



Also, note that the game $H^{(J, \msf{pat})}_{k-1}$ and $H^{(J, \msf{pat})}_{k}$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{H:IND:proof:invariant:base:eq:3} that 
$$
\ket{\psi^{(1)}} 
=  
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} 
 \ket{\rho^{(1)}_{p_1, \ldots, p_k}}.
$$ 
 Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:H:IND:proof:invariant:target-format:Hk} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.



\subsection{Induction Step ($t \ge 2$)} 
\label{sec:lem:H:IND:proof:invariant:induction}

 \xiao{add remark for the induction step. Going up is handled as in the proof of XXX and going down is handled as in the proof of xxx.}

We assume $\ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t-1)}}$ satisfy the requirements in \Cref{lem:H:IND:proof:invariant}, and show in the following that \Cref{lem:H:IND:proof:invariant} holds when the global counter reaches $k$ for the $t$-th time.

We establish this claim by considering the following MECE (mutually exclusive and collectively exhaustive) cases:
\begin{enumerate}
\item \label[Case]{H:IND:proof:invariant:induction:case-1}
{\bf Case 1:} The $t$-th arrival at value $k$ happens because of the following operations performed by the simulator $\Sim$: 
\begin{enumerate}
\item 
$\Sim$ first applies her local unitary $S$ and then makes\footnote{Recall that this is determined by measuring the $\reg{u}$ reigster. And further recall that this measurement is replaced with the projector $\ketbra{\downarrow}_\reg{u}$ because we are in the sub-normalized game (see \Cref{MnR:game:redefine:hybrids}).} an $\uparrow$-query, which brings the global counter to $k-1$;

\item \label[Step]{H:IND:proof:invariant:induction:case-1:2}
Next, $\Sim$ could perform any operations, as long as they keep the global counter $\le k-1$. For instance, $\Sim$ can choose to further rewind the execution by making another $\uparrow$-query, or $\Sim$ can choose to make $\uparrow$ and $\downarrow$ queries that cause the global counter to jump between $i-1$ and $i$ as long as $i \le k-1$. The only restriction is that $\Sim$ will not bring the global counter back to $k$ (which is captured by the next step).

\vspace{0.5em}
{\bf Defining Operator $\Upsilon$:} We define the operations performed by $\Sim$ as an operator $\Upsilon$.

\item
After the application of $\Upsilon$, the simulator $\Sim$ eventually makes a $\downarrow$-query that bring the global counter back to $k$ (i.e., exactly the $t$-th arrival at value $k$).
\end{enumerate}

\item \label[Case]{H:IND:proof:invariant:induction:case-2}
{\bf Case 1:} The $t$-th arrival at value $k$ happens because of the following operations performed by the simulator $\Sim$: 
\begin{enumerate}
\item \label[Step]{H:IND:proof:invariant:induction:case-2:1}
$\Sim$ first applies her local unitary $S$ and then makes a $\downarrow$-query, which brings the global counter to $k+1$;

\item \label[Step]{H:IND:proof:invariant:induction:case-2:2}
Next, $\Sim$ could perform any operations, as long as they keep the global counter $\ge k+1$. For instance, $\Sim$ can choose to make another $\downarrow$-query, or $\Sim$ can choose to make $\uparrow$ and $\downarrow$ queries that cause the global counter to jump between $i$ and $i+1$ as long as $i \ge k+1$. The only restriction is that $\Sim$ will not bring the global counter back to $k$ (which is captured by the next step).

\item \label[Step]{H:IND:proof:invariant:induction:case-2:3}
After the application of $\Lambda$, the simulator $\Sim$ eventually makes a $\uparrow$-query that bring the global counter back to $k$ (i.e., exactly the $t$-th arrival at value $k$).
\end{enumerate}
Note that \Cref{H:IND:proof:invariant:induction:case-2:1,H:IND:proof:invariant:induction:case-2:2,H:IND:proof:invariant:induction:case-2:3} described above not only transition $\ket{\phi^{(t-1)}}$ to $\ket{\phi^{(t)}}$, but they also transition $\ket{\psi^{(t-1)}}$ to $\ket{\psi^{(t)}}$. This is because these three steps maintain the global counter $\ge k$, and $H^{(J, \msf{pat})}_{k-1}$ and $H^{(J, \msf{pat})}_{k}$ behave identically by definition until the global counter returns to $k$ (see \Cref{MnR:game:redefine:hybrids}).


\vspace{0.5em}
{\bf Defining Operator $\Lambda$:} We define the operations performed in \Cref{H:IND:proof:invariant:induction:case-2:1,H:IND:proof:invariant:induction:case-2:2,H:IND:proof:invariant:induction:case-2:3} as an operator $\Lambda$.
\end{enumerate}
In the following, we show the proof for these two cases in \Cref{H:IND:proof:invariant:induction:case-1:sec,H:IND:proof:invariant:induction:case-1:sec} respectively.

\subsubsection{Proving the Induction Step: \Cref{H:IND:proof:invariant:induction:case-1}}
\label{H:IND:proof:invariant:induction:case-1:sec}


We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) in \Cref{H:IND:proof:invariant:induction:case-1}. According to the description in \Cref{H:IND:proof:invariant:induction:case-1} and our notation in \Cref{MnR:game:redefine:hybrids}, it is clear that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ in this case can be written respectively as:
\begin{align}
\ket{\phi^{(t)}}
& = D_k C_k B_k A_k U_{gc} \Upsilon U^{\dagger}_{gc} A^\dagger_k B^\dagger_k C^\dagger_k D^\dagger_k S  \ket{\phi^{(t-1)}} \label{H:IND:proof:invariant:induction:case-1:eq:phi}\\ 
\ket{\psi^{(t)}}
& = D_k \ddot{C}_k A_k U_{gc} \Upsilon  U^{\dagger}_{gc} A^\dagger_k \ddot{C}^\dagger_k D^\dagger_k S \ket{\psi^{(t-1)}} \label{H:IND:proof:invariant:induction:case-1:eq:psi}
,\end{align}
where the operator $\Upsilon$ is defined in \Cref{H:IND:proof:invariant:induction:case-1:2}.

We first make a useful claim that specifies the registers on which the operator $\Upsilon$ (defined in \Cref{H:IND:proof:invariant:induction:case-1:2}) acts non-trivially. This claim can be treated as the analog of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}.
\begin{MyClaim}[Non-Trivial Registers for $\Upsilon$]\label{H:IND:proof:invariant:induction:case-1:Upsilon-register:claim}
The $\Upsilon$ defined in \Cref{H:IND:proof:invariant:induction:case-1:2} acts non-trivially only on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1 \ldots p_{k-1}}$, $\reg{t_1  \ldots t_{k-1}}$, $\reg{lc}$, and $\reg{gc}$ (i.e., it works as the identity operator on the other registers). 
\end{MyClaim}
\begin{proof}[Proof of \Cref{H:IND:proof:invariant:induction:case-1:Upsilon-register:claim}]
By definition, $\Upsilon$ only contains operations that happen when the global counter is $k-1$ or smaller. 

Also, recall that we are talking about hybrids $H^{(J, \msf{pat})}_{k-1}$ and $H^{(J, \msf{pat})}_{k}$ now. Thus, all the $\downarrow$ and $\uparrow$ queries happening at global counter $i \le k-1$ will be answered by the ``dummy'' operators $\ddot{V}$ and $\ddot{V}^\dagger$ respective. (One exception is the $\tilde{V}$ corresponding $\msf{sq}(i)$. But this does not matter in the current proof---Right before the behaviors defined in \Cref{H:IND:proof:invariant:induction:case-1} happen, the global counter is already $k$, which implies that $\msf{sq}(i)$ ($\forall i \in [k]$) has already happened and thus cannot be a part of the operator $\Upsilon$.)

Therefore, according to our notation in \Cref{MnR:game:redefine:hybrids}, operator $\Upsilon$ can be written as $\Upsilon = \Gamma_z \Gamma_{z-1} \cdots \Gamma_1$ (for some integer $z$) where each $\Gamma_i$ ($i \in [z]$) comes from the set of operators $\Set{S, U_{gc}} \cup \Set{A_i}_{i \in [k-1]} \cup \Set{\ddot{C}_i}_{i \in [k-1]} \cup \Set{D_i}_{i \in [k-1]}$. It then follows from \Cref{CPM-3ZK:non-trivial-registers:table} that $\Upsilon$ acts non-trivially only on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1 \ldots p_{k-1}}$, $\reg{t_1  \ldots t_{k-1}}$, $\reg{lc}$, and $\reg{gc}$.

This completes the proof of \Cref{H:IND:proof:invariant:induction:case-1:Upsilon-register:claim}.

\end{proof}



\para{High-Level Idea for the Sequel.} \xiao{chech the crefs} Recall that our eventual goal is to prove that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ are of the format shown in \Cref{lem:H:IND:proof:invariant:target-format:Hk-1,lem:H:IND:proof:invariant:target-format:Hk} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{H:IND:proof:invariant:induction:case-1:eq:phi,H:IND:proof:invariant:induction:case-1:eq:psi}. But we first need to perform some preparation work, putting \Cref{H:IND:proof:invariant:induction:case-1:eq:phi,H:IND:proof:invariant:induction:case-1:eq:psi} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim,H:IND:proof:invariant:induction:case-1:preparation-claim:2}. Then, we show on \Cpageref{H:IND:proof:invariant:induction:case-1:finish} how to use \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim,H:IND:proof:invariant:induction:case-1:preparation-claim:2} to complete the proof for the induction step. 

The following \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim} can be treated as an analog of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\begin{MyClaim}\label{H:IND:proof:invariant:induction:case-1:preparation-claim}
There exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}_{(p'_1, \ldots, p'_k) \in \bits^{k\ell}}$ so that the following holds
\begin{align*}
\ket{\phi^{(t)}}
& =  
D_k C_k B_k U_{gc} \Upsilon^{\reg{p_k}/\reg{m}} U_{gc}^\dagger   B^\dagger_k C^\dagger_k
\bigg( 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}  
+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}} 
\bigg) \numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(t)}}
& = 
D_k\ddot{C}_k U_{gc}\Upsilon^{\reg{p_k}/\reg{m}}  U_{gc}^\dagger \ddot{C}^\dagger_k 
\bigg( 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}  
+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}  
\bigg) 
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:psi}
\end{align*}
where $\Upsilon^{\reg{p_k}/\reg{m}}$ is identical to the $\Upsilon$ defined in \Cref{H:IND:proof:invariant:induction:case-1:2}, except that it treats register $\reg{p_k}$ as $\reg{m}$, and the summations are taken over all $(p'_1, \ldots, p'_k) \in \bits^{k\ell}\setminus \Set{(p_1, \ldots, p_k)}$ (abbreviated as $(p'_1, \ldots, p'_k) \ne (p_1, \ldots, p_k)$ in the above).
\end{MyClaim}
\begin{proof}[Proof of \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim}]
First, notice that  
\begin{align*}
 A_k U_{gc} \Upsilon U^\dagger_{gc} A^\dagger_k 
 & = 
 A_k U_{gc} \Upsilon A^\dagger_k U^\dagger_{gc}
 \numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S:1} \\ 
 & = 
 A_k U_{gc} A^\dagger_k \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S:2} \\
  & = 
 A_k A^\dagger_k U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S:3} \\
 & = 
U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S:1,H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S:3} follows from the fact that $U_{gc}$ acts non-trivially on different registers from $A_k$;

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S:2} from the fact that $\Upsilon$ acts as the identity operator on $\reg{p_k}$ (see \Cref{H:IND:proof:invariant:induction:case-1:Upsilon-register:claim}) and that $A_k$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_k}$ (see \Cref{CPM-3ZK:V:unitary}). 
\end{itemize}

\subpara{Proving \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(t)}}$:
\begin{align*}
\ket{\phi^{(t)}}
& =
D_k C_k B_k A_k U_{gc} \Upsilon U^{\dagger}_{gc} A^\dagger_k B^\dagger_k C^\dagger_k D^\dagger_2  S \ket{\phi^{(t-1)}}
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:0} \\ 
& =
D_k C_k B_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k D^\dagger_k  S \ket{\phi^{(t-1)}}
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:1} \\ 
& =
D_kC_kB_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k D^\dagger_k S 
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}} 
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:2} \\ 
& =
D_kC_kB_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k D^\dagger_k  
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} S \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}} S C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:3} \\ 
& =
D_kC_kB_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k  
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} D^\dagger_{k,1} S \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}} S C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:4} \\ 
& =
D_kC_kB_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k  
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} D^\dagger_{k,1} S \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{12em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} S^{\reg{t_k}/\reg{m}} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:5} \\ 
& =
D_kC_kB_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k  
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} D^\dagger_{k,1} S \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{12em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} S^{\reg{t_k}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:6} \\ 
& =
D_kC_kB_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc} B^\dagger_k C^\dagger_k  
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{12em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} \ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:0} follows from \Cref{H:IND:proof:invariant:induction:case-1:eq:phi};

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:1} follows from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S};

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:2} follows from our induction assumption;

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:3} from  from the fact that $S$ acts as the identity operator on registers $\reg{p_1 \ldots p_k}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:4} from the definition of $D_k$ (see \Cref{re-define:unitaries});

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:5} from the fact that $S$ acts as the identity operator on $\reg{t_k}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}) and $C_{k,0}$ is nothing but a swap operator between $\reg{t_k}$ and $\reg{m}$ (see \Cref{re-define:unitaries}); (Note that $S^{\reg{t_k}/\reg{m}}$ is defined to be an operator that is identical to $S$ except that it treats $\reg{t_k}$ as $\reg{m}$.)

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:6} follows from the fact that $S^{\reg{t_k}/\reg{m}}$ acts non-trivially on different registers from $B_{k,1}$ and $C_{k,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:7} follows by defining 
\begin{equation}
\label[Expression]{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:def:rho-dot}
\begin{cases}
\ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}   \coloneqq D^\dagger_{k,1} S \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}} & 
\vspace{0.3em} \\
\ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}  \coloneqq S^{\reg{t_k}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}} & ~~\forall (p'_1, \ldots, p'_k) \in \big(\bits^{k\ell} \setminus \Set{(p_1, \ldots, p_k)}\big).
\end{cases}
\end{equation}
\end{itemize}
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:7} finishes the proof of \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:phi} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim}.


\subpara{Proving \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:psi}.} We now show the derivation for $\ket{\psi^{(t)}}$. This is almost identical to the above proof for \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align*}
\ket{\psi^{(t)}}
& =
D_k \ddot{C}_k A_kU_{gc} \Upsilon U^{\dagger}_{gc} A^\dagger_k \ddot{C}^\dagger_k D^\dagger_k  S \ket{\psi^{(t-1)}}
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:0} \\ 
& =
D_k \ddot{C}_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_k D^\dagger_k  S \ket{\psi^{(t-1)}}
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:1} \\ 
& =
D_k \ddot{C}_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_k D^\dagger_k  S  
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}} 
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:2} \\ 
& =
D_k \ddot{C}_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_k   
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} D^\dagger_{k,1}  S \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{15em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} S^{\reg{t_k}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}} 
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:6} \\ 
& =
D_k \ddot{C}_k  U_{gc} \Upsilon^{\reg{p_k}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_k 
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}  
~+ \\ 
& \hspace{12em} 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} \ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}
\bigg)
\numberthis \label{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:0} follows from \Cref{H:IND:proof:invariant:induction:case-1:eq:psi};

\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:1} follows from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:eq:swap-S};


\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:2}  follows from our induction assumption;


\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:6} follows from a similar argument as we did to derive \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:6} from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:phi-derivation:2};


\item
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:7} follows from {\em the same definitions} of $\ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}$ and $\ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}$ as shown in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:def:rho-dot}.
\end{itemize}
\Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:psi-derivation:7} finishes the proof of \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:psi} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim}.

\vspace{1em}
This completes the proof of \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim}.

\end{proof}


The following \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} can be treated as an analog of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}. 
\begin{MyClaim}\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2}
Let $\Upsilon^{\reg{p_k}/\reg{m}}$ and $\Set{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}_{(p'_1, \ldots, p'_k ) \in \bits^{k\ell}}$ be as defined in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim}. Let
\begin{align}
\ket{\gamma^{(t-1)}_0} 
& \coloneqq 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}} 
\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:in:0} \\ 
\ket{\gamma^{(t-1)}_1} 
& \coloneqq 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}  
\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:in:1} \\ 
\ket{\gamma^{(t)}_0} 
& \coloneqq 
 C_k B_k U_{gc} \Upsilon^{\reg{p_k}/\reg{m}} U_{gc}^\dagger   B^\dagger_k C^\dagger_k \ket{\gamma^{(t-1)}_0} 
\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:out:0} \\ 
\ket{\gamma^{(t)}_1}
& \coloneqq 
\ddot{C}_k U_{gc}\Upsilon^{\reg{p_k}/\reg{m}}  U_{gc}^\dagger \ddot{C}^\dagger_k 
 \ket{\gamma^{(t-1)}_1}
\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:out:1} 
.\end{align}
Then, there exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}_{(p'_1, \ldots, p'_k ) \in \bits^{k\ell}}$ so that the following holds:
\begin{align}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}  
\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:target:0} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}} 
\label{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:target:1} 
.\end{align}
\end{MyClaim}
\begin{proof}[Proof of \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}]
This claim follows from an application of \Cref{lem:err-inv-com}, with the notation correspondence listed in \Cref{H:IND:proof:invariant:induction:case-1:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}}
\label{H:IND:proof:invariant:induction:case-1:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{90pt} c C{50pt} C{70pt} c C{50pt} C{80pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1 \ldots p_k}$  & & $W_1$ & $C_{k,1}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_0$ & $C_{k,0}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1, \ldots,p'_k}_{\reg{p_1 \ldots p_k}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_k}$ & & $W$   & $C_{k}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p_1, \ldots, p_k}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u}$, $\reg{s}$, $\reg{t_1 \ldots t_{k-1}}$, $\reg{gc}$, $\reg{lc}$ & & $\tilde{W}$ & $\ddot{C}_k$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p'_1, \ldots, p'_k}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_1$ & $B_{k,1}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & $\ket{\gamma^{(t-1)}_0}$ \\ 
\addlinespace[0.3em]
   & & & $U$   & $B_k$ & & $\ket{\eta^{(\msf{in})}_1}$ & $\ket{\gamma^{(t-1)}_1}$  \\ 
\addlinespace[0.3em]
 &  & &   $S$   & $U_{gc}\Upsilon^{\reg{p_k}/\reg{m}}U^\dagger_{gc}$ & &  $\ket{\rho^{(\msf{out})}_a}_\reg{mtso}$    & $\ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}$  \\ 
\addlinespace[0.3em]
  &  & &   &  & &  $\ket{\rho^{(\msf{out})}_{a'}}_\reg{mtso}$     & $\ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}$  \\  
  \addlinespace[0.3em]
 &  & & & & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\gamma^{(t)}_0}$  \\
\addlinespace[0.3em] 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\gamma^{(t)}_1}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{H:IND:proof:invariant:induction:case-1:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_1$ should act as the identity operator on register $\reg{s}$. In terms of the \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} notation, this is satisfied by $C_{k,1}$ (playing the role of $W_1$) who works as identity on registers $\reg{u}$, $\reg{s}$, $\reg{t_1\ldots t_{k-1}}$, $\reg{gc}$, and $\reg{lc}$ (playing the role of registers $\reg{s}$). (Recall $C_{k,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)


\item
\Cref{lem:err-inv-com} requires that $W_0$ should be the swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} notation, this is satisfied by $C_{k,0}$ (playing the role of $W_0$), who is the swap operator between registers $\reg{m}$ and $\reg{t_k}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively). (Recall $C_{k,0}$ from \Cref{re-define:unitaries}.)

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_0$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} notation, this is satisfied by $\ddot{C}_k$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $C_{k,0}$ (playing the role of $W_0$) on branches $\ket{p'_1, \ldots, p'_k}_{\reg{p_1\ldots p_k}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, \ldots, p'_k) \ne (p_1, \ldots, p_k)$. (Recall $\ddot{C}_k$ from \Cref{re-define:unitaries})

\item
 \Cref{lem:err-inv-com} requires that $U_1$ should work as identity on register $\reg{s}$. In terms of the \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} notation, this is satisfied by $B_{k,1}$ (playing the role of $U_1$), who works as identity on registers $\reg{u}$, $\reg{s}$, $\reg{t_1\ldots t_{k-1}}$, $\reg{gc}$, and $\reg{lc}$ (playing the role of register $\reg{s}$). (Recall $B_{k,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2} notation, this is satisfied by $U_{gc}\Upsilon^{\reg{p_k}/\reg{m}}U^\dagger_{gc}$ (playing the role of $S$)---recall from \Cref{H:IND:proof:invariant:induction:case-1:Upsilon-register:claim} that $\Upsilon$ acts non-trivially on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1\ldots p_{k-1}}$, $\reg{t_1 \ldots t_{k-1}}$, $\reg{lc}$, and $\reg{gc}$. Thus, $U_{gc}\Upsilon^{\reg{p_k}/\reg{m}}U^\dagger_{gc}$ acts non-trivially on registers $\reg{p_k}$, $\reg{u}$, $\reg{s}$, $\reg{p_1 \ldots p_{k-1}}$, $\reg{t_1 \ldots t_{k-1}}$, $\reg{lc}$, and $\reg{gc}$, which constitute registers $\reg{a}$ and $\reg{s}$ (see \Cref{H:IND:proof:invariant:induction:case-1:cor-table}). 
\end{itemize}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{H:IND:proof:invariant:induction:case-1:cor-table}) to the $\ket{\gamma^{(t-1)}_0}$ and $\ket{\gamma^{(t-1)}_1}$ defined in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:in:0,H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:in:1}  (playing the role of $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ in \Cref{lem:err-inv-com}). This implies the existence of (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}}_{(p'_1, \ldots, p'_k)\in\bits^{k\ell}}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}}  \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+  
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1\ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}   \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}}  \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+  
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1\ldots p_k}}  C_{k,0}  \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}   
,\end{align*}
which are exactly \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:target:0,H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:target:1} in  \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}. 






This completes the proof of \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}.

\end{proof}



\para{Finishing the Proof for the Induction Step.}\label{H:IND:proof:invariant:induction:case-1:finish} With \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim,H:IND:proof:invariant:induction:case-1:preparation-claim:2} at hand, we now finish the proof for the induction Step.

\subpara{Proof for \Cref{lem:H:IND:proof:invariant:target-format:Hk-1}.} We first establish \Cref{lem:H:IND:proof:invariant:target-format:Hk-1}:
\begin{align}
\ket{\phi^{(t)}} 
& = D_k \ket{\gamma^{(t)}_0} 
\label{H:IND:proof:invariant:induction:case-1:final:phi:1} \\ 
& = D_k 
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}   
\bigg) 
\label{H:IND:proof:invariant:induction:case-1:final:phi:2} \\ 
& = 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} D_{k,1} \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}  
\label{H:IND:proof:invariant:induction:case-1:final:phi:3} \\ 
& = 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\rho^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1}  \ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}   
\label{H:IND:proof:invariant:induction:case-1:final:phi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{H:IND:proof:invariant:induction:case-1:final:phi:1} follows from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:phi} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim} and \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:out:0} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}; 

\item
\Cref{H:IND:proof:invariant:induction:case-1:final:phi:2} follows from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:target:0} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2};

\item
\Cref{H:IND:proof:invariant:induction:case-1:final:phi:3} follows from the definition of $D_k$ (see \Cref{re-define:unitaries});

\item
\Cref{H:IND:proof:invariant:induction:case-1:final:phi:4} follows by defining
\begin{equation}
\label[Expression]{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:def:rho}
\begin{cases}
\ket{\rho^{(t)}_{p_1,\ldots,p_k}}   
\coloneqq 
D_{k,1} \ket{\dot{\rho}^{(t)}_{p_1,\ldots,p_k}} & 
\vspace{0.3em}\\
\ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}  
\coloneqq 
\ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}} & \forall (p'_1, \ldots, p'_k) \in \big(\bits^{k\ell} \setminus \Set{(p_1, \ldots, p_k)}\big).
\end{cases}
\end{equation}
\end{itemize}
Note that \Cref{H:IND:proof:invariant:induction:case-1:final:phi:4} is exactly 
\Cref{lem:H:IND:proof:invariant:target-format:Hk-1} in \Cref{lem:H:IND:proof:invariant}. 


\subpara{Proof for \Cref{lem:H:IND:proof:invariant:target-format:Hk}.} Next, we establish \Cref{lem:H:IND:proof:invariant:target-format:Hk}:
\begin{align}
\ket{\psi^{(t)}} 
& = D_k \ket{\gamma^{(t)}_1} 
\label{H:IND:proof:invariant:induction:case-1:final:psi:1} \\ 
& = D_k 
\bigg(
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}  \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}   
\bigg) 
\label{H:IND:proof:invariant:induction:case-1:final:psi:2} \\ 
& = 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} D_{k,1} \ket{\dot{\rho}^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}   \ket{\dot{\rho}^{(t)}_{p'_1, \ldots, p'_k}}  
\label{H:IND:proof:invariant:induction:case-1:final:psi:3} \\ 
& = 
\ket{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \ket{\rho^{(t)}_{p_1, \ldots, p_k}}  
+ 
\sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)}  \ket{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}}  C_{k,0}   \ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}   
\label{H:IND:proof:invariant:induction:case-1:final:psi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{H:IND:proof:invariant:induction:case-1:final:psi:1} follows from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:eq:target:psi} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim} and \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:out:1} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2}; 

\item
\Cref{H:IND:proof:invariant:induction:case-1:final:psi:2} follows from \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2:eq:target:1} in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:2};

\item
\Cref{H:IND:proof:invariant:induction:case-1:final:psi:3} follows from the definition of $D_k$ (see \Cref{re-define:unitaries});

\item
\Cref{H:IND:proof:invariant:induction:case-1:final:psi:4} follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1,\ldots,p_k}}$ and $\ket{\rho^{(t)}_{p'_1,\ldots,p'_k}}$ shown in \Cref{H:IND:proof:invariant:induction:case-1:preparation-claim:proof:def:rho}.
\end{itemize}
Note that \Cref{H:IND:proof:invariant:induction:case-1:final:psi:4} is exactly 
\Cref{lem:H:IND:proof:invariant:target-format:Hk} in \Cref{lem:H:IND:proof:invariant}. 

\vspace{1em}
This completes the proof of the induction step of \Cref{lem:H:IND:proof:invariant} for \Cref{H:IND:proof:invariant:induction:case-1}.


\subsubsection{Proving the Induction Step: \Cref{H:IND:proof:invariant:induction:case-2}}
\label{H:IND:proof:invariant:induction:case-2:sec}


According to the description of \Cref{H:IND:proof:invariant:induction:case-2}, it holds that
\begin{align}
\ket{\phi^{(t)}} 
& = 
\Lambda \ket{\phi^{(t-1)}} 
\label{H:IND:proof:invariant:induction:case-2:initial:phi} \\ 
\ket{\psi^{(t)}} 
& = 
\Lambda \ket{\psi^{(t-1)}}
\label{H:IND:proof:invariant:induction:case-2:initial:psi}
,\end{align} 
where recall that the operator $\Lambda$ was defined toward the end of the description of \Cref{H:IND:proof:invariant:induction:case-2}.

\para{Structure of $\Lambda$.} While the exact format of $\Lambda$ will not be substantial, our proof of \Cref{H:IND:proof:invariant:induction:case-2} will rely on certain properties of $\Lambda$. We formalize these useful properties in the following \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}, which can be treated as an analog of \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.
\begin{MyClaim}\label{H:IND:proof:invariant:induction:case-2:claim:operator-commute}
For the operator $\Lambda$ defined above, there exist two operators $\Lambda_0$ and $\Lambda_1$ so that
\begin{itemize}
\item
both  $\Lambda_1$ and $\Lambda_0$ act as the identity operator on $\reg{p_1\ldots p_k}$;
\item
$\Lambda_0$ acts as the identity operator on $\reg{t_k}$;
\end{itemize}
and the following holds
\begin{align}
& 
\Lambda = \ketbra{p_1, \ldots,p_k}_{\reg{p_1\ldots p_k}} \tensor \Lambda_1 + \sum_{(p'_1,\ldots,p'_k) \ne (p_1, \ldots, p_k)}\ketbra{p'_1, \ldots,p'_k}_{\reg{p_1\ldots p_k}} \tensor \Lambda_0, \label{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:1} \\ 
& 
\Lambda_0 C_{k,0}  = C_{k,0} \Lambda^{\reg{t_k}/\reg{m}}_0, \label{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:2} \\ 
& 
\Lambda_0 C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} = C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} \Lambda^{\reg{t_k}/\reg{m}}_0 \label{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:3} 
,\end{align}
where $\Lambda^{\reg{t_k}/\reg{m}}_0$ is identical to $\Lambda_0$ except that it treats $\reg{t_k}$ as $\reg{m}$, and the summation is taken over all $(p'_1, \ldots, p'_k) \in \bits^{k\ell}\setminus \Set{(p_1, \ldots, p_k)}$ (abbreviated as $(p'_1, \ldots, p'_k) \ne (p_1, \ldots, p_k)$ in the above).  
\end{MyClaim}
\begin{proof}[Proof of \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}]

First, note that $\Lambda$ can be written as $\Lambda = \Gamma_z \Gamma_{z-1} \cdots \Gamma_1$ (for some integer $z$), where each $\Gamma_i$ ($i \in [z]$) comes from the following set 
\begin{equation}\label[Expression]{H:IND:proof:invariant:induction:case-2:claim:operator-commute:set}
\Set{S,  U_{gc}} \cup \Set{(A_i, B_i, C_i, D_i)}_{i \in \Set{k+1, k+2, \ldots, K}} \cup \Set{\ketbra{p_1, \ldots, p_i}_{\reg{p_1\ldots p_i}}}_{i \in \Set{k+1, k+2, \ldots, K}}.
\end{equation} 
This is because $\Lambda$ only corresponds to the operations that happen when the global counter ``jumps'' between some $i$ and $i+1$ with $i \ge k$ (see \Cref{MnR:game:redefine:hybrids}). We remark that $\Sim$ may also apply projectors on $\reg{u}$, but we consider it as a part of $S$ as per \Cref{rmk:CPM-3ZK:hid-proj-u}.


Therefore, to prove \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}, it suffices to show that for each operator $\Gamma$ in the set shown in \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:set}, there exist two operators $\Gamma_0$ and $\Gamma_1$ so that
\begin{itemize}
\item
both  $\Gamma_1$ and $\Gamma_0$ act as the identity operator on $\reg{p_1 \ldots p_k}$;
\item
$\Gamma_0$ acts as the identity operator on $\reg{t_k}$;
\end{itemize}
and the following holds
\begin{align*}
& 
\Gamma = \ketbra{p_1, \ldots,p_k}_{\reg{p_1\ldots p_k}} \tensor \Gamma_1 + \sum_{(p'_1,\ldots,p'_k) \ne (p_1, \ldots, p_k)}\ketbra{p'_1, \ldots,p'_k}_{\reg{p_1\ldots p_k}} \tensor \Gamma_0,\\ 
& 
\Gamma_0 C_{k,0}  = C_{k,0} \Gamma^{\reg{t_k}/\reg{m}}_0, \\ 
& 
\Gamma_0 C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} = C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} \Gamma^{\reg{t_k}/\reg{m}}_0 
.\end{align*}
In the following, we prove it for each possible $\Gamma$.

First, notice that the above is true for $\Gamma =\ketbra{p_1, \ldots, p_i}_{\reg{p_1 \ldots p_i}}$ for each $i \in \Set{k+1, k+2, \ldots, K}$, simply because such a $\Gamma$ can be written in the following format:
\begin{align*}
\Gamma 
& = 
\ketbra{p_1, \ldots, p_i}_{\reg{p_1 \ldots p_i}} \\ 
& = 
\ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \tensor \Gamma_1  
+ 
\sum_{(p'_1,\ldots,p'_k) \ne (p_1, \ldots, p_k)}\ketbra{p'_1, \ldots,p'_k}_{\reg{p_1\ldots p_k}} \tensor \Gamma_0,
\end{align*}
with $\Gamma_1  \coloneqq \ketbra{p_{k+1}, p_{k+2} \ldots, p_i}_{\reg{p_{k+1} \ldots p_i}}$ and $\Gamma_0  \coloneqq I$, and such a $\Gamma_0$ vacuously satisfies the requires $\Gamma_0 C_{k,0}  = C_{k,0} \Gamma^{\reg{t_k}/\reg{m}}_0$ and $\Gamma_0 C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} = C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} \Gamma^{\reg{t_k}/\reg{m}}_0$.

The above is true for $\Gamma = U_{gc}$ as well, because $U_{gc}$ acts non-trivially only on register $\reg{gc}$.


The above is also true for $\Gamma = S$ because (1) $S$ does not act on $\reg{p_1 \ldots p_k}$, (2) $S$ does not act on $\reg{t_k}$ and $C_{k,0}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_k}$, and (3) $S^{\reg{t_k}/\reg{m}}$ acts non-trivially on different registers from $B_{k,1}$ and $C_{k,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}).

The above is true for $\Gamma \in \Set{A_i}_{i \in \Set{k+1, k+2, \ldots, K}}$ as well, because for each $i\in \Set{k+1, k+2, \ldots, K}$, $A_i$ is nothing but the swap operator between registers $\reg{p_i}$ and $\reg{m}$ (see \Cref{CPM-3ZK:V:unitary}).

The only  cases left are $\Gamma \in \Set{(B_i, C_i, D_i)}_{i \in \Set{k+1, k+2, \ldots, K}}$. The proof for these cases are (almost) identical. In the following, we only present the proof for $\Gamma = C_i$ $(\forall i \in \Set{k+1, k+2, \ldots, K})$ as a representative example:
\begin{align*}
\Gamma 
& = 
C_i 
\\
& = 
\ketbra{p_1, \ldots, p_i}_{\reg{p_1 \ldots p_i}} \tensor C_{i,1} 
+ 
\sum_{(p'_1,\ldots,p'_i) \ne (p_1, \ldots, p_i)} \ketbra{p'_1, \ldots,p'_i}_{\reg{p_1\ldots p_i}} \tensor C_{i,0}
\numberthis \label{H:IND:proof:invariant:induction:case-2:claim:operator-commute:proof:C2:1} \\ 
& =
\ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \tensor \ketbra{p_{k+1}, \ldots, p_i}_{\reg{p_{k+1} \ldots p_i}} \tensor C_{i,1}
~ +  \\ 
& \hspace{2em}
\sum_{(p'_1,\ldots,p'_i) \ne (p_1, \ldots, p_i)}  \ketbra{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}} \tensor \ketbra{p'_{k+1}, \ldots, p'_i}_{\reg{p_{k+1} \ldots p_i}} \tensor C_{i,0} 
\\ 
& =
\ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \tensor \ketbra{p_{k+1}, \ldots, p_i}_{\reg{p_{k+1} \ldots p_i}} \tensor C_{i,1}
~ +  \\ 
& \hspace{2em}
 \ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \tensor 
 \bigg( 
 \sum_{(p'_{k+1},\ldots,p'_i) \ne (p_{k+1}, \ldots, p_i)} 
 \ketbra{p'_{k+1}, \ldots, p'_i}_{\reg{p_{k+1} \ldots p_i}}
 \bigg) 
\tensor C_{i,0} 
~ + \\ 
& \hspace{2em}
\sum_{(p'_1,\ldots,p'_k) \ne (p_1, \ldots, p_k)}  \ketbra{p'_1, \ldots, p'_k}_{\reg{p_1 \ldots p_k}} 
\tensor 
 \bigg( 
 \sum_{(p'_{k+1},\ldots,p'_i) \in \bits^{(i - k)\cdot \ell} } 
 \ketbra{p'_{k+1}, \ldots, p'_i}_{\reg{p_{k+1} \ldots p_i}}
 \bigg) 
\tensor C_{i,0} 
\\ 
& =
\ketbra{p_1, \ldots, p_k}_{\reg{p_1 \ldots p_k}} \tensor \Gamma_1  
+ 
\sum_{(p'_1,\ldots,p'_k) \ne (p_1, \ldots, p_k)}\ketbra{p'_1, \ldots,p'_k}_{\reg{p_1\ldots p_k}} \tensor \Gamma_0,
 \numberthis \label{H:IND:proof:invariant:induction:case-2:claim:operator-commute:proof:C2:2}
,\end{align*}
where \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:proof:C2:1} follows from the definition of $C_i$ (see \Cref{re-define:unitaries}), and \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:proof:C2:2} follows by defining $\Gamma_0$ and $\Gamma_1$ as follows 
\begin{align*}
 \Gamma_1 
 & \coloneqq 
 \ketbra{p_{k+1}, \ldots, p_i}_{\reg{p_{k+1} \ldots p_i}} \tensor C_{i,1}
~ + \\ 
& \hspace{6em}
\bigg( 
 \sum_{(p'_{k+1},\ldots,p'_i) \ne (p_{k+1}, \ldots, p_i)} 
 \ketbra{p'_{k+1}, \ldots, p'_i}_{\reg{p_{k+1} \ldots p_i}}
 \bigg) 
\tensor C_{i,0} 
\\ 
 \Gamma_0 
 & \coloneqq 
  \bigg( 
 \sum_{(p'_{k+1},\ldots,p'_i) \in \bits^{(i - k)\cdot \ell} } 
 \ketbra{p'_{k+1}, \ldots, p'_i}_{\reg{p_{k+1} \ldots p_i}}
 \bigg) 
\tensor C_{i,0}.
\end{align*} 
Clearly, such a $\Gamma_0$ satisfies the requires $\Gamma_0 C_{k,0}  = C_{k,0} \Gamma^{\reg{t_k}/\reg{m}}_0$ and $\Gamma_0 C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} = C_{k,0}  B^\dagger_{k,1} C^\dagger_{k,1} \Gamma^{\reg{t_k}/\reg{m}}_0$, because (1) we are in the case $i \in \Set{k+1, k+2, \ldots, K}$, (2) $C_{i,0}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_i}$, and (3) $C_{i,0}^{\reg{t_k}/\reg{m}}$ acts non-trivially on different registers from $B_{k,1}$ and $ C_{k,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}).

\vspace{1em}
This finishes the proof of \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}.   

\end{proof}


\para{Finishing the Proof for \Cref{H:IND:proof:invariant:induction:case-2}.} With \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute} in hand, we now show how to finish the proof for \Cref{H:IND:proof:invariant:induction:case-2}.

\subpara{Proof of \Cref{lem:H:IND:proof:invariant:target-format:Hk-1}.} First, we establish \Cref{lem:H:IND:proof:invariant:target-format:Hk-1}:
\begin{align*}
 \ket{\phi^{(t)}} 
 & = 
 \Lambda  \ket{\phi^{(t-1)}}  
 \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:0}\\ 
& = 
\Lambda  
  \bigg(
  \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
   ~+~ \\ 
   & \hspace{10em}
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1} \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
  \bigg)  
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:1}\\ 
  & =  
  \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \Lambda_1  \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
   ~+~ \\ 
   & \hspace{10em}
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k} \Lambda_0  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1} \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:2}\\ 
  & =  
    \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \Lambda_1  \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
    ~+~ \\ 
   & \hspace{10em}
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}   C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1} \Lambda^{\reg{t_k}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:3}\\ 
& =  
  \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \ket{\rho^{(t)}_{p_1, \ldots, p_k}}  
   ~+~ 
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}  C_{k,0} B^\dagger_{k,1} C^\dagger_{k,1} \ket{\rho^{(t)}_{p'_1, \ldots, p'_k}} 
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:4}
,\end{align*}
where  
\begin{itemize}
\item

\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:0} follows from \Cref{H:IND:proof:invariant:induction:case-2:initial:phi}; 

\item
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:1} follows from our induction assumption; 

\item
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:2}  follows from \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:1} in \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}; 

\item
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:3} follows from \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:3} in \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}; 

\item 
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:4} follows by defining
\begin{equation}\label[Expression]{H:IND:proof:invariant:induction:case-2:final:derivation:def:rho-t}
\begin{cases}
\ket{\rho^{(t)}_{p_1, \ldots, p_k}}
\coloneqq 
 \Lambda_1 \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}} & 
 \vspace{0.3em}
 \\ 
\ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}
\coloneqq 
\Lambda^{\reg{t_k}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}} 
& ~~\forall (p'_1, \ldots, p'_k) \in \big(\bits^{k\ell} \setminus \Set{(p_1, \ldots,p_k)}\big). 
\end{cases}
\end{equation}
\end{itemize}
Clearly, \Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:4} is of the same format as \Cref{lem:H:IND:proof:invariant:target-format:Hk-1} in \Cref{lem:H:IND:proof:invariant}.


\subpara{Proof of \Cref{lem:H:IND:proof:invariant:target-format:Hk}.} Next, we present the derivation for \Cref{lem:H:IND:proof:invariant:target-format:Hk}:
\begin{align*}
 \ket{\psi^{(t)}} 
 & = 
 \Lambda  \ket{\psi^{(t-1)}}  
 \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:0}\\ 
& = 
\Lambda  
  \bigg(
  \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
   ~+~ \\ 
   & \hspace{10em}
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}  C_{k,0}  \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
  \bigg)  
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:1}\\ 
  & =  
  \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \Lambda_1  \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
   ~+~ \\ 
   & \hspace{10em}
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k} \Lambda_0  C_{k,0} \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:2}\\ 
  & =  
    \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \Lambda_1  \ket{\rho^{(t-1)}_{p_1, \ldots, p_k}}  
    ~+~ \\ 
   & \hspace{10em}
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}   C_{k,0} \Lambda^{\reg{t_k}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1, \ldots, p'_k}}
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:3}\\ 
& =  
  \ket{p_1, \ldots, p_k}_{\reg{p_1\ldots p_k}} \ket{\rho^{(t)}_{p_1, \ldots, p_k}}  
   ~+~ 
   \sum_{(p'_1, \ldots, p'_k)\ne (p_1, \ldots, p_k)} \ket{p'_1, \ldots, p'_k}_{\reg{p_1} \ldots p_k}  C_{k,0} \ket{\rho^{(t)}_{p'_1, \ldots, p'_k}} 
  \numberthis \label{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:4}
,\end{align*}
where  
\begin{itemize}
\item

\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:0} follows from \Cref{H:IND:proof:invariant:induction:case-2:initial:psi}; 

\item
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:1} follows from our induction assumption; 

\item
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:2}  follows from \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:1} in \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}; 

\item
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:3} follows from \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute:eq:2} in \Cref{H:IND:proof:invariant:induction:case-2:claim:operator-commute}; 

\item 
\Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:4} follows from {\em the same definitions of} $\ket{\rho^{(t)}_{p_1, \ldots, p_k}}$ and $\ket{\rho^{(t)}_{p'_1, \ldots, p'_k}}$ as shown in \Cref{H:IND:proof:invariant:induction:case-2:final:derivation:def:rho-t}.
\end{itemize}
Clearly, \Cref{H:IND:proof:invariant:induction:case-2:final:derivation:eq:psi:4} is of the same format as \Cref{lem:H:IND:proof:invariant:target-format:Hk} in \Cref{lem:H:IND:proof:invariant}.


\vspace{1em}
This completes the proof of the induction step of \Cref{lem:H:IND:proof:invariant} for \Cref{H:IND:proof:invariant:induction:case-2}.



\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:H:IND:proof:invariant:base} and the proof for the induction step in \Cref{sec:lem:H:IND:proof:invariant:induction} together finish the proof of \Cref{lem:H:IND:proof:invariant}, which in turn finishes the proof of \Cref{lem:H:IND} eventually.

==> sections/CPM-warmup.tex <==

\section{CPM: Warm-Up}
\label{sec:CMP:warm-up}

In this section, we prove \Cref{lem:H:IND} for the special case $K = 2$. 


In this setting, there are only three hybrids to consider, namely $H^{(J, \msf{pat})}_0$, $H^{(J, \msf{pat})}_1$, and $H^{(J, \msf{pat})}_2$. To provide better intuition, we illustrate them in \Cref{figure:CPM-3ZK:hybrids}, with difference between adjacent hybrids highlighted in \red{red color}. In more detail, \Cref{figure:CPM-3ZK:hybrids} illustrates these three hybrids for some particular $(J, \msf{pat})$:
\begin{itemize}
 \item
In hybrid $H^{(J, \msf{pat})}_0$, it can be seen from \Cref{figure:CPM-3ZK:hybrids:H0} that all the $\downarrow$-queries are answered using $\tilde{V}$ and all the $\uparrow$-queries are answered using $\tilde{V}^\dagger$.  

\item
The hybrid $H^{(J, \msf{pat})}_1$ shown in \Cref{figure:CPM-3ZK:hybrids:H1} is identical to hybrid $H^{(J, \msf{pat})}_0$ except that the $\downarrow$-queries that bring the global counter from $\ket{0}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ (except for  the  $\msf{sq}(1)$ query) are answered using the ``dummy-version'' unitary$\ddot{V}$, and the $\uparrow$-queries that bring the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{0}_{\reg{gc}}$ are answered using the ``dummy-version'' unitary $\ddot{V}^\dagger$.

\item
The hybrid $H^{(J, \msf{pat})}_2$ shown in \Cref{figure:CPM-3ZK:hybrids:H2} is identical to hybrid $H^{(J, \msf{pat})}_1$ except that the $\downarrow$-queries that bring the global counter from $\ket{1}_{\reg{gc}}$ to $\ket{2}_{\reg{gc}}$ (except for  the  $\msf{sq}(2)$ query) are answered using the ``dummy-version'' unitary$\ddot{V}$, and the $\uparrow$-queries that bring the global counter from $\ket{2}_{\reg{gc}}$ to $\ket{1}_{\reg{gc}}$ are answered using the ``dummy-version'' unitary $\ddot{V}^\dagger$.
 \end{itemize} 


\begin{figure}[!tb]
\centering
     \begin{subfigure}[t]{0.47\textwidth}
         \fbox{
         \includegraphics[width=\textwidth,page=1]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H0}
     \end{subfigure}
     \hspace{15pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=2]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H1}
     \end{subfigure}
     
     \centering\vspace{1em}
     \begin{subfigure}[t]{0.47\textwidth}
         
         \fbox{
         \includegraphics[width=\textwidth,page=3]{figures/CPM-3ZK-figures.pdf}
         }
         \caption{}
         \label{figure:CPM-3ZK:hybrids:H2}
     \end{subfigure}
     \caption{Illustration of Hybrids $H^{(J, \msf{pat})}_0$, $H^{(J, \msf{pat})}_1$, and $H^{(J, \msf{pat})}_2$}
     \label{figure:CPM-3ZK:hybrids}
\end{figure}

For these hybrids, to prove \Cref{lem:H:IND}, it now suffices to establish the following \Cref{lem:CPM-3ZK:H01,lem:CPM-3ZK:H12}. 
\begin{lemma}\label{lem:CPM-3ZK:H01}
For all $(J, \msf{pat})$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_1 \big].$$
\end{lemma}

\begin{lemma}\label{lem:CPM-3ZK:H12}
For all $(J, \msf{pat})$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_1 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_2 \big].$$
\end{lemma}

In the sequel, we prove these two lemmas in \Cref{sec:lem:CPM-3ZK:H01:proof,sec:lem:CPM-3ZK:H12:proof} respectively. We emphasize that in the following, we use the notation established in \Cref{sec:CPM:hybrids:restate}.


\subsection{Proving \Cref{lem:CPM-3ZK:H01}}
\label{sec:lem:CPM-3ZK:H01:proof}

We present a lemma (\Cref{lem:CPM-3ZK-hyb01:proof:invariant}) that characterizes how the overall state evolves in $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$. This lemma is the major workhorse that implies \Cref{lem:CPM-3ZK:H01}. In the sequel, we first show how to establish \Cref{lem:CPM-3ZK:H01} assuming that \Cref{lem:CPM-3ZK-hyb01:proof:invariant} holds. After that, we will present the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.




\begin{lemma}[Invariance in $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$]\label{lem:CPM-3ZK-hyb01:proof:invariant}
Assume that during the execution of $H^{(J, \msf{pat})}_0$ (and $H^{(J, \msf{pat})}_1$), the global counter reaches value $1$ for $T$ times in total. For each $t \in [T]$, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds: in hybrid $H^{(J, \msf{pat})}_0$ (resp.\ $H^{(J, \msf{pat})}_1$), when the global counter reaches value $1$ for the $t$-th time, the overall state can be written as $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows
\begin{align}
\ket{\phi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}}, \label{lem:CPM-3ZK-hyb01:proof:target-format:H0}\\ 
\ket{\psi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \red{C_{1,0}} \ket{\rho^{(t)}_{p'_1}}. \label{lem:CPM-3ZK-hyb01:proof:target-format:H1}
\end{align}
where the $p_1$ is defined in $\msf{pat}$ and  the unitaries $B_{1,1}$, $C_{1,0}$, and $C_{1,1}$  are as defined in \Cref{re-define:unitaries}.
\end{lemma}



\para{Finishing the Proof of \Cref{lem:CPM-3ZK:H01}}. Let us consider the last time when the global counter reaches value $1$. By \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, the overall states in $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$ would be of the following format respectively
\begin{align}
\ket{\phi^{(T)}} 
& = 
\overbrace{
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}} ,\\ 
\ket{\psi^{(T)}}
& = 
\overbrace{
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(T)}_{p_1}}
}^{\msf{Good}}  ~+~
\overbrace{
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(T)}_{p'_1}}
}^{\msf{Bad}}. 
\end{align}
Since this is the last time the global counter reaches value $1$, the two hybrids $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$ by definition behave identically after that (see \Cref{figure:CPM-3ZK:hybrids}). That is, the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ will go through the same quantum procedure (let us denote it by $\mcal{F}$) and finally measured by the predicate $\msf{Pred}$.	



Next, note that the states $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the identical ``branch'' corresponding to $\ket{p_1}_{\reg{p_1}}$ (labeled as $\msf{Good}$ in the above equations). Also, the $\msf{Bad}$ branch will not contribute any shares to the accepting probability of the predicate $\msf{Pred}$---this is because the quantum procedure $\mcal{F}$ will not change the fact that $p'_1 \ne p_1$ for the $\msf{Bad}$ branch, and recall that, as a consequence of \Cref{counter-structure:lemma}, $\msf{Pred}$ will output $0$ if a branch in the superposition does not have any non-zero amplitude for $\ket{p_1}_{\reg{p_1}}$.	

In summary, only the $\msf{Good}$ branch matters for the remaining execution (i.e., that after the last time when the global counter reaches value 1), contributing to the event $\msf{Pred}(\rho) = 1$. Therefore, \Cref{lem:CPM-3ZK:H01} holds simply because $\ket{\phi^{(T)}}$ and $\ket{\psi^{(T)}}$ share the same $\msf{Good}$ branch. 



\para{Proving \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.} Now, the only task remaining is to prove \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. We will demonstrate this lemma through mathematical induction on the number $t \in [T]$, indicating the time at which the global counter reaches the value $1$. Throughout this proof, we will monitor the evolution of the overall states in both $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$ simultaneously. This is done in \Cref{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:base:sec,sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:sec} respectively.


\subsubsection{Base Case ($t = 1$)}
\label{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:base:sec} 

We first derive how the overall state evolves in $H^{(J, \msf{pat})}_0$. 

This case corresponds to the very first time the global counter reaches $1$. By definition, this is due to the $\msf{sq}(1)$ query. In more detail,  $\Sim$ will first apply her local unitary $S$, followed by the projector $\ketbra{\downarrow}_{\reg{u}}$. Next, according to the notation in \Cref{MnR:game:redefine:hybrids}, the operator $D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc}$ will be applied. Thus, if we assume that the initial state across all the registers are $\ket{\rho}$, then the state $\ket{\phi^{(1)}}$ will be as follows:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_1C_1B_1 \ketbra{p_1}_{\reg{p_1}} A_1 U_{gc} \ketbra{\downarrow}_{\reg{u}} S  
\ket{\rho}
\\
& =
D_1C_1B_1  
 \ket{p_1}_{\reg{p_1}} \ket{\rho_{p_1}} 
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:4} \\ 
& =  
 \ket{p_1}_{\reg{p_1}}  D_{1,1}  C_{1,1}B_{1,1} \ket{\rho_{p_1}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:5} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} 
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:4} follows by defining $\ket{\rho_{p_1}} \coloneqq \bra{p_1}_{\reg{p_1}} A_1 U_{gc} \ketbra{\downarrow}_{\reg{u}} S  
\ket{\rho}$;
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:5} follows from the definition of $B_1$  $C_1$, and $D_1$ (see \Cref{re-define:unitaries});
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} follows by defining $\ket{\rho^{(1)}_{p_1}} \coloneqq D_{1,1} C_{1,1}B_{1,1} \ket{\rho_{p_1}}$.
\end{itemize}
% Obviously, $\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7}$ is a special case of \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} when $t = 1$.
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} satisfies the format shown in \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} when $t = 1$.


Also, note that the hybrids $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:base:eq:7} that 
$$\ket{\psi^{(1)}} =  \ket{p_1}_{\reg{p_1}} \ket{\rho^{(1)}_{p_1}} .$$ Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.




\subsubsection{Induction Step ($t \ge 2$)} 
\label{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:sec} 


We assume that $\ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t-1)}}$ satisfy \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, and show in the following that \Cref{lem:CPM-3ZK-hyb01:proof:invariant} holds when the global counter reaches $1$ for the $t$-th time.

We establish this claim by considering the following MECE (mutually exclusive and collectively exhaustive) cases:
\begin{enumerate}
\item \label[Case]{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}
{\bf Case 1:} The $t$-th arrival at value $1$ is due to an immediate $\uparrow \downarrow$ after the $(t-1)$-th arrival. That is, after the $(t-1)$-th arrival, $\Sim$ first makes a $\uparrow$ query, bringing the global counter to $0$, and then makes an $\downarrow$ query, bringing the global counter back to $1$. 
\item \label[Case]{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}
{\bf Case 2:} The $t$-th arrival at value $1$  is due to an immediate $\downarrow \uparrow $ after the $(t-1)$-th arrival. That is, after the $(t-1)$-th arrival, $\Sim$ first makes a $\downarrow$ query, bringing the global counter to $2$, and then makes an $\uparrow$ query, bringing the global counter back to $1$. 
\end{enumerate}


\subsubsubsection{Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}}

We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) in \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}:
\begin{enumerate}
 \item
$\Sim$'s local unitary $S$ is applied, followed by the projector $\ketbra{\uparrow}_{\reg{u}}$. Note that this step is identical for both $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$. 

\begin{remark}[Hiding the Projector on Register $\reg{u}$]\label{rmk:CPM-3ZK:hid-proj-u}
In the sequel, we overload the notation $S$ to think of it as already including the projection $\ketbra{\uparrow}_{\reg{u}}$, and thus do not spell the $\ketbra{\uparrow}_{\reg{u}}$ out explicitly. We remark that this will not affect our proof, because what matters for $S$ in the following proof is the registers on which it operates, and the original $S$ already operates non-trivially on register $\reg{u}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}). 
\end{remark}

\item
An $\uparrow$-query is made, bringing the global counter from 1 to 0. According to the notation in \Cref{MnR:game:redefine:hybrids}: 
\begin{itemize}
    \item
    In $H^{(J, \msf{pat})}_0$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1$; 

    \item
    In $H^{(J, \msf{pat})}_1$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1$. 
\end{itemize}
\item
$\Sim$ will apply her local operation $S$ again (followed by $\ketbra{\downarrow}_{\reg{u}}$ which we hide as per \Cref{rmk:CPM-3ZK:hid-proj-u}).  Note that this step is again identical for both $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$.
\item
An $\downarrow$-query is made, bringing the global counter from 0 back to 1, which is the global counter's $t$-th arrival at value 1. According to the notation in \Cref{MnR:game:redefine:hybrids}: 
\begin{itemize}
    \item
    In $H^{(J, \msf{pat})}_0$, this corresponds to applying $D_1C_1B_1A_1U_{gc}$; 
    \item
    In $H^{(J, \msf{pat})}_1$, this corresponds to applying $D_1\ddot{C}_1A_1U_{gc}$. 
\end{itemize} 
\end{enumerate}
It follows from the above description (and \Cref{rmk:CPM-3ZK:hid-proj-u}) that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
\begin{align}
\ket{\phi^{(t)}}
& = D_1C_1B_1A_1U_{gc} S U^{\dagger}_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1 S  \ket{\phi^{(t-1)}}, \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}\\ 
\ket{\psi^{(t)}}
& = D_1 \ddot{C}_1A_1U_{gc} S  U^{\dagger}_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1 S \ket{\psi^{(t-1)}}. \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}
\end{align}

% We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) in  \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}:
% \begin{enumerate}
%  \item
% $\Sim$'s local unitary $S$ is applied. Note that this step is identical for both $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$. 
% \item
% An $\uparrow$-query is made, bringing the global counter from $1$ to $0$. 
% \begin{itemize}
%     \item
%     In $H^{(J, \msf{pat})}_0$, this corresponds to applying $\tilde{V}^\dagger$; 
%     \item
%     In $H^{(J, \msf{pat})}_1$, this corresponds to applying $\ddot{V}^\dagger$. 
% \end{itemize}
% \item
% The local operation $S$ is applied. Note that this step is identical for both $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$ as well.
% \item
% An $\downarrow$-query is made, resulting in the global counter's $t$-th arrive to $1$.
% \begin{itemize}
%     \item
%     In $H^{(J, \msf{pat})}_0$, this corresponds to applying $\tilde{V}$; 
%     \item
%     In $H^{(J, \msf{pat})}_1$, this corresponds to applying $\ddot{V}$. 
% \end{itemize} 
% \end{enumerate}
% It follows from the above description that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
% \begin{align}
% \ket{\phi^{(t)}}
% & = \tilde{V} S \tilde{V}^\dagger S  \ket{\phi^{(t-1)}}, \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0}\\ 
% \ket{\psi^{(t)}}
% & = \ddot{V} S \ddot{V}^\dagger S \ket{\psi^{(t-1)}}. \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}
% \end{align}

\para{High-Level Idea for the Sequel.}
Recall that our eventual goal is to prove that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ are of the format shown in \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0,lem:CPM-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1}. But we first need to perform some preparation work, putting \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. Then, we show on \Cpageref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} how to use \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} to complete the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}. 



\begin{MyClaim}\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}
There exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ so that the following holds
\begin{align}
\ket{\phi^{(t)}}
& =  
D_1C_1 B_1 U_{gc} S^{\reg{p_1}/\reg{m}} U^\dagger_{gc} B^\dagger_1 C^\dagger_1
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\bigg) \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(t)}}
& = 
D_1\ddot{C}_1 U_{gc} S^{\reg{p_1}/\reg{m}} U^\dagger_{gc}   \ddot{C}^\dagger_1 
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\bigg) 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} 
,\end{align}
where $S^{\reg{p_1}/\reg{m}}$ is identical to $S$ except that it treats register $\reg{p_1}$ as register $\reg{m}$.
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}]

First, notice that  
\begin{align*}
 A_1 U_{gc} S U^\dagger_{gc} A^\dagger_1 
 & = 
 A_1 U_{gc} S A^\dagger_1 U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:1} \\ 
 & = 
 A_1 U_{gc} A^\dagger_1 S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:2} \\
  & = 
 A_1 A^\dagger_1 U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:3} \\
 & = 
U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:1,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:3} follows from the fact that $U_{gc}$ acts on different registers from $A_1$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S:2} from the fact that $S$ acts as the identity operator on $\reg{p_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}) and that $A_1$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_1}$ (see \Cref{CPM-3ZK:V:unitary}). 
\end{itemize}



\subpara{Proving \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(t)}}$:
\begin{align*}
\ket{\phi^{(t)}}
& =
D_1C_1B_1A_1U_{gc} S U^{\dagger}_{gc} A^\dagger_1 B^\dagger_1 C^\dagger_1 D^\dagger_1  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:0} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1 D^\dagger_1  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1 D^\dagger_1 S 
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  +
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1 D^\dagger_1  
\bigg(
\ket{p_1}_{\reg{p_1}} S \ket{\rho^{(t-1)}_{p_1}}  +
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} S C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc} B^\dagger_1 C^\dagger_1  
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  +
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} S C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} \\
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  B^\dagger_1 C^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  + \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} S^{\reg{t_1}/\reg{m}} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  B^\dagger_1 C^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  + \\ 
& \hspace{18em} 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} \\ 
& =
D_1C_1B_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  B^\dagger_1 C^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H0};

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S};

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2} follows from our induction assumption;

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:3} from  from the fact that $S$ acts as the identity operator on $\reg{p_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:4} from  from the definition of $D_1$ (see \Cref{re-define:unitaries});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:5} from the fact that $S$ acts as the identity operator on $\reg{t_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}) and $C_{1,0}$ is nothing but a swap operator between $\reg{t_1}$ and $\reg{m}$ (see \Cref{re-define:unitaries}); (Note that $S^{\reg{t_1}/\reg{m}}$ is defined to be an operator that is identical to $S$ except that it treats $\reg{t_1}$ as $\reg{m}$.)

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} follows from the fact that $S^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $C_{1,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} follows by defining 
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}
\ket{\dot{\rho}^{(t-1)}_{p_1}}   \coloneqq D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}} ~~~\text{and}~~~
\ket{\dot{\rho}^{(t-1)}_{p'_1}}  \coloneqq S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}).
\end{equation}
\end{itemize}
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\subpara{Proving \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi}.} We now show the derivation for $\ket{\psi^{(t)}}$. This is almost identical to the above proof for \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
\begin{align*}
\ket{\psi^{(t)}}
& =
D_1 \ddot{C}_1 A_1U_{gc} S U^{\dagger}_{gc} A^\dagger_1 \ddot{C}^\dagger_1 D^\dagger_1  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:0} \\ 
& =
D_1 \ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1 D^\dagger_1  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} \\ 
& =
D_1 \ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1 D^\dagger_1  S  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2} \\ 
& =
D_1\ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} D^\dagger_{1,1} S \ket{\rho^{(t-1)}_{p_1}}  ~+~ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0}  S^{\reg{t_1}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:6} \\ 
& =
D_1\ddot{C}_1  U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_1
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  ~+~ 
 \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:eq:k:H1};

\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:eq:swap-S};


\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:2}  follows from our induction assumption;


\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:6} follows from a similar argument as we did to derive \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:6} from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:phi-derivation:2};


\item
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} follows from {\em the same definitions} of $\ket{\dot{\rho}^{(t-1)}_{p_1}}$ and $\ket{\dot{\rho}^{(t-1)}_{p'_1}}$ as shown in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho-dot}.
\end{itemize}
\Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:psi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\vspace{1em}
This completes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.

\end{proof}

\vspace{1em}

\begin{MyClaim}\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}
Let $S^{\reg{p_1}/\reg{m}}$ and $\Set{\dot{\rho}^{(t-1)}_{p'_1}}_{p'_1 \in \bits^\ell}$ be as defined in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}. Let
\begin{align}
\ket{\gamma^{(t-1)}_0} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:0} \\ 
\ket{\gamma^{(t-1)}_1} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t-1)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t-1)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:1} \\ 
\ket{\gamma^{(t)}_0} 
& \coloneqq 
C_1 B_1 U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}    B^\dagger_1 C^\dagger_1 \ket{\gamma^{(t-1)}_0} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0} \\ 
\ket{\gamma^{(t)}_1}
& \coloneqq 
\ddot{C}_1 U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}   \ddot{C}^\dagger_1  \ket{\gamma^{(t-1)}_1}
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1} 
.\end{align}
Then, there exist (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1}}}_{p'_1 \in \bits^\ell}$ so that the following holds:
\begin{align}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} 
.\end{align}
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}]
This claim follows from an application of \Cref{lem:err-inv-com}, with the notation correspondence listed in \Cref{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}}
\label{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}  \\ 
\midrule
\addlinespace[0.3em]
$\reg{a}$   & $\reg{p_1}$ & & $W_1$ & $C_{1,1}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_0$ & $C_{1,0}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_1}$ & & $W$   & $C_{1}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p_1}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u}$, $\reg{s}$, $\reg{gc}$ & & $\tilde{W}$ & $\ddot{C}_1$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p'_1}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_1$ & $B_{1,1}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & $\ket{\gamma^{(t-1)}_0}$ \\ 
\addlinespace[0.3em]
   & & & $U$   & $B_1$ & & $\ket{\eta^{(\msf{in})}_1}$ & $\ket{\gamma^{(t-1)}_1}$  \\ 
\addlinespace[0.3em]
 &  & &   $S$   & $U_{gc} S^{\reg{p_1}/\reg{m}}  U^\dagger_{gc}$ & &  $\ket{\rho^{(\msf{out})}_a}_\reg{mtso}$    & $\ket{\dot{\rho}^{(t)}_{p_1}}$  \\ 
\addlinespace[0.3em]
  &  & &   &  & &  $\ket{\rho^{(\msf{out})}_{a'}}_\reg{mtso}$     & $\ket{\dot{\rho}^{(t)}_{p'_1}}$  \\  
  \addlinespace[0.3em]
 &  & & & & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\gamma^{(t)}_0}$  \\
\addlinespace[0.3em] 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\gamma^{(t)}_1}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_1$ should work as the identity operator on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{1,1}$ (playing the role of $W_1$) who works as identity on registers $\reg{u}$, $\reg{s}$, and $\reg{gc}$ (playing the role of registers $\reg{s}$). (Recall $C_{1,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
\Cref{lem:err-inv-com} requires that $W_0$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $C_{1,0}$ (playing the role of $W_0$), who is a swap operator between registers $\reg{m}$ and $\reg{t_1}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively). (Recall $C_{1,0}$ from \Cref{re-define:unitaries}.)

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_0$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $\ddot{C}_1$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $C_{1,0}$ (playing the role of $W_0$) on branches $\ket{p'_1}_{\reg{p_1}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $p'_1 \ne p_1$. (Recall $\ddot{C}_1$ from \Cref{re-define:unitaries})

\item
 \Cref{lem:err-inv-com} requires that $U_1$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $B_{1,1}$ (playing the role of $U_1$), who works as identity on registers $\reg{u}$, $\reg{s}$, and $\reg{gc}$ (playing the role of register $\reg{s}$). (Recall $B_{1,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} notation, this is satisfied by $U_{gc}S^{\reg{p_1}/\reg{m}}U^\dagger_{gc}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{u}$, $\reg{s}$, and $\reg{gc}$ (playing the role of registers $\reg{a}$ and $\reg{s}$). (Recall $S$ from \Cref{CPM-3ZK:non-trivial-registers:table} and the fact that $S^{\reg{p_1}/\reg{m}}$ is identical to $S$ except that it treats $\reg{p_1}$ as $\reg{m}$.)
\end{itemize}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:CPM-3ZK-hyb01:proof:case-1:cor-table}) to the $\ket{\gamma^{(t-1)}_0}$ and $\ket{\gamma^{(t-1)}_1}$ defined in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:in:1}  (playing the role of $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ in \Cref{lem:err-inv-com}). This implies the existence of (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1}}}_{p'_1\in\bits^\ell }$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\gamma^{(t)}_0} 
& = \ket{p_1}_{\reg{p_1}}\ket{\dot{\rho}^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\dot{\rho}^{(t)}_{p'_1}} \\ 
\ket{\gamma^{(t)}_1} 
& = \ket{p_1}_{\reg{p_1}}\ket{\dot{\rho}^{(t)}_{p_1}}  +  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\dot{\rho}^{(t)}_{p'_1}} 
,\end{align*}
which are exactly \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} in  \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. 






This completes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}.

\end{proof}

\para{Finishing the Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}.}\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:finish} With \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim,lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2} at hand, we now finish the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}.

\subpara{Proof for \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}.} We first establish \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}:
\begin{align}
\ket{\phi^{(t)}} 
& = D_1 \ket{\gamma^{(t)}_0} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:1} \\ 
& = D_1 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\bigg) 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} D_{1,1}\ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1}  \ket{\rho^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:2} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:3} follows from the definition of $D_1$ (see \Cref{re-define:unitaries});

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:4} follows by defining
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho}
\ket{\rho^{(t)}_{p_1}}   \coloneqq D_{1,1} \ket{\dot{\rho}^{(t)}_{p_1}} ~~~\text{and}~~~
\ket{\rho^{(t)}_{p'_1}}  \coloneqq \ket{\dot{\rho}^{(t)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}).
\end{equation}
\end{itemize}
Note that \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:phi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. 


\subpara{Proof for \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}.}  Next, we establish \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}:


\begin{align}
\ket{\psi^{(t)}} 
& = D_1 \ket{\gamma^{(t)}_1} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:1} \\ 
& = D_1 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\dot{\rho}^{(t)}_{p'_1}} 
\bigg) 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} D_{1,1}\ket{\dot{\rho}^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0}  \ket{\dot{\rho}^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  
+  
\sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}  \ket{p'_1}_{\reg{p_1}}  C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
\label{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:1} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim} and \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:out:1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:2} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2:eq:target:1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:3} follows from the definition of $D_1$ (see \Cref{re-define:unitaries});

\item
\Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:4} follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1}}$ and $\ket{\rho^{(t)}_{p'_1}}$ in \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:proof:def:rho}.
\end{itemize}
Note that \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1:final:psi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. 

~\\ 
This eventually completes the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-1}.


\subsubsubsection{Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}} 
We first remark that in \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}, the computation that brings $\ket{\phi^{(t-1)}}$ to $\ket{\phi^{(t)}}$ is identical to that brings $\ket{\psi^{(t-1)}}$ to $\ket{\psi^{(t)}}$, because $H^{(J, \msf{pat})}_0$ and $H^{(J, \msf{pat})}_1$ are identical when the global counter ``jumps'' between $1$ and $2$. (This can be also seen pictorially by comparing \Cref{figure:CPM-3ZK:hybrids:H0} and \Cref{figure:CPM-3ZK:hybrids:H1}.) In the following, we refer to this computation as $\Lambda$. That is, we have 
\begin{align}
\ket{\phi^{(t)}} 
& = 
\Lambda \ket{\phi^{(t-1)}} 
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi} \\ 
\ket{\psi^{(t)}} 
& = 
\Lambda \ket{\psi^{(t-1)}}
\label{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi}
.\end{align} 

\para{Structure of $\Lambda$.} While the exact format of $\Lambda$ will not be substantial, our proof of \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2} will rely on certain properties of $\Lambda$, which we formalize in the following \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.

\begin{MyClaim}\label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}
For the operator $\Lambda$ defined above, there exist two operators $\Lambda_0$ and $\Lambda_1$ so that
\begin{itemize}
\item
both  $\Lambda_1$ and $\Lambda_0$ act as the identity operator on $\reg{p_1}$;
\item
$\Lambda_0$ acts as the identity operator on $\reg{t_1}$;
\end{itemize}
and the following holds
\begin{align}
& 
\Lambda = \ketbra{p_1}_{\reg{p_1}} \tensor \Lambda_1 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Lambda_0, \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} \\ 
& 
\Lambda_0 C_{1,0}  = C_{1,0} \Lambda^{\reg{t_1}/\reg{m}}_0, \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} \\ 
& 
\Lambda_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Lambda^{\reg{t_1}/\reg{m}}_0 \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} 
,\end{align}
where $\Lambda^{\reg{t_1}/\reg{m}}_0$ is identical to $\Lambda_0$ except that it treats $\reg{t_1}$ as $\reg{m}$.  
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}]

First, note that $\Lambda$ can be written as $\Lambda = \Gamma_z \Gamma_{z-1} \cdots \Gamma_1$ (for some integer $z$), where each $\Gamma_i$ ($i \in [z]$) comes from the set of operators $\Set{S, A_2, B_2, C_2, D_2, U_{gc}, \ketbra{p_1, p_2}_{\reg{p_1p_2}}}$. This is because $\Lambda$ only corresponds to the operations that happen when the global counter is no less than value $1$ (see  \Cref{MnR:game:redefine:hybrids} and \Cref{figure:CPM-3ZK:hybrids:H1}). We remark that $\Sim$ may also apply projectors on $\reg{u}$, but we consider it as a part of $S$ as per \Cref{rmk:CPM-3ZK:hid-proj-u}.


Therefore, to prove \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, it suffices to show that for each operator $\Gamma \in \Set{\ketbra{p_1, p_2}_{\reg{p_1p_2}}, U_{gc}, S, A_2, B_2, C_2, D_2}$, there exist two operators $\Gamma_0$ and $\Gamma_1$ so that
\begin{itemize}
\item
both  $\Gamma_1$ and $\Gamma_0$ act as the identity operator on $\reg{p_1}$;
\item
$\Gamma_0$ acts as the identity operator on $\reg{t_1}$;
\end{itemize}
and the following holds
\begin{align*}
& 
\Gamma = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_1 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_0,\\ 
& 
\Gamma_0 C_{1,0}  = C_{1,0} \Gamma^{\reg{t_1}/\reg{m}}_0, \\ 
& 
\Gamma_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Gamma^{\reg{t_1}/\reg{m}}_0 
.\end{align*}
In the following, we prove it for each possible $\Gamma$.

First, notice that the above is true for $\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}}$, simply because such a $\Gamma$ can be written in the following format:
$$\Gamma =\ketbra{p_1,p_2}_{\reg{p_1}\reg{p_2}} = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_1  + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}}\ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_0,$$
with $\Gamma_1  \coloneqq \ketbra{p_2}_{\reg{p_2}}$ and $\Gamma_0  \coloneqq I$, and such a $\Gamma_0$ vacuously satisfies the requires $\Gamma_0 C_{1,0}  = C_{1,0} \Gamma^{\reg{t_1}/\reg{m}}_0$ and $\Gamma_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Gamma^{\reg{t_1}/\reg{m}}_0$.

The above is true for $\Gamma = U_{gc}$ as well, because $U_{gc}$ acts non-trivially only on register $\reg{gc}$.


The above is also true for $\Gamma = S$ because (1) $S$ does not act on $\reg{p_1}$, (2) $S$ does not work on $\reg{t_1}$ and $C_{1,0}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_1}$, and (3) $S^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $C_{1,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}).

The above is true for $\Gamma = A_2$ as well, because $A_2$ is nothing but the swap operator between registers $\reg{p_2}$ and $\reg{m}$ (see \Cref{CPM-3ZK:V:unitary}).

The only  cases left are $\Gamma \in \Set{B_2, C_2, D_2}$. The proof for these cases are (almost) identical. In the following, we only prove it for $\Gamma = C_2$.
\begin{align*}
\Gamma = C_2 
& = 
\ketbra{p_1, p_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,1} + \sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1, p'_2}_{\reg{p_1}\reg{p_2}} \tensor C_{2,0} \numberthis \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:1} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor C_{2,1}
+ 
\sum_{(p'_1, p'_2) \in \bits^{2\ell} \setminus \Set{(p_1, p_2)}}  \ketbra{p'_1}_{\reg{p_1}} \tensor \ketbra{p'_2}_{\reg{p_2}} \tensor C_{2,0} \\ 
& =
\ketbra{p_1}_{\reg{p_1}} \tensor \ketbra{p_2}_{\reg{p_2}} \tensor C_{2,1} 
+ \ketbra{p_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0} \\ 
& \hspace{15em} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0} \\ 
& = \ketbra{p_1}_{\reg{p_1}} \tensor \Gamma_1 + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ketbra{p'_1}_{\reg{p_1}} \tensor \Gamma_0 \numberthis \label{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:2}
,\end{align*}
where \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:1} follows from the definition of $C_2$ (see \Cref{re-define:unitaries}), and \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:proof:C2:2} follows by defining $\Gamma_0$ and $\Gamma_1$ as follows 
\begin{align*}
 \Gamma_1 & \coloneqq \ketbra{p_2}_{\reg{p_2}} \tensor C_{2,1} 
+ \big(\sum_{p'_2 \in \bits^{\ell} \setminus \Set{p_2}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0} \\ 
 \Gamma_0 & \coloneqq \big(\sum_{p'_2 \in \bits^{\ell}}  \ketbra{p'_2}_{\reg{p_2}} \big) \tensor C_{2,0}.
\end{align*} 
Clearly, such a $\Gamma_0$ satisfies the requires $\Gamma_0 C_{1,0}  = C_{1,0} \Gamma^{\reg{t_1}/\reg{m}}_0$ and $\Gamma_0 C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} = C_{1,0}  B^\dagger_{1,1} C^\dagger_{1,1} \Gamma^{\reg{t_1}/\reg{m}}_0$, because (1) $C_{2,0}$ is nothing but a swap operator between $\reg{m}$ and $\reg{t_2}$, and (2) $C_{2,0}^{\reg{t_1}/\reg{m}}$ acts non-trivially on different registers from $B_{1,1}$ and $ C_{1,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}).

\vspace{1em}
This finishes the proof of \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}.	

\end{proof}





\para{Finishing the Proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}.} With \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute} in hand, we now show how to finish the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}.

\subpara{Proof of \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}.} First, we establish \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0}:
\begin{align}
 \ket{\phi^{(t)}} 
 & = 
 \Lambda  \ket{\phi^{(t-1)}}  
 \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:0}\\ 
& = 
\Lambda  
  \bigg(
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}}
  \bigg)  
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:1}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \Lambda_0 C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:2}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \Lambda^{\reg{t_1}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:3}\\ 
    & =  
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} B^\dagger_{1,1} C^\dagger_{1,1} \ket{\rho^{(t)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:4}
,\end{align}
where  
\begin{itemize}
\item

\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:phi}; 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:1} follows from our induction assumption; 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:2}  follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}; 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:3} follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:3} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}; 

\item 
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:4} follows by defining
\begin{equation}\label[Expression]{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:def:rho-t}
\ket{\rho^{(t)}_{p_1}} 
\coloneqq 
 \Lambda_1 \ket{\rho^{(t-1)}_{p_1}} ~~~\text{and}~~~ 
\ket{\rho^{(t)}_{p'_1}} 
\coloneqq 
\Lambda^{\reg{t_1}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1}} ~~(\forall p'_1 \in \bits^\ell \setminus \Set{p_1}). 
\end{equation}
\end{itemize}
Clearly, \Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:eq:4} is of the same format as \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H0} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.

\subpara{Proof of \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}.} Next, we present the derivation for  \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1}:
\begin{align}
 \ket{\psi^{(t)}} 
 & = 
 \Lambda  \ket{\psi^{(t-1)}}  
 \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0}\\ 
& = 
\Lambda  
  \bigg(
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0}  \ket{\rho^{(t-1)}_{p'_1}}
  \bigg)  
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} \Lambda_0 C_{1,0}  \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2}\\ 
  & =  
  \ket{p_1}_{\reg{p_1}} \Lambda_1 \ket{\rho^{(t-1)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \Lambda^{\reg{t_1}/\reg{m}}_0 \ket{\rho^{(t-1)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3}\\ 
    & =  
  \ket{p_1}_{\reg{p_1}}\ket{\rho^{(t)}_{p_1}}  ~+~
   \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho^{(t)}_{p'_1}} 
  \label{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4}
,\end{align}
where  
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:0} follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2:initial:psi}, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:1} follows from our induction assumption, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:2}  follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:1} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, 

\item
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:3} follows from \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute:eq:2} in \Cref{lem:CPM-3ZK-hyb01:proof:case-2-1:claim:operator-commute}, 

\item 
\Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1}}$ and $\ket{\rho^{(t)}_{p'_1}}$ as shown in \Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:def:rho-t}.
\end{itemize}
Clearly, \Cref{lem:CPM-3ZK-hyb01:proof:case-2:final:derivation:psi:eq:4} is of the same format as \Cref{lem:CPM-3ZK-hyb01:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb01:proof:invariant}.



This finishes the proof for \Cref{CPM-3ZK-hyb01:proof:invariant:proof:induction:case-2}.


\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:sec} together finish the proof of \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, which in turn finishes the proof of \Cref{lem:CPM-3ZK:H01} eventually.



\subsection{Proof of \Cref{lem:CPM-3ZK:H12}}
\label{sec:lem:CPM-3ZK:H12:proof}

Due to a similar argument as we did at the beginning of \Cref{sec:lem:CPM-3ZK:H01:proof}, we claim that: to prove \Cref{lem:CPM-3ZK:H12}, it suffices to establish the following \Cref{lem:CPM-3ZK-hyb12:proof:invariant}.

\begin{lemma}[Invariance in $H^{(J, \msf{pat})}_1$ and $H^{(J, \msf{pat})}_2$]\label{lem:CPM-3ZK-hyb12:proof:invariant}
Assume that during the execution of $H^{(J, \msf{pat})}_1$ (and $H^{(J, \msf{pat})}_2$), the global counter reaches value $2$ for $T$ times in total. For each $t \in [T]$, there exist (possibly sub-normalized) pure states $\Set{\ket{\rho^{(t)}_{p'_1, p'_2}}}_{p'_1, p'_2 \in \bits^\ell \times \bits^\ell}$ so that the following holds: in hybrid $H^{(J, \msf{pat})}_1$ (resp.\ $H^{(J, \msf{pat})}_2$), when the global counter reaches value $2$ for the $t$-th time, the overall state can be written as $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$) defined as follows
\begin{align}
\ket{\phi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1, p_2}}  ~+~
   \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t)}_{p'_1, p'_2}}, \label{lem:CPM-3ZK-hyb12:proof:target-format:H1}\\ 
\ket{\psi^{(t)}} 
& =  \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1, p_2}}  ~+~
 \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \red{C_{2,0}} \ket{\rho^{(t)}_{p'_1, p'_2}} \label{lem:CPM-3ZK-hyb12:proof:target-format:H2}
,\end{align}
where the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above), the $(p_1,p_2)$ are defined in $\msf{pat}$, and  the unitaries $B_{2,1}$, $C_{2,0}$, and $C_{2,1}$  are as defined in \Cref{re-define:unitaries}. 
\end{lemma}





\para{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant}.} Similar as the proof for \Cref{lem:CPM-3ZK-hyb01:proof:invariant}, 
we establish \Cref{lem:CPM-3ZK-hyb12:proof:invariant} through mathematical induction on the number $t \in [T]$, indicating the time at which the global counter reaches the value $2$. Throughout this proof, we will monitor the evolution of the overall states in both $H^{(J, \msf{pat})}_1$ and $H^{(J, \msf{pat})}_2$ simultaneously. This is done in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec,sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec} respectively.







\subsubsection{Base Case ($t = 1$)}
\label{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec} 


We first derive how the overall state evolves in $H^{(J, \msf{pat})}_1$. 

This case corresponds to the very first time the global counter reaches $2$. By definition, this is due to the $\msf{sq}(2)$ query. We assume w.l.o.g.\ that the overall state right before this query is some pure state $\ket{\rho}$.

\begin{remark}
Actually, we know the exact format of this $\ket{\rho}$ from the already-established \Cref{lem:CPM-3ZK-hyb01:proof:invariant}. That is, this state must be of the format  $\ket{\rho} = \ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho_{p'_1}}$. However, we remark that the exact format of $\ket{\rho}$ is not useful anywhere in this proof, and thus we do not need to refer to this long expression in the following derivation.
\end{remark}

By definition, the $\msf{sq}(2)$ query corresponds to the following procedure:  $\Sim$ will first apply her local unitary $S$ (followed by the projector $\ketbra{\downarrow}_{\reg{u}}$ which we hide as per \Cref{rmk:CPM-3ZK:hid-proj-u}). Next, according to the notation in \Cref{MnR:game:redefine:hybrids}, the operator $D_2C_2B_2 \ketbra{p_1,p_2}_{\reg{p_1p_2}} A_2 U_{gc}$ will be applied. 
% Moreover, note that the state right before this query must have global counter $\ket{1}_\reg{gc}$. It then follows from \Cref{lem:CPM-3ZK-hyb01:proof:invariant} that the state must be of the format  $\ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho_{p'_1}}$. 
In summary, the state $\ket{\phi^{(1)}}$ in $H^{(J, \msf{pat})}_1$ can be written as follows:
\begin{align*}
\ket{\phi^{(1)}} 
& =  
D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}A_2U_{gc} S   
\ket{\rho}
\\
& =  
D_2C_2B_2\ket{p_1, p_2}_{\reg{p_1p_2}} \ket{\rho_{p_1, p_2}}  
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:1} \\
& =  
\ket{p_1, p_2}_{\reg{p_1p_2}} 
D_{2,1} C_{2,1} B_{2,1}\ket{\rho_{p_1, p_2}}  
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:2} \\ 
& =  
\ket{p_1, p_2}_{\reg{p_1p_2}}\ket{\rho^{(1)}_{p_1, p_2}} 
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3}
,\end{align*}
where
\begin{itemize}
\item 
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:1} follows by defining $\ket{\rho_{p_1, p_2}}  \coloneqq \bra{p_1, p_2}_{\reg{p_1p_2}}A_2U_{gc} S \ket{\rho}$;

\item 
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:2} follows from the definitions of $B_2$, $C_2$, and $D_2$ (see \Cref{re-define:unitaries});

\item 
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3} follows by defining $\ket{\rho^{(1)}_{p_1, p_2}} \coloneqq D_{2,1} C_{2,1} B_{2,1}\ket{\rho_{p_1, p_2}}$.
\end{itemize}
% \begin{align*}
% \ket{\phi^{(1)}} 
% & =  
% D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}A_2U_{gc} S   
% \bigg(
% \ket{p_1}_{\reg{p_1}}\ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}} C_{1,0} \ket{\rho_{p'_1}}
% \bigg)
% \\
% & =  
% D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}   
% \bigg(
% \ket{p_1}_{\reg{p_1}} A_2U_{gc} S \ket{\rho_{p_1}} + \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  A_2U_{gc}S C_{1,0}\ket{\rho_{p'_1}}
% \bigg)
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:1}\\
% & =  
% D_2C_2B_2\ketbra{p_1, p_2}_{\reg{p_1p_2}}   
% \bigg(
% \ket{p_1}_{\reg{p_1}} \sum_{p'_2 \in \bits^\ell} \ket{p'_2}_{\reg{p_2}} \ket{\rho_{p_1, p'_2}} + \\ 
% & \hspace{18em}
%  \sum_{p'_1 \in \bits^\ell \setminus \Set{p_1}} \ket{p'_1}_{\reg{p_1}}  \sum_{p'_2 \in \bits^\ell} \ket{p'_2}_{\reg{p_2}} \ket{\rho_{p_1, p'_2}}
% \bigg)
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:2}\\ 
% & =  
% D_2C_2B_2\ket{p_1, p_2}_{\reg{p_1p_2}} \ket{\rho_{p_1, p_2}} \\ 
% & =  
% \ket{p_1, p_2}_{\reg{p_1p_2}}D_{2,1}C_{2,1}B_{2,1}\ket{\rho_{p_1, p_2}} 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3}\\ 
% & =  
% \ket{p_1, p_2}_{\reg{p_1p_2}}\ket{\rho^{(1)}_{p_1, p_2}} 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:4}
% ,\end{align*}
% where
% \begin{itemize}
% \item
% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:1} follows from the fact that $A_2$, $U_{gc}$  and $S$ act as the identity operator on $\reg{p_1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});
% \item
% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:2} follows from expanding the $\reg{p_2}$ register in the computational basis for states $A_2U_{gc} S \ket{\rho_{p_1}}$ and $A_2U_{gc} S C_{1,0} \ket{\rho_{p'_1}}$;
% \item
% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3} follows from the definitions of $B_2$, $C_2$, and $D_2$ (see \Cref{re-define:unitaries});
% \item
% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:4} follows by defining $\ket{\rho^{(1)}_{p_1, p_2}} \coloneqq D_{2,1}C_{2,1}B_{2,1}\ket{\rho_{p_1, p_2}}$.
% \end{itemize}
It is straightforward that the $\ket{\phi^{(1)}}$ shown in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3} satisfies the format shown in \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1} when $t = 1$.

Also, note that the game $H^{(J, \msf{pat})}_1$ and $H^{(J, \msf{pat})}_2$ are identical so far and thus $\ket{\phi^{(1)}} = \ket{\psi^{(1)}}$. Therefore, it follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:base:eq:3} that 
$$\ket{\psi^{(1)}} =  \ket{p_1, p_2}_{\reg{p_1p_2}} \ket{\rho^{(1)}_{p_1,p_2}}.$$ Such a $\ket{\psi^{(1)}}$ satisfies the format shown in \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2} with $t = 1$ as well.

This finishes the proof for the base case $t =1$.



\subsubsection{Induction Step ($t \ge 2$)} 
\label{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec} 

We assume $\ket{\phi^{(t-1)}}$ and $\ket{\psi^{(t-1)}}$ satisfy \Cref{lem:CPM-3ZK-hyb12:proof:invariant}, and show in the following that \Cref{lem:CPM-3ZK-hyb12:proof:invariant} holds when the global counter reaches $2$ for the $t$-th time.

We first describe formally how $\ket{\phi^{(t-1)}}$ (resp.\ $\ket{\psi^{(t-1)}}$) evolves into $\ket{\phi^{(t)}}$ (resp.\ $\ket{\psi^{(t)}}$):
\begin{enumerate}
 \item
$\Sim$'s local unitary $S$ is applied (followed by the projector $\ketbra{\uparrow}_{\reg{u}}$ which we hide as per \Cref{rmk:CPM-3ZK:hid-proj-u}). Note that this step is identical for both $H^{(J, \msf{pat})}_1$ and $H^{(J, \msf{pat})}_2$. 

\item
An $\uparrow$-query is made, bringing the global counter from 2 to 1. According to the notation in \Cref{MnR:game:redefine:hybrids}: 
\begin{itemize}
    \item
    In $H^{(J, \msf{pat})}_1$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_2 B^\dagger_2 C^\dagger_2 D^\dagger_2$; 
    \item
    In $H^{(J, \msf{pat})}_2$, this corresponds to applying $U^{\dagger}_{gc} A^\dagger_2 \ddot{C}^\dagger_2 D^\dagger_2$. 
\end{itemize}
\item \label[Step]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:description:def:lambda}
At this point, there are two cases to consider: 
\begin{enumerate}
\item \label[Case]{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-1}
 $\Sim$ can make a $\downarrow$-query immediately, bringing the global counter back to $2$; {\em or } 
\item \label[Case]{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-2}
 $\Sim$ can rewind the verifier $\tilde{\Verifier}$ further, bringing the global counter to $0$.  
\end{enumerate}
{\bf Defining Operator $\Lambda$:} Looking ahead, our proof can handle these two cases at one stroke. To do that, we denote the execution from this point until (exclusively) {\em the next $\downarrow$ query that brings the global counter to value $2$} (i.e., the exact query that yields the global counter's $t$-th arrival at value $2$) as an operator $\Lambda$. $\Lambda$ might be $\Sim$ local operator $S$ {\em only}, corresponding to \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-1}; $\Lambda$ might also be the combonation of some other operators, representing the operations performed in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:case-2-2} before the global counter's next arrival at value 2. 

\item
After the application of the operator $\Lambda$ defined above, an $\downarrow$-query is made, bringing the global counter from 1 back to 2, which is the global counter's $t$-th arrival at value 2. According to the notation in \Cref{MnR:game:redefine:hybrids}:  
\begin{itemize}
    \item
    In $H^{(J, \msf{pat})}_0$, this corresponds to applying $D_2C_2B_2A_2U_{gc}$; 
    \item
    In $H^{(J, \msf{pat})}_1$, this corresponds to applying $D_2\ddot{C}_2A_2U_{gc}$. 
\end{itemize} 
\end{enumerate}
It follows from the above description that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ can be written as:
\begin{align}
\ket{\phi^{(t)}}
& = D_2C_2B_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 B^\dagger_2 C^\dagger_2 D^\dagger_2 S  \ket{\phi^{(t-1)}}, \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1}\\ 
\ket{\psi^{(t)}}
& = D_2 \ddot{C}_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 \ddot{C}^\dagger_2 D^\dagger_2 S \ket{\psi^{(t-1)}}. \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2}
\end{align}

We first make a useful claim that specifies the registers on which the $\Lambda$ defined above acts non-trivially. 
\begin{MyClaim}[Non-Trivial Registers for $\Lambda$]\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}
The $\Lambda$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:description:def:lambda} acts non-trivially only on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$ (i.e., it works as the identity operator on the other registers). 
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}]

By definition, $\Lambda$ only contains operations that happen when the global counter is $1$ or smaller. This is best illustrated by \Cref{figure:CPM-3ZK:hybrids:H1}---$\Lambda$ only contains operations that happen in between the line corresponding to $\ket{0}_{\reg{gc}}$ and the line corresponding to $\ket{1}_{\reg{gc}}$. That is, all the $\downarrow$ and $\uparrow$ queries are answered by the ``dummy'' operators $\ddot{V}$ and $\ddot{V}^\dagger$. (One exception is the $\tilde{V}$ corresponding $\msf{sq}(1)$. But this does not matter in the current proof---Before the application of operator $\Lambda$, the global counter has already been $2$ (for $t-1$ times), which implies that the $\msf{sq}(1)$ query has already happened and thus cannot be a part of the operator $\Lambda$.)

Therefore, according to our notation in \Cref{MnR:game:redefine:hybrids}, operator $\Lambda$ can be written as $\Lambda = \Gamma_z \Gamma_{z-1} \cdots \Gamma_1$ (for some integer $z$) where each $\Gamma_i$ ($i \in [z]$) comes from the set of operators $\Set{S, A_1,  \ddot{C}_1, D_1, U_{gc}}$. It then follows from \Cref{CPM-3ZK:non-trivial-registers:table} that $\Lambda$ acts non-trivially only on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$.

This completes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}.

\end{proof}

\para{High-Level Idea for the Sequel.} Recall that our eventual goal is to prove that the states $\ket{\phi^{(t)}}$ and $\ket{\psi^{(t)}}$ are of the format shown in \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1,lem:CPM-3ZK-hyb12:proof:target-format:H2} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. At a high level, we prove it by applying \Cref{lem:err-inv-com} to \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2}. But we first need to perform some preparation work, putting \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2} into a format that is more ``compatible'' with \Cref{lem:err-inv-com}. In the sequel, we first perform the preparation work in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}. Then, we show on \Cpageref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish} how to use \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} to complete the proof for the induction step. 





The following \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} can be viewed as an analog of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim}.
\begin{MyClaim}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}
There exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds
\begin{align*}
\ket{\phi^{(t)}}
& =  
D_2C_2 B_2 U_{gc} \Lambda^{\reg{p_2}/\reg{m}} U_{gc}^\dagger   B^\dagger_2 C^\dagger_2
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}  
+ \\ 
& \hspace{16em} 
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\bigg) \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} \\ 
\ket{\psi^{(t)}}
& = 
D_2\ddot{C}_2 U_{gc}\Lambda^{\reg{p_2}/\reg{m}}  U_{gc}^\dagger \ddot{C}^\dagger_2 
\bigg( 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}   +  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\bigg) 
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} 
\end{align*}
where $\Lambda^{\reg{p_2}/\reg{m}}$ is identical to the $\Lambda$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:description:def:lambda}, except that it treats register $\reg{p_2}$ as $\reg{m}$, and the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}]
First, notice that  
\begin{align*}
 A_2 U_{gc} \Lambda U^\dagger_{gc} A^\dagger_2 
 & = 
 A_2 U_{gc} \Lambda A^\dagger_2 U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:1} \\ 
 & = 
 A_2 U_{gc} A^\dagger_2 \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:2} \\
  & = 
 A_2 A^\dagger_2 U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:3} \\
 & = 
U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}
 \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:1,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:3} follows from the fact that $U_{gc}$ acts non-trivially on different registers from $A_2$;

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S:2} from the fact that $\Lambda$ acts as the identity operator on $\reg{p_2}$ (see \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim}) and that $A_2$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_2}$ (see \Cref{CPM-3ZK:V:unitary}). 
\end{itemize}

\subpara{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(t)}}$:
\begin{align*}
\ket{\phi^{(t)}}
& =
D_2C_2B_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 B^\dagger_2 C^\dagger_2 D^\dagger_2  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:0} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2 D^\dagger_2  S \ket{\phi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:1} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2 D^\dagger_2 S 
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:2} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2 D^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} SC_{2,0} B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:3} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} S C_{2,0}  B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:4} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} S^{\reg{t_2}/\reg{m}}  B^\dagger_{2,1} C^\dagger_{2,1} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:5} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  S^{\reg{t_2}/\reg{m}}  \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:6} \\ 
& =
D_2C_2B_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} B^\dagger_2 C^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}  + \\ 
& \hspace{16em}
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}     \ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H1};

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S};

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:2} follows from our induction assumption;

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:3} from  from the fact that $S$ acts as the identity operator on $\reg{p_1}$ and $\reg{p_2}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:4} from the definition of $D_2$ (see \Cref{re-define:unitaries});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:5} from the fact that $S$ acts as the identity operator on $\reg{t_2}$ (see \Cref{CPM-3ZK:non-trivial-registers:table}) and $C_{2,0}$ is nothing but a swap operator between $\reg{t_2}$ and $\reg{m}$ (see \Cref{re-define:unitaries}); (Note that $S^{\reg{t_2}/\reg{m}}$ is defined to be an operator that is identical to $S$ except that it treats $\reg{t_2}$ as $\reg{m}$.)

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:6} follows from the fact that $S^{\reg{t_2}/\reg{m}}$ acts non-trivially on different registers from $B_{2,1}$ and $C_{2,1}$ (see \Cref{CPM-3ZK:non-trivial-registers:table});

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:7} follows by defining 
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho-dot}
\ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}   \coloneqq D^\dagger_{2,1} S \ket{\rho^{(t-1)}_{p_1,p_2}} ~~~\text{and}~~~
\ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}  \coloneqq S^{\reg{t_2}/\reg{m}} \ket{\rho^{(t-1)}_{p'_1,p'_2}} ~~\big(\forall (p'_1,p'_2) \in \big(\bits^\ell \times \bits^\ell\big) \setminus \Set{(p_1,p_2)}\big).
\end{equation}
\end{itemize}
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\subpara{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi}.} We now show the derivation for $\ket{\psi^{(t)}}$. This is almost identical to the above proof for \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.


\begin{align*}
\ket{\psi^{(t)}}
& =
D_2\ddot{C}_2A_2U_{gc} \Lambda U^{\dagger}_{gc} A^\dagger_2 \ddot{C}^\dagger_2 D^\dagger_2  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:0} \\ 
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} \ddot{C}^\dagger_2 D^\dagger_2  S \ket{\psi^{(t-1)}}
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:1} \\ 
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} \ddot{C}^\dagger_2 D^\dagger_2 S 
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(t-1)}_{p_1,p_2}} 
+
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} C_{2,0} \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:2} \\  
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc} \ddot{C}^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} D^\dagger_{2,1} S\ket{\rho^{(t-1)}_{p_1,p_2}}  
+ 
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}  S^{\reg{t_2}/\reg{m}}  \ket{\rho^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:6} \\ 
& =
D_2 \ddot{C}_2  U_{gc} \Lambda^{\reg{p_2}/\reg{m}}  U^\dagger_{gc}  \ddot{C}^\dagger_2  
\bigg(
\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1,p_2}} 
+
 \sum_{(p'_1, p'_2) \ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}  \ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}
\bigg)
\numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:7} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:0} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:H2};

\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:eq:swap-S};


\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:2}  follows from our induction assumption;


\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:6} follows from a similar argument as we did to derive \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:6} from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:phi-derivation:2};


\item
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:7} follows from {\em the same definitions} of $\ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}$ and $\ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}$ as shown in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho-dot}.
\end{itemize}
\Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:psi-derivation:7} finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\vspace{1em}
This finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

\end{proof}

The following \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} can be treated as an analog of \Cref{lem:CPM-3ZK-hyb01:proof:invariant:proof:induction:case1:preparation-claim:2}. 
\begin{MyClaim}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}
Let $\Lambda^{\reg{p_2}/\reg{m}}$ and $\Set{\dot{\rho}^{(t-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ be as defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}. Let
\begin{align}
\ket{\gamma^{(t-1)}_0} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:in:0} \\ 
\ket{\gamma^{(t-1)}_1} 
& \coloneqq 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t-1)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}   \ket{\dot{\rho}^{(t-1)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:in:1} \\ 
\ket{\gamma^{(t)}_0} 
& \coloneqq 
C_2 B_2 U_{gc} \Lambda^{\reg{p_2}/\reg{m}} U_{gc}^\dagger   B^\dagger_2 C^\dagger_2 \ket{\gamma^{(t-1)}_0} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:0} \\ 
\ket{\gamma^{(t)}_1}
& \coloneqq 
\ddot{C}_2 U_{gc}\Lambda^{\reg{p_2}/\reg{m}}  U_{gc}^\dagger \ddot{C}^\dagger_2 
 \ket{\gamma^{(t-1)}_1}
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:1} 
.\end{align}
Then, there exist (possibly sub-normalized) pure states $\Set{\dot{\rho}^{(t)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds:
\begin{align}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:0} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}   \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}} 
\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:1} 
.\end{align}
\end{MyClaim}
\begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}]
This claim follows from an application of \Cref{lem:err-inv-com}, with the notation correspondence listed in \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}. We provide a detailed explanation below.
\begin{table}[!htb]
\centering
\caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}}
\label{lem:CPM-3ZK-hyb12:proof:cor-table}
\vspace{0.5em}
\begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
\toprule
 \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
\phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
\cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}  \\ 
\midrule
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$\reg{a}$    & $\reg{p_1}$, $\reg{p_2}$ & & $W_1$ & $C_{2,1}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1,p_2}_{\reg{p_1p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{m}$    & $\reg{m}$ & & $W_0$ & $C_{2,0}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1,p'_2}_{\reg{p_1p_2}}$  \\
\addlinespace[0.3em]
$\reg{t}$    & $\reg{t_2}$ & & $W$   & $C_{2}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p_1,p_2}}$  \\ 
\addlinespace[0.3em]
$\reg{s}$    & $\reg{u}$, $\reg{s}$, $\reg{t_1}$, $\reg{gc}$, $\reg{lc}$ & & $\tilde{W}$ & $\ddot{C}_2$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(t-1)}_{p'_1,p'_2}}$ \\ 
\addlinespace[0.3em]
$\reg{o}$    & other registers & & $U_1$ & $B_{2,1}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & $\ket{\gamma^{(t-1)}_0}$ \\ 
\addlinespace[0.3em]
   & & & $U$   & $B_2$ & & $\ket{\eta^{(\msf{in})}_1}$ & $\ket{\gamma^{(t-1)}_1}$  \\ 
\addlinespace[0.3em]
 &  & &   $S$   & $U_{gc}\Lambda^{\reg{p_2}/\reg{m}}U^\dagger_{gc}$ & &  $\ket{\rho^{(\msf{out})}_a}_\reg{mtso}$    & $\ket{\dot{\rho}^{(t)}_{p_1,p_2}}$  \\ 
\addlinespace[0.3em]
  &  & &   &  & &  $\ket{\rho^{(\msf{out})}_{a'}}_\reg{mtso}$     & $\ket{\dot{\rho}^{(t)}_{p'_1,p'_2}}$  \\  
  \addlinespace[0.3em]
 &  & & & & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\gamma^{(t)}_0}$  \\
\addlinespace[0.3em] 
  &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\gamma^{(t)}_1}$  \\   
\bottomrule
\end{tabular}
\end{table}

First, we argue that the premises in \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}:
\begin{itemize}
\item
\Cref{lem:err-inv-com} requires that $W_1$ should work as the identity operator on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} notation, this is satisfied by $C_{2,1}$ (playing the role of $W_1$) who works as identity on registers $\reg{u}$, $\reg{s}$, $\reg{t_1}$, $\reg{gc}$, and $\reg{lc}$ (playing the role of registers $\reg{s}$). (Recall $C_{2,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)


\item
\Cref{lem:err-inv-com} requires that $W_0$ should be the swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} notation, this is satisfied by $C_{2,0}$ (playing the role of $W_0$), who is the swap operator between registers $\reg{m}$ and $\reg{t_2}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively). (Recall $C_{2,0}$ from \Cref{re-define:unitaries}.)

\item
\Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_0$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} notation, this is satisfied by $\ddot{C}_2$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1, p_2}_{\reg{p_1p_2}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $C_{2,0}$ (playing the role of $W_0$) on branches $\ket{p'_1, p'_2}_{\reg{p_1p_2}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, p'_2) \ne (p_1, p_2)$. (Recall $\ddot{C}_2$ from \Cref{re-define:unitaries})

\item
 \Cref{lem:err-inv-com} requires that $U_1$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} notation, this is satisfied by $B_{2,1}$ (playing the role of $U_1$), who works as identity on registers $\reg{u}$, $\reg{s}$, $\reg{t_1}$, $\reg{gc}$, and $\reg{lc}$ (playing the role of register $\reg{s}$). (Recall $B_{2,1}$ from \Cref{CPM-3ZK:non-trivial-registers:table}.)

\item
 \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} notation, this is satisfied by $U_{gc}\Lambda^{\reg{p_2}/\reg{m}}U^\dagger_{gc}$ (playing the role of $S$)---recall from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:Lambda-register:claim} that $\Lambda$ acts non-trivially on registers $\reg{m}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$. Thus, $U_{gc}\Lambda^{\reg{p_2}/\reg{m}}U^\dagger_{gc}$ acts non-trivially on registers $\reg{p_2}$, $\reg{u}$, $\reg{s}$, $\reg{p_1}$, $\reg{t_1}$, $\reg{lc}$, and $\reg{gc}$, which constitute registers $\reg{a}$ and $\reg{s}$ (see \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}). 
\end{itemize}

Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:CPM-3ZK-hyb12:proof:cor-table}) to the $\ket{\gamma^{(t-1)}_0}$ and $\ket{\gamma^{(t-1)}_1}$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:in:0,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:in:1}  (playing the role of $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ in \Cref{lem:err-inv-com}). This implies the existence of (possibly sub-normalized) pure states $\Set{\ket{\dot{\rho}^{(t)}_{p'_1,p'_2}}}_{(p'_1, p'_2)\in\bits^\ell \times \bits^\ell}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
\begin{align*}
\ket{\gamma^{(t)}_0} 
& =
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}   \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}} \\ 
\ket{\gamma^{(t)}_1} 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1, p_2}}  
+  
\sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}   C_{2,0}   \ket{\dot{\rho}^{(t)}_{p'_1, p'_2}}  
,\end{align*}
which are exactly \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:0,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:1} in  \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}. 






This completes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}.

\end{proof}





% \begin{MyClaim}
% % \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}
% There exist (potentially sub-normalized) pure states $\Set{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}_{(p'_1,p'_2 ) \in \bits^\ell\times\bits^\ell}$ so that the following holds
% \begin{align}
% \ket{\phi^{(k)}}
% & = \tilde{U}_6 \tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}}   \tilde{U}^\dagger_5 \tilde{U}^\dagger_6
% \bigg( 
% \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} \\ 
% \ket{\psi^{(k)}}
% & = 
% B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}}  B^\dagger_{\msf{dmy}}
% \bigg( 
% \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \bigg) \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} 
% \end{align}
% where $\Lambda^{\reg{p_2}/\reg{m}}$ is identical to $\Lambda$ except that it treats register $\reg{p_2}$ as $\reg{m}$, and the summations are taken over all $(p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}$ (abbreviated as $(p'_1, p'_2) \ne (p_1, p_2)$ in the above).
% \end{MyClaim}
% \begin{proof}[Proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}]
% First, notice that
% \begin{equation}\label{lem:CPM-3ZK-hyb12:proof:case-2:eq:swap-Lambda} 
% \tilde{U}_4 \Lambda \tilde{U}^\dagger_4 = \tilde{U}_4  \tilde{U}^\dagger_4 \Lambda^{\reg{p_2}/\reg{m}} = \Lambda^{\reg{p_2}/\reg{m}},
% \end{equation}
% where the first equality follows from the fact that $\Lambda^{\reg{p_2}/\reg{m}}$ does not operate on $\reg{p_2}$ and $\tilde{U}^\dagger_4$ is nothing but a swap operator between $\reg{m}$ and $\reg{p_2}$.

% \para{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}.} We now show the derivation for $\ket{\phi^{(k)}}$:

% \begin{align*}
% \ket{\phi^{(k)}}
% & = 
% \tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \ket{\phi^{(k-1)}} \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1} \\
% & = 
% \tilde{U}_6\tilde{U}_5\tilde{U}_4 \Lambda \tilde{U}^\dagger_4 \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6  S_j \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} S_j \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}
% ,\end{align*}
% where \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:1}  follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:phi}, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2} follows from our induction assumption, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:3} follows from \Cref{lem:CPM-3ZK-hyb12:proof:case-2:eq:swap-Lambda}, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:4}  follows from the fact that $S_j$ works as identity on registers $\reg{p_1}$ and $\reg{p_2}$ (see \Cref{CPM-3ZK:table:non-trivial-registers}), \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:5}  follows from the definitions of $\tilde{U}_{6,1}$ and $S^{\reg{t_2}/\reg{m}}_j$, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6}  follows from the fact that $S^{\reg{t_2}/\reg{m}}_j$ and $\tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} $ act non-trivially on different registers (see \Cref{CPM-3ZK:table:non-trivial-registers}), and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  follows by defining
% \begin{equation}
% \label[Expression]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}
% \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}} \coloneqq S_j \ket{\rho^{(k-1)}_{p_1, p_2}} ~~~\text{and}~~~ \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}} \coloneqq S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}~~~(\forall (p'_1, p'_2) \in \bits^{\ell} \times  \bits^{\ell} \setminus \Set{(p_1, p_2)}).
% \end{equation}
% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:7}  finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

% \para{Proving \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi}.} This proof is almost identical to the above proof for \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi}. Nevertheless, we present it for the sake of completeness.
% \begin{align*}
% \ket{\psi^{(k)}}
% & = 
% B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \ket{\psi^{(k-1)}} \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} \\
% & = 
% B_{\msf{dmy}} \tilde{U}_4  \Lambda \tilde{U}^\dagger_4 B^\dagger_{\msf{dmy}}  S_j \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}\ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1}  \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2} \\ 
% & =
% B_{\msf{dmy}} \Lambda^{\reg{p_2}/\reg{m}} B^\dagger_{\msf{dmy}} \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} S_j \ket{\rho^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1} S^{\reg{t_2}/\reg{m}}_j \ket{\rho^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} \\ 
% & =
% \tilde{U}_6\tilde{U}_5 \Lambda^{\reg{p_2}/\reg{m}} \tilde{U}^\dagger_5 \tilde{U}^\dagger_6 \cdot \bigg( 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}  \ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2)} \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}  \tilde{U}_{6,1}  \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}
% \bigg) 
% \numberthis \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}
% ,\end{align*}
% where \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:eq:k:psi}, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:2}  follows from our induction assumption, \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:3} follows from a similar argument as we did to \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:6} from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:phi:2}, and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4} follows from the same definition of $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$ and $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ as shown in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:def:rho-dot}

% \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:derivation:psi:4}  finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.


% This eventually finishes the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}.

% \end{proof}


% \para{Finishing the Induction Step.}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish} 
%  With the above \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} in hand, we can finish the induction step by applying \Cref{lem:err-inv-com}. Formally, we apply \Cref{lem:err-inv-com} to the states and operators in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}, with the notation correspondence listed in \Cref{lem:CPM-3ZK-hyb12:proof:induction:cor-table}. We provide a detailed explanation below.
% \begin{table}[!htb]
% \centering
% \caption{Notation Correspondence between \Cref{lem:err-inv-com} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}}
% \label{lem:CPM-3ZK-hyb12:proof:induction:cor-table}
% \vspace{0.5em}
% \begin{tabular}{ C{50pt} C{60pt} c C{50pt} C{60pt} c C{50pt} C{60pt} }
% \toprule
%  \multicolumn{2}{c}{Registers}   & \phantom{abc}   & \multicolumn{2}{c}{Operators}   &
% \phantom{abc}   & \multicolumn{2}{c}{Random Variables}  \\
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
% In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} & & In \Cref{lem:err-inv-com} & In \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim}  \\ 
% \midrule
% % \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
% \addlinespace[0.3em]
% $\reg{a}$    & $\reg{p_1}$, $\reg{p_2}$ & & $W_0$ & $\tilde{U}_{6,0}$ & & $\ket{a}_{\reg{a}}$    & $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$  \\ 
% \addlinespace[0.3em]
% $\reg{m}$    & $\reg{m}$ & & $W_1$ & $\tilde{U}_{6,1}$ & & $\ket{a'}_{\reg{a}}$    & $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$  \\
% \addlinespace[0.3em]
% $\reg{t}$    & $\reg{t_2}$ & & $W$   & $\tilde{U}_{6}$ & & $\ket{\rho^{(\msf{in})}_a}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p_1, p_2}}$  \\ 
% \addlinespace[0.3em]
% $\reg{s}$    & $\reg{t_1}$,  $\reg{u}$, $\reg{s}$ & & $\tilde{W}$ & $B_{\msf{dmy}}$ & & $\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}$    & $\ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}$ \\ 
% \addlinespace[0.3em]
% $\reg{o}$    & other registers & & $U_0$ & $\tilde{U}_{5,0}$ & &   $\ket{\eta^{(\msf{in})}_0}$ & \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0} \\ 
% \addlinespace[0.3em]
%    & & & $U$   & $\tilde{U}_{5}$ & & $\ket{\eta^{(\msf{in})}_1}$ & \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}  \\ 
%    \addlinespace[0.3em]
%  &  & & $S$   & $\Lambda^{\reg{p_2}/\reg{m}}$ & &  $\ket{\eta^{(\msf{out})}_0}$    & $\ket{\phi^{(\msf{k})}}$  \\ 
%   &  & &   &  & &  $\ket{\eta^{(\msf{out})}_1}$    & $\ket{\psi^{(\msf{k})}}$  \\   
% \bottomrule
% \end{tabular}
% \end{table}

% First, we argue that the premises of \Cref{lem:err-inv-com} are satisfied with the notation listed in \Cref{lem:CPM-3ZK-hyb12:proof:induction:cor-table}:
% \begin{itemize}
% \item
% \Cref{lem:err-inv-com} requires that $W_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,0}$ (playing the role of $W_0$) who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$ (playing the role of registers $\reg{s}$).

% \item
% \Cref{lem:err-inv-com} requires that $W_1$ should be a swap operator between $\reg{m}$ and $\reg{t}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{6,1}$ (playing the role of $W_1$), who is a swap operator between registers $\reg{m}$ and $\reg{t_2}$ (playing the role of $\reg{m}$ and $\reg{t}$ respectively).

% \item
% \Cref{lem:err-inv-com} requires that $\tilde{W}$ is the identity operator on branch $\ket{a}_{\reg{a}}$ and is identical to $W_1$ on branches $\ket{a'}_{\reg{a}}$ with $a' \ne a$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $B_{\msf{dmy}}$ (playing the role of $\tilde{W}$), who is the identity operator on branch $\ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}}$ (playing the role of $\ket{a}_{\reg{a}}$) and is identical to $\tilde{U}_{6,1}$ (playing the role of $W_1$) on branches $\ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}$ (playing the role of $\ket{a'}_{\reg{a}}$) with $(p'_1, p'_2) \ne (p_1, p_2)$.

% \item
%  \Cref{lem:err-inv-com} requires that $U_0$ should work as identity on register $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\tilde{U}_{5,0}$ (playing the role of $U_0$), who works as identity on registers $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of register $\reg{s}$).

% \item
%  \Cref{lem:err-inv-com} requires that $S$ should act non-trivially {\em only} on registers $\reg{a}$ and $\reg{s}$. In terms of the \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} notation, this is satisfied by $\Lambda^{\reg{p_2}/\reg{m}}$ (playing the role of $S$), who does not touch registers beyond $\reg{p_1}$, $\reg{p_2}$,  $\reg{t_1}$, $\reg{u}$, and $\reg{s}$  (playing the role of registers $\reg{a}$ and $\reg{s}$).
% \end{itemize}

% Next, using the above notation, we could define
% \begin{align}
% \ket{\eta^{(\msf{in})}_0}
% & \coloneqq 
% \ket{p_1}_{\reg{p_1}}\ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}}\ket{p'_2}_{\reg{p_2}}   \tilde{U}_{6,1}  \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{4,0} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}, \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0}  \\ 
% \ket{\eta^{(\msf{in})}_1}
% & \coloneqq 
%  \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(k-1)}_{p_1,p_2}}  +  \sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\dot{\rho}^{(k-1)}_{p'_1, p'_2}}.  \label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}   
% \end{align}

% Finally, we apply \Cref{lem:err-inv-com} (with the notation in \Cref{lem:CPM-3ZK-hyb12:proof:induction:cor-table}) to the $\ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{in})}_1}$ defined in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-0,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish:def:eta-in-1}. This implies the existence of (potentially non-normalized) pure states $\Set{\ket{\rho^{(k)}_{p'_1, p'_2}}}_{(p'_1, p'_2) \in\bits^\ell \times \bits^\ell}$  (playing the role of $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a'\in\bits^\ell }$ in \Cref{lem:err-inv-com}) such that the following holds
% \begin{align*}
% \ket{\phi^{(k)}} 
% & = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \tilde{U}^\dagger_{5,0} \tilde{U}^\dagger_{6,0} \ket{\rho^{(k)}_{p'_1,p'_2}} \\ 
% \ket{\psi^{(k)}} 
% & = \ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(k)}_{p_1, p_2}}  +  \sum_{(p'_1, p'_2)\ne (p_1, p_2) } \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}} \tilde{U}_{6,1} \ket{\rho^{(k)}_{p'_1,p'_2}} 
% ,\end{align*}
% which are exactly \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1,lem:CPM-3ZK-hyb12:proof:target-format:H2} in  \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. 

% This finishes the induction step.


% \vspace{1em}
% Finally, we remark that our proof for the base case in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec}   together finish the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant} eventually.




\para{Finishing the Proof for the Induction Step.}\label{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:finish} With \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim,lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2} at hand, we now finish the proof for the induction Step.

\subpara{Proof for \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1}.} We first establish \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1}:
\begin{align}
\ket{\phi^{(t)}} 
& = D_2 \ket{\gamma^{(t)}_0} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:1} \\ 
& = D_2 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\bigg) 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} D_{2,1} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} B^\dagger_{2,1} C^\dagger_{2,1}  \ket{\rho^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:phi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:0} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:2} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:0} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:3} follows from the definition of $D_2$ (see \Cref{re-define:unitaries});

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:4} follows by defining
\begin{equation}
\label[Expression]{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho}
\ket{\rho^{(t)}_{p_1,p_2}}   \coloneqq D_{2,1} \ket{\dot{\rho}^{(t)}_{p_1,p_2}} ~~~\text{and}~~~
\ket{\rho^{(t)}_{p'_1,p'_2}}  \coloneqq \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} ~~\big(\forall (p'_1, p'_2) \in \big(\bits^\ell \times \bits^\ell\big) \setminus \Set{(p_1,p_2)}\big).
\end{equation}
\end{itemize}
Note that \Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:phi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb12:proof:target-format:H1} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. 


\subpara{Proof for \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2}.} We next establish \Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2}:
\begin{align}
\ket{\psi^{(t)}} 
& = D_2 \ket{\gamma^{(t)}_1} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:1} \\ 
& = D_2 
\bigg(
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0} \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\bigg) 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:2} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} D_{2,1} \ket{\dot{\rho}^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}   \ket{\dot{\rho}^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:3} \\ 
& = 
\ket{p_1}_{\reg{p_1}} \ket{p_2}_{\reg{p_2}} \ket{\rho^{(t)}_{p_1,p_2}}  
+  
\sum_{(p'_1, p'_2) \ne (p_1, p_2)}  \ket{p'_1}_{\reg{p_1}} \ket{p'_2}_{\reg{p_2}}  C_{2,0}  \ket{\rho^{(t)}_{p'_1,p'_2}} 
\label{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:4} 
,\end{align}
where 
\begin{itemize}
\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:1} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:eq:target:psi} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim} and \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:out:1} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2}; 

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:2} follows from \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2:eq:target:1} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:2};

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:3} follows from the definition of $D_2$ (see \Cref{re-define:unitaries});

\item
\Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:4} follows from {\em the same definitions} of $\ket{\rho^{(t)}_{p_1, p_2}}$ and $\ket{\rho^{(t)}_{p'_1, p'_2}}$ in \Cref{lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:preparation-claim:proof:def:rho}.
\end{itemize}
Note that \Cref{CPM-3ZK-hyb12:proof:invariant:proof:induction:final:psi:4} is exactly 
\Cref{lem:CPM-3ZK-hyb12:proof:target-format:H2} in \Cref{lem:CPM-3ZK-hyb12:proof:invariant}. 

This finishes the proof of the induction step of \Cref{lem:CPM-3ZK-hyb12:proof:invariant}.

\vspace{1em}
Finally, we remark that our proof for the base case in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:base:sec} and the proof for the induction step in \Cref{sec:lem:CPM-3ZK-hyb12:proof:invariant:proof:induction:sec} together finish the proof of \Cref{lem:CPM-3ZK-hyb12:proof:invariant}, which in turn finishes the proof of \Cref{lem:CPM-3ZK:H12} eventually.


==> sections/QCCC.tex <==
\section{Impossibility in the QCCC model}


Similar as \cite{FOCS:CCLY21}, we first show the impossibility result with an inefficient $\tilde{V}$. The inefficiency is only due to a random function $H$ hard-wired in $\tilde{V}$. We will make $\tilde{V}$ efficient later by replacing $H$ by a $q$-wise independent hash.


\subsection{The Model}

\para{Round Numbering.} W.l.o.g., we assume that the protocol has $2k$ rounds of the form\footnote{Note that this form means that the verifier sends the first message. To capture protocols where the prover sends the first message, one can add an extra $a_0$ message from the prover at the beginning. Our results hold for this case as well.}
 $$(p_1, v_1, p_2, v_2, \ldots, p_k, v_k, p_{k+1}),$$ 
where $\Set{p_1, \ldots, p_{k+1}}$ are prover messages and $\Set{v_1, \ldots, v_k}$ are verifier messages. We assume that all the messages are of the same length $\ell(\secpar)$.

% We focus on a $k$ round protocol where $k$ is an  constant even number. We denote the messages as $\Set{m_1, \ldots, m_k}$. W.l.o.g., we assume that the $V$ sends the first message and $P$ sends the last message. That is, for all $i \in \Set{1, \ldots, k/2}$, it holds that $m_{2i-1}$ is a verifier message and $m_{2i}$ is a prover message.





\para{$\tilde{V}$'s Registers.} $\tilde{V}$ starts by initializing the following registers (see \Cref{figure:QCCC-V:registers} for an explanation):
\begin{equation}\label[Expression]{QCCC:V:inital:expr}
\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{p_1}}\ket{\vb{0}}_{\reg{v_1}} \ldots \ket{\vb{0}}_{\reg{p_k}}\ket{\vb{0}}_{\reg{v_k}} \ket{\vb{0}}_{\reg{p_{k+1}}} \ket{1}_{\reg{f_1}} \ldots \ket{1}_{\reg{f_k}} \ket{\vb{0}}_{\reg{m}} \ket{0}_{\reg{Out}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w}
\end{equation}


\begin{FigureBox}[label={figure:QCCC-V:registers}]{Registers}
We explain the meaning of the registers defined in \Cref{QCCC:V:inital:expr}:
\begin{itemize}
    \item
    $\reg{ins}$ stores the input instance $x$;
\item
$\Set{\reg{p_1}, \reg{v_1}, \reg{p_k}, \reg{v_k},\ldots,  \reg{p_{k+1}}}$ will be used to store the execution transcript (i.e., the messages $\Set{{p}_1, {v}_1, {p}_k, {v}_k, \ldots, {p}_{k+1}}$ exchanged between the prover and verifier); As will become clear in our proof, storing all the exchanged messages turns out to be critical for our proof to work.

\item
$\Set{\reg{f_1}, \ldots, \reg{f_k}}$ are $k$ flags registers, each containing a single qubit. They will be used to make sure that the simulator must ``return'' the original message without modification when she wants to rewind/un-compute a certain round. See \red{ref:XXX} for details. 

\item
$\reg{m}$ is the register to store messages from/to the prove.

\item
$\reg{out}$ is a single-qubit register to store the verifier's final decision (Let 0 denote rejection and 1 denote acceptance).

\item
$\reg{aux}$ stores the truth table of the random function $H$. This is the only register that is of super-polynomial size. 

\item
$\reg{w}$ is the working space of the verifier initialized with enough ancilla qubits that will be used for purposes like purification and dilation etc.

\end{itemize}
% We emphasize that all of these registers need to be initialized to proper length. To simplify the notation, we do not specify the length of them. But it is easy to see that their length is bounded by a fixed polynomial of the security parameter, and this polynomial can be determined in advance. 
\end{FigureBox}

\para{$\tilde{V}$'s Unitary.}  We next describe the unitary $\tilde{U}$ for $\tilde{V}$. We describe $\tilde{V}$'s behavior for the first $k$ moves together, and the final $(k+1)$-th move (i.e., $\tilde{V}$'s final decision) separately:

\subpara{Unitary $\tilde{U}_i$ for Round $i \le k$:} Upon receiving message $p_i$ in register $\reg{m}$, $\tilde{V}$ proceeds as follows:
\begin{enumerate}
\item
Conditioned on $\ket{1}_{\reg{f_i}}$,\footnote{This is a shortcut for the following sentence ``it first checks if the $\reg{f_i}$ register contains $1$; if so, it execute the following instruction, otherwise, it does nothing.'' We will use this convention through out the description of $\tilde{V}$.} it swaps the contents between $\reg{m}$ and $\reg{p_i}$;
\item
Conditioned on $\ket{1}_{\reg{f_i}}$, it applies a unitary $F_i$ that is defined as follows: 
% \begin{equation}
% F\coloneqq 
% \begin{cases}
% I & H(p_1, v_1, \ldots, p_i) = 0 \\
% U & H(p_1, v_1, \ldots, p_i) = 1
% \end{cases}
% \end{equation}
\begin{enumerate}
\item
If $H(p_1, v_1, \ldots, p_i) = 0$, then do nothing;
\item
If $H(p_1, v_1, \ldots, p_i) = 1$, then apply $U_i$. 
\end{enumerate}
\begin{MyComment}
Recall \xiao{from XXX} that $U_i$ is the unitary of the honest verifier $V$ for the $i$-th move, which works non-trivially on registers $\reg{ins}$,  $\Set{\reg{p_j}, \reg{v_j}}_{j \in [i]}$, and $\reg{w}$. In particular, it generates the next verifier message $v_i$ on register $\reg{v_i}$ (together with some residual state on $\reg{w}$).
\end{MyComment}

\item
Conditioned on $\ket{1}_{\reg{f_i}}$, it sets the content in register $\reg{m}$ to $\ket{m \xor v_i}_{\reg{m}}$, where $m$ is the original content in register $\reg{m}$ and $v_i$ is the content in register $\reg{v_i}$. 

\begin{MyComment}
Note that this step can be understood as a controlled-XOR gate that is controlled by the $\reg{f_i}$ register to xor the $\reg{v_i}$ register into the $\reg{m}$ register.  It is  worth noting that in the real execution, the original content $m$ is nothing but a  all-0 string; In that case, this step is simply copy $\reg{v_i}$ into $\reg{m}$ (of course, controlled by $\reg{f_i}$).
\end{MyComment}

\item
Conditioned on $\ket{1}_{\reg{f_i}}$, do the following: Compare the contents of $\reg{v_i}$ and $\reg{m}$; If they are equal, modify the $\reg{f_i}$ register to $\ket{f \xor 1}_{\reg{f_i}}$, where $f$ is the original content on $\reg{f_i}$; Otherwise, do nothing.

\begin{MyComment}
Note that this step can be understood as first write the value $\neg (v_i \xor m)$ into a register $\reg{t}$ in the working space. Then,  apply a $\msf{CNOT}$ on  (the control register) $\reg{t}$ and  (the target register) $\reg{f_i}$. Note that in the real execution, the register $\reg{f_i}$ will contain a classical bit 0 after this step, because the original content $f$ is 1 and $\reg{v_i}$ and $\reg{m}$ have exactly the same content, right before this step (in the real execution).
\end{MyComment}
\end{enumerate}



\subpara{Unitary $\tilde{U}_{k+1}$ Round $k+1$:} 
\begin{enumerate}
\item
Upon receiving the last message $p_{k+1}$ in register $\reg{m}$, swap the registers $\reg{m}$ and $\reg{p_{k+1}}$. 
\item
it applies a unitary $F_{k+1}$ that is defined as follows: 
% \begin{equation}
% F\coloneqq 
% \begin{cases}
% I & H(p_1, v_1, \ldots, p_i) = 0 \\
% U & H(p_1, v_1, \ldots, p_i) = 1
% \end{cases}
% \end{equation}
\begin{enumerate}
\item
If $H(p_1, v_1, \ldots, p_k, v_k, p_{k+1}) = 0$, then do nothing;
\item
If $H(p_1, v_1, \ldots, p_k, v_k, p_{k+1}) = 1$, then apply $U_{k+1}$. 
\end{enumerate}
\begin{MyComment}
Recall \xiao{from XXX} that $U_{k+1}$ is the unitary of the honest verifier $V$ for the $(k+1)$-th move, which works non-trivially on registers $\reg{ins}$,  $\Set{\reg{p_1}, \reg{v_1}, \ldots, \reg{p_{k+1}}}_{j \in [i]}$, and $\reg{w}$. In particular, it generates the final output of the verifier on register $\reg{out}$ (together with some residual state on $\reg{w}$).
\end{MyComment}
\end{enumerate}

\UpdateLine 

\xiao{to do...}

\begin{remark}[On $\tilde{V}$'s Counter]
Note that the above description of $\tilde{V}$ implicitly assumes that $\tilde{V}$ knows in which round it is. This is without loss of generality because we can quip $\tilde{V}$ with a counter register recording the current round number in the same manner as \cite[Section 3.1]{FOCS:CCLY21}. Since this counter is not crucial to our security proof, we choose to omit it to keep notation succinct. 
\end{remark}






==> sections/Xiao-sketch.tex <==


\section{New Notes for Reduction to Soundness}

The final BQP decider is always defined as in \Cref{item:final:BQP:decider}. And the $x \in \Lang$ case can be handled as in \Cref{sec:xiao-sketch}. However, it seems the case $x \notin \Lang$ requires extra caution.

The logic chain should be as follows:
\begin{enumerate}
\item \label[Step]{item:soundness:step:1}
Assume that the BQP decider on input $x \notin \Lang$ make the final state of $\tilde{V}^{H_0}$ (in the MnR game) accept, with non-negligible probability.

\item \label[Step]{item:soundness:step:2}
Consider a new BQP decider who is identical to the one in \Cref{item:soundness:step:1}, except that this new decider halts immediately (and outputs `Reject') as long as the measured message (in the MnR game) starts to disorder.
\begin{itemize}
	\item
We will show that this new decider output `Reject' with a probability negligibly close to that in \Cref{item:soundness:step:1}.
\end{itemize}
Note that we are not making this claim for arbitrary protocols. Instead, here we use Kai-min's idea to include the `history' in every prover's message, plus a long random string from $V$ in each round, so that we can argue that the simulator cannot gain advantages to use incorrectly ordered messages (or to skip particular rounds---the long random string prevent this from happening).

\item \label[Step]{item:soundness:step:3}
Argue that the game in \Cref{item:soundness:step:2} is similar to the ``dummy-up-n-down'' game. This step makes use of the hybrids I designed, as well as the almost commutativity lemma. Note that with \Cref{item:soundness:step:2} in hand, the job of this step should become easier---\Cref{item:soundness:step:2} essentially allows us to sole focuses on correctly ordered messages.

\item \label[Step]{item:soundness:step:4}
We are ready to forward out the messages to an external honest verifier. Essentially, \Cref{item:soundness:step:3} ensures that the reduction doesn't need to keep the internal state $\tilde{V}$, and \Cref{item:soundness:step:2} ensures that no rewinding would happen (i.e., the messages are in the correct order).
\end{enumerate}

\subsection{Modified Malicious Verifiers (Version 1)}

We need to modify the malicious verifier we built before. The new $\tilde{V}$ has $k$ tokens $(t_1, \ldots, t_k)$ hard-wired in, one for each round, where each $t_i \picks \bits^\secpar$. Note that they are random and thus hard to predict.
\begin{enumerate}
\item
Recall that the messages of the protocol is named as $(p_1, v_1, p_2, v_2, \ldots, p_{k-1}, v_{k-1}, p_k)$.

\item
When $\tilde{V}$ sends $v_{i}$, it also sends $t_{i}$.

\item
We require the prover to include $t_{i}$ as a part of $p_{i+1}$. Upon receiving this $p_{i+1}$, 
\begin{enumerate}
 \item
 $\tilde{V}$ checks if $p_{i+1}$ includes the correct $t_{i}$ (as hard-wired in $\tilde{V}$). if this check fails, $\tilde{V}$ does not do anything; Otherwise, go to next step.
 \item
 If this step is reached, $\tilde{V}$ works as the previously defined $\tilde{V}$.
 \end{enumerate} 
\end{enumerate}



\subsection{Modified Malicious Verifiers (Version 2)}
\label{sec:new-malicous-V-counter}
I realized that we do not need the modifications shown in the previous subsection (i.e., version 1). I think the original CCLY model (with a slight modification) can already prevent the measured messages from being out of order. The CCLY model asks $V$ to keep a counter register, which will {\em increase immediately} when Sim/P makes a (down) query, before $V$ actually perform any operation to answer this query. We can modify this by asking the $V$ to perform $H$ query first; $V$ will only increase the counter only if it does perform the computation (i.e., $H$ instructs $V$ to answer on this query).  

By the above modification, we know that in the MnR game where we use a $H_0$ oracle, $Sim$ won't be able to skip rounds in the measured query. 


\para{More to say about the MnR game using the version-2 malicious verifiers.} I think we can claim that the MnR game with the version-2 malicious verifier enjoys the following specific properties:
\begin{enumerate}
\item
If we take a look at the measured queries, their length must be in strictly increasing order---one more measured query, one message longer.
\item
By definition of the MnR game, it seems possible that we end up measuring less than $k$ queries. However, for the particular version-2 $V^*$, we claim that this is indeed impossible (if we consider the predicate that $V^*$ eventually accept). The reason is: if less than $k$ queries are measured, then the counter will eventually contains a number smaller than $k$. $V^*$ will never accept when the counter has not reached $k$.

\end{enumerate}


\subsection{Branch-Wise Equivalence Lemma (New Version)}
\label{sec:branch-wise-equiv-lemma-new}

 Let $\ket{\phi^0}$ be a pure state over registers $\reg{m}$ and $\reg{o}$. Let $P = \Set{\Pi_0, \Pi_1}$ be a binary-outcome POVM over these registers. Consider the following game

\para{Game $G(\ket{\phi^0})$:} on input $\ket{\phi^0}$, it performs the following operations:
\begin{enumerate}
    \item 
    Apply $U_1$;
    \item
    Measure register $\reg{m}$ in computational basis;
    \item
    Apply $U_2$;
    \item
    Measure register $\reg{m}$ in computational basis;.
    \item
    Apply the POVM $P$ and output the measurement outcome.
\end{enumerate}

\begin{lemma}\label{lem:branchwise:preparation}
For each $m_1, m_2 \in \bits^\ell$, let $\ket{\psi^2_{m_1, m_2}} \coloneqq \ketbra{m_2}_{\reg{m}} U_2 \ketbra{m_1}_{\reg{m}} U_1\ket{\phi_0}$. Then, it holds that
$$\Pr[\msf{Out}(G(\ket{\phi^0})) = 1] = \sum_{m_1, m_2 \in \bits^\ell} \bra{\psi^2_{m_1, m_2}}\Pi_1\ket{\psi^2_{m_1, m_2}}.$$
\end{lemma}
\begin{proof}
Let's first track the steps in game $G(\ket{\phi^0})$. Right after $U_1$, the state can be written as
$$U_1 \ket{\phi^0} = \sum_{m_1} \alpha_{m_1} \ket{m_1}_{\reg{m}}\ket{\phi^1_{m_1}}_{\reg{m}}.$$
Measuring the $\reg{m}$ register results in the following mixture:
$$\text{with probability}~|\alpha_{m_1}|^2,~\text{collapsing to state}~\ket{m_1}\ket{\phi^1_{m_1}}.$$
\xiao{At the same time, we know that $\ket{\psi^1_{m_1}} \coloneqq \ketbra{m_1}U_1 \ket{\phi^0} = \alpha_{m_1} \ket{m_1}_{\reg{m}}\ket{\phi^1_{m_1}}_{\reg{m}}.$}

For each possible state $\ket{m_1}\ket{\phi^1_{m_1}}$, applying $U_2$ yields
$$U_2 \ket{m_1}\ket{\phi^1_{m_1}} = \sum_{m_2}\beta_{m_1, m_2} \ket{m_2}\ket{\phi^2_{m_1, m_2}}.$$


Measuring the $\reg{m_2}$ register results in the following mixture:
$$\text{with probability}~|\beta_{m_1,m_2}|^2,~\text{collapsing to state}~\ket{m_2}\ket{\phi^2_{m_1, m_2}}.$$
\xiao{At the same time, we know that  $\ket{\psi^2_{m_1, m_2}} = \ketbra{m_2} U_2 \ket{\psi^1_{m_1}} = \alpha_{m_1}  \beta_{m_1, m_2} \ket{m_2} \ket{\phi^2_{m_1, m_2}}$.}

Using the above notation, we can say that the state right before the POVM is applied is the following mixture:
$$\text{with probability}~|\alpha_{m_1}|^2 \cdot |\beta_{m_1,m_2}|^2,~\text{collapsing to state}~\ket{m_2}\ket{\phi^2_{m_1, m_2}}.$$
It then follows that 
\begin{align*}
\Pr\big[\msf{Out}(G(\phi^0)) = 1\big] 
& = 
\sum_{m_1, m_2} |\alpha_{m_1}|^2 \cdot |\beta_{m_1,m_2}|^2 \cdot \bra{m_2, \phi^2_{m_1, m_2}}\Pi_1\ket{m_2, \phi^2_{m_1, m_2}} \\ 
& = 
\sum_{m_1, m_2} \alpha^*_{m_1}\cdot \alpha_{m_1} \cdot \beta^*_{m_1,m_2} \cdot \beta_{m_1,m_2} \cdot \bra{m_2, \phi^2_{m_1, m_2}}\Pi_1\ket{m_2, \phi^2_{m_1, m_2}} \\ 
& = 
\sum_{m_1, m_2}   \bra{m_2, \phi^2_{m_1, m_2}}\alpha^*_{m_1}\beta^*_{m_1,m_2} \Pi_1 \alpha_{m_1} \beta_{m_1,m_2}\ket{m_2, \phi^2_{m_1, m_2}} \\ 
& = 
\sum_{m_1, m_2} \bra{\psi^2_{m_1, m_2}}\Pi_1\ket{\psi^2_{m_1, m_2}}
.\end{align*}


This finishes the proof of \Cref{lem:branchwise:preparation}. 

\end{proof}




\subsection{Branch-Wise Equivalence Lemma (Old Version 2)}


I think the following version of branch-wise equivalence lemma is what I want.

\para{Branch-Wise Equivalence (Baby Case).}
 Let $\ket{\eta^0}$ be a pure state over registers $\reg{m_1}$, $\reg{m_2}$, and $\reg{o}$. Let $\msf{pred}$ be a quantum predicate over these three registers. Consider the two games defined in \Cref{table:LOCC-3ZK:branch-wise:lem:new}. Also, for any classical strings $m_1$ and $m_2$, define the following (sub-normalized) states:
\begin{align*}
 \ket{\phi^1_{m_1}} & \coloneqq \ketbra{m_1}_\reg{m_1} U_1 \ket{\eta_0} \\
 \ket{\phi^2_{m_1,m_2}} & \coloneqq \ketbra{m_2}_\reg{m_2} U_2 \ketbra{m_1}_\reg{m_1} U_1 \ket{\eta_0} \\
 \ket{\tilde{\phi}^1_{m_1}} & \coloneqq \ketbra{m_1}_\reg{m_1} \tilde{U}_1 \ket{\eta_0} \\
 \ket{\tilde{\phi}^2_{m_1,m_2}} & \coloneqq \ketbra{m_2}_\reg{m_2} \tilde{U}_2 \ketbra{m_1}_\reg{m_1} U_1 \ket{\eta_0} \\
\end{align*}


\begin{table}
\begin{center}
\caption{Baby-Case Game \purple{(need a better title)}}
\label{table:LOCC-3ZK:branch-wise:lem:new}
\begin{tabular}{|c|c|}
\hline
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $G(\ket{\eta^0})$:}
    \begin{enumerate}
    \item 
    Apply $U_1$;
    \item
    Measure register $\reg{m_1}$ in computational basis;
    \item
    Apply $U_2$;
    \item
    Measure register $\reg{m_2}$ in computational basis;.
    \item
    Output the value of $\msf{pred}$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage} 
        &~
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $\tilde{G}(\ket{\eta^0})$:}
    \begin{enumerate}
    \item 
    Apply \red{$\tilde{U}_1$};
    \item
    Measure register $\reg{m_1}$ in computational basis;
    \item
    Apply \red{$\tilde{U}_2$};
    \item
    Measure register $\reg{m_2}$ in computational basis;.
    \item
    Output the value of $\msf{pred}$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage} \\
\hline
\end{tabular}
\end{center}
\end{table}

\begin{lemma}[Branch-wise Equivalence---Baby Case]
If for all $m_1,m_2\in \bits^\ell$ it holds that 
\begin{align}
\braket{\phi^1_{m_1}} & = \braket{\tilde{\phi}^1_{m_1}} \\	
\braket{\phi^2_{m_1,m_2}} & = \braket{\tilde{\phi}^2_{m_1,m_2}} \\ 
\Pr[\msf{pred}(\ket{\phi^2_{m_1,m_2}}) = 1] & = \Pr[\msf{pred}(\ket{\tilde{\phi}^2_{m_1,m_2}}) = 1],
\end{align}
\xiao{The last item requires explanation, because the state $\ket{\phi^2_{m_1,m_2}}$ is sub-normalized.}

then it must hold that
\begin{equation}
\Pr\big[\msf{Out}(G(\eta^0)) = 1\big]  = \Pr\big[\msf{Out}(\tilde{G}(\eta^0)) = 1\big]. 
\end{equation}
\end{lemma}

\begin{proof}
Let's first track the steps in game $G(\ket{\eta^0})$. Right after Step-1, the state can be written as
$$U_1 \ket{\eta^0} = \ket{\eta^1} = \sum_{m_1} \alpha_{m_1} \ket{m_1}\ket{\eta^1_{m_1}}.$$
\xiao{Note that $\ket{\phi^1_{m_1}} = \alpha_{m_1} \ket{m_1}\ket{\eta^1_{m_1}}$}

Measuring the $\reg{m_1}$ register results in the following mixture:
$$\text{with probability}~|\alpha_{m_1}|^2,~\text{collapsing to state}~\ket{m_1}\ket{\eta^1_{m_1}}.$$
For each possible state $\ket{m_1}\ket{\eta^1_{m_1}}$, Step-3 yields
$$U_2 \ket{m_1}\ket{\eta^1_{m_1}} = \ket{\eta^2_{m_1}} = \sum_{m_2}\beta_{m_1, m_2} \ket{m_2}\ket{\eta^2_{m_1, m_2}}.$$
\xiao{Note that $\ket{\phi^2_{m_1, m_2}} = \beta_{m_1, m_2} \ket{m_2}\ket{\eta^1_{m_1, m_2}}$}

Therefore, for each possible state $\ket{m_1}\ket{\eta^1_{m_1}}$, measuring the $\reg{m_2}$ register results in the following mixture:
$$\text{with probability}~|\beta_{m_1,m_2}|^2,~\text{collapsing to state}~\ket{m_2}\ket{\eta^2_{m_1, m_2}}.$$
Using the above notation, we can say that the state at the end of Step-4 is the following mixture:
$$\text{with probability}~|\alpha_{m_1}|^2 \cdot |\beta_{m_1,m_2}|^2,~\text{collapsing to state}~\ket{m_2}\ket{\eta^2_{m_1, m_2}}.$$
It then follows that 
$$\Pr\big[\msf{Out}(G(\eta^0)) = 1\big] = \sum_{m_1, m_2} |\alpha_{m_1}|^2 \cdot |\beta_{m_1,m_2}|^2 \cdot \Pr\big[\msf{pred}\big(\ket{m_2}\ket{\eta^2_{m_1, m_2}}\big) = 1\big].$$

Using the analog notation for game $\tilde{G}(\ket{\eta_0})$, we can derive the following as well:
$$\Pr\big[\msf{Out}(\tilde{G}(\eta^0)) = 1\big] = \sum_{m_1, m_2} |\tilde{\alpha}_{m_1}|^2 \cdot |\tilde{\beta}_{m_1,m_2}|^2 \cdot \Pr\big[\msf{pred}\big(\ket{m_2}\ket{\tilde{\eta}^2_{m_1, m_2}}\big) = 1\big].$$

Finally, the lemma follows by noticing that 
\begin{align*}
\braket{\phi^1_{m_1}} 
& = 
|\alpha_{m_1}|^2 \\ 
\braket{\tilde{\phi}^1_{m_1}} 
& = 
|\tilde{\alpha}_{m_1}|^2 \\ 
\braket{\phi^2_{m_1,m_2}} 
& = 
|\beta_{m_1, m_2}|^2 \\ 
\braket{\tilde{\phi}^2_{m_1,m_2}} 
& = 
|\tilde{\beta}_{m_1, m_2}|^2
\end{align*}

\end{proof}


\para{Branch-Wise Equivalence (Full Version).}  Let $\ket{\eta^0}$ be a pure state over registers $\reg{m_1}$, $\reg{m_2}$, and $\reg{o}$. Let $\msf{pred}$ be a quantum predicate over these three registers. Consider the two games defined in \Cref{table:LOCC-3ZK:branch-wise:lem:new:full}. Also, for all $\vb{m} = (m_1, \ldots, m_k)$, define the following (sub-normalized) states:
\begin{align*}
 \forall i \in [k],~ \ket{\phi^i_{\vb{m}}} & \coloneqq \big(\ketbra{m_i}_\reg{m_i} U_{i}\big) \cdot \big(\ketbra{m_{i-1}}_\reg{m_{i-1}} U_{i-1}\big) \cdots \big(\ketbra{m_1}_\reg{m_1} U_1\big) \cdot \ket{\eta_0} \\
 \forall i \in [k],~ \ket{\tilde{\phi}^i_{\vb{m}}} & \coloneqq \big(\ketbra{m_i}_\reg{m_i} \red{\tilde{U}_{i}}\big) \cdot \big(\ketbra{m_{i-1}}_\reg{m_{i-1}} \red{\tilde{U}_{i-1}}\big) \cdots \big(\ketbra{m_1}_\reg{m_1} \red{\tilde{U}_1}\big) \cdot \ket{\eta_0}
\end{align*}


\begin{table}
\begin{center}
\caption{Full-Version Game \purple{(need a better title)}}
\label{table:LOCC-3ZK:branch-wise:lem:new:full}
\begin{tabular}{|c|c|}
\hline
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $G(\ket{\eta^0})$:}
    \begin{enumerate}
    \item	
    For each $i \in [k]$:
    \begin{enumerate}
	    \item 
	    Apply $U_1$;
	    \item
	    Measure register $\reg{m_1}$ in computational basis;
    \end{enumerate}
    \item
    Output the value of $\msf{pred}$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage} 
        &~
\begin{minipage}[t]{0.45\textwidth}
    \vspace{-3pt}
    {\bf Game $\tilde{G}(\ket{\eta^0})$:}
    \begin{enumerate}
    \item	
    For each $i \in [k]$:
    \begin{enumerate}
	    \item 
	    Apply $\red{\tilde{U}_1}$;
	    \item
	    Measure register $\reg{m_1}$ in computational basis;
    \end{enumerate}
    \item
    Output the value of $\msf{pred}$.
    \end{enumerate}
    \vspace{3pt}
\end{minipage} \\
\hline
\end{tabular}
\end{center}
\end{table}

\begin{lemma}[Branch-wise Equivalence]
If for all $m_1,\ldots, m_2\in \bits^\ell$ it holds that 
\begin{align}
\forall i \in [k],~\braket{\phi^i_{\vb{m}}} & = \braket{\tilde{\phi}^i_{\vb{m}}} \\	
\Pr[\msf{pred}(\ket{\phi^k_{\vb{m}}}) = 1] & = \Pr[\msf{pred}(\ket{\tilde{\phi}^k_{\vb{m}}}) = 1],
\end{align}
then it must hold that
\begin{equation}
\Pr\big[\msf{Out}(G(\eta^0)) = 1\big]  = \Pr\big[\msf{Out}(\tilde{G}(\eta^0)) = 1\big]. 
\end{equation}
\end{lemma}
\begin{proof}
\xiao{It follows a similar argument as for the baby case.}
\end{proof}

\subsection{Modified Measure-and-Reprogram Game}

Note that in the MnR game, we know if a query is ``up'' or ``down''. This is because we do not allow the simulator to make a query by putting both $U$ and $U^\dagger$ in superposition, though each query of Sim can be a super-position query (to either $U$ or $U^\dagger$).

\para{New MnR Game.} We then define the new measure-and-reprogram game as follows. It halts and output ``Reject'' if the measured queries are not in the order of $(p_1, p_2, .\ldots, p_k)$. Note that this {\em cannot} be determined by merely looking at the selected (for measuring) positions---as a counter example, Sim may keep asking for ``going down'' until she goes down successfully for the first time; for this case, measuring the 10-th ``going down'' query may actually lead to the message $p_1$, i.e.,  the first ``going down'' message. \xiao{Ask Kai-Min: Kai-Min thinks that it does not make sense to require that Sim has to obtain a successful $(p_i, v_i)$ message to move to the next round $p_{i+1}$. But isn't it true that what we actually does is to enforce Sim to do so?}


Next, we show that the ``early rejection'' above does not affect the probability of accepting too much. This is stated as the following \Cref{lem:early-rejection}.	
\begin{lemma}\label{lem:early-rejection}
The new MnR game output an accepting state of $\tilde{V}$ with a probability negligible close to the old MnR game. 
\end{lemma}



\subsection{The Final Road Map}

\para{Step 1.} We first prove the IND between the real and dummy game for the layered diagram. This diagram represents a simplified setting of the MnR game with oracle $H_0$. The main workhorse of this proof is my almost commutative lemma (\Cref{lem:err-inv-com}).

The hybrids are designed in the following way. We need to first replace all queries in Layer 1 with dummy ones. Then, we do Layer 2. Next, Layer 3 etc. I need this particular order because in this way, when I'm at Layer $i$, {\em all} queries above Layer $i$ are handled in the same way between the current hybrid and the previous one, and importantly, these queries have nice commutativity (since they are dummies) with lower-layer operators so that it becomes easier to argue the invariant condition.

A caveat: at each hybrid, in addition to the invariant condition, we need to argue that the game at the very end output 1 with the same probability as the previous hybrid (indeed, this is our real goal. the invariant condition is merely a means to this end). Say, we are at Layer $i$ and have already established the invariant condition. I plan to argue it in the following way:
\begin{itemize}
\item
First, notice that the invariant condition holds in particular for the {\em last arrival} at Layer $i$. After this point, the queries will never go beyond (aka above) Layer $i$. (also recall that the invariant condition say that the ``good'' branch of the two cases are identical, and the ``bad'' branch has the same amplitudes. The only difference is the $W_1U^\dagger_0W^\dagger_0$ part and the $W_1$ party, using the notation from \Cref{lem:err-inv-com}).
\item
Next, notice that all the operations below Layer $i$ are identical for these two cases. {\bf Moreover, these operations commute with the $W_1U^\dagger_0W^\dagger_0$ (and $W_1$) because they only touches upon registers corresponding to layers lower than Layer $i+1$ (because we considers the execution after the LAST arrival at Layer $i$).} Therefore, the two cases should lead to the same final accepting probability.
\end{itemize}

\para{Step 2.}
But there are gaps between the layered diagram and the final reduction to soundness, where we need to use $Sim$ to build a malicious $P^*$ breaking the soundness. There are mainly two issues:
\begin{enumerate}
\item
In the diagram, every time it jumps from layer $i$ to $(i+1)$ for the first time, this query is measured. Importantly, Prover's messages $p_1, p_2, \ldots, p_k$ are measured in this order. However, this is not guaranteed by the MnR lemma. \\~

In particular, there are two issues w.r.t.\ the MnR lemma formalized in CCLY: (1) it does not guarantee the order of measured messages; (2) it is possible that there are less than $k$ queries measured. This is because the measured positions are sampled from $[q] \cup \Set{\bot}$, where $\bot$ means ``do not measure this position, and take the $x_i$ from $\Adv$'s final output to put in te corresponding position''. \\~

Note that these two issues do not appear in CCLY. This is because in the post-quantum setting, the honest $V$'s algorithm is a classical circuit. It does not matter if the messages are measured out in order or out of order---the $P^*$ can always forward out the correct messages. But in our LOCC setting, it is important that we have to measure the messages in correct order (to forward out); otherwise, it is unclear if the event that the MnR outputs 1 is equivalent to the event that the external $V^*$ accepts. \\~

Our technique to deal with these two issues is to set the $\reg{Count}$ register in a slightly different way than CCLY, as detailed in \Cref{sec:new-malicous-V-counter}.

\item
The second issue: The diagram assumes for simplicity that everything is unitary. However, the real execution contains two types of measurements: (1) $Sim$ needs to measure the $\reg{u_i}$ register to determine which oracle ($U$ or $U^\dagger$) she wants to make the $i$-th query to; (2) the MnR game needs to measure the selected queries to program the oracle. \\~

To deal with these two types of measurements, I want to make use of the ``branch-wise equivalence lemma'' as formalized in \Cref{sec:branch-wise-equiv-lemma-new}. (Yes, I hope to deal with these {\em two} types of measurements using the same branch-wise equivalence lemma.) This lemma allows me to talk about the equivalence between the real game and the dummy game for each fixed query pattern and MnR measurement outcomes, which corresponds to exactly the layered diagram setting.
\end{enumerate}
    

\para{Other Subtleties.} There are some subtle issues:
\begin{enumerate}
    \item
    Need to incorporate in the current writing that $\red{u_j}$'s are measured each time $S_j$'s are applied. (The new branch-wise equivalence lemma also handle this.)
\item
Note that there is a coin $b$ after each measurement int he MnR game, determining if the current query need to be answered using the programmed oracle. This requires extra caution to deal with.
\xiao{This can be handled because my almost commutativity lemma holds even if we take into consideration the value $b=0$ and $b=1$, namely, it holds for both case.}
\item
Need to take care of $\Sim$'s queries at a new layer {\em before the real measurement happens} (i.e., before this query is really answered.) \xiao{This can be handled because if the $\downarrow$ query to a new layer is not actually measured out, $H$ will always return 0. So the only unitary performed by verifier is only the swap operator between $\reg{m}_i$ and $\reg{t}_i$. This operator (at least almost using the notation $\reg{t_2}/\reg{m_2}$) commutes with all the operators happening before the new layer.}
\end{enumerate}

\section{Xiao's Sketch}
\label{sec:xiao-sketch}
At a high-level, we build a $\QMA$ decider $\mcal{B}$ that simply runs the simulator $\Sim$ with $\tilde{V}^{H_0}$ (i.e.,  the single-point real-up-and-down execution), and output the final decision of the $\tilde{V}$. More accurately, 
\begin{enumerate}
\item \label{item:final:BQP:decider}
$\mcal{B}$ runs the $\Adv[H_0, \bs{1}, \msf{real}]$ game to learn the $(a, d)$ values, and outputs 1 iff $H'_0(a) = \bs{1}$ and $d = 1$.
\end{enumerate}




Two lemmas need to prove:
\begin{itemize}
\item
For $x \in \Lang$, argue that $\tilde{V}^{H_0}$ accepts with noticeable probability. The strategy is to connect the acceptance probability $\tilde{V}^{H_0}$ to that of $\tilde{V}^{H_\epsilon}$, whose acceptance probability follows by definition of ZK. Here, we need to deal with the big loss $32k^2q^2\epsilon$. This is done in \Cref{sec:completeness-of-B}.
\item
For $x \notin \Lang$, argue that $\tilde{V}^{H_0}$ accepts with negligible probability. The strategy is to connect  acceptance probability $\tilde{V}^{H_0}$ to that of the single-point dummy-up-and-down version, which can be then bounded by the soundness error of $\Prot_\textsc{zk}$ with the original honest verifier $V$. This is done in \Cref{sec:single-dummy-to-soundness,sec:single-dummy-to-real}.
\end{itemize}


\begin{xiaoenv}{Assumptions}
Assumptions to make: 
\begin{itemize}
\item
$\Sim$ defer all the measurements to the very end of the game. (Reasonable due to deferred measurement principle)
\item
$A_2$ can lead to the structure of $\gamma_a \ket{a} \cdot \Delta_0 + \sum_{a' \ne a} \gamma_{a'} \ket{a'} \cdot \Delta_1$ even if we consider $\Sim$'s internal working register.
\item
A malicious $P^*$'s advantage will not increase even if $\tilde{V}$ sends the message $b$ as a quantum register (reasonable because $\tilde{V}$ keeps an internal copy of $b$. So the $b$ given to $P^*$ `looks like' it has been measured?) Or I think the easist solution is to just define the target protocol $\Prot_\textsc{zk}$ to be a CPM (``classical-prover-message'') protocol, where both parties are allowed to be quantum and the only requirement is that the prover's messages are all classical.
\end{itemize}
\end{xiaoenv}





\subsection{Connecting Single-Point Dummy-Up-and-Down to Soundness}\label{sec:single-dummy-to-soundness}


Consider the following experiment. 
\begin{xiaoenv}{Make assumptions about $\Sim$'s qeury patterns}
Make assumptions about $\Sim$'s qeury patterns:
\begin{itemize}
\item
$\Sim$ keeps asking down-queries until the first time its down query is answered;
\item
After that, $\Sim$ will alternating between up and down-queries. That it, $\Sim$ will never ask consecutive queries of the same type.
\item
$\Sim$'s last query must be a down-query.
\end{itemize}
Also, the following experiments are not really rigorous about the oracle $H$. What the following claims holds only in the setting where $H$ is programmed to output 1 only at point $a$. I will take care of this later.
\end{xiaoenv}


\begin{ExperimentBox}[label={single-dummy:expr}]{Single-Point\text{,} Dummy Up and Down}
This experiment will run the simulator internally, simulating the interface of $\tilde{U}$ and $\tilde{U}^\dagger$ for it. The experiment will sample a random $\tilde{U}$ query, measure the $\reg{m}$ register, and apply $\tilde{U}$ honestly. But for subsequent queries, the experiment will answer with simulated $\tilde{U}$ or $\tilde{U}^\dagger$. Formally, it proceeds as follows: 
\begin{enumerate}
\item
Initialize registers $\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{a}}\ket{\vb{0}}_{\reg{b}}  \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w} \ket{\phi}_{\reg{s}}$.
\item
$k \picks [q(\secpar)]$. Recall that $q(\secpar)$ is the total number of queries $\Sim$ will make.
\item
For the $i$-th ($i \in [q(n)]$) query made by $\Sim$, the experiment proceeds as follows:
\begin{enumerate}
\item
If $i < k$: do nothing;
\item \label[Step]{single-dummy:query:2}
If $i = k$: Note that this query must be a down-query (\red{We assume w.l.o.g.\ that $\Sim$ will not make up-queries until its down-query has been answered}). The experiment first measures the $\reg{m}$ register to learn a classical value $a$, and then apply $\tilde{U}$ as the honest $\tilde{V}$.
\item
If $i > k$: Simply swap the $\reg{a}$ register with the $\reg{m}$ register. An intuitive explanation of this step is as follows. If this query is an up-query (resp.\ down-query), the experiment answers by applying a simulated $\tilde{U}_{\sf{dummy}}$ (resp.\ $\tilde{U}^\dagger_{\sf{dummy}}$) which is meant to simulate the real $\tilde{U}$ (resp.\ $\tilde{U}^\dagger$) operation. This $\tilde{U}_{\sf{dummy}}$ is defined to be swapping the $\reg{a}$ register with the $\reg{m}$ register (and thus $\tilde{U}_{\sf{dummy}} = \tilde{U}^\dagger_{\sf{dummy}}$).
\end{enumerate}
\item
{\bf Output:} When $\Sim$ halts, the experiment measures the $\reg{a}$ register and the first qubit of the $\reg{w}$ register (which contains $\tilde{V}$'s decision bit). It out 1 iff $\reg{a}$ measures to $a$ (defined in \Cref{single-dummy:query:2}) {\em and} the first qubit of $\reg{w}$ measures to 1. We use $\msf{Out}(\mrm{\Cref{single-dummy:expr}})$ to denote the output of this experiment.
\end{enumerate}
\end{ExperimentBox}
\begin{lemma}\label{lem:dummy-to-soundness}
If $\Prot_\textsc{zk}$ is sound, then $\Pr[\msf{Out}(\mrm{\Cref{single-dummy:expr}}) = 1] = \negl(\secpar)$.
\end{lemma}
\begin{proof}
\xiao{We first build a hybrid experiment. This hybrid experiment will eventually allow use to build a malicious $P^*$ that reduces \Cref{lem:dummy-to-soundness} to the soundness of $\Prot_\textsc{zk}$.}

This experiment is identical to \Cref{single-dummy:expr} except for the following two differences:
\begin{enumerate}
\item
It makes use of an extra $\dot{\reg{a}}$ register to keep a copy of the (classical) measurement outcome $a$ in \Cref{single-dummy:query:2} of \Cref{single-dummy:expr}. This $\dot{\reg{a}}$ register will be used in place of the original $\reg{a}$ register in the sequential steps, where the  $\reg{a}$ register will not be touched anymore.
\item
Its output is determined only by the first bit of the (measured) $\reg{w}$ register, where as the output of \Cref{single-dummy:expr} is determined by {\em both} the first bit of $\reg{w}$ {\em and} the contents of the $\reg{a}$ register at the end of the execution. 
\end{enumerate}
We present this hybrid in \Cref{single-dummy:hybrid:expr}, high-lighting the difference with \Cref{single-dummy:expr} \purple{in purple color}.
\begin{ExperimentBox}[label={single-dummy:hybrid:expr}]{Hybrid Experiment}
\begin{enumerate}
\item
Initialize registers $\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{a}} \purple{\ket{\vb{0}}_{\dot{\reg{a}}}}\ket{\vb{0}}_{\reg{b}}  \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\vb{0}}_\reg{w} \ket{\phi}_{\reg{s}}$.
\item
$k \picks [q(\secpar)]$. Recall that $q(\secpar)$ is the total number of queries $\Sim$ will make.
\item
For the $i$-th ($i \in [q(n)]$) query made by $\Sim$, the experiment proceeds as follows:
\begin{enumerate}
\item
If $i < k$: do nothing;

\item 
If $i = k$: Note that this query must be a down-query (\red{We assume w.l.o.g.\ that $\Sim$ will not make up-queries until its down-query has been answered}). The experiment first measures the $\reg{m}$ register to learn a classical value $a$. \purple{It writes $a$ into the $\dot{\reg{a}}$ register,} and then applies $\tilde{U}$ as the honest $\tilde{V}$.

\item
If $i > k$: This query is handled in the same way as in \Cref{single-dummy:expr}, \purple{but using $\dot{\reg{a}}$ in place of $\reg{a}$}. Namely, the experiment simply swaps the \purple{$\dot{\reg{a}}$} register with the $\reg{m}$ register.
\end{enumerate}

\item
{\bf Output:} When $\Sim$ halts, the experiment measures \purple{the first qubit of the $\reg{w}$ register}. \purple{It outputs 1 iff the measurement outcome is 1}. We use $\msf{Out}(\mrm{\Cref{single-dummy:hybrid:expr}})$ to denote the output of this experiment.
\end{enumerate}
\end{ExperimentBox}


It is not hard to see that the contents of the $\reg{w}$ register are identical in both \Cref{single-dummy:expr} and \Cref{single-dummy:hybrid:expr} {\em up to the last {\bf Output} step}. The reason is that \Cref{single-dummy:hybrid:expr} can be viewed as simply re-naming $\reg{a}$ to $\dot{\reg{a}}$, and leaving the original $\reg{a}$ untouched after that. Moreover, compared with \Cref{single-dummy:expr}, \Cref{single-dummy:hybrid:expr} outputs 1 with less restrictive conditions. Therefore, the following holds
\begin{equation}\label[Inequality]{lem:dummy-to-soundness:eq:expr-hybrid}
\Pr[\msf{Out}(\mrm{\Cref{single-dummy:hybrid:expr}})=1] ~\ge~ \Pr[\msf{Out}(\mrm{\Cref{single-dummy:expr}})=1].
\end{equation}

Using \Cref{single-dummy:hybrid:expr}, we now build a malicious prover $P^*$ talking to the honest verifier $V$ \xiao{(Note that I do mean the original verifier $V$, not that $\tilde{V}$ that uses $H$)}. The interaction between them is identical to \Cref{single-dummy:hybrid:expr}, but the registers are distributed between $P^*$ (who will internally emulate $\Sim$) and $V$. This is possible because the simulator $\Sim$ in \Cref{single-dummy:hybrid:expr} does not touch the registers corresponding to the honest $V$, i.e., the $\reg{a}$, $\reg{b}$, $\reg{m}$, and $\reg{w}$ registers.


\subpara{Malicious Prover $P^*$:}  The (external) honest verifier $V$ initialize the registers  $\ket{x}_{\reg{ins}} \ket{\vb{0}}_{\reg{a}}\ket{\vb{0}}_{\reg{b}}  \ket{\vb{0}}_\reg{w}$. $P^*$ initialize the register $\ket{\vb{0}}_{\dot{\reg{a}}} \ket{\vb{0}}_{\reg{m}} \ket{H}_{\reg{aux}}\ket{\phi}_{\reg{s}}$. $P^*$ essentially emulates \Cref{single-dummy:expr} with the help of the external $V$. Formally, it proceeds as follows:
\begin{enumerate}
\item
$P^*$ samples $k \picks [q(n)]$  and invokes $\Sim$ internally.
\item
For the $i$-th ($i \in [q(n)]$) query made by $\Sim$, the $P^*$ proceeds as follows:
\begin{enumerate}
\item
If $i < k$: do nothing;
\item \label[Step]{single-dummy:query:2}
If $i = k$: $P^*$ measures the $\reg{m}$ register to learn a classical value $a$. $P^*$ writes $a$ in to the $\dot{\reg{a}}$ register, and then sends the register $\ket{a}_\reg{m}$ to the external $V$. By definition, $V$ will return the $\reg{m}$ register back after it applies $\tilde{U}$ on its internal registers $\reg{a}$, $\reg{b}$, $\reg{m}$, and $\reg{w}$. $P^*$ simply forwards the returned $\reg{m}$ register to its internal $\Sim$. 

\item
If $i > k$: Simply swap the $\dot{\reg{a}}$ register with the $\reg{m}$ register. 
\end{enumerate}
\item
{\bf Output:} By definition, the honest $V$ will measure the first qubit of $\reg{w}$ and output it as its decision bit.
% \item
% {\bf Output:} When $\Sim$ halts, the experiment measures the $\reg{a}$ register and the first qubit of the $\reg{w}$ register (which contains $\tilde{V}$'s decision bit). It out 1 iff $\reg{a}$ measures to $a$ (defined in \Cref{single-dummy:query:2}) {\em and} the first qubit of $\reg{w}$ measures to 1.
\end{enumerate}
From the above description, it is straightforward that the execution between $P^*$ and $V$ are identical to \Cref{single-dummy:hybrid:expr}. In particular, $V$ outputs 1 with the same probability that \Cref{single-dummy:hybrid:expr} outputs 1. Therefore, it holds that
\begin{equation}\label{lem:dummy-to-soundness:eq:hybrid-real}
\Pr[P^* ~\text{breaks soundness of}~\Prot_\textsc{zk}] ~=~ \Pr[\msf{Out}(\mrm{\Cref{single-dummy:hybrid:expr}})=1].
\end{equation}

\Cref{lem:dummy-to-soundness:eq:expr-hybrid} and \Cref{lem:dummy-to-soundness:eq:hybrid-real} together imply \Cref{lem:dummy-to-soundness}.

\end{proof}

\subsection{Connecting Single-Point Real-Up-and-Down to Single-Point Dummy-Up-and-Down} \label{sec:single-dummy-to-real}
\xiao{This is what Jiahui is working on.}
Once we show that Single-Point Real-Up-and-Down  leads to the same acceptance probability as the Single-Point Dummy-Up-and-Down, the upper-bound we derived in  \Cref{sec:single-dummy-to-soundness} also upper-bound the machine $\mcal{B}$ (which is identical to Single-Point Real-Up-and-Down).


\subsection{Completeness}\label{sec:completeness-of-B}
% We now show that for any $x \in \Lang$, $\mcal{B}$ indeed output 1 with noticeable probability.
% \begin{equation}
% \Pr\big[H'_0(a) = 1 \wedge d=1: (a, d)\la\Adv[H_0, \mbf{1}, \msf{dummy}]\big] = \Pr\big[H'_0(a) = 1 \wedge d=1: \Adv[H_0, \mbf{1}, \msf{real}]\big]
% \end{equation}
% This follows from Jiahui's part.

We now show that for any $x \in \Lang$, $\mcal{B}$ indeed output 1 with noticeable probability.

First, it follows from Equation (3) in \cite{FOCS:CCLY21} (the sparsity property) that 
\begin{equation}
\Pr\big[H'_0(a) = 1 \wedge d=1: \Adv[H_0, \mbf{1}, \msf{real}]\big] \ge \Pr_{H_\epsilon}\big[H'_\epsilon(a) = 1 \wedge d=1: \Adv[H_\epsilon, \mbf{1}, \msf{real}]\big] - 32k^2q^2\epsilon.
\end{equation}


Next, we proceed to lower-bound the RHS of the above inequality. By the measure-and-reprogram lemma, it holds that
\begin{align*}
\Pr_{H_\epsilon}\big[H'_\epsilon(a) = 1 \wedge d=1: \Adv[H_\epsilon, \mbf{1}, \msf{real}]\big] 
& \ge 
\frac{1}{(4kq+1)^{2k}} \cdot \sum_{a^* \in \bits^\secpar} \Pr_{H_\epsilon}\big[a = a^* \wedge d=1: \Adv^{H_\epsilon[a^*,\mbf{1}]}\big]\\
& =
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{a^* \in \bits^\secpar} \Pr_{H_\epsilon, \bs{\beta}}\big[a = a^* \wedge d=1 \wedge \bs{\beta} = \bs{1}: \Adv^{H_\epsilon[a^*,\bs{\beta}]}\big]\\
& =
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \sum_{a^* \in \bits^\secpar} \Pr_{H_\epsilon}\big[a = a^* \wedge d=1 \wedge \hat{H}_\epsilon(a) = \bs{1}: \Adv^{H_\epsilon}\big] \\ 
& = 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \Pr_{H_\epsilon}\big[d=1 \wedge \hat{H}_\epsilon(a) = \bs{1}: (a,d)\la\Adv^{H_\epsilon}\big] 
\end{align*}
Then, by the ZK property, 
\begin{equation}
\Pr_{H_\epsilon}\big[d=1 \wedge \hat{H}_\epsilon(a) = \bs{1}: (a,d)\la\Adv^{H_\epsilon}\big]  \ge \frac{\epsilon^k}{4} - \negl(\secpar).
\end{equation}
Finally, combining the above gives us:
\begin{align*}
\Pr[\mcal{B} ~\text{outputs 1 on}~x] 
& =
\Pr\big[H'_0(a) = 1 \wedge d=1: (a, d)\la\Adv[H_0, \mbf{1}, \msf{real}]\big] \\
& \ge 
\frac{\epsilon^{-k}}{(4kq+1)^{2k}} \cdot \bigg(\frac{\epsilon^k}{4} - \negl(\secpar)\bigg) - 32k^2q^2\epsilon \\ 
& = 
\frac{1}{8(4kq+1)^{2k}} - \negl(\secpar),
\end{align*}
which is noticeable.


\subsection{Non-Programmable EPR model}

First, it seems to me that the EPR model does not affect our derivation of the completeness (i.e., \Cref{sec:single-dummy-to-real}) of the $\QMA$ decider $\mcal{B}$. So, all we need to do is to re-examine the soundness of $\mcal{B}$.

Weirdly, the soundness analysis seems to extend to the EPR model as well. This seem to contradict the counter example proposed by Kai-Min in our last meeting. Need to discuss about it.




==> sections/concurrent_locc_quantum.tex <==
\subsection{LOCC and Quantum Lower Bound for Concurrent Zero-Knowledge Protocols}

\begin{conjecture}
\label{thm:quantum_concurrent_zk}
Let $n$ be the security parameter, and let $\Pi = (P, V)$ be a $m(n)$-round concurrent black-box quantum zero-knowledge argument for a language $L$, with perfect completeness and negligible soundness against any QPT adversaries. If $m(n) \in o(\log n/ \log \log n)$, then $L \in \BQP$.
\end{conjecture}
To lift to the LOCC setting, we need to make some changes to the design of the $k$-parallel verifier $\Vbase$. Recall that the post-quantum $\Vbase$ is defined in \Cref{sec:quantum_parallel_verifier} and the LOCC version's next message function is defined in \Cref{sec:parallel_locc_lowerbound}.

Now we make further changes to the next-message unitary in the $j$-th session by including a classical randomness $r$ as input:

    \begin{align*}
V_{j, i}\ket{x,H,(\MSG_{1},...,\MSG_{i}), r_j, \psi_j}:=
\begin{cases}
\ket{\msg^j_{i}}\bra{\msg^j_{i} } \otimes V_{i,\msg^j_{i}} \ket{x, \psi_j}
&\text{~if~} H_j(\MSG_{1},...,\MSG_{i}; {\color{red}r_j})=1 \\
\mathbf{I} \ket{x, \psi_j} %\text{ for abort-and-accept} 
&\text{~otherwise~}
\end{cases}.    
\end{align*}
where $\msg^j$ is the transcript, $r_j$ is the classical fixed randomness and $\ket{\psi_j}$ is prover's internal state in the $j$-th session. 

Note that when we run $\Vbase(\lambda, r)$ as a subroutine, $r = g(\tau)$ is computed from the current global transcript $\tau$ in the concurrent interaction $S^{\Vconc}$ to ensure that we have fresh base
randomness even when rewound by the simulator. 

Note that the post-quantum $\Vbase$ can take in $r$ as an input because its next-message function $F^*[x, r, \cdot]$ is a classical function that can have its randomness fixed, but we cannot fix such a randomness for a quantum V.

We let the new $\Vbase$ query the random-termination oracle $H_j$ on the string $\MSG_1, \cdots, \MSG_i, r_j$. 
By including 



==> sections/error-inv-commute-new.tex <==

\section{Error-Invariant Commutativity Lemma}

In this section, we present a information-theoretic lemma regarding the commutativity of some unitary operators. As will become evident later, this lemma will serve as a clean abstraction of the behaviors of the ZK simulator and a malicious verifier we designed for the impossibility results. 

\subsection{Statement and Interpretation}


\begin{xiaoenv}{An intuitive explanation of the operators in \Cref{lem:err-inv-com}}
\begin{itemize}
\item
$U$ will the verifier's operation to generate the next message
\item
$W$ is the verifiiere's operator to move the message (indeed, its response to $P$) to the correct register.
\item
$\tilde{W}$ is the dummy-up operator 
\item
$S$ is simulator's local unitary.
\end{itemize}
\end{xiaoenv}


\xiao{Need to make this lemma a ``sub-normalized'' version. Remove the amplitude $\gamma_a$ and $\gamma_{a'}$.}
\begin{lemma}[Error-Invariant Commutativity Lemma]\label{lem:err-inv-com}
% Let $\ell$ be an integer and $a \in \bits^{\ell}$ be a fixed string. Let $\reg{a}$, $\reg{m}$, $\reg{t}$, $\reg{s}$, and $\reg{o}$ be registers over Hilbert space. 
Let $W_0$, $W_1$, and $U_0$ be unitary operators over $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$ satisfying the following requirements:
\begin{itemize}
\item
$W_0$ acts non-trivially only on $\Hil_{\reg{m}} \tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{o}}$, and is identity on $\Hil_\reg{s}$. 
% That is, it is of the form $W_0 = I_{\reg{t}} \tensor U_{\reg{mso}}$, where $I_{\reg{t}}$ is the identity operator on $\Hil_{\reg{t}}$ and $U_{\reg{mso}}$ is some unitary on $\Hil_{\reg{m}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$.
\item
$W_1$ is the swap operator between registers $\reg{m}$ and $\reg{t}$, and is identity on $\Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$.

\item
$U_0$  acts non-trivially only on $ \Hil_{\reg{m}} \tensor \Hil_{\reg{t}}\tensor \Hil_\reg{o}$, and is identity on $\Hil_{\reg{s}}$. \xiao{indeed, this $U_0$ in our application will be identity on $\Hil_{\reg{m}} \tensor \Hil_{\reg{t}}$  as well. But it seems I never used this stronger property when proving the current lemma. So in this lemma, I don't spell it out explicitly.}
\end{itemize}
 
Let $\Hil_{\reg{a}}$ be a Hilbert space of $\ell$ qubits. Let $a \in \bits^{\ell}$ be a fixed classical string. Define the following unitary operators on $\Hil_{\reg{a}} \tensor \Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$:
\begin{itemize}
\item
$W \coloneqq \ketbra{a}_{\reg{a}} \tensor W_0 + \sum_{a'\ne a} \ketbra{a'}_{\reg{a}} \tensor W_1$, where $W_0$ and $W_1$ are as specified above.

\item
$\tilde{W} \coloneqq \ketbra{a}_{\reg{a}} \tensor I_{\reg{mtso}}+ \sum_{a'\ne a} \ketbra{a'}_{\reg{a}} \tensor W_1$, where $I_{\reg{mtso}}$ is the identity operator on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$ and $W_1$ are as specified above.

\item
$U \coloneqq \ketbra{a}_{\reg{a}} \tensor U_0 + \sum_{a'\ne a} \ketbra{a'}_{\reg{a}} \tensor I_{\reg{mtso}}$, where $U_0$ is as specified above and $I_{\reg{mtso}}$ is the identity operator on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$.

\item
$S$ is an operator that acts non-trivially only on $\Hil_\reg{a} \tensor \Hil_\reg{s}$, and is identity on $\Hil_{\reg{m}} \tensor \Hil_{\reg{t}}\tensor  \Hil_{\reg{o}}$. \xiao{In our applications, the $S$ may not be a unitary. It will be alternating between unitary and projections. Make sure that the proof can go through.}


 % $\coloneqq S_{\reg{as}} \tensor I_{\reg{mto}}$, where $S_{\reg{as}}$ is some unitary operator on $\Hil_{\reg{a}}\tensor \Hil_{\reg{s}}$ and $I_{\reg{mto}}$ is the identity operator on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{o}}$. 
\end{itemize}
These operators satisfy the following property:
\begin{itemize}
\item 
Let $\Set{\ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}}_{a' \in \bits^\ell}$ be a sequence of (potentially sub-normalized) pure states over registers $\reg{m}$, $\reg{t}$, $\reg{s}$, and $\reg{o}$. Define states $\ket{\eta^{(\msf{in})}_0}$, $\ket{\eta^{(\msf{in})}_1}$, $\ket{\eta^{(\msf{out})}_0}$ and $\ket{\eta^{(\msf{out})}_1}$  follows:
\begin{align}
& \ket{\eta^{(\msf{in})}_0} 
\coloneqq 
\ket{a}_{\reg{a}} \ket{\rho^{(\msf{in})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} \red{W_1 U_0^\dagger W_0^\dagger} \ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}} 
\label{lem:err-inv-com:def:in-0} \\
& \ket{\eta^{(\msf{in})}_1} 
\coloneqq
\ket{a}_{\reg{a}} \ket{\rho^{(\msf{in})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} \red{W_1}  \ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}} 
\label{lem:err-inv-com:def:in-1}\\ 
& \ket{\eta^{(\msf{out})}_0} 
\coloneqq 
\red{W U} S \red{U^\dagger W^\dagger} \cdot \ket{\eta^{(\msf{in})}_0} 
\label{lem:err-inv-com:def:out-0}\\ 
& \ket{\eta^{(\msf{out})}_1} 
\coloneqq 
\red{\tilde{W}} S \red{\tilde{W}^\dagger} \cdot \ket{\eta^{(\msf{in})}_1}
\label{lem:err-inv-com:def:out-1}
\end{align}
Then, there exists a sequence of (potentially sub-normalized) pure states  $\Set{\ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}}}_{a' \in \bits^\ell}$ so that the states $\ket{\eta^{(\msf{out})}_0}$ and $\ket{\eta^{(\msf{out})}_1}$ defined above can be written in the following format:
\begin{align}
\ket{\eta^{(\msf{out})}_0}
& = 
\ket{a}_{\reg{a}} \ket{\rho^{(\msf{out})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} \red{W_1 U_0^\dagger W_0^\dagger} \ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}} \label{eq:lem:err-inv-com:property-2:real} \\
\ket{\eta^{(\msf{out})}_1}
& = 
 \ket{a}_{\reg{a}} \ket{\rho^{(\msf{out})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} \red{W_1} \ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}} \label{eq:lem:err-inv-com:property-2:dummy}
\end{align}
\end{itemize}
\end{lemma}




\para{Interpretation.} \xiao{Before presenting the proof, give a intuitive explanation of \Cref{lem:cond-com}.}

\xiao{Also, emphasize that this lemma holds even if there are entanglement between $\Hil_{\reg{s}}$ and $\Hil_\reg{o}$...}

\subsection{Proof of \Cref{lem:err-inv-com}}

In this proof, we assume for simplicity that each of the registers $\reg{m}$, $\reg{t}$, $\reg{s}$, and $\reg{o}$ consists of $\ell$ qubits. This assumption is without loss of generality because the subsequent derivation works regardless of the length of these registers. 


We first note that since $S$ acts non-trivially only on $\Hil_{\reg{a}} \tensor \Hil_{\reg{s}}$, it holds that for any $a'\in\bits^\ell$, $s\in \bits^\ell$, and any pure state $\ket{\rho_{a',s}}_{\reg{mto}}$,
\begin{equation}\label{proof:err-inv-com:property-1:derive:S-format}
S\ket{a'}_{\reg{a}} \ket{s}_{\reg{s}} \ket{\rho_{a',s}}_{\reg{mto}} = \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}},
\end{equation}
where each $\beta^{a', s}_{a^*, s^*}$ is a complex number that depends on $(a', s, a^*, s^*)$.\footnote{It is worth noting that \Cref{proof:err-inv-com:property-1:derive:S-format} holds for {\em any} $a'\in \bits^\ell$, including the case where $a'$ equals to the $a$ we fixed.} \xiao{Note that $S$ may not be unitary, so the $\beta$ may not be normalized. But this does not affect our proof as we work with sub-normalized states anyway.}

In the following, we derive \Cref{eq:lem:err-inv-com:property-2:real,eq:lem:err-inv-com:property-2:dummy} one by one.




\subsubsection{Deriving \Cref{eq:lem:err-inv-com:property-2:real}}
We first derive \Cref{eq:lem:err-inv-com:property-2:real}:
\begin{align*}
\ket{\eta^{(\msf{out})}_0}
& = WU SU^\dagger W^\dagger  \cdot \ket{\eta^{(\msf{in})}_0} 
\numberthis \label{proof:err-inv-com:property-2:real:derive:00} \\
& = 
W U SU^\dagger W^\dagger  \cdot 
\Big(
\ket{a}_{\reg{a}} \ket{\rho^{(\msf{in})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}} 
\Big) 
\numberthis \label{proof:err-inv-com:property-2:real:derive:0} \\ 
& = 
W U SU^\dagger W^\dagger  \cdot 
\Big(
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U SU^\dagger W^\dagger  \cdot 
\Big(
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:1} \\ 
& =  
W U SU^\dagger \cdot 
\Big(
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \ket{s}_{\reg{s}} W^\dagger_0 \ket{\rho^{(\msf{in})}_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:2} \\ 
& =  
W U S \cdot 
\Big(
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:3} \\ 
& = 
W U S \cdot 
\Big(
\sum_{a' \in \bits^{\ell}} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U S \cdot 
\Big(
\sum_{a',s \in \bits^\ell} \ket{a'}_{\reg{a}} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U \cdot 
\Big(
\sum_{a', s \in \bits^\ell} S \ket{a'}_{\reg{a}} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big)  \\ 
\text{(by \Cref{proof:err-inv-com:property-1:derive:S-format})}~~ & =
W  U \cdot 
\Big(
\sum_{a', s \in \bits^\ell}   \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U \cdot 
\sum_{a', s \in \bits^\ell} 
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\Big) \\
& = 
W \cdot 
\sum_{a', s \in \bits^\ell}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}  W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:4} \\ 
& = 
\sum_{a', s \in \bits^\ell}   
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    W_1 U^\dagger_0 W^\dagger_0 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:5} \\ 
& = 
\ket{a}_{\reg{a}}
\sum_{a',s, s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{8em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \ket{a^*}_{\reg{a}}   W_1 U^\dagger_0 W^\dagger_0     \sum_{a', s, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\numberthis \label{proof:err-inv-com:property-2:real:derive:6} \\ 
& = 
\ket{a}_{\reg{a}} \ket{\rho^{(\msf{out})}_{a}}_{\reg{mto}}
+ 
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \ket{a^*}_{\reg{a}}   W_1 U^\dagger_0 W^\dagger_0     \ket{\rho^{(\msf{out})}_{a^*}}_{\reg{mto}}
\numberthis \label{proof:err-inv-com:property-2:real:derive:7} \\ 
& = 
\ket{a}_{\reg{a}} \ket{\rho^{(\msf{out})}_{a}}_{\reg{mto}}
+ 
\sum_{a' \in \bits^{\ell} \setminus \Set{a}} \ket{a'}_{\reg{a}}   W_1 U^\dagger_0 W^\dagger_0     \ket{\rho^{(\msf{out})}_{a'}}_{\reg{mto}}
\numberthis \label{proof:err-inv-com:property-2:real:derive:8}
,\end{align*}
where \Cref{proof:err-inv-com:property-2:real:derive:00} follows from  \Cref{lem:err-inv-com:def:out-0},  \Cref{proof:err-inv-com:property-2:real:derive:0} follows from  \Cref{lem:err-inv-com:def:in-0}, \Cref{proof:err-inv-com:property-2:real:derive:1} follows from the fact that all the unitary  operators $W_1$, $U^\dagger_0$, and $W^\dagger_0$ act as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:2} follows from the definition of $W^\dagger$ and the fact that $W^\dagger_0$ and $W^\dagger_1$ act as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:3} follow from the definition of $U^\dagger$ and the fact that $U^\dagger_0$ acts as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:4} follow from the definition of $U$ and the fact that $U_0$ acts as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:5} follow from the definition of $W$ and the fact that $W_0$ and $W_1$ act as identity on $\Hil_{\reg{s}}$, and \Cref{proof:err-inv-com:property-2:real:derive:6} follows from standard algebraic calculation and the fact that all the unitary operators $W_1$, $U^\dagger_0$, and $W^\dagger_0$ act as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:7} follows by defining
\begin{equation}\label[Expression]{proof:err-inv-com:property-2:real:derive:def:rho-out}
\forall~a^* \in \bits^\ell,~~~ \ket{\rho^{(\msf{out})}_{a^*}} \coloneqq \sum_{a',s, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}},
\end{equation}
and \Cref{proof:err-inv-com:property-2:real:derive:8} follows simply by renaming $a^*$ to $a'$.


This concludes the proof of \Cref{eq:lem:err-inv-com:property-2:real}.



\subsubsection{Deriving \Cref{eq:lem:err-inv-com:property-2:dummy}}



Finally, we derive \Cref{eq:lem:err-inv-com:property-2:dummy}:
\begin{align*}
\ket{\eta^{(\msf{out})}_1}
& = 
\tilde{W} S\tilde{W}^\dagger \cdot \ket{\eta^{(\msf{in})}_1} 
\numberthis \label{proof:err-inv-com:property-2:dummy:derive:00} \\ 
& = 
\tilde{W} S\tilde{W}^\dagger \cdot 
\Big(
 \ket{a}_{\reg{a}} \ket{\rho^{(\msf{in})}_a}_{\reg{mtso}} 
 + \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} W_1 \ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}} 
\Big) 
\numberthis \label{proof:err-inv-com:property-2:dummy:derive:0} \\ 
& = 
\tilde{W} S\tilde{W}^\dagger \cdot 
\Big(
 \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}}  \ket{a'}_{\reg{a}} W_1 \sum_{s \in \bits^\ell} \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\
& = 
\tilde{W} S \cdot 
\Big(
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell}\setminus \Set{a}}  \ket{a'}_{\reg{a}} \sum_{s \in \bits^\ell}  \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big)  \numberthis \label{proof:err-inv-com:property-2:dummy:derive:1} \\ 
& = 
\tilde{W} S \cdot \Big(
\sum_{a' \in \bits^{\ell}}  \ket{a'}_{\reg{a}} \sum_{s \in \bits^\ell} \ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
\tilde{W}  \cdot 
\Big(
\sum_{a',s \in \bits^{\ell}}  S\ket{a'}_{\reg{a}}\ket{s}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
\text{(by \Cref{proof:err-inv-com:property-1:derive:S-format})}
~~ & =
\tilde{W} \cdot 
\Big(
\sum_{a', s \in \bits^\ell}  \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
\tilde{W} \cdot 
\sum_{a', s \in \bits^\ell}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}   \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\Big) \\
& = 
\sum_{a', s \in \bits^\ell}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}} \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}} W_1 \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\Big) \numberthis \label{proof:err-inv-com:property-2:dummy:derive:2} \\ 
& = 
\ket{a}_{\reg{a}}   
\sum_{a', s, s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \ket{a^*}_{\reg{a}}  W_1  \sum_{a', s, s^* \in \bits^{\ell}}  \ket{s^*}_{\reg{s}}  \ket{\rho^{(\msf{in})}_{a', s}}_{\reg{mto}}
\numberthis \label{proof:err-inv-com:property-2:dummy:derive:3} \\ 
& = 
\ket{a}_{\reg{a}}   
 \ket{\rho^{(\msf{out})}_{a}}_{\reg{mto}} 
+ 
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \ket{a^*}_{\reg{a}}  W_1  \ket{\rho^{(\msf{out})}_{a^*}}_{\reg{mto}} 
\numberthis \label{proof:err-inv-com:property-2:dummy:derive:4} \\ 
& = 
\ket{a}_{\reg{a}}   
 \ket{\rho^{(\msf{out})}_{a}}_{\reg{mto}} 
+ 
\sum_{a' \in \bits^{\ell} \setminus \Set{a}} \ket{a'}_{\reg{a}}  W_1  \ket{\rho^{(\msf{out})}_{a'}}_{\reg{mto}} 
\numberthis \label{proof:err-inv-com:property-2:dummy:derive:5}
,\end{align*}
where \Cref{proof:err-inv-com:property-2:dummy:derive:00} follows from  \Cref{lem:err-inv-com:def:out-1},  \Cref{proof:err-inv-com:property-2:dummy:derive:0} follows from  \Cref{lem:err-inv-com:def:in-1}, \Cref{proof:err-inv-com:property-2:dummy:derive:1} follows from the definition of $\tilde{W}^\dagger$, \Cref{proof:err-inv-com:property-2:dummy:derive:2} follows from the definition of $\tilde{W}$ and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$, and \Cref{proof:err-inv-com:property-2:dummy:derive:3} follows from standard algebraic calculation and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:dummy:derive:4} follows from {\em the same definition of} $\Set{\ket{\rho^{(\msf{out})}_{a^*}}}_{a^* \in \bits^\ell}$ as shown in \Cref{proof:err-inv-com:property-2:real:derive:def:rho-out}, and \Cref{proof:err-inv-com:property-2:dummy:derive:5} follows by renaming $a^*$ to $a'$.



This concludes the proof of \Cref{eq:lem:err-inv-com:property-2:dummy}. 

\vspace{1em}

This eventually completes the proof of \Cref{lem:err-inv-com}.

==> sections/error-inv-commute.tex <==

\section{Error-Invariant Commutativity Lemma}

In this section, we present a information-theoretic lemma regarding the commutativity of some unitary operators. As will become evident later, this lemma will serve as a clean abstraction of the behaviors of the ZK simulator and a malicious verifier we designed for the impossibility results. 

\subsection{Statement and Interpretation}


\begin{xiaoenv}{An intuitive explanation of the operators in \Cref{lem:err-inv-com}}
\begin{itemize}
\item
$U$ will the verifier's operation to generate the next message
\item
$W$ is the verifiiere's operator to move the message (indeed, its response to $P$) to the correct register.
\item
$\tilde{W}$ is the dummy-up operator 
\item
$S$ is simulator's local unitary.
\end{itemize}
\end{xiaoenv}


\xiao{Need to make this lemma a ``sub-normalized'' version. Remove the amplitude $\gamma_a$ and $\gamma_{a'}$.}
\begin{lemma}[Error-Invariant Commutativity Lemma]\label{lem:err-inv-com}
% Let $\ell$ be an integer and $a \in \bits^{\ell}$ be a fixed string. Let $\reg{a}$, $\reg{m}$, $\reg{t}$, $\reg{s}$, and $\reg{o}$ be registers over Hilbert space. 
Let $W_0$, $W_1$, and $U_0$ be unitary operators over $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$ satisfying the following requirements:
\begin{itemize}
\item
$W_0$ acts non-trivially only on $\Hil_{\reg{m}} \tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{o}}$, and is identity on $\Hil_\reg{s}$. 
% That is, it is of the form $W_0 = I_{\reg{t}} \tensor U_{\reg{mso}}$, where $I_{\reg{t}}$ is the identity operator on $\Hil_{\reg{t}}$ and $U_{\reg{mso}}$ is some unitary on $\Hil_{\reg{m}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$.
\item
$W_1$ is the swap operator between registers $\reg{m}$ and $\reg{t}$, and is identity on $\Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$.

\item
$U_0$  acts non-trivially only on $ \Hil_{\reg{m}} \tensor \Hil_{\reg{t}}\tensor \Hil_\reg{o}$, and is identity on $\Hil_{\reg{s}}$. \xiao{indeed, this $U_0$ in our application will be identity on $\Hil_{\reg{m}} \tensor \Hil_{\reg{t}}$  as well. But it seems I never used this stronger property when proving the current lemma. So in this lemma, I don't spell it out explicitly.}
\end{itemize}
 
Let $\Hil_{\reg{a}}$ be a Hilbert space of $\ell$ qubits. Let $a \in \bits^{\ell}$ be a fixed classical string. Define the following unitary operators on $\Hil_{\reg{a}} \tensor \Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$:
\begin{itemize}
\item
$W \coloneqq \ketbra{a}_{\reg{a}} \tensor W_0 + \sum_{a'\ne a} \ketbra{a'}_{\reg{a}} \tensor W_1$, where $W_0$ and $W_1$ are as specified above.

\item
$\tilde{W} \coloneqq \ketbra{a}_{\reg{a}} \tensor I_{\reg{mtso}}+ \sum_{a'\ne a} \ketbra{a'}_{\reg{a}} \tensor W_1$, where $I_{\reg{mtso}}$ is the identity operator on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$ and $W_1$ are as specified above.

\item
$U \coloneqq \ketbra{a}_{\reg{a}} \tensor U_0 + \sum_{a'\ne a} \ketbra{a'}_{\reg{a}} \tensor I_{\reg{mtso}}$, where $U_0$ is as specified above and $I_{\reg{mtso}}$ is the identity operator on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}}\tensor  \Hil_{\reg{o}}$.

\item
$S$ is a unitary operator that acts non-trivially only on $\Hil_\reg{a} \tensor \Hil_\reg{s}$, and is identity on $\Hil_{\reg{m}} \tensor \Hil_{\reg{t}}\tensor  \Hil_{\reg{o}}$. 


 % $\coloneqq S_{\reg{as}} \tensor I_{\reg{mto}}$, where $S_{\reg{as}}$ is some unitary operator on $\Hil_{\reg{a}}\tensor \Hil_{\reg{s}}$ and $I_{\reg{mto}}$ is the identity operator on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{o}}$. 
\end{itemize}
These operators satisfy the following properties:
\begin{enumerate}
\item \label[Property]{lem:err-inv-com:property-1}
{\bf (Almost-Commutative.)} \xiao{(Not sure if this property is really needed.)}
Let $\ket{\eta} \coloneqq \ket{a}_{\reg{a}} \ket{\rho_a}_{\reg{mtso}}$, where $\ket{\rho_a}_{\reg{mtso}}$ is an arbitrary pure state (that may depend on the value $a$) on $\Hil_{\reg{m}}\tensor \Hil_{\reg{t}} \tensor \Hil_{\reg{s}} \tensor  \Hil_{\reg{o}}$. Then, the states $W U SU^\dagger W^\dagger \ket{\eta} $ and $\tilde{W}  S \tilde{W}^\dagger \ket{\eta} $ are of the following format: \xiao{Kai-Min suggests that we should say ``there exist $\tilde{\rho}_a$ and $\tilde{\rho}_{a'}$ ...''}
\begin{align}
W U SU^\dagger W^\dagger \ket{\eta} 
& = 
\gamma_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'}\ket{a'}_{\reg{a}} \red{W_1 U_0^\dagger W_0^\dagger} \ket{\tilde{\rho}_{a'}}_{\reg{mtso}} \label{eq:lem:err-inv-com:property-1:real} \\
\tilde{W} S \tilde{W}^\dagger \ket{\eta} 
& = 
\gamma_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'}\ket{a'}_{\reg{a}} \red{W_1} \ket{\tilde{\rho}_{a'}}_{\reg{mtso}}  \label{eq:lem:err-inv-com:property-1:dummy}  
\end{align}
% where for each $a' \in \bits^{\ell}$, $\ket{\rho_{a'}}_{\reg{msto}}$ is some pure state on $\Hil_{\reg{m}} \tensor\Hil_{\reg{t}} \tensor\Hil_{\reg{s}} \tensor\Hil_{\reg{o}} \tensor$ that may depend on $a'$.

\item \label[Property]{lem:err-inv-com:property-2}
{\bf (Error-Invariant).}
Let $\ket{\eta^{(\msf{in})}_0}$ \xiao{change $\ket{\eta_0}$ to $\ket{\eta^{(\msf{in})}_0}$} and $\ket{\eta^{(\msf{in})}_1}$ \xiao{change $\ket{\eta_1}$ to $\ket{\eta^{(\msf{in})}_1}$} pure states of the following format:
\begin{align}
 \ket{\eta^{(\msf{in})}_0} 
 &\coloneqq 
 \gamma_a \ket{a}_{\reg{a}} \ket{\rho^{(\msf{in})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} \red{W_1 U_0^\dagger W_0^\dagger} \ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}} \\
 \ket{\eta^{(\msf{in})}_1} 
 &\coloneqq
  \gamma_a \ket{a}_{\reg{a}} \ket{\rho^{(\msf{in})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} \red{W_1}  \ket{\rho^{(\msf{in})}_{a'}}_{\reg{mtso}}
\end{align}
Then, the states $\ket{\eta^{(\msf{out})}_0} \coloneqq W U SU^\dagger W^\dagger \ket{\eta^{(\msf{in})}_0}$ and $\ket{\eta^{(\msf{out})}_1} \coloneqq \tilde{W} S \tilde{W}^\dagger \ket{\eta^{(\msf{in})}_1} $ are of the following format:
\begin{align}
\ket{\eta^{(\msf{out})}_0}
& = 
\tilde{\gamma}_a \ket{a}_{\reg{a}} \ket{\rho^{(\msf{out})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \tilde{\gamma}_{a'}\ket{a'}_{\reg{a}} \red{W_1 U_0^\dagger W_0^\dagger} \ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}} \label{eq:lem:err-inv-com:property-2:real} \\
\ket{\eta^{(\msf{out})}_1}
& = 
\tilde{\gamma}_a \ket{a}_{\reg{a}} \ket{\rho^{(\msf{out})}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \tilde{\gamma}_{a'}\ket{a'}_{\reg{a}} \red{W_1} \ket{\rho^{(\msf{out})}_{a'}}_{\reg{mtso}} \label{eq:lem:err-inv-com:property-2:dummy}
\end{align}
\end{enumerate}
\end{lemma}




\para{Interpretation.} \xiao{Before presenting the proof, give a intuitive explanation of \Cref{lem:cond-com}.}

\xiao{Also, emphasize that this lemma holds even if there are entanglement between $\Hil_{\reg{s}}$ and $\Hil_\reg{o}$...}

\subsection{Proof of \Cref{lem:err-inv-com}}

In this proof, we assume for simplicity that each of the registers $\reg{m}$, $\reg{t}$, $\reg{s}$, and $\reg{o}$ consists of $\ell$ qubits. This assumption is without loss of generality because the subsequent derivation works regardless of the length of these registers. 


We first note that since $S$ acts non-trivially only on $\Hil_{\reg{a}} \tensor \Hil_{\reg{s}}$, it holds that for any $a'\in\bits^\ell$, $s\in \bits^\ell$, and any pure state $\ket{\rho_{a',s}}_{\reg{mto}}$,
\begin{equation}\label{proof:err-inv-com:property-1:derive:S-format}
S\ket{a'}_{\reg{a}} \ket{s}_{\reg{s}} \ket{\rho_{a',s}}_{\reg{mto}} = \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}},
\end{equation}
where each $\beta^{a', s}_{a^*, s^*}$ is an amplitude that depend on $(a', s, a^*, s^*)$.\footnote{It is worth noting that \Cref{proof:err-inv-com:property-1:derive:S-format} holds for {\em any} $a'\in \bits^\ell$, including the case where $a'$ equals to the $a$ we fixed.} 

In the following, we derive \Cref{eq:lem:err-inv-com:property-1:real,eq:lem:err-inv-com:property-1:dummy,eq:lem:err-inv-com:property-2:real,eq:lem:err-inv-com:property-2:dummy} one by one.

% \subsubsection{Proving \Cref{lem:err-inv-com:property-1}}

\subsubsection{Deriving \Cref{eq:lem:err-inv-com:property-1:real}}

 We first derive \Cref{eq:lem:err-inv-com:property-1:real}:
%In the following, we use ``$a'=a$'' as an abbreviation for ``$a' \in \bits^{\ell} \setminus \Set{a}$'' when taking summation over $a'$.
\begin{align*}
W U SU^\dagger W^\dagger \cdot \ket{\eta} 
&= 
W U SU^\dagger W^\dagger \cdot \ket{a}_{\reg{a}}\ket{\rho_a}_{\reg{mtso}} \\ 
& =
W U SU^\dagger W^\dagger \cdot \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} \\ 
& = 
W U SU^\dagger \cdot \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} \numberthis \label{proof:err-inv-com:property-1:derive:1} \\ 
& =
W U S \cdot \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} \numberthis \label{proof:err-inv-com:property-1:derive:2} \\ 
& = 
W U \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} S \ket{a}_{\reg{a}} \ket{s}_{\reg{s}} U_0^\dagger W_0^\dagger \ket{\rho_{a, s}}_{\reg{mto}} \\ 
\text{(by \Cref{proof:err-inv-com:property-1:derive:S-format})}~~ & = 
W U \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   U_0^\dagger W_0^\dagger \ket{\rho_{a, s}}_{\reg{mto}} \\ 
% & =
% W^\dagger U^\dagger \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} \left(
% \begin{array}{c}
% \displaystyle\sum_{ s^* \in \bits^{\ell}} \beta^{a, s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}   U_0 W_0 \ket{\rho_{a, s}}_{\reg{mto}} 
% \\ 
% +
% \\
% \displaystyle\sum_{\substack{a^* \in \bits^{\ell} \setminus \Set{a}\\ s^* \in \bits^{\ell}}} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   U_0 W_0 \ket{\rho_{a, s}}_{\reg{mto}} 
% \end{array}
% \right) \\
& =
W U \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} 
\Bigg(
\sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}   U_0^\dagger W_0^\dagger \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{14em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \sum_{~s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   U_0^\dagger W_0^\dagger \ket{\rho_{a, s}}_{\reg{mto}} 
\Bigg) \\
& =
W \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} 
\Bigg(
\sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}} W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{12em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \sum_{~s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   U^\dagger_0 W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} 
\Bigg) \numberthis \label{proof:err-inv-com:property-1:derive:3} \\ 
& =
\sum_{s \in \bits^\ell} \alpha_{a, s} 
\Bigg(
\sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}  \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{12em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \sum_{~s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} 
\Bigg) \numberthis \label{proof:err-inv-com:property-1:derive:4} \\ 
& =
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{7em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \ket{a^*}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \sum_{s \in \bits^\ell} \alpha_{a, s} \sum_{s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*}  \ket{s^*}_{\reg{s}}    \ket{\rho_{a, s}}_{\reg{mto}} \numberthis \label{proof:err-inv-com:property-1:derive:5} 
,\end{align*}
where \Cref{proof:err-inv-com:property-1:derive:1} follows from the definition of $W^\dagger$ and the fact that $W^\dagger_0$ is identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-1:derive:2,proof:err-inv-com:property-1:derive:3} follow from the definition of $U^\dagger$ and $U$ and the fact that $U^\dagger_0$ and $U_0$ are identities on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-1:derive:4} follows from the definition of $W$ and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$, and \Cref{proof:err-inv-com:property-1:derive:5} follows from standard algebraic calculation and the fact that all the unitary  operators $W_1$, $U^\dagger_0$, and $W^\dagger_0$ act as identity on $\Hil_{\reg{s}}$.

As a vigilant reader may already notice, the RHS of \Cref{proof:err-inv-com:property-1:derive:5} can be equivalently written in the same format as the RHS of \Cref{eq:lem:err-inv-com:property-1:real}, by properly setting the parameters $\gamma_a$, $\gamma_{a'}$, $\tilde{\rho}_a$, and $\tilde{\rho}_{a'}$. For the sake of completeness, we provide the formal derivation below. 

\para{Equivalence of \Cref{proof:err-inv-com:property-1:derive:5} and  \Cref{eq:lem:err-inv-com:property-1:real}.\label{proof:err-inv-com:property-1:normalization}} For any $a^*, s \in \bits^\ell$, define\footnote{Recall that in this lemma, $a$ is a {\em fixed} classical string. So we do not view it as a variable.}
$$
\tau_{a, a^*, s} \coloneqq \sqrt{\sum_{s^* \in \bits^\ell} |\beta^{a, s}_{a^*, s^*}|^2}~~~~~\text{and}~~~~~ \ket{\phi_{a, a^*, s}}_{\reg{s}} \coloneqq \sum_{s^* \in \bits^\ell} \frac{\beta^{a, s}_{a^*, s^*}}{\tau_{a, a^*, s}} \ket{s^*}_{\reg{s}}.
$$
Plugging these notations into \Cref{proof:err-inv-com:property-1:derive:5} yields
\begin{align*}
W U SU^\dagger W^\dagger \cdot \ket{\eta} 
% & = 
% \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \tau_{a, a, s} \ket{\phi_{a, a, s}}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
% & \hspace{8em}
% \sum_{a^* \in \bits^\ell \setminus \Set{a}} \ket{a^*}_{\reg{a}}  \sum_{s \in \bits^\ell} \alpha_{a, s} \tau_{a, a^*, s} \ket{\phi_{a, a^*, s}}_{\reg{s}}  W^\dagger_1 U_0 W_0 \ket{\rho_{a, s}}_{\reg{mto}} \\ 
& = 
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \tau_{a, a, s} \ket{\phi_{a, a, s}}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{8em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \ket{a^*}_{\reg{a}}  W_1 U^\dagger_0 W^\dagger_0 \sum_{s \in \bits^\ell} \alpha_{a, s} \tau_{a, a^*, s} \ket{\phi_{a, a^*, s}}_{\reg{s}}  \ket{\rho_{a, s}}_{\reg{mto}}. \numberthis \label{proof:err-inv-com:property-1:derive:6}
\end{align*}
% where \Cref{proof:err-inv-com:property-1:derive:6} follows from the fact that all the unitary  operators $W^\dagger_1$, $U_0$, and $W_0$ act as identity on $\Hil_{\reg{s}}$.
Next, for any $a^* \in \bits^\ell$, define
$$
\gamma_{a, a^*} \coloneqq \sqrt{\sum_{s \in \bits^\ell} |\alpha_{a, s} \tau_{a, a^*, s}|^2}~~~~~\text{and}~~~~~ \ket{\tilde{\rho}_{a, a^*}}_{\reg{mtso}} \coloneqq \sum_{s \in \bits^\ell} \frac{\alpha_{a, s} \tau_{a, a^*, s}}{\gamma_{a, a^*}} \ket{\phi_{a, a^*, s}}_{\reg{s}}\ket{\rho_{a, s}}_{\reg{mto}}.
$$
Plugging these notations into \Cref{proof:err-inv-com:property-1:derive:6} yields
\begin{align*}
W U SU^\dagger W^\dagger \cdot \ket{\eta} 
& = 
\ket{a}_{\reg{a}} \gamma_{a, a} \ket{\tilde{\rho}_{a, a}}_{\reg{mtso}} ~~+ 
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \ket{a^*}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \gamma_{a, a^*} \ket{\tilde{\rho}_{a, a^*}}_{\reg{mtso}}\\ 
& =
 \gamma_{a, a} \ket{a}_{\reg{a}}  \ket{\tilde{\rho}_{a, a}}_{\reg{mtso}} ~~+ 
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \gamma_{a, a^*} \ket{a^*}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0  \ket{\tilde{\rho}_{a, a^*}}_{\reg{mtso}} \\ 
& =
 \gamma_{a} \ket{a}_{\reg{a}}  \ket{\tilde{\rho}_{a}}_{\reg{mtso}} ~~+ 
\sum_{a' \in \bits^\ell \setminus \Set{a}} \gamma_{a, a'} \ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0  \ket{\tilde{\rho}_{a, a'}}_{\reg{mtso}}
, \numberthis \label{proof:err-inv-com:property-1:derive:7}
\end{align*}
where \Cref{proof:err-inv-com:property-1:derive:7} follows from renaming $\gamma_{a, a}$ to $\gamma_a$, renaming $\tilde{\rho}_{a, a}$ to $\tilde{\rho}_{a}$, and renaming $a^*$ to $a'$.

Finally, recall that in this lemma we view $a$ (and $\rho_a$) as fixed values, instead of variables. Therefore, for the second term (corresponding to $a' \in \bits^\ell \setminus \Set{a}$) in the RHS of \Cref{proof:err-inv-com:property-1:derive:7}, {\em syntactically}, we can remove its dependence on $a$.\footnote{Indeed, we can remove the dependence of $a$ in the first term in the RHS of \Cref{proof:err-inv-com:property-1:derive:7} as well. But we choose to keep it there to indicate that it is a branch in the superposition corresponding to $a' = a$. These things are only syntactical choices and do not affect the meaning of the current lemma.} Thus, we can equivalently write \Cref{proof:err-inv-com:property-1:derive:7} as
\begin{equation}
W U SU^\dagger W^\dagger \ket{\eta} 
= 
\gamma_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'}\ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \ket{\tilde{\rho}_{a'}}_{\reg{mtso}}, 
\end{equation}
which is exactly \Cref{eq:lem:err-inv-com:property-1:real}. 

This concludes the proof of \Cref{eq:lem:err-inv-com:property-1:real}.

\subsubsection{Deriving \Cref{eq:lem:err-inv-com:property-1:dummy}}
We now derive \Cref{eq:lem:err-inv-com:property-1:dummy}:
\begin{align*}
\tilde{W} S \tilde{W}^\dagger \cdot \ket{\eta} 
& = 
\tilde{W} S \tilde{W}^\dagger  \cdot \ket{a}_{\reg{a}}\ket{\rho_a}_{\reg{mtso}} \\ 
& = 
\tilde{W} S \tilde{W}^\dagger  \cdot  \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}}  \\
& =
\tilde{W} S \cdot  \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}}  \numberthis \label{proof:err-inv-com:property-1:dummy:derive:1} \\& = 
\tilde{W}  \cdot  \sum_{s \in \bits^\ell} \alpha_{a, s} S \ket{a}_{\reg{a}}  \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} \\ 
\text{(by \Cref{proof:err-inv-com:property-1:derive:S-format})}~~ & = 
\tilde{W} \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   \ket{\rho_{a, s}}_{\reg{mto}} \\ 
& = 
\tilde{W} \cdot \sum_{s \in \bits^\ell} \alpha_{a, s} 
\Bigg(
\sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}   \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{14em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \sum_{~s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}   \ket{\rho_{a, s}}_{\reg{mto}} 
\Bigg) \\ 
& = 
\sum_{s \in \bits^\ell} \alpha_{a, s} 
\Bigg(
\sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}   \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{14em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \sum_{~s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*} \ket{a^*}_{\reg{a}}  W_1 \ket{s^*}_{\reg{s}}  \ket{\rho_{a, s}}_{\reg{mto}} 
\Bigg) \numberthis \label{proof:err-inv-com:property-1:dummy:derive:2} \\
& =
\ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \sum_{ s^* \in \bits^\ell} \beta^{a, s}_{a, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho_{a, s}}_{\reg{mto}} ~~+  \\
& \hspace{7em}
\sum_{a^* \in \bits^\ell \setminus \Set{a}} \ket{a^*}_{\reg{a}} \red{W_1} \sum_{s \in \bits^\ell} \alpha_{a, s} \sum_{s^* \in \bits^\ell} \beta^{a, s}_{a^*, s^*}  \ket{s^*}_{\reg{s}}    \ket{\rho_{a, s}}_{\reg{mto}} \numberthis \label{proof:err-inv-com:property-1:dummy:derive:3} 
,\end{align*}
where \Cref{proof:err-inv-com:property-1:dummy:derive:1} follows from the definition of $\tilde{W}^\dagger$,  \Cref{proof:err-inv-com:property-1:dummy:derive:2} follows from the definition of $\tilde{W}$ and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$, and \Cref{proof:err-inv-com:property-1:dummy:derive:3} follows from standard algebraic calculation and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$.

Comparing the RHS of \Cref{proof:err-inv-com:property-1:dummy:derive:3} with the RHS of \Cref{proof:err-inv-com:property-1:derive:5}, we obtain the following observation
\begin{quote}
{\bf Observation:} the RHS of \Cref{proof:err-inv-com:property-1:dummy:derive:3} and the RHS of \Cref{proof:err-inv-com:property-1:derive:5} are identical, except that the \red{$W^\dagger_1$} in \Cref{proof:err-inv-com:property-1:dummy:derive:3} is instead being $W_1^\dagger U_0W_0$ in \Cref{proof:err-inv-com:property-1:derive:5}.
\end{quote}
Recall that previously, we have already proven that  \Cref{proof:err-inv-com:property-1:derive:5} can be equivalently written as (i.e., \Cref{eq:lem:err-inv-com:property-1:real}) 
$$
W U SU^\dagger W^\dagger  \ket{\eta} 
= 
\gamma_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'}\ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \ket{\tilde{\rho}_{a'}}_{\reg{mtso}}. 
$$
This equation, together with the above {\bf Observation}, implies that \Cref{proof:err-inv-com:property-1:dummy:derive:3} can be equivalently written (with exactly the same $\gamma_a$, $\gamma_{a'}$, $\tilde{\rho}_{a}$, and $\tilde{\rho}_{a'}$) as
$$
\tilde{W} S \tilde{W}^\dagger \ket{\eta} 
= 
\gamma_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'}\ket{a'}_{\reg{a}} \red{W_1} \ket{\tilde{\rho}_{a'}}_{\reg{mtso}}.  
$$
This concludes the proof of \Cref{eq:lem:err-inv-com:property-1:dummy} (and \Cref{lem:err-inv-com:property-1}). 

\subsubsection{Deriving \Cref{eq:lem:err-inv-com:property-2:real}}
We now derive \Cref{eq:lem:err-inv-com:property-2:real}:
\begin{align*}
WU SU^\dagger W^\dagger  \cdot \ket{\eta_0} 
& = 
W U SU^\dagger W^\dagger  \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \ket{\rho_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{a'}}_{\reg{mtso}} 
\Big) \\ 
& = 
W U SU^\dagger W^\dagger  \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U SU^\dagger W^\dagger  \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:1} \\ 
& =  
W U SU^\dagger \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:2} \\ 
& =  
W U S \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:3} \\ 
& = 
W U S \cdot 
\Big(
\sum_{a' \in \bits^{\ell}} \gamma_{a'} \ket{a'}_{\reg{a}}  \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U S \cdot 
\Big(
\sum_{a',s \in \bits^\ell} \gamma_{a'}\alpha_{a', s} \ket{a'}_{\reg{a}} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U \cdot 
\Big(
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s} S \ket{a'}_{\reg{a}} \ket{s}_{\reg{s}} U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big)  \\ 
\text{(by \Cref{proof:err-inv-com:property-1:derive:S-format})}~~ & =
W  U \cdot 
\Big(
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
W U \cdot 
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}}
\Big) \\
& = 
W \cdot 
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}  W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}}
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:4} \\ 
& = 
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}  \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    W_1 U^\dagger_0 W^\dagger_0 \ket{\rho_{a', s}}_{\reg{mto}}
\Big) \numberthis \label{proof:err-inv-com:property-2:real:derive:5} \\ 
& = 
\ket{a}_{\reg{a}} \sum_{a' \in \bits^\ell} \gamma_{a'} \sum_{ s \in \bits^\ell}  \alpha_{a', s}  
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{0em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \ket{a^*}_{\reg{a}}   W_1 U^\dagger_0 W^\dagger_0    \sum_{a' \in \bits^\ell} \gamma_{a'} \sum_{s \in \bits^\ell} \alpha_{a', s}  \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho_{a', s}}_{\reg{mto}}
\numberthis \label{proof:err-inv-com:property-2:real:derive:6}
,\end{align*}
where \Cref{proof:err-inv-com:property-2:real:derive:1} follows from the fact that all the unitary  operators $W_1$, $U^\dagger_0$, and $W^\dagger_0$ act as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:2} follows from the definition of $W^\dagger$ and the fact that $W^\dagger_0$ and $W^\dagger_1$ act as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:3} follow from the definition of $U^\dagger$ and the fact that $U^\dagger_0$ acts as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:4} follow from the definition of $U$ and the fact that $U_0$ acts as identity on $\Hil_{\reg{s}}$, \Cref{proof:err-inv-com:property-2:real:derive:5} follow from the definition of $W$ and the fact that $W_0$ and $W_1$ act as identity on $\Hil_{\reg{s}}$, and \Cref{proof:err-inv-com:property-2:real:derive:6} follows from standard algebraic calculation and the fact that all the unitary  operators $W_1$, $U^\dagger_0$, and $W^\dagger_0$ act as identity on $\Hil_{\reg{s}}$.

It is now not hard to see that the RHS of \Cref{proof:err-inv-com:property-2:real:derive:6} can be equivalently written in the same format as the RHS of \Cref{eq:lem:err-inv-com:property-2:real}, by properly setting the parameters $\tilde{\gamma}_a$, $\tilde{\gamma}_{a'}$, $\tilde{\rho}_a$, and $\tilde{\rho}_{a'}$. This step is almost identical to the normalization procedure we described in the part starting with ``{\bf Equivalence of \Cref{proof:err-inv-com:property-1:derive:5} and  \Cref{eq:lem:err-inv-com:property-1:real}}'' on \Cpageref{proof:err-inv-com:property-1:normalization}. Thus, we do not repeat it here.

This concludes the proof of \Cref{eq:lem:err-inv-com:property-2:real}.



\subsubsection{Deriving \Cref{eq:lem:err-inv-com:property-2:dummy}}


Finally, we derive \Cref{eq:lem:err-inv-com:property-2:dummy}:
\begin{align*}
\tilde{W} S\tilde{W}^\dagger \cdot \ket{\eta_1} 
& = 
\tilde{W} S\tilde{W}^\dagger \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \ket{\rho_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} W_1 \ket{\rho_{a'}}_{\reg{mtso}} 
\Big) \\ 
& = 
\tilde{W} S\tilde{W}^\dagger \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} W_1 \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\
& = 
\tilde{W} S \cdot 
\Big(
\gamma_a \ket{a}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a, s} \ket{s}_{\reg{s}} \ket{\rho_{a, s}}_{\reg{mto}} ~~+ \\ 
& \hspace{10em}
 \sum_{a' \in \bits^{\ell}\setminus \Set{a}} \gamma_{a'} \ket{a'}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}} 
\Big)  \numberthis \label{proof:err-inv-com:property-2:dummy:derive:1} \\ 
& = 
\tilde{W} S \cdot \Big(\sum_{a' \in \bits^{\ell}} \gamma_{a'} \ket{a'}_{\reg{a}} \sum_{s \in \bits^\ell} \alpha_{a', s} \ket{s}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
\tilde{W}  \cdot \Big(\sum_{a',s \in \bits^{\ell}} \gamma_{a'}  \alpha_{a', s} S\ket{a'}_{\reg{a}}\ket{s}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
\text{(by \Cref{proof:err-inv-com:property-1:derive:S-format})}~~ & =
\tilde{W} \cdot 
\Big(
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  \sum_{a^*, s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}    \ket{\rho_{a', s}}_{\reg{mto}} 
\Big) \\ 
& = 
\tilde{W} \cdot 
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}}   \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}}  \ket{\rho_{a', s}}_{\reg{mto}}
\Big) \\
& = 
\sum_{a', s \in \bits^\ell} \gamma_{a'}\alpha_{a', s}  
\Big(
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*} \ket{a}_{\reg{a}} \ket{s^*}_{\reg{s}} \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{12em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*} \ket{a^*}_{\reg{a}} \ket{s^*}_{\reg{s}} W_1 \ket{\rho_{a', s}}_{\reg{mto}}
\Big) \numberthis \label{proof:err-inv-com:property-2:dummy:derive:2} \\ 
& = 
\ket{a}_{\reg{a}} \sum_{a' \in \bits^\ell} \gamma_{a'} \sum_{ s \in \bits^\ell}  \alpha_{a', s}  
\sum_{ s^* \in \bits^{\ell}} \beta^{a', s}_{a, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho_{a', s}}_{\reg{mto}} ~~+ \\ 
& \hspace{0em}
\sum_{a^* \in \bits^{\ell} \setminus \Set{a}} \ket{a^*}_{\reg{a}}   \red{W_1}     \sum_{a' \in \bits^\ell} \gamma_{a'} \sum_{s \in \bits^\ell} \alpha_{a', s}  \sum_{~s^* \in \bits^{\ell}} \beta^{a', s}_{a^*, s^*}  \ket{s^*}_{\reg{s}}  \ket{\rho_{a', s}}_{\reg{mto}}
\numberthis \label{proof:err-inv-com:property-2:dummy:derive:3}
,\end{align*}
where \Cref{proof:err-inv-com:property-2:dummy:derive:1} follows from the definition of $\tilde{W}^\dagger$, \Cref{proof:err-inv-com:property-2:dummy:derive:2} follows from the definition of $\tilde{W}$ and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$, and \Cref{proof:err-inv-com:property-2:dummy:derive:3} follows from standard algebraic calculation and the fact that $W_1$ acts as identity on $\Hil_{\reg{s}}$.

Comparing the RHS of \Cref{proof:err-inv-com:property-2:dummy:derive:3} with the RHS of \Cref{proof:err-inv-com:property-2:real:derive:6}, we obtain the following observation
\begin{quote}
{\bf Observation:} the RHS of \Cref{proof:err-inv-com:property-2:dummy:derive:3} and the RHS of \Cref{proof:err-inv-com:property-2:real:derive:6} are identical, except that the \red{$W_1$} in \Cref{proof:err-inv-com:property-2:dummy:derive:3} is instead being $W_1 U^\dagger_0 W^\dagger_0$ in \Cref{proof:err-inv-com:property-2:real:derive:6}.
\end{quote}
Recall that previously, we have already proven that  \Cref{proof:err-inv-com:property-2:real:derive:6} can be equivalently written as (i.e., \Cref{eq:lem:err-inv-com:property-2:real}) 
$$
W U SU^\dagger W^\dagger \ket{\eta_0} 
= 
\tilde{\gamma}_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \tilde{\gamma}_{a'}\ket{a'}_{\reg{a}} W_1 U^\dagger_0 W^\dagger_0 \ket{\tilde{\rho}_{a'}}_{\reg{mtso}}. 
$$
This equation, together with the above {\bf Observation}, implies that \Cref{proof:err-inv-com:property-2:dummy:derive:3} can be equivalently written (with exactly the same $\tilde{\gamma}_a$, $\tilde{\gamma}_{a'}$, $\tilde{\rho}_{a}$, and $\tilde{\rho}_{a'}$) as
$$
\tilde{W} S \tilde{W}^\dagger \ket{\eta_1} 
= 
\tilde{\gamma}_a \ket{a}_{\reg{a}} \ket{\tilde{\rho}_a}_{\reg{mtso}} + \sum_{a' \in \bits^{\ell} \setminus \Set{a}} \tilde{\gamma}_{a'}\ket{a'}_{\reg{a}} \red{W_1} \ket{\tilde{\rho}_{a'}}_{\reg{mtso}}.  
$$
This concludes the proof of \Cref{eq:lem:err-inv-com:property-2:dummy} (and \Cref{lem:err-inv-com:property-2}). 


==> sections/main-lemma.tex <==
\section{Proving \Cref{CPM-3ZK:MnR:game:dummy:lem} (Preparation)}

\subsection{Branch-Wise Equivalence Suffices}
We first notice that \Cref{CPM-3ZK:MnR:game:real} can be treated as a sequence of alternating unitaries and measurements. In particular, there are two types of measurements (and $(q+K)$ measurements are made in total):
\begin{enumerate}
\item
\label[Type]{CPM-3ZK:branchwise:measure:type:1}
{\bf Type-1:} Recall that the simulator $\Sim$ simply alternates between her local unitary $S$ and the measurement on register $\reg{u}$, which determines the type of her next query (i.e., either $\tilde{V}$ or $\tilde{V}^\dagger$). Note that there are $q$ such measurements on $\reg{u}$ since $\Sim$ makes $q$ queries in total.
\item
\label[Type]{CPM-3ZK:branchwise:measure:type:2}
{\bf Type-2:}
When $\Sim$ makes the $\msf{sq}(i)$-th query, it triggers a measurement on registers $\reg{p_1} \ldots \reg{p_i}$. Note that there are $K$ such measurements (if the game is not aborted prematurely).
\end{enumerate}
Also, notice that in \Cref{CPM-3ZK:MnR:game:real}, the values $\Set{j_i}_{i \in [K]}$ are sampled at the very beginning and after that the timing of all the measurements are fixed. It then follows from \Cref{branchwise:lem} that the accepting probability $\Pr[\msf{Pred}(\rho)=1]$ w.r.t.\  \Cref{CPM-3ZK:MnR:game:real} can be equivalently expressed as the summation of all accepting probabilities w.r.t.\ a ``sub-normalized'' version of \Cref{CPM-3ZK:MnR:game:real} where all the $(q+ K)$ measurements are replaced with projections. Formally, we defined the ``sub-normalized'' \Cref{CPM-3ZK:MnR:game:real} (and similarly for \Cref{CPM-3ZK:MnR:game:dummy}) in \Cref{CPM-3ZK:MnR:game:subnormalized}.

\begin{GameBox}[label={CPM-3ZK:MnR:game:subnormalized}]{Sub-Normalized Games \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$} and \textnormal{$\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$}}
{\bf Parameters.} Fix $J = \Set{j_i}_{i \in [K]}$ such that each $j_i \in [q]$ and $j_1 < j_2 < \ldots < j_K$. Also fix a classical string of $(q+K)$ symbols $\msf{pat} = (u_1, u_2, \ldots, u_q, p_1, p_2,  \ldots, p_K)$ with each $u_i \in \Set{\uparrow, \downarrow}$, and each $p_i \in \Set{0, 1}^{\ell}$. The following games are parameterized by $(J, \msf{pat})$.

\para{Game $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} It behaves identically to \Cref{CPM-3ZK:MnR:game:real} except for the following differences: 
\begin{enumerate}
	\item
	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

\item
When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
\item
When the measurement on registers $\reg{p_1\ldots p_i}$ is triggered (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1, \ldots, p_i}$ registers $\reg{p_1\ldots p_i}$; 
\end{enumerate}

\para{Game $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$.} This is defined in a similar way as the above. Namely, It behaves identically to \Cref{CPM-3ZK:MnR:game:dummy} except for the following differences: 
\begin{enumerate}
	\item
	It does not sample $j_i$'s but use the $j_i$'s contained in $J$ instead 

\item
When $\Sim$ needs to make the $i$-th measurement on $\reg{u}$ (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:1} above), it instead applies the projector $\ketbra{u_i}$ to $\reg{u}$;
\item
When the measurement on registers $\reg{p_1\ldots p_i}$ is triggered (corresponding to \Cref{CPM-3ZK:branchwise:measure:type:2} above), it instead applies the projector $\ketbra{p_1, \ldots, p_i}$ registers $\reg{p_1\ldots p_i}$; 
\end{enumerate}
\end{GameBox}

It then follows from \Cref{branchwise:lem} that
\begin{align*}
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier})] 
& = 
\frac{K!}{\binom{q}{K}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] \\
\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier})] 
& = 
\frac{K!}{\binom{q}{K}} \cdot \sum_{J, \msf{pat}}\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})],
\end{align*}
where the summations are taken over all possible $J$ and $\msf{pat}$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}.\footnote{Note that the multiplicative factor $K!/\binom{q}{K}$ is to compensate for the fact that the $J$ in is fixed in \Cref{CPM-3ZK:MnR:game:subnormalized}, instead of being sampled randomly as in the original real and dummy games.}

Therefore, to prove \Cref{CPM-3ZK:MnR:game:dummy:lem}, it suffices to prove the following \Cref{CPM-3ZK:branch-wise:suffices}.
\begin{lemma}[Branch-Wise Equivalence Suffices]\label{CPM-3ZK:branch-wise:suffices}
For all $(J, \msf{pat})$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}, it holds that 
$$\Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})] = \Pr[\msf{Pred}(\rho) = 1~:~ (\vb{p}, \rho) \la \msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})].$$
\end{lemma}
\xiao{say that from now on, we prove \Cref{CPM-3ZK:branch-wise:suffices}.}

\xiao{Henceforth, we fix $(J, \msf{pat})$}


\subsection{Proving \Cref{CPM-3ZK:branch-wise:suffices}: Define Hybrids}
\label{sec:orignal:hybrids}

Next, we define a sequence of hybrids $H_0, H_1, \ldots, H_K$. 

\para{Hybrid $H_0^{(J, \msf{pat})}$.} This is exactly the execution of $\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. Therefore, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H_0 \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Real}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$




\para{Hybrid $H_k^{(J, \msf{pat})}$ $(k \in [K])$.} This hybrid is identical to $H^{(J, \msf{pat})}_{k-1}$, except for the following difference:
\begin{itemize}
\item
The first query (made by $\Sim$) that brings the global counter from $\ket{k-1}_{\reg{gc}}$ to $\ket{k}_{\reg{gc}}$ (i.e., query $\msf{sq}(k)$) is answered with $\tilde{V}$ (as in the previous hybrid). However, all subsequent queries that brings the global counter from $\ket{k-1}_{\reg{gc}}$ to $\ket{k}_{\reg{gc}}$ (resp.\ from $\ket{k}_{\reg{gc}}$ to $\ket{k-1}_{\reg{gc}}$) are answered with the ``dummy'' unitary $\ddot{V}$ (resp.\ $\ddot{V}^\dagger$).
\end{itemize}

\xiao{add intuitive explanation and refer to the $k=2$ figures}

It is easy to see that hybrid $H^{(J, \msf{pat})}_K$ is exactly the execution of $\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})$. Thus, it holds that
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_K \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la\msf{Dummy}(\Sim, \tilde{\Verifier}, J, \msf{pat})\big].$$


With the above hybrids, to prove \Cref{CPM-3ZK:branch-wise:suffices}, it now suffices to establish the following \Cref{lem:H:IND}. 
\begin{lemma}\label{lem:H:IND}
For all $(J, \msf{pat})$ satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized} and all $k \in [K]$, it holds that 
$$\Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_{k-1} \big] = \Pr\big[\msf{Pred}(\rho) = 1~:~(\vb{p}, \rho)\la H^{(J, \msf{pat})}_k \big].$$
\end{lemma}

\xiao{say that from now on, we prove \Cref{lem:H:IND}.}



\subsection{Prove \Cref{lem:H:IND}: Structure of Counters}

\xiao{add intuitive explanation about counter structure lemma.}


\begin{lemma}[Counter Structure.]\label{counter-structure:lemma}
For each  pair $(J, \msf{pat})$ satisfying satisfying the requirements in \Cref{CPM-3ZK:MnR:game:subnormalized}, each $k \in [K] \cup \Set{0}$, in hybrid $H^{(J, \msf{pat})}_{k}$, let $\ket{\phi^{(t,i)}}$ denote the overall state right after the $\Sim$'s query that leads to the global counter's $t$-th arrival at value $i$.

Then, the state $\ket{\phi^{(t,i)}}$ can be written in the following format:
\begin{align*}
\ket{\phi^{(t,i)}} 
& =  
\ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}\ket{\rho^{(t,i)}} ~+  \\
& \hspace{8em} 
\ket{i}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(t,i)}_{p'_{j+1}}}
\numberthis \label{counter-strucutre:psi:format}
\end{align*}
where the summation over $p'_{j+1} \ne p_{j+1}$ means to take the summation over $p'_{j+1} \in \bits^\ell \setminus \Set{p_{j+1}}$.

For readability, we expand the above succinct \Cref{counter-strucutre:psi:format}:
\begin{align*}
\ket{\phi^{(t,i)}}
= & 
\ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}\ket{\rho^{(t,i)}} ~+  \\ 
&
\ket{i}_{\reg{gc}} \ket{i-1}_{\reg{lc}} \ket{p_1, \ldots, p_{i-1}}_{\reg{p_1, \ldots, p_{i-1}}} \sum_{p'_i \ne p_i} \ket{p'_i}_{\reg{p_i}} \ket{\rho^{(t,i)}_{ p'_i}} ~+  \\ 
&
\ket{i}_{\reg{gc}} \ket{i-2}_{\reg{lc}} \ket{p_1, \ldots, p_{i-2}}_{\reg{p_1, \ldots, p_{i-2}}} \sum_{p'_{i-1} \ne p_{i-1}} \ket{p'_{i-1}}_{\reg{p_{i-1}}} \ket{\rho^{(t,i)}_{p'_{i-1}}} ~+  \\ 
& \cdots \\ 
&
\ket{i}_{\reg{gc}} \ket{1}_{\reg{lc}} \ket{p_1}_{\reg{p_1}} \sum_{p'_{2} \ne p_2} \ket{p'_2}_{\reg{p_2}} \ket{\rho^{(t,i)}_{p'_2}} ~+  \\ 
&
\ket{i}_{\reg{gc}} \ket{0}_{\reg{lc}} \sum_{p'_{1}} \ket{p'_1}_{\reg{p_1}} \ket{\rho^{(t,i)}_{p'_1 \ne p_1}} 
.\end{align*}
\end{lemma}


\begin{proof}[Proof of \Cref{counter-structure:lemma}]
We prove this lemma via mathematical induction over the operations performed by the simulator $\Sim$. That is, we first prove that the initial state at the very beginning of the MnR game is of the format shown in \Cref{counter-strucutre:psi:format} (i.e., the base case), and then show that each movement of $\Sim$ will lead to a new state of the same format shown in \Cref{counter-strucutre:psi:format} as well (i.e., the induction step).

\para{Base Case.} This corresponds to the state at the very beginning of the MnR game. By definition, the initial sate is of the format $\ket{0}_{\reg{gc}}\ket{0}_{\reg{lc}}\ket{\rho}$. It satisfies the format shown in \Cref{counter-strucutre:psi:format} (by setting $\ket{\rho^{(0,0)}} \coloneqq \ket{\rho}$).

\para{Induction Step.} We assume that the lemma is true for the global counter's $t$-th arrival at value $i$, namely, the current overall state $\ket{\phi^{(t,i)}}$ satisfies the format shown in \Cref{counter-strucutre:psi:format}. We prove that the simulator's next query, no matter what this query is, will lead to a new state that satisfies the format shown in \Cref{counter-strucutre:psi:format} as well.

Toward that, let us first classify the possible movements of $\Sim$ when the state is $\ket{\phi^{(t,i)}}$.
\begin{itemize}
 \item
 \underline{Case 1:} after applying the local operator $S$ and measuring register $\reg{u}$, $\Sim$ makes the $\msf{sq}(i+1)$ query for some $i \in [K]$. (Recall that when the global counter is $i$ and $\Sim$ is about to make a $\msf{sq}(j)$ query, then it must be the $\msf{sq}(i+1)$ query.) 

 \item
 \underline{Case 2:} after applying the local operator $S$ and measuring register $\reg{u}$, $\Sim$ makes a $\tilde{V}$ query that is not the $\msf{sq}(i+1)$ query. (This could happen only if the global counter $i \ge k$)

\item
 \underline{Case 3:} after applying the local operator $S$ and measuring register $\reg{u}$, $\Sim$ makes a $\tilde{V}^\dagger$ query. (This could happen only if the global counter $i > k$)

 \item
 \underline{Case 4:} after applying the local operator $S$ and measuring register $\reg{u}$, $\Sim$ makes a $\ddot{V}$ query. (This could happen if the global counter $i < k$.)

 \item
 \underline{Case 5:} after applying the local operator $S$ and measuring register $\reg{u}$, $\Sim$ makes a $\ddot{V}^\dagger$ query. (This could happen if the global counter $i \le k$.)
 \end{itemize} 
The proof for the above five cases are very similar. In the following, we only show the proofs for \underline{Case 2} and \underline{Case 3}, which are the most representative cases as they cover the cases of both a ``going-up'' query and a ``going-down'' query.



\subpara{Proof of Case 2:} In this case, $\Sim$ first applies the local operator $S$. Then, she measures the $\reg{u}$ register. Recall that we are in the ``sub-normalized'' game $H^{(J, \msf{pat})}_{k}$, and thus this measurement is replaced with a projector $\ketbra{\downarrow}_{\reg{u}}$ (it must be a $\downarrow$ because in this case the coming query is $\tilde{V}$). Finally, $\Sim$ makes a $\tilde{V}$ query. Notation-wise, we assume this leads to the global counter's $z$-th arrival at value $i+1$.

In summary, the state $\ket{\phi^{(t,i)}}$ evolves as follows 
\begin{align*}
 \ket{\phi^{(z,i+1)}} 
 &= 
 \tilde{V} \ketbra{\downarrow}_{\reg{u}} S \ket{\phi^{(t,i)}} 
\\
& = 
\tilde{V} \ketbra{\downarrow}_{\reg{u}} S 
\bigg(
\ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}\ket{\rho^{(t,i)}} ~+  \\
& \hspace{8em} 
\ket{i}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(t,i)}_{p'_{j+1}}}
\bigg) 
\numberthis \label{counter-strucutre:proof:case2:eq:1} \\ 
& =
\tilde{V}
\bigg(\ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}} ~+  \\
& \hspace{8em} 
\ket{i}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}}
\bigg) 
\numberthis \label{counter-strucutre:proof:case2:eq:2} \\ 
& =
D_{i+1}C_{i+1}B_{i+1}A_{i+1}\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}}
~+ \\ 
& \hspace{6em}
C'_{i+1}A_{i+1}\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:3} \\ 
& =
D_{i+1}C_{i+1}B_{i+1}\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}} A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}}
~+ \\ 
& \hspace{6em}
\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} C'_{i+1}A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:4} \\
& =
D_{i+1}C_{i+1}B_{i+1}\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}  \sum_{p'_{i+1} \in \bits^{\ell}} \ket{p'_{i+1}}_{\reg{p_{i+1}}} \ket{\rho^{(t,i)}_{p'_{i+1}}}
~+ \\ 
& \hspace{6em}
\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} C'_{i+1}A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:5} \\  
& =
D_{i+1}C_{i+1}B_{i+1}\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}  
\bigg( 
\ket{p_{i+1}}_{\reg{p_{i+1}}} \ket{\rho^{(t,i)}_{p_{i+1}}} 
~+ \\ 
& \hspace{22em}
\sum_{p'_{i+1} \ne p_{i+1}} \ket{p'_{i+1}}_{\reg{p_{i+1}}} \ket{\rho^{(t,i)}_{p'_{i+1}}}
\bigg)
~+ \\ 
& \hspace{6em}
\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} C'_{i+1}A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\\  
& =
D_{i+1}\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}  
\bigg( 
\ket{p_{i+1}}_{\reg{p_{i+1}}} C_{i+1,1}B_{i+1,1} \ket{\rho^{(t,i)}_{p_{i+1}}} 
~+ \\ 
& \hspace{22em}
\sum_{p'_{i+1} \ne p_{i+1}} \ket{p'_{i+1}}_{\reg{p_{i+1}}} C_{i+1,0}B_{i+1,0}\ket{\rho^{(t,i)}_{p'_{i+1}}}
\bigg)
~+ \\ 
& \hspace{6em}
\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} C'_{i+1}A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:6} \\ 
& =
D_{i+1}\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}  
\bigg( 
\ket{p_{i+1}}_{\reg{p_{i+1}}}  \ket{\rho^{(z,i+1)}} 
~+~
\sum_{p'_{i+1} \ne p_{i+1}} \ket{p'_{i+1}}_{\reg{p_{i+1}}} \ket{\rho^{(z,i+1)}_{p'_{i+1}}}
\bigg)
~+ \\ 
& \hspace{13em}
\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(z,i+1)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:7} \\ 
& =
\ket{i+1}_{\reg{gc}} \ket{i+1}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}  
\ket{p_{i+1}}_{\reg{p_{i+1}}}  \ket{\rho^{(z,i+1)}} 
~+~ \\ 
& \hspace{8em}
\ket{i+1}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}} \sum_{p'_{i+1} \ne p_{i+1}} \ket{p'_{i+1}}_{\reg{p_{i+1}}} \ket{\rho^{(z,i+1)}_{p'_{i+1}}}
~+ \\ 
& \hspace{13em}
\ket{i+1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(z,i+1)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:8} \\ 
& =
\ket{i+1}_{\reg{gc}} \ket{i+1}_{\reg{lc}} \ket{p_1, \ldots, p_{i+1}}_{\reg{p_1, \ldots, p_{i+1}}}\ket{\rho^{(z,i+1)}} 
~+~ \\ 
& \hspace{10em}
\ket{i+1}_{\reg{gc}} \sum^{i}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(z,i+1)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case2:eq:9} 
,\end{align*}
where
\begin{itemize}
\item
\Cref{counter-strucutre:proof:case2:eq:1} follows from our induction assumption.

\item
\Cref{counter-strucutre:proof:case2:eq:2} follows from the fact that $\ketbra{\downarrow}_{\reg{u}}S$ does not operate on the $\reg{gc}$, $\reg{lc}$, and $\reg{p_1 \ldots p_i}$ registers. 

\item
\Cref{counter-strucutre:proof:case2:eq:3} follows from the definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}).

\item
\Cref{counter-strucutre:proof:case2:eq:4} follows from the fact that $C'_{i+1}$ and $A_{i+1}$ do not act on  registers $\reg{p_1 \ldots p_i}$.

\item
\Cref{counter-strucutre:proof:case2:eq:5} follows by expanding the $\reg{p_{i+1}}$ register under the computational basis for the state:
$$A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}} = \sum_{p'_{i+1} \in \bits^{\ell}} \ket{p'_{i+1}}_{\reg{p_{i+1}}} \ket{\rho^{(t,i)}_{p'_{i+1}}}.$$

\item
\Cref{counter-strucutre:proof:case2:eq:6} follows from the following definitions: 
\begin{itemize}
\item
Define $C_{i+1, 1}$ and $B_{i+1, 1}$ as the parts of $C_{i+1}$ and $B_{i+1}$ (see \Cref{CPM-3ZK:V:unitary}) w.r.t.\ to the $H(p_1, \ldots, p_{i+1}) = 1$ branch, and define $C_{i+1, 0}$ and $B_{i+1, 0}$ as the parts of $C_{i+1}$ and $B_{i+1}$ (see \Cref{CPM-3ZK:V:unitary}) w.r.t.\ the $H(p_1, \ldots, p_{i+1}) = 0$ branch. (Therefore, none of $C_{i+1, 1}$, $C_{i+1, 0}$, $B_{i+1, 1}$, or $B_{i+1, 0}$ act on registers $\reg{p_1 \ldots p_{i+1}}$.) 
\end{itemize}  

\item
\Cref{counter-strucutre:proof:case2:eq:7} follows by defining
\begin{align*}
 \ket{\rho^{(z,i+1)}} 
 & \coloneqq  
 C_{i+1,1}B_{i+1,1} \ket{\rho^{(t,i)}_{p_{i+1}}}   
 \\
  \ket{\rho^{(z,i+1)}_{p'_{i+1}}} 
 & \coloneqq  
C_{i+1,0}B_{i+1,0}\ket{\rho^{(t,i)}_{p'_{i+1}}} ~~\big(\forall p'_{i+1} \ne p_{i+1}\big)
 \\
\ket{\rho^{(z,i+1)}_{p'_{j+1}}} 
  & \coloneqq 
  C'_{i+1}A_{i+1} \ketbra{\downarrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}}  ~~\big(\forall j \in \Set{0,1, \ldots, i-1},~\forall p'_{j+1} \ne p_{j+1}\big)
.\end{align*}  

\item
\Cref{counter-strucutre:proof:case2:eq:8} follows by the definition of $D_{i+1}$ (see \Cref{CPM-3ZK:V:unitary}).
\end{itemize}
Obviously, \Cref{counter-strucutre:proof:case2:eq:9} satisfies the format of \Cref{counter-strucutre:psi:format} with $t$ updated to $z$ and $i$ updated to $i+1$. This finishes the proof of \underline{Case 2}.


\subpara{Proof of Case 3:} In this case, $\Sim$ first applies the local operator $S$. Then, she measures the $\reg{u}$ register. Recall that we are in the ``sub-normalized'' game $H^{(J, \msf{pat})}_{k}$, and thus this measurement is replaced with a projector $\ketbra{\uparrow}_{\reg{u}}$ (it must be a $\uparrow$ because in this case the coming query is $\tilde{V}^\dagger$). Finally, $\Sim$ makes a $\tilde{V}^\dagger$ query. Notation-wise, we assume this leads to the global counter's $z$-th arrival at value $i-1$.

In summary, the state $\ket{\phi^{(t,i)}}$ evolves as follows 
\begin{align*}
 \ket{\phi^{(z,i-1)}} 
 &= 
 \tilde{V}^\dagger \ketbra{\uparrow}_{\reg{u}} S \ket{\phi^{(t,i)}} 
\\
& = 
\tilde{V}^\dagger \ketbra{\uparrow}_{\reg{u}} S 
\bigg(
\ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}}\ket{\rho^{(t,i)}} ~+  \\
& \hspace{8em} 
\ket{i}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(t,i)}_{p'_{j+1}}}
\bigg) 
\numberthis \label{counter-strucutre:proof:case3:eq:1} \\ 
& = 
\tilde{V}^\dagger  
\bigg(
\ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}} \ketbra{\uparrow}_{\reg{u}} S \ket{\rho^{(t,i)}} ~+  \\
& \hspace{8em} 
\ket{i}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ketbra{\uparrow}_{\reg{u}} S \ket{\rho^{(t,i)}_{p'_{j+1}}}
\bigg) 
\numberthis \label{counter-strucutre:proof:case3:eq:2} \\ 
& =
U^\dagger_{gc} A^\dagger_i B^\dagger_i C^\dagger_i D^\dagger_i  \ket{i}_{\reg{gc}} \ket{i}_{\reg{lc}} \ket{p_1, \ldots, p_i}_{\reg{p_1, \ldots, p_i}} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}}
~+ \\ 
& \hspace{6em}
U^\dagger_{gc} A^\dagger_{i} C'^\dagger_{i} \ket{i}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}\ket{p'_{j+1}}_{\reg{p_{j+1}}} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case3:eq:3} \\ 
& =
\ket{i-1}_{\reg{gc}} \ket{i-1}_{\reg{lc}} \ket{p_1, \ldots, p_{i-1}}_{\reg{p_1, \ldots, p_{i-1}}} A^\dagger_i \ket{p_i}_{\reg{p_i}} B^\dagger_{i,1} C^\dagger_{i,1}  \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}}
~+ \\ 
& \hspace{6em}
 \ket{i-1}_{\reg{gc}} \sum^{i-1}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}} A^\dagger_{i}  \ket{p'_{j+1}}_{\reg{p_{j+1}}} C'^\dagger_{i} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case3:eq:4} \\ 
& =
\ket{i-1}_{\reg{gc}} \ket{i-1}_{\reg{lc}} \ket{p_1, \ldots, p_{i-1}}_{\reg{p_1, \ldots, p_{i-1}}} A^\dagger_i \ket{p_i}_{\reg{p_i}} B^\dagger_{i,1} C^\dagger_{i,1}  \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}}
~+ \\ 
& \hspace{6em}
 \ket{i-1}_{\reg{gc}} \ket{i-1}_{\reg{lc}} \ket{p_1, \ldots, p_{i-1}}_{\reg{p_1, \ldots, p_{i-1}}} \sum_{p'_{i} \ne p_{i}} A^\dagger_{i}  \ket{p'_{i}}_{\reg{p_{i}}} C'^\dagger_{i} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{i}}}   
 \\
& \hspace{6em}
 \ket{i-1}_{\reg{gc}} \sum^{i-2}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}  \ket{p'_{j+1}}_{\reg{p_{j+1}}} A^\dagger_{i}  C'^\dagger_{i} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case3:eq:5} \\ 
& =
\ket{i-1}_{\reg{gc}} \ket{i-1}_{\reg{lc}} \ket{p_1, \ldots, p_{i-1}}_{\reg{p_1, \ldots, p_{i-1}}} \ket{\rho^{(z,i-1)}}
~+  \\
& \hspace{6em}
 \ket{i-1}_{\reg{gc}} \sum^{i-2}_{j = 0} \ket{j}_{\reg{lc}} \ket{p_1, \ldots, p_j}_{\reg{p_1, \ldots, p_j}} \sum_{p'_{j+1} \ne p_{j+1}}  \ket{p'_{j+1}}_{\reg{p_{j+1}}} \ket{\rho^{(z,i-1)}_{p'_{j+1}}} 
\numberthis \label{counter-strucutre:proof:case3:eq:6} 
,\end{align*}
where 
\begin{itemize}
\item
\Cref{counter-strucutre:proof:case3:eq:1} follows from our induction assumption

\item
\Cref{counter-strucutre:proof:case3:eq:2} follows from the fact that $\ketbra{\uparrow}_{\reg{u}}S$ does not operate on the $\reg{gc}$, $\reg{lc}$, and $\reg{p_1 \ldots p_i}$ registers. 

\item
\Cref{counter-strucutre:proof:case3:eq:3} follows from the definition of $\tilde{V}$ (see \Cref{CPM-3ZK:V:unitary}).

\item
\Cref{counter-strucutre:proof:case3:eq:4} follows from the definition of $D_i$ and $U_{gc}$ (see \Cref{CPM-3ZK:V:unitary}),   the fact that $A_{i}$ does not act on registers $\reg{p_1\ldots p_{i-1}}$, the fact that $C'_{i}$ does not act on registers $\reg{p_1\ldots p_{i}}$, and the following definitions. 
\begin{itemize}
\item
Define $C_{i, 1}$ and $B_{i, 1}$ as the part of $C_{i}$ and $B_{i}$ (see \Cref{CPM-3ZK:V:unitary}) corresponding to the $H(p_1, \ldots, p_i) = 1$ branch (and thus $C_{i, 1}$ and $B_{i, 1}$ do not act on registers $\reg{p_1 \ldots p_i}$).
\end{itemize} 

\item
\Cref{counter-strucutre:proof:case3:eq:5}  follows by isolating the $(j = i-1)$ term and that $A_{i}$ does not act on registers $\reg{p_1\ldots p_{i-1}}$.

\item
\Cref{counter-strucutre:proof:case3:eq:6} follows by defining
\begin{align*}
 \ket{\rho^{(z,i-1)}} 
 & \coloneqq  
 A^\dagger_i \ket{p_i}_{\reg{p_i}} B^\dagger_{i,1} C^\dagger_{i,1}  \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}} 
 + 
 \sum_{p'_{i} \ne p_{i}} A^\dagger_{i}  \ket{p'_{i}}_{\reg{p_{i}}} C'^\dagger_{i} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{i}}}  
 \\
\ket{\rho^{(z,i-1)}_{p'_{j+1}}} 
  & \coloneqq 
  A^\dagger_{i}  C'^\dagger_{i} \ketbra{\uparrow}_{\reg{u}}S \ket{\rho^{(t,i)}_{p'_{j+1}}} ~~\big(\forall j \in \Set{0,1, \ldots, i-2},~\forall p'_{j+1} \ne p_{j+1}\big)
.\end{align*}  
\end{itemize}
Obviously, \Cref{counter-strucutre:proof:case3:eq:6} satisfies the format of \Cref{counter-strucutre:psi:format} with $t$ updated to $z$ and $i$ updated to $i-1$. This finishes the proof of \underline{Case 3}.

\vspace{1em}
This finishes the proof of \Cref{counter-structure:lemma}.

\end{proof}

\subsection{Re-Stating the Hybrids}
\label{sec:CPM:hybrids:restate}

With \Cref{counter-structure:lemma} in hand, we can re-state the hybrids without explicitly mentioning the $\reg{lc}$ register anymore. \xiao{Explain the benefits of this.}


For a fixed $(J, \msf{pat})$, recall that $\msf{pat}$ contain a fix sequence $\vb{p} = (p_1, \ldots, p_K)$. For such a fixed $\vb{p}$, we re-define (in \Cref{re-define:unitaries}) the unitaries $\Set{(A_i, B_i, C_i, D_i)}_{i \in [K]}$ {\em that depend on this $\vb{p}$}. We emphasize that these uintaries were originally defined in \Cref{CPM-3ZK:V:unitary}. Now, we re-load them w.r.t.\ a fix $\vb{p}$. (Technically, we should have include $\vb{p}$ in the superscript, such as $A^{\vb{p}}_i$, to indicate the dependence on $\vb{p}$. But we choose to omit it for succinct notation.)

\xiao{if possible, change the index from $i$ to $k$.}
\begin{AlgorithmBox}[label={re-define:unitaries}]{Re-Define Verifier's Unitaries for Fixed \textnormal{$(p_1, \ldots, p_K)$}}
For the $\vb{p} = (p_1, \ldots, p_K)$ contained in $(J, \msf{pat})$, we keep the $U_{gc}$, $U_{lc}$, and $A_i$ the same as in \Cref{CPM-3ZK:V:unitary}, but we re-define the unitaries $B_i$, $C_i$, $\ddot{C}_i$, and $D_i$ ($\forall i \in [K]$) in the following format:
\begin{enumerate} 
\item \label{CPM-3ZK:renaming:Bi}
Let $B_i = \ketbra{p_1, \ldots, p_i}_{\reg{p_1}\ldots\reg{p_i}} \tensor B_{i,1} + \sum_{(p'_1, \ldots, p'_i) \ne (p_1, \ldots, p_i)}  \ketbra{p'_1, \ldots, p'_i}_{\reg{p_1}\ldots\reg{p_i}} \tensor I$. Note that $B_{i,1}$ is exactly the $V_{p_1,\ldots,p_i}$ in \Cref{CPM-3ZK:V:unitary}, which acts non-trivially only on $\reg{v_i}$ and $\reg{w}$, and works as identity on other registers.

\item \label{CPM-3ZK:renaming:Ci}
Let $C_i = \ketbra{p_1, \ldots, p_i}_{\reg{p_1}\ldots\reg{p_i}} \tensor C_{i,1} + \sum_{(p'_1, \ldots, p'_i) \ne (p_1, \ldots, p_i)}  \ketbra{p'_1, \ldots, p'_i}_{\reg{p_1}\ldots\reg{p_i}} \tensor C_{i,0}$. Note that $C_{i,1}$ is the swap operator between $\reg{m}$ and $\reg{v_i}$, and $C_{i,0}$ is the swap operator between $\reg{m}$ and $\reg{t_i}$.

\item \label{CPM-3ZK:renaming:ddotCi}
Let $\ddot{C}_i = \ketbra{p_1, \ldots, p_i}_{\reg{p_1}\ldots\reg{p_i}} \tensor I + \sum_{(p'_1, \ldots, p'_i) \ne (p_1, \ldots, p_i)}  \ketbra{p'_1, \ldots, p'_i}_{\reg{p_1}\ldots\reg{p_i}}  \tensor C_{i,0}$. (Recall the definition of $C_{i,0}$ from \Cref{CPM-3ZK:renaming:Ci}.)

\item \label{CPM-3ZK:renaming:Di}
Let $D_i = \ketbra{p_1, \ldots, p_i}_{\reg{p_1}\ldots\reg{p_i}}  \tensor D_{i,1} + \sum_{(p'_1, \ldots, p'_i) \ne (p_1, \ldots, p_i)}  \ketbra{p'_1, \ldots, p'_i}_{\reg{p_1}\ldots\reg{p_i}}  \tensor I$. Note that $D_{i,1}$ is the local-counter increasing unitary $U_{lc}$, which acts non-trivially only on $\reg{lc}$. 
\end{enumerate}
\end{AlgorithmBox}

It will be helpful to keep track of the registers on which the unitaries (in \Cref{re-define:unitaries}) acts on {\em non-trivially}. For the reader's convenience, we summarize it in \Cref{CPM-3ZK:non-trivial-registers:table}. For a unitary shown in the table, it acts as the identity on registers not shown in its row. \xiao{check the facts regarding {\bf Assumptions 3}.}
\begin{table}[!htb]
\centering
\caption{Registers on which the unitaries acts non-trivially}
\label{CPM-3ZK:non-trivial-registers:table}
\vspace{0.5em}
\begin{tabular}{C{50pt} C{70pt} c C{50pt} C{70pt}}
\toprule
Unitary operators & Non-trivial registers & \phantom{abcde}  & Unitary operators & Non-trivial registers \\ 
\cmidrule{1-2} \cmidrule{4-5}
% \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\addlinespace[0.3em]
$A_i$    	& $\reg{p_i}, \reg{m}$ & & 
$\ddot{C}_i$    	&  $\reg{p_1 \ldots p_i}$,  $\reg{t_i}$, $\reg{m}$   \\ 
\addlinespace[0.3em]
$B_i$ 		& $\reg{p_1 \ldots p_i}$,  $\reg{v_i}$, $\reg{w}$   & & 
$D_i$		&  $\reg{p_1 \ldots p_i}$, $\reg{lc}$ \\
\addlinespace[0.3em]
$B_{i,1}$ 	& $\reg{v_i}$, $\reg{w}$  & & 
$D_{i,1}$		& $\reg{lc}$   \\ 
\addlinespace[0.3em]
$C_i$    	&  $\reg{p_1 \ldots p_i}$,  $\reg{v_i}$, $\reg{t_i}$, $\reg{m}$ & & 
$U_{gc}$ & $\reg{gc}$  \\ 
\addlinespace[0.3em]
$C_{i,1}$   & $\reg{v_i}$, $\reg{m}$  & & 
$S$ 		& $\reg{m}$, $\reg{u}$, $\reg{s}$  \\ 
\addlinespace[0.3em]
$C_{i,0}$  	& $\reg{t_i}$, $\reg{m}$ & & 
&  \\   
\bottomrule
\end{tabular}
\end{table}

Next, we re-state the hybrids $\Set{H^{(J, \msf{pat})}_k}_{k \in [K] \cup \Set{0}}$ in \xiao{cref} and prove (via \Cref{counter-structure:lemma}) that they are indeed equivalent to the original version defined in \Cref{sec:orignal:hybrids}.

\begin{GameBox}[label={MnR:game:redefine:hybrids}]{Re-Define the Hybrids \textnormal{$\Set{H^{(J, \msf{pat})}_k}_{k \in [K] \cup \Set{0}}$} }
{\bf Parameters.} Use the same $(J, \msf{pat})$ as defined \Cref{CPM-3ZK:MnR:game:subnormalized}. Use the unitaries defined in \Cref{re-define:unitaries}. We emphasize that this game inherits the ``sub-normalized'' nature of \Cref{CPM-3ZK:MnR:game:subnormalized} for the fixed $(J, \msf{pat})$ (this was already there in its original version defined in \Cref{sec:orignal:hybrids}), where all the measurements are replaced with projectors to the corresponding value contained in $\msf{pat}$.

\para{Hybrid $H^{(J, \msf{pat})}_k$ $(k \in [K] \cup \Set{0})$.} The hybrid behaves as follows for all $j \in [K]$:
\begin{enumerate}
	\item 
	{\bf When $\Sim$ makes the $\msf{sq}(j)$ Query:} Note that by definition, this is the first $\downarrow$-query that brings the global counter from $\ket{j-1}_{\reg{gc}}$ to $\ket{j}_{\reg{gc}}$. The hybrid answers this query by applying 
	$$D_{j}C_{j}B_{j} \ketbra{p_1, \ldots, p_j}_{\reg{p_1\ldots p_j}} A_{j} U_{gc}$$ to the overall state.

	\item
	{\bf When $\Sim$ makes a qeury between the $\msf{sq}(j-1)$ and $\msf{sq}(j)$ queries:} it behaves based on the query type and the value of the global counter value $i$:
	\begin{enumerate}
	\item \label[Case]{MnR:game:redefine:hybrids:case:a}
	{\bf For $\downarrow$-query and $i < k$:} This corresponds to a $\ddot{V}$-query bringing the global counter from $\ket{i}_{\reg{gc}}$ to $\ket{i+1}_{\reg{gc}}$. The hybrid answers it by applying $D_{i+1}\ddot{C}_{i+1} A_{i+1} U_{gc}$ to the overall state.

	\item
	{\bf For $\downarrow$-query and $i \ge k$:} This corresponds to a $\tilde{V}$-query bringing the global counter from $\ket{i}_{\reg{gc}}$ to $\ket{i+1}_{\reg{gc}}$. The hybrid answers it by applying $D_{i+1} C_{i+1} B_{i+1} A_{i+1} U_{gc}$ to the overall state.

	\item
	{\bf For $\uparrow$-query and $i \le k$:} This corresponds to a $\ddot{V}^\dagger$-query bringing the global counter from $\ket{i}_{\reg{gc}}$ to $\ket{i-1}_{\reg{gc}}$. The hybrid answers it by applying $U^\dagger_{gc} A^\dagger_i \ddot{C}^\dagger_i D^\dagger_i$ to the overall state.

	\item \label[Case]{MnR:game:redefine:hybrids:case:d}
	{\bf For $\uparrow$-query and $i > k$:} This corresponds to a ${V}^\dagger$-query bringing the global counter from $\ket{i}_{\reg{gc}}$ to $\ket{i-1}_{\reg{gc}}$. The hybrid answers it by applying $U^\dagger_{gc} A^\dagger_i {B}^\dagger_i {C}^\dagger_i {D}^\dagger_i$ to the overall state.
	\end{enumerate}
\end{enumerate}

\end{GameBox}

\begin{corollary}[of \Cref{counter-structure:lemma}]\label{MnR:game:redefine:hybrids:cor}
The hybrids $\Set{H^{(J, \msf{pat})}_k}_{k \in [K] \cup \Set{0}}$ defined in \Cref{MnR:game:redefine:hybrids} are equivalent to those defined in \Cref{sec:orignal:hybrids}.
\end{corollary}
\begin{proof}[Proof of \Cref{MnR:game:redefine:hybrids:cor}]
In the following, consider an (arbitrarily) fix $(J, \msf{pat})$ and $k \in [K] \cup \Set{0}$.

The main idea of this proof as follows. First, note that the original $H^{(J, \msf{pat})}_k$ (in \Cref{sec:orignal:hybrids}) makes use of the $\tilde{V}$ and $\ddot{V}$, which by definition determine what to do by checking the global counter and the local counter (see \Cref{CPM-3ZK:V:unitary,CPM-3ZK:V-dummy}). On the other hand, \Cref{counter-structure:lemma} provides a full characterization of the relation among the global counter, the local counters, and the $\reg{p_1 \ldots p_K}$ registers throughout the execution, which essentially allows the hybrid to determine what to do by checking the (classical) value contained in the global counter only.	This can be easily seen by comparing the original  $H^{(J, \msf{pat})}_k$ (in \Cref{sec:orignal:hybrids}) and the one defined in \Cref{MnR:game:redefine:hybrids} (together with the re-named unitaries in \Cref{re-define:unitaries}). In the following, we show as examples why they are equivalent for two representative types of queries. Other types of queries can be argued in the same manner.


As the first example, consider the case when $\Sim$ makes the $\msf{sq}(j)$ query for some $j$. By definition (and \Cref{rmk:sq:type}), this is a $\tilde{V}$ query bringing the global counter from $\ket{j-1}_{\reg{gc}}$ to $\ket{j}_{\reg{gc}}$. This query is handled as follows in the original  $H^{(J, \msf{pat})}_k$ (in \Cref{sec:orignal:hybrids}):
\begin{enumerate}
\item 
$U_{gc}$ is first applied to increase the global counter from $\ket{j-1}_{\reg{gc}}$ to $\ket{j}_{\reg{gc}}$. 
\item
Then, according to \Cref{CPM-3ZK:V:unitary}, $A_{j}$ is applied, and then it applies the projector $\ketbra{p_1, \ldots, p_j}_\reg{p_1 \ldots p_j}$. (Recall that we are currently in the ``sub-normalized'' game $H^{(J, \msf{pat})}_k$. Thus, the measurement on register $\reg{p_1 \ldots p_j}$ has been replaced with this projection.)
\item \label[Step]{MnR:game:redefine:hybrids:cor:example:1:step:3}
Next, the behavior depends on the value of the local register (in superposition). For a branch in the superposition where the local register value $\ell$ is equal to $j-1$ (i.e., the global counter value before this step), the operator $D_{j}C_{j}B_{j}$ (defined in \Cref{CPM-3ZK:V:unitary}) will be applied; for a branch in the superposition where the local register value $\ell \ne j-1$, the operator $C'_{j}$ (defined in \Cref{CPM-3ZK:V:unitary})  will be applied; 
\end{enumerate}
On the other hand, it follows from \Cref{counter-structure:lemma} that when the global counter is $\ket{j}_{\reg{gc}}$, the branches in the superposition with $\ket{\ell \ne j-1}_{\reg{lc}}$ all correspond to some values $(p_1, \ldots, p_{\ell-1}, p'_{\ell})$ in the $\reg{p_1 \ldots p_\ell}$ registers with some $p'_\ell \ne p_\ell$. Therefore, it follows that we do not need to consider the classification in \Cref{MnR:game:redefine:hybrids:cor:example:1:step:3}; instead, we can apply in \Cref{MnR:game:redefine:hybrids:cor:example:1:step:3}  the re-defined unitaries $D_jC_jB_j$ (see \Cref{re-define:unitaries}), which has {\em the identical effect} as the $C'_j$ (defined \Cref{CPM-3ZK:V:unitary}) on branches with $(p_1, \ldots, p_{\ell-1}, p'_{\ell})$ in the $\reg{p_1 \ldots p_\ell}$ registers! In summary, the above three steps can be unified as applying the operator $D_jC_jB_j \ketbra{p_1, \ldots, p_j}_{\reg{p_1 \ldots p_j}}A_jU_{gc}$ (as defined in \Cref{re-define:unitaries}) to the overall states, without worrying about the status of the local counter register. This is exactly what happens in \Cref{MnR:game:redefine:hybrids}.	


As another example, consider the \Cref{MnR:game:redefine:hybrids:case:a} in \Cref{MnR:game:redefine:hybrids}. In this case, by the original definition of $H^{(J, \msf{pat})}_k$ (in \Cref{sec:orignal:hybrids}), since $i < k$, this $\downarrow$ query will be answered by the $\ddot{V}$ (defined in \Cref{CPM-3ZK:V-dummy}). Again, this depends on the value of the local counter value $\ell$ (in superposition). In particular
\begin{enumerate}
\item
If $j = \ell$, the operator $D_{j+1}\ddot{C}_{j+1}A_{j+1}U_{gc}$ will be applied (with the unitaries defined in \Cref{CPM-3ZK:V:unitary,CPM-3ZK:V-dummy});

\item
If $j \ne \ell$, the operator ${C}'_{j+1}A_{j+1}U_{gc}$ will be applied (with the unitaries defined in \Cref{CPM-3ZK:V:unitary,CPM-3ZK:V-dummy}).
\end{enumerate}
Using a similar argument as we did in the first example, we claim that for the branches with $j \ne \ell$ in the superposition, the operator $\ddot{C}_{j+1}$ (defined in \Cref{re-define:unitaries}) has the identical effect as the ${C}'_{j+1}$ (defined \Cref{CPM-3ZK:V:unitary}). Therefore, the above two cases can be unified as applying the operator $\ddot{C}_{j+1}A_{j+1}U_{gc}$ (as defined in \Cref{re-define:unitaries}) to the overall states, without worrying about the status of the local counter register. This is exactly what happens in \Cref{MnR:game:redefine:hybrids}.	

\vspace{1em}
This completes the proof of \Cref{MnR:game:redefine:hybrids:cor}.

\end{proof}



==> sections/parallel_tightness_locc.tex <==
\subsection{Lifting the Knowledge Tightness Lower Bound to the LOCC Setting}
\label{sec:parallel_locc_lowerbound}

We show that the above knowledge tightness result can be extended to the LOCC setting in a relatively natural way. We will describe the modifications of the algorithm design for the BQP decider.

\begin{theorem}\label{thm:locc_parallel_zk}
Suppose $\Pi$ is a $O(\frac{\log n}{\log \log n})$ black-box zero knowledge protocol in the CPM model,  for $L$ with perfect completeness and negligible soundness error against any QPT adversaries, and suppose there exists a polynomial $k(n) \geq n$ such that parallel composition of $k$-copies of the protocol remains black-box zero-knowledge (against any QPT verifier) with simulator-query complexity $O(k^{1/m})$. Then $L \in \BQP$.
\end{theorem}

We now describe how we modify the above result into the CPM setting.

We combine the algorithm in \Cref{sec:parallel_pq_zk_bqp_algo} with the algorithm
\Cref{CPM:MnR:game}.\jiahui{add a new reference later for the full algorithm}:
\jiahui{Revise this part according to Algorithm 6.1}
\begin{itemize}
    \item The BQP decision algorithm $\A$ simulates the interaction between a $k$-session 
 CPM malicious verifier and simulator $S$.
    Note that $\qVk$'s next-message function is no longer the same as the classical function defined in \Cref{sec:quantum_parallel_verifier}. %bu\Cref{CPM:MnR:game}. 
    It does not take in any fixed classical randomness $r$. The next message unitary on the $i$-th message first copies the query $\MSG$ to $k$ registers and performs $V_i = V_{1,i} \otimes \cdots \otimes V_{k,i}$, where the $j$-th session's unitary $V_{i,j}$ is as follows:

    \begin{align*}
V_{j, i}:=
\begin{cases}
\ket{\msg^j_{i}}\bra{\msg^j_{i} } \otimes V_{i,\msg^j_{i}} \ket{x, \psi_j}
&\text{~if~} H_j(\MSG_{1},...,\MSG_{i})=1 \\
\mathbf{I}  %\text{ for abort-and-accept} 
&\text{~otherwise~}
\end{cases}.    
\end{align*}
$V_{i,j}$ acts on the registers $\ket{x,H,(\MSG_{1},...,\MSG_{i}), r_j, \psi_j}$ and $\ket{\msg^j_{i}}\bra{\msg^j_{i} } \otimes V_{i,\msg^j_{i}}$ acts on the register $\ket{\msg^j_i, x, \psi_j}$.

Here, $\msg^j$ is the transcript for the $j$-th session, $r_j$ is the classical fixed randomness and $\ket{\psi_j}$ is prover's internal state in the $j$-th session, respectively. $\msg^j_i$ is the $i$-th prover message in $j$-th session.
%\msg^j_{1},...,
    
    
    \item $\A$ initializes $k$ copies of an honest CPM verifier's initial state as the malicious $\qVk$'s initial state (the honest verifier does not have any auxiliary quantum state and can prepare any quantum state it needs from the $\ket{00\cdots 0}$ state). 


   

    \item $\A$ then applies the algorithm in \Cref{CPM:MnR:game_parallel} and similar to \Cref{sec:parallel_pq_zk_bqp_algo}, it only reprograms the oracle replies corresponding to the verifier messages and aborting information for the $\jstar$-th session, which is the guess made by $\A$ at the beginning of the algorithm.

    \item In the end of the algorithm in \Cref{CPM:MnR:game_parallel}, the output is a transcript $(\MSG_1,\cdots, \MSG_m)$ and state $\rho_{\msf{out}}$ over registers $\reg{1}, \cdots, \reg{k}$ where register $j$ corresponds to the output state of the $j$-th session. 

    Let $\MSG^{\jstar}$ denotes the full transcript of messages for the $\jstar$-th session in $(\MSG_1,\cdots, \MSG_m)$.
    $\A$ checks a quantum predicate $\pred(\rho_{\jstar}, \MSG^{\jstar}) = 1$. If 1, accept, else reject.
\end{itemize}


More, specifically, the measure-and-reprogram algorithm works as follows:

\jiahui{modify the notation of this part later}

\begin{GameBox}[label={CPM:MnR:game_parallel}]{$k$-Parallel Measure-and-Reprogram Game \textnormal{$\Sim^{\tilde{\Verifier}}[H, \vb{y}](x)$}}
 It works as follows
\begin{enumerate}
\item \label[Step]{CPM:MnR:game:step:1}
For each $i\in[K]$, uniformly pick $(\ell_i,b_i)\in ([2mq]\times \bits) \cup \{(\bot,\bot)\}$  conditioned on that there exists at most one $i\in [m]$ such that $\ell_i=\ell^*$  for all $\ell^*\in [2mq]$.

\item \label[Step]{CPM:MnR:game:step:2}
    Let $s$ denote the number of $j_i$'s in $\Set{j_i}_{i \in [K]}$ that are not $\bot$.  We re-label the indices $i$ for pairs $\Set{(j_i, b_i)}_{i \in [K]}$ so that $j_1 < j_2 < \ldots < j_s$ and $j_{s+1} = j_{s+2} =\ldots = j_K = \bot$.

\item
Run the oracle machine $\msf{SIM}(x)$ with oracle $\mcal{O}$, which is initialized to be a quantumly-accessible classical oracle that computes $H$, and when $\msf{SIM}(x)$ makes its $j$-th query, the oracle is simulated as follows:
\begin{enumerate}
      \item If $j=j_i$ for some $i\in[K]$, measure this query to obtain $\vb{p}_i=(p_{i,1}, \ldots,p_{i, z_i})$ where $z_i \in [K]$ is determined by the measurement outcome, and then behaves according to the value $b_i$ as follows:
        \begin{enumerate}
        \item 
        If $b_i=0$: First reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$, and then answer the $j_i$-th query using the reprogrammed oracle. 
        \item 
        If $b_i=1$: First answer the $j_i$-th query  using the oracle before the reprogramming, and then reprogram $\mcal{O} \leftarrow \reprogram(\mcal{O},\vb{p}_i,y_i)$. 
        \end{enumerate}
    \item Otherwise (i.e., $j \ne j_i$ $\forall i \in [s]$), answer the $j$-th query just using the oracle $\mcal{O}$ without any measurement or  reprogramming. 
    \end{enumerate}

\item
Let $(\vb{p}^* = (p^*_1, p^*_2), \rho_{\msf{out}})$ be the output of $\Sim^{\tilde{\Verifier}}$ at halt (as per \Cref{CPM:MnR:notation:item:2}).

\item
For all $i \in \Set{s+1, s+2, \ldots, K}$, set $\vb{p}_i = \vb{p}^*_i$ where $\vb{p}^*_i \coloneqq (p^*_1, \ldots, p^*_i)$. 

\item
{\bf Output:} The output of this game is defined as follows
\begin{itemize}
\item
If it holds for all $i \in [K]$ that $\vb{p}_i$ is a prefix of $\vb{p}_K$, then output $(\vb{p}_K, \rho_{\msf{out}})$;

\item
Otherwise, output $(\bot, \bot)$.
\end{itemize}
\end{enumerate}
\end{GameBox}


\paragraph{Completeness}
The completeness analysis follows from the same analysis as in \Cref{sec:parallel_pqzk_completeness} by replacing the accepting condition $\MSG^{\jstar} \in \acc[x, r_{\jstar}]$ with the condition $\pred(\rho_{\jstar}, \MSG^{\jstar}) = 1$.

\paragraph{Soundness}
The soundness follows from the same analysis as the stand-alone setting.
\jiahui{should follow directly but add more formalization later}

==> sections/pq_concurrent_zk.tex <==
\section{Round Complexity Lower Bound on Concurrent Zero-Knowledge}
In this section, we give a proof for a $\Omega(\log n/ \log \log n)$ round lower bound for  black-box concurrent zero-knowledge protocol in the post-quantum, classical computation and communication setting. We can then lift the result to the LOCC setting and the quantum communication setting via a relatively straightforward argument.

\subsection{Post-quantum Lower Bound for Classical Concurrent Zero-knowledge Protocols}

\begin{theorem}\label{thm:pq_concurrent_zk}
Let $n$ be the security parameter, and let $\Pi = (P, V)$ be a $m(n)$-round classical concurrent black-box zero-knowledge argument for a language $L$ with perfect completeness and negligible soundness against any QPT adversaries. If $m(n) \in o(\log n/ \log \log n)$, then $L \in \BQP$.
\end{theorem}

Our proof is a post-quantum adaptation of the proof provided in \cite{chung2012knowledge}. 
On a high level, the proof works by designing a modularized concurrent malicious verifier that invokes many instances of an underlying parallel zero-knowledge malicious verifier $\qVk$ we constructed in \cref{sec:quantum_parallel_verifier}, in a recursive fashion. By assigning a proper depth to the recursion in the above design, we can make sure that any simulator must make superpolynomial queries to finish the simulation. Otherwise, if there exists a simulator who can use polynomial queries, then there must an invocation of the parallel protocol where the simulator makes fewer than $o(k^{1/m})$ queries to convince the malicious parallel verifier in that invocation, contradicting the statement in \Cref{thm:pq_parallel_tightness}.


\subsection{Design and Schedule of the Malicious Concurrent Verifier  $\Vconc$}
\label{sec:concurrent_verifier_schedule}


In this section, we design the malicious concurrent verifier called $\Vconc$. 


Let $\Vconc$ be a concurrent verifier for protocol $\Pi$ that schedules some polynomial sessions of $\Pi$ into $m$ rounds of interaction. Let $\Vbase(\lambda, r)$ represent a base
incarnation of $\Vconc$, given security parameter $\lambda$ and random tape $r$. The behavior of $\Vbase$ is the same as the random-terminating parallel verifier we defined in \Cref{sec:quantum_parallel_verifier}.

On input base
$\lambda$ (a security parameter), $d$ (a nesting depth parameter), and $r$ (a random tape). Let $g$ be a function samples from a $2q$-wise independent function family, where $q$ is the total number of queries made by the simulator.
$\Vconc (\lambda, d)$ does the following:


\begin{mdframed}
 %Let $\Vconc$ be the verifier with the global view of the entire transcript.

 $\Vconc(\lambda, d)$ denotes the behavior of $\Vconc$ at depth $d$.

 Let $d_{max} = \log_m \lambda$
 





\begin{itemize}
    \item At depth $d < d_{max}$, $\Vconc(\lambda, d)$ generates a  random tape $r = g(\MSG)$ for $\Vbase$, where $\MSG$ is the current global transcript of prover messages \footnote{ $\Vconc(\lambda, d)$ has a global view on the transcript.} when $\Vconc$ is about to invoke $\Vbase$;

    \item $\Vconc(\lambda, d)$ invokes $\Vbase(\lambda,r)$ with the following modification:

    \begin{itemize}
        \item After every prover query $\msg$ in the local 
        interaction between the prover and $\Vbase(\lambda, r)$ \footnote{$\Vbase$ also has a global view on the transcript and uses the global transcript when querying the random-terminating oracle.}%and $\Vconc$ feeds the corresponding part of the prover message 
        , where the prover $P$ expects a verifier response from $\Vbase(\lambda, r)$,
        $\Vconc$ delays the response from $\Vbase$.
        
        \item $\Vbase$  instead recursively calls itself $\Vconc(\lambda,d+1)$(increased depth).\footnote{We call $\msg$
the initiating query for $\Vconc(\lambda,d+1)$}. 

\item  If $\Vconc(\lambda,d+1)$ returns 1\footnote{which means the $\Vbase$ invoked by $\Vconc(\lambda,d+1)$ returns 1} on the final some final prover query $\msg'$ \footnote{We call $\msg'$ the closing query for $\Vconc(\lambda, d+1)$}, then reply $\Vbase(\lambda, r)$ on the original query $\msg$; else abort and output 0.
    \end{itemize}

\item When $\Vconc(\lambda, d)$ receives the closing query for $\Vbase(\lambda, r)$, it outputs 1 if and only if $\Vbase(\lambda, r)$ outputs 1.

\item If $d = d_{max} = \log_m \lambda$,  we stop all recursive calls (i.e., $\Vconc(\lambda, d_{max}, r)$ answers each prover query without delay).
\end{itemize}

\end{mdframed}

 Given security parameter $\lambda$, function $g$, the final concurrent verifier $\Vconc(\lambda, g)$ starts by running $\Vconc(\lambda, g, d = 1)$.

 \subsection{Induction properties of $\Vconc$}

 In this section, we show that the above design of $\Vconc$ can "amplify" the number of queries needed by the simulator in the parallel composition of the protocol, to be the number of queries needed by a simulator in the concurrent schedule.
 
For the following lemma and \Cref{lem:concurrent_reduction_to_parallel}, since our proofs resemble the proof in \cite{chung2012knowledge}, we take it mostly verbatim from the original proof by making some necessary changes regarding the post-quantum setting (we do not omit the following proofs despite the resemblance, due to these necessary changes and the fact that the conference version of \cite{chung2012knowledge} does not in include the following proofs).
 
\begin{lemma}
\label{lem:induction_query_concurrent}
    Let $q(\lambda) \geq m$ be a parameter. If $S^{\Vconc}$ outputs an accepting view of
accept and during the execution of $S^{\Vconc}$ , all accepting incarnations $\Vbase$ respond 
to at least $q$ distinct initiating queries, then $S$ makes at least $q^{d_{max}}$ queries to $\Vconc$.
\end{lemma}

\begin{proof}
    We prove the lemma by an induction on the nesting depth
$d$, in a reversed order (i.e. from $d_{max}$ back to 1). In the induction, instead of bounding the number of queries that $S$ makes,
we consider the number of responses that $\Vconc$ actually responds to $S$, which
makes our induction cleaner. We say that a query $\MSG$ is inside $\Vconc(\lambda, g, d)$ if $\MSG$
is a query to some $\Vconc(\lambda,g,d′)$ (with $d′ \geq d$) that is recursively called from
$\Vconc(\lambda,g,d)$.

We use the following induction hypothesis.

If all accepting incarnations $\Vbase$ responds to at 
least $q$ distinct initiating queries, then for every accepting incarnation $\Vconc(\lambda, r)$
at depth $d$ (invoked by some $\Vconc(\lambda, g, d)$), then $\Vconc$ 
must respond to at least $q^{d_{max}-d +1}$
distinct initiating queries that is inside $\Vconc(\lambda, g, d)$.

\textbf{Base case: $d = d_{max}$.}  This follows naturally from the fact that all
accepting incarnations $\Vbase$ responds to at least $q$ distinct initiating queries. 

Now suppose the induction holds for depth $d + 1$, we show that the induction holds for depth $d$. Let $\Vbase(\lambda, r)$ be an invocation that outputs accept in its end at depth $d$, incoked by $\Vconc(\lambda,r, d)$. By our construction, $\Vbase(\lambda, r)$ responds to at least $q$ different initiating queries $\msg_1, \cdots, \msg_q$ since we invoke a child $\Vconc(\lambda, g, d+1)$ right after receiving the initiating query and each distinct query invokes distinct $\Vbase(\lambda, r_i)$ because the $r_i$ is computed from different transcripts.

The invocation of the child  $\Vconc(\lambda, r', d+1)$ will respond to at least $q^{d_{max}-d}$ queries
by the induction hypothesis. 
By definition, all these queries also belong to $\Vconc(\lambda, r, d)$. The queries inside different calls of $\Vconc(\lambda, g, d+1)$ must be distinct. Therefore, $\Vconc$ responds to at least $q^{d_{max}-d+1}$
distinct initiating queries inside $\Vconc(\lambda, g, d)$.
This completes the proof of the
induction.

Conclusively, if $S^{\Vconc}$ outputs an accepting view in the end, then it must contain
an accepting invocation of $\Vbase(\lambda, r)$ of $\Vconc(\lambda, g, 1)$. By the above induction,  must respond to at least $q^{d_{max}}$ distinct initiating queries during the interaction, which implies that $S$ must make at least $q^{d_{max}}$ queries to $\Vconc$.
\end{proof}

We will use \Cref{lem:induction_query_concurrent} in a contrapositive form stated as follows.

\begin{corollary}
\label{cor:concur_induction_contrapositive}
Let $q(n) \geq m$ be a parameter. If $S^{\Vconc}$ outputs an accepting view
and makes less than $q^{d_{max}}$ queries to $\Vconc$, then during the execution, there must exist an accepting invocation of $\Vconc$ that responds
to less than $q$ distinct initiating queries.    
\end{corollary}


\subsection{Reduction to Post-quantum Parallel Tightness}

Now using the above lemmas, we are ready to build a reduction that contradicts the knowledge tightness lower bound in \Cref{thm:pq_parallel_tightness}.

\begin{lemma}
\label{lem:concurrent_reduction_to_parallel}
Let $q(n) \geq m^{\omega(1)}$ be a parameter. Let $\Vconc$ be a concurrent verifier
for $\Pi$ that schedules in $m$ rounds. Let $\Vconc$ be the concurrent verifier constructed 
in \Cref{sec:concurrent_verifier_schedule} using $\Vbase$ as a base verifier. Let $x \notin L$ be an input. If for every
base
oracle QPT machine $\Sbase$ that makes at most $q$ queries to the oracle, $\Sbase$ can
only output an accepting view of $V$ with negligible probability, then for every $\Vbase$
oracle QPT machine $S$, $S^{\Vconc}$ can only output an accepting view of $\Vconc$ with negligible probability.
\end{lemma}

\begin{proof}
    Suppose for  that there exists an $x \notin L$ such that
$S^{\Vconc}(x)$ outputs an accepting view of $\Vconc$ with some noticeable probability $\epsilon$, we can then construct from $S$, an oracle QPT machine $\Sbase$ such that $\Sbase$ makes at most $q$ queries to $\Vbase$ and outputs an accepting view of  with noticeable
probability, contradicting to the premise of the lemma.

$S$ interacts with an external verifier $\Vbaseext$ and embeds the interaction into the interaction of $S$ and $\Vconc$. Let $T(\lambda)$ be a time bound on the simulator $S$. Now we construct $\Sbase$:

$\Sbase$ samples a random $i \gets [T]$ and simulates the interaction of $S$ and $\Vconc$ in his head. When it comes to the $i$-th invocation of $\Vbase$, we will embed $\Vbaseext$ here to play the role of the $i$-th invocation of $\Vbase$ (invoked by some $\Vconc(\lambda, g, d))$):
\begin{itemize}
    \item When $\Vbase$ is invoked, $\Vbase$ needs to send the first verifier message. $\Sbase$ 
uses the first message of $\Vbaseext$ to simulate $\Vbase$’s first message.


\item When $\Vbase$ needs to respond to a prover query $\msg$, $\Sbase$ forwards the query 
to $\Vbaseext$ and use its answer to simulate $\Vbase$.
Note that classically, $\Vbase$ may need to respond to the same prover query multiple base times with the same response.
%(e.g. when $S$ makes multiple closing queries to $\Vconc(\lambda, g, d+1)$)
But since the $\Sbase$ can also make repeated queries when interacting exteral $\Vbaseext$ so $\Sbase$ can directly forward. 
%would also expect such repeated queries
\jiahui{quantumly, we prevent repteated queries by the COUNT registers?}

\item The remaining case is when S makes a closing query to $\Vconc(\lambda, g, d)$. In this
case, $\Sbase$ does not forward the query out. Note that we assume (w.l.o.g.) that the decision of $\Vbase$ can be computed from a complete transcription,
so $\Sbase$ can compute whether $\Vconc(\lambda, g, d)$ accepts or not and continue the
simulation.

\item In the end, if $\Sbase$ needs to forward more than $q$ queries, then $\Sbase$ simply
aborts. If S finished the simulation of $S^{\Vconc}$ , then $\Sbase$ outputs an accepting view of $\Vbaseext$ if such a view exists.
\end{itemize}

%Hence, $\Sbase$ only forwards the query once, and simulate the extra ones with the same response without forwarding.

By construction, $\Sbase$ forward exactly one query for every initiating
queries responded by $\Vconc(\lambda, g, d)$. Also note that since $S$ runs in $T(n) \leq \poly(n)$ 
time, $S$ can makes at most
$T < d^{d_{max}} = q^{\log_m n} = n^{\omega(1)}$.


Recall that our design of $\Vbase$ follows the random termination $k$-session parallel verifier in \Cref{sec:quantum_parallel_verifier}. Here, we can set $k$ to be simply $\lambda$. Then we can let $q = \lambda^{1/m}/\log^2\lambda$ and when $m = o(\log \lambda/\log\log \lambda)$, we have $q = \lambda^{1/m}/\log^2\lambda \geq m^{\omega(1)}$.

By \Cref{lem:parallel_pq_soundness}, we can design a malicious prover $\mP$ that simulates the interaction between $\Sbase$ and $\Vbaseext$ with the algorithm in the proof of \Cref{lem:parallel_pq_soundness} to break the soundness of a \textbf{single-session(standalone)} zero knowledge protocol, with an honest external verifier $V^{\text{ext}}$.


By \Cref{cor:concur_induction_contrapositive}, there must exist an accepting invocation of $\Vbase$ that responds to at most $q$ queries.
Let us define the event "$\Sbase \text{~chooses a good invocation of~} S^{\Vconc}$" to mean that all following conditon is met:
\begin{itemize}
    \item $\Sbase$ chooses an invocation of $\Vbase$ in $S^{\Vconc}$ such that $\Vbase$ responds to $\leq q$ queries.

    %\item There exists a malicious prover $\mP$ that simulates $\Sbase^{\Vbaseext}$ using the algorithm in \Cref{lem:parallel_pq_soundness} and convinces a standalone $V^{\text{ext}}$ on the input instance $x \notin L$.
\end{itemize}
We also have:
\begin{align*}
    & \Pr[\mP \text{~outputs an accepting view by~} V^{\text{ext}}] \\
    & \geq \Pr[ \left(S^{\Vconc}\text{ outputs an accepting view } \right)\vee \left( \Sbase \text{~chooses a good invocation of~} S^{\Vconc}\right)] \\
    & \geq \epsilon/T
\end{align*}

The above lemma then follows from \Cref{cor:concur_induction_contrapositive} and \Cref{lem:parallel_pq_soundness}. $S^{\Vconc}$ will output an accepting view with only negligible probability because otherwise there exists a malicious prover $\mP$ that simulates $\Sbase^{\Vbaseext}$ using the algorithm in \Cref{lem:parallel_pq_soundness} and convinces a standalone $V^{\text{ext}}$ on the input instance $x \notin L$ with non-negligible probability. 


\end{proof}

\jiahui{add argument about correctness}



\input{sections/concurrent_locc_quantum}

==> sections/pq_parallel_tightness.tex <==
\section{Knowledge Tightness Lower Bound for Post-Quantum and Quantum Parallel Zero Knowledge}
\label{sec:quantum_parallel_tightness}

In this section, we show a lower bound on parallel-composition of black-box zero knowledge protocols in terms of \textbf{knowledge tightness}, in the post-quantum as well as QZK setting.
 That is, a black-box zero-knowledge protocol having round complexity $O(\frac{\log \lambda}{\log\log \lambda})$ that remains secure under parallel composition (of arbitrarily polynomially many sessions) requires the simulator to make over a specific number of queries, specified below:

\jiahui{change all $n$ to $\lambda$}
Let $\lambda$ be the security parameter and $L$ be a language.
\begin{theorem}\label{thm:pq_parallel_tightness}
Suppose $\Pi$ is a $O(\frac{\log \lambda}{\log \log \lambda})$ black-box classical zero knowledge protocol for $L$ with perfect completeness and negligible soundness error, and suppose there exists a polynomial $k(\lambda) \geq \lambda$ such that parallel composition of $k$-copies of the protocol remains black-box zero-knowledge (against any QPT verifier) with simulator-query complexity $O(k^{1/m}/\log^2 \lambda)$. Then $L \in \BQP$.
\end{theorem}

Our result is a post-quantum (resp. quantum) version of the result in \cite{chung2012knowledge}. 

\begin{comment}
    

\jiahui{Will remove the following section later}
\subsection{Quantum Malicious Verifier}

To design the algorithm,  we design a malicious QPT verifier $V*$ running a parallel composition of $k$ sessions.

To build up such a verifier step-by-step, we first consider a \emph{classical single-session honest} verifier $V$ as a next-message function $F(x; r, \MSG)$, where $x$ is the input instance, $r$ is a fixed random tape chosen at the beginning and $\MSG = (\msg_1, \cdots, \msg_i)$ is the transcript of the current execution of protocol, i.e. all the prover and verifier messages exchanged.
$F(x; r, \MSG)$ outputs the next verifier message $\msg_{i+1}$.


\jiahui{move the classical verifier to previous sections?}
\paragraph{Classical Single-Session Malicious Verifier with Random Termination}


We can consider such a verifier to be a next-message function with a random function(implemented with a hash function) $h \gets \mathcal{H}$,  $\Vh(x; r, \MSG)$ that does the following:
\begin{itemize}
    \item At each round $i < m:$ on query $\MSG = (\msg_1, \cdots, \msg_i)$ where $\msg_i$ is the message exchanged in the $i$-th round:
    \begin{gather*}
      \text{ if } h(\MSG) = 0, \text{ then output } \msg_{i+1} \gets F(x; r, \MSG). \\
     \text{ else, abort and accept.}
\end{gather*}

\item In the final round $m$, $\Vh$ first checks if  $h(\msg_1, \cdots, \msg_i) = 1$ for all $i \leq m$: if not, abort; if yes, outputs  accept/reject $\gets F(x; r, \MSG)$.
\end{itemize}




\jiahui{describe this $\Vh$ as one that records history}
Every time $\Vh$ queries $h(\MSG)$, it stores $\MSG$ as well as $h(\MSG)$, so that in the final round $m$, it doesn't have to query $h$ again on all transcript prefixes. 

\begin{remark}
In most works with randomly-terminating verifier $\Vh$, normally after aborting, $\Vh$ will output reject. Here we define $\Vh$ to output accept after aborting since later the completeness of parallel composition will not hold if for every session, $\Vh$ outputs  reject at every abort.
\end{remark}



%\subsection{ Quantum  Verifier with Random Termination}
\paragraph{(Inefficient) Quantum Single-Session Verifier with Random Termination}
For now, we consider such a quantum malicious verifier with random termination using \emph{real random} functions $\cH$. We will later modify the verifier to an efficient one in \Cref{sec:efficient_verifier}.  

$\mV$ is essentially the same function as the classical single-session malicious verifier with random termination described above $\Vh(x; r, \msg)$, except that $\mV$ can be queried in superposition (by a QPT simulator).

\jiahui{TODO: specify all the registers of $\mV$ and what to do with them}

Formally, we specify how $\mV$ works with its internal registers: Input register $\regX$: to store input instance $x$; Auxiliary information $\regaux=(\regR,\regH)$: to store randomness $r$ and function $H$; Working register $\regW = ( \regcount, \regM_1,...,\regM_k, \regB))$: $\regcount$ for storing a count of current round, $\regM_1,...,\regM_k$ for storing the messages from/to the prover and $\regB$ stores a single bit; additionally, there's a message register $\regM$. 

We will initialize the auxiliary state in $\regaux$ to be the following:

\begin{description}
\item $\ket{\psi_\epsilon}_{\regR,\regH}$ is a superposition of $(r,H)$ according to the distribution  $\{(r,H):r\gets \mathcal{R}, H\gets \mathcal{H}_\epsilon\}$ Formally,
\[
\ket{\psi_\epsilon}_{\regR,\regH}=\sum_{r\in \mathcal{R},H\in \func(\cM^{\leq k},\bits)}\sqrt{\frac{D(H)}{|\mathcal{R}|}}\ket{r,H}_{\regR,\regH}
\]
where $D$ is the density function corresponding to $\mathcal{H}_{\epsilon}$.
Here, $H$ is represented as a concatenation of function values $H(\MSG)$ for all $\MSG \in \cM^{\leq k}$. 
We denote by $\regH_{\MSG}$ the sub-register of $\regH$ that stores $H(\MSG)$.
\end{description}


\begin{remark}
In the proof for the tightness lower bound of parallel ZK and round lower bound for concurrent ZK, we can in fact consider an equivalent verifier with no auxiliary state $\regaux$, but it samples $H \gets \cH, r \gets \cR$ at the beginning of the protocol and can be queried in superposition as a black box by the simulator. However, for the convenience of later sections, here we consider such a verifier with an auxiliary state that is a superposition of the possible randomness and aborting functions used.
\end{remark}

\begin{enumerate}
\item $V^*$ takes inputs a statement $x$  and a quantum auxiliary input $\ket {\psi_\epsilon}$: $\regX$ is initialized to be $\ket{x}_{\regX}$ where $x$ is the statement to be proven, $\regaux$ is initialized to be $\ket{\psi_\epsilon}_{\regR,\regH}$,
%\takashi{This may be inconsistent to our definition of the model as we assume that all other registers are initialized to $0$?
%Probably, we can initialize this to $0$ if we swap the order of "reads" and "increments".
%}
and all other registers are initialized to be $0$.
    \item 
    \emph{Verifier $V^*$ on round $i < m$}: Upon receiving the $i$-th message from $P$ for $i< m$ in $\regM$, swap $\regM$ and  $\regM_i$ and increment the value in $\regcount$\footnote{More precisely, this maps $\ket i$ to $\ket {(i + 1) \mod s}$ where $s$ is some superpolynomial. }.  
    %\qipeng{should we also mention $\regcount$ as its internal register}.\takashi{Yes, added. Another possible choice might be to make it implicit, but that may be confusing.}
    We note that $V^*$ can know $i$ since it keeps track of which round it is playing by the value in $\regcount$.  
    Let $(\msg_1,...,\msg_i)$ be the messages sent from $P$ so far.
    Then do the following in superposition where 
    $(\msg_1,...,\msg_i)$, 
    $r$, $H$ and $m$ are values in registers 
    $(\regM_1,...,\regM_i)$,  
    $\regR$, $\regH$ and $\regM$: 
    \begin{itemize}
        \item If $H(\msg_1,...,\msg_i)=0$, then do nothing.
        \item If $H(\msg_1,...,\msg_i)=1$, then add  $F[x,r](\msg_1,...,\msg_i)$ to the message register $m$.
    \end{itemize}
    
    It then measures the register $\regM$ and sends the result to the prover $P$. \xiao{It's unclear what happens here. Do you mean to collapse the $\regM$ register such that the verifier has to send out a classical message? Or is this again happens in one branch of the superposition?} 
    
\vspace{1em}
    
    \emph{Unitary $U^*$ on $\regcount < m - 1$}: It acts on registers $\regcount$ (whose value is less than $m - 1$), $\regX, (\regM_1,...,\regM_k)$,
    $\regR$, $\regH$ and $\regM$: 
        \begin{itemize}
            \item It reads the value $j$ in $\regcount$ and increments it to $i:=j+1$. It swaps $\regM$ and $\regM_{i}$ (in superposition).  %\qipeng{I realize another problem, we need to change all $i$ to $i+1$ for the remaining bullet points. Use $i = j + 1$ would solve this problem. Not sure which one is more helpful for readers. }
            %\takashi{I modified so.}
            
            
            %\item It reads and increments the value $i$ in $\regcount$; 
            %\item It swaps $\regM$ and $\regM_i$ (in superposition); 
            
            \item Let $x, (\msg_1, \cdots, \msg_i), r, H$ and $m$ be the values in registers $\regX, (\regM_1, \cdots, \regM_i), \regR, \regH$ and $\regM$. \xiao{These registers could contain superposition of messages. Are you performing this computation in super-position?} Let $F^*[x, r, H]$ be the following function: on input $(\msg_1, \cdots, \msg_i) \in \cM^{\leq m - 1}$, 
\begin{align*}
F^*[x,r,H](\msg_1,...,\msg_i):=
\begin{cases}
F[x,r](\msg_1,...,\msg_{i}) &\text{~if~} H(\msg_1,...,\msg_{i})=1 \\
0 &\text{~otherwise~}
\end{cases}.    
\end{align*}

It then applies the function in superposition. \xiao{Clarify the meaning of ``$+$'' below. Bit-wise XOR? Or group operation in some (undefined) group?}
\begin{align*}
    \ket {x, \msg_1, \cdots, m_i, r, H, m}  \to \ket {x, \msg_1, \cdots, \msg_i, r, H, m + F^*[x, r, H](\msg_1, \cdots, m_i)}. 
\end{align*}
\end{itemize}
        
    
    
    \item 
    \emph{Verifier $V^*$ on round $m$}: 
    %\qipeng{we have round $<k-1$ and round $k$, one of them should be consistent with others.} 
    %\takashi{I modified the other one to $<k$.}
    Upon receiving the $m$-th message from $P$ in $\regM$,  swap $\regM$ and $\regM_k$  and increment the value in $\regcount$. 
    Then flip the bit in $\regB$ if 
    $(\msg_1, \cdots, \msg_k) \in \acc[x,r]$ and 
    $H(\msg_1,...,\msg_i)=1$ for all $i\in[k]$
    where 
    $(\msg_1,...,\msg_k)$, 
    $r$, and $H$ are values in registers 
    $(\regM_1,...,\regM_k)$,  
    $\regR$, and $\regH$.

\vspace{1em}
    
\emph{Unitary $U^*$ on $\regcount= k - 1$}: It acts on registers $\regcount$ (whose value is exactly equal to $k-1$), $\regX, (\regM_1,...,\regM_k)$,
    $\regR$, $\regH$ and $\regB$: 
        \begin{itemize}
            \item  It reads the value $j = k-1$ in $\regcount$ and sets it to $0$. It swaps $\regM$ and $\regM_{k}$ (in superposition). 
            %\item \revise{It reads the value $k-1$ in $\regcount$, lets $i = j + 1 = k$. It swaps $\regM$ and $\regM_i$ (in superposition). Then it increments the value in $\regcount$. }
            \item Let $x, (m_1, \cdots, m_k), r, H$ and $b$ be the values in registers $\regX, (\regM_1, \cdots, \regM_k), \regR, \regH$ and $\regB$. Let $F^*[x, r, H]$ be the following function: on input $(m_1, \cdots, m_k) \in \cM^k$, 
\begin{align*}
F^*[x,r,H](\msg_1,...,\msg_k):=
\begin{cases}
1 & \substack{\text{~if~} H(\msg_1,...,\msg_{i})=1,\,\forall i \in [k] \\ \text{~and~}  F[x, r](m_1, \cdots, m_k) = \top} \\
0 &\text{~otherwise~} 
\end{cases}.    
\end{align*}
            
            
            
It applies the function in superposition. 
\begin{align*}
    \ket {x, m_1, \cdots, m_k, r, H, b}  \to \ket {x, m_1, \cdots, m_k, r, H, b + F^*[x, r, H](m_1, \cdots, m_k)}. 
\end{align*}
\end{itemize}
\end{enumerate}

\end{comment}


\subsection{Quantum Malicious Verifier with Random Termination of $k$ Parallel Sessions}
\label{sec:quantum_parallel_verifier}

\jiahui{Ca replace $\{H_j\}$ with  a single oracle $H$ that has $k$-bit output}

\paragraph{Notations} We will slightly deviate from the notations used in the previous sections on stand-alone (single-session) setting.

We denote $m$ as the number of rounds in the protocol (more specifically, number of prover messages) and $k$ as the number of \textbf{sessions} opened by the verifier.

Since there will be messages in different sessions and rounds, we denote $\MSG$ as the entire prover message containing all sessions and up to the current round; $\MSG_i$ as the message across all $k$ sessions, but only for the $i$-th round; $\MSG^j$ as the message for only the $j$-th session, but containing all prover messages up to the current round.

%\paragraph{(Inefficient) Quantum Malicious Verifier with Random Termination of $k$ Parallel Sessions}


\paragraph{Design of the $k$-parallel Malicious Verifier with Random Termination}
A quantum malicious verifier $\qVk$ with random termination running $k$ parallel sessions can be described as follows.

%Each session $j \in [k]$ uses independent randomness $r_j \gets \cR$ and independent functions for aborting sampled from the same family $H_j \gets \cH: \cM^{\leq m} \to \{0,1\}$ such that each of them outputs 0 with probability $1-p$.

%\jiahui{need to set aborting prob to be larger than $1-\frac{1}{q}$ because changing the zero oracle has a lot of loss }.
%where $q$ is the number of queries made by the simulator.



 $\qVk$ on instance $x$, fixed random tape $r_1, \cdots, r_k \gets \cR$, and function
 $H: \cM^{\leq mk} \to \bits^k, H \in \cH^k_\epsilon$.
 $\cH^k_\epsilon$ is a family of hash functions such that on any input $\MSG \in  \cM^{\leq mk}$, for all $i \in [k]$ $H_i(\MSG) = 0$ with probability $1-\epsilon$ and $H_i(\MSG) = 1$ with probability $\epsilon$, where $H_i(\MSG)$ is the $i$-th bit on the output. %defined in \Cref{def:H-epsilon}
 
Equivalently, we can  think of $H$ on input $\MSG = (\MSG_1, \cdots, \MSG_{k})$ as $H_1(\MSG), \cdots, H_k(\MSG)$ where each $H_i$ is a function that on any input $\MSG \in  \cM^{\leq mk}$, $H_i(\MSG) = 0$ with probability $1-\epsilon$ and $H_i(\MSG) = 1$ with probability $\epsilon$.
    
   
     On each (quantum) query  $\ket{\MSG_1} \ket{\MSG_2} \cdots \ket{\MSG_k}$,  $\qVk$ does the following:
\begin{itemize}


\item Let $F^*[x, r, H, \ket{\MSG}]$ be the following function: 
\jiahui{same as \cite{CCLY21-impossibility} page 19 item 2} 
$F^*[x, r, H, \MSG] = (F_1^*[x,r,H, \MSG], \cdots, F_k^*[x,r,H, \MSG])$ where $F_j^*[x,r,H, \MSG]$ denotes the  verifier message in the $j$-th session in the entire verifier message. 
\begin{align*}
F_j^*[x,r,H](\MSG_{1},...,\MSG_{i}):=
\begin{cases}
F[x,r_j](\msg_{j,1},...,\msg_{j,i}) &\text{~if~} H_j(\MSG_{1},...,\MSG_{i})=1 \\
1 %\text{ for abort-and-accept} 
&\text{~otherwise~}
\end{cases}.    
\end{align*}
where $\MSG^j = (\msg_{j,1}, \cdots, \msg_{j,i})$ is the transcript in the $j$-th session up to the $i$-th round.  $F[x,r_j]$ is the honest verifier next-message function for a single session (when taking input $r_j$, corresponds to the $j$-th session).

When querying $\qVk$ in superposition, it is the same as applying the next-message function $F^*[x, r, \ket{\MSG}]$ in superposition:
$$
\ket{x, \MSG, r, H, 0} \rightarrow \ket{x, \MSG, r, H, F^*[x, r, \MSG]}
$$

\item When it comes to final round $i = m$, 
\begin{itemize}
    \item Let $F^*[x, r, H, \MSG] =  (F_1^*[x, r_1, H, \MSG], \cdots, F_k^*[x, r,_k H, \MSG])$, where $F_j^*[x, r, H, \MSG]$ is the verifier reply for the $j$-th  session in $F^*[x, r, H, \MSG]$,   be the following function:
    \begin{align*}
F_j^*[x,r,H](\MSG_{1},...,\MSG_{m}):=
\begin{cases}
1 & \substack{\text{~if~}  H_j(\MSG_{1},...,\MSG_{m})=1,\,\forall i \in [m] \\ \text{~and~}  F[x, r_j](\msg_{j,1},...,\msg_{j,m}) = 1}  \\ 
1 &
\text{~or~} \exists i\in [m], H_j(\MSG_{1},...,\MSG_{i})=0  \\ %\top?
0 &\text{~otherwise~} 
\end{cases}.    
\end{align*}

  \item measure the output registers of each $\qVj(x, r_j, H_j, \ket{\MSG_j})$. Accept if and only if
  all sessions accept.
  
\end{itemize}

\end{itemize}

\iffalse

\jiahui{The following is old: comment out later}


\item  For each  $j \in [k]$,  run the single-session verifier  $\qVj(x, r_j, H_j, \ket{\MSG_j})$ as a subroutine:

\item Let $F^*[x, r, H_j, \ket{\MSG}]$ be the following function: 
\jiahui{same as \cite{CCLY21-impossibility} page 19 item 2} 
\begin{align*}
F^*[x,r_j,H_j](\msg_{j,1},...,\msg_{j,i}):=
\begin{cases}
F[x,r_j](\msg_{j,1},...,\msg_{j,i}) &\text{~if~} H_j(\msg_{j,1},...,\msg_{j,i})=1 \\
0 &\text{~otherwise~}
\end{cases}.    
\end{align*}




\begin{remark}
Each query $\ket{\MSG_1} \cdots \ket{\MSG_k}$ can be seen as a product state $\otimes_{j = 1}^k \ket{\MSG_j}$, where $\ket{\MSG_j} = \ket{\msg_{j,1}, \msg_{j,2}, \cdots, \msg_{j,i}}$ and $\msg_{j,i}$ is the $i$-th message exchanged in the execution of session $j$.   
%Since the behavior of simulator 
\end{remark}
\fi


\begin{remark}
We use a $k$-bit output random oracle $H^k:  \cM^{\leq m} \to \{0,1\}^k$ on each query of the entire transcript that outputs $k$ bits.
It is equivalent to using
a different binary-output random oracle $H_1, \cdots, H_K$ for each session $i \in [k]$.

%since in the measure-and-regrogram technique,


%we cannot make too many queries to the random oracle we need to measure and regrogram. This change also won't influence our proof: (1) each session's randomness only needs to be consistent with its own and independent of other sessions. %Each session's aborting decision is made independently. (2) Intuitively, a malicious verifier using different random functions for different sessions to abort is at least as powerful as a verifier using one function to abort: we can see from the simulator analysis  in the parallel composition setting in \cite{goldreich2002concurrent-timing} that if the verifier's aborting behaviors vary from session to session, it will be more difficult for the simulator to rewind successfully.

%if a verifier using one random oracle to terminate can give us such a lower bound, a verifier using 
\end{remark}

%\jiahui{Do we actually need to argue the following for analysis purpose?  TODO}
%\jiahui{argue why if simulator uses entangled queries as a strategy, there will always be a strategy using unentangled queries that achieve the same success probability. }

%Each state (entangled with the environment) can be seen as a mixed state; then a convex combination of pure states, one of which must perform as good as the whole mixted state in outputting any transcript; then the simulator can simply use this pure state to query instead.

\subsection{$\BQP$-language Decision Algorithm}
We describe the idea of the BQP decision algorithm on a high-level:

   $\A$ performs the following: $\A$ simulates the interaction between simulator $S$ and $\Vzero$.
    Suppose $S$ makes $q$ queries, then $\Vzero$ will make $mq$ queries to the oracle $H_0$ to answer the queries in session $\jstar$. 

    Among these $mq$ queries made to oracle $H_0$, $\A$ performs the following "measure-and-reprogram"  algorthms for queries in the set $T$. The major difference from the stand

    
    These queries are reprogrammed to be not aborting and answered with the next verifier message computed from the honest verifier function $F(x,r_{\jstar}, \cdot)$. 

\label{sec:parallel_pq_zk_bqp_algo}
The $\BQP$ Algorithm $\A$ for language $L$ is as follows: 

\begin{itemize}
   % \item $D$ is a quantum polynomial-time simulator. 
    
    \item $\A$ simulates the interaction between a regular quantum polynomial-time simulator $S$ making at most $q = O(k^{1/m}/m)$ queries and $\Vzero(x,r_1, \cdots, r_k, \{h_j\}_{j \in [k], j \neq j^*} \cdot)$. To initialize such a verifier, $\A$ does the following:
    \begin{itemize}
        \item $\A$ samples a session index $j^* \in [k]$. 
        %chooses a random session $j^* \in [k]$.
        %takes input:

        %\jiahui{replace with h that outputs 0 all the tim at position $j^*$ and random elsewhere}
        \item $H_{0}: \cM^{\leq m} \to \{0,1\}$ is a function that outputs $0$ all the time; samples $H_j \in \cH_\epsilon$ for $j \neq \jstar$ are oracles that output 0 with probability $1-\epsilon$
        %at the $j^*$-th output bit and for the output at indices $j \neq \jstar$, $H_0^j(m) = 0$ with probability $1-\epsilon$. 
        
        %Function $H_0^{\jstar}$ is used to determine aborting/non-aborting for
        
        \item $\A$ samples randomness $\vr = (r_i, \cdots, r_k)$, $r_j \gets \cR$ for each $j \in [k]$.
        
        % \item 
         
    %     \item $\A$ simulates the verifier $\qVk$ for each of the sessions $j$  where $j \neq j^*$: using function $H_{j}\gets \cH_{\epsilon}$ and the single-session honest verifier function $F(x, r_j, \cdot)$; 
    
         %the $j$-th bit %
            %run $F^*(x, r_j, h_j, \cdot)$ by itself. 
         %takes input
         
         %\jiahui{Here we take all $h_j$ for  $j \neq j^*$ to have succinct description directly, instead of first making them random functions and then move to efficient description; does this work? We will specify later that an inefficient V can be made efficient by replacing all the random functions with $2q$-wise independent functions.}
         
    \end{itemize}
     
    
   
    %on input instance $x$.

   % \item Run $S$ where the oracle $F^*[x, r, H]$ is simulated by additional oracles $\cO$ and $F$ where $\cO$ and $F$ play the roles of $H$ and $F[x, r]$, respectively.






 

\item $\A$ then runs algorithm $\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecone]$ . $\vecone = (1, \cdots, 1)$ is a length-$m$ string where all entries are 1's. 

%    The algorithm is similar to  \Cref{lem:measure_and_reprogram_ordered} except that it only performs "measure-and-reprogram" for the oracle queries in session $\jstar$ and simulates the verifier $\qVk$ for each of the sessions $j$  where $j \neq j^*$: using function $H_{j}\gets \cH_{\epsilon}$ and the single-session honest verifier function $F(x, r_j, \cdot)$
    
    We elaborate $\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecbeta]$'s  behavior as below.

 

    
\end{itemize}

    \jiahui{revise the language and details later}


    
\begin{mdframed}
[frametitle = {Algorithm $\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecbeta]$}]

\begin{enumerate}
     \item  Simulate the $\qVk$ oracle for simulator $S$: as discussed in \Cref{sec:quantum_parallel_verifier}, we can view the $\qVk$ as the passing $S$'s query $\MSG$ to the quantum-accessible oracle function $F^*[x, r, H, \MSG] $ defined in \Cref{sec:quantum_parallel_verifier}, which can again be viewed as $k$ separate oracles $ (F_1^*[x, r_1, H_1, \MSG], \cdots, F_{\jstar}^*[x, r_{\jstar}, H_{\jstar}, \MSG], F_k^*[x, r,_k H_k, \MSG])$.
     
     \item Among them, the
     $F_{\jstar}^*[x, r_{\jstar}, H_0]$ oracle machine is simulated with oracle $H_0$ and the honest verifier's single-session next-message function $F[x, r_{\jstar}, \cdot]$. The oracles $H_0$ %$\cO$ (for simulating ) 
     and  $F_{\jstar}^*[x, r_{\jstar}, \cdot]$
     are initialized to be an
oracles that just return 0. 
The rest of the oracles $F_j^*[x, r_j, H_j, \MSG],  j \neq \jstar$
 are simulated as they are defined in \Cref{sec:quantum_parallel_verifier} using oracles $H_j$ respectively.

For the rest of the description, we can assume $S$ is making queries to all oracles $\H_0, \{H_j\}_{j \in [k], j \neq \jstar}$ and as well as $F^*[x, \vr, H]$. 



   
    
    \item $\A$ randomly chooses a set of queries and  uniform random bits $T \times \{b_\ell\} \subseteq \{[q] \cup \{\bot\}\}^m \times  \{0,1\}^m$ with $|T| = m$, and satisfying $\ell_i \neq \ell_j$ for all $i \neq j$ unless $\ell_i = \ell_j = \bot$.

 
    \item When $S^{\qVk}$ makes its $\ell$-th query, the oracle $F^*[x, \vr, H]$ is simulated as follows. 
    %(\ket{\msg_1}, \cdots, \ket{\msg_m})
    If we have $\ell \in T$:
    \begin{itemize}
        \item $\A$ measures $\qVk$'s  query register to oracle $F^*_{\jstar}[x, \vr, H_0, \cdot]$ to obtain $\MSG_{\ell}$. 
        %Note that we only measure the part of the messag for session $\jstar$; 
        Note that the following reprogramming is also only for oracle $F^*_{\jstar}[x, \vr, H_0, \cdot]$ (when $S^{\qVk}$ is making a query to the oracle $F^*_{\jstar}[x, r_{\jstar}, \cdot]$, it will first go through oracle $H_0$ as well).
        \footnote{The above description has the view that only the queries made to the oracle $F_j^*[x, r_{\jstar}, H_{\jstar},\cdot], \j \neq \jstar$ used in the other sessions are not reprogrammed and the oracles $\{H_j\}_{j\neq \jstar}$ are not reprogrammed. Since essentially $S$ makes a query of the format $\MSG_\ell$ to the $k$-session verifier next-message oracle $F^*[x, \vr, H, \cdot]$, when $\Aord$ measures  the query register to the entire verifier oracle $F^*_{\jstar}[c, r_{\jstar}, H_0, \cdot]$, it implicitly collapses the input register to other oracles $F^*_{j}[c, r_{j}, H_j, \cdot], j\neq \jstar$. But again, we can use the alternative view that we measure the $\ell$-th query to the entire $k$-session verifier oracle $F^*[x, \vr, H, \cdot]$ and a $k$-bit output oracle $H$ such that $H:\cM^{mk} \tp \{0,1\}^k$ string that is a concatenetion of the output of $H_1, \cdots, H_{\jstar} = H_0, \cdots, H_k$, and only reprogram the part of the output corresponding to the $\jstar$-th session. }
        
        
           \item If $b_\ell = 0$, reprogram $H_0(\MSG_\ell)$ to output 1 \emph{before} answering the $\ell$-th query.
        
        %$F^*_{\jstar}[x, \vr, H_0(\MSG_\ell)]$ to output the single session honest verifier function, on input $x, r_j, \MSG^{\jstar}$: $F[x, \r_{\jstar}, \MSG^{\jstar}_\ell]$ 
        
        
        %where the input $\MSG^{\jstar}$ %\jiahui{only reprogram for session $\jstar$; other sessions can still abort independently!}
        
        \item If $b = 1$, 
        %$F^*_{\jstar}[x, \vr, H_0(\MSG_\ell)]$ to output the single session honest verifier function, on input $x, r_j, \MSG^{\jstar}$: 
        %$F[x, \r_{\jstar}, \MSG^{\jstar}_\ell]$ 
        reprogram $H_0(\MSG_\ell) \to 1$
        \emph{after} answering the $\ell$-th query.
        %If $b_\ell = 0$, reprograms $F^*_{\jstar}[x, \vr, H_0(\MSG_\ell)]$ to output the single session honest verifier function, on input $x, r_j, \MSG^{\jstar}$: $F[x, \r_{\jstar}, \MSG^{\jstar}_\ell]$ \emph{before} answering the $\ell$-th query where the input $\MSG^{\jstar}$ is the part of the transcript $\MSG_\ell$ that corresponds to the $\jstar$-th session in the $\ell$-th query and has the format $\MSG^{\jstar} = (\MSG^{\jstar}_1, \cdots, \MSG^{\jstar}_{i_\ell}), i_\ell \leq m$; %\jiahui{only reprogram for session $\jstar$; other sessions can still abort independently!}
        
       % \item If $b = 1$, $F^*_{\jstar}[x, \vr, H_0(\MSG_\ell)]$ to output the single session honest verifier function, on input $x, r_j, \MSG^{\jstar}$: $F[x, \r_{\jstar}, \MSG^{\jstar}_\ell]$ \emph{after} answering the $\ell$-th query.

       
    \end{itemize}

    \item If the $\ell$-th query satisfies $\ell \notin T$, do nothing and answer the query using the current oracle.
    
    %\item $\A$ runs an honest classical single-session verifier next-message function $F(x,r_{\jstar}, \cdot)$ with the same random tape $r_{\jstar}$ used by $\Vzero(x,r_1, \cdots, r_k, \cdot)$ in session $j$ and the same input instance $x$.
    %initializes
    \item In the end, $S$ outputs a transcript 
    $(\MSG_{1}', \cdots \MSG_{m}')$.
    
     \item Accordingly, $\A$ outputs a classical transcript $(\MSG_{1}, \cdots \MSG_{m})$, where:
     \begin{itemize}

   % \item for all $j \neq \jstar$: the transcript $(\MSG_{j\neq \jstar, \ell_1}, \cdots, \MSG_{j\neq \jstar, \ell_m}) = (\MSG_{j\neq \jstar, \ell_1}', \cdots, \MSG_{j\neq \jstar, \ell_m}')$ comes from the output of $S$; 
     
 \item %For the $\jstar$'s session: 
 for all $\ell_i \neq \bot$
 the transcript $\MSG_{i}$ is the message $\MSG_{\ell_i}$ obtained from measuring the $\ell_i$-th query in the above procedure;

 \item for all $\ell_i = \bot, i \in [m]$, the partial transcript $\MSG_{\ell_i} = \MSG_{i}' $ comes from the final output of $S$;

 
     \end{itemize}
    
\end{enumerate}
\end{mdframed}



%\jiahui{todo: $B$ uses $\A$'s output to decide $L$}
Then there exists a $\BQP$-language Decision algorithm $\A$ which will use $\Aord[x, \vr, \{H_j\}_{j \neq \jstar}][H_0, \vecone]$ to decide if $x \in L$:
\begin{itemize}
%  \item $\Bs$ takes $x$ as input; it chooses random $\jstar \gets [k]$,  $\vr \gets \cR^k$, $H_j \gets \cH$, for $j \in [k], j \neq \jstar$.
    
    \item $\A$ runs $\Aord[x, \vr, \{H_j\}_{j \neq \jstar}][H_0, \vecone]$ which outputs a %\emph{single-session} 
    transcript $\MSG = (\MSG_{1}, \cdots \MSG_{m})$. %and a session index $\jstar$.

    %\forall i \in [m]
    %$\MSG_{\jstar} = (\MSG_{\jstar,\ell_1}, \cdots \MSG_{\jstar,\ell_m})$
    
    \item Let $\MSG^{\jstar} = (\MSG_{1, \jstar}, \cdots \MSG_{m, \jstar})$ be the full transcript of the messages in the $\jstar$-th session.
    If the honest verifier function $F(x, r_{\jstar}, \MSG^{\jstar})$ for session $\jstar$ outputs accept, then accept; else reject.
    %\in [k]
\end{itemize}

\jiahui{maybe for simplicity and clarity of writing: take all the $H_j$ for $j \neq \jstar$ to be part of $r_i$?  }


\jiahui{check the following}

\paragraph{Observation} The number of queries made by $\A$ to $H$ o simulate the behavior of $F^*(x, r_{\jstar}, H_\jstar, \cdot)$ is $2mq$.
We need $mq$ queries first to the $H_\jstar$ oracle since one needs to check if all $H_\jstar(\MSG_{\jstar,1}), \cdots , H_\jstar(\MSG_{\jstar, \ell})$ output, supposing when replying to the $\ell$-th prover message. Morevoer, 
we need  $2mq$ instead of $mq$ queries to $H$ since we need to query $U^\dagger_H$ later uncompute the register that records abort/non-abort queries to avoid interference. The query reply $H(\MSG_{\jstar})$ is copied to another register as in the common uncomputing operations. 

%he actual unitaries applied here are $U^\dagger_H U_F U_H$.
%no uncomputing needed?
%


%For each query $\MSG = (\msg_1, \cdots, \msg_i)$,  $D$ needs to query $H(\msg_1), H(\msg_1, \msg_1), \cdots, H(\msg_1, \cdots, \msg_i)$ and makes sure none of them outputs 0 to continue. 

%\jiahui{don't really need this $m$ overhead; can just let $V*$ record history}


\begin{itemize}
   \item Measure and reprogram loss in completeness:
$ 1/(4q+1)^{2m} \geq 1/(4k^{1/m})^{2m}$ by taking $q = k^{1/m}-1$ for example.%  %= \frac{1}{k^2 \cdot n^{4/\log \log n}}$.

\item Changing to all zero oracle $H_0$ loss:
$ 8 \cdot (2 \cdot k^{1/m} )^2  \cdot p $, where $p$ is non-aborting probability.
\end{itemize}

Here are some notations:
\begin{enumerate}

\item We slightly abuse the notation 
$\Aord_{\jstar}[x, \vr, \{H_j\}_{j \neq\jstar}][H_0, \vecone]$ as 
%the transcript of the $\jstar$-th session in
the  output of the
    algorithm $\Aord[x, \vr, \{H_j\}_{j \neq\jstar}][H_0, \vecone]$ described above,  which outputs a transcript $(\MSG_1, \cdots, \MSG_k)$.
    \item We denote $\Aord_{\jstar}[x, \vr, \{H_j\}_{j \neq\jstar}][H_0, \vecone]$ as $\jstar$-th session's transcript in the the 
    output
    algorithm. %which outputs the $\jstar$-th session's transcript. %for algorithm $\Aord[x, \vr, \{h_j\}_{j \neq\jstar}][H_0, \vecone]$.
    \item We denote $\acc^{*}_k[x,\vr, H]$ as the set of all accepting transcripts of all $k$ sessions by a random-aborting $V^*_k$; $\acc^*[x,\vr]$ as the set of accepting transcripts of a single session. %$j$-th session for $j \in [k]$.
    
   
    \item We denote 
    $\acc_k[x,\vr]$ as a "non-trivially" accepting transcript of all $k$ sessions: that is, there exists at least one session that does not abort and is an accepting transcript. Similarly, 
    $\acc[x,\vr]$ as the set of non-trivially accepting transcripts of a single session. i.e. an accepted transcript by an honest verifier. 
    %for $j \in [k]$.

   % \item Denote %$\vec{t}$ as the transcript $(\MSG_1, \cdots, \MSG_m)$  and   $\vec{t}_{\jstar}$ as the transcript output by $\A$, i.e. the $\jstar$-th session transcript $(\MSG_{\jstar, 1}, \cdots, \MSG_{\jstar, m})$ in $\vec{t}$.

    \item Denote $\Aord_{\jstar}[x, \vr, \{H_j\}_{j \in [k]}]$ as the $\jstar$-session's trascript in the output of the same algorithm as $\Aord_{\jstar}[x, \vr, \{H_j\}_{j \neq \jstar}][H_0, \vecone]$ except that all oracles $h_j$ used for $j \in [k]$ are random oracles from the family $\cH_\epsilon$.

      \item Denote $\A_\jstar[x, \vr, H = \{H_j\}_{j \in [k]}]$ as the algorithm that: 
      \begin{enumerate}
      \item guess a random $\jstar \gets [k]$;
          \item runs the simulator $S$ on input $x$ ad $V^k_H$ on input $x, \vr$  without any measure-and-reprogram.

        \item  In the end, $S$ outputs a transcript 
    $(\MSG_{\ell_1}', \cdots \MSG_{\ell_m}')$.
    
          \item  simply outputs the final transcript of the $\jstar$-th session: $(\MSG_{\ell_1, \jstar}', \cdots \MSG_{\ell_m, \jstar}')$. 
      \end{enumerate}

      \item  Denote $\A[x, \vr, H = \{H_j\}_{j \in [k]}]$ as an algorithm same as $\A_\jstar[x, \vr, H = \{H_j\}_{j \in [k]}]$ except that $\A$ outputs the full transcript output by simulator $S$. 

      Note that $\A[x, \vr, H = \{H_j\}_{j \in [k]}]$ also implicitly guesses an index $\jstar \gets [k]$ but does nothing when simulating the interaction between $S$ and $\qVk$.
      %\langle S, V^*_k \rangle
      
      %s the same algorithm as $\Aord[x, \vr, \{h_j\}_{j \neq \jstar}][H_0, \vecone]$ except that all oracles $h_j$ used for $j \in [k]$ are random oracles from the family $\cH_p$.
\end{enumerate}


\subsection{Completeness}
\label{sec:parallel_pqzk_completeness}
Set query number of simulator to be $q = 
O(k^{1/m})$ %for some constant $c$.
%O(\frac{k^{1/m}}{m}) if m overhead is needed

\begin{lemma}
\label{lem:parallel_pqzk_completeness}
For any $\NP$ language $L$, and for any input $x \in L$, there exists a polynomial $\poly(\lambda)$ such that:
$$\Pr_{\vr, \{H_j\}_{j \neq \jstar}}[\Aord[x, \vr, \{H_j\}_{j \neq \jstar}][H_0, \vecone] \in \acc[x, \vr]] \geq \frac{1}{\poly(\lambda)}.$$
%$$\Pr_{\vr, \{H_j\}_{j \neq \jstar}}[\cA[x, \vr,  \{H_j\}_{j \neq \jstar}]^{\Hord_{\jstar}} \in \acc[x, \vr]] \geq \frac{1}{\poly(\lambda)}.$$
\end{lemma}





%Now we before we prove  

%Overall loss on the soundess side:


\jiahui{add the probability of 1. getting a non-trivial accepting transcript among all transcripts 2. guessing a correct session in line 6}

Before we go into the proof for \Cref{lem:parallel_pqzk_completeness}, we analyze the probability of the following event. We denote $\A[x, \vr, H] := \A[x, \vr, H = \{H_j\}_{j \in [k]}] $.
\begin{align*}
   & \Pr[(\A[x, \vr, H] \text{ guesses } j: j = \jstar) \wedge %\langle S, \qVk \rangle
   \A[x, \vr, H] \in \acc^*_k[x, \vr] \wedge (\exists \jstar \in [k] \text{ s.t. $\jstar$-th session does not abort})] \\
    \geq & \frac{1}{k} (1 - (1-\epsilon)^m)^k \\ 
    \geq & \frac{1}{k} (1 - \negl(\lambda))   
    %\langle \rangle
\end{align*}


Now we analyze the correctness, i.e. success probability of  $\Aord_{\jstar}[x, \vr, \{H_j\}_{j \neq\jstar}][H_0, \vecone]$ outputting an accepting transcript by an honest verifier.

\begin{align*}
    & \Pr[\Aord_{\jstar}[x, \vr, \{H_j\}_{j \neq\jstar}][H_0, \vecone] \to \MSG_{\jstar}  \in \acc[x,\vr]]  \\ %\vec{t}_{\jstar} 
   \geq  &  \Pr[\Aord_{\jstar}[x, \vr,  \{H_j\}_{j \neq\jstar} ][H_{\jstar}, \vecone] \in \acc[x,\vr]] - 32 \cdot m^2  k^{2/m}  \epsilon \\
    =  &   \sum_{\MSG_{\jstar} \in \acc[x,r]} \Pr_{\vr,H_{\jstar}}[\Aord_{\jstar}[x, \vr,  \{H_j\}_{j \neq\jstar} ][H_{\jstar}, \vecone] = \MSG_{\jstar} ] - 32  m^2 k^{2/m}  \epsilon\\ 
    \geq & \frac{1}{(4mq + 1)^{2m}} \sum_{\MSG_{\jstar} \in \acc[x,r]}  \Pr_{\vr, H}[\A_{\jstar}[x, \vr,  \{H_j\}_{j \neq\jstar}]^{\Hord_{\jstar, \MSG_{\jstar}, \vecone}} \to \MSG_{\jstar}]  - 32 m^2 k^{2/m} \epsilon\\  
= & \frac{1}{(4mq + 1)^{2m}}  \Pr[\A_{\jstar}[x,\vr]^{\Hord_{\jstar}, \MSG_{\jstar}, \vecone} \to \MSG_{\jstar} \wedge \MSG_{\jstar} \in \acc[x, \vr] ]   - 32  m^2 k^{2/m}  \epsilon          \\
= & \frac{1}{(4mq + 1)^{2m}} \Pr_{\vr, H}[\A_{\jstar}[x, \vr,  \{H_j\}_{j \neq\jstar}, H_{\jstar}] \to \MSG_{\jstar}: \MSG_{\jstar} \in \acc_k^*[x,\vr, H] \wedge  H_{\jstar}(\MSG) = \vecone]  - 32 \cdot m^2  k^{2/m}  \epsilon \\
\geq & \frac{1}{(4mq + 1)^{2m}} \Pr_{\vr, H}[\A[x, \vr,  \{H_j\}_{j \in [k]}]\to \MSG: \MSG \in \acc_k^*[x,\vr, H] \wedge  (\exists \jstar : H_{\jstar}(\vec{\MSG}_i) = \vecone ) \wedge (\A \text{ guesses } \jstar)]  - 32 \cdot  m^2 k^{2/m}  \epsilon \\
   \geq  & \frac{1}{(4mq + 1)^{2m}} \cdot \frac{1}{k}(1 - \negl(\lambda)) - 32 \cdot m^2  k^{2/m} \epsilon \\
   \geq & \frac{1}{\poly(\lambda)}
  %  = & \frac{p^{-m}}{(4q+1)^{2m}}  \sum_{\MSG_{\jstar} = \MSG^* \in \acc[x,\vr]} \Pr_{\vr, H,\vecbeta \gets \cD_p}[\MSG_{\jstar} = \MSG^* \cap \vecbeta = \vecone \cap : \MSG \gets \A[x,\vr]^{\Hord_{\jstar}, \MSG_{\jstar}, \vecbeta}] - 32 k^{2/m}  p  \\
%  = & \frac{p^{-m}}{(4q+1)^{2m}}  \sum_{\MSG = \MSG_{\jstar} \in \acc[x,\vr]} \Pr_{\vr, H}[\MSG_{\jstar} = \msgstar \cap \hatH(\MSG_{\jstar}) = \vecone  :  \MSG \gets \A[x,\vr]^{\Hord_{\jstar}, \MSG_{\jstar}, \vecbeta}] - 32 k^{2/m} p \\
 %  = & \frac{p^{-m}}{(4q+1)^{2m}}  \Pr_{\vr, H}[\MSG \in \acc[x, \vr] \cap \hatH(\MSG_{\jstar}) = \vecone:  \MSG \gets \A[x,\vr]^{\Hord_{\jstar}}] - 32 k^{2/m} p \\   
   %\geq & \frac{1}{32k^2} - \negl(\lambda)
\end{align*}
The last inequality is obtained by setting probability $\epsilon = \frac{1}{96(m)^{m+2} k^{3+2/m}} $
 and since $m = \frac{\log \lambda}{\log \log \lambda}$, 
 The result on the RHS of the above inequality is an inverse polynomial.
 %we have $p = \frac{1}{96 \lambda \cdot m^2 k^{3+2/m}}$ which is an inverse polynomial.
 
\jiahui{bring in the probability that the algorithm guesses correctly the session that has a non-trivial transcript and the final accepting transcript is a non-trivial one.}






\jiahui{ parallel composition tightness result for eps-zk: Simulator running time is still $k^{1/m}$}
\begin{remark}
A simple observation is that our lower bound can extend to $\epsilon$-zero knowledge by taking the round number to constant round. Then the loss in completeness 
is $1/k(4mk^{1/m} + 1)^{2m}(1-\epsilon) - 32m^2k^{2/m}p$, where $\epsilon$ is an inverse polynomial. By setting $p$ properly, we can have a noticeable probability on the completeness side. The soundness side can be argued similarly as the zero knowledge case.

Note that this tightness result in the $\epsilon$-zero knowledge setting does \emph{not} conflict with any $\epsilon$ zero knowledge positive results(i.e. upper bounds) of parallel ZK where the verifier is allowed to run in \emph{any} polynomial time in terms of $1/\epsilon$. 
%measure-and-repgrogram
\end{remark}


\subsection{Soundness}
%Soundness error:Suppose the algorithm $\A$ is not sound with non-negligible error $\epsilon$, then there exists malicious prover $P^*$ that can convince an honest verifier on some $x \notin L$ to accept with probability $\epsilon \cdot  \frac{1}{k^2 \cdot n^{2/\log \log n}}$.

\begin{lemma}
\label{lem:parallel_pq_soundness}
For any $\NP$ language $L$, and for any input $x \in \bits^\lambda \setminus L$:
$$\Pr_{\vr}[\cA[x, \vr]^{\Hord_{\jstar}} \in \acc[x, \vr]] = \negl(\lambda).$$
\end{lemma}

Suppose the algorithm $\A[x, \vr]^{\Hord_{\jstar}}$ outputs an accepting transcript with non-negligible probability $\epsilon$, then we can construct a malicious prover $P^*$ that can convince an honest verifier on some $x \notin L$ to accept with non-negligible probability $\epsilon$.
% \cdot  \frac{1}{(4q+1)^{2m}} (1 - \negl(\lambda))


We describe the malicious prover $\mP$: $\mP$ plays as the verifier $\qVk$ to interact with a simulator;  $\mP$ chooses a random session $\jstar$ and interacts with an external honest verifier $V$; 
$\mP$ is almost the same as $\Aord[x, \vr, \{h_{\jstar}\}][H_0,\vecone]$ except that $\mP$ does not have the randomness $r_{\jstar}$ used by $F[x, r_{\jstar}, \cdot]$ as $\A$ does. 


\jiahui{TODO: describe more in details below}

%$\epsilon \cdot  \frac{1}{k^2 \cdot n^{2/\log \log n}}$.

\jiahui{The following should be the loss on the soundness side:
need to take into account: 1. probability that there exists a session with meaningful/non-trivial transcript $(1-\negl)$, i.e. not abort/accept in the middle; 2. probability that $\cA$ chooses this session, $1/k$}.

\begin{lemma}
For any $\NP$ language $L$, and for any input $x \notin L$, if $\A[x, \vr]^{\Hord_{\jstar}}$ outputs an accepting transcript with non-negligible probability $\epsilon$, then we can construct a $\BQP$ prover $P^*$ such that:

$$\Pr_{r}[\langle P^*, V \rangle (x,r)] \in \acc[x, r]] \geq \epsilon'.$$ 


\begin{proof}
     $P^*$ simulates the interaction between a regular quantum polynomial-time simulator $S$ making at most $q = O(k^{1/m})$ queries and $\qVk = \Vzero(x,r_1, \cdots, r_k, \{H_j\}_{j \in [k], j \neq j^*} \cdot)$. 
    $P^*$ also interacts with an external honest single-session verifier $V$.
    
    To initialize such a verifier, $P^*$ does the following:
    \begin{itemize}
        \item $P^*$ samples a random session index $j^* \in [k]$. 
        %chooses a random session $j^* \in [k]$. 

        %\jiahui{replace with h that outputs 0 all the tim at position $j^*$ and random elsewhere}
        \item $H_{0,}: \cM^{\leq km} \to \{0,1\}$ is a function that outputs $0$ all the time;  
        %at the $j^*$-th output bit and for the output at indices $j \neq \jstar$, $H_0^j(m) = 0$ with probability $1-\epsilon$. 
        
        %Function $H_0^{\jstar}$ is used to determine aborting/non-aborting for
        
        \item $P^*$ samples randomness $\vr = (r_i, \cdots, r_k)$, $r_j \gets \cR$ for each $j \neq \jstar, j \in [k]$.
        
  
         
    \end{itemize}


\begin{enumerate}



\item $\mP$'s algorithm of simulating interaction between $S$ and $\qVk$ is as below.

%then runs algorithm $\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecone]$ . $\vecone = (1, \cdots, 1)$ is a length-$m$ string where all entries are 1's. 

%    The algorithm is similar to  \Cref{lem:measure_and_reprogram_ordered} except that it only performs "measure-and-reprogram" for the oracle queries in session $\jstar$ and simulates the verifier $\qVk$ for each of the sessions $j$  where $j \neq j^*$: using function $H_{j}\gets \cH_{\epsilon}$ and the single-session honest verifier function $F(x, r_j, \cdot)$
    
    We elaborate $\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecbeta]$'
    
    \jiahui{revise the language and details later}

\begin{enumerate}
     \item  Simulate the $\qVk$ oracle for simulator $S$: as discussed in \Cref{sec:quantum_parallel_verifier}, we can view the $\qVk$ as the passing $S$'s query $\MSG$ to the quantum-accessible oracle function $F^*[x, r, H, \MSG] $ defined in \Cref{sec:quantum_parallel_verifier}, which can again be viewed as $k$ separate oracles $ (F_1^*[x, r_1, H_1, \MSG], \cdots, F_{\jstar}^*[x, r_{\jstar}, H_{\jstar}, \MSG], F_k^*[x, r,_k H_k, \MSG])$.
     
     \item Among them, the
     $F_{\jstar}^*[x, r_{\jstar}, H_0]$ oracle machine is simulated with oracle $H_0$ and honest verifier's single-session next-message function
     $F_{\jstar}[x, r_{\jstar}, \cdot]$
     %messages from external honest verifier $V$
     . The oracle $H_0$ %$\cO$ 
     %(for simulating $H_0$) 
     and  $F_{\jstar}^*[x, r_{\jstar}, H_0, \cdot]$
     are initialized to be
oracles that just return 0. 
The rest of the oracles $F_j^*[x, r_j, H_j, \MSG],  j \neq \jstar$
 are simulated as they are defined in \Cref{sec:quantum_parallel_verifier} using oracles $H_j$ respectively.

For the rest of the description, we can assume $S$ is making queries to all oracles $H_0, \{H_j\}_{j \in [k], j \neq \jstar}$ as well as $F^*[x, \vr, H]$. 


   
    
    \item $\mP$ randomly chooses a set of queries and  uniform random bits $T \times \{b_\ell\} \subseteq \{[q] \cup \{\bot\}\}^m \times  \{0,1\}^m$ with $|T| = m$, and satisfying $\ell_i \neq \ell_j$ for all $i \neq j$ unless $\ell_i = \ell_j = \bot$.



    \item When $S^{\qVk}$ makes its $\ell$-th query, the oracle $F^*[x, \vr, H]$ is simulated as follows. 
    %(\ket{\msg_1}, \cdots, \ket{\msg_m})
    If we have $\ell \in T$:
    \begin{itemize}
         \item $\mP$ measures $S^{\qVk}$'s  query register to oracle $H_0$%$F^*_{\jstar}[x, \vr, H_0, \cdot]$ 
        to obtain $\MSG_{\ell}$ (when $S^{\qVk}$ is making a query to the oracle $F^*_{\jstar}[x, r_{\jstar}, H_0, \cdot]$, it will first go through oracle $H_0$ as well).

          
        $\mP$ passes a message $\MSG^{\jstar}$ which is the part of the transcript $\MSG_\ell$ that corresponds to the $\jstar$-th session in the $\ell$-th query and has the format $\MSG^{\jstar} = (\MSG^{\jstar}_1, \cdots, \MSG^{\jstar}_{i_\ell}), i_\ell \leq m$ to the external verifier and gets back verifier message $\msg_{V,\ell}$
        . $\mP$ reprogram the $\jstar$-th session's honest verifier function $F_{\jstar}[x, r_{\jstar}, \MSG_\ell]$ to output $\msg_{V,\ell}$. \footnote{We make sure that the order of the messages measured are consistent with the round of interaction with $V$ by the method of having two $\mathrm{COUNT}$ registers discussed in \red{XXXXX}}\jiahui{add reference section}
        \xiao{Do not use comment macro in footnote environment.}

        
        %Note that we only measure the part of the messag for session $\jstar$; 
        %Note that the following reprogramming is also only for oracle $F^*_{\jstar}[x, \vr, H_0, \cdot]$.  The queries made to the oracles $F_j^*[x, r_{j}, H_{j},\cdot], j \neq \jstar$ used in the other sessions are unmeasured and the oracles $\{H_j\}_{j\neq \jstar}$ are neither measured nor reprogrammed.
        
        \item If $b_\ell = 0$, reprogram $H_0(\MSG_\ell)$ to output 1 \emph{before} answering the $\ell$-th query.
        
        %$F^*_{\jstar}[x, \vr, H_0(\MSG_\ell)]$ to output the single session honest verifier function, on input $x, r_j, \MSG^{\jstar}$: $F[x, \r_{\jstar}, \MSG^{\jstar}_\ell]$ 
        
        
        %where the input $\MSG^{\jstar}$ %\jiahui{only reprogram for session $\jstar$; other sessions can still abort independently!}
        
        \item If $b = 1$, 
        %$F^*_{\jstar}[x, \vr, H_0(\MSG_\ell)]$ to output the single session honest verifier function, on input $x, r_j, \MSG^{\jstar}$: 
        %$F[x, \r_{\jstar}, \MSG^{\jstar}_\ell]$ 
        reprogram $H_0(\MSG_\ell) \to 1$
        \emph{after} answering the $\ell$-th query.

       
    \end{itemize}

    \item If the $\ell$-th query satisfies $\ell \notin T$, do nothing and answer the query using the current oracle.
    
    %\item $\A$ runs an honest classical single-session verifier next-message function $F(x,r_{\jstar}, \cdot)$ with the same random tape $r_{\jstar}$ used by $\Vzero(x,r_1, \cdots, r_k, \cdot)$ in session $j$ and the same input instance $x$.
    %initializes
    \item In the end, $S$ outputs a transcript 
    $(\MSG_{1}', \cdots \MSG_{m}')$.
    
     \item Accordingly, $\mP$ outputs a classical transcript $(\MSG_{1}, \cdots \MSG_{m})$ to $V$, where:
     \begin{itemize}

   % \item for all $j \neq \jstar$: the transcript $(\MSG_{j\neq \jstar, \ell_1}, \cdots, \MSG_{j\neq \jstar, \ell_m}) = (\MSG_{j\neq \jstar, \ell_1}', \cdots, \MSG_{j\neq \jstar, \ell_m}')$ comes from the output of $S$; 
     
 \item %For the $\jstar$'s session: 
 for all $\ell_i \neq \bot$
, $\MSG_{i}$ is the message $\MSG_{\ell_i}$ obtained from the above measuring the $\ell_i$-th query;

 \item for all $\ell_i = \bot, i \in [m]$, the partial transcript $\MSG_{i} = \MSG_{i}' $ comes from the final output of $S$;


     \end{itemize}
The single-session honest verifier $V$ outputs Accept/Reject.

    
\end{enumerate}
\end{enumerate}

It is to observe that $\mP$
is the same algorithm as $\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecbeta]$
except that $\mP$ replaces the output of the single-session honest verifier next-message $F_{\jstar}[x,r_{\jstar}, \cdot]$ with the reply of the external single-session honest verifier $V$. Therefore, we have $\Pr[\mP \text{~convinces~} V] = \Pr[\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecbeta] \in \acc[x, r_{\jstar}]]$. By the soundness of the single-session protocol, we must have that $\Pr[\Aord[x, (\vr, \{H_j\}_{j \neq j^*})][H_0, \vecbeta] \in \acc[x, r_{\jstar}]] = \negl(\lambda)$ when $x \notin L$.



\end{proof}

% \cdot (\frac{1}{32k^{3}} - \negl(\lambda))

%$$\Pr_{\vr, \{H_j\}_{j \neq \jstar}}[\cA[x, \vr,  \{H_j\}_{j \neq \jstar}]^{\Hord_{\jstar}} \in \acc[x, \vr]] \geq \frac{1}{32k^{2}} - \negl(\lambda).$$
\end{lemma}





%\input{efficient_verifier}

==> sections/prelim_measure_reprogram.tex <==
%\section{Preliminaries}

\subsection{Useful Lemmas}
The following lemma will be used throughout the paper.
\begin{lemma}[\cite{zhandry2015secureIBEinqrom}]\label{lem:simulation_QRO}
For any sets $\calX$ and $\calY$ of classical strings and $q$-quantum-query algorithm $\A$, we have
\[
\Pr[\A^{H}=1:H\sample \func(\calX,\calY)]= \Pr[\A^{H}=1:H\sample \mathcal{H}_{2q}]
\]
where  $\mathcal{H}_{2q}$ is a family of $2q$-wise independent hash functions from $\calX$ to $\calY$.
\end{lemma}

The following lemma is used in \cref{sec:quantum_parallel_tightness}.

\xiao{The presentation of the following lemma is not clear at the first glance, in particular, the definition of $H_\epsilon$. I suggest that we use the original version from \cite[Def.\ 1 ]{HRS2016}.}
\begin{lemma}[{\cite[Lemma 3]{HRS2016}}]\label{lem:ind_sparse_and_zero}
Let $\calX$ be a finite set, $\epsilon\in [0,1]$ be a non-negative real number, and 
$\mathcal{H}_\epsilon$ be a distribution over $H:\calX\rightarrow \bits$ such that we have  $\Pr[H(x)=1]=\epsilon$ independently for each $x\in \calX$.
Let $H_0:\calX\rightarrow \bits$ be the function that returns $0$ for all inputs $x\in \calX$. 
Then for any algorithm $\A$ that makes at most $q$ quantum queries, we have 
\begin{align*}
    \left|\Pr\left[\A^{H}=1:H\sample \mathcal{H}_\epsilon\right]
    -
    \Pr\left[\A^{H_0}=1\right]
    \right|\leq 8q^2\epsilon.
\end{align*}
\end{lemma}



\subsection{Measure-and-Reprogram Lemma}

\xiao{I modified this subsection to put the MnR lemma into a clean format that suits our applications.}

We recall the measure-and-reprogram (MnR) lemma developed by \cite{C:DFMS19,C:DonFehMaj20}. In particular, we need the special ``ordered-query'' version of the (MnR) lemma formalized in \cite[Lemma 2.11]{FOCS:CCLY21}. We adapt it with some cosmetic changes to suit our applications.

We first give intuitive explanations for notation, which are taken from \cite{FOCS:CCLY21}.
For a quantumly-accessible classical oracle $\mcal{O}$, we denote by $\mcal{O}\leftarrow \reprogram(\mcal{O},x,y)$ to mean that we reprogram $\oracle$ to output $y$ on input $x$. For a $q$-quantum-query algorithm $\Adv$, function $H:\mcal{X} \rightarrow \mcal{Y}$, and  $\vb{y}=(y_1, \ldots ,y_k)\in \mcal{Y}^k$, we denote by $\Adv[H,\vb{y}]$  to mean an algorithm that runs $\Adv$ w.r.t.\ an oracle that computes $H$ except that randomly chosen $k$ queries are measured and the oracle is reprogrammed to output  $y_i$ on $i$-th measured query. Formal definitions are given below.

\begin{definition}[Reprogramming Oracle \textnormal{\cite[Definition 2.9]{FOCS:CCLY21}}]
\label{MnR:def:reprogram}
Let $\Adv$ be a quantum algorithm with quantumly-accessible oracle $\mcal{O}$ that is initialized to be an oracle that computes some classical function from $\mcal{X}$ to $\mcal{Y}$. At some point in an execution of $\Adv^{\mcal{O}}$, we say that we reprogram $\mcal{O}$ to output $y\in \mcal{Y}$ on $x\in \mcal{X}$ if we update the oracle to compute the function $H_{x,y}$ defined by
\begin{eqnarray*}
    H_{x,y}(x')
    \coloneqq
    \begin{cases} y   &\text{if~}  x'=x \\  
     H(x')  &\text{otherwise}
    \end{cases}
\end{eqnarray*}
where $H$ is the function computed by $\mcal{O}$ before the update. This updated oracle is used in the rest of execution of $\Adv$. We denote by $\mcal{O}\leftarrow \reprogram(\mcal{O},x,y)$ the above reprogramming procedure. 
\end{definition}


% \begin{lemma}(Measure-and-Reprogram Lemma, Rephrasing of \cite[Lemma 4]{DFS2020measure-reprogram2})
% \label{lem:measure_and_reprogram}
% Let $\calX$, $\calY$, and $\calZ$ be sets of classical strings and $k$ be a positive integer. 
% Let $\A$ be a $q$-quantum-query algorithm that is given quantum oracle access to an oracle that computes a function from $\calX$ to $\calY$ and a (possibly quantum) input $\inp$ and outputs $\vecx \in \calX^k$ and $z \in \calZ$.
% For a function $H:\calX \rightarrow \calY$ and $\vecy=(y_1,...,y_k) \in \calY^k$, we define a measure-and-reprogram algorithm $\tilde{\A}[H,\vecy]$ as follows:

% %\qipeng{some comments for the final version: (1) explain the intuition of $\tilde{A}$? (for example, using exact $k$ classical queries to simulate a $q$-quantum query algorithm, which is $\A^\ora$); (2) what is the meaning of `uniformly pick ', for those readers who are not familiar with DFM.  }
% %\takashi{For (1), I added the intuition before Def 2.5. For (2), 
% %I thought that "uniformly pick" is a formal term and  
% %I'm not sure how to make this more rigorous.}


% \begin{description}
% \item $\widetilde{A}[H,\vecy](\inp)$: Given a (possibly quantum) input $\inp$, it works as follows:
% \begin{enumerate}
% %    \item Randomly chooses a function $H:\calX \rightarrow \calY$ and 
% %\item Set $\ora$ to be a quantumly-accessible classical oracle that computes $H$. 
%     \item 
%     For each $i\in [k]$, uniformly pick $(j_i,b_i) \in ([q] \times \bits) \cup \{(\bot,\bot)\}$  conditioned on that there exists at most one $i\in [k]$ such that $j_i=j^*$  for all $j^*\in [q]$. 
%     \item Run $\A^{\ora}(\inp)$ 
%     where  the oracle $\ora$ is initialized to be a quantumly-accessible classical oracle that computes $H$, and when $\A$ makes its $j$-th query, the oracle is simulated as follows:
%     \begin{enumerate}
%       \item If $j=j_i$ for some $i\in[k]$, 
%         measure $\A$'s  query register to obtain $x'_i$, and do either of the following.
%         \begin{enumerate}
%         \item If $b_i=0$, reprogram $\ora\leftarrow \reprogram(\ora,x'_i,y_i)$ and answer $\A$'s $j_i$-th query by using the reprogrammed oracle. 
%         \item If $b_i=1$, answer  $\A$'s $j_i$-th query by using the oracle before the reprogramming and then reprogram $\ora\leftarrow \reprogram(\ora,x'_i,y_i)$.
%         \end{enumerate}
%     \item Otherwise, answer $\A$'s $j$-th query by just using the oracle $\ora$ without any measurement or  reprogramming.
%     \end{enumerate}
%     \item Let $(\vecx=(x_1,...,x_k),z)$ be $\A$'s output.
% \item For all $i\in[k]$ such that $j_i=\bot$, set $x'_i:=x_i$. %and pick $y_i\sample \calY$.
%     \item Output $\vecx':=((x'_1,...,x'_k),z)$.
% \end{enumerate}
% \end{description}

% Then for any $q$-quantum query algorithm $\A$, $\inp$, $H:\calX \rightarrow \calY$, $\vecx^*=(x^*_1,...,x^*_k) \in \calX^k$ such that $x^*_i\neq x^*_{i'}$ for all $i\neq i'$, $\vecy=(y_1,...,y_k) \in \calY^k$, and a relation $R\subseteq \calX^k \times \calY^k \times \calZ$, we have
% \begin{align*}
% &\Pr[ \vecx'=\vecx^* \land (\vecx',\vecy,z)\in R:(\vecx',z)\sample \widetilde{A}{[}H,\vecy{]}(\inp)]\\
%  &~~~~~~~~\geq \frac{1}{(2q+1)^{2k}}\Pr[\vecx=\vecx^* \land (\vecx,\vecy,z)\in R:(\vecx,z)\sample \A^{H_{\vecx^*,\vecy}}(\inp)].
% \end{align*}
% where $H_{\vecx^*,\vecy}:\calX\rightarrow \calY$ is defined as 
% \begin{eqnarray*}
%     H_{\vecx^*,\vecy}(x'):=
%     \begin{cases} y_i   &\text{if~} \,\exists i\in[k] \text{~s.t.~} x'=x^*_i \\  
%      H(x')  &\text{otherwise}
%     \end{cases}.
% \end{eqnarray*}
% \end{lemma}
% \begin{remark}
% The above lemma is a rephrasing of \cite[Lemma 4]{DFS2020measure-reprogram2} (taking \cite[Remark 5]{DFS2020measure-reprogram2} into account) given in \cite[Definition 4.5, Lemma 4.6]{yamakawa-zhandry2021classicalvsquanrum}.\footnote{Note a minor notational difference from \cite{yamakawa-zhandry2021classicalvsquanrum} that the roles of $i$ and $j$ are swapped.}
% \end{remark}




\begin{lemma}[Measure-and-Reprogram Lemma, Ordered Queries]\label{MnR:lem}
Let $\mcal{X}$ and $\mcal{Y}$ be sets of classical strings and $k$ be a positive integer. Let $\Adv$ be a $q$-quantum-query algorithm that is given quantum oracle access to an oracle that computes a function from $\mcal{X}$ to $\mcal{Y}$ and outputs $\vb{x} \in \mcal{X}^k$.
For a function $H:\mcal{X}^{\leq k} \rightarrow \mcal{Y}$ and  $\vb{y} =(y_1,...,y_k) \in \mcal{Y}^k$,  \xiao{Did we define the notation ``$\calX^{\leq k}$''?}
we define an algorithm $\Adv[H,\vb{y}]$ as follows:
%\takashi{I changed the notation from $\experiment{[}\A,H,\vecy{]}$ to $\Aord[H,\vecy]$ for the consistency to \Cref{lem:measure_and_reprogram}.} \qipeng{The current notation looks great.}
\begin{description}
\item $\Aord[H,\vecy]$: 
It  works as follows:
\begin{enumerate}
%    \item Randomly chooses a function $H:\calX \rightarrow \calY$ and 
%\item Set $\ora$ to be a quantumly-accessible classical oracle that computes $H$. 
    \item 
    For each $i\in[k]$, uniformly pick $(j_i,b_i)\in ([q]\times \bits) \cup \{(\bot,\bot)\}$  conditioned on that 
    there exists at most one $i\in [k]$ such that $j_i=j^*$  for all $j^*\in [q]$.
    \item Run $\A^{\ora}$ 
    where  the oracle $\ora$ is initialized to be a quantumly-accessible classical oracle that computes $H$, and when $\A$ makes its $j$-th query, the oracle is simulated as follows:
    \begin{enumerate}
      \item If $j=j_i$ for some $i\in[k]$, 
        measure $\A$'s  query register to obtain $\vecx'_i=(x'_{i,1},...,x'_{i,k_i})$ where $k_i\leq k$ is determined by the measurement outcome, and do either of the following.
        \begin{enumerate}
        \item If $b_i=0$, reprogram $\ora\leftarrow \reprogram(\ora,\vecx'_i,y_i)$ and answer $\A$'s $j_i$-th query by using the reprogrammed oracle. 
        \item If $b_i=1$, answer  $\A$'s $j_i$-th query by using the oracle before the reprogramming and then reprogram $\ora\leftarrow \reprogram(\ora,\vecx'_i,y_i)$. 
        \end{enumerate}
    \item Otherwise, answer $\A$'s $j$-th query by just using the oracle $\ora$ without any measurement or  reprogramming. 
    \end{enumerate}
    \item Let $\vecx=(x_1,...,x_k)$ be $\A$'s output.
     \item For all $i \in [k]$ such that $j_i = \bot$, set $\vecx'_i = \vecx_i$ where $\vecx_i := (x_1, \cdots, x_i)$. 
     \item Output $\vecx'_k$ if for all $i \in [k]$, $\vecx'_i$ is a prefix of $\vecx'_k$, and output $\bot$ otherwise. 
     
     %\qipeng{In Lemma 0.3, it never outputs $\bot$ when it fails.}
   % \item 
%    Set $\vecx'_k:=\vecx$ if $j_k=\bot$, and output $\vecx'_k$ if
 %   $\vecx'_i$ is a prefix of $\vecx'_k$ for all $i$ such that $j_i \neq \bot$.
 %   Otherwise, output $\bot$. 
 %   \takashi{I made a modification on the output of the experiment. In the older version, the experiment outputs $\vecx$, but I found that it should output $\vecx'_k$ if $j_k\neq \bot$. (Recall that the intuitive interpretation of $j_k$ is the guess of the first query that is equal to $\vecx^*=(x^*_1,...,x^*_k)$.)}
    
    %\qipeng{I think this should correspond to step 4 in the previous lemma. Thus, I feel it might be more understandable in the following way (although they might be equivalent): 
    %\begin{itemize}
    %    \item For all $i \in [k]$ such that $j_i = \bot$, set $\vecx'_i = \vecx_i$ where $\vecx_i = (x_1, x_2, \cdots, x_i)$. 
        
    %    \item Output $\vecx'_k$ if for all $i \in [k]$, $\vecx'_i$ is a prefix of $\vecx'_k$. 
    %\end{itemize}
    %}
    %\takashi{I revised these steps accordingly.}
\end{enumerate}
\end{description}
Then for any $q$-quantum query algorithm $\A$, 
$H:\calX^{\leq k}\rightarrow \calY$, 
$\vecx^*=(x^*_1,...,x^*_k) \in \calX^k$, and
$\vecy=(y_1,...,y_k)$, 
we have 
\begin{align*}
\Pr[\Aord[H,\vecy]=\vecx^*]\geq \frac{1}{(2q+1)^{2k}}\Pr\left[\A^{\Hord_{\vecx^*,\vecy}}=\vecx^*\right]
\end{align*}
where $\Hord_{\vecx^*,\vecy}: \calX^{\leq k}\rightarrow \calY$ is defined as 
\begin{eqnarray*}
    \Hord_{\vecx^*,\vecy}(\vecx'):=
    \begin{cases} y_i   &\text{if~} \exists i\in[k] \text{~s.t.~} \vecx'=(x^*_1,...,x^*_i) \\  
     H(\vecx')  &\text{otherwise}
    \end{cases}.
\end{eqnarray*}
%\takashi{I put $\mathsf{ord}$ to differentiate $\Hord_{\vecx^*,\vecy}$ from  $H_{\vecx^*,\vecy}$ in \Cref{lem:measure_and_reprogram}. We may want to think about a better notation later.}
\end{lemma}

\jiahui{maybe we can omit the proof?}

\xiao{I'm not sure if this lemma really holds. We need to check if the output of $\A$ matches the requirement in \Cref{lem:measure_and_reprogram}. In particular, it might be important that the output of $\A$ is a vector from $\calX^k$. }
\begin{proof}
We apply \Cref{lem:measure_and_reprogram} for the following setting, where we append $[\ref{lem:measure_and_reprogram}]$ and $[\ref{lem:measure_and_reprogram_ordered}]$ to characters to distinguish those in \Cref{lem:measure_and_reprogram} and \ref{lem:measure_and_reprogram_ordered}, respectively (e.g., $\calX[\ref{lem:measure_and_reprogram}]$ and $\calX[\ref{lem:measure_and_reprogram_ordered}]$ are $\calX$ in \Cref{lem:measure_and_reprogram} and \ref{lem:measure_and_reprogram_ordered}, respectively).
\begin{itemize}
    \item 
    %$k[\ref{lem:measure_and_reprogram}]:=k[\ref{lem:measure_and_reprogram_ordered}]$, 
    $\calX[\ref{lem:measure_and_reprogram}]:=\calX[\ref{lem:measure_and_reprogram_ordered}]^{\leq k}$, $\calY[\ref{lem:measure_and_reprogram}]:=\calY[\ref{lem:measure_and_reprogram_ordered}]$, $\calZ[\ref{lem:measure_and_reprogram}]:=\emptyset$  
    \item $\inp[\ref{lem:measure_and_reprogram}]$ is a null string and $H[\ref{lem:measure_and_reprogram}]:=H[\ref{lem:measure_and_reprogram_ordered}]$.
    \item 
    $\vecx^*[\ref{lem:measure_and_reprogram}]:=
    (x_1^*[\ref{lem:measure_and_reprogram_ordered}],(x_1^*[\ref{lem:measure_and_reprogram_ordered}],x_2^*[\ref{lem:measure_and_reprogram_ordered}]),...,(x_1^*[\ref{lem:measure_and_reprogram_ordered}],...,x_k^*[\ref{lem:measure_and_reprogram_ordered}]))$.
    %$(x_1^*[\ref{lem:measure_and_reprogram_ordered}],...,x_i^*[\ref{lem:measure_and_reprogram_ordered}])$, 
    \item $\A[\ref{lem:measure_and_reprogram}]$ works similarly to $\A[\ref{lem:measure_and_reprogram_ordered}]$
    except that $\A[\ref{lem:measure_and_reprogram}]$ outputs \[
    (x_1[\ref{lem:measure_and_reprogram}],...,x_k[\ref{lem:measure_and_reprogram}]):=(x_1[\ref{lem:measure_and_reprogram_ordered}],(x_1[\ref{lem:measure_and_reprogram_ordered}],x_2[\ref{lem:measure_and_reprogram_ordered}]),...,(x_1[\ref{lem:measure_and_reprogram_ordered}],...,x_k[\ref{lem:measure_and_reprogram_ordered}]))
    \]
    where $(x_1[\ref{lem:measure_and_reprogram_ordered}],...,x_k[\ref{lem:measure_and_reprogram_ordered}])$ is the output of $\A[\ref{lem:measure_and_reprogram_ordered}]$. 
    \item 
    $R[\ref{lem:measure_and_reprogram}]$ is a trivial relation, i.e., 
    $R[\ref{lem:measure_and_reprogram}]:=\calX[\ref{lem:measure_and_reprogram}]^k\times \calY[\ref{lem:measure_and_reprogram}]^{k}$. 
    
    %\nai{Should it be $R[0.4]$?}
    %\takashi{I meant $R[0,3]$ as $R$ only appears in Lemma 0.3.}
    %\nai{I see. Thanks!}
    
    %\qipeng{Should this be a relation that checks prefix?}
    
    %\takashi{I don't think that's needed.
    %The condition $\vecx'=\vecx^*$ in the l.h.s. of Lemma 0.3 already requires the prefix condition. (Note that we set $\vecx^*:=(x_1^*,(x_1^*,x_2^*),...,(x_1^*,...,x_k^*))$ where $\vecx^*$ in l.h.s. is in Lemma 0.3. and variables in r.h.s. are in Lemma 0.4.)
    %But we may need to improve the readability of this proof. 
    %}
    
    %\qipeng{That makes sense!}
    
    %\takashi{I slightly modified the above third item to emphasize $\vecx^*:=(x_1^*,(x_1^*,x_2^*),...,(x_1^*,...,x_k^*))$.  Hopefully, this helps readers to understand the proof.}
\end{itemize}
Then we have $H_{\vecx^*,\vecy}[\ref{lem:measure_and_reprogram}]=\Hord_{\vecx^*,\vecy}[\ref{lem:measure_and_reprogram_ordered}]$ are defined as the same functions in \cref{lem:measure_and_reprogram,lem:measure_and_reprogram_ordered}, and thus the r.h.s. of the inequalities in \Cref{lem:measure_and_reprogram,lem:measure_and_reprogram_ordered}  are the same probability. 
The l.h.s of the inequality in \Cref{lem:measure_and_reprogram} corresponds to the probability that we have $\vecx'_i = (x^*_1,...,x^*_i)$ for all $i\in [k]$ such that $\vecx'_i$ is defined (i.e., $i=k$ or $j_i\neq \bot$) where the probability is taken over randomness of $\Aord[H,\vecy]$. 
Especially, when this event happens, 
we have $\vecx'_k=\vecx^*$ and 
$\vecx'_i$ is a prefix of $\vecx'_k$ for all $i\in [k]$ such that $j_i\neq \bot$, i.e., $\Aord[H,\vecy]=\vecx^*$.  Therefore,  \Cref{lem:measure_and_reprogram} implies \Cref{lem:measure_and_reprogram_ordered}. 


%$\Pr[\experiment'[\A,H,\vecy]=\vecx^*]$ in \Cref{lem:measure_and_reprogram_ordered} where $\experiment'[\A,H,\vecy]$ is an experiment that works similarly to $\experiment[\A,H,\vecy]$ except that we modify the Step 4 as follows:
%\begin{itemize}
%    \item[4'.] 
%    For all $i\in [k]$ s.t. $j_i=\bot$, set $\vecx'_i:=(x_1,...,x_i)$.
%    Output $\bot$ if there exists $i\in[k]$ s.t. $\vecx'_i \neq (x^*_1,...,x^*_i)$. 
%    Otherwise, output $\vecx'_k$. 
%\end{itemize}
\end{proof}
%\takashi{This is different from what is proven in \cite{C:DonFehMaj20}.
%Especially, instead of considering the probability that $(\vecx,\vecy,z)$  satisfies a relation $R$ (where $z$ is an arbitrary additional output), we only consider the probability to output $\vecx^*$.   
%On the other hand, this does not seem an immediate consequence of any statement in \cite{C:DonFehMaj20} since we require all measured queries to be a prefix of the final output. (In the multi-round Fiat-Shamir, they also do a similar thing, but that is slightly different.)  
%I think we can prove it by an induction based on \cite[Lemma 1]{C:DonFehMaj20}. Probably, there may be a simpler direct proof since the statement is simpler than  those in \cite{C:DonFehMaj20}.}

==> sections/qc_imply_epr.tex <==
\section{QC-Model ZK Implies Non-Reprogrammable EPR(NEPR) Model ZK }
\label{sec:qc_imply_nepr}


\subsection{Definition: Protocol in the Non-Reprogrammable EPR(NEPR) Model}





\subsection{Implication between QC-Protocol and NEPR-Protocol}
We show that if there exists a constant round BBZK protocol with quantum messages, there exists a constant round BBZK protocol in the non-reprogrammable EPR model.

Given a constant round BBZK protocol with quantum messages(QC model):

Suppose the (honest) QC model protocol consists of $k$ quantum messages $(\rho_1, \cdots, \rho_k)$ between the verifier $V_Q$ and prover $P_Q$. Without loss of generality, we assume: each message has $n = n(\lambda)$-qubits (up to padding); there is one $n$-qubit message register $\reg{m}$ which both $V_Q$ and $P_Q$ will operate on. 



\begin{itemize}
    \item Initially, the prover $P_Q$ is initialized with input instance $x$, a witness $w$ and some (quantum) auxiliary information; the verifier $V_Q$ is initialized with input instance $x$ and some (quantum) auxiliary information. They do \emph{not} preshare any entanglement at this time of the protocol.
    
    \item The party that sends the first message operates a unitary $U_1$ on $\ket{0^n}_{\reg{m}} \bra{0^n}_{\reg{m}}, \rho_{\reg{aux}_1}$, where $\reg{aux}_1$ contains the input instance (and a witness if this is the prover) as well as any auxiliary/internal state,
    to obtain $\rho_1$ in register $\reg{m}$.
     It gives register $\reg{m}$ to the other party.    
\jiahui{I think the QC protocol P and V should NOT PRE-share any entanglement, but can possibly generate entanglement through out the protocol. Otherwise, might result in problems in the following reductions}

    \item The receiver of $\rho_1$, operates a unitary $U_2$ on register
     $\reg{m}$ and  $\reg{aux}_2$, where $\reg{aux}_2$ contains the input instance (and a witness if this is the prover) as well as any auxiliary/internal state. \footnote{After this round, $\reg{aux}_2$ can possibly be entangled with the other party's $\reg{aux}$.} 

    \item $\cdots$

    \item The protocol continues until the last message $m_k$ from $P_Q$ to $V_Q$; $V_Q$ uses it to recover the state $\rho_k$ and applies a measurement that outputs 1 for Accept or 0 for Reject. 
\end{itemize}


\paragraph{Transformation of Protocol to NEPR-model} We can transform this protocol into a classical-communication protocol in the NEPR-model in the following way:

\begin{itemize}
\item Let $(P_E, V_E)$ share $k\cdot n$ number of EPR pairs.
The rest of the setup is the same as the protocol in QC model.
%(in addition to any entanglement they already use in the QC-model protocol) 
%\jiahui{I think the QC protocol P and V should NOT PRE-share any entanglement, but can possibly generate entanglement through out the protocol. Otherwise, might result in problems in the following reduction}

    \item For  quantum message $\rho_1$ in the QC-model protocol,  the party which originally sends $\rho_1$ will compute it using the same circuit $U_1$ as the QC-protocol; then performs a teleportation on $\rho_1$ using the first $n$-qubits of EPRs on its side, to obtain measurement outcome $m_1$; send $m_1$ to the other party.

    \item The receiver party of $\rho_1$ in the original protocol will now receive a classical message $m_1$; it uses $m_1$ to recover state $\rho_1$ in the register that holds the first $n$-qubit of EPRs on its side; it then performs the same operation as in the QC-model protocol on $\rho_1$ and its internal state to obtain a state $\rho_2$. Finally, it performs teleportation measurement on the state $\rho_2$ using the second $n$-qubits of EPRs on its own side to obtain classical message $m_2$ and sends $m_2$.

    $\cdots$

    \item Each message $\rho_i$ is now turned into a classical message $m_i$ as above. The protocol continues until the last message $m_k$ from $P_Q$ to $V_Q$; $V_Q$ uses it to recover the state $\rho_k$ and applies a measurement that outputs 1 for Accept or 0 for Reject. 
\end{itemize}

We show that if the following three properties hold for the original QC-model protocol, then it holds for the above NEPR-model protocol:


\paragraph{Completeness}
The completeness is straightforward from the correctness of the QC-model protocol.  Since the quantum message sent from one party to the other is essentially the same in each round and the operation performed is the same.

\paragraph{Soundness}
\jiahui{the following reduction considers that $P,V$ in QC protocol do not PRE-share entanglement}
We show that the soundness of the protocol in QC-model implies the protocol in NEPR-model. Suppose there exists a malicious prover $P^*_E$ in the EPR model that convinces the verifier $V_E$ on some input $x \notin L$, then there exists a malicious prover $P^*_Q$ in the EPR model that convinces the verifier $V_Q$ on this input $x \notin L$.

$P^*_Q$ sets up with an honest verifier $V_Q$ in the QC model protocol. Note that $P^*_Q$ and $V_Q$ do not pre-share any entanglement before the protocol starts.

$P^*_Q$ also plays as an honest verifier in the NEPR protocol, $V_E$ with the malicious $P_E^*$, which it shares $k\cdot n$ number of EPR pairs.

\begin{itemize}
    \item Initially, $P^*_Q$ holds an empty register $\reg{TPstate}$ initialized to $0^n$.

    \item Whenever $P^*_Q$ receives a message from $V_Q$ in register $\reg{m}$, it swaps $\reg{TPstate}$ with register $\reg{m}$. Then, it
uses the EPR pairs it shares with $P_E^*$ to teleport this message in register $\reg{TP}$, sends the measurement outcomes of the teleportation protocol and does nothing else.

\item Whenever it receives a (classical) message from $P^*_E$ in the NEPR protocol, it parses as the correction information for the teleported state and applies them accordingly to the EPR-register $\reg{EPR}_{V,i}$ (which stands for the EPR register for $i$-th round on the verfier side) corresponding to this message in the protocol. It then swaps $\reg{EPR}_{V,i}$ with the message register $\reg{m}$ and sends register $\reg{m}$ to $V_Q$.


\end{itemize}




$P_Q^*$ perfectly simulates an honest verifier $V_E$ for the malicious $P^*_E$. Note that the computation done by the honest $V_E$ and $V_Q$  is exactly the same, except from $V_E$ uses the EPR's to do teleportation, which is performed by $P^*_Q$ here. Therefore, 
 if $V_E$ accepts at the end, then $V_Q$ should also accept.

%Note that $V_Q$ and $P^*_E$ auxiliary/internal states can possibly be entangled after the first round of the protocol


 
\paragraph{Zero-Knowledge}
Now we show the implication of zero knowledge property.

\jiahui{modify the proof for the following lemma. State that if the verifier in the EPR output a view, then the verifier in the QC model outputs the same view, so that the same distinguisher can distinguish}
\begin{lemma}
\label{lem:qczk_imply_eprzk}
Suppose there exists a QPT $V_E^*, D_E$ such that $D$ distinguishes $V_E^*$ 's interaction with any QPT simulator $S_E$ from a QPT prover $P_E$ in the protocol of the NEPR model, then there exists a QPT $V_Q^*, D_Q$ such that distinguishes $V_Q^*$'s interaction with any QPT simulator $S_Q$ from a prover $P_Q$ in the protocol of the QC model.
\end{lemma}

Suppose there exists the above $V_E^*$, we use it to construct a malicious $V_Q^*$: $V_Q^*$ also plays as a simulator $S_E$ in the $NEPR$ model protocol, interacting with $V^*_E$. 


We make notes on a few notations: 


\begin{itemize}

    \item With a slight abuse of notations, we denote the unitary of the malicious verifier in the QC model as $V_Q^* = V_{Q,k}^* \cdots. V_{Q,1}^* $--that is, at each round $i$ of the protocol, the operation performed is $V_{Q,i}^*$.
    Similarly for $V_E^*$.
   
    \item $S_Q$ has black-box access to $V_Q^*, \vqstardagger$. Similarly, $S_E$ has black-box access to $V_E^*, \vestardagger$


    \item We denote the registers that hold the $kn$ EPR pairs shared by $S_E, V_E$ as $\reg{EPR_{S,i}}, \reg{EPR_{V,i}}$, where $i$ denotes that they will use this pair in the $i$-th round of the protocol.

    \item We denote $\tp(m_i)$ as performing the Pauli correction operators on the $i$-th EPR register using the classical message $m_i$ as the Pauli one-time pad information.
\end{itemize}
 

We now describe $V^*_Q$:
\begin{enumerate}
    \item When $S_Q$ calls $V^*_Q$ on message $\rho_i$, $V^*_Q$ implements its operation as follows: 

\begin{itemize}
    \item Suppose $S_Q$ calls $V^*_{Q,i}$:  recall that $\rho$ is put in the communication register $\reg{m}$, $V^*_Q$ first swaps $\reg{m}$ with register $\tp_i$ which is used in the teleportation circuit of the $i$-th message. $V^*_Q$ then performs the measurement on $\reg{EPR}_{V,i}$ to obtain a classical message $m_i$. It writes $m_i$ at the end to the communication register $\commepr$ with $V^*_E$.

    \item $V^*_Q$ then calls $V^*_E$ on the communication register and $V^*_E$'s internal state, to obtain message $m_{i+1}$. $V^*_Q$ then applies $\tp(m_{i+1})$ on register $\reg{EPR}_{V,i+1}$.

    \item Finally it swaps $\reg{EPR}_{V,i+1}$ with register $\reg{m}$ in the QC protocol to answer $S_Q$'s query.
\end{itemize}

    \item When $S_Q$ calls $\vqstardagger$, it implements this operation as follows: (Note that this operation is exactly the inverse of the above $V^*_Q$) 
\begin{itemize}
    \item Suppose $S_Q$ calls $V^{*\dagger}_{Q,i}$ and now the communication register $\reg{m}$ in QC protocol holds an arbitrary state $\rho_{i+1}'$: first swap register $\reg{m}$ with register $\reg{EPR_{V,i+1}}$.

    \item Apply $\tp(m_i)^\dagger$ on register $\reg{EPR_{V,i+1}}$ since the communication register $\commepr$ in the NEPR-protocol contains only classical information $m_1, m_2, \cdots, m_{i+1}$. 
    Then apply $V^{*\dagger}_{E,i}$ (which acts on the communication register $\commepr$ and its own internal state register).

\end{itemize}

\item Whenever $V_E^*$ aborts, $V_Q^*$ will abort.

\item At the end, $V_E^*$ outputs its internal state $\rho_{V}$. $V_Q^*$ will pass this state on as its own output.
    
\end{enumerate}

%For any simulator strategy in the QC model, $V^*_Q$ converts it into a valid simulator strategy in the NEPR model. Since $V^*_E$ can distinguish any valid simulator strategy from a prover in the NEPR model with probability $\epsilon$, $V^*_Q$ can any valid simulator strategy from a prover in the QC model with the same probability $\epsilon$.



